A computer assisted proof of the symmetries of least energy nodal solutions on squares

In this article, we prove that the least energy nodal solutions to Lane-Emden equation $-{\Delta}u = |u|^{p-2}u$ with zero Dirichlet boundary conditions on a square are odd with respect to one diagonal and even with respect to the other one when $p$ is close to 2. We also show that this symmetry breaks on rectangles close to squares.

==> d2entropy-S.tex <==
\draw[fill] (0.695398, 0.317916) rectangle (0.785398, 0.340413);


==> d2entropy-singular.tex <==
\draw[fill] (0.695398, 0.394246) rectangle (0.785398, 3);% ymax=inf


==> entropy3D.tex <==
\begin{pgfscope}
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{0,0,0}{0.785398163397}{1.320796326795}{0.785398163397}{1.383296326795}
  \meshline{0,0,0}{0.785398163397}{1.102046326795}{0.785398163397}{1.133296326795}
  \meshline{0,0,0}{0.785398163397}{1.508296326795}{0.785398163397}{1.570796326795}
  \meshline{0,0,0}{0.722898163397}{1.570796326795}{0.660398163397}{1.570796326795}
  \meshline{0,0,0}{0.785398163397}{1.570796326795}{0.722898163397}{1.570796326795}
  \meshline{0,0,0}{0.660398163397}{1.570796326795}{0.580199081699}{1.570796326795}
  \meshline{0,0,0}{0.785398163397}{1.445796326795}{0.785398163397}{1.508296326795}
  \meshline{0,0,0}{0.785398163397}{1.383296326795}{0.785398163397}{1.445796326795}
  \meshline{0,0,0}{0.785398163397}{1.289546326795}{0.785398163397}{1.320796326795}
  \meshline{0,0,0}{0.580199081699}{1.570796326795}{0.500000000000}{1.570796326795}
  \meshline{0,0,0}{0.437500000000}{1.570796326795}{0.375000000000}{1.570796326795}
  \meshline{0,0,0}{0.500000000000}{1.570796326795}{0.437500000000}{1.570796326795}
  \meshline{0,0,0}{0.375000000000}{1.570796326795}{0.312500000000}{1.570796326795}
  \meshline{0,0,0}{0.312500000000}{1.570796326795}{0.250000000000}{1.570796326795}
  \meshline{0,0,0}{0.000000000000}{1.249723392973}{0.000000000000}{1.214048622548}
  \meshline{0,0,0}{0.000000000000}{1.445796326795}{0.000000000000}{1.365597245096}
  \meshline{0,0,0}{0.000000000000}{1.325497704247}{0.000000000000}{1.285398163397}
  \meshline{0,0,0}{0.785398163397}{1.195796326795}{0.785398163397}{1.258296326795}
  \meshline{0,0,0}{0.785398163397}{0.999446785946}{0.785398163397}{1.035121556370}
  \meshline{0,0,0}{0.785398163397}{1.086421326795}{0.785398163397}{1.102046326795}
  \meshline{0,0,0}{0.785398163397}{1.035121556370}{0.785398163397}{1.070796326795}
  \meshline{0,0,0}{0.785398163397}{1.070796326795}{0.785398163397}{1.086421326795}
  \meshline{0,0,0}{0.785398163397}{0.963772015521}{0.785398163397}{0.999446785946}
  \meshline{0,0,0}{0.785398163397}{0.441786466911}{0.785398163397}{0.490873852123}
  \meshline{0,0,0}{0.785398163397}{0.892422474671}{0.785398163397}{0.928097245096}
  \meshline{0,0,0}{0.785398163397}{0.928097245096}{0.785398163397}{0.963772015521}
  \meshline{0,0,0}{0.785398163397}{0.785398163397}{0.785398163397}{0.803235548610}
  \meshline{0,0,0}{0.785398163397}{0.638136007760}{0.785398163397}{0.687223392973}
  \meshline{0,0,0}{0.785398163397}{0.838910319034}{0.785398163397}{0.856747704247}
  \meshline{0,0,0}{0.785398163397}{0.821072933822}{0.785398163397}{0.838910319034}
  \meshline{0,0,0}{0.785398163397}{0.856747704247}{0.785398163397}{0.892422474671}
  \meshline{0,0,0}{0.785398163397}{0.803235548610}{0.785398163397}{0.821072933822}
  \meshline{0,0,0}{0.785398163397}{0.736310778185}{0.785398163397}{0.760854470791}
  \meshline{0,0,0}{0.785398163397}{0.687223392973}{0.785398163397}{0.736310778185}
  \meshline{0,0,0}{0.785398163397}{0.760854470791}{0.785398163397}{0.785398163397}
  \meshline{0,0,0}{0.785398163397}{1.133296326795}{0.785398163397}{1.195796326795}
  \meshline{0,0,0}{0.785398163397}{0.589048622548}{0.785398163397}{0.638136007760}
  \meshline{0,0,0}{0.785398163397}{0.490873852123}{0.785398163397}{0.539961237336}
  \meshline{0,0,0}{0.785398163397}{0.539961237336}{0.785398163397}{0.589048622548}
  \meshline{0,0,0}{0.785398163397}{0.392699081699}{0.785398163397}{0.441786466911}
  \meshline{0,0,0}{0.785398163397}{0.343611696486}{0.785398163397}{0.392699081699}
  \meshline{0,0,0}{0.000000000000}{0.687500000000}{0.000000000000}{0.625000000000}
  \meshline{0,0,0}{0.250000000000}{1.570796326795}{0.187500000000}{1.570796326795}
  \meshline{0,0,0}{0.785398163397}{1.258296326795}{0.785398163397}{1.289546326795}
  \meshline{0,0,0}{0.187500000000}{1.570796326795}{0.156250000000}{1.570796326795}
  \meshline{0,0,0}{0.000000000000}{1.365597245096}{0.000000000000}{1.325497704247}
  \meshline{0,0,0}{0.000000000000}{1.570796326795}{0.000000000000}{1.508296326795}
  \meshline{0,0,0}{0.156250000000}{1.570796326795}{0.125000000000}{1.570796326795}
  \meshline{0,0,0}{0.125000000000}{1.570796326795}{0.062500000000}{1.570796326795}
  \meshline{0,0,0}{0.062500000000}{1.570796326795}{0.000000000000}{1.570796326795}
  \meshline{0,0,0}{0.000000000000}{1.508296326795}{0.000000000000}{1.445796326795}
  \meshline{0,0,0}{0.000000000000}{1.285398163397}{0.000000000000}{1.249723392973}
  \meshline{0,0,0}{0.000000000000}{1.142699081699}{0.000000000000}{1.071349540849}
  \meshline{0,0,0}{0.000000000000}{1.071349540849}{0.000000000000}{1.000000000000}
  \meshline{0,0,0}{0.000000000000}{1.214048622548}{0.000000000000}{1.142699081699}
  \meshline{0,0,0}{0.000000000000}{0.750000000000}{0.000000000000}{0.687500000000}
  \meshline{0,0,0}{0.000000000000}{0.812500000000}{0.000000000000}{0.750000000000}
  \meshline{0,0,0}{0.000000000000}{1.000000000000}{0.000000000000}{0.937500000000}
  \meshline{0,0,0}{0.000000000000}{0.937500000000}{0.000000000000}{0.875000000000}
  \meshline{0,0,0}{0.000000000000}{0.875000000000}{0.000000000000}{0.812500000000}
  \meshline{0,0,0}{0.000000000000}{0.437500000000}{0.000000000000}{0.375000000000}
  \meshline{0,0,0}{0.000000000000}{0.375000000000}{0.000000000000}{0.312500000000}
  \meshline{0,0,0}{0.000000000000}{0.187500000000}{0.000000000000}{0.125000000000}
  \meshline{0,0,0}{0.000000000000}{0.250000000000}{0.000000000000}{0.187500000000}
  \meshline{0,0,0}{0.000000000000}{0.000000000000}{0.049087385212}{0.000000000000}
  \meshline{0,0,0}{0.147262155637}{0.000000000000}{0.196349540849}{0.000000000000}
  \meshline{0,0,0}{0.196349540849}{0.000000000000}{0.245436926062}{0.000000000000}
  \meshline{0,0,0}{0.343611696486}{0.000000000000}{0.392699081699}{0.000000000000}
  \meshline{0,0,0}{0.294524311274}{0.000000000000}{0.343611696486}{0.000000000000}
  \meshline{0,0,0}{0.245436926062}{0.000000000000}{0.294524311274}{0.000000000000}
  \meshline{0,0,0}{0.392699081699}{0.000000000000}{0.441786466911}{0.000000000000}
  \meshline{0,0,0}{0.441786466911}{0.000000000000}{0.490873852123}{0.000000000000}
  \meshline{0,0,0}{0.785398163397}{0.294524311274}{0.785398163397}{0.343611696486}
  \meshline{0,0,0}{0.785398163397}{0.049087385212}{0.785398163397}{0.098174770425}
  \meshline{0,0,0}{0.785398163397}{0.196349540849}{0.785398163397}{0.245436926062}
  \meshline{0,0,0}{0.539961237336}{0.000000000000}{0.589048622548}{0.000000000000}
  \meshline{0,0,0}{0.490873852123}{0.000000000000}{0.539961237336}{0.000000000000}
  \meshline{0,0,0}{0.785398163397}{0.098174770425}{0.785398163397}{0.147262155637}
  \meshline{0,0,0}{0.736310778185}{0.000000000000}{0.785398163397}{0.000000000000}
  \meshline{0,0,0}{0.785398163397}{0.000000000000}{0.785398163397}{0.049087385212}
  \meshline{0,0,0}{0.785398163397}{0.147262155637}{0.785398163397}{0.196349540849}
  \meshline{0,0,0}{0.638136007760}{0.000000000000}{0.687223392973}{0.000000000000}
  \meshline{0,0,0}{0.687223392973}{0.000000000000}{0.736310778185}{0.000000000000}
  \meshline{0,0,0}{0.589048622548}{0.000000000000}{0.638136007760}{0.000000000000}
  \meshline{0,0,0}{0.000000000000}{0.562500000000}{0.000000000000}{0.500000000000}
  \meshline{0,0,0}{0.000000000000}{0.625000000000}{0.000000000000}{0.562500000000}
  \meshline{0,0,0}{0.000000000000}{0.500000000000}{0.000000000000}{0.437500000000}
  \meshline{0,0,0}{0.000000000000}{0.312500000000}{0.000000000000}{0.250000000000}
  \meshline{0,0,0}{0.000000000000}{0.125000000000}{0.000000000000}{0.062500000000}
  \meshline{0,0,0}{0.049087385212}{0.000000000000}{0.098174770425}{0.000000000000}
  \meshline{0,0,0}{0.000000000000}{0.062500000000}{0.000000000000}{0.000000000000}
  \meshline{0,0,0}{0.098174770425}{0.000000000000}{0.147262155637}{0.000000000000}
  \meshline{0,0,0}{0.785398163397}{0.245436926062}{0.785398163397}{0.294524311274}
  \meshline{170,255,0}{0.667081020413}{1.474912954956}{0.674215371672}{1.522113535070}
  \meshline{0,0,0}{0.655275270170}{0.893782127577}{0.654225366444}{0.896476107665}
  \meshline{170,255,0}{0.531699426920}{1.210033645326}{0.557280306440}{1.246976269921}
  \meshline{0,0,0}{0.597211957376}{0.803953688962}{0.570928327438}{0.815532788264}
  \meshline{0,0,0}{0.781550190158}{1.105652573815}{0.785398163397}{1.106583071035}
  \meshline{0,0,0}{0.758257603117}{1.127481941481}{0.783625283061}{1.133616224178}
  \meshline{170,255,0}{0.667081020413}{1.474912954956}{0.658359890990}{1.445699432846}
  \meshline{0,255,0}{0.558806808575}{1.444701545820}{0.567334833917}{1.482635005281}
  \meshline{170,255,0}{0.674551682608}{1.526322559721}{0.681191019032}{1.570796326795}
  \meshline{0,170,255}{0.263029518062}{1.233111285192}{0.261896326900}{1.232100079374}
  \meshline{170,255,0}{0.636142517509}{1.393135971300}{0.651241586546}{1.425072725647}
  \meshline{0,255,170}{0.495828079163}{1.518863524637}{0.496718678940}{1.524489740016}
  \meshline{170,255,0}{0.674536513656}{1.523470033922}{0.674551682608}{1.526322559721}
  \meshline{170,255,0}{0.630960180517}{1.377742729047}{0.628332571580}{1.371380866526}
  \meshline{170,255,0}{0.658359890990}{1.445699432846}{0.651241586546}{1.425072725647}
  \meshline{170,255,0}{0.605462447709}{1.326086059066}{0.628332571580}{1.371380866526}
  \meshline{0,0,0}{0.734122629704}{1.192050057750}{0.765032031910}{1.202601593246}
  \meshline{170,255,0}{0.630960180517}{1.377742729047}{0.636142517509}{1.393135971300}
  \meshline{0,255,170}{0.474767287616}{1.423913695379}{0.468433661595}{1.405203170960}
  \meshline{255,170,0}{0.659779590664}{1.205714054792}{0.672711147206}{1.220033520889}
  \meshline{255,170,0}{0.659779590664}{1.205714054792}{0.657063065728}{1.201760061309}
  \meshline{0,0,0}{0.769581392463}{1.102046326795}{0.735909612593}{1.092908269832}
  \meshline{170,255,0}{0.602445254160}{1.319173820367}{0.605462447709}{1.326086059066}
  \meshline{255,170,0}{0.685298155599}{1.232700033313}{0.690570635637}{1.237507020157}
  \meshline{0,0,0}{0.722500340036}{1.185667797711}{0.718524583201}{1.182043049837}
  \meshline{0,0,0}{0.723369568616}{1.208573140177}{0.709448218042}{1.195880868496}
  \meshline{0,0,0}{0.724238797196}{1.231478482643}{0.700371852884}{1.209718687155}
  \meshline{0,255,0}{0.542455010995}{1.395803019729}{0.546194939340}{1.406427431997}
  \meshline{0,0,255}{0.357864467331}{1.523735949954}{0.358315907979}{1.530194604416}
  \meshline{255,170,0}{0.785398163397}{1.293559304821}{0.778688065626}{1.290335693495}
  \meshline{255,170,0}{0.722284193960}{1.267443984737}{0.751812562423}{1.278157239398}
  \meshline{255,0,170}{0.154199378195}{1.446340670167}{0.157579708255}{1.451228594340}
  \meshline{255,170,0}{0.685298155599}{1.232700033313}{0.672711147206}{1.220033520889}
  \meshline{0,0,0}{0.718524583201}{1.182043049837}{0.715576213933}{1.179076057619}
  \meshline{0,0,0}{0.709448218042}{1.195880868496}{0.699124326542}{1.185491767619}
  \meshline{0,0,0}{0.700371852884}{1.209718687155}{0.682672439152}{1.191907477619}
  \meshline{255,170,0}{0.722284193960}{1.267443984737}{0.690570635637}{1.237507020157}
  \meshline{0,255,170}{0.490758392054}{1.481344131286}{0.483961272759}{1.453997973058}
  \meshline{255,170,0}{0.616879700040}{1.154125505065}{0.621737418793}{1.159522124079}
  \meshline{0,0,0}{0.675200610307}{1.147105651555}{0.659457711490}{1.129616284341}
  \meshline{0,0,0}{0.647826801774}{1.136311395826}{0.672486475253}{1.163706737044}
  \meshline{0,0,0}{0.636195892057}{1.143006507311}{0.653413358198}{1.162134025777}
  \meshline{0,255,0}{0.538934772255}{1.388300752571}{0.520021650266}{1.343134329955}
  \meshline{0,255,0}{0.514529445547}{1.332696757012}{0.520021650266}{1.343134329955}
  \meshline{0,255,170}{0.474767287616}{1.423913695379}{0.483961272759}{1.453997973058}
  \meshline{0,255,170}{0.449037105637}{1.360928543120}{0.458917751745}{1.382054103267}
  \meshline{170,255,0}{0.602445254160}{1.319173820367}{0.598257280067}{1.311880209514}
  \meshline{0,255,0}{0.538934772255}{1.388300752571}{0.542455010995}{1.395803019729}
  \meshline{0,170,255}{0.374867857123}{1.364368113342}{0.380083883598}{1.373520391097}
  \meshline{0,255,0}{0.456582142163}{1.241159438888}{0.471160505661}{1.259998470536}
  \meshline{0,255,170}{0.458917751745}{1.382054103267}{0.468433661595}{1.405203170960}
  \meshline{0,255,170}{0.441006203620}{1.345009706445}{0.449037105637}{1.360928543120}
  \meshline{170,255,0}{0.598257280067}{1.311880209514}{0.579721672926}{1.278409292252}
  \meshline{170,255,0}{0.561304117774}{1.252861316246}{0.579721672926}{1.278409292252}
  \meshline{170,255,0}{0.561304117774}{1.252861316246}{0.559044394215}{1.249341850695}
  \meshline{0,255,0}{0.546194939340}{1.406427431997}{0.558806808575}{1.444701545820}
  \meshline{0,170,255}{0.390063580590}{1.394698303654}{0.398994263305}{1.413875799838}
  \meshline{0,170,255}{0.414108242194}{1.459204875709}{0.415758876130}{1.464015007206}
  \meshline{0,170,255}{0.425107969701}{1.509491896582}{0.428879660275}{1.556710678046}
  \meshline{0,170,255}{0.415758876130}{1.464015007206}{0.416931173389}{1.469059950961}
  \meshline{0,255,170}{0.496718678940}{1.524489740016}{0.498473421562}{1.561223312915}
  \meshline{0,255,0}{0.575021583498}{1.565279316580}{0.575494603570}{1.570796326795}
  \meshline{170,255,0}{0.674536513656}{1.523470033922}{0.674215371672}{1.522113535070}
  \meshline{0,255,0}{0.574943897383}{1.528426393026}{0.575021583498}{1.565279316580}
  \meshline{0,255,0}{0.567334833917}{1.482635005281}{0.569656211215}{1.498407012158}
  \meshline{0,255,0}{0.569656211215}{1.498407012158}{0.574943897383}{1.528426393026}
  \meshline{0,170,255}{0.429756959346}{1.570796326795}{0.428879660275}{1.556710678046}
  \meshline{0,255,170}{0.495828079163}{1.518863524637}{0.490758392054}{1.481344131286}
  \meshline{0,255,170}{0.498473421562}{1.561223312915}{0.498994089642}{1.570796326795}
  \meshline{0,255,170}{0.261160224826}{1.149242590499}{0.220539398102}{1.125825247268}
  \meshline{0,170,255}{0.414108242194}{1.459204875709}{0.398994263305}{1.413875799838}
  \meshline{170,0,255}{0.284186635789}{1.530678530717}{0.271261059869}{1.481605767289}
  \meshline{0,0,255}{0.345319272142}{1.467759817274}{0.341453080389}{1.456000430167}
  \meshline{0,170,255}{0.425107969701}{1.509491896582}{0.416931173389}{1.469059950961}
  \meshline{0,0,255}{0.357864467331}{1.523735949954}{0.355559497481}{1.513348105020}
  \meshline{170,0,255}{0.284186635789}{1.530678530717}{0.285090539400}{1.538631501986}
  \meshline{0,0,255}{0.355559497481}{1.513348105020}{0.345319272142}{1.467759817274}
  \meshline{0,0,255}{0.322056381646}{1.409643283158}{0.341453080389}{1.456000430167}
  \meshline{0,0,255}{0.358315907979}{1.530194604416}{0.360653133992}{1.570796326795}
  \meshline{170,0,255}{0.204694292371}{1.369507751682}{0.204699994130}{1.369514767643}
  \meshline{0,0,255}{0.291318930374}{1.359154896344}{0.317165960283}{1.400455595841}
  \meshline{170,0,255}{0.286228492161}{1.570796326795}{0.285090539400}{1.538631501986}
  \meshline{170,0,255}{0.264600356979}{1.461489117541}{0.251796142404}{1.434911451154}
  \meshline{255,0,170}{0.124872976638}{1.419080155208}{0.144899253140}{1.436818562636}
  \meshline{170,0,255}{0.264600356979}{1.461489117541}{0.271261059869}{1.481605767289}
  \meshline{0,0,255}{0.317165960283}{1.400455595841}{0.322056381646}{1.409643283158}
  \meshline{170,0,255}{0.204699994130}{1.369514767643}{0.244940808329}{1.421812529858}
  \meshline{0,170,255}{0.333245767767}{1.304170423480}{0.354752803065}{1.331740363330}
  \meshline{0,255,170}{0.294773615786}{1.172777308150}{0.322633930877}{1.196426841323}
  \meshline{0,170,255}{0.380083883598}{1.373520391097}{0.390063580590}{1.394698303654}
  \meshline{0,170,255}{0.354752803065}{1.331740363330}{0.374867857123}{1.364368113342}
  \meshline{0,0,255}{0.257903676560}{1.319703223490}{0.282611311928}{1.348325511556}
  \meshline{170,0,255}{0.251796142404}{1.434911451154}{0.244940808329}{1.421812529858}
  \meshline{255,0,170}{0.000000000000}{1.373435515642}{0.008778234110}{1.373715503820}
  \meshline{170,0,255}{0.170884461592}{1.340940520269}{0.204689047613}{1.369503032247}
  \meshline{170,0,255}{0.170884461592}{1.340940520269}{0.140538165168}{1.321042679425}
  \meshline{0,0,255}{0.291318930374}{1.359154896344}{0.282611311928}{1.348325511556}
  \meshline{0,0,255}{0.219638292004}{1.285417852556}{0.209215154376}{1.278235531622}
  \meshline{170,0,255}{0.204689047613}{1.369503032247}{0.204694292371}{1.369507751682}
  \meshline{170,0,255}{0.091137174654}{1.299782268960}{0.131208307351}{1.316093169293}
  \meshline{0,255,170}{0.145821547158}{1.094749398646}{0.121365844192}{1.088114884465}
  \meshline{0,255,0}{0.240012184892}{1.054727848093}{0.205047237003}{1.037616250882}
  \meshline{255,0,170}{0.086781907674}{1.392429943532}{0.089423572989}{1.393910918077}
  \meshline{0,0,255}{0.124678283965}{1.232947010066}{0.117656784755}{1.229805569269}
  \meshline{170,0,255}{0.140538165168}{1.321042679425}{0.131208307351}{1.316093169293}
  \meshline{255,0,170}{0.157579708255}{1.451228594340}{0.178460709550}{1.486090028062}
  \meshline{255,0,170}{0.154199378195}{1.446340670167}{0.144899253140}{1.436818562636}
  \meshline{0,0,0}{0.704349230027}{1.171183614381}{0.715576213933}{1.179076057619}
  \meshline{0,0,0}{0.678227315068}{1.170801403912}{0.699124326542}{1.185491767619}
  \meshline{0,0,0}{0.670688209145}{1.183482698901}{0.682672439152}{1.191907477619}
  \meshline{0,0,0}{0.752575197469}{1.152041877709}{0.739781136069}{1.147788934824}
  \meshline{0,0,0}{0.774172225342}{1.180831660403}{0.728765184177}{1.165737661196}
  \meshline{0,0,0}{0.785398163397}{1.207012240938}{0.765032031910}{1.202601593246}
  \meshline{0,0,0}{0.759378650501}{1.224733565118}{0.785398163397}{1.230368553019}
  \meshline{0,0,0}{0.781139062493}{1.252802481112}{0.785398163397}{1.253724865099}
  \meshline{0,0,0}{0.722500340036}{1.185667797711}{0.734122629704}{1.192050057750}
  \meshline{0,0,0}{0.723369568616}{1.208573140177}{0.740719197548}{1.218100509274}
  \meshline{0,0,0}{0.724238797196}{1.231478482643}{0.729903942239}{1.234589438388}
  \meshline{170,255,0}{0.559044394215}{1.249341850695}{0.557280306440}{1.246976269921}
  \meshline{0,0,0}{0.614846415897}{1.002561424640}{0.605801073493}{0.989564482134}
  \meshline{0,0,0}{0.593654289786}{1.006026720033}{0.595059802723}{1.008046253404}
  \meshline{255,170,0}{0.643823496504}{1.186816626075}{0.657063065728}{1.201760061309}
  \meshline{0,0,0}{0.721512301513}{1.110713715128}{0.735694365729}{1.120683547050}
  \meshline{0,0,0}{0.710224607360}{1.126068279923}{0.735683195216}{1.143965381362}
  \meshline{0,0,0}{0.698936913207}{1.141422844717}{0.714221298291}{1.152167595834}
  \meshline{0,0,0}{0.687649219054}{1.156777409512}{0.692759401366}{1.160369810305}
  \meshline{0,0,0}{0.695832765038}{1.065222777795}{0.683255470598}{1.054254096291}
  \meshline{255,170,0}{0.621737418793}{1.159522124079}{0.643823496504}{1.186816626075}
  \meshline{0,0,0}{0.672486475253}{1.163706737044}{0.678227315068}{1.170801403912}
  \meshline{0,0,0}{0.653413358198}{1.162134025777}{0.670688209145}{1.183482698901}
  \meshline{0,0,0}{0.721512301513}{1.110713715128}{0.716137086428}{1.106537523208}
  \meshline{0,0,0}{0.710224607360}{1.126068279923}{0.695327021160}{1.114493826038}
  \meshline{0,0,0}{0.698936913207}{1.141422844717}{0.674516955893}{1.122450128869}
  \meshline{0,0,0}{0.687649219054}{1.156777409512}{0.675200610307}{1.147105651555}
  \meshline{255,170,0}{0.616879700040}{1.154125505065}{0.609470573274}{1.146720764493}
  \meshline{0,0,0}{0.659457711490}{1.129616284341}{0.649783571115}{1.119947871045}
  \meshline{0,0,0}{0.647826801774}{1.136311395826}{0.622711311126}{1.111210773516}
  \meshline{0,0,0}{0.636195892057}{1.143006507311}{0.609935337320}{1.116761498788}
  \meshline{0,0,0}{0.769581392463}{1.102046326795}{0.781550190158}{1.105652573815}
  \meshline{0,0,0}{0.735694365729}{1.120683547050}{0.758257603117}{1.127481941481}
  \meshline{0,0,0}{0.664026526616}{1.090496761646}{0.661178735205}{1.087147682963}
  \meshline{0,0,0}{0.666005462398}{1.115924645472}{0.646438949715}{1.092913904494}
  \meshline{0,0,0}{0.649783571115}{1.119947871045}{0.631699164226}{1.098680126026}
  \meshline{0,0,0}{0.622711311126}{1.111210773516}{0.616959378737}{1.104446347557}
  \meshline{170,255,0}{0.501152142747}{1.169376678536}{0.492267915600}{1.159276900486}
  \meshline{170,255,0}{0.525326832241}{1.202223506591}{0.531699426920}{1.210033645326}
  \meshline{0,0,0}{0.516377531055}{0.981576708619}{0.510024471983}{0.973154604520}
  \meshline{0,0,0}{0.492392623017}{0.974902749316}{0.499279635815}{0.984032703572}
  \meshline{0,0,0}{0.633717535483}{1.056769383413}{0.636483248705}{1.060272507958}
  \meshline{0,0,0}{0.617286778652}{1.061323972259}{0.628103095244}{1.075024201132}
  \meshline{0,0,0}{0.600856021822}{1.065878561106}{0.603467928421}{1.069186870169}
  \meshline{170,255,0}{0.501152142747}{1.169376678536}{0.525326832241}{1.202223506591}
  \meshline{0,255,0}{0.426986966527}{1.202820367912}{0.435111207904}{1.212241140023}
  \meshline{0,0,0}{0.549364624712}{1.024726791961}{0.532773983551}{1.003071798047}
  \meshline{0,0,0}{0.525397532631}{1.015408486742}{0.533127434515}{1.025497968916}
  \meshline{255,170,0}{0.589369899889}{1.120931767883}{0.609470573274}{1.146720764493}
  \meshline{0,0,0}{0.605047525048}{1.110490476335}{0.609935337320}{1.116761498788}
  \meshline{255,170,0}{0.589369899889}{1.120931767883}{0.562741205621}{1.091480334960}
  \meshline{0,0,0}{0.605047525048}{1.110490476335}{0.597448211742}{1.102085608119}
  \meshline{0,0,0}{0.597448211742}{1.102085608119}{0.575387875417}{1.076256094926}
  \meshline{0,0,0}{0.659489417358}{1.085623100483}{0.661178735205}{1.087147682963}
  \meshline{0,0,0}{0.634832039550}{1.082438852732}{0.646438949715}{1.092913904494}
  \meshline{0,0,0}{0.620480244058}{1.088555229064}{0.631699164226}{1.098680126026}
  \meshline{0,0,0}{0.613391085307}{1.101226019507}{0.616959378737}{1.104446347557}
  \meshline{0,0,0}{0.516009747393}{1.004336428717}{0.509729811446}{0.996732081383}
  \meshline{0,0,0}{0.587159170370}{1.070501059257}{0.577150334094}{1.058647146235}
  \meshline{0,0,0}{0.636483248705}{1.060272507958}{0.643074129583}{1.068221250668}
  \meshline{0,0,0}{0.628103095244}{1.075024201132}{0.631620994507}{1.079266862567}
  \meshline{0,0,0}{0.620480244058}{1.088555229064}{0.603467928421}{1.069186870169}
  \meshline{0,0,0}{0.606093504170}{1.092917793070}{0.613391085307}{1.101226019507}
  \meshline{0,0,0}{0.679527401961}{1.050358793647}{0.678663527227}{1.049361787162}
  \meshline{0,0,0}{0.670871193051}{1.069928882486}{0.663425111335}{1.061335284984}
  \meshline{0,0,0}{0.655097433748}{1.081284535114}{0.648186695443}{1.073308782806}
  \meshline{0,0,0}{0.687020273808}{1.085242684015}{0.680439920135}{1.079926844310}
  \meshline{0,0,0}{0.664026526616}{1.090496761646}{0.678477711982}{1.102170934307}
  \meshline{0,0,0}{0.666005462398}{1.115924645472}{0.669935150156}{1.119099184600}
  \meshline{0,0,0}{0.678663527227}{1.049361787162}{0.677631348082}{1.048334662092}
  \meshline{0,0,0}{0.663425111335}{1.061335284984}{0.654528346616}{1.052482083349}
  \meshline{0,0,0}{0.648186695443}{1.073308782806}{0.643074129583}{1.068221250668}
  \meshline{0,0,0}{0.659489417358}{1.085623100483}{0.655097433748}{1.081284535114}
  \meshline{0,0,0}{0.634832039550}{1.082438852732}{0.631620994507}{1.079266862567}
  \meshline{0,0,0}{0.610852034078}{0.904493965649}{0.612944130559}{0.892677650239}
  \meshline{0,0,0}{0.650959456744}{0.962425110347}{0.653606291288}{0.969779583324}
  \meshline{0,0,0}{0.584043592537}{0.990804244261}{0.573086181847}{0.973911642923}
  \meshline{0,0,0}{0.633717535483}{1.056769383413}{0.630239096110}{1.052864322151}
  \meshline{0,0,0}{0.617286778652}{1.061323972259}{0.603683090027}{1.046051825249}
  \meshline{0,0,0}{0.600856021822}{1.065878561106}{0.598236898634}{1.062938209011}
  \meshline{0,0,0}{0.664105372291}{0.991783796483}{0.667004045591}{0.996147810736}
  \meshline{0,0,0}{0.584043592537}{0.990804244261}{0.593654289786}{1.006026720033}
  \meshline{0,0,0}{0.619398299177}{1.008897968683}{0.614846415897}{1.002561424640}
  \meshline{0,0,0}{0.595059802723}{1.008046253404}{0.603114325969}{1.019258720454}
  \meshline{0,0,0}{0.754757449322}{1.070534913948}{0.769293381398}{1.073153221930}
  \meshline{0,0,0}{0.576410113792}{1.035513178039}{0.586296415386}{1.047760147690}
  \meshline{0,0,0}{0.569895504904}{1.049516027638}{0.572701530863}{1.052992081290}
  \meshline{0,0,0}{0.673828277501}{1.044552996381}{0.677631348082}{1.048334662092}
  \meshline{0,0,0}{0.648179939045}{1.046169406601}{0.654528346616}{1.052482083349}
  \meshline{0,0,0}{0.576410113792}{1.035513178039}{0.569830210882}{1.027598472826}
  \meshline{0,0,0}{0.569895504904}{1.049516027638}{0.550687900330}{1.026411959062}
  \meshline{0,0,0}{0.606093504170}{1.092917793070}{0.587159170370}{1.070501059257}
  \meshline{0,0,0}{0.572351107157}{1.072689092584}{0.575387875417}{1.076256094926}
  \meshline{0,0,0}{0.567603276390}{0.999097704913}{0.566652124036}{0.997776313923}
  \meshline{0,0,0}{0.569830210882}{1.027598472826}{0.558543557534}{1.011918459029}
  \meshline{0,0,0}{0.550687900330}{1.026411959062}{0.550434991033}{1.026060604136}
  \meshline{0,0,0}{0.608715947310}{1.026699675145}{0.608147274754}{1.025968266769}
  \meshline{0,0,0}{0.598811622637}{1.040129818862}{0.588983027570}{1.027488595567}
  \meshline{0,0,0}{0.566652124036}{0.997776313923}{0.566347659311}{0.997396912266}
  \meshline{0,0,0}{0.558543557534}{1.011918459029}{0.547488542928}{0.998142508885}
  \meshline{0,0,0}{0.549364624712}{1.024726791961}{0.550434991033}{1.026060604136}
  \meshline{0,0,0}{0.546241360328}{0.966761993040}{0.545362929132}{0.965377491405}
  \meshline{0,0,0}{0.532904309180}{0.978131959057}{0.527682594835}{0.969901978057}
  \meshline{0,0,0}{0.608147274754}{1.025968266769}{0.603114325969}{1.019258720454}
  \meshline{0,0,0}{0.588983027570}{1.027488595567}{0.584419270799}{1.021404540526}
  \meshline{0,0,0}{0.567603276390}{0.999097704913}{0.584419270799}{1.021404540526}
  \meshline{0,0,0}{0.608715947310}{1.026699675145}{0.617727356600}{1.036635920881}
  \meshline{0,0,0}{0.598811622637}{1.040129818862}{0.600851230638}{1.042378750816}
  \meshline{0,0,0}{0.586296415386}{1.047760147690}{0.598236898634}{1.062938209011}
  \meshline{0,0,0}{0.572701530863}{1.052992081290}{0.577150334094}{1.058647146235}
  \meshline{0,0,0}{0.561274588869}{1.059215312634}{0.552628925742}{1.049191600635}
  \meshline{0,0,0}{0.530877415683}{0.937601121841}{0.530189524054}{0.936485123441}
  \meshline{0,0,0}{0.522591707696}{0.960140062258}{0.515255179403}{0.948237673153}
  \meshline{0,0,0}{0.663339574836}{1.032234479426}{0.673828277501}{1.044552996381}
  \meshline{170,255,0}{0.425954184681}{1.089603627511}{0.418209760529}{1.082586363523}
  \meshline{0,0,0}{0.516377531055}{0.981576708619}{0.527498805255}{0.996850194261}
  \meshline{0,0,0}{0.565667940664}{0.996454803526}{0.566347659311}{0.997396912266}
  \meshline{0,0,0}{0.542980104758}{0.991893689587}{0.547488542928}{0.998142508885}
  \meshline{0,0,0}{0.616301718781}{0.958085218865}{0.624780288131}{0.977010177495}
  \meshline{0,0,0}{0.559802930712}{0.948121046692}{0.569899136044}{0.969040460735}
  \meshline{0,0,0}{0.573086181847}{0.973911642923}{0.571512291339}{0.971466394559}
  \meshline{0,0,0}{0.556062125480}{0.981530891259}{0.565667940664}{0.996454803526}
  \meshline{255,170,0}{0.496669485483}{1.014462583107}{0.490373225651}{1.007134086207}
  \meshline{255,170,0}{0.476584025754}{0.991105731724}{0.468017784681}{0.980945588620}
  \meshline{0,0,0}{0.572351107157}{1.072689092584}{0.561274588869}{1.059215312634}
  \meshline{255,170,0}{0.545627276003}{1.071129579563}{0.544588724550}{1.070010170110}
  \meshline{0,0,0}{0.532904309180}{0.978131959057}{0.542980104758}{0.991893689587}
  \meshline{0,0,0}{0.571512291339}{0.971466394559}{0.569899136044}{0.969040460735}
  \meshline{0,0,0}{0.556062125480}{0.981530891259}{0.546241360328}{0.966761993040}
  \meshline{0,0,0}{0.532773983551}{1.003071798047}{0.527498805255}{0.996850194261}
  \meshline{0,0,0}{0.516009747393}{1.004336428717}{0.525397532631}{1.015408486742}
  \meshline{0,0,0}{0.499279635815}{0.984032703572}{0.509729811446}{0.996732081383}
  \meshline{0,0,0}{0.541200185218}{1.035067509003}{0.533127434515}{1.025497968916}
  \meshline{0,0,0}{0.552628925742}{1.049191600635}{0.541200185218}{1.035067509003}
  \meshline{255,170,0}{0.521788162093}{1.043107832124}{0.529001040759}{1.051654700157}
  \meshline{255,170,0}{0.496669485483}{1.014462583107}{0.507104208992}{1.026544207072}
  \meshline{255,170,0}{0.521788162093}{1.043107832124}{0.507104208992}{1.026544207072}
  \meshline{255,170,0}{0.545627276003}{1.071129579563}{0.560547839057}{1.088800117969}
  \meshline{255,170,0}{0.529001040759}{1.051654700157}{0.542123081034}{1.067335422078}
  \meshline{255,170,0}{0.561458291067}{1.089948445117}{0.560547839057}{1.088800117969}
  \meshline{0,0,0}{0.649369712148}{1.014908988514}{0.654733963499}{1.022091876349}
  \meshline{0,0,0}{0.634456949266}{1.030181829749}{0.635707539325}{1.031856406038}
  \meshline{0,0,0}{0.695832765038}{1.065222777795}{0.702204807809}{1.070533939524}
  \meshline{170,255,0}{0.240029093088}{0.664495838378}{0.233498095343}{0.664225113929}
  \meshline{255,170,0}{0.562741205621}{1.091480334960}{0.561458291067}{1.089948445117}
  \meshline{0,0,0}{0.634708954628}{0.992799735750}{0.643929419106}{1.007712616949}
  \meshline{0,0,0}{0.663339574836}{1.032234479426}{0.654733963499}{1.022091876349}
  \meshline{0,0,0}{0.745408776336}{1.067063181286}{0.731390104557}{1.059549817142}
  \meshline{0,0,0}{0.683255470598}{1.054254096291}{0.679527401961}{1.050358793647}
  \meshline{0,0,0}{0.670871193051}{1.069928882486}{0.680439920135}{1.079926844310}
  \meshline{255,170,0}{0.432910563427}{0.940054895185}{0.449633038861}{0.960008370804}
  \meshline{0,0,0}{0.635707539325}{1.031856406038}{0.648179939045}{1.046169406601}
  \meshline{0,0,0}{0.673249185673}{1.004798351334}{0.667004045591}{0.996147810736}
  \meshline{0,0,0}{0.617727356600}{1.036635920881}{0.630239096110}{1.052864322151}
  \meshline{0,0,0}{0.600851230638}{1.042378750816}{0.603683090027}{1.046051825249}
  \meshline{0,0,0}{0.632238938461}{1.027247864655}{0.619398299177}{1.008897968683}
  \meshline{0,0,0}{0.648445754012}{0.957258098397}{0.645033986634}{0.946802902719}
  \meshline{0,0,0}{0.649369712148}{1.014908988514}{0.643929419106}{1.007712616949}
  \meshline{0,0,0}{0.632238938461}{1.027247864655}{0.634456949266}{1.030181829749}
  \meshline{0,0,0}{0.612944130559}{0.892677650239}{0.617536769287}{0.885858693451}
  \meshline{0,0,0}{0.626764718828}{0.980541023388}{0.634708954628}{0.992799735750}
  \meshline{0,0,0}{0.625684678830}{0.978653202206}{0.624780288131}{0.977010177495}
  \meshline{0,0,0}{0.597780918086}{0.975202359928}{0.602774209933}{0.984273773315}
  \meshline{0,0,0}{0.597780918086}{0.975202359928}{0.591281099979}{0.962957363788}
  \meshline{0,0,0}{0.643799205882}{0.921545705826}{0.654225366444}{0.896476107665}
  \meshline{0,0,0}{0.687645799661}{0.939668749631}{0.689107148453}{0.955431189000}
  \meshline{0,0,0}{0.625684678830}{0.978653202206}{0.626764718828}{0.980541023388}
  \meshline{0,0,0}{0.602774209933}{0.984273773315}{0.605801073493}{0.989564482134}
  \meshline{0,0,0}{0.650959456744}{0.962425110347}{0.648445754012}{0.957258098397}
  \meshline{0,0,0}{0.581724235267}{0.940179302826}{0.584482082490}{0.945686679586}
  \meshline{0,0,0}{0.584482082490}{0.945686679586}{0.591281099979}{0.962957363788}
  \meshline{0,0,0}{0.653606291288}{0.969779583324}{0.664105372291}{0.991783796483}
  \meshline{0,0,0}{0.673249185673}{1.004798351334}{0.682972620650}{1.017447563152}
  \meshline{0,0,0}{0.705377863643}{1.040649442822}{0.685696765958}{1.020272516400}
  \meshline{0,0,0}{0.612020586615}{0.940985074452}{0.609719274904}{0.934758726098}
  \meshline{0,0,0}{0.698563689911}{0.979722261488}{0.691111449631}{0.964187849359}
  \meshline{0,0,0}{0.685696765958}{1.020272516400}{0.682972620650}{1.017447563152}
  \meshline{0,0,0}{0.644409192986}{0.941206746006}{0.643799205882}{0.921545705826}
  \meshline{0,0,0}{0.708941965878}{1.043004926949}{0.705377863643}{1.040649442822}
  \meshline{0,0,0}{0.719083714735}{1.083152862552}{0.735909612593}{1.092908269832}
  \meshline{0,0,0}{0.753633668429}{1.031137963306}{0.744154846207}{1.026764516338}
  \meshline{0,0,0}{0.708941965878}{1.043004926949}{0.716083754333}{1.048400152197}
  \meshline{0,0,0}{0.782450488986}{1.038176289249}{0.785398163397}{1.038353318638}
  \meshline{0,0,0}{0.716083754333}{1.048400152197}{0.731390104557}{1.059549817142}
  \meshline{0,0,0}{0.769293381398}{1.073153221930}{0.785398163397}{1.076128399420}
  \meshline{0,0,0}{0.745408776336}{1.067063181286}{0.754757449322}{1.070534913948}
  \meshline{0,0,0}{0.753633668429}{1.031137963306}{0.774030536646}{1.036022947735}
  \meshline{0,0,0}{0.782450488986}{1.038176289249}{0.774030536646}{1.036022947735}
  \meshline{0,0,0}{0.719352321518}{1.007001933026}{0.730116853025}{1.016958210408}
  \meshline{0,0,0}{0.719352321518}{1.007001933026}{0.712547633836}{0.999673747569}
  \meshline{0,0,0}{0.691111449631}{0.964187849359}{0.689107148453}{0.955431189000}
  \meshline{0,0,0}{0.704285303324}{0.989138041616}{0.712547633836}{0.999673747569}
  \meshline{0,0,0}{0.730116853025}{1.016958210408}{0.744154846207}{1.026764516338}
  \meshline{0,0,0}{0.714069137926}{1.080493730721}{0.702204807809}{1.070533939524}
  \meshline{0,0,0}{0.687020273808}{1.085242684015}{0.700872811173}{1.095277770367}
  \meshline{0,0,0}{0.678477711982}{1.102170934307}{0.686493894523}{1.107978035338}
  \meshline{0,0,0}{0.669935150156}{1.119099184600}{0.672114977873}{1.120678300309}
  \meshline{0,0,0}{0.719083714735}{1.083152862552}{0.714069137926}{1.080493730721}
  \meshline{0,0,0}{0.700872811173}{1.095277770367}{0.716137086428}{1.106537523208}
  \meshline{0,0,0}{0.686493894523}{1.107978035338}{0.695327021160}{1.114493826038}
  \meshline{0,0,0}{0.672114977873}{1.120678300309}{0.674516955893}{1.122450128869}
  \meshline{255,170,0}{0.476584025754}{0.991105731724}{0.484809499260}{1.001138292059}
  \meshline{0,0,0}{0.459914398672}{0.930357129809}{0.470020243396}{0.942860286309}
  \meshline{255,170,0}{0.490373225651}{1.007134086207}{0.484809499260}{1.001138292059}
  \meshline{0,0,0}{0.691207185518}{0.929287599439}{0.697496548143}{0.912223584891}
  \meshline{0,0,0}{0.698563689911}{0.979722261488}{0.704285303324}{0.989138041616}
  \meshline{0,0,0}{0.687645799661}{0.939668749631}{0.691207185518}{0.929287599439}
  \meshline{0,0,0}{0.644409192986}{0.941206746006}{0.645033986634}{0.946802902719}
  \meshline{0,0,0}{0.489994929249}{0.942634933358}{0.500144165684}{0.959553491635}
  \meshline{0,0,0}{0.475020260193}{0.950222522911}{0.480119786208}{0.958723322811}
  \meshline{0,0,0}{0.612020586615}{0.940985074452}{0.616301718781}{0.958085218865}
  \meshline{0,0,0}{0.608064727301}{0.925787548216}{0.610852034078}{0.904493965649}
  \meshline{255,170,0}{0.468017784681}{0.980945588620}{0.455376292375}{0.965943655658}
  \meshline{255,170,0}{0.432638646656}{0.939745836894}{0.432910563427}{0.940054895185}
  \meshline{0,0,0}{0.548988622350}{0.920467279175}{0.556084008792}{0.941112089755}
  \meshline{0,0,0}{0.641261694125}{0.860678342049}{0.645371495933}{0.858480720844}
  \meshline{0,0,0}{0.609719274904}{0.934758726098}{0.608064727301}{0.925787548216}
  \meshline{0,0,0}{0.548988622350}{0.920467279175}{0.548544581473}{0.918700906786}
  \meshline{0,0,0}{0.619727415424}{0.797313493167}{0.599726475278}{0.803159873102}
  \meshline{170,255,0}{0.334268626540}{1.012179758356}{0.309277389897}{0.994449102306}
  \meshline{0,255,0}{0.280841600955}{1.076726867911}{0.306003303243}{1.094541098932}
  \meshline{255,170,0}{0.408951038322}{0.908585577170}{0.420774288775}{0.924096744175}
  \meshline{0,0,0}{0.471812239501}{0.910955921781}{0.470635234388}{0.908937176086}
  \meshline{0,0,0}{0.459431494542}{0.929366279591}{0.451530076033}{0.915814125538}
  \meshline{255,170,0}{0.455376292375}{0.965943655658}{0.449633038861}{0.960008370804}
  \meshline{255,170,0}{0.432461174824}{0.939545711551}{0.432638646656}{0.939745836894}
  \meshline{0,255,170}{0.782891390756}{0.489241218316}{0.785398163397}{0.489242253933}
  \meshline{0,0,0}{0.493703191914}{0.904792795277}{0.489168926952}{0.888652488998}
  \meshline{0,0,0}{0.510024471983}{0.973154604520}{0.500474802780}{0.959984445824}
  \meshline{0,0,0}{0.492392623017}{0.974902749316}{0.489976450380}{0.971570552525}
  \meshline{255,170,0}{0.395971435476}{0.885462742032}{0.398089848482}{0.891321552313}
  \meshline{0,0,0}{0.441034094597}{0.896102511900}{0.434933752015}{0.882613349511}
  \meshline{0,0,0}{0.559802930712}{0.948121046692}{0.556084008792}{0.941112089755}
  \meshline{0,0,0}{0.530877415683}{0.937601121841}{0.545362929132}{0.965377491405}
  \meshline{0,0,0}{0.522591707696}{0.960140062258}{0.527682594835}{0.969901978057}
  \meshline{0,0,0}{0.501672509110}{0.925095002684}{0.498221681457}{0.913337107248}
  \meshline{0,0,0}{0.480230112392}{0.928174939602}{0.480174694326}{0.927986115389}
  \meshline{0,0,0}{0.529488613920}{0.935469490474}{0.528259746805}{0.932923785647}
  \meshline{0,0,0}{0.505150398442}{0.931958660192}{0.507779805652}{0.937405705317}
  \meshline{0,0,0}{0.479376836368}{0.926477392786}{0.471812239501}{0.910955921781}
  \meshline{0,0,0}{0.459914398672}{0.930357129809}{0.459431494542}{0.929366279591}
  \meshline{255,170,0}{0.420774288775}{0.924096744175}{0.432461174824}{0.939545711551}
  \meshline{0,0,0}{0.446884244652}{0.905620151577}{0.441034094597}{0.896102511900}
  \meshline{0,0,0}{0.498221681457}{0.913337107248}{0.493703191914}{0.904792795277}
  \meshline{0,0,0}{0.480174694326}{0.927986115389}{0.479376836368}{0.926477392786}
  \meshline{0,0,0}{0.489994929249}{0.942634933358}{0.480393490057}{0.928497367440}
  \meshline{0,0,0}{0.470020243396}{0.942860286309}{0.475020260193}{0.950222522911}
  \meshline{0,0,0}{0.500144165684}{0.959553491635}{0.500474802780}{0.959984445824}
  \meshline{0,0,0}{0.480119786208}{0.958723322811}{0.489976450380}{0.971570552525}
  \meshline{0,0,0}{0.530189524054}{0.936485123441}{0.529488613920}{0.935469490474}
  \meshline{0,0,0}{0.515255179403}{0.948237673153}{0.507779805652}{0.937405705317}
  \meshline{0,0,0}{0.467393173483}{0.901823382720}{0.462777507163}{0.887310270838}
  \meshline{0,0,0}{0.576486415606}{0.918438286978}{0.577924278826}{0.925813279456}
  \meshline{0,0,0}{0.555296463753}{0.861818300142}{0.551807468303}{0.870118965973}
  \meshline{0,0,0}{0.581169390348}{0.881180028210}{0.578383339511}{0.890969658017}
  \meshline{0,0,0}{0.581724235267}{0.940179302826}{0.577924278826}{0.925813279456}
  \meshline{0,0,0}{0.577426936057}{0.909316394725}{0.578383339511}{0.890969658017}
  \meshline{0,0,0}{0.528259746805}{0.932923785647}{0.522480728512}{0.913685966464}
  \meshline{0,0,0}{0.501672509110}{0.925095002684}{0.505150398442}{0.931958660192}
  \meshline{0,0,0}{0.480230112392}{0.928174939602}{0.480393490057}{0.928497367440}
  \meshline{0,0,0}{0.522480728512}{0.913685966464}{0.518260739464}{0.901375958208}
  \meshline{0,0,0}{0.680693352435}{0.873109817322}{0.668043554737}{0.881411166375}
  \meshline{0,0,0}{0.462777507163}{0.887310270838}{0.461315906298}{0.874275510176}
  \meshline{0,0,0}{0.470635234388}{0.908937176086}{0.467393173483}{0.901823382720}
  \meshline{0,0,0}{0.446884244652}{0.905620151577}{0.451530076033}{0.915814125538}
  \meshline{0,0,0}{0.490057975623}{0.859459092959}{0.491158463675}{0.857291338884}
  \meshline{0,0,0}{0.535155051153}{0.809508664656}{0.539037990697}{0.807900135601}
  \meshline{0,0,0}{0.541250191107}{0.785314468940}{0.538250709235}{0.786557020797}
  \meshline{0,0,0}{0.461315906298}{0.874275510176}{0.459449170817}{0.864725162110}
  \meshline{0,0,0}{0.489914170528}{0.861316940040}{0.488558697785}{0.880859067061}
  \meshline{0,0,0}{0.516169931241}{0.795767723220}{0.494661366341}{0.808317399274}
  \meshline{0,0,0}{0.494942926628}{0.784098334397}{0.493864196931}{0.784727744510}
  \meshline{0,0,0}{0.750461670443}{0.883816973276}{0.736996607420}{0.888149909700}
  \meshline{0,0,0}{0.711669513091}{0.899711001031}{0.719338472459}{0.894097776223}
  \meshline{0,0,0}{0.687743486212}{0.869033630098}{0.680693352435}{0.873109817322}
  \meshline{0,0,0}{0.775369228745}{0.880614911792}{0.763405168086}{0.881600532633}
  \meshline{0,0,0}{0.629738934597}{0.836873791711}{0.651974903769}{0.828292924284}
  \meshline{0,255,170}{0.322633930877}{1.196426841323}{0.330657501745}{1.202784947437}
  \meshline{170,255,0}{0.334268626540}{1.012179758356}{0.364758763095}{1.035932987027}
  \meshline{0,0,0}{0.645371495933}{0.858480720844}{0.663622137903}{0.849159034291}
  \meshline{0,0,0}{0.576486415606}{0.918438286978}{0.577426936057}{0.909316394725}
  \meshline{0,0,0}{0.546415699063}{0.888406862351}{0.551807468303}{0.870118965973}
  \meshline{0,0,0}{0.625080701429}{0.873955141941}{0.637082116857}{0.863545653022}
  \meshline{0,0,0}{0.561753443699}{0.819930098785}{0.570928327438}{0.815532788264}
  \meshline{0,0,0}{0.622803940963}{0.839991822373}{0.608242575461}{0.849471852648}
  \meshline{0,0,0}{0.581169390348}{0.881180028210}{0.587359465123}{0.870525020704}
  \meshline{0,0,0}{0.546415699063}{0.888406862351}{0.545879177151}{0.898863584935}
  \meshline{0,0,0}{0.567704085577}{0.847215285457}{0.555296463753}{0.861818300142}
  \meshline{0,0,0}{0.617536769287}{0.885858693451}{0.625080701429}{0.873955141941}
  \meshline{0,0,0}{0.651974903769}{0.828292924284}{0.667235265723}{0.822943214232}
  \meshline{0,0,0}{0.637082116857}{0.863545653022}{0.641261694125}{0.860678342049}
  \meshline{0,0,0}{0.541920341385}{0.833847947535}{0.549049878912}{0.828581440354}
  \meshline{0,0,0}{0.622803940963}{0.839991822373}{0.627362592320}{0.837760134566}
  \meshline{0,0,0}{0.625642632188}{0.815107520198}{0.621365699057}{0.817201292845}
  \meshline{0,0,0}{0.591675954360}{0.863955014420}{0.587359465123}{0.870525020704}
  \meshline{0,0,0}{0.621365699057}{0.817201292845}{0.592304710414}{0.829270612879}
  \meshline{0,0,0}{0.518547465246}{0.894241090332}{0.517322624572}{0.877266577661}
  \meshline{0,0,0}{0.567704085577}{0.847215285457}{0.570752007547}{0.843865868478}
  \meshline{0,0,0}{0.608242575461}{0.849471852648}{0.591675954360}{0.863955014420}
  \meshline{0,0,0}{0.573083921125}{0.842277763897}{0.570752007547}{0.843865868478}
  \meshline{0,0,0}{0.548544581473}{0.918700906786}{0.545879177151}{0.898863584935}
  \meshline{0,0,0}{0.518547465246}{0.894241090332}{0.518260739464}{0.901375958208}
  \meshline{0,0,0}{0.488558697785}{0.880859067061}{0.489168926952}{0.888652488998}
  \meshline{0,0,0}{0.521090319211}{0.863060329552}{0.517322624572}{0.877266577661}
  \meshline{0,0,0}{0.499510609945}{0.839699942725}{0.503848556537}{0.834035028263}
  \meshline{0,0,0}{0.541920341385}{0.833847947535}{0.532127585208}{0.844471243700}
  \meshline{0,0,0}{0.521090319211}{0.863060329552}{0.524459166082}{0.855009205963}
  \meshline{0,0,0}{0.499510609945}{0.839699942725}{0.491158463675}{0.857291338884}
  \meshline{0,0,0}{0.524459166082}{0.855009205963}{0.532127585208}{0.844471243700}
  \meshline{0,0,0}{0.489914170528}{0.861316940040}{0.489936853491}{0.860015349434}
  \meshline{0,0,0}{0.512583131622}{0.825385595973}{0.503848556537}{0.834035028263}
  \meshline{170,255,0}{0.226876420926}{0.948081827648}{0.217480368895}{0.943885399866}
  \meshline{0,0,0}{0.459933734009}{0.859060710553}{0.463979862436}{0.842432798679}
  \meshline{0,0,0}{0.459933734009}{0.859060710553}{0.459449170817}{0.864725162110}
  \meshline{0,0,0}{0.489936853491}{0.860015349434}{0.490057975623}{0.859459092959}
  \meshline{0,0,255}{0.211341877611}{0.360274085516}{0.163736984137}{0.360745083970}
  \meshline{0,0,0}{0.463979862436}{0.842432798679}{0.464630657689}{0.841512378248}
  \meshline{0,0,0}{0.450420852835}{0.818233891393}{0.457248453478}{0.808577608399}
  \meshline{0,0,0}{0.538250709235}{0.786557020797}{0.517517121753}{0.795251384088}
  \meshline{0,0,0}{0.434162607841}{0.835414220838}{0.431745229750}{0.850152150386}
  \meshline{255,170,0}{0.415534785326}{0.787641464333}{0.404338262719}{0.796714509569}
  \meshline{0,0,0}{0.431745229750}{0.850152150386}{0.430577276385}{0.863672966225}
  \meshline{0,0,0}{0.450420852835}{0.818233891393}{0.434162607841}{0.835414220838}
  \meshline{0,0,0}{0.671830257871}{0.786676694007}{0.655737250122}{0.788876557386}
  \meshline{0,0,0}{0.670006548544}{0.771531148826}{0.665326883942}{0.772170844211}
  \meshline{0,0,0}{0.519244937519}{0.821530223664}{0.535155051153}{0.809508664656}
  \meshline{0,0,0}{0.571080213963}{0.794451366502}{0.562642775853}{0.796865109701}
  \meshline{0,0,0}{0.570224580262}{0.776993361152}{0.541427952997}{0.785231366847}
  \meshline{0,0,0}{0.519244937519}{0.821530223664}{0.512583131622}{0.825385595973}
  \meshline{0,0,0}{0.539037990697}{0.807900135601}{0.562642775853}{0.796865109701}
  \meshline{0,0,0}{0.541250191107}{0.785314468940}{0.541427952997}{0.785231366847}
  \meshline{255,170,0}{0.437151664141}{0.775403042139}{0.434724657872}{0.777068566295}
  \meshline{0,0,0}{0.510406772922}{0.778171489682}{0.520955940055}{0.774179185108}
  \meshline{0,0,0}{0.544070115319}{0.767826361825}{0.557103594195}{0.763864703187}
  \meshline{0,0,0}{0.590364874951}{0.830102820153}{0.590756784127}{0.829929578393}
  \meshline{0,255,0}{0.715812198911}{0.556265907379}{0.696765368609}{0.556616956347}
  \meshline{0,0,0}{0.493104420077}{0.809083945149}{0.494661366341}{0.808317399274}
  \meshline{0,0,0}{0.493864196931}{0.784727744510}{0.490006820381}{0.786626882684}
  \meshline{255,170,0}{0.499155828317}{0.754106092813}{0.514678505922}{0.749604391181}
  \meshline{0,0,0}{0.464630657689}{0.841512378248}{0.465168823263}{0.841008681669}
  \meshline{0,0,0}{0.457248453478}{0.808577608399}{0.468845216171}{0.797723607380}
  \meshline{0,0,0}{0.490006820381}{0.786626882684}{0.477177952299}{0.793623062955}
  \meshline{255,170,0}{0.479001765194}{0.759393702938}{0.480973916562}{0.758918386658}
  \meshline{255,170,0}{0.557745873932}{0.740763992547}{0.562703390113}{0.739680216964}
  \meshline{0,0,0}{0.465168823263}{0.841008681669}{0.493104420077}{0.809083945149}
  \meshline{255,170,0}{0.459044225935}{0.766701919704}{0.455941628384}{0.768337522708}
  \meshline{0,0,0}{0.468845216171}{0.797723607380}{0.475114170022}{0.794418789535}
  \meshline{0,0,0}{0.516169931241}{0.795767723220}{0.517517121753}{0.795251384088}
  \meshline{0,0,0}{0.510406772922}{0.778171489682}{0.494942926628}{0.784098334397}
  \meshline{0,0,0}{0.523310243846}{0.773516035596}{0.521606786170}{0.774005366048}
  \meshline{0,0,0}{0.520955940055}{0.774179185108}{0.521606786170}{0.774005366048}
  \meshline{0,0,0}{0.573083921125}{0.842277763897}{0.590364874951}{0.830102820153}
  \meshline{0,0,0}{0.561753443699}{0.819930098785}{0.549049878912}{0.828581440354}
  \meshline{0,0,0}{0.619829252316}{0.765195309217}{0.593160425729}{0.771338834380}
  \meshline{0,0,0}{0.606613153602}{0.754014503134}{0.593877135140}{0.756948417367}
  \meshline{0,0,0}{0.590756784127}{0.829929578393}{0.592304710414}{0.829270612879}
  \meshline{0,0,0}{0.571080213963}{0.794451366502}{0.581859204887}{0.790836243202}
  \meshline{0,0,0}{0.580180040551}{0.773654438547}{0.570224580262}{0.776993361152}
  \meshline{0,0,0}{0.572293640326}{0.760640383402}{0.557103594195}{0.763864703187}
  \meshline{0,0,0}{0.523310243846}{0.773516035596}{0.544070115319}{0.767826361825}
  \meshline{255,170,0}{0.539348744807}{0.744346805542}{0.524707478334}{0.747463222745}
  \meshline{0,0,0}{0.772538466533}{0.792782123601}{0.785398163397}{0.792323908045}
  \meshline{0,0,0}{0.603665072071}{0.783934239154}{0.618054318141}{0.780914209723}
  \meshline{0,0,0}{0.637044460926}{0.776794436724}{0.647181272543}{0.775331626972}
  \meshline{0,0,0}{0.627539035566}{0.763949110380}{0.646999055736}{0.761140899243}
  \meshline{0,0,0}{0.598523312861}{0.803530764009}{0.599726475278}{0.803159873102}
  \meshline{0,0,0}{0.603665072071}{0.783934239154}{0.594497761029}{0.786760185393}
  \meshline{0,0,0}{0.618054318141}{0.780914209723}{0.637044460926}{0.776794436724}
  \meshline{0,0,0}{0.597211957376}{0.803953688962}{0.598523312861}{0.803530764009}
  \meshline{0,0,0}{0.581859204887}{0.790836243202}{0.594497761029}{0.786760185393}
  \meshline{0,0,0}{0.580180040551}{0.773654438547}{0.588464166589}{0.772084838485}
  \meshline{0,0,0}{0.572293640326}{0.760640383402}{0.580896242883}{0.759010441337}
  \meshline{255,170,0}{0.643254107777}{0.728749761147}{0.642413464547}{0.728835261883}
  \meshline{0,0,0}{0.635771855058}{0.749452871347}{0.645923817596}{0.748420328373}
  \meshline{255,170,0}{0.577776654662}{0.737612709313}{0.562703390113}{0.739680216964}
  \meshline{0,0,0}{0.588464166589}{0.772084838485}{0.593160425729}{0.771338834380}
  \meshline{0,0,0}{0.580896242883}{0.759010441337}{0.593877135140}{0.756948417367}
  \meshline{0,0,0}{0.619829252316}{0.765195309217}{0.621327562728}{0.764974667421}
  \meshline{0,0,0}{0.606613153602}{0.754014503134}{0.620771173640}{0.751929587392}
  \meshline{255,170,0}{0.588397256967}{0.735697529547}{0.599226815513}{0.734302123889}
  \meshline{170,255,0}{0.396827421373}{1.062779335023}{0.390726193023}{1.057357954266}
  \meshline{170,255,0}{0.390726193023}{1.057357954266}{0.364758763095}{1.035932987027}
  \meshline{255,170,0}{0.415534785326}{0.787641464333}{0.434724657872}{0.777068566295}
  \meshline{255,170,0}{0.437151664141}{0.775403042139}{0.455941628384}{0.768337522708}
  \meshline{255,170,0}{0.404338262719}{0.796714509569}{0.396872689519}{0.801998149233}
  \meshline{255,170,0}{0.390301815313}{0.811734925346}{0.396872689519}{0.801998149233}
  \meshline{255,170,0}{0.474018312661}{0.760928404269}{0.479001765194}{0.759393702938}
  \meshline{255,170,0}{0.474018312661}{0.760928404269}{0.459044225935}{0.766701919704}
  \meshline{0,0,0}{0.475114170022}{0.794418789535}{0.477177952299}{0.793623062955}
  \meshline{170,255,0}{0.420198937311}{0.646287004541}{0.393000958556}{0.649393436887}
  \meshline{255,170,0}{0.613188368374}{0.732278271579}{0.624641065282}{0.731442910585}
  \meshline{255,170,0}{0.480973916562}{0.758918386658}{0.499155828317}{0.754106092813}
  \meshline{255,170,0}{0.599226815513}{0.734302123889}{0.613188368374}{0.732278271579}
  \meshline{255,170,0}{0.588397256967}{0.735697529547}{0.577776654662}{0.737612709313}
  \meshline{0,0,0}{0.738863203279}{0.794399443569}{0.753383065593}{0.793542515682}
  \meshline{0,0,0}{0.757582812925}{0.850964794128}{0.760699569615}{0.850740615696}
  \meshline{0,0,0}{0.760699569615}{0.850740615696}{0.785398163397}{0.849934343921}
  \meshline{0,0,0}{0.655275270170}{0.893782127577}{0.657921134374}{0.890830987021}
  \meshline{0,0,0}{0.698954233023}{0.837259003668}{0.693546646333}{0.838306757843}
  \meshline{0,0,0}{0.701126195326}{0.815768655503}{0.689333114147}{0.818053639685}
  \meshline{0,0,0}{0.757582812925}{0.850964794128}{0.755944330791}{0.851204891322}
  \meshline{0,0,0}{0.732251435343}{0.855447413726}{0.755944330791}{0.851204891322}
  \meshline{0,0,0}{0.629738934597}{0.836873791711}{0.627362592320}{0.837760134566}
  \meshline{0,0,0}{0.634715659001}{0.811723406483}{0.625642632188}{0.815107520198}
  \meshline{0,0,0}{0.678779215398}{0.844540990277}{0.663622137903}{0.849159034291}
  \meshline{0,0,0}{0.619727415424}{0.797313493167}{0.639582812727}{0.792875671075}
  \meshline{0,0,0}{0.676988610625}{0.801501928690}{0.697890431314}{0.798746579768}
  \meshline{0,0,0}{0.692029359809}{0.783081749534}{0.693198600900}{0.782927616207}
  \meshline{0,0,0}{0.693381252790}{0.866335864055}{0.708849212998}{0.860958603336}
  \meshline{0,0,0}{0.732251435343}{0.855447413726}{0.717906926099}{0.858584092687}
  \meshline{0,0,0}{0.667235265723}{0.822943214232}{0.673927929344}{0.821505642765}
  \meshline{0,0,0}{0.673496085950}{0.802284535720}{0.668199451659}{0.803422242732}
  \meshline{0,0,0}{0.650273854202}{0.807910996429}{0.668199451659}{0.803422242732}
  \meshline{0,0,0}{0.655737250122}{0.788876557386}{0.648174532095}{0.790770339648}
  \meshline{0,0,0}{0.785398163397}{0.827413186680}{0.752577972258}{0.828731448870}
  \meshline{0,0,0}{0.668043554737}{0.881411166375}{0.657921134374}{0.890830987021}
  \meshline{0,0,0}{0.693381252790}{0.866335864055}{0.687743486212}{0.869033630098}
  \meshline{0,0,0}{0.719338472459}{0.894097776223}{0.736996607420}{0.888149909700}
  \meshline{0,0,0}{0.693546646333}{0.838306757843}{0.678779215398}{0.844540990277}
  \meshline{0,0,0}{0.650273854202}{0.807910996429}{0.634715659001}{0.811723406483}
  \meshline{0,0,0}{0.648174532095}{0.790770339648}{0.639582812727}{0.792875671075}
  \meshline{0,0,0}{0.621327562728}{0.764974667421}{0.627539035566}{0.763949110380}
  \meshline{0,0,0}{0.635771855058}{0.749452871347}{0.620771173640}{0.751929587392}
  \meshline{0,0,0}{0.775369228745}{0.880614911792}{0.785398163397}{0.881285011958}
  \meshline{0,0,0}{0.750461670443}{0.883816973276}{0.763405168086}{0.881600532633}
  \meshline{0,0,0}{0.703779790457}{0.836364955505}{0.698954233023}{0.837259003668}
  \meshline{0,0,0}{0.714050459371}{0.813374131206}{0.701126195326}{0.815768655503}
  \meshline{0,0,0}{0.742539056596}{0.810269013529}{0.726133553801}{0.812121486685}
  \meshline{0,0,0}{0.738863203279}{0.794399443569}{0.727093088004}{0.795728499000}
  \meshline{0,0,0}{0.697496548143}{0.912223584891}{0.711669513091}{0.899711001031}
  \meshline{0,0,0}{0.673927929344}{0.821505642765}{0.689333114147}{0.818053639685}
  \meshline{0,0,0}{0.673496085950}{0.802284535720}{0.676988610625}{0.801501928690}
  \meshline{0,0,0}{0.717906926099}{0.858584092687}{0.708849212998}{0.860958603336}
  \meshline{0,0,0}{0.742126034586}{0.752737079668}{0.723914694094}{0.753517022916}
  \meshline{0,0,0}{0.741979203118}{0.740691217305}{0.739998934696}{0.740776026931}
  \meshline{0,0,0}{0.671830257871}{0.786676694007}{0.692029359809}{0.783081749534}
  \meshline{0,0,0}{0.670006548544}{0.771531148826}{0.672747143429}{0.771043390189}
  \meshline{0,0,0}{0.727297749911}{0.832217234780}{0.703779790457}{0.836364955505}
  \meshline{0,0,0}{0.753460489658}{0.809509294296}{0.785398163397}{0.808655955672}
  \meshline{0,0,0}{0.752577972258}{0.828731448870}{0.745871504964}{0.829100569810}
  \meshline{0,0,0}{0.753460489658}{0.809509294296}{0.749250048850}{0.809741035062}
  \meshline{0,0,0}{0.723834002104}{0.812212380069}{0.714050459371}{0.813374131206}
  \meshline{0,0,0}{0.713429727677}{0.796268564727}{0.708924063876}{0.796803591781}
  \meshline{0,0,0}{0.744181342346}{0.829233541125}{0.745871504964}{0.829100569810}
  \meshline{0,0,0}{0.742539056596}{0.810269013529}{0.749250048850}{0.809741035062}
  \meshline{0,0,0}{0.727297749911}{0.832217234780}{0.744181342346}{0.829233541125}
  \meshline{0,0,0}{0.708924063876}{0.796803591781}{0.697890431314}{0.798746579768}
  \meshline{0,0,0}{0.693992668844}{0.782787783340}{0.693198600900}{0.782927616207}
  \meshline{0,0,0}{0.672747143429}{0.771043390189}{0.691076963737}{0.769155326423}
  \meshline{255,170,0}{0.693896616974}{0.725107294903}{0.679604653617}{0.726058310641}
  \meshline{0,0,0}{0.647181272543}{0.775331626972}{0.665326883942}{0.772170844211}
  \meshline{0,0,0}{0.646999055736}{0.761140899243}{0.653847403956}{0.759947985953}
  \meshline{255,170,0}{0.726244881333}{0.723268224191}{0.754972728182}{0.723645603818}
  \meshline{0,0,0}{0.686408723127}{0.756326899169}{0.670237677940}{0.758496402510}
  \meshline{0,0,0}{0.677123597708}{0.744961906317}{0.670807241515}{0.745809307069}
  \meshline{0,0,0}{0.713326453746}{0.781582447377}{0.693992668844}{0.782787783340}
  \meshline{0,0,0}{0.716274389740}{0.767268866713}{0.708033842626}{0.767782611323}
  \meshline{0,0,0}{0.723834002104}{0.812212380069}{0.726133553801}{0.812121486685}
  \meshline{0,0,0}{0.713429727677}{0.796268564727}{0.727093088004}{0.795728499000}
  \meshline{0,0,0}{0.769805457193}{0.751739729375}{0.785398163397}{0.751897460014}
  \meshline{0,0,0}{0.779107070960}{0.739988246358}{0.785398163397}{0.740051884960}
  \meshline{0,0,0}{0.772538466533}{0.792782123601}{0.753383065593}{0.793542515682}
  \meshline{255,170,0}{0.785398163397}{0.722954901654}{0.754972728182}{0.723645603818}
  \meshline{0,0,0}{0.785398163397}{0.777799382937}{0.760084610244}{0.777970435509}
  \meshline{0,0,0}{0.785398163397}{0.764176447514}{0.780435550807}{0.764209981631}
  \meshline{0,0,0}{0.691076963737}{0.769155326423}{0.708033842626}{0.767782611323}
  \meshline{0,0,0}{0.755265684178}{0.778075749290}{0.728749320933}{0.779481791586}
  \meshline{0,0,0}{0.744468022003}{0.764996023251}{0.739936836187}{0.765236291452}
  \meshline{0,0,0}{0.755265684178}{0.778075749290}{0.757414278161}{0.778081641183}
  \meshline{0,0,0}{0.744468022003}{0.764996023251}{0.760504710447}{0.765039999197}
  \meshline{0,0,0}{0.763595142733}{0.751998357210}{0.758906936590}{0.751985501171}
  \meshline{255,170,0}{0.714458296052}{0.723874655522}{0.693896616974}{0.725107294903}
  \meshline{0,0,0}{0.757414278161}{0.778081641183}{0.760084610244}{0.777970435509}
  \meshline{0,0,0}{0.760504710447}{0.765039999197}{0.780435550807}{0.764209981631}
  \meshline{0,0,0}{0.763595142733}{0.751998357210}{0.769805457193}{0.751739729375}
  \meshline{0,0,0}{0.745144874297}{0.740549434081}{0.779107070960}{0.739988246358}
  \meshline{0,0,0}{0.727596376824}{0.779560972734}{0.728749320933}{0.779481791586}
  \meshline{0,0,0}{0.721857938206}{0.766477902278}{0.739936836187}{0.765236291452}
  \meshline{0,0,0}{0.758906936590}{0.751985501171}{0.742126034586}{0.752737079668}
  \meshline{0,0,0}{0.745144874297}{0.740549434081}{0.741979203118}{0.740691217305}
  \meshline{255,170,0}{0.643254107777}{0.728749761147}{0.643966879625}{0.728664289346}
  \meshline{0,0,0}{0.645923817596}{0.748420328373}{0.658913945449}{0.746862621472}
  \meshline{0,0,0}{0.727596376824}{0.779560972734}{0.713326453746}{0.781582447377}
  \meshline{0,0,0}{0.721857938206}{0.766477902278}{0.716274389740}{0.767268866713}
  \meshline{255,170,0}{0.719723283092}{0.723856783583}{0.714458296052}{0.723874655522}
  \meshline{0,0,0}{0.713903626199}{0.754034036221}{0.718353233411}{0.754018932080}
  \meshline{0,0,0}{0.701961840875}{0.742740421120}{0.718868141860}{0.742683032873}
  \meshline{0,0,0}{0.670237677940}{0.758496402510}{0.653847403956}{0.759947985953}
  \meshline{0,0,0}{0.670807241515}{0.745809307069}{0.658913945449}{0.746862621472}
  \meshline{0,0,0}{0.713903626199}{0.754034036221}{0.692405839900}{0.755785241545}
  \meshline{0,0,0}{0.701961840875}{0.742740421120}{0.699490384518}{0.742941745455}
  \meshline{0,0,0}{0.692405839900}{0.755785241545}{0.686408723127}{0.756326899169}
  \meshline{0,0,0}{0.699490384518}{0.742941745455}{0.677123597708}{0.744961906317}
  \meshline{0,0,0}{0.432753544638}{0.872209552730}{0.430577276385}{0.863672966225}
  \meshline{255,170,0}{0.380278345584}{0.843708420242}{0.380723895286}{0.828778846271}
  \meshline{170,255,0}{0.396827421373}{1.062779335023}{0.418209760529}{1.082586363523}
  \meshline{255,170,0}{0.544588724550}{1.070010170110}{0.542123081034}{1.067335422078}
  \meshline{255,170,0}{0.514678505922}{0.749604391181}{0.519648537625}{0.748833263180}
  \meshline{0,255,170}{0.675710477704}{0.489828095930}{0.667626431139}{0.489845115209}
  \meshline{0,255,0}{0.751964668475}{0.556064556743}{0.740096317412}{0.556194985871}
  \meshline{255,170,0}{0.668669377004}{0.726744636946}{0.679604653617}{0.726058310641}
  \meshline{170,255,0}{0.695539866402}{0.630967734387}{0.738219990039}{0.630788094639}
  \meshline{255,170,0}{0.726244881333}{0.723268224191}{0.719723283092}{0.723856783583}
  \meshline{0,0,0}{0.718353233411}{0.754018932080}{0.723914694094}{0.753517022916}
  \meshline{0,0,0}{0.718868141860}{0.742683032873}{0.739998934696}{0.740776026931}
  \meshline{255,170,0}{0.643966879625}{0.728664289346}{0.668669377004}{0.726744636946}
  \meshline{0,0,0}{0.434933752015}{0.882613349511}{0.432753544638}{0.872209552730}
  \meshline{255,170,0}{0.390301815313}{0.811734925346}{0.380723895286}{0.828778846271}
  \meshline{255,170,0}{0.384600683661}{0.864501378446}{0.381991034569}{0.854509997843}
  \meshline{255,170,0}{0.380278345584}{0.843708420242}{0.381991034569}{0.854509997843}
  \meshline{255,170,0}{0.539348744807}{0.744346805542}{0.557745873932}{0.740763992547}
  \meshline{255,170,0}{0.519648537625}{0.748833263180}{0.524707478334}{0.747463222745}
  \meshline{255,170,0}{0.624641065282}{0.731442910585}{0.642413464547}{0.728835261883}
  \meshline{170,255,0}{0.562978833598}{0.636821518087}{0.610278887434}{0.634493312315}
  \meshline{170,255,0}{0.686981465257}{0.631385028207}{0.675955471435}{0.631643117457}
  \meshline{0,255,0}{0.331621079577}{1.113392066904}{0.356933898281}{1.132754890153}
  \meshline{170,255,0}{0.467047013283}{1.129822667478}{0.451071081705}{1.114119118885}
  \meshline{0,255,0}{0.364668869214}{1.139633468789}{0.400835073473}{1.174035525638}
  \meshline{170,255,0}{0.427927673773}{1.091435949320}{0.425954184681}{1.089603627511}
  \meshline{170,255,0}{0.467047013283}{1.129822667478}{0.492267915600}{1.159276900486}
  \meshline{170,255,0}{0.427927673773}{1.091435949320}{0.446038997397}{1.109212412590}
  \meshline{170,255,0}{0.771240453519}{0.629912413544}{0.738219990039}{0.630788094639}
  \meshline{170,255,0}{0.695539866402}{0.630967734387}{0.686981465257}{0.631385028207}
  \meshline{255,170,0}{0.395971435476}{0.885462742032}{0.384600683661}{0.864501378446}
  \meshline{255,170,0}{0.408951038322}{0.908585577170}{0.406779644971}{0.905677325993}
  \meshline{255,170,0}{0.398089848482}{0.891321552313}{0.406779644971}{0.905677325993}
  \meshline{0,0,0}{0.785398163397}{1.133965234021}{0.783625283061}{1.133616224178}
  \meshline{0,0,0}{0.752575197469}{1.152041877709}{0.785398163397}{1.158503418257}
  \meshline{0,0,0}{0.774172225342}{1.180831660403}{0.785398163397}{1.183041602494}
  \meshline{0,0,0}{0.735683195216}{1.143965381362}{0.739781136069}{1.147788934824}
  \meshline{0,0,0}{0.714221298291}{1.152167595834}{0.728765184177}{1.165737661196}
  \meshline{0,0,0}{0.692759401366}{1.160369810305}{0.704349230027}{1.171183614381}
  \meshline{0,255,0}{0.499242699086}{1.302701777599}{0.514529445547}{1.332696757012}
  \meshline{0,255,170}{0.441006203620}{1.345009706445}{0.419920679021}{1.309054063474}
  \meshline{170,255,0}{0.233498095343}{0.664225113929}{0.183417135704}{0.669024863900}
  \meshline{170,0,255}{0.608204566362}{0.286156478657}{0.631346595754}{0.286206631979}
  \meshline{170,255,0}{0.309277389897}{0.994449102306}{0.295034228594}{0.985298059338}
  \meshline{0,255,0}{0.265923140161}{1.067686308716}{0.280841600955}{1.076726867911}
  \meshline{0,170,255}{0.190512523228}{1.187646082472}{0.162755570914}{1.173995671211}
  \meshline{0,255,0}{0.265923140161}{1.067686308716}{0.244442219504}{1.057070069423}
  \meshline{0,255,170}{0.220539398102}{1.125825247268}{0.202653099805}{1.117281736462}
  \meshline{0,255,0}{0.400835073473}{1.174035525638}{0.404826511985}{1.178391088071}
  \meshline{170,255,0}{0.451071081705}{1.114119118885}{0.446038997397}{1.109212412590}
  \meshline{0,255,0}{0.696765368609}{0.556616956347}{0.692715843871}{0.556747459461}
  \meshline{170,255,0}{0.771240453519}{0.629912413544}{0.785398163397}{0.630038182821}
  \meshline{0,255,0}{0.687254597543}{0.556666044421}{0.692715843871}{0.556747459461}
  \meshline{0,255,170}{0.630584512720}{0.490115888665}{0.667626431139}{0.489845115209}
  \meshline{0,255,170}{0.782891390756}{0.489241218316}{0.736792203947}{0.489395539406}
  \meshline{0,255,170}{0.692319898991}{0.489574698809}{0.675710477704}{0.489828095930}
  \meshline{170,255,0}{0.562978833598}{0.636821518087}{0.547322911962}{0.637480894255}
  \meshline{0,255,0}{0.512536755405}{0.560899771060}{0.532098897421}{0.560195071025}
  \meshline{0,255,0}{0.499242699086}{1.302701777599}{0.478212855093}{1.270824589860}
  \meshline{0,255,170}{0.409205443014}{1.294232215704}{0.384679907429}{1.260410570671}
  \meshline{0,255,170}{0.419920679021}{1.309054063474}{0.417168662328}{1.304838284812}
  \meshline{0,255,170}{0.358269247484}{1.229960236364}{0.339304119616}{1.211281050108}
  \meshline{170,255,0}{0.247013602998}{0.662595355797}{0.240029093088}{0.664495838378}
  \meshline{170,255,0}{0.254887025570}{0.961672627310}{0.280045987671}{0.977726787595}
  \meshline{0,255,0}{0.163623163126}{1.021389799733}{0.186285659042}{1.031018181140}
  \meshline{170,255,0}{0.280045987671}{0.977726787595}{0.295034228594}{0.985298059338}
  \meshline{0,255,0}{0.186285659042}{1.031018181140}{0.205047237003}{1.037616250882}
  \meshline{170,255,0}{0.254887025570}{0.961672627310}{0.226876420926}{0.948081827648}
  \meshline{0,255,0}{0.472187189894}{0.562696469572}{0.460290263214}{0.563328817685}
  \meshline{170,255,0}{0.451074732779}{0.644407425896}{0.477310792877}{0.642601021526}
  \meshline{0,255,0}{0.401349048969}{0.564779681964}{0.378518355610}{0.566682007374}
  \meshline{0,255,0}{0.356933898281}{1.132754890153}{0.364668869214}{1.139633468789}
  \meshline{0,255,0}{0.306003303243}{1.094541098932}{0.317091634595}{1.101723011324}
  \meshline{0,255,170}{0.261160224826}{1.149242590499}{0.272864690572}{1.157261565538}
  \meshline{0,255,0}{0.331621079577}{1.113392066904}{0.317091634595}{1.101723011324}
  \meshline{0,255,170}{0.377448258348}{1.251555764691}{0.384679907429}{1.260410570671}
  \meshline{0,255,170}{0.624969152139}{0.490241877886}{0.630584512720}{0.490115888665}
  \meshline{0,170,255}{0.697205762717}{0.424675175353}{0.668997487122}{0.424819811100}
  \meshline{0,255,170}{0.692319898991}{0.489574698809}{0.736792203947}{0.489395539406}
  \meshline{0,170,255}{0.770510260053}{0.424474889988}{0.728028170965}{0.424606616696}
  \meshline{0,255,0}{0.646123615905}{0.557697620389}{0.687254597543}{0.556666044421}
  \meshline{0,255,0}{0.378518355610}{0.566682007374}{0.338003322379}{0.567258650946}
  \meshline{0,170,255}{0.592594854492}{0.425194849660}{0.631406779556}{0.425034413661}
  \meshline{0,0,255}{0.664313805968}{0.358292426484}{0.644272101088}{0.358546886278}
  \meshline{0,170,255}{0.668997487122}{0.424819811100}{0.646207961205}{0.424916383621}
  \meshline{0,255,0}{0.615348341152}{0.558180498365}{0.582447330266}{0.558688577752}
  \meshline{0,170,255}{0.646207961205}{0.424916383621}{0.631406779556}{0.425034413661}
  \meshline{170,255,0}{0.623241960746}{0.633663368577}{0.675955471435}{0.631643117457}
  \meshline{0,255,0}{0.646123615905}{0.557697620389}{0.615348341152}{0.558180498365}
  \meshline{170,255,0}{0.610278887434}{0.634493312315}{0.623241960746}{0.633663368577}
  \meshline{0,255,0}{0.426986966527}{1.202820367912}{0.404826511985}{1.178391088071}
  \meshline{0,255,0}{0.456582142163}{1.241159438888}{0.435111207904}{1.212241140023}
  \meshline{0,255,170}{0.358269247484}{1.229960236364}{0.377448258348}{1.251555764691}
  \meshline{0,255,170}{0.330657501745}{1.202784947437}{0.339304119616}{1.211281050108}
  \meshline{0,170,255}{0.333245767767}{1.304170423480}{0.312599700994}{1.278852829368}
  \meshline{0,170,255}{0.295217812132}{1.261072689779}{0.312599700994}{1.278852829368}
  \meshline{0,170,255}{0.506734967491}{0.425964008948}{0.475717556091}{0.426313579515}
  \meshline{0,255,0}{0.740096317412}{0.556194985871}{0.715812198911}{0.556265907379}
  \meshline{0,255,0}{0.785398163397}{0.556302743015}{0.751964668475}{0.556064556743}
  \meshline{0,170,255}{0.552095198068}{0.425486563030}{0.560888779300}{0.425533852933}
  \meshline{0,0,255}{0.550019096878}{0.358879943681}{0.551481887771}{0.358887810242}
  \meshline{0,170,255}{0.785398163397}{0.424488601878}{0.770510260053}{0.424474889988}
  \meshline{0,255,0}{0.478212855093}{1.270824589860}{0.471160505661}{1.259998470536}
  \meshline{0,255,170}{0.409205443014}{1.294232215704}{0.417168662328}{1.304838284812}
  \meshline{0,0,255}{0.719345522423}{0.358278681033}{0.703519631827}{0.358247170391}
  \meshline{0,0,255}{0.785398163397}{0.358095565671}{0.770244689013}{0.358141096689}
  \meshline{170,255,0}{0.000000000000}{0.679246438025}{0.011063268556}{0.678360122881}
  \meshline{0,255,170}{0.083277698266}{0.498685451866}{0.079984958205}{0.498767756933}
  \meshline{170,0,255}{0.649480666600}{0.286130048753}{0.650710589450}{0.286089526902}
  \meshline{170,255,0}{0.082813585185}{0.677022291040}{0.133633763463}{0.672614235889}
  \meshline{0,255,170}{0.040084973787}{0.499284505998}{0.001774838332}{0.499009087841}
  \meshline{0,255,0}{0.338003322379}{0.567258650946}{0.326639326620}{0.567736645564}
  \meshline{0,170,255}{0.697205762717}{0.424675175353}{0.728028170965}{0.424606616696}
  \meshline{255,0,170}{0.197564392478}{1.570796326795}{0.196538158061}{1.556860655044}
  \meshline{0,0,255}{0.719345522423}{0.358278681033}{0.770244689013}{0.358141096689}
  \meshline{0,0,0}{0.759378650501}{1.224733565118}{0.740719197548}{1.218100509274}
  \meshline{0,0,0}{0.781139062493}{1.252802481112}{0.729903942239}{1.234589438388}
  \meshline{255,170,0}{0.751812562423}{1.278157239398}{0.778688065626}{1.290335693495}
  \meshline{255,0,170}{0.178460709550}{1.486090028062}{0.186340224032}{1.507600946731}
  \meshline{255,0,170}{0.186340224032}{1.507600946731}{0.196538158061}{1.556860655044}
  \meshline{170,0,255}{0.091137174654}{1.299782268960}{0.070648331487}{1.293424969482}
  \meshline{255,0,170}{0.008778234110}{1.373715503820}{0.056085193499}{1.382358594864}
  \meshline{255,0,170}{0.084898443712}{1.391425015639}{0.056085193499}{1.382358594864}
  \meshline{255,0,170}{0.086781907674}{1.392429943532}{0.084898443712}{1.391425015639}
  \meshline{255,0,170}{0.117179634825}{1.413064858094}{0.089423572989}{1.393910918077}
  \meshline{255,0,170}{0.124872976638}{1.419080155208}{0.117179634825}{1.413064858094}
  \meshline{170,255,0}{0.499453926769}{0.641133099092}{0.477310792877}{0.642601021526}
  \meshline{0,255,0}{0.491941940510}{0.561235483984}{0.472187189894}{0.562696469572}
  \meshline{0,255,0}{0.437747648503}{0.563460200429}{0.460290263214}{0.563328817685}
  \meshline{170,255,0}{0.520685814070}{0.638834954451}{0.547322911962}{0.637480894255}
  \meshline{0,255,170}{0.477713905488}{0.492303419000}{0.434546784123}{0.493287242124}
  \meshline{0,255,0}{0.491941940510}{0.561235483984}{0.512536755405}{0.560899771060}
  \meshline{0,255,170}{0.478331200525}{0.492295296625}{0.477713905488}{0.492303419000}
  \meshline{0,255,0}{0.556817366410}{0.560184750207}{0.532098897421}{0.560195071025}
  \meshline{0,255,170}{0.513236818406}{0.491920006482}{0.551530180935}{0.491116439298}
  \meshline{0,255,170}{0.624969152139}{0.490241877886}{0.554334694091}{0.491080925841}
  \meshline{0,255,0}{0.582447330266}{0.558688577752}{0.556817366410}{0.560184750207}
  \meshline{0,255,170}{0.551530180935}{0.491116439298}{0.554334694091}{0.491080925841}
  \meshline{170,255,0}{0.520685814070}{0.638834954451}{0.499453926769}{0.641133099092}
  \meshline{170,255,0}{0.204754412550}{0.939623797891}{0.217480368895}{0.943885399866}
  \meshline{170,255,0}{0.115772533135}{0.902609344972}{0.082269023522}{0.898398473482}
  \meshline{170,255,0}{0.204754412550}{0.939623797891}{0.150234566153}{0.916524725166}
  \meshline{170,255,0}{0.314278543743}{0.655995895141}{0.320309871041}{0.655343760054}
  \meshline{0,255,0}{0.401349048969}{0.564779681964}{0.414201800425}{0.564630073848}
  \meshline{170,255,0}{0.420198937311}{0.646287004541}{0.451074732779}{0.644407425896}
  \meshline{170,255,0}{0.359912851167}{0.651734823222}{0.393000958556}{0.649393436887}
  \meshline{0,0,255}{0.161921200846}{0.360743714553}{0.163736984137}{0.360745083970}
  \meshline{170,255,0}{0.351890461567}{0.653309561423}{0.359912851167}{0.651734823222}
  \meshline{170,255,0}{0.277946854980}{0.660729103365}{0.247013602998}{0.662595355797}
  \meshline{170,255,0}{0.320309871041}{0.655343760054}{0.351890461567}{0.653309561423}
  \meshline{170,255,0}{0.312225569249}{0.656078344229}{0.314278543743}{0.655995895141}
  \meshline{0,255,170}{0.327122887826}{0.495149294827}{0.269472942303}{0.496354433046}
  \meshline{0,255,0}{0.313442429367}{0.568429659166}{0.273074367531}{0.570560270365}
  \meshline{170,255,0}{0.277946854980}{0.660729103365}{0.312225569249}{0.656078344229}
  \meshline{0,255,0}{0.175707790997}{0.572517357752}{0.213327883553}{0.572412714627}
  \meshline{0,255,0}{0.313442429367}{0.568429659166}{0.326639326620}{0.567736645564}
  \meshline{0,0,255}{0.231774832663}{1.295908549552}{0.257903676560}{1.319703223490}
  \meshline{0,0,255}{0.117656784755}{1.229805569269}{0.110072082114}{1.227769880381}
  \meshline{0,170,255}{0.260891841796}{1.231446853377}{0.207729665776}{1.195949779001}
  \meshline{0,170,255}{0.162755570914}{1.173995671211}{0.153696595667}{1.170218105164}
  \meshline{0,255,0}{0.163623163126}{1.021389799733}{0.137392934059}{1.014725862808}
  \meshline{0,255,0}{0.244442219504}{1.057070069423}{0.240012184892}{1.054727848093}
  \meshline{0,170,255}{0.261896326900}{1.232100079374}{0.260891841796}{1.231446853377}
  \meshline{0,255,170}{0.169302622826}{1.102868394362}{0.202653099805}{1.117281736462}
  \meshline{0,170,255}{0.132175540241}{1.162810914165}{0.153696595667}{1.170218105164}
  \meshline{0,255,0}{0.087182374539}{1.003903066839}{0.125667261340}{1.011191617861}
  \meshline{0,170,255}{0.207729665776}{1.195949779001}{0.190512523228}{1.187646082472}
  \meshline{0,255,170}{0.145821547158}{1.094749398646}{0.169302622826}{1.102868394362}
  \meshline{0,255,0}{0.137392934059}{1.014725862808}{0.125667261340}{1.011191617861}
  \meshline{0,0,255}{0.124678283965}{1.232947010066}{0.172665316686}{1.254557272227}
  \meshline{170,0,255}{0.000000000000}{1.283573681829}{0.035070496505}{1.287288708481}
  \meshline{0,255,170}{0.071507394707}{1.077499394876}{0.051923640055}{1.074274214319}
  \meshline{0,170,255}{0.132175540241}{1.162810914165}{0.117956063763}{1.158035678618}
  \meshline{0,170,255}{0.043326752622}{1.143273846553}{0.002973231502}{1.141151572576}
  \meshline{0,255,170}{0.121365844192}{1.088114884465}{0.097952902068}{1.081673668405}
  \meshline{0,170,255}{0.070360299739}{1.147272727255}{0.043326752622}{1.143273846553}
  \meshline{0,255,170}{0.071507394707}{1.077499394876}{0.097952902068}{1.081673668405}
  \meshline{0,0,255}{0.050714676190}{1.213770114147}{0.070935778865}{1.217202161952}
  \meshline{0,170,255}{0.080212773806}{1.148711173288}{0.104314650291}{1.154700525995}
  \meshline{170,0,255}{0.051615369455}{1.289011531557}{0.070648331487}{1.293424969482}
  \meshline{0,170,255}{0.070360299739}{1.147272727255}{0.080212773806}{1.148711173288}
  \meshline{0,0,255}{0.050714676190}{1.213770114147}{0.006192937578}{1.210133038455}
  \meshline{0,255,170}{0.000000000000}{1.071816313837}{0.000453176604}{1.071842692381}
  \meshline{0,170,255}{0.000000000000}{1.140978506458}{0.002973231502}{1.141151572576}
  \meshline{0,255,170}{0.051923640055}{1.074274214319}{0.000453176604}{1.071842692381}
  \meshline{0,255,0}{0.087182374539}{1.003903066839}{0.073917413717}{1.001051629694}
  \meshline{0,255,0}{0.070867890503}{1.000519713044}{0.073917413717}{1.001051629694}
  \meshline{0,0,255}{0.000000000000}{1.209841572846}{0.006192937578}{1.210133038455}
  \meshline{170,0,255}{0.035070496505}{1.287288708481}{0.051615369455}{1.289011531557}
  \meshline{0,170,255}{0.117956063763}{1.158035678618}{0.104314650291}{1.154700525995}
  \meshline{0,0,255}{0.110072082114}{1.227769880381}{0.070935778865}{1.217202161952}
  \meshline{0,255,170}{0.294773615786}{1.172777308150}{0.272864690572}{1.157261565538}
  \meshline{0,170,255}{0.263029518062}{1.233111285192}{0.295217812132}{1.261072689779}
  \meshline{0,255,170}{0.478949476240}{0.492275042688}{0.513236818406}{0.491920006482}
  \meshline{170,0,255}{0.702044848438}{0.286016117924}{0.734589772314}{0.285213933393}
  \meshline{170,255,0}{0.136347574612}{0.672513961557}{0.142695247392}{0.671838564585}
  \meshline{170,255,0}{0.136347574612}{0.672513961557}{0.133633763463}{0.672614235889}
  \meshline{170,255,0}{0.131631691373}{0.909433807531}{0.115772533135}{0.902609344972}
  \meshline{170,255,0}{0.183417135704}{0.669024863900}{0.142695247392}{0.671838564585}
  \meshline{170,255,0}{0.042605798966}{0.681379739123}{0.011063268556}{0.678360122881}
  \meshline{170,255,0}{0.082813585185}{0.677022291040}{0.071141812341}{0.676731249073}
  \meshline{170,255,0}{0.071141812341}{0.676731249073}{0.042605798966}{0.681379739123}
  \meshline{0,255,0}{0.070867890503}{1.000519713044}{0.004761351777}{0.995626659936}
  \meshline{0,255,0}{0.000000000000}{0.995284846282}{0.004761351777}{0.995626659936}
  \meshline{170,255,0}{0.082269023522}{0.898398473482}{0.073285070104}{0.897070476050}
  \meshline{170,255,0}{0.020171932279}{0.893168437858}{0.000000000000}{0.890400502499}
  \meshline{170,255,0}{0.036654573346}{0.892977896445}{0.055095021238}{0.896642323910}
  \meshline{170,255,0}{0.131631691373}{0.909433807531}{0.150234566153}{0.916524725166}
  \meshline{170,255,0}{0.036654573346}{0.892977896445}{0.020171932279}{0.893168437858}
  \meshline{170,255,0}{0.073285070104}{0.897070476050}{0.055095021238}{0.896642323910}
  \meshline{0,255,170}{0.478331200525}{0.492295296625}{0.478949476240}{0.492275042688}
  \meshline{0,255,0}{0.243285563495}{0.570295378082}{0.243283146117}{0.570295427652}
  \meshline{0,255,0}{0.172234584200}{0.572664887289}{0.168491470456}{0.572672097804}
  \meshline{0,255,0}{0.273074367531}{0.570560270365}{0.243285563495}{0.570295378082}
  \meshline{0,255,170}{0.208906990129}{0.497222050369}{0.226222573766}{0.497043301078}
  \meshline{0,255,0}{0.213327883553}{0.572412714627}{0.243283146117}{0.570295427652}
  \meshline{0,255,170}{0.269472942303}{0.496354433046}{0.244985624135}{0.496680553051}
  \meshline{0,170,255}{0.168440798709}{0.429186163878}{0.209376999490}{0.428875581703}
  \meshline{0,255,0}{0.175707790997}{0.572517357752}{0.172234584200}{0.572664887289}
  \meshline{0,170,255}{0.209376999490}{0.428875581703}{0.236261355783}{0.428710545292}
  \meshline{0,255,170}{0.162335800904}{0.498083413195}{0.143828916987}{0.498218292917}
  \meshline{0,170,255}{0.168440798709}{0.429186163878}{0.154867452333}{0.429349490124}
  \meshline{0,255,170}{0.208906990129}{0.497222050369}{0.162335800904}{0.498083413195}
  \meshline{0,255,0}{0.085754226681}{0.574539830503}{0.121545249432}{0.574228851950}
  \meshline{0,170,255}{0.000000000000}{0.429766307552}{0.007298094820}{0.429789819585}
  \meshline{0,255,170}{0.120624351139}{0.498637053486}{0.143828916987}{0.498218292917}
  \meshline{0,170,255}{0.154867452333}{0.429349490124}{0.148204113448}{0.429361213269}
  \meshline{0,255,170}{0.120624351139}{0.498637053486}{0.083277698266}{0.498685451866}
  \meshline{255,0,170}{0.115955988246}{0.198200543073}{0.112121907160}{0.198382618851}
  \meshline{0,170,255}{0.276551960597}{0.428265375802}{0.236261355783}{0.428710545292}
  \meshline{0,170,255}{0.536738293751}{0.425719133120}{0.552095198068}{0.425486563030}
  \meshline{0,0,255}{0.548643296890}{0.358900779256}{0.550019096878}{0.358879943681}
  \meshline{0,0,255}{0.407937173384}{0.359469925141}{0.398000541873}{0.359271750150}
  \meshline{170,0,255}{0.328882619846}{0.286366710416}{0.300501200266}{0.286035404579}
  \meshline{170,0,255}{0.202292021908}{0.286971178104}{0.192676652662}{0.287083069365}
  \meshline{0,0,255}{0.230373510487}{0.360073911129}{0.269702882904}{0.360188252700}
  \meshline{0,255,170}{0.226222573766}{0.497043301078}{0.244985624135}{0.496680553051}
  \meshline{0,255,170}{0.327122887826}{0.495149294827}{0.341695489970}{0.494895851847}
  \meshline{0,0,255}{0.230373510487}{0.360073911129}{0.211341877611}{0.360274085516}
  \meshline{0,0,255}{0.275078402990}{0.360124519363}{0.269702882904}{0.360188252700}
  \meshline{0,0,255}{0.275078402990}{0.360124519363}{0.286026072275}{0.360138122803}
  \meshline{0,170,255}{0.331478950844}{0.427731381599}{0.352386239881}{0.427473963574}
  \meshline{0,170,255}{0.276551960597}{0.428265375802}{0.301856612087}{0.428080800266}
  \meshline{0,0,255}{0.000000000000}{0.360666006210}{0.023720797815}{0.360878882393}
  \meshline{170,0,255}{0.109368775058}{0.286667749083}{0.091850926399}{0.286815161356}
  \meshline{0,170,255}{0.301856612087}{0.428080800266}{0.331478950844}{0.427731381599}
  \meshline{0,255,170}{0.398166485856}{0.493829638119}{0.434546784123}{0.493287242124}
  \meshline{0,255,170}{0.390186262066}{0.494081209968}{0.351286752832}{0.494714051374}
  \meshline{0,255,170}{0.343578238634}{0.494876284066}{0.351286752832}{0.494714051374}
  \meshline{0,255,170}{0.343578238634}{0.494876284066}{0.341695489970}{0.494895851847}
  \meshline{0,170,255}{0.407982651225}{0.426918269225}{0.364244235936}{0.427346543139}
  \meshline{0,170,255}{0.560888779300}{0.425533852933}{0.592594854492}{0.425194849660}
  \meshline{0,0,255}{0.615366455382}{0.358518477859}{0.588405902822}{0.358115495087}
  \meshline{0,170,255}{0.536738293751}{0.425719133120}{0.506734967491}{0.425964008948}
  \meshline{255,0,170}{0.330404980652}{0.196864282768}{0.354987796186}{0.197468260589}
  \meshline{170,0,255}{0.693068252088}{0.285775594320}{0.689350795577}{0.285785933090}
  \meshline{0,0,255}{0.588405902822}{0.358115495087}{0.551481887771}{0.358887810242}
  \meshline{0,0,255}{0.644272101088}{0.358546886278}{0.625631892885}{0.358424507193}
  \meshline{170,0,255}{0.649480666600}{0.286130048753}{0.631346595754}{0.286206631979}
  \meshline{0,0,255}{0.664313805968}{0.358292426484}{0.703519631827}{0.358247170391}
  \meshline{0,170,255}{0.414524761827}{0.426900460983}{0.407982651225}{0.426918269225}
  \meshline{0,170,255}{0.460917354285}{0.426393236886}{0.475717556091}{0.426313579515}
  \meshline{0,170,255}{0.364244235936}{0.427346543139}{0.352386239881}{0.427473963574}
  \meshline{0,170,255}{0.460917354285}{0.426393236886}{0.414524761827}{0.426900460983}
  \meshline{0,0,255}{0.350360217888}{0.359761111398}{0.382119657034}{0.359678648577}
  \meshline{170,0,255}{0.328882619846}{0.286366710416}{0.351737953385}{0.286286436052}
  \meshline{0,0,255}{0.286026072275}{0.360138122803}{0.322763046194}{0.359407467710}
  \meshline{255,0,170}{0.384755984530}{0.196661751814}{0.354987796186}{0.197468260589}
  \meshline{170,0,255}{0.300501200266}{0.286035404579}{0.271424453612}{0.286614377370}
  \meshline{170,0,255}{0.211707077801}{0.287052579922}{0.202292021908}{0.286971178104}
  \meshline{255,0,170}{0.281716774685}{0.198329245324}{0.270049726513}{0.197976952862}
  \meshline{255,0,170}{0.127393784848}{0.198544638303}{0.115955988246}{0.198200543073}
  \meshline{170,0,255}{0.211707077801}{0.287052579922}{0.258741612340}{0.286271170149}
  \meshline{170,0,255}{0.147953816558}{0.286440691030}{0.192676652662}{0.287083069365}
  \meshline{0,170,255}{0.148204113448}{0.429361213269}{0.112942970438}{0.429554411470}
  \meshline{255,0,170}{0.186250771388}{0.197957661804}{0.171802550750}{0.197633886967}
  \meshline{255,0,170}{0.260475905820}{0.198270477529}{0.267135597676}{0.198165363545}
  \meshline{170,0,255}{0.045335448586}{0.287115609284}{0.048380943798}{0.287170257086}
  \meshline{0,0,255}{0.161921200846}{0.360743714553}{0.160692588889}{0.360752037816}
  \meshline{0,0,255}{0.112699587598}{0.360531515154}{0.099733124638}{0.360754095606}
  \meshline{170,0,255}{0.147953816558}{0.286440691030}{0.109368775058}{0.286667749083}
  \meshline{255,0,170}{0.171802550750}{0.197633886967}{0.127393784848}{0.198544638303}
  \meshline{255,0,170}{0.260475905820}{0.198270477529}{0.223398133576}{0.197788344083}
  \meshline{255,0,170}{0.186250771388}{0.197957661804}{0.223398133576}{0.197788344083}
  \meshline{255,0,170}{0.270049726513}{0.197976952862}{0.267135597676}{0.198165363545}
  \meshline{170,0,255}{0.258741612340}{0.286271170149}{0.271424453612}{0.286614377370}
  \meshline{0,0,255}{0.112699587598}{0.360531515154}{0.160692588889}{0.360752037816}
  \meshline{0,0,255}{0.099733124638}{0.360754095606}{0.072334041639}{0.360730986221}
  \meshline{170,0,255}{0.042251783953}{0.287160809634}{0.045335448586}{0.287115609284}
  \meshline{255,0,170}{0.008123544184}{0.197773145916}{0.050769113696}{0.198608015064}
  \meshline{255,0,170}{0.057733110741}{0.198538342047}{0.112121907160}{0.198382618851}
  \meshline{170,0,255}{0.048380943798}{0.287170257086}{0.091850926399}{0.286815161356}
  \meshline{255,0,170}{0.008123544184}{0.197773145916}{0.000000000000}{0.197569784137}
  \meshline{255,0,170}{0.056065624844}{0.198507033770}{0.057733110741}{0.198538342047}
  \meshline{255,0,170}{0.050769113696}{0.198608015064}{0.056065624844}{0.198507033770}
  \meshline{255,0,170}{0.281716774685}{0.198329245324}{0.330404980652}{0.196864282768}
  \meshline{0,0,255}{0.322763046194}{0.359407467710}{0.350360217888}{0.359761111398}
  \meshline{170,0,255}{0.775719278330}{0.285668786601}{0.734589772314}{0.285213933393}
  \meshline{0,0,255}{0.451315502226}{0.358930855825}{0.407937173384}{0.359469925141}
  \meshline{255,0,170}{0.447520744930}{0.197103673266}{0.417570313407}{0.195681765345}
  \meshline{170,0,255}{0.605809489733}{0.286111079513}{0.608204566362}{0.286156478657}
  \meshline{0,0,255}{0.502470140672}{0.359030240529}{0.495841202691}{0.359092520894}
  \meshline{255,0,170}{0.417570313407}{0.195681765345}{0.384755984530}{0.196661751814}
  \meshline{170,0,255}{0.452586086692}{0.285929654611}{0.421635288409}{0.286490962936}
  \meshline{0,0,255}{0.382119657034}{0.359678648577}{0.398000541873}{0.359271750150}
  \meshline{170,0,255}{0.471317009434}{0.286061728910}{0.452586086692}{0.285929654611}
  \meshline{0,0,255}{0.502470140672}{0.359030240529}{0.535115177257}{0.358994669194}
  \meshline{170,0,255}{0.399903671700}{0.286083914001}{0.421635288409}{0.286490962936}
  \meshline{170,0,255}{0.351737953385}{0.286286436052}{0.390260381079}{0.286386002501}
  \meshline{170,0,255}{0.390260381079}{0.286386002501}{0.399903671700}{0.286083914001}
  \meshline{255,0,170}{0.464470659759}{0.197497000972}{0.447520744930}{0.197103673266}
  \meshline{0,0,255}{0.548643296890}{0.358900779256}{0.535115177257}{0.358994669194}
  \meshline{0,0,255}{0.495841202691}{0.359092520894}{0.451315502226}{0.358930855825}
  \meshline{0,0,255}{0.615366455382}{0.358518477859}{0.625631892885}{0.358424507193}
  \meshline{255,0,170}{0.490889570139}{0.196069321942}{0.464470659759}{0.197497000972}
  \meshline{170,0,255}{0.546978234256}{0.286334702662}{0.524904761640}{0.286279507834}
  \meshline{170,0,255}{0.471317009434}{0.286061728910}{0.524904761640}{0.286279507834}
  \meshline{255,0,170}{0.604738623959}{0.198300399832}{0.604454598235}{0.198307552130}
  \meshline{255,0,170}{0.537854201776}{0.198311274086}{0.539691338571}{0.198267021360}
  \meshline{170,0,255}{0.546978234256}{0.286334702662}{0.568101700514}{0.286046247533}
  \meshline{255,0,170}{0.720702696459}{0.197874197769}{0.714795414503}{0.197944578814}
  \meshline{255,0,170}{0.656328339859}{0.197782029316}{0.650933947205}{0.197601730859}
  \meshline{170,0,255}{0.605809489733}{0.286111079513}{0.568101700514}{0.286046247533}
  \meshline{255,0,170}{0.541226805878}{0.198253927706}{0.590579381529}{0.198333803000}
  \meshline{255,0,170}{0.537854201776}{0.198311274086}{0.490889570139}{0.196069321942}
  \meshline{255,0,170}{0.539691338571}{0.198267021360}{0.541226805878}{0.198253927706}
  \meshline{170,0,255}{0.650710589450}{0.286089526902}{0.689350795577}{0.285785933090}
  \meshline{255,0,170}{0.656328339859}{0.197782029316}{0.714795414503}{0.197944578814}
  \meshline{170,0,255}{0.693068252088}{0.285775594320}{0.702044848438}{0.286016117924}
  \meshline{255,0,170}{0.604738623959}{0.198300399832}{0.650933947205}{0.197601730859}
  \meshline{255,0,170}{0.785398163397}{0.198106640697}{0.783495098235}{0.198106192426}
  \meshline{255,0,170}{0.590579381529}{0.198333803000}{0.604454598235}{0.198307552130}
  \meshline{0,255,0}{0.414201800425}{0.564630073848}{0.437747648503}{0.563460200429}
  \meshline{0,255,170}{0.398166485856}{0.493829638119}{0.390186262066}{0.494081209968}
  \meshline{0,255,0}{0.013481340749}{0.575561127520}{0.000000000000}{0.576136194842}
  \meshline{0,255,0}{0.013481340749}{0.575561127520}{0.063573493640}{0.575123757486}
  \meshline{0,255,0}{0.073809748903}{0.575448359316}{0.063573493640}{0.575123757486}
  \meshline{0,255,0}{0.121545249432}{0.574228851950}{0.168491470456}{0.572672097804}
  \meshline{0,255,0}{0.073809748903}{0.575448359316}{0.085754226681}{0.574539830503}
  \meshline{0,255,170}{0.079984958205}{0.498767756933}{0.078655013229}{0.498736585548}
  \meshline{0,170,255}{0.112942970438}{0.429554411470}{0.075903421613}{0.429671175781}
  \meshline{0,170,255}{0.060864500018}{0.429701282715}{0.075903421613}{0.429671175781}
  \meshline{0,170,255}{0.060864500018}{0.429701282715}{0.054492783837}{0.429725154581}
  \meshline{0,170,255}{0.007298094820}{0.429789819585}{0.054492783837}{0.429725154581}
  \meshline{0,255,170}{0.040084973787}{0.499284505998}{0.078655013229}{0.498736585548}
  \meshline{0,255,170}{0.000000000000}{0.499027299728}{0.001774838332}{0.499009087841}
  \meshline{170,0,255}{0.042251783953}{0.287160809634}{0.000000000000}{0.286237996971}
  \meshline{0,0,255}{0.072334041639}{0.360730986221}{0.053521026279}{0.360658521710}
  \meshline{0,0,255}{0.053521026279}{0.360658521710}{0.023720797815}{0.360878882393}
  \meshline{255,0,170}{0.783495098235}{0.198106192426}{0.720702696459}{0.197874197769}
  \meshline{170,0,255}{0.775719278330}{0.285668786601}{0.785398163397}{0.285665143963}
  \meshline{0,0,255}{0.219638292004}{1.285417852556}{0.231774832663}{1.295908549552}
  \meshline{0,0,255}{0.172665316686}{1.254557272227}{0.209215154376}{1.278235531622}
\end{pgfscope}


==> integration.tex <==
\providecommand{\PrecisionAchieved}[4]{%
  % {x0,y0}{x1,y1}{xmid,ymid}{w}
  \draw[color=orange,fill] (#3) circle(#4);}
\providecommand{\HigherOrderColor}{light-green}
\draw[] (0.9375, 0.9375) rectangle (1, 1);% [-0.00819741, 0]
\PrecisionAchieved{0.9375,0.9375}{1,1}{0.96875,0.96875}{0.0125}
\draw[] (0.875, 0.9375) rectangle (0.9375, 1);% [-0.0243169, 0]
\PrecisionAchieved{0.875,0.9375}{0.9375,1}{0.90625,0.96875}{0.0125}
\draw[] (0.9375, 0.875) rectangle (1, 0.9375);% [-0.0243169, 0]
\PrecisionAchieved{0.9375,0.875}{1,0.9375}{0.96875,0.90625}{0.0125}
\draw[] (0.875, 0.875) rectangle (0.9375, 0.9375);% [-0.0379418, 0]
\PrecisionAchieved{0.875,0.875}{0.9375,0.9375}{0.90625,0.90625}{0.0125}
\draw[] (0.8125, 0.9375) rectangle (0.875, 1);% [-0.0428262, 0]
\PrecisionAchieved{0.8125,0.9375}{0.875,1}{0.84375,0.96875}{0.0125}
\draw[] (0.78125, 0.96875) rectangle (0.8125, 1);% [-0.0186564, 0]
\PrecisionAchieved{0.78125,0.96875}{0.8125,1}{0.796875,0.984375}{0.00625}
\draw[] (0.75, 0.96875) rectangle (0.78125, 1);% [-0.0221457, 0]
\PrecisionAchieved{0.75,0.96875}{0.78125,1}{0.765625,0.984375}{0.00625}
\draw[] (0.78125, 0.9375) rectangle (0.8125, 0.96875);% [-0.0258229, 0]
\PrecisionAchieved{0.78125,0.9375}{0.8125,0.96875}{0.796875,0.953125}{0.00625}
\draw[] (0.75, 0.9375) rectangle (0.78125, 0.96875);% [-0.0318472, 0]
\PrecisionAchieved{0.75,0.9375}{0.78125,0.96875}{0.765625,0.953125}{0.00625}
\draw[] (0.84375, 0.90625) rectangle (0.875, 0.9375);% [-0.0186996, 0]
\PrecisionAchieved{0.84375,0.90625}{0.875,0.9375}{0.859375,0.921875}{0.00625}
\draw[] (0.8125, 0.90625) rectangle (0.84375, 0.9375);% [-0.0243169, 0]
\PrecisionAchieved{0.8125,0.90625}{0.84375,0.9375}{0.828125,0.921875}{0.00625}
\draw[] (0.84375, 0.875) rectangle (0.875, 0.90625);% [-0.0196956, 0]
\PrecisionAchieved{0.84375,0.875}{0.875,0.90625}{0.859375,0.890625}{0.00625}
\draw[] (0.8125, 0.875) rectangle (0.84375, 0.90625);% [-0.0256307, 0]
\PrecisionAchieved{0.8125,0.875}{0.84375,0.90625}{0.828125,0.890625}{0.00625}
\draw[] (0.78125, 0.90625) rectangle (0.8125, 0.9375);% [-0.0312224, 0]
\PrecisionAchieved{0.78125,0.90625}{0.8125,0.9375}{0.796875,0.921875}{0.00625}
\draw[] (0.75, 0.90625) rectangle (0.78125, 0.9375);% [-0.0395592, 0]
\PrecisionAchieved{0.75,0.90625}{0.78125,0.9375}{0.765625,0.921875}{0.00625}
\draw[] (0.78125, 0.875) rectangle (0.8125, 0.90625);% [-0.0335055, 0]
\PrecisionAchieved{0.78125,0.875}{0.8125,0.90625}{0.796875,0.890625}{0.00625}
\draw[] (0.75, 0.875) rectangle (0.78125, 0.90625);% [-0.043624, 0]
\PrecisionAchieved{0.75,0.875}{0.78125,0.90625}{0.765625,0.890625}{0.00625}
\draw[] (0.9375, 0.8125) rectangle (1, 0.875);% [-0.0428262, 0]
\PrecisionAchieved{0.9375,0.8125}{1,0.875}{0.96875,0.84375}{0.0125}
\draw[] (0.90625, 0.84375) rectangle (0.9375, 0.875);% [-0.0186996, 0]
\PrecisionAchieved{0.90625,0.84375}{0.9375,0.875}{0.921875,0.859375}{0.00625}
\draw[] (0.875, 0.84375) rectangle (0.90625, 0.875);% [-0.0196956, 0]
\PrecisionAchieved{0.875,0.84375}{0.90625,0.875}{0.890625,0.859375}{0.00625}
\draw[] (0.90625, 0.8125) rectangle (0.9375, 0.84375);% [-0.0243169, 0]
\PrecisionAchieved{0.90625,0.8125}{0.9375,0.84375}{0.921875,0.828125}{0.00625}
\draw[] (0.875, 0.8125) rectangle (0.90625, 0.84375);% [-0.0256307, 0]
\PrecisionAchieved{0.875,0.8125}{0.90625,0.84375}{0.890625,0.828125}{0.00625}
\draw[] (0.96875, 0.78125) rectangle (1, 0.8125);% [-0.0186564, 0]
\PrecisionAchieved{0.96875,0.78125}{1,0.8125}{0.984375,0.796875}{0.00625}
\draw[] (0.9375, 0.78125) rectangle (0.96875, 0.8125);% [-0.0258229, 0]
\PrecisionAchieved{0.9375,0.78125}{0.96875,0.8125}{0.953125,0.796875}{0.00625}
\draw[] (0.96875, 0.75) rectangle (1, 0.78125);% [-0.0221457, 0]
\PrecisionAchieved{0.96875,0.75}{1,0.78125}{0.984375,0.765625}{0.00625}
\draw[] (0.9375, 0.75) rectangle (0.96875, 0.78125);% [-0.0318472, 0]
\PrecisionAchieved{0.9375,0.75}{0.96875,0.78125}{0.953125,0.765625}{0.00625}
\draw[] (0.90625, 0.78125) rectangle (0.9375, 0.8125);% [-0.0312224, 0]
\PrecisionAchieved{0.90625,0.78125}{0.9375,0.8125}{0.921875,0.796875}{0.00625}
\draw[] (0.875, 0.78125) rectangle (0.90625, 0.8125);% [-0.0335055, 0]
\PrecisionAchieved{0.875,0.78125}{0.90625,0.8125}{0.890625,0.796875}{0.00625}
\draw[] (0.90625, 0.75) rectangle (0.9375, 0.78125);% [-0.0395592, 0]
\PrecisionAchieved{0.90625,0.75}{0.9375,0.78125}{0.921875,0.765625}{0.00625}
\draw[] (0.875, 0.75) rectangle (0.90625, 0.78125);% [-0.043624, 0]
\PrecisionAchieved{0.875,0.75}{0.90625,0.78125}{0.890625,0.765625}{0.00625}
\draw[] (0.84375, 0.84375) rectangle (0.875, 0.875);% [-0.0180817, 0]
\PrecisionAchieved{0.84375,0.84375}{0.875,0.875}{0.859375,0.859375}{0.00625}
\draw[] (0.8125, 0.84375) rectangle (0.84375, 0.875);% [-0.0236217, 0]
\PrecisionAchieved{0.8125,0.84375}{0.84375,0.875}{0.828125,0.859375}{0.00625}
\draw[] (0.84375, 0.8125) rectangle (0.875, 0.84375);% [-0.0236217, 0]
\PrecisionAchieved{0.84375,0.8125}{0.875,0.84375}{0.859375,0.828125}{0.00625}
\draw[] (0.8125, 0.8125) rectangle (0.84375, 0.84375);% [-0.0180755, 0]
\PrecisionAchieved{0.8125,0.8125}{0.84375,0.84375}{0.828125,0.828125}{0.00625}
\draw[] (0.78125, 0.84375) rectangle (0.8125, 0.875);% [-0.0316975, 0]
\PrecisionAchieved{0.78125,0.84375}{0.8125,0.875}{0.796875,0.859375}{0.00625}
\draw[] (0.75, 0.84375) rectangle (0.78125, 0.875);% [-0.0428262, 0]
\PrecisionAchieved{0.75,0.84375}{0.78125,0.875}{0.765625,0.859375}{0.00625}
\draw[] (0.78125, 0.8125) rectangle (0.8125, 0.84375);% [-0.0253958, 0]
\PrecisionAchieved{0.78125,0.8125}{0.8125,0.84375}{0.796875,0.828125}{0.00625}
\draw[] (0.75, 0.8125) rectangle (0.78125, 0.84375);% [-0.036502, 0]
\PrecisionAchieved{0.75,0.8125}{0.78125,0.84375}{0.765625,0.828125}{0.00625}
\draw[] (0.84375, 0.78125) rectangle (0.875, 0.8125);% [-0.0316975, 0]
\PrecisionAchieved{0.84375,0.78125}{0.875,0.8125}{0.859375,0.796875}{0.00625}
\draw[] (0.8125, 0.78125) rectangle (0.84375, 0.8125);% [-0.0253958, 0]
\PrecisionAchieved{0.8125,0.78125}{0.84375,0.8125}{0.828125,0.796875}{0.00625}
\draw[] (0.84375, 0.75) rectangle (0.875, 0.78125);% [-0.0428262, 0]
\PrecisionAchieved{0.84375,0.75}{0.875,0.78125}{0.859375,0.765625}{0.00625}
\draw[] (0.8125, 0.75) rectangle (0.84375, 0.78125);% [-0.036502, 0]
\PrecisionAchieved{0.8125,0.75}{0.84375,0.78125}{0.828125,0.765625}{0.00625}
\draw[] (0.75, 0.75) rectangle (0.8125, 0.8125);% [-0.0373315, 0]
\PrecisionAchieved{0.75,0.75}{0.8125,0.8125}{0.78125,0.78125}{0.0125}
\draw[] (0.71875, 0.96875) rectangle (0.75, 1);% [-0.0254528, 0]
\PrecisionAchieved{0.71875,0.96875}{0.75,1}{0.734375,0.984375}{0.00625}
\draw[] (0.6875, 0.96875) rectangle (0.71875, 1);% [-0.028489, 0]
\PrecisionAchieved{0.6875,0.96875}{0.71875,1}{0.703125,0.984375}{0.00625}
\draw[] (0.71875, 0.9375) rectangle (0.75, 0.96875);% [-0.0390284, 0]
\PrecisionAchieved{0.71875,0.9375}{0.75,0.96875}{0.734375,0.953125}{0.00625}
\draw[] (0.6875, 0.9375) rectangle (0.71875, 0.96875);% [-0.0473243, 0]
\PrecisionAchieved{0.6875,0.9375}{0.71875,0.96875}{0.703125,0.953125}{0.00625}
\draw[] (0.65625, 0.96875) rectangle (0.6875, 1);% [-0.0311793, 0]
\PrecisionAchieved{0.65625,0.96875}{0.6875,1}{0.671875,0.984375}{0.00625}
\draw[] (0.625, 0.96875) rectangle (0.65625, 1);% [-0.0334617, 0]
\PrecisionAchieved{0.625,0.96875}{0.65625,1}{0.640625,0.984375}{0.00625}
\draw[] (0.65625, 0.9375) rectangle (0.6875, 0.96875);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.625, 0.9375) rectangle (0.65625, 0.96875);% [-0.0270614, -0.0228941]
\PrecisionAchieved{0.625,0.9375}{0.65625,0.96875}{0.640625,0.953125}{0.00625}
\draw[] (0.71875, 0.90625) rectangle (0.75, 0.9375);% [-0.050508, 0]
\draw[fill=\HigherOrderColor] (0.6875, 0.90625) rectangle (0.71875, 0.9375);% [-0.0253345, -0.023126]
\PrecisionAchieved{0.6875,0.90625}{0.71875,0.9375}{0.703125,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.875) rectangle (0.75, 0.90625);% [-0.0223134, -0.0203917]
\PrecisionAchieved{0.71875,0.875}{0.75,0.90625}{0.734375,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.875) rectangle (0.71875, 0.90625);% [-0.0362129, -0.0346317]
\PrecisionAchieved{0.6875,0.875}{0.71875,0.90625}{0.703125,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.65625, 0.90625) rectangle (0.6875, 0.9375);% [-0.0370912, -0.0353961]
\PrecisionAchieved{0.65625,0.90625}{0.6875,0.9375}{0.671875,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.90625) rectangle (0.65625, 0.9375);% [-0.051275, -0.0498579]
\PrecisionAchieved{0.625,0.90625}{0.65625,0.9375}{0.640625,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.65625, 0.875) rectangle (0.6875, 0.90625);% [-0.0539678, -0.0525059]
\PrecisionAchieved{0.65625,0.875}{0.6875,0.90625}{0.671875,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.875) rectangle (0.65625, 0.90625);% [-0.0745963, -0.0731945]
\PrecisionAchieved{0.625,0.875}{0.65625,0.90625}{0.640625,0.890625}{0.00625}
\draw[] (0.59375, 0.96875) rectangle (0.625, 1);% [-0.0352867, 0]
\PrecisionAchieved{0.59375,0.96875}{0.625,1}{0.609375,0.984375}{0.00625}
\draw[] (0.5625, 0.96875) rectangle (0.59375, 1);% [-0.0366166, 0]
\PrecisionAchieved{0.5625,0.96875}{0.59375,1}{0.578125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.59375, 0.9375) rectangle (0.625, 0.96875);% [-0.0350878, -0.0318305]
\PrecisionAchieved{0.59375,0.9375}{0.625,0.96875}{0.609375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.9375) rectangle (0.59375, 0.96875);% [-0.0442196, -0.0413198]
\PrecisionAchieved{0.5625,0.9375}{0.59375,0.96875}{0.578125,0.953125}{0.00625}
\draw[] (0.53125, 0.96875) rectangle (0.5625, 1);% [-0.0374249, 0]
\PrecisionAchieved{0.53125,0.96875}{0.5625,1}{0.546875,0.984375}{0.00625}
\draw[] (0.5, 0.96875) rectangle (0.53125, 1);% [-0.0376961, 0]
\PrecisionAchieved{0.5,0.96875}{0.53125,1}{0.515625,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.53125, 0.9375) rectangle (0.5625, 0.96875);% [-0.0537469, -0.0512044]
\PrecisionAchieved{0.53125,0.9375}{0.5625,0.96875}{0.546875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.9375) rectangle (0.53125, 0.96875);% [-0.0631646, -0.0610217]
\PrecisionAchieved{0.5,0.9375}{0.53125,0.96875}{0.515625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.875) rectangle (0.625, 0.9375);% [-0.0985275, -0.0852643]
\PrecisionAchieved{0.5625,0.875}{0.625,0.9375}{0.59375,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.875) rectangle (0.5625, 0.9375);% [-0.136228, -0.121679]
\PrecisionAchieved{0.5,0.875}{0.5625,0.9375}{0.53125,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.71875, 0.84375) rectangle (0.75, 0.875);% [-0.0255521, -0.0235068]
\PrecisionAchieved{0.71875,0.84375}{0.75,0.875}{0.734375,0.859375}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.84375) rectangle (0.71875, 0.875);% [-0.0434626, -0.0416773]
\PrecisionAchieved{0.6875,0.84375}{0.71875,0.875}{0.703125,0.859375}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.8125) rectangle (0.75, 0.84375);% [-0.0243226, -0.0219393]
\PrecisionAchieved{0.71875,0.8125}{0.75,0.84375}{0.734375,0.828125}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.8125) rectangle (0.71875, 0.84375);% [-0.0449652, -0.0429422]
\PrecisionAchieved{0.6875,0.8125}{0.71875,0.84375}{0.703125,0.828125}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.8125) rectangle (0.6875, 0.875);% [-0.0895606, -0.0760559]
\PrecisionAchieved{0.625,0.8125}{0.6875,0.875}{0.65625,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.71875, 0.78125) rectangle (0.75, 0.8125);% [-0.0183931, -0.0153567]
\PrecisionAchieved{0.71875,0.78125}{0.75,0.8125}{0.734375,0.796875}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.78125) rectangle (0.71875, 0.8125);% [-0.0398853, -0.037525]
\PrecisionAchieved{0.6875,0.78125}{0.71875,0.8125}{0.703125,0.796875}{0.00625}
\draw[] (0.71875, 0.75) rectangle (0.75, 0.78125);% [-0.0254528, 0]
\PrecisionAchieved{0.71875,0.75}{0.75,0.78125}{0.734375,0.765625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.75) rectangle (0.71875, 0.78125);% [-0.0284654, -0.0255542]
\PrecisionAchieved{0.6875,0.75}{0.71875,0.78125}{0.703125,0.765625}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.75) rectangle (0.6875, 0.8125);% [-0.0886292, -0.0745694]
\PrecisionAchieved{0.625,0.75}{0.6875,0.8125}{0.65625,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.8125) rectangle (0.625, 0.875);% [-0.14503, -0.132578]
\PrecisionAchieved{0.5625,0.8125}{0.625,0.875}{0.59375,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.8125) rectangle (0.5625, 0.875);% [-0.185228, -0.16844]
\PrecisionAchieved{0.5,0.8125}{0.5625,0.875}{0.53125,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.75) rectangle (0.625, 0.8125);% [-0.157796, -0.144785]
\PrecisionAchieved{0.5625,0.75}{0.625,0.8125}{0.59375,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.75) rectangle (0.5625, 0.8125);% [-0.191339, -0.17651]
\PrecisionAchieved{0.5,0.75}{0.5625,0.8125}{0.53125,0.78125}{0.0125}
\draw[] (0.96875, 0.71875) rectangle (1, 0.75);% [-0.0254528, 0]
\PrecisionAchieved{0.96875,0.71875}{1,0.75}{0.984375,0.734375}{0.00625}
\draw[] (0.9375, 0.71875) rectangle (0.96875, 0.75);% [-0.0390284, 0]
\PrecisionAchieved{0.9375,0.71875}{0.96875,0.75}{0.953125,0.734375}{0.00625}
\draw[] (0.96875, 0.6875) rectangle (1, 0.71875);% [-0.028489, 0]
\PrecisionAchieved{0.96875,0.6875}{1,0.71875}{0.984375,0.703125}{0.00625}
\draw[] (0.9375, 0.6875) rectangle (0.96875, 0.71875);% [-0.0473243, 0]
\PrecisionAchieved{0.9375,0.6875}{0.96875,0.71875}{0.953125,0.703125}{0.00625}
\draw[] (0.90625, 0.71875) rectangle (0.9375, 0.75);% [-0.050508, 0]
\draw[fill=\HigherOrderColor] (0.875, 0.71875) rectangle (0.90625, 0.75);% [-0.0223134, -0.0203917]
\PrecisionAchieved{0.875,0.71875}{0.90625,0.75}{0.890625,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.90625, 0.6875) rectangle (0.9375, 0.71875);% [-0.0253345, -0.023126]
\PrecisionAchieved{0.90625,0.6875}{0.9375,0.71875}{0.921875,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.6875) rectangle (0.90625, 0.71875);% [-0.0362129, -0.0346317]
\PrecisionAchieved{0.875,0.6875}{0.90625,0.71875}{0.890625,0.703125}{0.00625}
\draw[] (0.96875, 0.65625) rectangle (1, 0.6875);% [-0.0311793, 0]
\PrecisionAchieved{0.96875,0.65625}{1,0.6875}{0.984375,0.671875}{0.00625}
\draw[] (0.9375, 0.65625) rectangle (0.96875, 0.6875);% [-0.056005, 0]
\draw[] (0.96875, 0.625) rectangle (1, 0.65625);% [-0.0334617, 0]
\PrecisionAchieved{0.96875,0.625}{1,0.65625}{0.984375,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.625) rectangle (0.96875, 0.65625);% [-0.0270614, -0.0228941]
\PrecisionAchieved{0.9375,0.625}{0.96875,0.65625}{0.953125,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.90625, 0.65625) rectangle (0.9375, 0.6875);% [-0.0370912, -0.0353961]
\PrecisionAchieved{0.90625,0.65625}{0.9375,0.6875}{0.921875,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.65625) rectangle (0.90625, 0.6875);% [-0.0539678, -0.0525059]
\PrecisionAchieved{0.875,0.65625}{0.90625,0.6875}{0.890625,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.90625, 0.625) rectangle (0.9375, 0.65625);% [-0.051275, -0.0498579]
\PrecisionAchieved{0.90625,0.625}{0.9375,0.65625}{0.921875,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.625) rectangle (0.90625, 0.65625);% [-0.0745963, -0.0731945]
\PrecisionAchieved{0.875,0.625}{0.90625,0.65625}{0.890625,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.84375, 0.71875) rectangle (0.875, 0.75);% [-0.0255521, -0.0235068]
\PrecisionAchieved{0.84375,0.71875}{0.875,0.75}{0.859375,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.71875) rectangle (0.84375, 0.75);% [-0.0243226, -0.0219393]
\PrecisionAchieved{0.8125,0.71875}{0.84375,0.75}{0.828125,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.84375, 0.6875) rectangle (0.875, 0.71875);% [-0.0434626, -0.0416773]
\PrecisionAchieved{0.84375,0.6875}{0.875,0.71875}{0.859375,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.6875) rectangle (0.84375, 0.71875);% [-0.0449652, -0.0429422]
\PrecisionAchieved{0.8125,0.6875}{0.84375,0.71875}{0.828125,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.78125, 0.71875) rectangle (0.8125, 0.75);% [-0.0183931, -0.0153567]
\PrecisionAchieved{0.78125,0.71875}{0.8125,0.75}{0.796875,0.734375}{0.00625}
\draw[] (0.75, 0.71875) rectangle (0.78125, 0.75);% [-0.0254528, 0]
\PrecisionAchieved{0.75,0.71875}{0.78125,0.75}{0.765625,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.78125, 0.6875) rectangle (0.8125, 0.71875);% [-0.0398853, -0.037525]
\PrecisionAchieved{0.78125,0.6875}{0.8125,0.71875}{0.796875,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.75, 0.6875) rectangle (0.78125, 0.71875);% [-0.0284654, -0.0255542]
\PrecisionAchieved{0.75,0.6875}{0.78125,0.71875}{0.765625,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.625) rectangle (0.875, 0.6875);% [-0.0895606, -0.0760559]
\PrecisionAchieved{0.8125,0.625}{0.875,0.6875}{0.84375,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.625) rectangle (0.8125, 0.6875);% [-0.0886292, -0.0745694]
\PrecisionAchieved{0.75,0.625}{0.8125,0.6875}{0.78125,0.65625}{0.0125}
\draw[] (0.96875, 0.59375) rectangle (1, 0.625);% [-0.0352867, 0]
\PrecisionAchieved{0.96875,0.59375}{1,0.625}{0.984375,0.609375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.59375) rectangle (0.96875, 0.625);% [-0.0350878, -0.0318305]
\PrecisionAchieved{0.9375,0.59375}{0.96875,0.625}{0.953125,0.609375}{0.00625}
\draw[] (0.96875, 0.5625) rectangle (1, 0.59375);% [-0.0366166, 0]
\PrecisionAchieved{0.96875,0.5625}{1,0.59375}{0.984375,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.5625) rectangle (0.96875, 0.59375);% [-0.0442196, -0.0413198]
\PrecisionAchieved{0.9375,0.5625}{0.96875,0.59375}{0.953125,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.5625) rectangle (0.9375, 0.625);% [-0.0985275, -0.0852643]
\PrecisionAchieved{0.875,0.5625}{0.9375,0.625}{0.90625,0.59375}{0.0125}
\draw[] (0.96875, 0.53125) rectangle (1, 0.5625);% [-0.0374249, 0]
\PrecisionAchieved{0.96875,0.53125}{1,0.5625}{0.984375,0.546875}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.53125) rectangle (0.96875, 0.5625);% [-0.0537469, -0.0512044]
\PrecisionAchieved{0.9375,0.53125}{0.96875,0.5625}{0.953125,0.546875}{0.00625}
\draw[] (0.96875, 0.5) rectangle (1, 0.53125);% [-0.0376961, 0]
\PrecisionAchieved{0.96875,0.5}{1,0.53125}{0.984375,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.5) rectangle (0.96875, 0.53125);% [-0.0631646, -0.0610217]
\PrecisionAchieved{0.9375,0.5}{0.96875,0.53125}{0.953125,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.5) rectangle (0.9375, 0.5625);% [-0.136228, -0.121679]
\PrecisionAchieved{0.875,0.5}{0.9375,0.5625}{0.90625,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.5625) rectangle (0.875, 0.625);% [-0.14503, -0.132578]
\PrecisionAchieved{0.8125,0.5625}{0.875,0.625}{0.84375,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.5625) rectangle (0.8125, 0.625);% [-0.157796, -0.144785]
\PrecisionAchieved{0.75,0.5625}{0.8125,0.625}{0.78125,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.5) rectangle (0.875, 0.5625);% [-0.185228, -0.16844]
\PrecisionAchieved{0.8125,0.5}{0.875,0.5625}{0.84375,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.5) rectangle (0.8125, 0.5625);% [-0.191339, -0.17651]
\PrecisionAchieved{0.75,0.5}{0.8125,0.5625}{0.78125,0.53125}{0.0125}
\draw[] (0.6875, 0.6875) rectangle (0.75, 0.75);% [-0.0328859, 0]
\PrecisionAchieved{0.6875,0.6875}{0.75,0.75}{0.71875,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.65625, 0.71875) rectangle (0.6875, 0.75);% [-0.040695, -0.0376258]
\PrecisionAchieved{0.65625,0.71875}{0.6875,0.75}{0.671875,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.71875) rectangle (0.65625, 0.75);% [-0.0793242, -0.0771794]
\PrecisionAchieved{0.625,0.71875}{0.65625,0.75}{0.640625,0.734375}{0.00625}
\draw[] (0.65625, 0.6875) rectangle (0.6875, 0.71875);% [-0.0457006, 0]
\PrecisionAchieved{0.65625,0.6875}{0.6875,0.71875}{0.671875,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.6875) rectangle (0.65625, 0.71875);% [-0.0540898, -0.0506325]
\PrecisionAchieved{0.625,0.6875}{0.65625,0.71875}{0.640625,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.65625) rectangle (0.75, 0.6875);% [-0.040695, -0.0376258]
\PrecisionAchieved{0.71875,0.65625}{0.75,0.6875}{0.734375,0.671875}{0.00625}
\draw[] (0.6875, 0.65625) rectangle (0.71875, 0.6875);% [-0.0457006, 0]
\PrecisionAchieved{0.6875,0.65625}{0.71875,0.6875}{0.703125,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.625) rectangle (0.75, 0.65625);% [-0.0793242, -0.0771794]
\PrecisionAchieved{0.71875,0.625}{0.75,0.65625}{0.734375,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.625) rectangle (0.71875, 0.65625);% [-0.0540898, -0.0506325]
\PrecisionAchieved{0.6875,0.625}{0.71875,0.65625}{0.703125,0.640625}{0.00625}
\draw[] (0.65625, 0.65625) rectangle (0.6875, 0.6875);% [-0.0185805, 0]
\PrecisionAchieved{0.65625,0.65625}{0.6875,0.6875}{0.671875,0.671875}{0.00625}
\draw[] (0.625, 0.65625) rectangle (0.65625, 0.6875);% [-0.058991, 0]
\draw[] (0.65625, 0.625) rectangle (0.6875, 0.65625);% [-0.058991, 0]
\draw[] (0.625, 0.625) rectangle (0.65625, 0.65625);% [-0.0238312, 0]
\PrecisionAchieved{0.625,0.625}{0.65625,0.65625}{0.640625,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.6875) rectangle (0.625, 0.75);% [-0.141066, -0.123732]
\PrecisionAchieved{0.5625,0.6875}{0.625,0.75}{0.59375,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.6875) rectangle (0.5625, 0.75);% [-0.193587, -0.173249]
\PrecisionAchieved{0.5,0.6875}{0.5625,0.75}{0.53125,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.59375, 0.65625) rectangle (0.625, 0.6875);% [-0.0673359, -0.0635464]
\PrecisionAchieved{0.59375,0.65625}{0.625,0.6875}{0.609375,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.65625) rectangle (0.59375, 0.6875);% [-0.118051, -0.114501]
\PrecisionAchieved{0.5625,0.65625}{0.59375,0.6875}{0.578125,0.671875}{0.00625}
\draw[] (0.59375, 0.625) rectangle (0.625, 0.65625);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.5625, 0.625) rectangle (0.59375, 0.65625);% [-0.0792551, -0.0752509]
\PrecisionAchieved{0.5625,0.625}{0.59375,0.65625}{0.578125,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.625) rectangle (0.5625, 0.6875);% [-0.179181, -0.151183]
\PrecisionAchieved{0.5,0.625}{0.5625,0.6875}{0.53125,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.5625) rectangle (0.75, 0.625);% [-0.141066, -0.123732]
\PrecisionAchieved{0.6875,0.5625}{0.75,0.625}{0.71875,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.65625, 0.59375) rectangle (0.6875, 0.625);% [-0.0673359, -0.0635464]
\PrecisionAchieved{0.65625,0.59375}{0.6875,0.625}{0.671875,0.609375}{0.00625}
\draw[] (0.625, 0.59375) rectangle (0.65625, 0.625);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.65625, 0.5625) rectangle (0.6875, 0.59375);% [-0.118051, -0.114501]
\PrecisionAchieved{0.65625,0.5625}{0.6875,0.59375}{0.671875,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.5625) rectangle (0.65625, 0.59375);% [-0.0792551, -0.0752509]
\PrecisionAchieved{0.625,0.5625}{0.65625,0.59375}{0.640625,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.5) rectangle (0.75, 0.5625);% [-0.193587, -0.173249]
\PrecisionAchieved{0.6875,0.5}{0.75,0.5625}{0.71875,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.5) rectangle (0.6875, 0.5625);% [-0.179181, -0.151183]
\PrecisionAchieved{0.625,0.5}{0.6875,0.5625}{0.65625,0.53125}{0.0125}
\draw[] (0.59375, 0.59375) rectangle (0.625, 0.625);% [-0.0288048, 0]
\PrecisionAchieved{0.59375,0.59375}{0.625,0.625}{0.609375,0.609375}{0.00625}
\draw[] (0.5625, 0.59375) rectangle (0.59375, 0.625);% [-0.0823766, 0]
\draw[] (0.59375, 0.5625) rectangle (0.625, 0.59375);% [-0.0823766, 0]
\draw[] (0.5625, 0.5625) rectangle (0.59375, 0.59375);% [-0.0330265, 0]
\PrecisionAchieved{0.5625,0.5625}{0.59375,0.59375}{0.578125,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.53125, 0.59375) rectangle (0.5625, 0.625);% [-0.0888868, -0.0848121]
\PrecisionAchieved{0.53125,0.59375}{0.5625,0.625}{0.546875,0.609375}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.59375) rectangle (0.53125, 0.625);% [-0.1434, -0.13801]
\PrecisionAchieved{0.5,0.59375}{0.53125,0.625}{0.515625,0.609375}{0.00625}
\draw[] (0.53125, 0.5625) rectangle (0.5625, 0.59375);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.5, 0.5625) rectangle (0.53125, 0.59375);% [-0.0956646, -0.0914662]
\PrecisionAchieved{0.5,0.5625}{0.53125,0.59375}{0.515625,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.59375, 0.53125) rectangle (0.625, 0.5625);% [-0.0888868, -0.0848121]
\PrecisionAchieved{0.59375,0.53125}{0.625,0.5625}{0.609375,0.546875}{0.00625}
\draw[] (0.5625, 0.53125) rectangle (0.59375, 0.5625);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.59375, 0.5) rectangle (0.625, 0.53125);% [-0.1434, -0.13801]
\PrecisionAchieved{0.59375,0.5}{0.625,0.53125}{0.609375,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.5) rectangle (0.59375, 0.53125);% [-0.0956646, -0.0914662]
\PrecisionAchieved{0.5625,0.5}{0.59375,0.53125}{0.578125,0.515625}{0.00625}
\draw[] (0.53125, 0.53125) rectangle (0.5625, 0.5625);% [-0.0360884, 0]
\PrecisionAchieved{0.53125,0.53125}{0.5625,0.5625}{0.546875,0.546875}{0.00625}
\draw[] (0.5, 0.53125) rectangle (0.53125, 0.5625);% [-0.0957117, 0]
\draw[] (0.53125, 0.5) rectangle (0.5625, 0.53125);% [-0.0957117, 0]
\draw[] (0.5, 0.5) rectangle (0.53125, 0.53125);% [-0.0376961, 0]
\PrecisionAchieved{0.5,0.5}{0.53125,0.53125}{0.515625,0.515625}{0.00625}
\draw[] (0.46875, 0.96875) rectangle (0.5, 1);% [-0.0433027, 0]
\PrecisionAchieved{0.46875,0.96875}{0.5,1}{0.484375,0.984375}{0.00625}
\draw[] (0.4375, 0.96875) rectangle (0.46875, 1);% [-0.0485429, 0]
\PrecisionAchieved{0.4375,0.96875}{0.46875,1}{0.453125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.46875, 0.9375) rectangle (0.5, 0.96875);% [-0.0720375, -0.0702338]
\PrecisionAchieved{0.46875,0.9375}{0.5,0.96875}{0.484375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.9375) rectangle (0.46875, 0.96875);% [-0.0802649, -0.0780441]
\PrecisionAchieved{0.4375,0.9375}{0.46875,0.96875}{0.453125,0.953125}{0.00625}
\draw[] (0.40625, 0.96875) rectangle (0.4375, 1);% [-0.0528588, 0]
\draw[] (0.375, 0.96875) rectangle (0.40625, 1);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.40625, 0.9375) rectangle (0.4375, 0.96875);% [-0.0871423, -0.0843889]
\PrecisionAchieved{0.40625,0.9375}{0.4375,0.96875}{0.421875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.9375) rectangle (0.40625, 0.96875);% [-0.092245, -0.0890725]
\PrecisionAchieved{0.375,0.9375}{0.40625,0.96875}{0.390625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.875) rectangle (0.5, 0.9375);% [-0.167308, -0.145382]
\PrecisionAchieved{0.4375,0.875}{0.5,0.9375}{0.46875,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.875) rectangle (0.4375, 0.9375);% [-0.185555, -0.156982]
\PrecisionAchieved{0.375,0.875}{0.4375,0.9375}{0.40625,0.90625}{0.0125}
\draw[] (0.34375, 0.96875) rectangle (0.375, 1);% [-0.057785, 0]
\draw[] (0.3125, 0.96875) rectangle (0.34375, 1);% [-0.058056, 0]
\draw[fill=\HigherOrderColor] (0.34375, 0.9375) rectangle (0.375, 0.96875);% [-0.0953028, -0.0918834]
\PrecisionAchieved{0.34375,0.9375}{0.375,0.96875}{0.359375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.9375) rectangle (0.34375, 0.96875);% [-0.0961115, -0.0926563]
\PrecisionAchieved{0.3125,0.9375}{0.34375,0.96875}{0.328125,0.953125}{0.00625}
\draw[] (0.28125, 0.96875) rectangle (0.3125, 1);% [-0.0567321, 0]
\draw[] (0.25, 0.96875) rectangle (0.28125, 1);% [-0.0537898, 0]
\draw[fill=\HigherOrderColor] (0.28125, 0.9375) rectangle (0.3125, 0.96875);% [-0.0945283, -0.0912507]
\PrecisionAchieved{0.28125,0.9375}{0.3125,0.96875}{0.296875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.9375) rectangle (0.28125, 0.96875);% [-0.0904515, -0.0875645]
\PrecisionAchieved{0.25,0.9375}{0.28125,0.96875}{0.265625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.875) rectangle (0.375, 0.9375);% [-0.191703, -0.161008]
\PrecisionAchieved{0.3125,0.875}{0.375,0.9375}{0.34375,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.875) rectangle (0.3125, 0.9375);% [-0.188379, -0.160083]
\PrecisionAchieved{0.25,0.875}{0.3125,0.9375}{0.28125,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.8125) rectangle (0.5, 0.875);% [-0.192313, -0.171674]
\PrecisionAchieved{0.4375,0.8125}{0.5,0.875}{0.46875,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.8125) rectangle (0.4375, 0.875);% [-0.17443, -0.150596]
\PrecisionAchieved{0.375,0.8125}{0.4375,0.875}{0.40625,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.75) rectangle (0.5, 0.8125);% [-0.159889, -0.144234]
\PrecisionAchieved{0.4375,0.75}{0.5,0.8125}{0.46875,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.75) rectangle (0.4375, 0.8125);% [-0.0851179, -0.0668076]
\PrecisionAchieved{0.375,0.75}{0.4375,0.8125}{0.40625,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.8125) rectangle (0.375, 0.875);% [-0.158666, -0.130749]
\PrecisionAchieved{0.3125,0.8125}{0.375,0.875}{0.34375,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.8125) rectangle (0.3125, 0.875);% [-0.163549, -0.137671]
\PrecisionAchieved{0.25,0.8125}{0.3125,0.875}{0.28125,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.75) rectangle (0.375, 0.8125);% [-0.0266774, -0.00338735]
\PrecisionAchieved{0.3125,0.75}{0.375,0.8125}{0.34375,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.75) rectangle (0.3125, 0.8125);% [-0.0332953, -0.0128698]
\PrecisionAchieved{0.25,0.75}{0.3125,0.8125}{0.28125,0.78125}{0.0125}
\draw[] (0.21875, 0.96875) rectangle (0.25, 1);% [-0.0498517, 0]
\PrecisionAchieved{0.21875,0.96875}{0.25,1}{0.234375,0.984375}{0.00625}
\draw[] (0.1875, 0.96875) rectangle (0.21875, 1);% [-0.0449984, 0]
\PrecisionAchieved{0.1875,0.96875}{0.21875,1}{0.203125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.21875, 0.9375) rectangle (0.25, 0.96875);% [-0.0838951, -0.0814878]
\PrecisionAchieved{0.21875,0.9375}{0.25,0.96875}{0.234375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.9375) rectangle (0.21875, 0.96875);% [-0.0749884, -0.0729724]
\PrecisionAchieved{0.1875,0.9375}{0.21875,0.96875}{0.203125,0.953125}{0.00625}
\draw[] (0.15625, 0.96875) rectangle (0.1875, 1);% [-0.0388125, 0]
\PrecisionAchieved{0.15625,0.96875}{0.1875,1}{0.171875,0.984375}{0.00625}
\draw[] (0.125, 0.96875) rectangle (0.15625, 1);% [-0.0315693, 0]
\PrecisionAchieved{0.125,0.96875}{0.15625,1}{0.140625,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.15625, 0.9375) rectangle (0.1875, 0.96875);% [-0.0641254, -0.0619946]
\PrecisionAchieved{0.15625,0.9375}{0.1875,0.96875}{0.171875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.9375) rectangle (0.15625, 0.96875);% [-0.0513779, -0.0492824]
\PrecisionAchieved{0.125,0.9375}{0.15625,0.96875}{0.140625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.875) rectangle (0.25, 0.9375);% [-0.173944, -0.14974]
\PrecisionAchieved{0.1875,0.875}{0.25,0.9375}{0.21875,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.875) rectangle (0.1875, 0.9375);% [-0.139872, -0.121811]
\PrecisionAchieved{0.125,0.875}{0.1875,0.9375}{0.15625,0.90625}{0.0125}
\draw[] (0.09375, 0.96875) rectangle (0.125, 1);% [-0.0236772, 0]
\PrecisionAchieved{0.09375,0.96875}{0.125,1}{0.109375,0.984375}{0.00625}
\draw[] (0.0625, 0.96875) rectangle (0.09375, 1);% [-0.015697, 0]
\PrecisionAchieved{0.0625,0.96875}{0.09375,1}{0.078125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.9375) rectangle (0.125, 0.96875);% [-0.0375199, -0.0354476]
\PrecisionAchieved{0.09375,0.9375}{0.125,0.96875}{0.109375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.9375) rectangle (0.09375, 0.96875);% [-0.0235946, -0.0215828]
\PrecisionAchieved{0.0625,0.9375}{0.09375,0.96875}{0.078125,0.953125}{0.00625}
\draw[] (0, 0.9375) rectangle (0.0625, 1);% [-0.0250627, 0]
\PrecisionAchieved{0,0.9375}{0.0625,1}{0.03125,0.96875}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.875) rectangle (0.125, 0.9375);% [-0.0816588, -0.0721156]
\PrecisionAchieved{0.0625,0.875}{0.125,0.9375}{0.09375,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.90625) rectangle (0.0625, 0.9375);% [-0.0235946, -0.0215828]
\PrecisionAchieved{0.03125,0.90625}{0.0625,0.9375}{0.046875,0.921875}{0.00625}
\draw[] (0, 0.90625) rectangle (0.03125, 0.9375);% [-0.015697, 0]
\PrecisionAchieved{0,0.90625}{0.03125,0.9375}{0.015625,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.875) rectangle (0.0625, 0.90625);% [-0.0375199, -0.0354476]
\PrecisionAchieved{0.03125,0.875}{0.0625,0.90625}{0.046875,0.890625}{0.00625}
\draw[] (0, 0.875) rectangle (0.03125, 0.90625);% [-0.0236772, 0]
\PrecisionAchieved{0,0.875}{0.03125,0.90625}{0.015625,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.8125) rectangle (0.25, 0.875);% [-0.186856, -0.162723]
\PrecisionAchieved{0.1875,0.8125}{0.25,0.875}{0.21875,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.8125) rectangle (0.1875, 0.875);% [-0.193531, -0.169053]
\PrecisionAchieved{0.125,0.8125}{0.1875,0.875}{0.15625,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.75) rectangle (0.25, 0.8125);% [-0.106601, -0.091481]
\PrecisionAchieved{0.1875,0.75}{0.25,0.8125}{0.21875,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.75) rectangle (0.1875, 0.8125);% [-0.186856, -0.162723]
\PrecisionAchieved{0.125,0.75}{0.1875,0.8125}{0.15625,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.8125) rectangle (0.125, 0.875);% [-0.139872, -0.121811]
\PrecisionAchieved{0.0625,0.8125}{0.125,0.875}{0.09375,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.84375) rectangle (0.0625, 0.875);% [-0.0513779, -0.0492824]
\PrecisionAchieved{0.03125,0.84375}{0.0625,0.875}{0.046875,0.859375}{0.00625}
\draw[] (0, 0.84375) rectangle (0.03125, 0.875);% [-0.0315693, 0]
\PrecisionAchieved{0,0.84375}{0.03125,0.875}{0.015625,0.859375}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.8125) rectangle (0.0625, 0.84375);% [-0.0641254, -0.0619946]
\PrecisionAchieved{0.03125,0.8125}{0.0625,0.84375}{0.046875,0.828125}{0.00625}
\draw[] (0, 0.8125) rectangle (0.03125, 0.84375);% [-0.0388125, 0]
\PrecisionAchieved{0,0.8125}{0.03125,0.84375}{0.015625,0.828125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.75) rectangle (0.125, 0.8125);% [-0.173944, -0.14974]
\PrecisionAchieved{0.0625,0.75}{0.125,0.8125}{0.09375,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.78125) rectangle (0.0625, 0.8125);% [-0.0749884, -0.0729724]
\PrecisionAchieved{0.03125,0.78125}{0.0625,0.8125}{0.046875,0.796875}{0.00625}
\draw[] (0, 0.78125) rectangle (0.03125, 0.8125);% [-0.0449984, 0]
\PrecisionAchieved{0,0.78125}{0.03125,0.8125}{0.015625,0.796875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.75) rectangle (0.0625, 0.78125);% [-0.0838951, -0.0814878]
\PrecisionAchieved{0.03125,0.75}{0.0625,0.78125}{0.046875,0.765625}{0.00625}
\draw[] (0, 0.75) rectangle (0.03125, 0.78125);% [-0.0498517, 0]
\PrecisionAchieved{0,0.75}{0.03125,0.78125}{0.015625,0.765625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.6875) rectangle (0.5, 0.75);% [-0.154417, -0.134001]
\PrecisionAchieved{0.4375,0.6875}{0.5,0.75}{0.46875,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.6875) rectangle (0.4375, 0.75);% [-0.0422331, -0.019924]
\PrecisionAchieved{0.375,0.6875}{0.4375,0.75}{0.40625,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.625) rectangle (0.5, 0.6875);% [-0.187034, -0.159687]
\PrecisionAchieved{0.4375,0.625}{0.5,0.6875}{0.46875,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.625) rectangle (0.4375, 0.6875);% [-0.0909476, -0.0666031]
\PrecisionAchieved{0.375,0.625}{0.4375,0.6875}{0.40625,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.6875) rectangle (0.375, 0.75);% [0.0571403, 0.0883857]
\PrecisionAchieved{0.3125,0.6875}{0.375,0.75}{0.34375,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.6875) rectangle (0.3125, 0.75);% [0.0654339, 0.0948421]
\PrecisionAchieved{0.25,0.6875}{0.3125,0.75}{0.28125,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.625) rectangle (0.375, 0.6875);% [0.0230582, 0.0551483]
\PrecisionAchieved{0.3125,0.625}{0.375,0.6875}{0.34375,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.625) rectangle (0.3125, 0.6875);% [0.0571403, 0.0883857]
\PrecisionAchieved{0.25,0.625}{0.3125,0.6875}{0.28125,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.5625) rectangle (0.5, 0.625);% [-0.194365, -0.160213]
\PrecisionAchieved{0.4375,0.5625}{0.5,0.625}{0.46875,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.5625) rectangle (0.4375, 0.625);% [-0.177107, -0.14534]
\PrecisionAchieved{0.375,0.5625}{0.4375,0.625}{0.40625,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.46875, 0.53125) rectangle (0.5, 0.5625);% [-0.099267, -0.0947523]
\PrecisionAchieved{0.46875,0.53125}{0.5,0.5625}{0.484375,0.546875}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.53125) rectangle (0.46875, 0.5625);% [-0.151727, -0.145493]
\PrecisionAchieved{0.4375,0.53125}{0.46875,0.5625}{0.453125,0.546875}{0.00625}
\draw[] (0.46875, 0.5) rectangle (0.5, 0.53125);% [-0.0980218, 0]
\draw[fill=\HigherOrderColor] (0.4375, 0.5) rectangle (0.46875, 0.53125);% [-0.099267, -0.0947523]
\PrecisionAchieved{0.4375,0.5}{0.46875,0.53125}{0.453125,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.5) rectangle (0.4375, 0.5625);% [-0.194365, -0.160213]
\PrecisionAchieved{0.375,0.5}{0.4375,0.5625}{0.40625,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.5625) rectangle (0.375, 0.625);% [-0.0909476, -0.0666031]
\PrecisionAchieved{0.3125,0.5625}{0.375,0.625}{0.34375,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.5625) rectangle (0.3125, 0.625);% [-0.0422331, -0.019924]
\PrecisionAchieved{0.25,0.5625}{0.3125,0.625}{0.28125,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.5) rectangle (0.375, 0.5625);% [-0.187034, -0.159687]
\PrecisionAchieved{0.3125,0.5}{0.375,0.5625}{0.34375,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.5) rectangle (0.3125, 0.5625);% [-0.154417, -0.134001]
\PrecisionAchieved{0.25,0.5}{0.3125,0.5625}{0.28125,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.6875) rectangle (0.25, 0.75);% [-0.0332953, -0.0128698]
\PrecisionAchieved{0.1875,0.6875}{0.25,0.75}{0.21875,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.6875) rectangle (0.1875, 0.75);% [-0.163549, -0.137671]
\PrecisionAchieved{0.125,0.6875}{0.1875,0.75}{0.15625,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.625) rectangle (0.25, 0.6875);% [-0.0266774, -0.00338735]
\PrecisionAchieved{0.1875,0.625}{0.25,0.6875}{0.21875,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.625) rectangle (0.1875, 0.6875);% [-0.158666, -0.130749]
\PrecisionAchieved{0.125,0.625}{0.1875,0.6875}{0.15625,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.6875) rectangle (0.125, 0.75);% [-0.188379, -0.160083]
\PrecisionAchieved{0.0625,0.6875}{0.125,0.75}{0.09375,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.71875) rectangle (0.0625, 0.75);% [-0.0904515, -0.0875645]
\PrecisionAchieved{0.03125,0.71875}{0.0625,0.75}{0.046875,0.734375}{0.00625}
\draw[] (0, 0.71875) rectangle (0.03125, 0.75);% [-0.0537898, 0]
\draw[fill=\HigherOrderColor] (0.03125, 0.6875) rectangle (0.0625, 0.71875);% [-0.0945283, -0.0912507]
\PrecisionAchieved{0.03125,0.6875}{0.0625,0.71875}{0.046875,0.703125}{0.00625}
\draw[] (0, 0.6875) rectangle (0.03125, 0.71875);% [-0.0567321, 0]
\draw[fill=\HigherOrderColor] (0.0625, 0.625) rectangle (0.125, 0.6875);% [-0.191703, -0.161008]
\PrecisionAchieved{0.0625,0.625}{0.125,0.6875}{0.09375,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.65625) rectangle (0.0625, 0.6875);% [-0.0961115, -0.0926563]
\PrecisionAchieved{0.03125,0.65625}{0.0625,0.6875}{0.046875,0.671875}{0.00625}
\draw[] (0, 0.65625) rectangle (0.03125, 0.6875);% [-0.058056, 0]
\draw[fill=\HigherOrderColor] (0.03125, 0.625) rectangle (0.0625, 0.65625);% [-0.0953028, -0.0918834]
\PrecisionAchieved{0.03125,0.625}{0.0625,0.65625}{0.046875,0.640625}{0.00625}
\draw[] (0, 0.625) rectangle (0.03125, 0.65625);% [-0.057785, 0]
\draw[fill=\HigherOrderColor] (0.1875, 0.5625) rectangle (0.25, 0.625);% [-0.0851179, -0.0668076]
\PrecisionAchieved{0.1875,0.5625}{0.25,0.625}{0.21875,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.5625) rectangle (0.1875, 0.625);% [-0.17443, -0.150596]
\PrecisionAchieved{0.125,0.5625}{0.1875,0.625}{0.15625,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.5) rectangle (0.25, 0.5625);% [-0.159889, -0.144234]
\PrecisionAchieved{0.1875,0.5}{0.25,0.5625}{0.21875,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.5) rectangle (0.1875, 0.5625);% [-0.192313, -0.171674]
\PrecisionAchieved{0.125,0.5}{0.1875,0.5625}{0.15625,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.5625) rectangle (0.125, 0.625);% [-0.185555, -0.156982]
\PrecisionAchieved{0.0625,0.5625}{0.125,0.625}{0.09375,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.59375) rectangle (0.0625, 0.625);% [-0.092245, -0.0890725]
\PrecisionAchieved{0.03125,0.59375}{0.0625,0.625}{0.046875,0.609375}{0.00625}
\draw[] (0, 0.59375) rectangle (0.03125, 0.625);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.03125, 0.5625) rectangle (0.0625, 0.59375);% [-0.0871423, -0.0843889]
\PrecisionAchieved{0.03125,0.5625}{0.0625,0.59375}{0.046875,0.578125}{0.00625}
\draw[] (0, 0.5625) rectangle (0.03125, 0.59375);% [-0.0528588, 0]
\draw[fill=\HigherOrderColor] (0.0625, 0.5) rectangle (0.125, 0.5625);% [-0.167308, -0.145382]
\PrecisionAchieved{0.0625,0.5}{0.125,0.5625}{0.09375,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.53125) rectangle (0.0625, 0.5625);% [-0.0802649, -0.0780441]
\PrecisionAchieved{0.03125,0.53125}{0.0625,0.5625}{0.046875,0.546875}{0.00625}
\draw[] (0, 0.53125) rectangle (0.03125, 0.5625);% [-0.0485429, 0]
\PrecisionAchieved{0,0.53125}{0.03125,0.5625}{0.015625,0.546875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.5) rectangle (0.0625, 0.53125);% [-0.0720375, -0.0702338]
\PrecisionAchieved{0.03125,0.5}{0.0625,0.53125}{0.046875,0.515625}{0.00625}
\draw[] (0, 0.5) rectangle (0.03125, 0.53125);% [-0.0433027, 0]
\PrecisionAchieved{0,0.5}{0.03125,0.53125}{0.015625,0.515625}{0.00625}
\draw[] (0.96875, 0.46875) rectangle (1, 0.5);% [-0.0433027, 0]
\PrecisionAchieved{0.96875,0.46875}{1,0.5}{0.984375,0.484375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.46875) rectangle (0.96875, 0.5);% [-0.0720375, -0.0702338]
\PrecisionAchieved{0.9375,0.46875}{0.96875,0.5}{0.953125,0.484375}{0.00625}
\draw[] (0.96875, 0.4375) rectangle (1, 0.46875);% [-0.0485429, 0]
\PrecisionAchieved{0.96875,0.4375}{1,0.46875}{0.984375,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.4375) rectangle (0.96875, 0.46875);% [-0.0802649, -0.0780441]
\PrecisionAchieved{0.9375,0.4375}{0.96875,0.46875}{0.953125,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.4375) rectangle (0.9375, 0.5);% [-0.167308, -0.145382]
\PrecisionAchieved{0.875,0.4375}{0.9375,0.5}{0.90625,0.46875}{0.0125}
\draw[] (0.96875, 0.40625) rectangle (1, 0.4375);% [-0.0528588, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.40625) rectangle (0.96875, 0.4375);% [-0.0871423, -0.0843889]
\PrecisionAchieved{0.9375,0.40625}{0.96875,0.4375}{0.953125,0.421875}{0.00625}
\draw[] (0.96875, 0.375) rectangle (1, 0.40625);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.375) rectangle (0.96875, 0.40625);% [-0.092245, -0.0890725]
\PrecisionAchieved{0.9375,0.375}{0.96875,0.40625}{0.953125,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.375) rectangle (0.9375, 0.4375);% [-0.185555, -0.156982]
\PrecisionAchieved{0.875,0.375}{0.9375,0.4375}{0.90625,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.4375) rectangle (0.875, 0.5);% [-0.192313, -0.171674]
\PrecisionAchieved{0.8125,0.4375}{0.875,0.5}{0.84375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.4375) rectangle (0.8125, 0.5);% [-0.159889, -0.144234]
\PrecisionAchieved{0.75,0.4375}{0.8125,0.5}{0.78125,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.375) rectangle (0.875, 0.4375);% [-0.17443, -0.150596]
\PrecisionAchieved{0.8125,0.375}{0.875,0.4375}{0.84375,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.375) rectangle (0.8125, 0.4375);% [-0.0851179, -0.0668076]
\PrecisionAchieved{0.75,0.375}{0.8125,0.4375}{0.78125,0.40625}{0.0125}
\draw[] (0.96875, 0.34375) rectangle (1, 0.375);% [-0.057785, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.34375) rectangle (0.96875, 0.375);% [-0.0953028, -0.0918834]
\PrecisionAchieved{0.9375,0.34375}{0.96875,0.375}{0.953125,0.359375}{0.00625}
\draw[] (0.96875, 0.3125) rectangle (1, 0.34375);% [-0.058056, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.3125) rectangle (0.96875, 0.34375);% [-0.0961115, -0.0926563]
\PrecisionAchieved{0.9375,0.3125}{0.96875,0.34375}{0.953125,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.3125) rectangle (0.9375, 0.375);% [-0.191703, -0.161008]
\PrecisionAchieved{0.875,0.3125}{0.9375,0.375}{0.90625,0.34375}{0.0125}
\draw[] (0.96875, 0.28125) rectangle (1, 0.3125);% [-0.0567321, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.28125) rectangle (0.96875, 0.3125);% [-0.0945283, -0.0912507]
\PrecisionAchieved{0.9375,0.28125}{0.96875,0.3125}{0.953125,0.296875}{0.00625}
\draw[] (0.96875, 0.25) rectangle (1, 0.28125);% [-0.0537898, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.25) rectangle (0.96875, 0.28125);% [-0.0904515, -0.0875645]
\PrecisionAchieved{0.9375,0.25}{0.96875,0.28125}{0.953125,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.25) rectangle (0.9375, 0.3125);% [-0.188379, -0.160083]
\PrecisionAchieved{0.875,0.25}{0.9375,0.3125}{0.90625,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.3125) rectangle (0.875, 0.375);% [-0.158666, -0.130749]
\PrecisionAchieved{0.8125,0.3125}{0.875,0.375}{0.84375,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.3125) rectangle (0.8125, 0.375);% [-0.0266774, -0.00338735]
\PrecisionAchieved{0.75,0.3125}{0.8125,0.375}{0.78125,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.25) rectangle (0.875, 0.3125);% [-0.163549, -0.137671]
\PrecisionAchieved{0.8125,0.25}{0.875,0.3125}{0.84375,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.25) rectangle (0.8125, 0.3125);% [-0.0332953, -0.0128698]
\PrecisionAchieved{0.75,0.25}{0.8125,0.3125}{0.78125,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.4375) rectangle (0.75, 0.5);% [-0.154417, -0.134001]
\PrecisionAchieved{0.6875,0.4375}{0.75,0.5}{0.71875,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.4375) rectangle (0.6875, 0.5);% [-0.187034, -0.159687]
\PrecisionAchieved{0.625,0.4375}{0.6875,0.5}{0.65625,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.375) rectangle (0.75, 0.4375);% [-0.0422331, -0.019924]
\PrecisionAchieved{0.6875,0.375}{0.75,0.4375}{0.71875,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.375) rectangle (0.6875, 0.4375);% [-0.0909476, -0.0666031]
\PrecisionAchieved{0.625,0.375}{0.6875,0.4375}{0.65625,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.4375) rectangle (0.625, 0.5);% [-0.194365, -0.160213]
\PrecisionAchieved{0.5625,0.4375}{0.625,0.5}{0.59375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.53125, 0.46875) rectangle (0.5625, 0.5);% [-0.099267, -0.0947523]
\PrecisionAchieved{0.53125,0.46875}{0.5625,0.5}{0.546875,0.484375}{0.00625}
\draw[] (0.5, 0.46875) rectangle (0.53125, 0.5);% [-0.0980218, 0]
\draw[fill=\HigherOrderColor] (0.53125, 0.4375) rectangle (0.5625, 0.46875);% [-0.151727, -0.145493]
\PrecisionAchieved{0.53125,0.4375}{0.5625,0.46875}{0.546875,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.4375) rectangle (0.53125, 0.46875);% [-0.099267, -0.0947523]
\PrecisionAchieved{0.5,0.4375}{0.53125,0.46875}{0.515625,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.375) rectangle (0.625, 0.4375);% [-0.177107, -0.14534]
\PrecisionAchieved{0.5625,0.375}{0.625,0.4375}{0.59375,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.375) rectangle (0.5625, 0.4375);% [-0.194365, -0.160213]
\PrecisionAchieved{0.5,0.375}{0.5625,0.4375}{0.53125,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.3125) rectangle (0.75, 0.375);% [0.0571403, 0.0883857]
\PrecisionAchieved{0.6875,0.3125}{0.75,0.375}{0.71875,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.3125) rectangle (0.6875, 0.375);% [0.0230582, 0.0551483]
\PrecisionAchieved{0.625,0.3125}{0.6875,0.375}{0.65625,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.25) rectangle (0.75, 0.3125);% [0.0654339, 0.0948421]
\PrecisionAchieved{0.6875,0.25}{0.75,0.3125}{0.71875,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.25) rectangle (0.6875, 0.3125);% [0.0571403, 0.0883857]
\PrecisionAchieved{0.625,0.25}{0.6875,0.3125}{0.65625,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.3125) rectangle (0.625, 0.375);% [-0.0909476, -0.0666031]
\PrecisionAchieved{0.5625,0.3125}{0.625,0.375}{0.59375,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.3125) rectangle (0.5625, 0.375);% [-0.187034, -0.159687]
\PrecisionAchieved{0.5,0.3125}{0.5625,0.375}{0.53125,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.25) rectangle (0.625, 0.3125);% [-0.0422331, -0.019924]
\PrecisionAchieved{0.5625,0.25}{0.625,0.3125}{0.59375,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.25) rectangle (0.5625, 0.3125);% [-0.154417, -0.134001]
\PrecisionAchieved{0.5,0.25}{0.5625,0.3125}{0.53125,0.28125}{0.0125}
\draw[] (0.96875, 0.21875) rectangle (1, 0.25);% [-0.0498517, 0]
\PrecisionAchieved{0.96875,0.21875}{1,0.25}{0.984375,0.234375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.21875) rectangle (0.96875, 0.25);% [-0.0838951, -0.0814878]
\PrecisionAchieved{0.9375,0.21875}{0.96875,0.25}{0.953125,0.234375}{0.00625}
\draw[] (0.96875, 0.1875) rectangle (1, 0.21875);% [-0.0449984, 0]
\PrecisionAchieved{0.96875,0.1875}{1,0.21875}{0.984375,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.1875) rectangle (0.96875, 0.21875);% [-0.0749884, -0.0729724]
\PrecisionAchieved{0.9375,0.1875}{0.96875,0.21875}{0.953125,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.1875) rectangle (0.9375, 0.25);% [-0.173944, -0.14974]
\PrecisionAchieved{0.875,0.1875}{0.9375,0.25}{0.90625,0.21875}{0.0125}
\draw[] (0.96875, 0.15625) rectangle (1, 0.1875);% [-0.0388125, 0]
\PrecisionAchieved{0.96875,0.15625}{1,0.1875}{0.984375,0.171875}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.15625) rectangle (0.96875, 0.1875);% [-0.0641254, -0.0619946]
\PrecisionAchieved{0.9375,0.15625}{0.96875,0.1875}{0.953125,0.171875}{0.00625}
\draw[] (0.96875, 0.125) rectangle (1, 0.15625);% [-0.0315693, 0]
\PrecisionAchieved{0.96875,0.125}{1,0.15625}{0.984375,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.125) rectangle (0.96875, 0.15625);% [-0.0513779, -0.0492824]
\PrecisionAchieved{0.9375,0.125}{0.96875,0.15625}{0.953125,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.125) rectangle (0.9375, 0.1875);% [-0.139872, -0.121811]
\PrecisionAchieved{0.875,0.125}{0.9375,0.1875}{0.90625,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.1875) rectangle (0.875, 0.25);% [-0.186856, -0.162723]
\PrecisionAchieved{0.8125,0.1875}{0.875,0.25}{0.84375,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.1875) rectangle (0.8125, 0.25);% [-0.106601, -0.091481]
\PrecisionAchieved{0.75,0.1875}{0.8125,0.25}{0.78125,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.125) rectangle (0.875, 0.1875);% [-0.193531, -0.169053]
\PrecisionAchieved{0.8125,0.125}{0.875,0.1875}{0.84375,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.125) rectangle (0.8125, 0.1875);% [-0.186856, -0.162723]
\PrecisionAchieved{0.75,0.125}{0.8125,0.1875}{0.78125,0.15625}{0.0125}
\draw[] (0.96875, 0.09375) rectangle (1, 0.125);% [-0.0236772, 0]
\PrecisionAchieved{0.96875,0.09375}{1,0.125}{0.984375,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.09375) rectangle (0.96875, 0.125);% [-0.0375199, -0.0354476]
\PrecisionAchieved{0.9375,0.09375}{0.96875,0.125}{0.953125,0.109375}{0.00625}
\draw[] (0.96875, 0.0625) rectangle (1, 0.09375);% [-0.015697, 0]
\PrecisionAchieved{0.96875,0.0625}{1,0.09375}{0.984375,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.0625) rectangle (0.96875, 0.09375);% [-0.0235946, -0.0215828]
\PrecisionAchieved{0.9375,0.0625}{0.96875,0.09375}{0.953125,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.0625) rectangle (0.9375, 0.125);% [-0.0816588, -0.0721156]
\PrecisionAchieved{0.875,0.0625}{0.9375,0.125}{0.90625,0.09375}{0.0125}
\draw[] (0.9375, 0) rectangle (1, 0.0625);% [-0.0250627, 0]
\PrecisionAchieved{0.9375,0}{1,0.0625}{0.96875,0.03125}{0.0125}
\draw[fill=\HigherOrderColor] (0.90625, 0.03125) rectangle (0.9375, 0.0625);% [-0.0235946, -0.0215828]
\PrecisionAchieved{0.90625,0.03125}{0.9375,0.0625}{0.921875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.03125) rectangle (0.90625, 0.0625);% [-0.0375199, -0.0354476]
\PrecisionAchieved{0.875,0.03125}{0.90625,0.0625}{0.890625,0.046875}{0.00625}
\draw[] (0.90625, 0) rectangle (0.9375, 0.03125);% [-0.015697, 0]
\PrecisionAchieved{0.90625,0}{0.9375,0.03125}{0.921875,0.015625}{0.00625}
\draw[] (0.875, 0) rectangle (0.90625, 0.03125);% [-0.0236772, 0]
\PrecisionAchieved{0.875,0}{0.90625,0.03125}{0.890625,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.0625) rectangle (0.875, 0.125);% [-0.139872, -0.121811]
\PrecisionAchieved{0.8125,0.0625}{0.875,0.125}{0.84375,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.0625) rectangle (0.8125, 0.125);% [-0.173944, -0.14974]
\PrecisionAchieved{0.75,0.0625}{0.8125,0.125}{0.78125,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.84375, 0.03125) rectangle (0.875, 0.0625);% [-0.0513779, -0.0492824]
\PrecisionAchieved{0.84375,0.03125}{0.875,0.0625}{0.859375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.03125) rectangle (0.84375, 0.0625);% [-0.0641254, -0.0619946]
\PrecisionAchieved{0.8125,0.03125}{0.84375,0.0625}{0.828125,0.046875}{0.00625}
\draw[] (0.84375, 0) rectangle (0.875, 0.03125);% [-0.0315693, 0]
\PrecisionAchieved{0.84375,0}{0.875,0.03125}{0.859375,0.015625}{0.00625}
\draw[] (0.8125, 0) rectangle (0.84375, 0.03125);% [-0.0388125, 0]
\PrecisionAchieved{0.8125,0}{0.84375,0.03125}{0.828125,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.78125, 0.03125) rectangle (0.8125, 0.0625);% [-0.0749884, -0.0729724]
\PrecisionAchieved{0.78125,0.03125}{0.8125,0.0625}{0.796875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.75, 0.03125) rectangle (0.78125, 0.0625);% [-0.0838951, -0.0814878]
\PrecisionAchieved{0.75,0.03125}{0.78125,0.0625}{0.765625,0.046875}{0.00625}
\draw[] (0.78125, 0) rectangle (0.8125, 0.03125);% [-0.0449984, 0]
\PrecisionAchieved{0.78125,0}{0.8125,0.03125}{0.796875,0.015625}{0.00625}
\draw[] (0.75, 0) rectangle (0.78125, 0.03125);% [-0.0498517, 0]
\PrecisionAchieved{0.75,0}{0.78125,0.03125}{0.765625,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.1875) rectangle (0.75, 0.25);% [-0.0332953, -0.0128698]
\PrecisionAchieved{0.6875,0.1875}{0.75,0.25}{0.71875,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.1875) rectangle (0.6875, 0.25);% [-0.0266774, -0.00338735]
\PrecisionAchieved{0.625,0.1875}{0.6875,0.25}{0.65625,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.125) rectangle (0.75, 0.1875);% [-0.163549, -0.137671]
\PrecisionAchieved{0.6875,0.125}{0.75,0.1875}{0.71875,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.125) rectangle (0.6875, 0.1875);% [-0.158666, -0.130749]
\PrecisionAchieved{0.625,0.125}{0.6875,0.1875}{0.65625,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.1875) rectangle (0.625, 0.25);% [-0.0851179, -0.0668076]
\PrecisionAchieved{0.5625,0.1875}{0.625,0.25}{0.59375,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.1875) rectangle (0.5625, 0.25);% [-0.159889, -0.144234]
\PrecisionAchieved{0.5,0.1875}{0.5625,0.25}{0.53125,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.125) rectangle (0.625, 0.1875);% [-0.17443, -0.150596]
\PrecisionAchieved{0.5625,0.125}{0.625,0.1875}{0.59375,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.125) rectangle (0.5625, 0.1875);% [-0.192313, -0.171674]
\PrecisionAchieved{0.5,0.125}{0.5625,0.1875}{0.53125,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.0625) rectangle (0.75, 0.125);% [-0.188379, -0.160083]
\PrecisionAchieved{0.6875,0.0625}{0.75,0.125}{0.71875,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.0625) rectangle (0.6875, 0.125);% [-0.191703, -0.161008]
\PrecisionAchieved{0.625,0.0625}{0.6875,0.125}{0.65625,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.71875, 0.03125) rectangle (0.75, 0.0625);% [-0.0904515, -0.0875645]
\PrecisionAchieved{0.71875,0.03125}{0.75,0.0625}{0.734375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.03125) rectangle (0.71875, 0.0625);% [-0.0945283, -0.0912507]
\PrecisionAchieved{0.6875,0.03125}{0.71875,0.0625}{0.703125,0.046875}{0.00625}
\draw[] (0.71875, 0) rectangle (0.75, 0.03125);% [-0.0537898, 0]
\draw[] (0.6875, 0) rectangle (0.71875, 0.03125);% [-0.0567321, 0]
\draw[fill=\HigherOrderColor] (0.65625, 0.03125) rectangle (0.6875, 0.0625);% [-0.0961115, -0.0926563]
\PrecisionAchieved{0.65625,0.03125}{0.6875,0.0625}{0.671875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.03125) rectangle (0.65625, 0.0625);% [-0.0953028, -0.0918834]
\PrecisionAchieved{0.625,0.03125}{0.65625,0.0625}{0.640625,0.046875}{0.00625}
\draw[] (0.65625, 0) rectangle (0.6875, 0.03125);% [-0.058056, 0]
\draw[] (0.625, 0) rectangle (0.65625, 0.03125);% [-0.057785, 0]
\draw[fill=\HigherOrderColor] (0.5625, 0.0625) rectangle (0.625, 0.125);% [-0.185555, -0.156982]
\PrecisionAchieved{0.5625,0.0625}{0.625,0.125}{0.59375,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.0625) rectangle (0.5625, 0.125);% [-0.167308, -0.145382]
\PrecisionAchieved{0.5,0.0625}{0.5625,0.125}{0.53125,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.59375, 0.03125) rectangle (0.625, 0.0625);% [-0.092245, -0.0890725]
\PrecisionAchieved{0.59375,0.03125}{0.625,0.0625}{0.609375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.03125) rectangle (0.59375, 0.0625);% [-0.0871423, -0.0843889]
\PrecisionAchieved{0.5625,0.03125}{0.59375,0.0625}{0.578125,0.046875}{0.00625}
\draw[] (0.59375, 0) rectangle (0.625, 0.03125);% [-0.056005, 0]
\draw[] (0.5625, 0) rectangle (0.59375, 0.03125);% [-0.0528588, 0]
\draw[fill=\HigherOrderColor] (0.53125, 0.03125) rectangle (0.5625, 0.0625);% [-0.0802649, -0.0780441]
\PrecisionAchieved{0.53125,0.03125}{0.5625,0.0625}{0.546875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.03125) rectangle (0.53125, 0.0625);% [-0.0720375, -0.0702338]
\PrecisionAchieved{0.5,0.03125}{0.53125,0.0625}{0.515625,0.046875}{0.00625}
\draw[] (0.53125, 0) rectangle (0.5625, 0.03125);% [-0.0485429, 0]
\PrecisionAchieved{0.53125,0}{0.5625,0.03125}{0.546875,0.015625}{0.00625}
\draw[] (0.5, 0) rectangle (0.53125, 0.03125);% [-0.0433027, 0]
\PrecisionAchieved{0.5,0}{0.53125,0.03125}{0.515625,0.015625}{0.00625}
\draw[] (0.46875, 0.46875) rectangle (0.5, 0.5);% [-0.0376961, 0]
\PrecisionAchieved{0.46875,0.46875}{0.5,0.5}{0.484375,0.484375}{0.00625}
\draw[] (0.4375, 0.46875) rectangle (0.46875, 0.5);% [-0.0957117, 0]
\draw[] (0.46875, 0.4375) rectangle (0.5, 0.46875);% [-0.0957117, 0]
\draw[] (0.4375, 0.4375) rectangle (0.46875, 0.46875);% [-0.0360884, 0]
\PrecisionAchieved{0.4375,0.4375}{0.46875,0.46875}{0.453125,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.40625, 0.46875) rectangle (0.4375, 0.5);% [-0.0956646, -0.0914662]
\PrecisionAchieved{0.40625,0.46875}{0.4375,0.5}{0.421875,0.484375}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.46875) rectangle (0.40625, 0.5);% [-0.1434, -0.13801]
\PrecisionAchieved{0.375,0.46875}{0.40625,0.5}{0.390625,0.484375}{0.00625}
\draw[] (0.40625, 0.4375) rectangle (0.4375, 0.46875);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.375, 0.4375) rectangle (0.40625, 0.46875);% [-0.0888868, -0.0848121]
\PrecisionAchieved{0.375,0.4375}{0.40625,0.46875}{0.390625,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.46875, 0.40625) rectangle (0.5, 0.4375);% [-0.0956646, -0.0914662]
\PrecisionAchieved{0.46875,0.40625}{0.5,0.4375}{0.484375,0.421875}{0.00625}
\draw[] (0.4375, 0.40625) rectangle (0.46875, 0.4375);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.46875, 0.375) rectangle (0.5, 0.40625);% [-0.1434, -0.13801]
\PrecisionAchieved{0.46875,0.375}{0.5,0.40625}{0.484375,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.375) rectangle (0.46875, 0.40625);% [-0.0888868, -0.0848121]
\PrecisionAchieved{0.4375,0.375}{0.46875,0.40625}{0.453125,0.390625}{0.00625}
\draw[] (0.40625, 0.40625) rectangle (0.4375, 0.4375);% [-0.0330265, 0]
\PrecisionAchieved{0.40625,0.40625}{0.4375,0.4375}{0.421875,0.421875}{0.00625}
\draw[] (0.375, 0.40625) rectangle (0.40625, 0.4375);% [-0.0823766, 0]
\draw[] (0.40625, 0.375) rectangle (0.4375, 0.40625);% [-0.0823766, 0]
\draw[] (0.375, 0.375) rectangle (0.40625, 0.40625);% [-0.0288048, 0]
\PrecisionAchieved{0.375,0.375}{0.40625,0.40625}{0.390625,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.4375) rectangle (0.375, 0.5);% [-0.179181, -0.151183]
\PrecisionAchieved{0.3125,0.4375}{0.375,0.5}{0.34375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.4375) rectangle (0.3125, 0.5);% [-0.193587, -0.173249]
\PrecisionAchieved{0.25,0.4375}{0.3125,0.5}{0.28125,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.34375, 0.40625) rectangle (0.375, 0.4375);% [-0.0792551, -0.0752509]
\PrecisionAchieved{0.34375,0.40625}{0.375,0.4375}{0.359375,0.421875}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.40625) rectangle (0.34375, 0.4375);% [-0.118051, -0.114501]
\PrecisionAchieved{0.3125,0.40625}{0.34375,0.4375}{0.328125,0.421875}{0.00625}
\draw[] (0.34375, 0.375) rectangle (0.375, 0.40625);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.3125, 0.375) rectangle (0.34375, 0.40625);% [-0.0673359, -0.0635464]
\PrecisionAchieved{0.3125,0.375}{0.34375,0.40625}{0.328125,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.375) rectangle (0.3125, 0.4375);% [-0.141066, -0.123732]
\PrecisionAchieved{0.25,0.375}{0.3125,0.4375}{0.28125,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.3125) rectangle (0.5, 0.375);% [-0.179181, -0.151183]
\PrecisionAchieved{0.4375,0.3125}{0.5,0.375}{0.46875,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.40625, 0.34375) rectangle (0.4375, 0.375);% [-0.0792551, -0.0752509]
\PrecisionAchieved{0.40625,0.34375}{0.4375,0.375}{0.421875,0.359375}{0.00625}
\draw[] (0.375, 0.34375) rectangle (0.40625, 0.375);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.40625, 0.3125) rectangle (0.4375, 0.34375);% [-0.118051, -0.114501]
\PrecisionAchieved{0.40625,0.3125}{0.4375,0.34375}{0.421875,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.3125) rectangle (0.40625, 0.34375);% [-0.0673359, -0.0635464]
\PrecisionAchieved{0.375,0.3125}{0.40625,0.34375}{0.390625,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.25) rectangle (0.5, 0.3125);% [-0.193587, -0.173249]
\PrecisionAchieved{0.4375,0.25}{0.5,0.3125}{0.46875,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.25) rectangle (0.4375, 0.3125);% [-0.141066, -0.123732]
\PrecisionAchieved{0.375,0.25}{0.4375,0.3125}{0.40625,0.28125}{0.0125}
\draw[] (0.34375, 0.34375) rectangle (0.375, 0.375);% [-0.0238312, 0]
\PrecisionAchieved{0.34375,0.34375}{0.375,0.375}{0.359375,0.359375}{0.00625}
\draw[] (0.3125, 0.34375) rectangle (0.34375, 0.375);% [-0.058991, 0]
\draw[] (0.34375, 0.3125) rectangle (0.375, 0.34375);% [-0.058991, 0]
\draw[] (0.3125, 0.3125) rectangle (0.34375, 0.34375);% [-0.0185805, 0]
\PrecisionAchieved{0.3125,0.3125}{0.34375,0.34375}{0.328125,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.34375) rectangle (0.3125, 0.375);% [-0.0540898, -0.0506325]
\PrecisionAchieved{0.28125,0.34375}{0.3125,0.375}{0.296875,0.359375}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.34375) rectangle (0.28125, 0.375);% [-0.0793242, -0.0771794]
\PrecisionAchieved{0.25,0.34375}{0.28125,0.375}{0.265625,0.359375}{0.00625}
\draw[] (0.28125, 0.3125) rectangle (0.3125, 0.34375);% [-0.0457006, 0]
\PrecisionAchieved{0.28125,0.3125}{0.3125,0.34375}{0.296875,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.3125) rectangle (0.28125, 0.34375);% [-0.040695, -0.0376258]
\PrecisionAchieved{0.25,0.3125}{0.28125,0.34375}{0.265625,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.28125) rectangle (0.375, 0.3125);% [-0.0540898, -0.0506325]
\PrecisionAchieved{0.34375,0.28125}{0.375,0.3125}{0.359375,0.296875}{0.00625}
\draw[] (0.3125, 0.28125) rectangle (0.34375, 0.3125);% [-0.0457006, 0]
\PrecisionAchieved{0.3125,0.28125}{0.34375,0.3125}{0.328125,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.25) rectangle (0.375, 0.28125);% [-0.0793242, -0.0771794]
\PrecisionAchieved{0.34375,0.25}{0.375,0.28125}{0.359375,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.25) rectangle (0.34375, 0.28125);% [-0.040695, -0.0376258]
\PrecisionAchieved{0.3125,0.25}{0.34375,0.28125}{0.328125,0.265625}{0.00625}
\draw[] (0.25, 0.25) rectangle (0.3125, 0.3125);% [-0.0328859, 0]
\PrecisionAchieved{0.25,0.25}{0.3125,0.3125}{0.28125,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.4375) rectangle (0.25, 0.5);% [-0.191339, -0.17651]
\PrecisionAchieved{0.1875,0.4375}{0.25,0.5}{0.21875,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.4375) rectangle (0.1875, 0.5);% [-0.185228, -0.16844]
\PrecisionAchieved{0.125,0.4375}{0.1875,0.5}{0.15625,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.375) rectangle (0.25, 0.4375);% [-0.157796, -0.144785]
\PrecisionAchieved{0.1875,0.375}{0.25,0.4375}{0.21875,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.375) rectangle (0.1875, 0.4375);% [-0.14503, -0.132578]
\PrecisionAchieved{0.125,0.375}{0.1875,0.4375}{0.15625,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.4375) rectangle (0.125, 0.5);% [-0.136228, -0.121679]
\PrecisionAchieved{0.0625,0.4375}{0.125,0.5}{0.09375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.46875) rectangle (0.0625, 0.5);% [-0.0631646, -0.0610217]
\PrecisionAchieved{0.03125,0.46875}{0.0625,0.5}{0.046875,0.484375}{0.00625}
\draw[] (0, 0.46875) rectangle (0.03125, 0.5);% [-0.0376961, 0]
\PrecisionAchieved{0,0.46875}{0.03125,0.5}{0.015625,0.484375}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.4375) rectangle (0.0625, 0.46875);% [-0.0537469, -0.0512044]
\PrecisionAchieved{0.03125,0.4375}{0.0625,0.46875}{0.046875,0.453125}{0.00625}
\draw[] (0, 0.4375) rectangle (0.03125, 0.46875);% [-0.0374249, 0]
\PrecisionAchieved{0,0.4375}{0.03125,0.46875}{0.015625,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.375) rectangle (0.125, 0.4375);% [-0.0985275, -0.0852643]
\PrecisionAchieved{0.0625,0.375}{0.125,0.4375}{0.09375,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.40625) rectangle (0.0625, 0.4375);% [-0.0442196, -0.0413198]
\PrecisionAchieved{0.03125,0.40625}{0.0625,0.4375}{0.046875,0.421875}{0.00625}
\draw[] (0, 0.40625) rectangle (0.03125, 0.4375);% [-0.0366166, 0]
\PrecisionAchieved{0,0.40625}{0.03125,0.4375}{0.015625,0.421875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.375) rectangle (0.0625, 0.40625);% [-0.0350878, -0.0318305]
\PrecisionAchieved{0.03125,0.375}{0.0625,0.40625}{0.046875,0.390625}{0.00625}
\draw[] (0, 0.375) rectangle (0.03125, 0.40625);% [-0.0352867, 0]
\PrecisionAchieved{0,0.375}{0.03125,0.40625}{0.015625,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.3125) rectangle (0.25, 0.375);% [-0.0886292, -0.0745694]
\PrecisionAchieved{0.1875,0.3125}{0.25,0.375}{0.21875,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.3125) rectangle (0.1875, 0.375);% [-0.0895606, -0.0760559]
\PrecisionAchieved{0.125,0.3125}{0.1875,0.375}{0.15625,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.21875, 0.28125) rectangle (0.25, 0.3125);% [-0.0284654, -0.0255542]
\PrecisionAchieved{0.21875,0.28125}{0.25,0.3125}{0.234375,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.28125) rectangle (0.21875, 0.3125);% [-0.0398853, -0.037525]
\PrecisionAchieved{0.1875,0.28125}{0.21875,0.3125}{0.203125,0.296875}{0.00625}
\draw[] (0.21875, 0.25) rectangle (0.25, 0.28125);% [-0.0254528, 0]
\PrecisionAchieved{0.21875,0.25}{0.25,0.28125}{0.234375,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.25) rectangle (0.21875, 0.28125);% [-0.0183931, -0.0153567]
\PrecisionAchieved{0.1875,0.25}{0.21875,0.28125}{0.203125,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.15625, 0.28125) rectangle (0.1875, 0.3125);% [-0.0449652, -0.0429422]
\PrecisionAchieved{0.15625,0.28125}{0.1875,0.3125}{0.171875,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.28125) rectangle (0.15625, 0.3125);% [-0.0434626, -0.0416773]
\PrecisionAchieved{0.125,0.28125}{0.15625,0.3125}{0.140625,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.15625, 0.25) rectangle (0.1875, 0.28125);% [-0.0243226, -0.0219393]
\PrecisionAchieved{0.15625,0.25}{0.1875,0.28125}{0.171875,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.25) rectangle (0.15625, 0.28125);% [-0.0255521, -0.0235068]
\PrecisionAchieved{0.125,0.25}{0.15625,0.28125}{0.140625,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.34375) rectangle (0.125, 0.375);% [-0.0745963, -0.0731945]
\PrecisionAchieved{0.09375,0.34375}{0.125,0.375}{0.109375,0.359375}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.34375) rectangle (0.09375, 0.375);% [-0.051275, -0.0498579]
\PrecisionAchieved{0.0625,0.34375}{0.09375,0.375}{0.078125,0.359375}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.3125) rectangle (0.125, 0.34375);% [-0.0539678, -0.0525059]
\PrecisionAchieved{0.09375,0.3125}{0.125,0.34375}{0.109375,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.3125) rectangle (0.09375, 0.34375);% [-0.0370912, -0.0353961]
\PrecisionAchieved{0.0625,0.3125}{0.09375,0.34375}{0.078125,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.34375) rectangle (0.0625, 0.375);% [-0.0270614, -0.0228941]
\PrecisionAchieved{0.03125,0.34375}{0.0625,0.375}{0.046875,0.359375}{0.00625}
\draw[] (0, 0.34375) rectangle (0.03125, 0.375);% [-0.0334617, 0]
\PrecisionAchieved{0,0.34375}{0.03125,0.375}{0.015625,0.359375}{0.00625}
\draw[] (0.03125, 0.3125) rectangle (0.0625, 0.34375);% [-0.056005, 0]
\draw[] (0, 0.3125) rectangle (0.03125, 0.34375);% [-0.0311793, 0]
\PrecisionAchieved{0,0.3125}{0.03125,0.34375}{0.015625,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.28125) rectangle (0.125, 0.3125);% [-0.0362129, -0.0346317]
\PrecisionAchieved{0.09375,0.28125}{0.125,0.3125}{0.109375,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.28125) rectangle (0.09375, 0.3125);% [-0.0253345, -0.023126]
\PrecisionAchieved{0.0625,0.28125}{0.09375,0.3125}{0.078125,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.25) rectangle (0.125, 0.28125);% [-0.0223134, -0.0203917]
\PrecisionAchieved{0.09375,0.25}{0.125,0.28125}{0.109375,0.265625}{0.00625}
\draw[] (0.0625, 0.25) rectangle (0.09375, 0.28125);% [-0.050508, 0]
\draw[] (0.03125, 0.28125) rectangle (0.0625, 0.3125);% [-0.0473243, 0]
\PrecisionAchieved{0.03125,0.28125}{0.0625,0.3125}{0.046875,0.296875}{0.00625}
\draw[] (0, 0.28125) rectangle (0.03125, 0.3125);% [-0.028489, 0]
\PrecisionAchieved{0,0.28125}{0.03125,0.3125}{0.015625,0.296875}{0.00625}
\draw[] (0.03125, 0.25) rectangle (0.0625, 0.28125);% [-0.0390284, 0]
\PrecisionAchieved{0.03125,0.25}{0.0625,0.28125}{0.046875,0.265625}{0.00625}
\draw[] (0, 0.25) rectangle (0.03125, 0.28125);% [-0.0254528, 0]
\PrecisionAchieved{0,0.25}{0.03125,0.28125}{0.015625,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.1875) rectangle (0.5, 0.25);% [-0.191339, -0.17651]
\PrecisionAchieved{0.4375,0.1875}{0.5,0.25}{0.46875,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.1875) rectangle (0.4375, 0.25);% [-0.157796, -0.144785]
\PrecisionAchieved{0.375,0.1875}{0.4375,0.25}{0.40625,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.125) rectangle (0.5, 0.1875);% [-0.185228, -0.16844]
\PrecisionAchieved{0.4375,0.125}{0.5,0.1875}{0.46875,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.125) rectangle (0.4375, 0.1875);% [-0.14503, -0.132578]
\PrecisionAchieved{0.375,0.125}{0.4375,0.1875}{0.40625,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.1875) rectangle (0.375, 0.25);% [-0.0886292, -0.0745694]
\PrecisionAchieved{0.3125,0.1875}{0.375,0.25}{0.34375,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.28125, 0.21875) rectangle (0.3125, 0.25);% [-0.0284654, -0.0255542]
\PrecisionAchieved{0.28125,0.21875}{0.3125,0.25}{0.296875,0.234375}{0.00625}
\draw[] (0.25, 0.21875) rectangle (0.28125, 0.25);% [-0.0254528, 0]
\PrecisionAchieved{0.25,0.21875}{0.28125,0.25}{0.265625,0.234375}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.1875) rectangle (0.3125, 0.21875);% [-0.0398853, -0.037525]
\PrecisionAchieved{0.28125,0.1875}{0.3125,0.21875}{0.296875,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.1875) rectangle (0.28125, 0.21875);% [-0.0183931, -0.0153567]
\PrecisionAchieved{0.25,0.1875}{0.28125,0.21875}{0.265625,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.125) rectangle (0.375, 0.1875);% [-0.0895606, -0.0760559]
\PrecisionAchieved{0.3125,0.125}{0.375,0.1875}{0.34375,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.28125, 0.15625) rectangle (0.3125, 0.1875);% [-0.0449652, -0.0429422]
\PrecisionAchieved{0.28125,0.15625}{0.3125,0.1875}{0.296875,0.171875}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.15625) rectangle (0.28125, 0.1875);% [-0.0243226, -0.0219393]
\PrecisionAchieved{0.25,0.15625}{0.28125,0.1875}{0.265625,0.171875}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.125) rectangle (0.3125, 0.15625);% [-0.0434626, -0.0416773]
\PrecisionAchieved{0.28125,0.125}{0.3125,0.15625}{0.296875,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.125) rectangle (0.28125, 0.15625);% [-0.0255521, -0.0235068]
\PrecisionAchieved{0.25,0.125}{0.28125,0.15625}{0.265625,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.0625) rectangle (0.5, 0.125);% [-0.136228, -0.121679]
\PrecisionAchieved{0.4375,0.0625}{0.5,0.125}{0.46875,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.0625) rectangle (0.4375, 0.125);% [-0.0985275, -0.0852643]
\PrecisionAchieved{0.375,0.0625}{0.4375,0.125}{0.40625,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.46875, 0.03125) rectangle (0.5, 0.0625);% [-0.0631646, -0.0610217]
\PrecisionAchieved{0.46875,0.03125}{0.5,0.0625}{0.484375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.03125) rectangle (0.46875, 0.0625);% [-0.0537469, -0.0512044]
\PrecisionAchieved{0.4375,0.03125}{0.46875,0.0625}{0.453125,0.046875}{0.00625}
\draw[] (0.46875, 0) rectangle (0.5, 0.03125);% [-0.0376961, 0]
\PrecisionAchieved{0.46875,0}{0.5,0.03125}{0.484375,0.015625}{0.00625}
\draw[] (0.4375, 0) rectangle (0.46875, 0.03125);% [-0.0374249, 0]
\PrecisionAchieved{0.4375,0}{0.46875,0.03125}{0.453125,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.40625, 0.03125) rectangle (0.4375, 0.0625);% [-0.0442196, -0.0413198]
\PrecisionAchieved{0.40625,0.03125}{0.4375,0.0625}{0.421875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.03125) rectangle (0.40625, 0.0625);% [-0.0350878, -0.0318305]
\PrecisionAchieved{0.375,0.03125}{0.40625,0.0625}{0.390625,0.046875}{0.00625}
\draw[] (0.40625, 0) rectangle (0.4375, 0.03125);% [-0.0366166, 0]
\PrecisionAchieved{0.40625,0}{0.4375,0.03125}{0.421875,0.015625}{0.00625}
\draw[] (0.375, 0) rectangle (0.40625, 0.03125);% [-0.0352867, 0]
\PrecisionAchieved{0.375,0}{0.40625,0.03125}{0.390625,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.09375) rectangle (0.375, 0.125);% [-0.0745963, -0.0731945]
\PrecisionAchieved{0.34375,0.09375}{0.375,0.125}{0.359375,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.09375) rectangle (0.34375, 0.125);% [-0.0539678, -0.0525059]
\PrecisionAchieved{0.3125,0.09375}{0.34375,0.125}{0.328125,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.0625) rectangle (0.375, 0.09375);% [-0.051275, -0.0498579]
\PrecisionAchieved{0.34375,0.0625}{0.375,0.09375}{0.359375,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.0625) rectangle (0.34375, 0.09375);% [-0.0370912, -0.0353961]
\PrecisionAchieved{0.3125,0.0625}{0.34375,0.09375}{0.328125,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.09375) rectangle (0.3125, 0.125);% [-0.0362129, -0.0346317]
\PrecisionAchieved{0.28125,0.09375}{0.3125,0.125}{0.296875,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.09375) rectangle (0.28125, 0.125);% [-0.0223134, -0.0203917]
\PrecisionAchieved{0.25,0.09375}{0.28125,0.125}{0.265625,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.0625) rectangle (0.3125, 0.09375);% [-0.0253345, -0.023126]
\PrecisionAchieved{0.28125,0.0625}{0.3125,0.09375}{0.296875,0.078125}{0.00625}
\draw[] (0.25, 0.0625) rectangle (0.28125, 0.09375);% [-0.050508, 0]
\draw[fill=\HigherOrderColor] (0.34375, 0.03125) rectangle (0.375, 0.0625);% [-0.0270614, -0.0228941]
\PrecisionAchieved{0.34375,0.03125}{0.375,0.0625}{0.359375,0.046875}{0.00625}
\draw[] (0.3125, 0.03125) rectangle (0.34375, 0.0625);% [-0.056005, 0]
\draw[] (0.34375, 0) rectangle (0.375, 0.03125);% [-0.0334617, 0]
\PrecisionAchieved{0.34375,0}{0.375,0.03125}{0.359375,0.015625}{0.00625}
\draw[] (0.3125, 0) rectangle (0.34375, 0.03125);% [-0.0311793, 0]
\PrecisionAchieved{0.3125,0}{0.34375,0.03125}{0.328125,0.015625}{0.00625}
\draw[] (0.28125, 0.03125) rectangle (0.3125, 0.0625);% [-0.0473243, 0]
\PrecisionAchieved{0.28125,0.03125}{0.3125,0.0625}{0.296875,0.046875}{0.00625}
\draw[] (0.25, 0.03125) rectangle (0.28125, 0.0625);% [-0.0390284, 0]
\PrecisionAchieved{0.25,0.03125}{0.28125,0.0625}{0.265625,0.046875}{0.00625}
\draw[] (0.28125, 0) rectangle (0.3125, 0.03125);% [-0.028489, 0]
\PrecisionAchieved{0.28125,0}{0.3125,0.03125}{0.296875,0.015625}{0.00625}
\draw[] (0.25, 0) rectangle (0.28125, 0.03125);% [-0.0254528, 0]
\PrecisionAchieved{0.25,0}{0.28125,0.03125}{0.265625,0.015625}{0.00625}
\draw[] (0.1875, 0.1875) rectangle (0.25, 0.25);% [-0.0373315, 0]
\PrecisionAchieved{0.1875,0.1875}{0.25,0.25}{0.21875,0.21875}{0.0125}
\draw[] (0.15625, 0.21875) rectangle (0.1875, 0.25);% [-0.036502, 0]
\PrecisionAchieved{0.15625,0.21875}{0.1875,0.25}{0.171875,0.234375}{0.00625}
\draw[] (0.125, 0.21875) rectangle (0.15625, 0.25);% [-0.0428262, 0]
\PrecisionAchieved{0.125,0.21875}{0.15625,0.25}{0.140625,0.234375}{0.00625}
\draw[] (0.15625, 0.1875) rectangle (0.1875, 0.21875);% [-0.0253958, 0]
\PrecisionAchieved{0.15625,0.1875}{0.1875,0.21875}{0.171875,0.203125}{0.00625}
\draw[] (0.125, 0.1875) rectangle (0.15625, 0.21875);% [-0.0316975, 0]
\PrecisionAchieved{0.125,0.1875}{0.15625,0.21875}{0.140625,0.203125}{0.00625}
\draw[] (0.21875, 0.15625) rectangle (0.25, 0.1875);% [-0.036502, 0]
\PrecisionAchieved{0.21875,0.15625}{0.25,0.1875}{0.234375,0.171875}{0.00625}
\draw[] (0.1875, 0.15625) rectangle (0.21875, 0.1875);% [-0.0253958, 0]
\PrecisionAchieved{0.1875,0.15625}{0.21875,0.1875}{0.203125,0.171875}{0.00625}
\draw[] (0.21875, 0.125) rectangle (0.25, 0.15625);% [-0.0428262, 0]
\PrecisionAchieved{0.21875,0.125}{0.25,0.15625}{0.234375,0.140625}{0.00625}
\draw[] (0.1875, 0.125) rectangle (0.21875, 0.15625);% [-0.0316975, 0]
\PrecisionAchieved{0.1875,0.125}{0.21875,0.15625}{0.203125,0.140625}{0.00625}
\draw[] (0.15625, 0.15625) rectangle (0.1875, 0.1875);% [-0.0180755, 0]
\PrecisionAchieved{0.15625,0.15625}{0.1875,0.1875}{0.171875,0.171875}{0.00625}
\draw[] (0.125, 0.15625) rectangle (0.15625, 0.1875);% [-0.0236217, 0]
\PrecisionAchieved{0.125,0.15625}{0.15625,0.1875}{0.140625,0.171875}{0.00625}
\draw[] (0.15625, 0.125) rectangle (0.1875, 0.15625);% [-0.0236217, 0]
\PrecisionAchieved{0.15625,0.125}{0.1875,0.15625}{0.171875,0.140625}{0.00625}
\draw[] (0.125, 0.125) rectangle (0.15625, 0.15625);% [-0.0180817, 0]
\PrecisionAchieved{0.125,0.125}{0.15625,0.15625}{0.140625,0.140625}{0.00625}
\draw[] (0.09375, 0.21875) rectangle (0.125, 0.25);% [-0.043624, 0]
\PrecisionAchieved{0.09375,0.21875}{0.125,0.25}{0.109375,0.234375}{0.00625}
\draw[] (0.0625, 0.21875) rectangle (0.09375, 0.25);% [-0.0395592, 0]
\PrecisionAchieved{0.0625,0.21875}{0.09375,0.25}{0.078125,0.234375}{0.00625}
\draw[] (0.09375, 0.1875) rectangle (0.125, 0.21875);% [-0.0335055, 0]
\PrecisionAchieved{0.09375,0.1875}{0.125,0.21875}{0.109375,0.203125}{0.00625}
\draw[] (0.0625, 0.1875) rectangle (0.09375, 0.21875);% [-0.0312224, 0]
\PrecisionAchieved{0.0625,0.1875}{0.09375,0.21875}{0.078125,0.203125}{0.00625}
\draw[] (0.03125, 0.21875) rectangle (0.0625, 0.25);% [-0.0318472, 0]
\PrecisionAchieved{0.03125,0.21875}{0.0625,0.25}{0.046875,0.234375}{0.00625}
\draw[] (0, 0.21875) rectangle (0.03125, 0.25);% [-0.0221457, 0]
\PrecisionAchieved{0,0.21875}{0.03125,0.25}{0.015625,0.234375}{0.00625}
\draw[] (0.03125, 0.1875) rectangle (0.0625, 0.21875);% [-0.0258229, 0]
\PrecisionAchieved{0.03125,0.1875}{0.0625,0.21875}{0.046875,0.203125}{0.00625}
\draw[] (0, 0.1875) rectangle (0.03125, 0.21875);% [-0.0186564, 0]
\PrecisionAchieved{0,0.1875}{0.03125,0.21875}{0.015625,0.203125}{0.00625}
\draw[] (0.09375, 0.15625) rectangle (0.125, 0.1875);% [-0.0256307, 0]
\PrecisionAchieved{0.09375,0.15625}{0.125,0.1875}{0.109375,0.171875}{0.00625}
\draw[] (0.0625, 0.15625) rectangle (0.09375, 0.1875);% [-0.0243169, 0]
\PrecisionAchieved{0.0625,0.15625}{0.09375,0.1875}{0.078125,0.171875}{0.00625}
\draw[] (0.09375, 0.125) rectangle (0.125, 0.15625);% [-0.0196956, 0]
\PrecisionAchieved{0.09375,0.125}{0.125,0.15625}{0.109375,0.140625}{0.00625}
\draw[] (0.0625, 0.125) rectangle (0.09375, 0.15625);% [-0.0186996, 0]
\PrecisionAchieved{0.0625,0.125}{0.09375,0.15625}{0.078125,0.140625}{0.00625}
\draw[] (0, 0.125) rectangle (0.0625, 0.1875);% [-0.0428262, 0]
\PrecisionAchieved{0,0.125}{0.0625,0.1875}{0.03125,0.15625}{0.0125}
\draw[] (0.21875, 0.09375) rectangle (0.25, 0.125);% [-0.043624, 0]
\PrecisionAchieved{0.21875,0.09375}{0.25,0.125}{0.234375,0.109375}{0.00625}
\draw[] (0.1875, 0.09375) rectangle (0.21875, 0.125);% [-0.0335055, 0]
\PrecisionAchieved{0.1875,0.09375}{0.21875,0.125}{0.203125,0.109375}{0.00625}
\draw[] (0.21875, 0.0625) rectangle (0.25, 0.09375);% [-0.0395592, 0]
\PrecisionAchieved{0.21875,0.0625}{0.25,0.09375}{0.234375,0.078125}{0.00625}
\draw[] (0.1875, 0.0625) rectangle (0.21875, 0.09375);% [-0.0312224, 0]
\PrecisionAchieved{0.1875,0.0625}{0.21875,0.09375}{0.203125,0.078125}{0.00625}
\draw[] (0.15625, 0.09375) rectangle (0.1875, 0.125);% [-0.0256307, 0]
\PrecisionAchieved{0.15625,0.09375}{0.1875,0.125}{0.171875,0.109375}{0.00625}
\draw[] (0.125, 0.09375) rectangle (0.15625, 0.125);% [-0.0196956, 0]
\PrecisionAchieved{0.125,0.09375}{0.15625,0.125}{0.140625,0.109375}{0.00625}
\draw[] (0.15625, 0.0625) rectangle (0.1875, 0.09375);% [-0.0243169, 0]
\PrecisionAchieved{0.15625,0.0625}{0.1875,0.09375}{0.171875,0.078125}{0.00625}
\draw[] (0.125, 0.0625) rectangle (0.15625, 0.09375);% [-0.0186996, 0]
\PrecisionAchieved{0.125,0.0625}{0.15625,0.09375}{0.140625,0.078125}{0.00625}
\draw[] (0.21875, 0.03125) rectangle (0.25, 0.0625);% [-0.0318472, 0]
\PrecisionAchieved{0.21875,0.03125}{0.25,0.0625}{0.234375,0.046875}{0.00625}
\draw[] (0.1875, 0.03125) rectangle (0.21875, 0.0625);% [-0.0258229, 0]
\PrecisionAchieved{0.1875,0.03125}{0.21875,0.0625}{0.203125,0.046875}{0.00625}
\draw[] (0.21875, 0) rectangle (0.25, 0.03125);% [-0.0221457, 0]
\PrecisionAchieved{0.21875,0}{0.25,0.03125}{0.234375,0.015625}{0.00625}
\draw[] (0.1875, 0) rectangle (0.21875, 0.03125);% [-0.0186564, 0]
\PrecisionAchieved{0.1875,0}{0.21875,0.03125}{0.203125,0.015625}{0.00625}
\draw[] (0.125, 0) rectangle (0.1875, 0.0625);% [-0.0428262, 0]
\PrecisionAchieved{0.125,0}{0.1875,0.0625}{0.15625,0.03125}{0.0125}
\draw[] (0.0625, 0.0625) rectangle (0.125, 0.125);% [-0.0379418, 0]
\PrecisionAchieved{0.0625,0.0625}{0.125,0.125}{0.09375,0.09375}{0.0125}
\draw[] (0, 0.0625) rectangle (0.0625, 0.125);% [-0.0243169, 0]
\PrecisionAchieved{0,0.0625}{0.0625,0.125}{0.03125,0.09375}{0.0125}
\draw[] (0.0625, 0) rectangle (0.125, 0.0625);% [-0.0243169, 0]
\PrecisionAchieved{0.0625,0}{0.125,0.0625}{0.09375,0.03125}{0.0125}
\draw[] (0, 0) rectangle (0.0625, 0.0625);% [-0.00819741, 0]
\PrecisionAchieved{0,0}{0.0625,0.0625}{0.03125,0.03125}{0.0125}


==> integration3.tex <==
\providecommand{\PrecisionAchieved}[4]{%
  % {x0,y0}{x1,y1}{xmid,ymid}{w}
  \draw[color=orange,fill] (#3) circle(#4);}
\providecommand{\HigherOrderColor}{light-green}
\draw[] (0.9375, 0.9375) rectangle (1, 1);% [-0.00819741, 0]
\PrecisionAchieved{0.9375,0.9375}{1,1}{0.96875,0.96875}{0.0125}
\draw[] (0.875, 0.9375) rectangle (0.9375, 1);% [-0.0243169, 0]
\PrecisionAchieved{0.875,0.9375}{0.9375,1}{0.90625,0.96875}{0.0125}
\draw[] (0.9375, 0.875) rectangle (1, 0.9375);% [-0.0243169, 0]
\PrecisionAchieved{0.9375,0.875}{1,0.9375}{0.96875,0.90625}{0.0125}
\draw[] (0.875, 0.875) rectangle (0.9375, 0.9375);% [-0.0379418, 0]
\PrecisionAchieved{0.875,0.875}{0.9375,0.9375}{0.90625,0.90625}{0.0125}
\draw[] (0.8125, 0.9375) rectangle (0.875, 1);% [-0.0428262, 0]
\PrecisionAchieved{0.8125,0.9375}{0.875,1}{0.84375,0.96875}{0.0125}
\draw[] (0.78125, 0.96875) rectangle (0.8125, 1);% [-0.0186564, 0]
\PrecisionAchieved{0.78125,0.96875}{0.8125,1}{0.796875,0.984375}{0.00625}
\draw[] (0.75, 0.96875) rectangle (0.78125, 1);% [-0.0221457, 0]
\PrecisionAchieved{0.75,0.96875}{0.78125,1}{0.765625,0.984375}{0.00625}
\draw[] (0.78125, 0.9375) rectangle (0.8125, 0.96875);% [-0.0258229, 0]
\PrecisionAchieved{0.78125,0.9375}{0.8125,0.96875}{0.796875,0.953125}{0.00625}
\draw[] (0.75, 0.9375) rectangle (0.78125, 0.96875);% [-0.0318472, 0]
\PrecisionAchieved{0.75,0.9375}{0.78125,0.96875}{0.765625,0.953125}{0.00625}
\draw[] (0.84375, 0.90625) rectangle (0.875, 0.9375);% [-0.0186996, 0]
\PrecisionAchieved{0.84375,0.90625}{0.875,0.9375}{0.859375,0.921875}{0.00625}
\draw[] (0.8125, 0.90625) rectangle (0.84375, 0.9375);% [-0.0243169, 0]
\PrecisionAchieved{0.8125,0.90625}{0.84375,0.9375}{0.828125,0.921875}{0.00625}
\draw[] (0.84375, 0.875) rectangle (0.875, 0.90625);% [-0.0196956, 0]
\PrecisionAchieved{0.84375,0.875}{0.875,0.90625}{0.859375,0.890625}{0.00625}
\draw[] (0.8125, 0.875) rectangle (0.84375, 0.90625);% [-0.0256307, 0]
\PrecisionAchieved{0.8125,0.875}{0.84375,0.90625}{0.828125,0.890625}{0.00625}
\draw[] (0.78125, 0.90625) rectangle (0.8125, 0.9375);% [-0.0312224, 0]
\PrecisionAchieved{0.78125,0.90625}{0.8125,0.9375}{0.796875,0.921875}{0.00625}
\draw[] (0.75, 0.90625) rectangle (0.78125, 0.9375);% [-0.0395592, 0]
\PrecisionAchieved{0.75,0.90625}{0.78125,0.9375}{0.765625,0.921875}{0.00625}
\draw[] (0.78125, 0.875) rectangle (0.8125, 0.90625);% [-0.0335055, 0]
\PrecisionAchieved{0.78125,0.875}{0.8125,0.90625}{0.796875,0.890625}{0.00625}
\draw[] (0.75, 0.875) rectangle (0.78125, 0.90625);% [-0.043624, 0]
\PrecisionAchieved{0.75,0.875}{0.78125,0.90625}{0.765625,0.890625}{0.00625}
\draw[] (0.9375, 0.8125) rectangle (1, 0.875);% [-0.0428262, 0]
\PrecisionAchieved{0.9375,0.8125}{1,0.875}{0.96875,0.84375}{0.0125}
\draw[] (0.90625, 0.84375) rectangle (0.9375, 0.875);% [-0.0186996, 0]
\PrecisionAchieved{0.90625,0.84375}{0.9375,0.875}{0.921875,0.859375}{0.00625}
\draw[] (0.875, 0.84375) rectangle (0.90625, 0.875);% [-0.0196956, 0]
\PrecisionAchieved{0.875,0.84375}{0.90625,0.875}{0.890625,0.859375}{0.00625}
\draw[] (0.90625, 0.8125) rectangle (0.9375, 0.84375);% [-0.0243169, 0]
\PrecisionAchieved{0.90625,0.8125}{0.9375,0.84375}{0.921875,0.828125}{0.00625}
\draw[] (0.875, 0.8125) rectangle (0.90625, 0.84375);% [-0.0256307, 0]
\PrecisionAchieved{0.875,0.8125}{0.90625,0.84375}{0.890625,0.828125}{0.00625}
\draw[] (0.96875, 0.78125) rectangle (1, 0.8125);% [-0.0186564, 0]
\PrecisionAchieved{0.96875,0.78125}{1,0.8125}{0.984375,0.796875}{0.00625}
\draw[] (0.9375, 0.78125) rectangle (0.96875, 0.8125);% [-0.0258229, 0]
\PrecisionAchieved{0.9375,0.78125}{0.96875,0.8125}{0.953125,0.796875}{0.00625}
\draw[] (0.96875, 0.75) rectangle (1, 0.78125);% [-0.0221457, 0]
\PrecisionAchieved{0.96875,0.75}{1,0.78125}{0.984375,0.765625}{0.00625}
\draw[] (0.9375, 0.75) rectangle (0.96875, 0.78125);% [-0.0318472, 0]
\PrecisionAchieved{0.9375,0.75}{0.96875,0.78125}{0.953125,0.765625}{0.00625}
\draw[] (0.90625, 0.78125) rectangle (0.9375, 0.8125);% [-0.0312224, 0]
\PrecisionAchieved{0.90625,0.78125}{0.9375,0.8125}{0.921875,0.796875}{0.00625}
\draw[] (0.875, 0.78125) rectangle (0.90625, 0.8125);% [-0.0335055, 0]
\PrecisionAchieved{0.875,0.78125}{0.90625,0.8125}{0.890625,0.796875}{0.00625}
\draw[] (0.90625, 0.75) rectangle (0.9375, 0.78125);% [-0.0395592, 0]
\PrecisionAchieved{0.90625,0.75}{0.9375,0.78125}{0.921875,0.765625}{0.00625}
\draw[] (0.875, 0.75) rectangle (0.90625, 0.78125);% [-0.043624, 0]
\PrecisionAchieved{0.875,0.75}{0.90625,0.78125}{0.890625,0.765625}{0.00625}
\draw[] (0.84375, 0.84375) rectangle (0.875, 0.875);% [-0.0180817, 0]
\PrecisionAchieved{0.84375,0.84375}{0.875,0.875}{0.859375,0.859375}{0.00625}
\draw[] (0.8125, 0.84375) rectangle (0.84375, 0.875);% [-0.0236217, 0]
\PrecisionAchieved{0.8125,0.84375}{0.84375,0.875}{0.828125,0.859375}{0.00625}
\draw[] (0.84375, 0.8125) rectangle (0.875, 0.84375);% [-0.0236217, 0]
\PrecisionAchieved{0.84375,0.8125}{0.875,0.84375}{0.859375,0.828125}{0.00625}
\draw[] (0.8125, 0.8125) rectangle (0.84375, 0.84375);% [-0.0180755, 0]
\PrecisionAchieved{0.8125,0.8125}{0.84375,0.84375}{0.828125,0.828125}{0.00625}
\draw[] (0.78125, 0.84375) rectangle (0.8125, 0.875);% [-0.0316975, 0]
\PrecisionAchieved{0.78125,0.84375}{0.8125,0.875}{0.796875,0.859375}{0.00625}
\draw[] (0.75, 0.84375) rectangle (0.78125, 0.875);% [-0.0428262, 0]
\PrecisionAchieved{0.75,0.84375}{0.78125,0.875}{0.765625,0.859375}{0.00625}
\draw[] (0.78125, 0.8125) rectangle (0.8125, 0.84375);% [-0.0253958, 0]
\PrecisionAchieved{0.78125,0.8125}{0.8125,0.84375}{0.796875,0.828125}{0.00625}
\draw[] (0.75, 0.8125) rectangle (0.78125, 0.84375);% [-0.036502, 0]
\PrecisionAchieved{0.75,0.8125}{0.78125,0.84375}{0.765625,0.828125}{0.00625}
\draw[] (0.84375, 0.78125) rectangle (0.875, 0.8125);% [-0.0316975, 0]
\PrecisionAchieved{0.84375,0.78125}{0.875,0.8125}{0.859375,0.796875}{0.00625}
\draw[] (0.8125, 0.78125) rectangle (0.84375, 0.8125);% [-0.0253958, 0]
\PrecisionAchieved{0.8125,0.78125}{0.84375,0.8125}{0.828125,0.796875}{0.00625}
\draw[] (0.84375, 0.75) rectangle (0.875, 0.78125);% [-0.0428262, 0]
\PrecisionAchieved{0.84375,0.75}{0.875,0.78125}{0.859375,0.765625}{0.00625}
\draw[] (0.8125, 0.75) rectangle (0.84375, 0.78125);% [-0.036502, 0]
\PrecisionAchieved{0.8125,0.75}{0.84375,0.78125}{0.828125,0.765625}{0.00625}
\draw[] (0.75, 0.75) rectangle (0.8125, 0.8125);% [-0.0373315, 0]
\PrecisionAchieved{0.75,0.75}{0.8125,0.8125}{0.78125,0.78125}{0.0125}
\draw[] (0.71875, 0.96875) rectangle (0.75, 1);% [-0.0254528, 0]
\PrecisionAchieved{0.71875,0.96875}{0.75,1}{0.734375,0.984375}{0.00625}
\draw[] (0.6875, 0.96875) rectangle (0.71875, 1);% [-0.028489, 0]
\PrecisionAchieved{0.6875,0.96875}{0.71875,1}{0.703125,0.984375}{0.00625}
\draw[] (0.71875, 0.9375) rectangle (0.75, 0.96875);% [-0.0390284, 0]
\PrecisionAchieved{0.71875,0.9375}{0.75,0.96875}{0.734375,0.953125}{0.00625}
\draw[] (0.6875, 0.9375) rectangle (0.71875, 0.96875);% [-0.0473243, 0]
\PrecisionAchieved{0.6875,0.9375}{0.71875,0.96875}{0.703125,0.953125}{0.00625}
\draw[] (0.65625, 0.96875) rectangle (0.6875, 1);% [-0.0311793, 0]
\PrecisionAchieved{0.65625,0.96875}{0.6875,1}{0.671875,0.984375}{0.00625}
\draw[] (0.625, 0.96875) rectangle (0.65625, 1);% [-0.0334617, 0]
\PrecisionAchieved{0.625,0.96875}{0.65625,1}{0.640625,0.984375}{0.00625}
\draw[] (0.65625, 0.9375) rectangle (0.6875, 0.96875);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.625, 0.9375) rectangle (0.65625, 0.96875);% [-0.0259361, -0.0244928]
\PrecisionAchieved{0.625,0.9375}{0.65625,0.96875}{0.640625,0.953125}{0.00625}
\draw[] (0.71875, 0.90625) rectangle (0.75, 0.9375);% [-0.050508, 0]
\draw[fill=\HigherOrderColor] (0.6875, 0.90625) rectangle (0.71875, 0.9375);% [-0.0245751, -0.0239929]
\PrecisionAchieved{0.6875,0.90625}{0.71875,0.9375}{0.703125,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.875) rectangle (0.75, 0.90625);% [-0.0215929, -0.0211726]
\PrecisionAchieved{0.71875,0.875}{0.75,0.90625}{0.734375,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.875) rectangle (0.71875, 0.90625);% [-0.0355016, -0.0353161]
\PrecisionAchieved{0.6875,0.875}{0.71875,0.90625}{0.703125,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.65625, 0.90625) rectangle (0.6875, 0.9375);% [-0.0363955, -0.0361427]
\PrecisionAchieved{0.65625,0.90625}{0.6875,0.9375}{0.671875,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.90625) rectangle (0.65625, 0.9375);% [-0.0506441, -0.0504214]
\PrecisionAchieved{0.625,0.90625}{0.65625,0.9375}{0.640625,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.65625, 0.875) rectangle (0.6875, 0.90625);% [-0.0532269, -0.053073]
\PrecisionAchieved{0.65625,0.875}{0.6875,0.90625}{0.671875,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.875) rectangle (0.65625, 0.90625);% [-0.0737784, -0.0736248]
\PrecisionAchieved{0.625,0.875}{0.65625,0.90625}{0.640625,0.890625}{0.00625}
\draw[] (0.59375, 0.96875) rectangle (0.625, 1);% [-0.0352867, 0]
\PrecisionAchieved{0.59375,0.96875}{0.625,1}{0.609375,0.984375}{0.00625}
\draw[] (0.5625, 0.96875) rectangle (0.59375, 1);% [-0.0366166, 0]
\PrecisionAchieved{0.5625,0.96875}{0.59375,1}{0.578125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.59375, 0.9375) rectangle (0.625, 0.96875);% [-0.0339776, -0.0334197]
\PrecisionAchieved{0.59375,0.9375}{0.625,0.96875}{0.609375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.9375) rectangle (0.59375, 0.96875);% [-0.0432031, -0.042753]
\PrecisionAchieved{0.5625,0.9375}{0.59375,0.96875}{0.578125,0.953125}{0.00625}
\draw[] (0.53125, 0.96875) rectangle (0.5625, 1);% [-0.0374249, 0]
\PrecisionAchieved{0.53125,0.96875}{0.5625,1}{0.546875,0.984375}{0.00625}
\draw[] (0.5, 0.96875) rectangle (0.53125, 1);% [-0.0376961, 0]
\PrecisionAchieved{0.5,0.96875}{0.53125,1}{0.515625,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.53125, 0.9375) rectangle (0.5625, 0.96875);% [-0.0528228, -0.0524048]
\PrecisionAchieved{0.53125,0.9375}{0.5625,0.96875}{0.546875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.9375) rectangle (0.53125, 0.96875);% [-0.0623243, -0.0619205]
\PrecisionAchieved{0.5,0.9375}{0.53125,0.96875}{0.515625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.875) rectangle (0.625, 0.9375);% [-0.0935202, -0.0877598]
\PrecisionAchieved{0.5625,0.875}{0.625,0.9375}{0.59375,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.875) rectangle (0.5625, 0.9375);% [-0.127849, -0.124431]
\PrecisionAchieved{0.5,0.875}{0.5625,0.9375}{0.53125,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.71875, 0.84375) rectangle (0.75, 0.875);% [-0.0246791, -0.0244497]
\PrecisionAchieved{0.71875,0.84375}{0.75,0.875}{0.734375,0.859375}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.84375) rectangle (0.71875, 0.875);% [-0.0426038, -0.0424524]
\PrecisionAchieved{0.6875,0.84375}{0.71875,0.875}{0.703125,0.859375}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.8125) rectangle (0.75, 0.84375);% [-0.0233757, -0.0230647]
\PrecisionAchieved{0.71875,0.8125}{0.75,0.84375}{0.734375,0.828125}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.8125) rectangle (0.71875, 0.84375);% [-0.0440094, -0.0438448]
\PrecisionAchieved{0.6875,0.8125}{0.71875,0.84375}{0.703125,0.828125}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.8125) rectangle (0.6875, 0.875);% [-0.083917, -0.0797423]
\PrecisionAchieved{0.625,0.8125}{0.6875,0.875}{0.65625,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.71875, 0.78125) rectangle (0.75, 0.8125);% [-0.0174752, -0.0167406]
\PrecisionAchieved{0.71875,0.78125}{0.75,0.8125}{0.734375,0.796875}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.78125) rectangle (0.71875, 0.8125);% [-0.0388906, -0.0386336]
\PrecisionAchieved{0.6875,0.78125}{0.71875,0.8125}{0.703125,0.796875}{0.00625}
\draw[] (0.71875, 0.75) rectangle (0.75, 0.78125);% [-0.0254528, 0]
\PrecisionAchieved{0.71875,0.75}{0.75,0.78125}{0.734375,0.765625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.75) rectangle (0.71875, 0.78125);% [-0.0275286, -0.0270409]
\PrecisionAchieved{0.6875,0.75}{0.71875,0.78125}{0.703125,0.765625}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.75) rectangle (0.6875, 0.8125);% [-0.0827364, -0.078422]
\PrecisionAchieved{0.625,0.75}{0.6875,0.8125}{0.65625,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.8125) rectangle (0.625, 0.875);% [-0.137758, -0.135382]
\PrecisionAchieved{0.5625,0.8125}{0.625,0.875}{0.59375,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.8125) rectangle (0.5625, 0.875);% [-0.174754, -0.172535]
\PrecisionAchieved{0.5,0.8125}{0.5625,0.875}{0.53125,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5625, 0.75) rectangle (0.625, 0.8125);% [-0.149499, -0.147395]
\PrecisionAchieved{0.5625,0.75}{0.625,0.8125}{0.59375,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.75) rectangle (0.5625, 0.8125);% [-0.181892, -0.17996]
\PrecisionAchieved{0.5,0.75}{0.5625,0.8125}{0.53125,0.78125}{0.0125}
\draw[] (0.96875, 0.71875) rectangle (1, 0.75);% [-0.0254528, 0]
\PrecisionAchieved{0.96875,0.71875}{1,0.75}{0.984375,0.734375}{0.00625}
\draw[] (0.9375, 0.71875) rectangle (0.96875, 0.75);% [-0.0390284, 0]
\PrecisionAchieved{0.9375,0.71875}{0.96875,0.75}{0.953125,0.734375}{0.00625}
\draw[] (0.96875, 0.6875) rectangle (1, 0.71875);% [-0.028489, 0]
\PrecisionAchieved{0.96875,0.6875}{1,0.71875}{0.984375,0.703125}{0.00625}
\draw[] (0.9375, 0.6875) rectangle (0.96875, 0.71875);% [-0.0473243, 0]
\PrecisionAchieved{0.9375,0.6875}{0.96875,0.71875}{0.953125,0.703125}{0.00625}
\draw[] (0.90625, 0.71875) rectangle (0.9375, 0.75);% [-0.050508, 0]
\draw[fill=\HigherOrderColor] (0.875, 0.71875) rectangle (0.90625, 0.75);% [-0.0215929, -0.0211726]
\PrecisionAchieved{0.875,0.71875}{0.90625,0.75}{0.890625,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.90625, 0.6875) rectangle (0.9375, 0.71875);% [-0.0245751, -0.0239929]
\PrecisionAchieved{0.90625,0.6875}{0.9375,0.71875}{0.921875,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.6875) rectangle (0.90625, 0.71875);% [-0.0355016, -0.0353161]
\PrecisionAchieved{0.875,0.6875}{0.90625,0.71875}{0.890625,0.703125}{0.00625}
\draw[] (0.96875, 0.65625) rectangle (1, 0.6875);% [-0.0311793, 0]
\PrecisionAchieved{0.96875,0.65625}{1,0.6875}{0.984375,0.671875}{0.00625}
\draw[] (0.9375, 0.65625) rectangle (0.96875, 0.6875);% [-0.056005, 0]
\draw[] (0.96875, 0.625) rectangle (1, 0.65625);% [-0.0334617, 0]
\PrecisionAchieved{0.96875,0.625}{1,0.65625}{0.984375,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.625) rectangle (0.96875, 0.65625);% [-0.0259361, -0.0244928]
\PrecisionAchieved{0.9375,0.625}{0.96875,0.65625}{0.953125,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.90625, 0.65625) rectangle (0.9375, 0.6875);% [-0.0363955, -0.0361427]
\PrecisionAchieved{0.90625,0.65625}{0.9375,0.6875}{0.921875,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.65625) rectangle (0.90625, 0.6875);% [-0.0532269, -0.053073]
\PrecisionAchieved{0.875,0.65625}{0.90625,0.6875}{0.890625,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.90625, 0.625) rectangle (0.9375, 0.65625);% [-0.0506441, -0.0504214]
\PrecisionAchieved{0.90625,0.625}{0.9375,0.65625}{0.921875,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.625) rectangle (0.90625, 0.65625);% [-0.0737784, -0.0736248]
\PrecisionAchieved{0.875,0.625}{0.90625,0.65625}{0.890625,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.84375, 0.71875) rectangle (0.875, 0.75);% [-0.0246791, -0.0244497]
\PrecisionAchieved{0.84375,0.71875}{0.875,0.75}{0.859375,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.71875) rectangle (0.84375, 0.75);% [-0.0233757, -0.0230647]
\PrecisionAchieved{0.8125,0.71875}{0.84375,0.75}{0.828125,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.84375, 0.6875) rectangle (0.875, 0.71875);% [-0.0426038, -0.0424524]
\PrecisionAchieved{0.84375,0.6875}{0.875,0.71875}{0.859375,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.6875) rectangle (0.84375, 0.71875);% [-0.0440094, -0.0438448]
\PrecisionAchieved{0.8125,0.6875}{0.84375,0.71875}{0.828125,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.78125, 0.71875) rectangle (0.8125, 0.75);% [-0.0174752, -0.0167406]
\PrecisionAchieved{0.78125,0.71875}{0.8125,0.75}{0.796875,0.734375}{0.00625}
\draw[] (0.75, 0.71875) rectangle (0.78125, 0.75);% [-0.0254528, 0]
\PrecisionAchieved{0.75,0.71875}{0.78125,0.75}{0.765625,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.78125, 0.6875) rectangle (0.8125, 0.71875);% [-0.0388906, -0.0386336]
\PrecisionAchieved{0.78125,0.6875}{0.8125,0.71875}{0.796875,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.75, 0.6875) rectangle (0.78125, 0.71875);% [-0.0275286, -0.0270409]
\PrecisionAchieved{0.75,0.6875}{0.78125,0.71875}{0.765625,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.625) rectangle (0.875, 0.6875);% [-0.083917, -0.0797423]
\PrecisionAchieved{0.8125,0.625}{0.875,0.6875}{0.84375,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.625) rectangle (0.8125, 0.6875);% [-0.0827364, -0.078422]
\PrecisionAchieved{0.75,0.625}{0.8125,0.6875}{0.78125,0.65625}{0.0125}
\draw[] (0.96875, 0.59375) rectangle (1, 0.625);% [-0.0352867, 0]
\PrecisionAchieved{0.96875,0.59375}{1,0.625}{0.984375,0.609375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.59375) rectangle (0.96875, 0.625);% [-0.0339776, -0.0334197]
\PrecisionAchieved{0.9375,0.59375}{0.96875,0.625}{0.953125,0.609375}{0.00625}
\draw[] (0.96875, 0.5625) rectangle (1, 0.59375);% [-0.0366166, 0]
\PrecisionAchieved{0.96875,0.5625}{1,0.59375}{0.984375,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.5625) rectangle (0.96875, 0.59375);% [-0.0432031, -0.042753]
\PrecisionAchieved{0.9375,0.5625}{0.96875,0.59375}{0.953125,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.5625) rectangle (0.9375, 0.625);% [-0.0935202, -0.0877598]
\PrecisionAchieved{0.875,0.5625}{0.9375,0.625}{0.90625,0.59375}{0.0125}
\draw[] (0.96875, 0.53125) rectangle (1, 0.5625);% [-0.0374249, 0]
\PrecisionAchieved{0.96875,0.53125}{1,0.5625}{0.984375,0.546875}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.53125) rectangle (0.96875, 0.5625);% [-0.0528228, -0.0524048]
\PrecisionAchieved{0.9375,0.53125}{0.96875,0.5625}{0.953125,0.546875}{0.00625}
\draw[] (0.96875, 0.5) rectangle (1, 0.53125);% [-0.0376961, 0]
\PrecisionAchieved{0.96875,0.5}{1,0.53125}{0.984375,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.5) rectangle (0.96875, 0.53125);% [-0.0623243, -0.0619205]
\PrecisionAchieved{0.9375,0.5}{0.96875,0.53125}{0.953125,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.5) rectangle (0.9375, 0.5625);% [-0.127849, -0.124431]
\PrecisionAchieved{0.875,0.5}{0.9375,0.5625}{0.90625,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.5625) rectangle (0.875, 0.625);% [-0.137758, -0.135382]
\PrecisionAchieved{0.8125,0.5625}{0.875,0.625}{0.84375,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.5625) rectangle (0.8125, 0.625);% [-0.149499, -0.147395]
\PrecisionAchieved{0.75,0.5625}{0.8125,0.625}{0.78125,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.8125, 0.5) rectangle (0.875, 0.5625);% [-0.174754, -0.172535]
\PrecisionAchieved{0.8125,0.5}{0.875,0.5625}{0.84375,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.5) rectangle (0.8125, 0.5625);% [-0.181892, -0.17996]
\PrecisionAchieved{0.75,0.5}{0.8125,0.5625}{0.78125,0.53125}{0.0125}
\draw[] (0.6875, 0.6875) rectangle (0.75, 0.75);% [-0.0328859, 0]
\PrecisionAchieved{0.6875,0.6875}{0.75,0.75}{0.71875,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.65625, 0.71875) rectangle (0.6875, 0.75);% [-0.0397028, -0.0391373]
\PrecisionAchieved{0.65625,0.71875}{0.6875,0.75}{0.671875,0.734375}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.71875) rectangle (0.65625, 0.75);% [-0.0781648, -0.0778609]
\PrecisionAchieved{0.625,0.71875}{0.65625,0.75}{0.640625,0.734375}{0.00625}
\draw[] (0.65625, 0.6875) rectangle (0.6875, 0.71875);% [-0.0457006, 0]
\PrecisionAchieved{0.65625,0.6875}{0.6875,0.71875}{0.671875,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.6875) rectangle (0.65625, 0.71875);% [-0.052898, -0.0521554]
\PrecisionAchieved{0.625,0.6875}{0.65625,0.71875}{0.640625,0.703125}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.65625) rectangle (0.75, 0.6875);% [-0.0397028, -0.0391373]
\PrecisionAchieved{0.71875,0.65625}{0.75,0.6875}{0.734375,0.671875}{0.00625}
\draw[] (0.6875, 0.65625) rectangle (0.71875, 0.6875);% [-0.0457006, 0]
\PrecisionAchieved{0.6875,0.65625}{0.71875,0.6875}{0.703125,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.71875, 0.625) rectangle (0.75, 0.65625);% [-0.0781648, -0.0778609]
\PrecisionAchieved{0.71875,0.625}{0.75,0.65625}{0.734375,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.625) rectangle (0.71875, 0.65625);% [-0.052898, -0.0521554]
\PrecisionAchieved{0.6875,0.625}{0.71875,0.65625}{0.703125,0.640625}{0.00625}
\draw[] (0.65625, 0.65625) rectangle (0.6875, 0.6875);% [-0.0185805, 0]
\PrecisionAchieved{0.65625,0.65625}{0.6875,0.6875}{0.671875,0.671875}{0.00625}
\draw[] (0.625, 0.65625) rectangle (0.65625, 0.6875);% [-0.058991, 0]
\draw[] (0.65625, 0.625) rectangle (0.6875, 0.65625);% [-0.058991, 0]
\draw[] (0.625, 0.625) rectangle (0.65625, 0.65625);% [-0.0238312, 0]
\PrecisionAchieved{0.625,0.625}{0.65625,0.65625}{0.640625,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.6875) rectangle (0.625, 0.75);% [-0.13095, -0.127149]
\PrecisionAchieved{0.5625,0.6875}{0.625,0.75}{0.59375,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.6875) rectangle (0.5625, 0.75);% [-0.179991, -0.177648]
\PrecisionAchieved{0.5,0.6875}{0.5625,0.75}{0.53125,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.59375, 0.65625) rectangle (0.625, 0.6875);% [-0.0658831, -0.0649798]
\PrecisionAchieved{0.59375,0.65625}{0.625,0.6875}{0.609375,0.671875}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.65625) rectangle (0.59375, 0.6875);% [-0.115611, -0.11519]
\PrecisionAchieved{0.5625,0.65625}{0.59375,0.6875}{0.578125,0.671875}{0.00625}
\draw[] (0.59375, 0.625) rectangle (0.625, 0.65625);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.5625, 0.625) rectangle (0.59375, 0.65625);% [-0.0775213, -0.0764971]
\PrecisionAchieved{0.5625,0.625}{0.59375,0.65625}{0.578125,0.640625}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.625) rectangle (0.5625, 0.6875);% [-0.160944, -0.156768]
\PrecisionAchieved{0.5,0.625}{0.5625,0.6875}{0.53125,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.6875, 0.5625) rectangle (0.75, 0.625);% [-0.13095, -0.127149]
\PrecisionAchieved{0.6875,0.5625}{0.75,0.625}{0.71875,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.65625, 0.59375) rectangle (0.6875, 0.625);% [-0.0658831, -0.0649798]
\PrecisionAchieved{0.65625,0.59375}{0.6875,0.625}{0.671875,0.609375}{0.00625}
\draw[] (0.625, 0.59375) rectangle (0.65625, 0.625);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.65625, 0.5625) rectangle (0.6875, 0.59375);% [-0.115611, -0.11519]
\PrecisionAchieved{0.65625,0.5625}{0.6875,0.59375}{0.671875,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.5625) rectangle (0.65625, 0.59375);% [-0.0775213, -0.0764971]
\PrecisionAchieved{0.625,0.5625}{0.65625,0.59375}{0.640625,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.5) rectangle (0.75, 0.5625);% [-0.179991, -0.177648]
\PrecisionAchieved{0.6875,0.5}{0.75,0.5625}{0.71875,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.5) rectangle (0.6875, 0.5625);% [-0.160944, -0.156768]
\PrecisionAchieved{0.625,0.5}{0.6875,0.5625}{0.65625,0.53125}{0.0125}
\draw[] (0.59375, 0.59375) rectangle (0.625, 0.625);% [-0.0288048, 0]
\PrecisionAchieved{0.59375,0.59375}{0.625,0.625}{0.609375,0.609375}{0.00625}
\draw[] (0.5625, 0.59375) rectangle (0.59375, 0.625);% [-0.0823766, 0]
\draw[] (0.59375, 0.5625) rectangle (0.625, 0.59375);% [-0.0823766, 0]
\draw[] (0.5625, 0.5625) rectangle (0.59375, 0.59375);% [-0.0330265, 0]
\PrecisionAchieved{0.5625,0.5625}{0.59375,0.59375}{0.578125,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.53125, 0.59375) rectangle (0.5625, 0.625);% [-0.0869012, -0.0858123]
\PrecisionAchieved{0.53125,0.59375}{0.5625,0.625}{0.546875,0.609375}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.59375) rectangle (0.53125, 0.625);% [-0.139353, -0.138895]
\PrecisionAchieved{0.5,0.59375}{0.53125,0.625}{0.515625,0.609375}{0.00625}
\draw[] (0.53125, 0.5625) rectangle (0.5625, 0.59375);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.5, 0.5625) rectangle (0.53125, 0.59375);% [-0.0934099, -0.0923178]
\PrecisionAchieved{0.5,0.5625}{0.53125,0.59375}{0.515625,0.578125}{0.00625}
\draw[fill=\HigherOrderColor] (0.59375, 0.53125) rectangle (0.625, 0.5625);% [-0.0869012, -0.0858123]
\PrecisionAchieved{0.59375,0.53125}{0.625,0.5625}{0.609375,0.546875}{0.00625}
\draw[] (0.5625, 0.53125) rectangle (0.59375, 0.5625);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.59375, 0.5) rectangle (0.625, 0.53125);% [-0.139353, -0.138895]
\PrecisionAchieved{0.59375,0.5}{0.625,0.53125}{0.609375,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.5) rectangle (0.59375, 0.53125);% [-0.0934099, -0.0923178]
\PrecisionAchieved{0.5625,0.5}{0.59375,0.53125}{0.578125,0.515625}{0.00625}
\draw[] (0.53125, 0.53125) rectangle (0.5625, 0.5625);% [-0.0360884, 0]
\PrecisionAchieved{0.53125,0.53125}{0.5625,0.5625}{0.546875,0.546875}{0.00625}
\draw[] (0.5, 0.53125) rectangle (0.53125, 0.5625);% [-0.0957117, 0]
\draw[] (0.53125, 0.5) rectangle (0.5625, 0.53125);% [-0.0957117, 0]
\draw[] (0.5, 0.5) rectangle (0.53125, 0.53125);% [-0.0376961, 0]
\PrecisionAchieved{0.5,0.5}{0.53125,0.53125}{0.515625,0.515625}{0.00625}
\draw[] (0.46875, 0.96875) rectangle (0.5, 1);% [-0.0433027, 0]
\PrecisionAchieved{0.46875,0.96875}{0.5,1}{0.484375,0.984375}{0.00625}
\draw[] (0.4375, 0.96875) rectangle (0.46875, 1);% [-0.0485429, 0]
\PrecisionAchieved{0.4375,0.96875}{0.46875,1}{0.453125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.46875, 0.9375) rectangle (0.5, 0.96875);% [-0.0712278, -0.0708219]
\PrecisionAchieved{0.46875,0.9375}{0.5,0.96875}{0.484375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.9375) rectangle (0.46875, 0.96875);% [-0.079113, -0.0786605]
\PrecisionAchieved{0.4375,0.9375}{0.46875,0.96875}{0.453125,0.953125}{0.00625}
\draw[] (0.40625, 0.96875) rectangle (0.4375, 1);% [-0.0528588, 0]
\draw[] (0.375, 0.96875) rectangle (0.40625, 1);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.40625, 0.9375) rectangle (0.4375, 0.96875);% [-0.0855846, -0.0851018]
\PrecisionAchieved{0.40625,0.9375}{0.4375,0.96875}{0.421875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.9375) rectangle (0.40625, 0.96875);% [-0.0903529, -0.0898592]
\PrecisionAchieved{0.375,0.9375}{0.40625,0.96875}{0.390625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.875) rectangle (0.5, 0.9375);% [-0.153054, -0.150215]
\PrecisionAchieved{0.4375,0.875}{0.5,0.9375}{0.46875,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.875) rectangle (0.4375, 0.9375);% [-0.166337, -0.163336]
\PrecisionAchieved{0.375,0.875}{0.4375,0.9375}{0.40625,0.90625}{0.0125}
\draw[] (0.34375, 0.96875) rectangle (0.375, 1);% [-0.057785, 0]
\draw[] (0.3125, 0.96875) rectangle (0.34375, 1);% [-0.058056, 0]
\draw[fill=\HigherOrderColor] (0.34375, 0.9375) rectangle (0.375, 0.96875);% [-0.0931972, -0.0927126]
\PrecisionAchieved{0.34375,0.9375}{0.375,0.96875}{0.359375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.9375) rectangle (0.34375, 0.96875);% [-0.093953, -0.093489]
\PrecisionAchieved{0.3125,0.9375}{0.34375,0.96875}{0.328125,0.953125}{0.00625}
\draw[] (0.28125, 0.96875) rectangle (0.3125, 1);% [-0.0567321, 0]
\draw[] (0.25, 0.96875) rectangle (0.28125, 1);% [-0.0537898, 0]
\draw[fill=\HigherOrderColor] (0.28125, 0.9375) rectangle (0.3125, 0.96875);% [-0.0925069, -0.0920331]
\PrecisionAchieved{0.28125,0.9375}{0.3125,0.96875}{0.296875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.9375) rectangle (0.28125, 0.96875);% [-0.0887299, -0.0882644]
\PrecisionAchieved{0.25,0.9375}{0.28125,0.96875}{0.265625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.875) rectangle (0.375, 0.9375);% [-0.170389, -0.167579]
\PrecisionAchieved{0.3125,0.875}{0.375,0.9375}{0.34375,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.875) rectangle (0.3125, 0.9375);% [-0.168545, -0.165707]
\PrecisionAchieved{0.25,0.875}{0.3125,0.9375}{0.28125,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.75) rectangle (0.5, 0.875);% [-0.162335, -0.121901]
\PrecisionAchieved{0.375,0.75}{0.5,0.875}{0.4375,0.8125}{0.025}
\draw[fill=\HigherOrderColor] (0.25, 0.75) rectangle (0.375, 0.875);% [-0.105502, -0.0615991]
\PrecisionAchieved{0.25,0.75}{0.375,0.875}{0.3125,0.8125}{0.025}
\draw[] (0.21875, 0.96875) rectangle (0.25, 1);% [-0.0498517, 0]
\PrecisionAchieved{0.21875,0.96875}{0.25,1}{0.234375,0.984375}{0.00625}
\draw[] (0.1875, 0.96875) rectangle (0.21875, 1);% [-0.0449984, 0]
\PrecisionAchieved{0.1875,0.96875}{0.21875,1}{0.203125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.21875, 0.9375) rectangle (0.25, 0.96875);% [-0.0825715, -0.0821088]
\PrecisionAchieved{0.21875,0.9375}{0.25,0.96875}{0.234375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.9375) rectangle (0.21875, 0.96875);% [-0.0740435, -0.0735891]
\PrecisionAchieved{0.1875,0.9375}{0.21875,0.96875}{0.203125,0.953125}{0.00625}
\draw[] (0.15625, 0.96875) rectangle (0.1875, 1);% [-0.0388125, 0]
\PrecisionAchieved{0.15625,0.96875}{0.1875,1}{0.171875,0.984375}{0.00625}
\draw[] (0.125, 0.96875) rectangle (0.15625, 1);% [-0.0315693, 0]
\PrecisionAchieved{0.125,0.96875}{0.15625,1}{0.140625,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.15625, 0.9375) rectangle (0.1875, 0.96875);% [-0.0632948, -0.0628678]
\PrecisionAchieved{0.15625,0.9375}{0.1875,0.96875}{0.171875,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.9375) rectangle (0.15625, 0.96875);% [-0.0506974, -0.0503137]
\PrecisionAchieved{0.125,0.9375}{0.15625,0.96875}{0.140625,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.875) rectangle (0.25, 0.9375);% [-0.157884, -0.154558]
\PrecisionAchieved{0.1875,0.875}{0.25,0.9375}{0.21875,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.875) rectangle (0.1875, 0.9375);% [-0.129493, -0.125514]
\PrecisionAchieved{0.125,0.875}{0.1875,0.9375}{0.15625,0.90625}{0.0125}
\draw[] (0.09375, 0.96875) rectangle (0.125, 1);% [-0.0236772, 0]
\PrecisionAchieved{0.09375,0.96875}{0.125,1}{0.109375,0.984375}{0.00625}
\draw[] (0.0625, 0.96875) rectangle (0.09375, 1);% [-0.015697, 0]
\PrecisionAchieved{0.0625,0.96875}{0.09375,1}{0.078125,0.984375}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.9375) rectangle (0.125, 0.96875);% [-0.0369255, -0.0365921]
\PrecisionAchieved{0.09375,0.9375}{0.125,0.96875}{0.109375,0.953125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.9375) rectangle (0.09375, 0.96875);% [-0.0230462, -0.0227563]
\PrecisionAchieved{0.0625,0.9375}{0.09375,0.96875}{0.078125,0.953125}{0.00625}
\draw[] (0, 0.9375) rectangle (0.0625, 1);% [-0.0250627, 0]
\PrecisionAchieved{0,0.9375}{0.0625,1}{0.03125,0.96875}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.875) rectangle (0.125, 0.9375);% [-0.0784735, -0.0736601]
\PrecisionAchieved{0.0625,0.875}{0.125,0.9375}{0.09375,0.90625}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.90625) rectangle (0.0625, 0.9375);% [-0.0230462, -0.0227563]
\PrecisionAchieved{0.03125,0.90625}{0.0625,0.9375}{0.046875,0.921875}{0.00625}
\draw[] (0, 0.90625) rectangle (0.03125, 0.9375);% [-0.015697, 0]
\PrecisionAchieved{0,0.90625}{0.03125,0.9375}{0.015625,0.921875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.875) rectangle (0.0625, 0.90625);% [-0.0369255, -0.0365921]
\PrecisionAchieved{0.03125,0.875}{0.0625,0.90625}{0.046875,0.890625}{0.00625}
\draw[] (0, 0.875) rectangle (0.03125, 0.90625);% [-0.0236772, 0]
\PrecisionAchieved{0,0.875}{0.03125,0.90625}{0.015625,0.890625}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.75) rectangle (0.25, 0.875);% [-0.177979, -0.129661]
\PrecisionAchieved{0.125,0.75}{0.25,0.875}{0.1875,0.8125}{0.025}
\draw[fill=\HigherOrderColor] (0.0625, 0.8125) rectangle (0.125, 0.875);% [-0.129493, -0.125514]
\PrecisionAchieved{0.0625,0.8125}{0.125,0.875}{0.09375,0.84375}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.84375) rectangle (0.0625, 0.875);% [-0.0506974, -0.0503137]
\PrecisionAchieved{0.03125,0.84375}{0.0625,0.875}{0.046875,0.859375}{0.00625}
\draw[] (0, 0.84375) rectangle (0.03125, 0.875);% [-0.0315693, 0]
\PrecisionAchieved{0,0.84375}{0.03125,0.875}{0.015625,0.859375}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.8125) rectangle (0.0625, 0.84375);% [-0.0632948, -0.0628678]
\PrecisionAchieved{0.03125,0.8125}{0.0625,0.84375}{0.046875,0.828125}{0.00625}
\draw[] (0, 0.8125) rectangle (0.03125, 0.84375);% [-0.0388125, 0]
\PrecisionAchieved{0,0.8125}{0.03125,0.84375}{0.015625,0.828125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.75) rectangle (0.125, 0.8125);% [-0.157884, -0.154558]
\PrecisionAchieved{0.0625,0.75}{0.125,0.8125}{0.09375,0.78125}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.78125) rectangle (0.0625, 0.8125);% [-0.0740435, -0.0735891]
\PrecisionAchieved{0.03125,0.78125}{0.0625,0.8125}{0.046875,0.796875}{0.00625}
\draw[] (0, 0.78125) rectangle (0.03125, 0.8125);% [-0.0449984, 0]
\PrecisionAchieved{0,0.78125}{0.03125,0.8125}{0.015625,0.796875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.75) rectangle (0.0625, 0.78125);% [-0.0825715, -0.0821088]
\PrecisionAchieved{0.03125,0.75}{0.0625,0.78125}{0.046875,0.765625}{0.00625}
\draw[] (0, 0.75) rectangle (0.03125, 0.78125);% [-0.0498517, 0]
\PrecisionAchieved{0,0.75}{0.03125,0.78125}{0.015625,0.765625}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.625) rectangle (0.5, 0.75);% [-0.130874, -0.0819702]
\PrecisionAchieved{0.375,0.625}{0.5,0.75}{0.4375,0.6875}{0.025}
\draw[fill=\HigherOrderColor] (0.25, 0.625) rectangle (0.375, 0.75);% [0.0387812, 0.0753957]
\PrecisionAchieved{0.25,0.625}{0.375,0.75}{0.3125,0.6875}{0.025}
\draw[fill=\HigherOrderColor] (0.4375, 0.5625) rectangle (0.5, 0.625);% [-0.170799, -0.16686]
\PrecisionAchieved{0.4375,0.5625}{0.5,0.625}{0.46875,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.5625) rectangle (0.4375, 0.625);% [-0.157502, -0.153137]
\PrecisionAchieved{0.375,0.5625}{0.4375,0.625}{0.40625,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.46875, 0.53125) rectangle (0.5, 0.5625);% [-0.0967344, -0.0956435]
\PrecisionAchieved{0.46875,0.53125}{0.5,0.5625}{0.484375,0.546875}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.53125) rectangle (0.46875, 0.5625);% [-0.146956, -0.146476]
\PrecisionAchieved{0.4375,0.53125}{0.46875,0.5625}{0.453125,0.546875}{0.00625}
\draw[] (0.46875, 0.5) rectangle (0.5, 0.53125);% [-0.0980218, 0]
\draw[fill=\HigherOrderColor] (0.4375, 0.5) rectangle (0.46875, 0.53125);% [-0.0967344, -0.0956435]
\PrecisionAchieved{0.4375,0.5}{0.46875,0.53125}{0.453125,0.515625}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.5) rectangle (0.4375, 0.5625);% [-0.170799, -0.16686]
\PrecisionAchieved{0.375,0.5}{0.4375,0.5625}{0.40625,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.5) rectangle (0.375, 0.625);% [-0.130874, -0.0819702]
\PrecisionAchieved{0.25,0.5}{0.375,0.625}{0.3125,0.5625}{0.025}
\draw[fill=\HigherOrderColor] (0.125, 0.625) rectangle (0.25, 0.75);% [-0.105502, -0.0615991]
\PrecisionAchieved{0.125,0.625}{0.25,0.75}{0.1875,0.6875}{0.025}
\draw[fill=\HigherOrderColor] (0.0625, 0.6875) rectangle (0.125, 0.75);% [-0.168545, -0.165707]
\PrecisionAchieved{0.0625,0.6875}{0.125,0.75}{0.09375,0.71875}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.71875) rectangle (0.0625, 0.75);% [-0.0887299, -0.0882644]
\PrecisionAchieved{0.03125,0.71875}{0.0625,0.75}{0.046875,0.734375}{0.00625}
\draw[] (0, 0.71875) rectangle (0.03125, 0.75);% [-0.0537898, 0]
\draw[fill=\HigherOrderColor] (0.03125, 0.6875) rectangle (0.0625, 0.71875);% [-0.0925069, -0.0920331]
\PrecisionAchieved{0.03125,0.6875}{0.0625,0.71875}{0.046875,0.703125}{0.00625}
\draw[] (0, 0.6875) rectangle (0.03125, 0.71875);% [-0.0567321, 0]
\draw[fill=\HigherOrderColor] (0.0625, 0.625) rectangle (0.125, 0.6875);% [-0.170389, -0.167579]
\PrecisionAchieved{0.0625,0.625}{0.125,0.6875}{0.09375,0.65625}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.65625) rectangle (0.0625, 0.6875);% [-0.093953, -0.093489]
\PrecisionAchieved{0.03125,0.65625}{0.0625,0.6875}{0.046875,0.671875}{0.00625}
\draw[] (0, 0.65625) rectangle (0.03125, 0.6875);% [-0.058056, 0]
\draw[fill=\HigherOrderColor] (0.03125, 0.625) rectangle (0.0625, 0.65625);% [-0.0931972, -0.0927126]
\PrecisionAchieved{0.03125,0.625}{0.0625,0.65625}{0.046875,0.640625}{0.00625}
\draw[] (0, 0.625) rectangle (0.03125, 0.65625);% [-0.057785, 0]
\draw[fill=\HigherOrderColor] (0.125, 0.5) rectangle (0.25, 0.625);% [-0.162335, -0.121901]
\PrecisionAchieved{0.125,0.5}{0.25,0.625}{0.1875,0.5625}{0.025}
\draw[fill=\HigherOrderColor] (0.0625, 0.5625) rectangle (0.125, 0.625);% [-0.166337, -0.163336]
\PrecisionAchieved{0.0625,0.5625}{0.125,0.625}{0.09375,0.59375}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.59375) rectangle (0.0625, 0.625);% [-0.0903529, -0.0898592]
\PrecisionAchieved{0.03125,0.59375}{0.0625,0.625}{0.046875,0.609375}{0.00625}
\draw[] (0, 0.59375) rectangle (0.03125, 0.625);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.03125, 0.5625) rectangle (0.0625, 0.59375);% [-0.0855846, -0.0851018]
\PrecisionAchieved{0.03125,0.5625}{0.0625,0.59375}{0.046875,0.578125}{0.00625}
\draw[] (0, 0.5625) rectangle (0.03125, 0.59375);% [-0.0528588, 0]
\draw[fill=\HigherOrderColor] (0.0625, 0.5) rectangle (0.125, 0.5625);% [-0.153054, -0.150215]
\PrecisionAchieved{0.0625,0.5}{0.125,0.5625}{0.09375,0.53125}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.53125) rectangle (0.0625, 0.5625);% [-0.079113, -0.0786605]
\PrecisionAchieved{0.03125,0.53125}{0.0625,0.5625}{0.046875,0.546875}{0.00625}
\draw[] (0, 0.53125) rectangle (0.03125, 0.5625);% [-0.0485429, 0]
\PrecisionAchieved{0,0.53125}{0.03125,0.5625}{0.015625,0.546875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.5) rectangle (0.0625, 0.53125);% [-0.0712278, -0.0708219]
\PrecisionAchieved{0.03125,0.5}{0.0625,0.53125}{0.046875,0.515625}{0.00625}
\draw[] (0, 0.5) rectangle (0.03125, 0.53125);% [-0.0433027, 0]
\PrecisionAchieved{0,0.5}{0.03125,0.53125}{0.015625,0.515625}{0.00625}
\draw[] (0.96875, 0.46875) rectangle (1, 0.5);% [-0.0433027, 0]
\PrecisionAchieved{0.96875,0.46875}{1,0.5}{0.984375,0.484375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.46875) rectangle (0.96875, 0.5);% [-0.0712278, -0.0708219]
\PrecisionAchieved{0.9375,0.46875}{0.96875,0.5}{0.953125,0.484375}{0.00625}
\draw[] (0.96875, 0.4375) rectangle (1, 0.46875);% [-0.0485429, 0]
\PrecisionAchieved{0.96875,0.4375}{1,0.46875}{0.984375,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.4375) rectangle (0.96875, 0.46875);% [-0.079113, -0.0786605]
\PrecisionAchieved{0.9375,0.4375}{0.96875,0.46875}{0.953125,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.4375) rectangle (0.9375, 0.5);% [-0.153054, -0.150215]
\PrecisionAchieved{0.875,0.4375}{0.9375,0.5}{0.90625,0.46875}{0.0125}
\draw[] (0.96875, 0.40625) rectangle (1, 0.4375);% [-0.0528588, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.40625) rectangle (0.96875, 0.4375);% [-0.0855846, -0.0851018]
\PrecisionAchieved{0.9375,0.40625}{0.96875,0.4375}{0.953125,0.421875}{0.00625}
\draw[] (0.96875, 0.375) rectangle (1, 0.40625);% [-0.056005, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.375) rectangle (0.96875, 0.40625);% [-0.0903529, -0.0898592]
\PrecisionAchieved{0.9375,0.375}{0.96875,0.40625}{0.953125,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.375) rectangle (0.9375, 0.4375);% [-0.166337, -0.163336]
\PrecisionAchieved{0.875,0.375}{0.9375,0.4375}{0.90625,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.375) rectangle (0.875, 0.5);% [-0.162335, -0.121901]
\PrecisionAchieved{0.75,0.375}{0.875,0.5}{0.8125,0.4375}{0.025}
\draw[] (0.96875, 0.34375) rectangle (1, 0.375);% [-0.057785, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.34375) rectangle (0.96875, 0.375);% [-0.0931972, -0.0927126]
\PrecisionAchieved{0.9375,0.34375}{0.96875,0.375}{0.953125,0.359375}{0.00625}
\draw[] (0.96875, 0.3125) rectangle (1, 0.34375);% [-0.058056, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.3125) rectangle (0.96875, 0.34375);% [-0.093953, -0.093489]
\PrecisionAchieved{0.9375,0.3125}{0.96875,0.34375}{0.953125,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.3125) rectangle (0.9375, 0.375);% [-0.170389, -0.167579]
\PrecisionAchieved{0.875,0.3125}{0.9375,0.375}{0.90625,0.34375}{0.0125}
\draw[] (0.96875, 0.28125) rectangle (1, 0.3125);% [-0.0567321, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.28125) rectangle (0.96875, 0.3125);% [-0.0925069, -0.0920331]
\PrecisionAchieved{0.9375,0.28125}{0.96875,0.3125}{0.953125,0.296875}{0.00625}
\draw[] (0.96875, 0.25) rectangle (1, 0.28125);% [-0.0537898, 0]
\draw[fill=\HigherOrderColor] (0.9375, 0.25) rectangle (0.96875, 0.28125);% [-0.0887299, -0.0882644]
\PrecisionAchieved{0.9375,0.25}{0.96875,0.28125}{0.953125,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.25) rectangle (0.9375, 0.3125);% [-0.168545, -0.165707]
\PrecisionAchieved{0.875,0.25}{0.9375,0.3125}{0.90625,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.25) rectangle (0.875, 0.375);% [-0.105502, -0.0615991]
\PrecisionAchieved{0.75,0.25}{0.875,0.375}{0.8125,0.3125}{0.025}
\draw[fill=\HigherOrderColor] (0.625, 0.375) rectangle (0.75, 0.5);% [-0.130874, -0.0819702]
\PrecisionAchieved{0.625,0.375}{0.75,0.5}{0.6875,0.4375}{0.025}
\draw[fill=\HigherOrderColor] (0.5625, 0.4375) rectangle (0.625, 0.5);% [-0.170799, -0.16686]
\PrecisionAchieved{0.5625,0.4375}{0.625,0.5}{0.59375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.53125, 0.46875) rectangle (0.5625, 0.5);% [-0.0967344, -0.0956435]
\PrecisionAchieved{0.53125,0.46875}{0.5625,0.5}{0.546875,0.484375}{0.00625}
\draw[] (0.5, 0.46875) rectangle (0.53125, 0.5);% [-0.0980218, 0]
\draw[fill=\HigherOrderColor] (0.53125, 0.4375) rectangle (0.5625, 0.46875);% [-0.146956, -0.146476]
\PrecisionAchieved{0.53125,0.4375}{0.5625,0.46875}{0.546875,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.4375) rectangle (0.53125, 0.46875);% [-0.0967344, -0.0956435]
\PrecisionAchieved{0.5,0.4375}{0.53125,0.46875}{0.515625,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.375) rectangle (0.625, 0.4375);% [-0.157502, -0.153137]
\PrecisionAchieved{0.5625,0.375}{0.625,0.4375}{0.59375,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.375) rectangle (0.5625, 0.4375);% [-0.170799, -0.16686]
\PrecisionAchieved{0.5,0.375}{0.5625,0.4375}{0.53125,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.25) rectangle (0.75, 0.375);% [0.0387812, 0.0753957]
\PrecisionAchieved{0.625,0.25}{0.75,0.375}{0.6875,0.3125}{0.025}
\draw[fill=\HigherOrderColor] (0.5, 0.25) rectangle (0.625, 0.375);% [-0.130874, -0.0819702]
\PrecisionAchieved{0.5,0.25}{0.625,0.375}{0.5625,0.3125}{0.025}
\draw[] (0.96875, 0.21875) rectangle (1, 0.25);% [-0.0498517, 0]
\PrecisionAchieved{0.96875,0.21875}{1,0.25}{0.984375,0.234375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.21875) rectangle (0.96875, 0.25);% [-0.0825715, -0.0821088]
\PrecisionAchieved{0.9375,0.21875}{0.96875,0.25}{0.953125,0.234375}{0.00625}
\draw[] (0.96875, 0.1875) rectangle (1, 0.21875);% [-0.0449984, 0]
\PrecisionAchieved{0.96875,0.1875}{1,0.21875}{0.984375,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.1875) rectangle (0.96875, 0.21875);% [-0.0740435, -0.0735891]
\PrecisionAchieved{0.9375,0.1875}{0.96875,0.21875}{0.953125,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.1875) rectangle (0.9375, 0.25);% [-0.157884, -0.154558]
\PrecisionAchieved{0.875,0.1875}{0.9375,0.25}{0.90625,0.21875}{0.0125}
\draw[] (0.96875, 0.15625) rectangle (1, 0.1875);% [-0.0388125, 0]
\PrecisionAchieved{0.96875,0.15625}{1,0.1875}{0.984375,0.171875}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.15625) rectangle (0.96875, 0.1875);% [-0.0632948, -0.0628678]
\PrecisionAchieved{0.9375,0.15625}{0.96875,0.1875}{0.953125,0.171875}{0.00625}
\draw[] (0.96875, 0.125) rectangle (1, 0.15625);% [-0.0315693, 0]
\PrecisionAchieved{0.96875,0.125}{1,0.15625}{0.984375,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.125) rectangle (0.96875, 0.15625);% [-0.0506974, -0.0503137]
\PrecisionAchieved{0.9375,0.125}{0.96875,0.15625}{0.953125,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.125) rectangle (0.9375, 0.1875);% [-0.129493, -0.125514]
\PrecisionAchieved{0.875,0.125}{0.9375,0.1875}{0.90625,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.125) rectangle (0.875, 0.25);% [-0.177979, -0.129661]
\PrecisionAchieved{0.75,0.125}{0.875,0.25}{0.8125,0.1875}{0.025}
\draw[] (0.96875, 0.09375) rectangle (1, 0.125);% [-0.0236772, 0]
\PrecisionAchieved{0.96875,0.09375}{1,0.125}{0.984375,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.09375) rectangle (0.96875, 0.125);% [-0.0369255, -0.0365921]
\PrecisionAchieved{0.9375,0.09375}{0.96875,0.125}{0.953125,0.109375}{0.00625}
\draw[] (0.96875, 0.0625) rectangle (1, 0.09375);% [-0.015697, 0]
\PrecisionAchieved{0.96875,0.0625}{1,0.09375}{0.984375,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.9375, 0.0625) rectangle (0.96875, 0.09375);% [-0.0230462, -0.0227563]
\PrecisionAchieved{0.9375,0.0625}{0.96875,0.09375}{0.953125,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.0625) rectangle (0.9375, 0.125);% [-0.0784735, -0.0736601]
\PrecisionAchieved{0.875,0.0625}{0.9375,0.125}{0.90625,0.09375}{0.0125}
\draw[] (0.9375, 0) rectangle (1, 0.0625);% [-0.0250627, 0]
\PrecisionAchieved{0.9375,0}{1,0.0625}{0.96875,0.03125}{0.0125}
\draw[fill=\HigherOrderColor] (0.90625, 0.03125) rectangle (0.9375, 0.0625);% [-0.0230462, -0.0227563]
\PrecisionAchieved{0.90625,0.03125}{0.9375,0.0625}{0.921875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.875, 0.03125) rectangle (0.90625, 0.0625);% [-0.0369255, -0.0365921]
\PrecisionAchieved{0.875,0.03125}{0.90625,0.0625}{0.890625,0.046875}{0.00625}
\draw[] (0.90625, 0) rectangle (0.9375, 0.03125);% [-0.015697, 0]
\PrecisionAchieved{0.90625,0}{0.9375,0.03125}{0.921875,0.015625}{0.00625}
\draw[] (0.875, 0) rectangle (0.90625, 0.03125);% [-0.0236772, 0]
\PrecisionAchieved{0.875,0}{0.90625,0.03125}{0.890625,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.0625) rectangle (0.875, 0.125);% [-0.129493, -0.125514]
\PrecisionAchieved{0.8125,0.0625}{0.875,0.125}{0.84375,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.75, 0.0625) rectangle (0.8125, 0.125);% [-0.157884, -0.154558]
\PrecisionAchieved{0.75,0.0625}{0.8125,0.125}{0.78125,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.84375, 0.03125) rectangle (0.875, 0.0625);% [-0.0506974, -0.0503137]
\PrecisionAchieved{0.84375,0.03125}{0.875,0.0625}{0.859375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.8125, 0.03125) rectangle (0.84375, 0.0625);% [-0.0632948, -0.0628678]
\PrecisionAchieved{0.8125,0.03125}{0.84375,0.0625}{0.828125,0.046875}{0.00625}
\draw[] (0.84375, 0) rectangle (0.875, 0.03125);% [-0.0315693, 0]
\PrecisionAchieved{0.84375,0}{0.875,0.03125}{0.859375,0.015625}{0.00625}
\draw[] (0.8125, 0) rectangle (0.84375, 0.03125);% [-0.0388125, 0]
\PrecisionAchieved{0.8125,0}{0.84375,0.03125}{0.828125,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.78125, 0.03125) rectangle (0.8125, 0.0625);% [-0.0740435, -0.0735891]
\PrecisionAchieved{0.78125,0.03125}{0.8125,0.0625}{0.796875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.75, 0.03125) rectangle (0.78125, 0.0625);% [-0.0825715, -0.0821088]
\PrecisionAchieved{0.75,0.03125}{0.78125,0.0625}{0.765625,0.046875}{0.00625}
\draw[] (0.78125, 0) rectangle (0.8125, 0.03125);% [-0.0449984, 0]
\PrecisionAchieved{0.78125,0}{0.8125,0.03125}{0.796875,0.015625}{0.00625}
\draw[] (0.75, 0) rectangle (0.78125, 0.03125);% [-0.0498517, 0]
\PrecisionAchieved{0.75,0}{0.78125,0.03125}{0.765625,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.125) rectangle (0.75, 0.25);% [-0.105502, -0.0615991]
\PrecisionAchieved{0.625,0.125}{0.75,0.25}{0.6875,0.1875}{0.025}
\draw[fill=\HigherOrderColor] (0.5, 0.125) rectangle (0.625, 0.25);% [-0.162335, -0.121901]
\PrecisionAchieved{0.5,0.125}{0.625,0.25}{0.5625,0.1875}{0.025}
\draw[fill=\HigherOrderColor] (0.6875, 0.0625) rectangle (0.75, 0.125);% [-0.168545, -0.165707]
\PrecisionAchieved{0.6875,0.0625}{0.75,0.125}{0.71875,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.625, 0.0625) rectangle (0.6875, 0.125);% [-0.170389, -0.167579]
\PrecisionAchieved{0.625,0.0625}{0.6875,0.125}{0.65625,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.71875, 0.03125) rectangle (0.75, 0.0625);% [-0.0887299, -0.0882644]
\PrecisionAchieved{0.71875,0.03125}{0.75,0.0625}{0.734375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.6875, 0.03125) rectangle (0.71875, 0.0625);% [-0.0925069, -0.0920331]
\PrecisionAchieved{0.6875,0.03125}{0.71875,0.0625}{0.703125,0.046875}{0.00625}
\draw[] (0.71875, 0) rectangle (0.75, 0.03125);% [-0.0537898, 0]
\draw[] (0.6875, 0) rectangle (0.71875, 0.03125);% [-0.0567321, 0]
\draw[fill=\HigherOrderColor] (0.65625, 0.03125) rectangle (0.6875, 0.0625);% [-0.093953, -0.093489]
\PrecisionAchieved{0.65625,0.03125}{0.6875,0.0625}{0.671875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.625, 0.03125) rectangle (0.65625, 0.0625);% [-0.0931972, -0.0927126]
\PrecisionAchieved{0.625,0.03125}{0.65625,0.0625}{0.640625,0.046875}{0.00625}
\draw[] (0.65625, 0) rectangle (0.6875, 0.03125);% [-0.058056, 0]
\draw[] (0.625, 0) rectangle (0.65625, 0.03125);% [-0.057785, 0]
\draw[fill=\HigherOrderColor] (0.5625, 0.0625) rectangle (0.625, 0.125);% [-0.166337, -0.163336]
\PrecisionAchieved{0.5625,0.0625}{0.625,0.125}{0.59375,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.5, 0.0625) rectangle (0.5625, 0.125);% [-0.153054, -0.150215]
\PrecisionAchieved{0.5,0.0625}{0.5625,0.125}{0.53125,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.59375, 0.03125) rectangle (0.625, 0.0625);% [-0.0903529, -0.0898592]
\PrecisionAchieved{0.59375,0.03125}{0.625,0.0625}{0.609375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.5625, 0.03125) rectangle (0.59375, 0.0625);% [-0.0855846, -0.0851018]
\PrecisionAchieved{0.5625,0.03125}{0.59375,0.0625}{0.578125,0.046875}{0.00625}
\draw[] (0.59375, 0) rectangle (0.625, 0.03125);% [-0.056005, 0]
\draw[] (0.5625, 0) rectangle (0.59375, 0.03125);% [-0.0528588, 0]
\draw[fill=\HigherOrderColor] (0.53125, 0.03125) rectangle (0.5625, 0.0625);% [-0.079113, -0.0786605]
\PrecisionAchieved{0.53125,0.03125}{0.5625,0.0625}{0.546875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.5, 0.03125) rectangle (0.53125, 0.0625);% [-0.0712278, -0.0708219]
\PrecisionAchieved{0.5,0.03125}{0.53125,0.0625}{0.515625,0.046875}{0.00625}
\draw[] (0.53125, 0) rectangle (0.5625, 0.03125);% [-0.0485429, 0]
\PrecisionAchieved{0.53125,0}{0.5625,0.03125}{0.546875,0.015625}{0.00625}
\draw[] (0.5, 0) rectangle (0.53125, 0.03125);% [-0.0433027, 0]
\PrecisionAchieved{0.5,0}{0.53125,0.03125}{0.515625,0.015625}{0.00625}
\draw[] (0.46875, 0.46875) rectangle (0.5, 0.5);% [-0.0376961, 0]
\PrecisionAchieved{0.46875,0.46875}{0.5,0.5}{0.484375,0.484375}{0.00625}
\draw[] (0.4375, 0.46875) rectangle (0.46875, 0.5);% [-0.0957117, 0]
\draw[] (0.46875, 0.4375) rectangle (0.5, 0.46875);% [-0.0957117, 0]
\draw[] (0.4375, 0.4375) rectangle (0.46875, 0.46875);% [-0.0360884, 0]
\PrecisionAchieved{0.4375,0.4375}{0.46875,0.46875}{0.453125,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.40625, 0.46875) rectangle (0.4375, 0.5);% [-0.0934099, -0.0923178]
\PrecisionAchieved{0.40625,0.46875}{0.4375,0.5}{0.421875,0.484375}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.46875) rectangle (0.40625, 0.5);% [-0.139353, -0.138895]
\PrecisionAchieved{0.375,0.46875}{0.40625,0.5}{0.390625,0.484375}{0.00625}
\draw[] (0.40625, 0.4375) rectangle (0.4375, 0.46875);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.375, 0.4375) rectangle (0.40625, 0.46875);% [-0.0869012, -0.0858123]
\PrecisionAchieved{0.375,0.4375}{0.40625,0.46875}{0.390625,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.46875, 0.40625) rectangle (0.5, 0.4375);% [-0.0934099, -0.0923178]
\PrecisionAchieved{0.46875,0.40625}{0.5,0.4375}{0.484375,0.421875}{0.00625}
\draw[] (0.4375, 0.40625) rectangle (0.46875, 0.4375);% [-0.0905978, 0]
\draw[fill=\HigherOrderColor] (0.46875, 0.375) rectangle (0.5, 0.40625);% [-0.139353, -0.138895]
\PrecisionAchieved{0.46875,0.375}{0.5,0.40625}{0.484375,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.375) rectangle (0.46875, 0.40625);% [-0.0869012, -0.0858123]
\PrecisionAchieved{0.4375,0.375}{0.46875,0.40625}{0.453125,0.390625}{0.00625}
\draw[] (0.40625, 0.40625) rectangle (0.4375, 0.4375);% [-0.0330265, 0]
\PrecisionAchieved{0.40625,0.40625}{0.4375,0.4375}{0.421875,0.421875}{0.00625}
\draw[] (0.375, 0.40625) rectangle (0.40625, 0.4375);% [-0.0823766, 0]
\draw[] (0.40625, 0.375) rectangle (0.4375, 0.40625);% [-0.0823766, 0]
\draw[] (0.375, 0.375) rectangle (0.40625, 0.40625);% [-0.0288048, 0]
\PrecisionAchieved{0.375,0.375}{0.40625,0.40625}{0.390625,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.4375) rectangle (0.375, 0.5);% [-0.160944, -0.156768]
\PrecisionAchieved{0.3125,0.4375}{0.375,0.5}{0.34375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.25, 0.4375) rectangle (0.3125, 0.5);% [-0.179991, -0.177648]
\PrecisionAchieved{0.25,0.4375}{0.3125,0.5}{0.28125,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.34375, 0.40625) rectangle (0.375, 0.4375);% [-0.0775213, -0.0764971]
\PrecisionAchieved{0.34375,0.40625}{0.375,0.4375}{0.359375,0.421875}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.40625) rectangle (0.34375, 0.4375);% [-0.115611, -0.11519]
\PrecisionAchieved{0.3125,0.40625}{0.34375,0.4375}{0.328125,0.421875}{0.00625}
\draw[] (0.34375, 0.375) rectangle (0.375, 0.40625);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.3125, 0.375) rectangle (0.34375, 0.40625);% [-0.0658831, -0.0649798]
\PrecisionAchieved{0.3125,0.375}{0.34375,0.40625}{0.328125,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.375) rectangle (0.3125, 0.4375);% [-0.13095, -0.127149]
\PrecisionAchieved{0.25,0.375}{0.3125,0.4375}{0.28125,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.3125) rectangle (0.5, 0.375);% [-0.160944, -0.156768]
\PrecisionAchieved{0.4375,0.3125}{0.5,0.375}{0.46875,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.40625, 0.34375) rectangle (0.4375, 0.375);% [-0.0775213, -0.0764971]
\PrecisionAchieved{0.40625,0.34375}{0.4375,0.375}{0.421875,0.359375}{0.00625}
\draw[] (0.375, 0.34375) rectangle (0.40625, 0.375);% [-0.071571, 0]
\draw[fill=\HigherOrderColor] (0.40625, 0.3125) rectangle (0.4375, 0.34375);% [-0.115611, -0.11519]
\PrecisionAchieved{0.40625,0.3125}{0.4375,0.34375}{0.421875,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.3125) rectangle (0.40625, 0.34375);% [-0.0658831, -0.0649798]
\PrecisionAchieved{0.375,0.3125}{0.40625,0.34375}{0.390625,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.25) rectangle (0.5, 0.3125);% [-0.179991, -0.177648]
\PrecisionAchieved{0.4375,0.25}{0.5,0.3125}{0.46875,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.25) rectangle (0.4375, 0.3125);% [-0.13095, -0.127149]
\PrecisionAchieved{0.375,0.25}{0.4375,0.3125}{0.40625,0.28125}{0.0125}
\draw[] (0.34375, 0.34375) rectangle (0.375, 0.375);% [-0.0238312, 0]
\PrecisionAchieved{0.34375,0.34375}{0.375,0.375}{0.359375,0.359375}{0.00625}
\draw[] (0.3125, 0.34375) rectangle (0.34375, 0.375);% [-0.058991, 0]
\draw[] (0.34375, 0.3125) rectangle (0.375, 0.34375);% [-0.058991, 0]
\draw[] (0.3125, 0.3125) rectangle (0.34375, 0.34375);% [-0.0185805, 0]
\PrecisionAchieved{0.3125,0.3125}{0.34375,0.34375}{0.328125,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.34375) rectangle (0.3125, 0.375);% [-0.052898, -0.0521554]
\PrecisionAchieved{0.28125,0.34375}{0.3125,0.375}{0.296875,0.359375}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.34375) rectangle (0.28125, 0.375);% [-0.0781648, -0.0778609]
\PrecisionAchieved{0.25,0.34375}{0.28125,0.375}{0.265625,0.359375}{0.00625}
\draw[] (0.28125, 0.3125) rectangle (0.3125, 0.34375);% [-0.0457006, 0]
\PrecisionAchieved{0.28125,0.3125}{0.3125,0.34375}{0.296875,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.3125) rectangle (0.28125, 0.34375);% [-0.0397028, -0.0391373]
\PrecisionAchieved{0.25,0.3125}{0.28125,0.34375}{0.265625,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.28125) rectangle (0.375, 0.3125);% [-0.052898, -0.0521554]
\PrecisionAchieved{0.34375,0.28125}{0.375,0.3125}{0.359375,0.296875}{0.00625}
\draw[] (0.3125, 0.28125) rectangle (0.34375, 0.3125);% [-0.0457006, 0]
\PrecisionAchieved{0.3125,0.28125}{0.34375,0.3125}{0.328125,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.25) rectangle (0.375, 0.28125);% [-0.0781648, -0.0778609]
\PrecisionAchieved{0.34375,0.25}{0.375,0.28125}{0.359375,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.25) rectangle (0.34375, 0.28125);% [-0.0397028, -0.0391373]
\PrecisionAchieved{0.3125,0.25}{0.34375,0.28125}{0.328125,0.265625}{0.00625}
\draw[] (0.25, 0.25) rectangle (0.3125, 0.3125);% [-0.0328859, 0]
\PrecisionAchieved{0.25,0.25}{0.3125,0.3125}{0.28125,0.28125}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.4375) rectangle (0.25, 0.5);% [-0.181892, -0.17996]
\PrecisionAchieved{0.1875,0.4375}{0.25,0.5}{0.21875,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.4375) rectangle (0.1875, 0.5);% [-0.174754, -0.172535]
\PrecisionAchieved{0.125,0.4375}{0.1875,0.5}{0.15625,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.1875, 0.375) rectangle (0.25, 0.4375);% [-0.149499, -0.147395]
\PrecisionAchieved{0.1875,0.375}{0.25,0.4375}{0.21875,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.375) rectangle (0.1875, 0.4375);% [-0.137758, -0.135382]
\PrecisionAchieved{0.125,0.375}{0.1875,0.4375}{0.15625,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.0625, 0.4375) rectangle (0.125, 0.5);% [-0.127849, -0.124431]
\PrecisionAchieved{0.0625,0.4375}{0.125,0.5}{0.09375,0.46875}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.46875) rectangle (0.0625, 0.5);% [-0.0623243, -0.0619205]
\PrecisionAchieved{0.03125,0.46875}{0.0625,0.5}{0.046875,0.484375}{0.00625}
\draw[] (0, 0.46875) rectangle (0.03125, 0.5);% [-0.0376961, 0]
\PrecisionAchieved{0,0.46875}{0.03125,0.5}{0.015625,0.484375}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.4375) rectangle (0.0625, 0.46875);% [-0.0528228, -0.0524048]
\PrecisionAchieved{0.03125,0.4375}{0.0625,0.46875}{0.046875,0.453125}{0.00625}
\draw[] (0, 0.4375) rectangle (0.03125, 0.46875);% [-0.0374249, 0]
\PrecisionAchieved{0,0.4375}{0.03125,0.46875}{0.015625,0.453125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.375) rectangle (0.125, 0.4375);% [-0.0935202, -0.0877598]
\PrecisionAchieved{0.0625,0.375}{0.125,0.4375}{0.09375,0.40625}{0.0125}
\draw[fill=\HigherOrderColor] (0.03125, 0.40625) rectangle (0.0625, 0.4375);% [-0.0432031, -0.042753]
\PrecisionAchieved{0.03125,0.40625}{0.0625,0.4375}{0.046875,0.421875}{0.00625}
\draw[] (0, 0.40625) rectangle (0.03125, 0.4375);% [-0.0366166, 0]
\PrecisionAchieved{0,0.40625}{0.03125,0.4375}{0.015625,0.421875}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.375) rectangle (0.0625, 0.40625);% [-0.0339776, -0.0334197]
\PrecisionAchieved{0.03125,0.375}{0.0625,0.40625}{0.046875,0.390625}{0.00625}
\draw[] (0, 0.375) rectangle (0.03125, 0.40625);% [-0.0352867, 0]
\PrecisionAchieved{0,0.375}{0.03125,0.40625}{0.015625,0.390625}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.3125) rectangle (0.25, 0.375);% [-0.0827364, -0.078422]
\PrecisionAchieved{0.1875,0.3125}{0.25,0.375}{0.21875,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.125, 0.3125) rectangle (0.1875, 0.375);% [-0.083917, -0.0797423]
\PrecisionAchieved{0.125,0.3125}{0.1875,0.375}{0.15625,0.34375}{0.0125}
\draw[fill=\HigherOrderColor] (0.21875, 0.28125) rectangle (0.25, 0.3125);% [-0.0275286, -0.0270409]
\PrecisionAchieved{0.21875,0.28125}{0.25,0.3125}{0.234375,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.28125) rectangle (0.21875, 0.3125);% [-0.0388906, -0.0386336]
\PrecisionAchieved{0.1875,0.28125}{0.21875,0.3125}{0.203125,0.296875}{0.00625}
\draw[] (0.21875, 0.25) rectangle (0.25, 0.28125);% [-0.0254528, 0]
\PrecisionAchieved{0.21875,0.25}{0.25,0.28125}{0.234375,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.1875, 0.25) rectangle (0.21875, 0.28125);% [-0.0174752, -0.0167406]
\PrecisionAchieved{0.1875,0.25}{0.21875,0.28125}{0.203125,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.15625, 0.28125) rectangle (0.1875, 0.3125);% [-0.0440094, -0.0438448]
\PrecisionAchieved{0.15625,0.28125}{0.1875,0.3125}{0.171875,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.28125) rectangle (0.15625, 0.3125);% [-0.0426038, -0.0424524]
\PrecisionAchieved{0.125,0.28125}{0.15625,0.3125}{0.140625,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.15625, 0.25) rectangle (0.1875, 0.28125);% [-0.0233757, -0.0230647]
\PrecisionAchieved{0.15625,0.25}{0.1875,0.28125}{0.171875,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.125, 0.25) rectangle (0.15625, 0.28125);% [-0.0246791, -0.0244497]
\PrecisionAchieved{0.125,0.25}{0.15625,0.28125}{0.140625,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.34375) rectangle (0.125, 0.375);% [-0.0737784, -0.0736248]
\PrecisionAchieved{0.09375,0.34375}{0.125,0.375}{0.109375,0.359375}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.34375) rectangle (0.09375, 0.375);% [-0.0506441, -0.0504214]
\PrecisionAchieved{0.0625,0.34375}{0.09375,0.375}{0.078125,0.359375}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.3125) rectangle (0.125, 0.34375);% [-0.0532269, -0.053073]
\PrecisionAchieved{0.09375,0.3125}{0.125,0.34375}{0.109375,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.3125) rectangle (0.09375, 0.34375);% [-0.0363955, -0.0361427]
\PrecisionAchieved{0.0625,0.3125}{0.09375,0.34375}{0.078125,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.03125, 0.34375) rectangle (0.0625, 0.375);% [-0.0259361, -0.0244928]
\PrecisionAchieved{0.03125,0.34375}{0.0625,0.375}{0.046875,0.359375}{0.00625}
\draw[] (0, 0.34375) rectangle (0.03125, 0.375);% [-0.0334617, 0]
\PrecisionAchieved{0,0.34375}{0.03125,0.375}{0.015625,0.359375}{0.00625}
\draw[] (0.03125, 0.3125) rectangle (0.0625, 0.34375);% [-0.056005, 0]
\draw[] (0, 0.3125) rectangle (0.03125, 0.34375);% [-0.0311793, 0]
\PrecisionAchieved{0,0.3125}{0.03125,0.34375}{0.015625,0.328125}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.28125) rectangle (0.125, 0.3125);% [-0.0355016, -0.0353161]
\PrecisionAchieved{0.09375,0.28125}{0.125,0.3125}{0.109375,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.0625, 0.28125) rectangle (0.09375, 0.3125);% [-0.0245751, -0.0239929]
\PrecisionAchieved{0.0625,0.28125}{0.09375,0.3125}{0.078125,0.296875}{0.00625}
\draw[fill=\HigherOrderColor] (0.09375, 0.25) rectangle (0.125, 0.28125);% [-0.0215929, -0.0211726]
\PrecisionAchieved{0.09375,0.25}{0.125,0.28125}{0.109375,0.265625}{0.00625}
\draw[] (0.0625, 0.25) rectangle (0.09375, 0.28125);% [-0.050508, 0]
\draw[] (0.03125, 0.28125) rectangle (0.0625, 0.3125);% [-0.0473243, 0]
\PrecisionAchieved{0.03125,0.28125}{0.0625,0.3125}{0.046875,0.296875}{0.00625}
\draw[] (0, 0.28125) rectangle (0.03125, 0.3125);% [-0.028489, 0]
\PrecisionAchieved{0,0.28125}{0.03125,0.3125}{0.015625,0.296875}{0.00625}
\draw[] (0.03125, 0.25) rectangle (0.0625, 0.28125);% [-0.0390284, 0]
\PrecisionAchieved{0.03125,0.25}{0.0625,0.28125}{0.046875,0.265625}{0.00625}
\draw[] (0, 0.25) rectangle (0.03125, 0.28125);% [-0.0254528, 0]
\PrecisionAchieved{0,0.25}{0.03125,0.28125}{0.015625,0.265625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.1875) rectangle (0.5, 0.25);% [-0.181892, -0.17996]
\PrecisionAchieved{0.4375,0.1875}{0.5,0.25}{0.46875,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.1875) rectangle (0.4375, 0.25);% [-0.149499, -0.147395]
\PrecisionAchieved{0.375,0.1875}{0.4375,0.25}{0.40625,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.4375, 0.125) rectangle (0.5, 0.1875);% [-0.174754, -0.172535]
\PrecisionAchieved{0.4375,0.125}{0.5,0.1875}{0.46875,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.125) rectangle (0.4375, 0.1875);% [-0.137758, -0.135382]
\PrecisionAchieved{0.375,0.125}{0.4375,0.1875}{0.40625,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.3125, 0.1875) rectangle (0.375, 0.25);% [-0.0827364, -0.078422]
\PrecisionAchieved{0.3125,0.1875}{0.375,0.25}{0.34375,0.21875}{0.0125}
\draw[fill=\HigherOrderColor] (0.28125, 0.21875) rectangle (0.3125, 0.25);% [-0.0275286, -0.0270409]
\PrecisionAchieved{0.28125,0.21875}{0.3125,0.25}{0.296875,0.234375}{0.00625}
\draw[] (0.25, 0.21875) rectangle (0.28125, 0.25);% [-0.0254528, 0]
\PrecisionAchieved{0.25,0.21875}{0.28125,0.25}{0.265625,0.234375}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.1875) rectangle (0.3125, 0.21875);% [-0.0388906, -0.0386336]
\PrecisionAchieved{0.28125,0.1875}{0.3125,0.21875}{0.296875,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.1875) rectangle (0.28125, 0.21875);% [-0.0174752, -0.0167406]
\PrecisionAchieved{0.25,0.1875}{0.28125,0.21875}{0.265625,0.203125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.125) rectangle (0.375, 0.1875);% [-0.083917, -0.0797423]
\PrecisionAchieved{0.3125,0.125}{0.375,0.1875}{0.34375,0.15625}{0.0125}
\draw[fill=\HigherOrderColor] (0.28125, 0.15625) rectangle (0.3125, 0.1875);% [-0.0440094, -0.0438448]
\PrecisionAchieved{0.28125,0.15625}{0.3125,0.1875}{0.296875,0.171875}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.15625) rectangle (0.28125, 0.1875);% [-0.0233757, -0.0230647]
\PrecisionAchieved{0.25,0.15625}{0.28125,0.1875}{0.265625,0.171875}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.125) rectangle (0.3125, 0.15625);% [-0.0426038, -0.0424524]
\PrecisionAchieved{0.28125,0.125}{0.3125,0.15625}{0.296875,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.125) rectangle (0.28125, 0.15625);% [-0.0246791, -0.0244497]
\PrecisionAchieved{0.25,0.125}{0.28125,0.15625}{0.265625,0.140625}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.0625) rectangle (0.5, 0.125);% [-0.127849, -0.124431]
\PrecisionAchieved{0.4375,0.0625}{0.5,0.125}{0.46875,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.375, 0.0625) rectangle (0.4375, 0.125);% [-0.0935202, -0.0877598]
\PrecisionAchieved{0.375,0.0625}{0.4375,0.125}{0.40625,0.09375}{0.0125}
\draw[fill=\HigherOrderColor] (0.46875, 0.03125) rectangle (0.5, 0.0625);% [-0.0623243, -0.0619205]
\PrecisionAchieved{0.46875,0.03125}{0.5,0.0625}{0.484375,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.4375, 0.03125) rectangle (0.46875, 0.0625);% [-0.0528228, -0.0524048]
\PrecisionAchieved{0.4375,0.03125}{0.46875,0.0625}{0.453125,0.046875}{0.00625}
\draw[] (0.46875, 0) rectangle (0.5, 0.03125);% [-0.0376961, 0]
\PrecisionAchieved{0.46875,0}{0.5,0.03125}{0.484375,0.015625}{0.00625}
\draw[] (0.4375, 0) rectangle (0.46875, 0.03125);% [-0.0374249, 0]
\PrecisionAchieved{0.4375,0}{0.46875,0.03125}{0.453125,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.40625, 0.03125) rectangle (0.4375, 0.0625);% [-0.0432031, -0.042753]
\PrecisionAchieved{0.40625,0.03125}{0.4375,0.0625}{0.421875,0.046875}{0.00625}
\draw[fill=\HigherOrderColor] (0.375, 0.03125) rectangle (0.40625, 0.0625);% [-0.0339776, -0.0334197]
\PrecisionAchieved{0.375,0.03125}{0.40625,0.0625}{0.390625,0.046875}{0.00625}
\draw[] (0.40625, 0) rectangle (0.4375, 0.03125);% [-0.0366166, 0]
\PrecisionAchieved{0.40625,0}{0.4375,0.03125}{0.421875,0.015625}{0.00625}
\draw[] (0.375, 0) rectangle (0.40625, 0.03125);% [-0.0352867, 0]
\PrecisionAchieved{0.375,0}{0.40625,0.03125}{0.390625,0.015625}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.09375) rectangle (0.375, 0.125);% [-0.0737784, -0.0736248]
\PrecisionAchieved{0.34375,0.09375}{0.375,0.125}{0.359375,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.09375) rectangle (0.34375, 0.125);% [-0.0532269, -0.053073]
\PrecisionAchieved{0.3125,0.09375}{0.34375,0.125}{0.328125,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.34375, 0.0625) rectangle (0.375, 0.09375);% [-0.0506441, -0.0504214]
\PrecisionAchieved{0.34375,0.0625}{0.375,0.09375}{0.359375,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.3125, 0.0625) rectangle (0.34375, 0.09375);% [-0.0363955, -0.0361427]
\PrecisionAchieved{0.3125,0.0625}{0.34375,0.09375}{0.328125,0.078125}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.09375) rectangle (0.3125, 0.125);% [-0.0355016, -0.0353161]
\PrecisionAchieved{0.28125,0.09375}{0.3125,0.125}{0.296875,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.25, 0.09375) rectangle (0.28125, 0.125);% [-0.0215929, -0.0211726]
\PrecisionAchieved{0.25,0.09375}{0.28125,0.125}{0.265625,0.109375}{0.00625}
\draw[fill=\HigherOrderColor] (0.28125, 0.0625) rectangle (0.3125, 0.09375);% [-0.0245751, -0.0239929]
\PrecisionAchieved{0.28125,0.0625}{0.3125,0.09375}{0.296875,0.078125}{0.00625}
\draw[] (0.25, 0.0625) rectangle (0.28125, 0.09375);% [-0.050508, 0]
\draw[fill=\HigherOrderColor] (0.34375, 0.03125) rectangle (0.375, 0.0625);% [-0.0259361, -0.0244928]
\PrecisionAchieved{0.34375,0.03125}{0.375,0.0625}{0.359375,0.046875}{0.00625}
\draw[] (0.3125, 0.03125) rectangle (0.34375, 0.0625);% [-0.056005, 0]
\draw[] (0.34375, 0) rectangle (0.375, 0.03125);% [-0.0334617, 0]
\PrecisionAchieved{0.34375,0}{0.375,0.03125}{0.359375,0.015625}{0.00625}
\draw[] (0.3125, 0) rectangle (0.34375, 0.03125);% [-0.0311793, 0]
\PrecisionAchieved{0.3125,0}{0.34375,0.03125}{0.328125,0.015625}{0.00625}
\draw[] (0.28125, 0.03125) rectangle (0.3125, 0.0625);% [-0.0473243, 0]
\PrecisionAchieved{0.28125,0.03125}{0.3125,0.0625}{0.296875,0.046875}{0.00625}
\draw[] (0.25, 0.03125) rectangle (0.28125, 0.0625);% [-0.0390284, 0]
\PrecisionAchieved{0.25,0.03125}{0.28125,0.0625}{0.265625,0.046875}{0.00625}
\draw[] (0.28125, 0) rectangle (0.3125, 0.03125);% [-0.028489, 0]
\PrecisionAchieved{0.28125,0}{0.3125,0.03125}{0.296875,0.015625}{0.00625}
\draw[] (0.25, 0) rectangle (0.28125, 0.03125);% [-0.0254528, 0]
\PrecisionAchieved{0.25,0}{0.28125,0.03125}{0.265625,0.015625}{0.00625}
\draw[] (0.1875, 0.1875) rectangle (0.25, 0.25);% [-0.0373315, 0]
\PrecisionAchieved{0.1875,0.1875}{0.25,0.25}{0.21875,0.21875}{0.0125}
\draw[] (0.15625, 0.21875) rectangle (0.1875, 0.25);% [-0.036502, 0]
\PrecisionAchieved{0.15625,0.21875}{0.1875,0.25}{0.171875,0.234375}{0.00625}
\draw[] (0.125, 0.21875) rectangle (0.15625, 0.25);% [-0.0428262, 0]
\PrecisionAchieved{0.125,0.21875}{0.15625,0.25}{0.140625,0.234375}{0.00625}
\draw[] (0.15625, 0.1875) rectangle (0.1875, 0.21875);% [-0.0253958, 0]
\PrecisionAchieved{0.15625,0.1875}{0.1875,0.21875}{0.171875,0.203125}{0.00625}
\draw[] (0.125, 0.1875) rectangle (0.15625, 0.21875);% [-0.0316975, 0]
\PrecisionAchieved{0.125,0.1875}{0.15625,0.21875}{0.140625,0.203125}{0.00625}
\draw[] (0.21875, 0.15625) rectangle (0.25, 0.1875);% [-0.036502, 0]
\PrecisionAchieved{0.21875,0.15625}{0.25,0.1875}{0.234375,0.171875}{0.00625}
\draw[] (0.1875, 0.15625) rectangle (0.21875, 0.1875);% [-0.0253958, 0]
\PrecisionAchieved{0.1875,0.15625}{0.21875,0.1875}{0.203125,0.171875}{0.00625}
\draw[] (0.21875, 0.125) rectangle (0.25, 0.15625);% [-0.0428262, 0]
\PrecisionAchieved{0.21875,0.125}{0.25,0.15625}{0.234375,0.140625}{0.00625}
\draw[] (0.1875, 0.125) rectangle (0.21875, 0.15625);% [-0.0316975, 0]
\PrecisionAchieved{0.1875,0.125}{0.21875,0.15625}{0.203125,0.140625}{0.00625}
\draw[] (0.15625, 0.15625) rectangle (0.1875, 0.1875);% [-0.0180755, 0]
\PrecisionAchieved{0.15625,0.15625}{0.1875,0.1875}{0.171875,0.171875}{0.00625}
\draw[] (0.125, 0.15625) rectangle (0.15625, 0.1875);% [-0.0236217, 0]
\PrecisionAchieved{0.125,0.15625}{0.15625,0.1875}{0.140625,0.171875}{0.00625}
\draw[] (0.15625, 0.125) rectangle (0.1875, 0.15625);% [-0.0236217, 0]
\PrecisionAchieved{0.15625,0.125}{0.1875,0.15625}{0.171875,0.140625}{0.00625}
\draw[] (0.125, 0.125) rectangle (0.15625, 0.15625);% [-0.0180817, 0]
\PrecisionAchieved{0.125,0.125}{0.15625,0.15625}{0.140625,0.140625}{0.00625}
\draw[] (0.09375, 0.21875) rectangle (0.125, 0.25);% [-0.043624, 0]
\PrecisionAchieved{0.09375,0.21875}{0.125,0.25}{0.109375,0.234375}{0.00625}
\draw[] (0.0625, 0.21875) rectangle (0.09375, 0.25);% [-0.0395592, 0]
\PrecisionAchieved{0.0625,0.21875}{0.09375,0.25}{0.078125,0.234375}{0.00625}
\draw[] (0.09375, 0.1875) rectangle (0.125, 0.21875);% [-0.0335055, 0]
\PrecisionAchieved{0.09375,0.1875}{0.125,0.21875}{0.109375,0.203125}{0.00625}
\draw[] (0.0625, 0.1875) rectangle (0.09375, 0.21875);% [-0.0312224, 0]
\PrecisionAchieved{0.0625,0.1875}{0.09375,0.21875}{0.078125,0.203125}{0.00625}
\draw[] (0.03125, 0.21875) rectangle (0.0625, 0.25);% [-0.0318472, 0]
\PrecisionAchieved{0.03125,0.21875}{0.0625,0.25}{0.046875,0.234375}{0.00625}
\draw[] (0, 0.21875) rectangle (0.03125, 0.25);% [-0.0221457, 0]
\PrecisionAchieved{0,0.21875}{0.03125,0.25}{0.015625,0.234375}{0.00625}
\draw[] (0.03125, 0.1875) rectangle (0.0625, 0.21875);% [-0.0258229, 0]
\PrecisionAchieved{0.03125,0.1875}{0.0625,0.21875}{0.046875,0.203125}{0.00625}
\draw[] (0, 0.1875) rectangle (0.03125, 0.21875);% [-0.0186564, 0]
\PrecisionAchieved{0,0.1875}{0.03125,0.21875}{0.015625,0.203125}{0.00625}
\draw[] (0.09375, 0.15625) rectangle (0.125, 0.1875);% [-0.0256307, 0]
\PrecisionAchieved{0.09375,0.15625}{0.125,0.1875}{0.109375,0.171875}{0.00625}
\draw[] (0.0625, 0.15625) rectangle (0.09375, 0.1875);% [-0.0243169, 0]
\PrecisionAchieved{0.0625,0.15625}{0.09375,0.1875}{0.078125,0.171875}{0.00625}
\draw[] (0.09375, 0.125) rectangle (0.125, 0.15625);% [-0.0196956, 0]
\PrecisionAchieved{0.09375,0.125}{0.125,0.15625}{0.109375,0.140625}{0.00625}
\draw[] (0.0625, 0.125) rectangle (0.09375, 0.15625);% [-0.0186996, 0]
\PrecisionAchieved{0.0625,0.125}{0.09375,0.15625}{0.078125,0.140625}{0.00625}
\draw[] (0, 0.125) rectangle (0.0625, 0.1875);% [-0.0428262, 0]
\PrecisionAchieved{0,0.125}{0.0625,0.1875}{0.03125,0.15625}{0.0125}
\draw[] (0.21875, 0.09375) rectangle (0.25, 0.125);% [-0.043624, 0]
\PrecisionAchieved{0.21875,0.09375}{0.25,0.125}{0.234375,0.109375}{0.00625}
\draw[] (0.1875, 0.09375) rectangle (0.21875, 0.125);% [-0.0335055, 0]
\PrecisionAchieved{0.1875,0.09375}{0.21875,0.125}{0.203125,0.109375}{0.00625}
\draw[] (0.21875, 0.0625) rectangle (0.25, 0.09375);% [-0.0395592, 0]
\PrecisionAchieved{0.21875,0.0625}{0.25,0.09375}{0.234375,0.078125}{0.00625}
\draw[] (0.1875, 0.0625) rectangle (0.21875, 0.09375);% [-0.0312224, 0]
\PrecisionAchieved{0.1875,0.0625}{0.21875,0.09375}{0.203125,0.078125}{0.00625}
\draw[] (0.15625, 0.09375) rectangle (0.1875, 0.125);% [-0.0256307, 0]
\PrecisionAchieved{0.15625,0.09375}{0.1875,0.125}{0.171875,0.109375}{0.00625}
\draw[] (0.125, 0.09375) rectangle (0.15625, 0.125);% [-0.0196956, 0]
\PrecisionAchieved{0.125,0.09375}{0.15625,0.125}{0.140625,0.109375}{0.00625}
\draw[] (0.15625, 0.0625) rectangle (0.1875, 0.09375);% [-0.0243169, 0]
\PrecisionAchieved{0.15625,0.0625}{0.1875,0.09375}{0.171875,0.078125}{0.00625}
\draw[] (0.125, 0.0625) rectangle (0.15625, 0.09375);% [-0.0186996, 0]
\PrecisionAchieved{0.125,0.0625}{0.15625,0.09375}{0.140625,0.078125}{0.00625}
\draw[] (0.21875, 0.03125) rectangle (0.25, 0.0625);% [-0.0318472, 0]
\PrecisionAchieved{0.21875,0.03125}{0.25,0.0625}{0.234375,0.046875}{0.00625}
\draw[] (0.1875, 0.03125) rectangle (0.21875, 0.0625);% [-0.0258229, 0]
\PrecisionAchieved{0.1875,0.03125}{0.21875,0.0625}{0.203125,0.046875}{0.00625}
\draw[] (0.21875, 0) rectangle (0.25, 0.03125);% [-0.0221457, 0]
\PrecisionAchieved{0.21875,0}{0.25,0.03125}{0.234375,0.015625}{0.00625}
\draw[] (0.1875, 0) rectangle (0.21875, 0.03125);% [-0.0186564, 0]
\PrecisionAchieved{0.1875,0}{0.21875,0.03125}{0.203125,0.015625}{0.00625}
\draw[] (0.125, 0) rectangle (0.1875, 0.0625);% [-0.0428262, 0]
\PrecisionAchieved{0.125,0}{0.1875,0.0625}{0.15625,0.03125}{0.0125}
\draw[] (0.0625, 0.0625) rectangle (0.125, 0.125);% [-0.0379418, 0]
\PrecisionAchieved{0.0625,0.0625}{0.125,0.125}{0.09375,0.09375}{0.0125}
\draw[] (0, 0.0625) rectangle (0.0625, 0.125);% [-0.0243169, 0]
\PrecisionAchieved{0,0.0625}{0.0625,0.125}{0.03125,0.09375}{0.0125}
\draw[] (0.0625, 0) rectangle (0.125, 0.0625);% [-0.0243169, 0]
\PrecisionAchieved{0.0625,0}{0.125,0.0625}{0.09375,0.03125}{0.0125}
\draw[] (0, 0) rectangle (0.0625, 0.0625);% [-0.00819741, 0]
\PrecisionAchieved{0,0}{0.0625,0.0625}{0.03125,0.03125}{0.0125}


==> nodal_rect_D.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.4, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{144,144,144}{0.566369652215}{0.360222344776}{0.562446316304}{0.369879653919}
  \meshline{144,144,144}{0.517662800148}{0.148018234662}{0.519877042062}{0.148047338729}
  \meshline{144,144,144}{0.874854116135}{0.101815183783}{0.869821597325}{0.096848185092}
  \meshline{144,144,144}{0.936698633128}{0.228642504814}{0.938980433190}{0.242706159624}
  \meshline{144,144,144}{0.925858046523}{0.184619709549}{0.928731816437}{0.195351349364}
  \meshline{144,144,144}{0.919628593324}{0.167787233505}{0.925858046523}{0.184619709549}
  \meshline{144,144,144}{0.931610221756}{0.205534388855}{0.930358098027}{0.200238205098}
  \meshline{144,144,144}{0.893707215184}{0.121930203194}{0.887005114723}{0.113317397089}
  \meshline{144,144,144}{0.918212208595}{0.164041740499}{0.916721874231}{0.161242048408}
  \meshline{144,144,144}{0.847770745172}{0.272529771550}{0.844526715117}{0.262525189595}
  \meshline{144,144,144}{0.897883196562}{0.126981988154}{0.893707215184}{0.121930203194}
  \meshline{144,144,144}{0.897883196562}{0.126981988154}{0.902361672363}{0.134443214821}
  \meshline{144,144,144}{0.874854116135}{0.101815183783}{0.887005114723}{0.113317397089}
  \meshline{144,144,144}{0.907975691154}{0.142841667031}{0.902361672363}{0.134443214821}
  \meshline{144,144,144}{0.907975691154}{0.142841667031}{0.916721874231}{0.161242048408}
  \meshline{144,144,144}{0.918212208595}{0.164041740499}{0.919628593324}{0.167787233505}
  \meshline{144,144,144}{0.860536333181}{0.090220277912}{0.854308239316}{0.085596630974}
  \meshline{144,144,144}{0.928731816437}{0.195351349364}{0.930358098027}{0.200238205098}
  \meshline{144,144,144}{0.934788651320}{0.220490745782}{0.936698633128}{0.228642504814}
  \meshline{144,144,144}{0.849165366774}{0.278439046319}{0.847770745172}{0.272529771550}
  \meshline{144,144,144}{0.931610221756}{0.205534388855}{0.934788651320}{0.220490745782}
  \meshline{144,144,144}{0.939779717584}{0.248160066374}{0.939246677390}{0.244074415323}
  \meshline{144,144,144}{0.850784458298}{0.083818666293}{0.854308239316}{0.085596630974}
  \meshline{144,144,144}{0.869821597325}{0.096848185092}{0.860536333181}{0.090220277912}
  \meshline{144,144,144}{0.945066208339}{0.298668078431}{0.945711324462}{0.310393300084}
  \meshline{144,144,144}{0.836901541701}{0.240049729722}{0.833028655367}{0.230283968698}
  \meshline{144,144,144}{0.850784458298}{0.083818666293}{0.837447146460}{0.075593226169}
  \meshline{144,144,144}{0.822022250984}{0.068960869390}{0.809215285699}{0.063645559022}
  \meshline{144,144,144}{0.796929742836}{0.174676536493}{0.806707889216}{0.186714605922}
  \meshline{144,144,144}{0.825111416565}{0.070186117504}{0.826377937520}{0.070730748106}
  \meshline{144,144,144}{0.837447146460}{0.075593226169}{0.826377937520}{0.070730748106}
  \meshline{144,144,144}{0.943446211635}{0.278759133649}{0.943293951798}{0.276971318574}
  \meshline{144,144,144}{0.840445701433}{0.248610609170}{0.844526715117}{0.262525189595}
  \meshline{144,144,144}{0.813243921903}{0.195977978727}{0.819734421110}{0.205693180662}
  \meshline{144,144,144}{0.939246677390}{0.244074415323}{0.938980433190}{0.242706159624}
  \meshline{144,144,144}{0.939779717584}{0.248160066374}{0.941510567564}{0.261345038894}
  \meshline{144,144,144}{0.941510567564}{0.261345038894}{0.943293951798}{0.276971318574}
  \meshline{144,144,144}{0.857495573206}{0.346236577472}{0.857033586905}{0.339484416846}
  \meshline{144,144,144}{0.849165366774}{0.278439046319}{0.852199175844}{0.292793733689}
  \meshline{144,144,144}{0.852199175844}{0.292793733689}{0.853314240212}{0.298333554795}
  \meshline{144,144,144}{0.855268994095}{0.313050677309}{0.856568224031}{0.326189514597}
  \meshline{144,144,144}{0.853314240212}{0.298333554795}{0.855053461680}{0.311158372426}
  \meshline{144,144,144}{0.855053461680}{0.311158372426}{0.855268994095}{0.313050677309}
  \meshline{144,144,144}{0.823931728457}{0.212755833106}{0.829638194170}{0.223477513398}
  \meshline{144,144,144}{0.833028655367}{0.230283968698}{0.829638194170}{0.223477513398}
  \meshline{144,144,144}{0.836901541701}{0.240049729722}{0.840445701433}{0.248610609170}
  \meshline{144,144,144}{0.823931728457}{0.212755833106}{0.819734421110}{0.205693180662}
  \meshline{144,144,144}{0.813243921903}{0.195977978727}{0.809831471221}{0.190650906930}
  \meshline{144,144,144}{0.809831471221}{0.190650906930}{0.806707889216}{0.186714605922}
  \meshline{144,144,144}{0.782938894658}{0.160811376630}{0.787672048328}{0.165103442466}
  \meshline{144,144,144}{0.753873469605}{0.137472416131}{0.763102651165}{0.144094643342}
  \meshline{144,144,144}{0.796929742836}{0.174676536493}{0.787672048328}{0.165103442466}
  \meshline{144,144,144}{0.943446211635}{0.278759133649}{0.943642935653}{0.281563566338}
  \meshline{144,144,144}{0.945066208339}{0.298668078431}{0.944626123373}{0.292606720858}
  \meshline{144,144,144}{0.946334628211}{0.328158479793}{0.946073045796}{0.317016582373}
  \meshline{144,144,144}{0.944626123373}{0.292606720858}{0.943642935653}{0.281563566338}
  \meshline{144,144,144}{0.946334628211}{0.328158479793}{0.946655476618}{0.340624593441}
  \meshline{144,144,144}{0.946073045796}{0.317016582373}{0.945711324462}{0.310393300084}
  \meshline{144,144,144}{0.857376737133}{0.352365475512}{0.857260077045}{0.362911014331}
  \meshline{144,144,144}{0.857376737133}{0.352365475512}{0.857495573206}{0.346236577472}
  \meshline{144,144,144}{0.856136973950}{0.379474998544}{0.856263654605}{0.376973099536}
  \meshline{144,144,144}{0.857260077045}{0.362911014331}{0.856263654605}{0.376973099536}
  \meshline{144,144,144}{0.856568224031}{0.326189514597}{0.857033586905}{0.339484416846}
  \meshline{144,144,144}{0.946651203537}{0.353106622138}{0.946655476618}{0.340624593441}
  \meshline{144,144,144}{0.946664282905}{0.358651539538}{0.946286790032}{0.378437957286}
  \meshline{144,144,144}{0.945764462919}{0.388464598961}{0.946140659317}{0.382513038989}
  \meshline{144,144,144}{0.946651203537}{0.353106622138}{0.946664282905}{0.358651539538}
  \meshline{144,144,144}{0.945764462919}{0.388464598961}{0.945241245209}{0.400695885994}
  \meshline{144,144,144}{0.946140659317}{0.382513038989}{0.946286790032}{0.378437957286}
  \meshline{144,144,144}{0.855225496096}{0.387135027014}{0.856136973950}{0.379474998544}
  \meshline{144,144,144}{0.944499212579}{0.409201274803}{0.943095848309}{0.428382831396}
  \meshline{144,144,144}{0.822022250984}{0.068960869390}{0.825111416565}{0.070186117504}
  \meshline{144,144,144}{0.801776918856}{0.060974301330}{0.807733821997}{0.062984504311}
  \meshline{144,144,144}{0.809215285699}{0.063645559022}{0.807733821997}{0.062984504311}
  \meshline{144,144,144}{0.791197164798}{0.057431539441}{0.801776918856}{0.060974301330}
  \meshline{144,144,144}{0.757151326606}{0.048280575434}{0.771839866066}{0.052077328113}
  \meshline{144,144,144}{0.776514414816}{0.052871993733}{0.771839866066}{0.052077328113}
  \meshline{144,144,144}{0.738473186145}{0.044605414739}{0.748360745867}{0.046979595824}
  \meshline{144,144,144}{0.729018570568}{0.122603158728}{0.722018464718}{0.119444329582}
  \meshline{144,144,144}{0.748360745867}{0.046979595824}{0.757151326606}{0.048280575434}
  \meshline{144,144,144}{0.788786061028}{0.056830250866}{0.776514414816}{0.052871993733}
  \meshline{144,144,144}{0.788786061028}{0.056830250866}{0.791197164798}{0.057431539441}
  \meshline{144,144,144}{0.744198260217}{0.301395725284}{0.743952160955}{0.300505725152}
  \meshline{144,144,144}{0.743952160955}{0.300505725152}{0.739008227686}{0.286329214120}
  \meshline{144,144,144}{0.735623380190}{0.276752708261}{0.727341159325}{0.259254575753}
  \meshline{144,144,144}{0.716556100359}{0.242577608560}{0.727341159325}{0.259254575753}
  \meshline{144,144,144}{0.672318850851}{0.197749649555}{0.682538696294}{0.205468232510}
  \meshline{144,144,144}{0.714723749729}{0.239852649182}{0.715562006624}{0.240959272227}
  \meshline{144,144,144}{0.745260954525}{0.131832846923}{0.738687649447}{0.127792859565}
  \meshline{144,144,144}{0.684798014727}{0.207314180422}{0.691690084969}{0.214147629706}
  \meshline{144,144,144}{0.782938894658}{0.160811376630}{0.772143178195}{0.150887202176}
  \meshline{144,144,144}{0.763102651165}{0.144094643342}{0.772143178195}{0.150887202176}
  \meshline{144,144,144}{0.744198260217}{0.301395725284}{0.744443537485}{0.302546991065}
  \meshline{144,144,144}{0.507339928537}{0.215239780306}{0.520078677845}{0.215430274558}
  \meshline{144,144,144}{0.700166571664}{0.222108980760}{0.691690084969}{0.214147629706}
  \meshline{144,144,144}{0.603616302644}{0.083941819176}{0.612257741181}{0.085449446443}
  \meshline{144,144,144}{0.700166571664}{0.222108980760}{0.702768604579}{0.225082397047}
  \meshline{144,144,144}{0.702768604579}{0.225082397047}{0.714723749729}{0.239852649182}
  \meshline{144,144,144}{0.672318850851}{0.197749649555}{0.666538038012}{0.193193361910}
  \meshline{144,144,144}{0.647622340950}{0.181457071557}{0.663942636955}{0.191568484800}
  \meshline{144,144,144}{0.682538696294}{0.205468232510}{0.684798014727}{0.207314180422}
  \meshline{144,144,144}{0.511918078305}{0.297894345451}{0.514872132020}{0.298412698754}
  \meshline{144,144,144}{0.853872285693}{0.398433394001}{0.849237097789}{0.423283004470}
  \meshline{144,144,144}{0.855225496096}{0.387135027014}{0.854251768295}{0.396210106225}
  \meshline{144,144,144}{0.853872285693}{0.398433394001}{0.854251768295}{0.396210106225}
  \meshline{144,144,144}{0.750623851259}{0.342410258234}{0.749391245483}{0.328808604876}
  \meshline{144,144,144}{0.747141735918}{0.313501479426}{0.749163836833}{0.326897719892}
  \meshline{144,144,144}{0.753873469605}{0.137472416131}{0.745260954525}{0.131832846923}
  \meshline{144,144,144}{0.666538038012}{0.193193361910}{0.663942636955}{0.191568484800}
  \meshline{144,144,144}{0.738687649447}{0.127792859565}{0.729018570568}{0.122603158728}
  \meshline{144,144,144}{0.722018464718}{0.119444329582}{0.706204078391}{0.111846473736}
  \meshline{144,144,144}{0.659188977536}{0.095801965372}{0.676586512052}{0.100985083478}
  \meshline{144,144,144}{0.715562006624}{0.240959272227}{0.716556100359}{0.242577608560}
  \meshline{144,144,144}{0.736015685628}{0.277610928033}{0.739008227686}{0.286329214120}
  \meshline{144,144,144}{0.736015685628}{0.277610928033}{0.735623380190}{0.276752708261}
  \meshline{144,144,144}{0.629234684973}{0.172434710739}{0.632621168210}{0.174063979432}
  \meshline{144,144,144}{0.632621168210}{0.174063979432}{0.647622340950}{0.181457071557}
  \meshline{144,144,144}{0.625122320186}{0.170832574433}{0.610232590082}{0.164786653682}
  \meshline{144,144,144}{0.640469379609}{0.090902267469}{0.658088608516}{0.095552103936}
  \meshline{144,144,144}{0.623930464171}{0.031237114815}{0.636383968615}{0.031826618071}
  \meshline{144,144,144}{0.640469379609}{0.090902267469}{0.629569514128}{0.088750534558}
  \meshline{144,144,144}{0.749391245483}{0.328808604876}{0.749328382676}{0.327884037080}
  \meshline{144,144,144}{0.749328382676}{0.327884037080}{0.749163836833}{0.326897719892}
  \meshline{144,144,144}{0.750741593283}{0.356455499259}{0.750703520621}{0.348854565129}
  \meshline{144,144,144}{0.750623851259}{0.342410258234}{0.750703520621}{0.348854565129}
  \meshline{144,144,144}{0.844879757948}{0.439669727120}{0.849075245108}{0.423961804853}
  \meshline{144,144,144}{0.837336273620}{0.461160951518}{0.837842617726}{0.459667303126}
  \meshline{144,144,144}{0.701497399363}{0.110092685151}{0.706204078391}{0.111846473736}
  \meshline{144,144,144}{0.701497399363}{0.110092685151}{0.679387660689}{0.101870759091}
  \meshline{144,144,144}{0.582206608153}{0.230586288160}{0.572777865144}{0.226947377023}
  \meshline{144,144,144}{0.747141735918}{0.313501479426}{0.744443537485}{0.302546991065}
  \meshline{144,144,144}{0.750741593283}{0.356455499259}{0.749631290502}{0.369193555877}
  \meshline{144,144,144}{0.562886614171}{0.331553010546}{0.565505201817}{0.335878795283}
  \meshline{144,144,144}{0.636844369069}{0.272541571633}{0.632287056807}{0.267455997662}
  \meshline{144,144,144}{0.603093554678}{0.242212124611}{0.612935724522}{0.248990096574}
  \meshline{144,144,144}{0.636844369069}{0.272541571633}{0.641962838624}{0.279781708419}
  \meshline{144,144,144}{0.622785302128}{0.257588902090}{0.623963948782}{0.258656542156}
  \meshline{144,144,144}{0.650773626231}{0.295121178514}{0.646290121368}{0.286169264442}
  \meshline{144,144,144}{0.849075245108}{0.423961804853}{0.849237097789}{0.423283004470}
  \meshline{144,144,144}{0.650773626231}{0.295121178514}{0.654761850739}{0.302604192083}
  \meshline{144,144,144}{0.654761850739}{0.302604192083}{0.657276805154}{0.308413962209}
  \meshline{144,144,144}{0.641962838624}{0.279781708419}{0.646290121368}{0.286169264442}
  \meshline{144,144,144}{0.587889113863}{0.233606969317}{0.582206608153}{0.230586288160}
  \meshline{144,144,144}{0.746539944040}{0.390525221503}{0.747921782033}{0.381430282533}
  \meshline{144,144,144}{0.749375407717}{0.372679749917}{0.747921782033}{0.381430282533}
  \meshline{144,144,144}{0.738279580966}{0.418301885957}{0.745656562961}{0.393790546673}
  \meshline{144,144,144}{0.746226017779}{0.391967316082}{0.746539944040}{0.390525221503}
  \meshline{144,144,144}{0.662111931377}{0.325094216247}{0.662302752296}{0.325734171750}
  \meshline{144,144,144}{0.662111931377}{0.325094216247}{0.657276805154}{0.308413962209}
  \meshline{144,144,144}{0.746226017779}{0.391967316082}{0.745656562961}{0.393790546673}
  \meshline{144,144,144}{0.749375407717}{0.372679749917}{0.749631290502}{0.369193555877}
  \meshline{144,144,144}{0.662387342987}{0.326139200964}{0.662563893324}{0.327928289008}
  \meshline{144,144,144}{0.664088081895}{0.358788625552}{0.663422505510}{0.368473494814}
  \meshline{144,144,144}{0.662302752296}{0.325734171750}{0.662387342987}{0.326139200964}
  \meshline{144,144,144}{0.632287056807}{0.267455997662}{0.623963948782}{0.258656542156}
  \meshline{144,144,144}{0.622785302128}{0.257588902090}{0.612935724522}{0.248990096574}
  \meshline{144,144,144}{0.738153856779}{0.418602948709}{0.738279580966}{0.418301885957}
  \meshline{144,144,144}{0.823485947872}{0.490108369800}{0.831056760679}{0.475939093967}
  \meshline{144,144,144}{0.603093554678}{0.242212124611}{0.599850562103}{0.240013275127}
  \meshline{144,144,144}{0.520078677845}{0.215430274558}{0.526041687593}{0.215960941272}
  \meshline{144,144,144}{0.623383663737}{0.087336697183}{0.629569514128}{0.088750534558}
  \meshline{144,144,144}{0.596509383587}{0.160542289408}{0.588314951031}{0.157998757003}
  \meshline{144,144,144}{0.625122320186}{0.170832574433}{0.629234684973}{0.172434710739}
  \meshline{144,144,144}{0.623383663737}{0.087336697183}{0.612257741181}{0.085449446443}
  \meshline{144,144,144}{0.557290455317}{0.151606248521}{0.565478265001}{0.153194984132}
  \meshline{144,144,144}{0.576360922390}{0.155184498700}{0.580408509536}{0.156056768467}
  \meshline{144,144,144}{0.599121183233}{0.083431456488}{0.603616302644}{0.083941819176}
  \meshline{144,144,144}{0.559900784248}{0.079110131222}{0.552462267614}{0.078448482943}
  \meshline{144,144,144}{0.572217459985}{0.080033774955}{0.580478699918}{0.080849561238}
  \meshline{144,144,144}{0.731869258297}{0.433044078820}{0.729993925000}{0.436659907961}
  \meshline{144,144,144}{0.738153856779}{0.418602948709}{0.731869258297}{0.433044078820}
  \meshline{144,144,144}{0.844879757948}{0.439669727120}{0.837842617726}{0.459667303126}
  \meshline{144,144,144}{0.837196641944}{0.461491649318}{0.837336273620}{0.461160951518}
  \meshline{144,144,144}{0.712362102980}{0.464766218026}{0.715386659873}{0.460964566279}
  \meshline{144,144,144}{0.718597461788}{0.455841447747}{0.724873023466}{0.446554740533}
  \meshline{144,144,144}{0.823041900834}{0.490990963649}{0.822458256741}{0.491893417148}
  \meshline{144,144,144}{0.712362102980}{0.464766218026}{0.706489020157}{0.471232393859}
  \meshline{144,144,144}{0.718597461788}{0.455841447747}{0.715386659873}{0.460964566279}
  \meshline{144,144,144}{0.823485947872}{0.490108369800}{0.823041900834}{0.490990963649}
  \meshline{144,144,144}{0.837196641944}{0.461491649318}{0.836772603942}{0.462433518335}
  \meshline{144,144,144}{0.831056760679}{0.475939093967}{0.836772603942}{0.462433518335}
  \meshline{144,144,144}{0.811062814633}{0.510001248979}{0.822458256741}{0.491893417148}
  \meshline{144,144,144}{0.811062814633}{0.510001248979}{0.806333708084}{0.516421974672}
  \meshline{144,144,144}{0.794229168487}{0.530442257742}{0.806333708084}{0.516421974672}
  \meshline{144,144,144}{0.733030639861}{0.577482768295}{0.733715112254}{0.577138106596}
  \meshline{144,144,144}{0.562886614171}{0.331553010546}{0.555914939504}{0.318939854441}
  \meshline{144,144,144}{0.566970004538}{0.355733558958}{0.566606785952}{0.340516354437}
  \meshline{144,144,144}{0.587889113863}{0.233606969317}{0.599850562103}{0.240013275127}
  \meshline{144,144,144}{0.554097008083}{0.221153961809}{0.545581794335}{0.218835543489}
  \meshline{144,144,144}{0.572777865144}{0.226947377023}{0.564894055538}{0.224038167771}
  \meshline{144,144,144}{0.596509383587}{0.160542289408}{0.610232590082}{0.164786653682}
  \meshline{144,144,144}{0.580478699918}{0.080849561238}{0.599121183233}{0.083431456488}
  \meshline{144,144,144}{0.598712786022}{0.029690392896}{0.584612550334}{0.028875812397}
  \meshline{144,144,144}{0.611088832084}{0.030154187207}{0.598712786022}{0.029690392896}
  \meshline{144,144,144}{0.724873023466}{0.446554740533}{0.729993925000}{0.436659907961}
  \meshline{144,144,144}{0.555914939504}{0.318939854441}{0.545080564486}{0.310706329770}
  \meshline{144,144,144}{0.566369652215}{0.360222344776}{0.566970004538}{0.355733558958}
  \meshline{144,144,144}{0.588314951031}{0.157998757003}{0.580408509536}{0.156056768467}
  \meshline{144,144,144}{0.576133435421}{0.028620206429}{0.584612550334}{0.028875812397}
  \meshline{144,144,144}{0.623930464171}{0.031237114815}{0.617287726367}{0.030619318573}
  \meshline{144,144,144}{0.694642802155}{0.037928344268}{0.703556372312}{0.038978080858}
  \meshline{144,144,144}{0.648589193412}{0.033009264542}{0.636383968615}{0.031826618071}
  \meshline{144,144,144}{0.648589193412}{0.033009264542}{0.651694268451}{0.033187326104}
  \meshline{144,144,144}{0.671800540884}{0.035358946527}{0.682189000609}{0.036090436950}
  \meshline{144,144,144}{0.676586512052}{0.100985083478}{0.679387660689}{0.101870759091}
  \meshline{144,144,144}{0.682189000609}{0.036090436950}{0.694642802155}{0.037928344268}
  \meshline{144,144,144}{0.658088608516}{0.095552103936}{0.659188977536}{0.095801965372}
  \meshline{144,144,144}{0.721650656757}{0.042143511023}{0.738473186145}{0.044605414739}
  \meshline{144,144,144}{0.714981270126}{0.040821683515}{0.721650656757}{0.042143511023}
  \meshline{144,144,144}{0.671800540884}{0.035358946527}{0.651694268451}{0.033187326104}
  \meshline{144,144,144}{0.714981270126}{0.040821683515}{0.703556372312}{0.038978080858}
  \meshline{144,144,144}{0.488658565690}{0.301117879113}{0.497105868928}{0.299233830101}
  \meshline{144,144,144}{0.566606785952}{0.340516354437}{0.565505201817}{0.335878795283}
  \meshline{144,144,144}{0.558886480563}{0.376467513914}{0.549444110076}{0.387064455861}
  \meshline{144,144,144}{0.549444110076}{0.387064455861}{0.534203189010}{0.396715329009}
  \meshline{144,144,144}{0.562446316304}{0.369879653919}{0.558886480563}{0.376467513914}
  \meshline{144,144,144}{0.505260854991}{0.401388725049}{0.515635860624}{0.401425315899}
  \meshline{144,144,144}{0.508256255679}{0.297630173222}{0.511918078305}{0.297894345451}
  \meshline{144,144,144}{0.545080564486}{0.310706329770}{0.537942587604}{0.305718979129}
  \meshline{144,144,144}{0.564894055538}{0.224038167771}{0.554097008083}{0.221153961809}
  \meshline{144,144,144}{0.545581794335}{0.218835543489}{0.542348158067}{0.218209793126}
  \meshline{144,144,144}{0.565478265001}{0.153194984132}{0.576360922390}{0.155184498700}
  \meshline{144,144,144}{0.541689104493}{0.149680079818}{0.537392493628}{0.149136521297}
  \meshline{144,144,144}{0.477180749479}{0.149180393497}{0.484725163261}{0.148727959872}
  \meshline{144,144,144}{0.541689104493}{0.149680079818}{0.557290455317}{0.151606248521}
  \meshline{144,144,144}{0.524458867566}{0.148362769953}{0.519877042062}{0.148047338729}
  \meshline{144,144,144}{0.535005707846}{0.077528650766}{0.532750295507}{0.077407416743}
  \meshline{144,144,144}{0.517662800148}{0.148018234662}{0.497654327403}{0.147904117795}
  \meshline{144,144,144}{0.537392493628}{0.149136521297}{0.524458867566}{0.148362769953}
  \meshline{144,144,144}{0.617287726367}{0.030619318573}{0.611088832084}{0.030154187207}
  \meshline{144,144,144}{0.537942587604}{0.305718979129}{0.522728747477}{0.300432049340}
  \meshline{144,144,144}{0.664744335552}{0.348781203691}{0.662563893324}{0.327928289008}
  \meshline{144,144,144}{0.664088081895}{0.358788625552}{0.664744335552}{0.348781203691}
  \meshline{144,144,144}{0.488658565690}{0.301117879113}{0.480757676736}{0.304420716154}
  \meshline{144,144,144}{0.470263549050}{0.310137606644}{0.480757676736}{0.304420716154}
  \meshline{144,144,144}{0.465302280915}{0.314213363902}{0.470263549050}{0.310137606644}
  \meshline{144,144,144}{0.654444948608}{0.607305167360}{0.643959660853}{0.610138608738}
  \meshline{144,144,144}{0.450281984126}{0.355650025873}{0.449835614679}{0.344735676688}
  \meshline{144,144,144}{0.497105868928}{0.299233830101}{0.508256255679}{0.297630173222}
  \meshline{144,144,144}{0.450035787699}{0.224160738897}{0.455020646296}{0.222713749905}
  \meshline{144,144,144}{0.499089596106}{0.215223972175}{0.507339928537}{0.215239780306}
  \meshline{144,144,144}{0.485525264741}{0.216274197355}{0.482581873953}{0.216575718131}
  \meshline{144,144,144}{0.542348158067}{0.218209793126}{0.536720102092}{0.217418844906}
  \meshline{144,144,144}{0.499089596106}{0.215223972175}{0.485525264741}{0.216274197355}
  \meshline{144,144,144}{0.526041687593}{0.215960941272}{0.536720102092}{0.217418844906}
  \meshline{144,144,144}{0.514872132020}{0.298412698754}{0.522728747477}{0.300432049340}
  \meshline{144,144,144}{0.451732367594}{0.334470964255}{0.453243434387}{0.330206719012}
  \meshline{144,144,144}{0.940502655781}{0.449727675091}{0.940181136697}{0.452358618038}
  \meshline{144,144,144}{0.940502655781}{0.449727675091}{0.940943739189}{0.445519689812}
  \meshline{144,144,144}{0.927085448252}{0.513970728273}{0.926660700862}{0.515085092190}
  \meshline{144,144,144}{0.926660700862}{0.515085092190}{0.922138808538}{0.527113682592}
  \meshline{144,144,144}{0.535288494928}{0.027579794642}{0.550823041006}{0.027825476982}
  \meshline{144,144,144}{0.566176731493}{0.028355751619}{0.557217532580}{0.028010030538}
  \meshline{144,144,144}{0.566176731493}{0.028355751619}{0.576133435421}{0.028620206429}
  \meshline{144,144,144}{0.559900784248}{0.079110131222}{0.572217459985}{0.080033774955}
  \meshline{144,144,144}{0.535005707846}{0.077528650766}{0.552462267614}{0.078448482943}
  \meshline{144,144,144}{0.517965802831}{0.076983531390}{0.532750295507}{0.077407416743}
  \meshline{144,144,144}{0.509415399287}{0.076951973529}{0.499276044931}{0.076949594277}
  \meshline{144,144,144}{0.535288494928}{0.027579794642}{0.524353219340}{0.027426489766}
  \meshline{144,144,144}{0.557217532580}{0.028010030538}{0.550823041006}{0.027825476982}
  \meshline{144,144,144}{0.516232470401}{0.027378941203}{0.524353219340}{0.027426489766}
  \meshline{144,144,144}{0.754434575719}{0.564557625339}{0.766086782717}{0.556245576607}
  \meshline{144,144,144}{0.766086782717}{0.556245576607}{0.777450237187}{0.546990868510}
  \meshline{144,144,144}{0.730266983763}{0.578827749670}{0.715851438075}{0.586230582504}
  \meshline{144,144,144}{0.790587787698}{0.534515767196}{0.794229168487}{0.530442257742}
  \meshline{144,144,144}{0.733715112254}{0.577138106596}{0.752417631615}{0.565956527235}
  \meshline{144,144,144}{0.754434575719}{0.564557625339}{0.752824410334}{0.565717833032}
  \meshline{144,144,144}{0.786991861166}{0.537769323821}{0.781462866211}{0.543456479616}
  \meshline{144,144,144}{0.829613284798}{0.632473744697}{0.824006558954}{0.634502683948}
  \meshline{144,144,144}{0.777450237187}{0.546990868510}{0.781462866211}{0.543456479616}
  \meshline{144,144,144}{0.790587787698}{0.534515767196}{0.786991861166}{0.537769323821}
  \meshline{144,144,144}{0.900280939049}{0.573361010186}{0.898548486258}{0.575950840240}
  \meshline{144,144,144}{0.786892306620}{0.648028719223}{0.787158108545}{0.647925586529}
  \meshline{144,144,144}{0.752824410334}{0.565717833032}{0.752417631615}{0.565956527235}
  \meshline{144,144,144}{0.515635860624}{0.401425315899}{0.530431294195}{0.398501981499}
  \meshline{144,144,144}{0.456232862330}{0.374086140248}{0.454588690179}{0.369659962357}
  \meshline{144,144,144}{0.453243434387}{0.330206719012}{0.455994395213}{0.325771148466}
  \meshline{144,144,144}{0.465302280915}{0.314213363902}{0.455994395213}{0.325771148466}
  \meshline{144,144,144}{0.451732367594}{0.334470964255}{0.449835614679}{0.344735676688}
  \meshline{144,144,144}{0.456232862330}{0.374086140248}{0.458258284870}{0.377752284976}
  \meshline{144,144,144}{0.659519729808}{0.385800076335}{0.661457285641}{0.377445233671}
  \meshline{144,144,144}{0.461157785655}{0.221252534849}{0.475976184761}{0.218069698121}
  \meshline{144,144,144}{0.497654327403}{0.147904117795}{0.484725163261}{0.148727959872}
  \meshline{144,144,144}{0.477180749479}{0.149180393497}{0.472261502688}{0.149814226205}
  \meshline{144,144,144}{0.477895296212}{0.027614057611}{0.489127152471}{0.027445569429}
  \meshline{144,144,144}{0.517965802831}{0.076983531390}{0.509415399287}{0.076951973529}
  \meshline{144,144,144}{0.460413710518}{0.151114564658}{0.472261502688}{0.149814226205}
  \meshline{144,144,144}{0.498021692823}{0.027417414537}{0.489127152471}{0.027445569429}
  \meshline{144,144,144}{0.439699310261}{0.028553122263}{0.438972873578}{0.028553122263}
  \meshline{144,144,144}{0.483653152614}{0.077343223616}{0.483637721526}{0.077343475371}
  \meshline{144,144,144}{0.498021692823}{0.027417414537}{0.516232470401}{0.027378941203}
  \meshline{144,144,144}{0.470456665445}{0.027704653853}{0.477895296212}{0.027614057611}
  \meshline{144,144,144}{0.475976184761}{0.218069698121}{0.482581873953}{0.216575718131}
  \meshline{144,144,144}{0.450035787699}{0.224160738897}{0.438300300311}{0.228834714741}
  \meshline{144,144,144}{0.376861550057}{0.274690161344}{0.372938534774}{0.280082889912}
  \meshline{144,144,144}{0.364218485970}{0.295056754732}{0.362305743784}{0.298279109333}
  \meshline{144,144,144}{0.438300300311}{0.228834714741}{0.423360774117}{0.235514844253}
  \meshline{144,144,144}{0.432612524225}{0.156555289368}{0.435969131102}{0.155932476527}
  \meshline{144,144,144}{0.419613570775}{0.237592991034}{0.414457864771}{0.241300456096}
  \meshline{144,144,144}{0.421409824690}{0.082518186894}{0.418435712259}{0.082950447056}
  \meshline{144,144,144}{0.460413710518}{0.151114564658}{0.453649653694}{0.152344969989}
  \meshline{144,144,144}{0.453649653694}{0.152344969989}{0.435969131102}{0.155932476527}
  \meshline{144,144,144}{0.470456665445}{0.027704653853}{0.467630968587}{0.027789030432}
  \meshline{144,144,144}{0.467630968587}{0.027789030432}{0.462902780470}{0.027937557931}
  \meshline{144,144,144}{0.438972873578}{0.028553122263}{0.437402566640}{0.028594237811}
  \meshline{144,144,144}{0.454728221130}{0.028075291406}{0.462902780470}{0.027937557931}
  \meshline{144,144,144}{0.454728221130}{0.028075291406}{0.439699310261}{0.028553122263}
  \meshline{144,144,144}{0.455020646296}{0.222713749905}{0.461157785655}{0.221252534849}
  \meshline{144,144,144}{0.397236721658}{0.253269151208}{0.414457864771}{0.241300456096}
  \meshline{144,144,144}{0.385315182336}{0.172436048700}{0.400153458429}{0.166605273292}
  \meshline{144,144,144}{0.483653152614}{0.077343223616}{0.499276044931}{0.076949594277}
  \meshline{144,144,144}{0.483631196082}{0.077343806773}{0.483637721526}{0.077343475371}
  \meshline{144,144,144}{0.483631196082}{0.077343806773}{0.465219579154}{0.078248331431}
  \meshline{144,144,144}{0.446089009067}{0.079751877497}{0.460395554790}{0.078650467670}
  \meshline{144,144,144}{0.423513269655}{0.082315485181}{0.443219608186}{0.079980435563}
  \meshline{144,144,144}{0.423360774117}{0.235514844253}{0.419613570775}{0.237592991034}
  \meshline{144,144,144}{0.383999586242}{0.266120128313}{0.389050540624}{0.261429940054}
  \meshline{144,144,144}{0.430261411458}{0.157166702464}{0.432612524225}{0.156555289368}
  \meshline{144,144,144}{0.403800476716}{0.165186278238}{0.400153458429}{0.166605273292}
  \meshline{144,144,144}{0.465219579154}{0.078248331431}{0.460395554790}{0.078650467670}
  \meshline{144,144,144}{0.443219608186}{0.079980435563}{0.446089009067}{0.079751877497}
  \meshline{144,144,144}{0.410439849675}{0.029776038207}{0.402539667328}{0.030380319290}
  \meshline{144,144,144}{0.402539667328}{0.030380319290}{0.394120256193}{0.030816095721}
  \meshline{144,144,144}{0.376861550057}{0.274690161344}{0.383999586242}{0.266120128313}
  \meshline{144,144,144}{0.372938534774}{0.280082889912}{0.364218485970}{0.295056754732}
  \meshline{144,144,144}{0.361466419861}{0.300227634880}{0.354925795007}{0.318557044613}
  \meshline{144,144,144}{0.361466419861}{0.300227634880}{0.362305743784}{0.298279109333}
  \meshline{144,144,144}{0.353465019632}{0.324768738747}{0.354925795007}{0.318557044613}
  \meshline{144,144,144}{0.289557829873}{0.254734971086}{0.289868050985}{0.254171693061}
  \meshline{144,144,144}{0.389050540624}{0.261429940054}{0.397236721658}{0.253269151208}
  \meshline{144,144,144}{0.320290331694}{0.106769081781}{0.315946025070}{0.108433824287}
  \meshline{144,144,144}{0.283781558897}{0.123099143001}{0.292240596217}{0.118581873811}
  \meshline{144,144,144}{0.329986489927}{0.036511330508}{0.331083107096}{0.036389640851}
  \meshline{144,144,144}{0.389837855206}{0.087581937557}{0.371861358728}{0.091543986481}
  \meshline{144,144,144}{0.437402566640}{0.028594237811}{0.418653844991}{0.029506444809}
  \meshline{144,144,144}{0.374061682932}{0.032108690507}{0.391489125004}{0.031057357066}
  \meshline{144,144,144}{0.355842335488}{0.095480586871}{0.346823231246}{0.098034029478}
  \meshline{144,144,144}{0.410439849675}{0.029776038207}{0.418653844991}{0.029506444809}
  \meshline{144,144,144}{0.286916800719}{0.042752522209}{0.300938455867}{0.040405628049}
  \meshline{144,144,144}{0.366099676541}{0.092741922064}{0.355842335488}{0.095480586871}
  \meshline{144,144,144}{0.355835805596}{0.034003524377}{0.367358979019}{0.032785538029}
  \meshline{144,144,144}{0.330945698843}{0.103014892716}{0.340395892810}{0.100264441387}
  \meshline{144,144,144}{0.374061682932}{0.032108690507}{0.367358979019}{0.032785538029}
  \meshline{144,144,144}{0.394120256193}{0.030816095721}{0.391489125004}{0.031057357066}
  \meshline{144,144,144}{0.423513269655}{0.082315485181}{0.421409824690}{0.082518186894}
  \meshline{144,144,144}{0.418435712259}{0.082950447056}{0.395984948010}{0.086587140094}
  \meshline{144,144,144}{0.389837855206}{0.087581937557}{0.395984948010}{0.086587140094}
  \meshline{144,144,144}{0.366099676541}{0.092741922064}{0.371861358728}{0.091543986481}
  \meshline{144,144,144}{0.304631664310}{0.039663986730}{0.300938455867}{0.040405628049}
  \meshline{144,144,144}{0.355835805596}{0.034003524377}{0.348989701228}{0.034428203108}
  \meshline{144,144,144}{0.348989701228}{0.034428203108}{0.331083107096}{0.036389640851}
  \meshline{144,144,144}{0.329986489927}{0.036511330508}{0.329618407493}{0.036576758293}
  \meshline{144,144,144}{0.277537716855}{0.044167130622}{0.286916800719}{0.042752522209}
  \meshline{144,144,144}{0.329618407493}{0.036576758293}{0.304631664310}{0.039663986730}
  \meshline{144,144,144}{0.326208133365}{0.210466975672}{0.321107821832}{0.214907920937}
  \meshline{144,144,144}{0.315946025070}{0.108433824287}{0.301203547355}{0.114866504738}
  \meshline{144,144,144}{0.293790140834}{0.117941358529}{0.301203547355}{0.114866504738}
  \meshline{144,144,144}{0.340395892810}{0.100264441387}{0.346823231246}{0.098034029478}
  \meshline{144,144,144}{0.320290331694}{0.106769081781}{0.330945698843}{0.103014892716}
  \meshline{144,144,144}{0.317004260779}{0.219395196258}{0.321107821832}{0.214907920937}
  \meshline{144,144,144}{0.385315182336}{0.172436048700}{0.380978338466}{0.174490615850}
  \meshline{144,144,144}{0.403800476716}{0.165186278238}{0.418149869345}{0.160400643605}
  \meshline{144,144,144}{0.277537716855}{0.044167130622}{0.275590261008}{0.044392650744}
  \meshline{144,144,144}{0.266160430422}{0.046425892351}{0.251708905358}{0.049028815106}
  \meshline{144,144,144}{0.275590261008}{0.044392650744}{0.266160430422}{0.046425892351}
  \meshline{144,144,144}{0.380978338466}{0.174490615850}{0.365161469820}{0.182712288790}
  \meshline{144,144,144}{0.351863163261}{0.190502425394}{0.341607776353}{0.198137906990}
  \meshline{144,144,144}{0.341607776353}{0.198137906990}{0.336448561088}{0.201694041869}
  \meshline{144,144,144}{0.219243261688}{0.170092757151}{0.209747048336}{0.180457641571}
  \meshline{144,144,144}{0.283781558897}{0.123099143001}{0.272415631535}{0.129047233981}
  \meshline{144,144,144}{0.272415631535}{0.129047233981}{0.268633205919}{0.131601100109}
  \meshline{144,144,144}{0.351863163261}{0.190502425394}{0.359678823516}{0.185914313257}
  \meshline{144,144,144}{0.268633205919}{0.131601100109}{0.253964217185}{0.140454057799}
  \meshline{144,144,144}{0.240892951252}{0.150546291509}{0.253964217185}{0.140454057799}
  \meshline{144,144,144}{0.292240596217}{0.118581873811}{0.293790140834}{0.117941358529}
  \meshline{144,144,144}{0.236669260707}{0.154037045812}{0.238356681728}{0.152437876090}
  \meshline{144,144,144}{0.219243261688}{0.170092757151}{0.222349528293}{0.166727075158}
  \meshline{144,144,144}{0.182994648596}{0.219980720079}{0.184061197686}{0.218188923469}
  \meshline{144,144,144}{0.181997418589}{0.222095807631}{0.182994648596}{0.219980720079}
  \meshline{144,144,144}{0.222349528293}{0.166727075158}{0.236669260707}{0.154037045812}
  \meshline{144,144,144}{0.418149869345}{0.160400643605}{0.430261411458}{0.157166702464}
  \meshline{144,144,144}{0.245455314085}{0.050814800350}{0.251708905358}{0.049028815106}
  \meshline{144,144,144}{0.365161469820}{0.182712288790}{0.359678823516}{0.185914313257}
  \meshline{144,144,144}{0.326208133365}{0.210466975672}{0.336448561088}{0.201694041869}
  \meshline{144,144,144}{0.303740441169}{0.234075595305}{0.300736287851}{0.237935305367}
  \meshline{144,144,144}{0.303740441169}{0.234075595305}{0.317004260779}{0.219395196258}
  \meshline{144,144,144}{0.289557829873}{0.254734971086}{0.280258049195}{0.272126583911}
  \meshline{144,144,144}{0.289868050985}{0.254171693061}{0.300736287851}{0.237935305367}
  \meshline{144,144,144}{0.194678266710}{0.200494841253}{0.199679943824}{0.193251319820}
  \meshline{144,144,144}{0.353465019632}{0.324768738747}{0.350866947773}{0.348729062004}
  \meshline{144,144,144}{0.238356681728}{0.152437876090}{0.240892951252}{0.150546291509}
  \meshline{144,144,144}{0.181997418589}{0.222095807631}{0.176295394175}{0.233497818941}
  \meshline{144,144,144}{0.194749323296}{0.065885854509}{0.207402403461}{0.061787677901}
  \meshline{144,144,144}{0.227723766668}{0.055387573731}{0.237136355145}{0.053267931757}
  \meshline{144,144,144}{0.168543465698}{0.078113120216}{0.178106624841}{0.073008640267}
  \meshline{144,144,144}{0.160000674661}{0.082655945921}{0.149205122461}{0.088965453741}
  \meshline{144,144,144}{0.213762694918}{0.059381356341}{0.227723766668}{0.055387573731}
  \meshline{144,144,144}{0.213762694918}{0.059381356341}{0.207402403461}{0.061787677901}
  \meshline{144,144,144}{0.209747048336}{0.180457641571}{0.199679943824}{0.193251319820}
  \meshline{144,144,144}{0.130487092554}{0.103417540533}{0.144633418928}{0.092773709511}
  \meshline{144,144,144}{0.149205122461}{0.088965453741}{0.144633418928}{0.092773709511}
  \meshline{144,144,144}{0.184265565046}{0.070199045254}{0.178106624841}{0.073008640267}
  \meshline{144,144,144}{0.237136355145}{0.053267931757}{0.245455314085}{0.050814800350}
  \meshline{144,144,144}{0.176295394175}{0.233497818941}{0.171470186238}{0.245873862224}
  \meshline{144,144,144}{0.117010514402}{0.117358096063}{0.126425581163}{0.107532966025}
  \meshline{144,144,144}{0.126425581163}{0.107532966025}{0.130487092554}{0.103417540533}
  \meshline{144,144,144}{0.160000674661}{0.082655945921}{0.164467493981}{0.079920617685}
  \meshline{144,144,144}{0.184265565046}{0.070199045254}{0.194749323296}{0.065885854509}
  \meshline{144,144,144}{0.164467493981}{0.079920617685}{0.168543465698}{0.078113120216}
  \meshline{144,144,144}{0.194678266710}{0.200494841253}{0.184061197686}{0.218188923469}
  \meshline{144,144,144}{0.171470186238}{0.245873862224}{0.168077375954}{0.254213895048}
  \meshline{144,144,144}{0.060783729083}{0.280535803854}{0.059754726355}{0.293991762120}
  \meshline{144,144,144}{0.350946582061}{0.353127513193}{0.350748738939}{0.350861566244}
  \meshline{144,144,144}{0.352085488075}{0.366799179405}{0.354640252557}{0.379325671157}
  \meshline{144,144,144}{0.350748738939}{0.350861566244}{0.350866947773}{0.348729062004}
  \meshline{144,144,144}{0.350946582061}{0.353127513193}{0.352085488075}{0.366799179405}
  \meshline{144,144,144}{0.367058730384}{0.409379397960}{0.361900585659}{0.399598507965}
  \meshline{144,144,144}{0.944499212579}{0.409201274803}{0.945241245209}{0.400695885994}
  \meshline{144,144,144}{0.943095848309}{0.428382831396}{0.940943739189}{0.445519689812}
  \meshline{144,144,144}{0.922138808538}{0.527113682592}{0.916249566371}{0.543560865844}
  \meshline{144,144,144}{0.932906931711}{0.492038197349}{0.933435652079}{0.489400347826}
  \meshline{144,144,144}{0.932781381362}{0.492488337380}{0.932906931711}{0.492038197349}
  \meshline{144,144,144}{0.932581345847}{0.493108141561}{0.927085448252}{0.513970728273}
  \meshline{144,144,144}{0.937112740136}{0.471752769465}{0.937455936089}{0.469089562299}
  \meshline{144,144,144}{0.933435652079}{0.489400347826}{0.937112740136}{0.471752769465}
  \meshline{144,144,144}{0.940181136697}{0.452358618038}{0.937455936089}{0.469089562299}
  \meshline{144,144,144}{0.932581345847}{0.493108141561}{0.932781381362}{0.492488337380}
  \meshline{144,144,144}{0.634355392384}{0.431700809310}{0.636657395504}{0.428941683835}
  \meshline{144,144,144}{0.695448770103}{0.484172998742}{0.706489020157}{0.471232393859}
  \meshline{144,144,144}{0.664321554983}{0.509395527637}{0.669418692219}{0.505486863924}
  \meshline{144,144,144}{0.639474986339}{0.424691265962}{0.636657395504}{0.428941683835}
  \meshline{144,144,144}{0.654587565591}{0.398742169881}{0.653290659684}{0.402176318233}
  \meshline{144,144,144}{0.686163443705}{0.492555766595}{0.695448770103}{0.484172998742}
  \meshline{144,144,144}{0.680987504275}{0.497007650321}{0.669418692219}{0.505486863924}
  \meshline{144,144,144}{0.686163443705}{0.492555766595}{0.680987504275}{0.497007650321}
  \meshline{144,144,144}{0.678860168187}{0.600526002133}{0.669260006112}{0.603276926215}
  \meshline{144,144,144}{0.669260006112}{0.603276926215}{0.657423573734}{0.606641744371}
  \meshline{144,144,144}{0.760313028012}{0.655041814292}{0.765526448811}{0.653847485181}
  \meshline{144,144,144}{0.695627372244}{0.594747032796}{0.682538936393}{0.599119569587}
  \meshline{144,144,144}{0.628085750008}{0.613335125054}{0.617194219105}{0.615296395975}
  \meshline{144,144,144}{0.714949566028}{0.663212236372}{0.700867557542}{0.664646785235}
  \meshline{144,144,144}{0.711009509610}{0.588272438877}{0.695627372244}{0.594747032796}
  \meshline{144,144,144}{0.740167334667}{0.659124501967}{0.745798244665}{0.657789216415}
  \meshline{144,144,144}{0.725631164628}{0.661220148157}{0.714949566028}{0.663212236372}
  \meshline{144,144,144}{0.711009509610}{0.588272438877}{0.715851438075}{0.586230582504}
  \meshline{144,144,144}{0.678860168187}{0.600526002133}{0.682538936393}{0.599119569587}
  \meshline{144,144,144}{0.725631164628}{0.661220148157}{0.740167334667}{0.659124501967}
  \meshline{144,144,144}{0.695575901736}{0.665541582633}{0.700867557542}{0.664646785235}
  \meshline{144,144,144}{0.657423573734}{0.606641744371}{0.654444948608}{0.607305167360}
  \meshline{144,144,144}{0.369202183471}{0.413238649787}{0.373875015272}{0.420452814980}
  \meshline{144,144,144}{0.423125345623}{0.463605465380}{0.439497441585}{0.471601980298}
  \meshline{144,144,144}{0.695575901736}{0.665541582633}{0.675727684782}{0.667566557042}
  \meshline{144,144,144}{0.631888046227}{0.612509470694}{0.628085750008}{0.613335125054}
  \meshline{144,144,144}{0.643959660853}{0.610138608738}{0.631888046227}{0.612509470694}
  \meshline{144,144,144}{0.614697090659}{0.534485120445}{0.630660289703}{0.527775312360}
  \meshline{144,144,144}{0.662286937911}{0.510695661211}{0.664321554983}{0.509395527637}
  \meshline{144,144,144}{0.633204264561}{0.526785006137}{0.630660289703}{0.527775312360}
  \meshline{144,144,144}{0.595646830161}{0.540725246999}{0.583670448411}{0.543676987142}
  \meshline{144,144,144}{0.576448092717}{0.472143114293}{0.585654515058}{0.468210112168}
  \meshline{144,144,144}{0.635269216795}{0.525765162095}{0.633204264561}{0.526785006137}
  \meshline{144,144,144}{0.649846332640}{0.518318108110}{0.635269216795}{0.525765162095}
  \meshline{144,144,144}{0.662286937911}{0.510695661211}{0.649846332640}{0.518318108110}
  \meshline{144,144,144}{0.602071649131}{0.459141567650}{0.604563885831}{0.457440937136}
  \meshline{144,144,144}{0.530578484918}{0.551706684440}{0.513072711424}{0.552429275595}
  \meshline{144,144,144}{0.603221254947}{0.617415552257}{0.602674131470}{0.617507940277}
  \meshline{144,144,144}{0.604545889294}{0.538033262645}{0.614697090659}{0.534485120445}
  \meshline{144,144,144}{0.578129710927}{0.545180382591}{0.583670448411}{0.543676987142}
  \meshline{144,144,144}{0.599615408077}{0.539687293126}{0.595646830161}{0.540725246999}
  \meshline{144,144,144}{0.733030639861}{0.577482768295}{0.730266983763}{0.578827749670}
  \meshline{144,144,144}{0.685160061627}{0.741651342268}{0.692163480530}{0.742567564371}
  \meshline{144,144,144}{0.745798244665}{0.657789216415}{0.760313028012}{0.655041814292}
  \meshline{144,144,144}{0.423469576151}{0.779822770564}{0.436799270789}{0.778658793296}
  \meshline{144,144,144}{0.582095767480}{0.620124661370}{0.571922423815}{0.621021185195}
  \meshline{144,144,144}{0.675574714702}{0.667590480804}{0.674636367184}{0.667675222812}
  \meshline{144,144,144}{0.499442446327}{0.484898877195}{0.516947157525}{0.484966316164}
  \meshline{144,144,144}{0.604545889294}{0.538033262645}{0.599615408077}{0.539687293126}
  \meshline{144,144,144}{0.561538200077}{0.477490560051}{0.567791229661}{0.475602030256}
  \meshline{144,144,144}{0.551422826648}{0.549835751348}{0.554945457951}{0.549301562750}
  \meshline{144,144,144}{0.786404000942}{0.648169593642}{0.786892306620}{0.648028719223}
  \meshline{144,144,144}{0.787158108545}{0.647925586529}{0.788415557757}{0.647448274491}
  \meshline{144,144,144}{0.786404000942}{0.648169593642}{0.765526448811}{0.653847485181}
  \meshline{144,144,144}{0.803877050155}{0.642530093464}{0.788415557757}{0.647448274491}
  \meshline{144,144,144}{0.809559304973}{0.640893286673}{0.824006558954}{0.634502683948}
  \meshline{144,144,144}{0.809559304973}{0.640893286673}{0.803877050155}{0.642530093464}
  \meshline{144,144,144}{0.602071649131}{0.459141567650}{0.585654515058}{0.468210112168}
  \meshline{144,144,144}{0.604563885831}{0.457440937136}{0.619481640497}{0.446518748615}
  \meshline{144,144,144}{0.630651625937}{0.435351614900}{0.619481640497}{0.446518748615}
  \meshline{144,144,144}{0.634355392384}{0.431700809310}{0.630651625937}{0.435351614900}
  \meshline{144,144,144}{0.639474986339}{0.424691265962}{0.652429806573}{0.403871173475}
  \meshline{144,144,144}{0.576448092717}{0.472143114293}{0.567791229661}{0.475602030256}
  \meshline{144,144,144}{0.541656913769}{0.482421166241}{0.561538200077}{0.477490560051}
  \meshline{144,144,144}{0.530431294195}{0.398501981499}{0.534203189010}{0.396715329009}
  \meshline{144,144,144}{0.541378074336}{0.482480085515}{0.541099403121}{0.482520389644}
  \meshline{144,144,144}{0.489488826614}{0.484124185274}{0.499442446327}{0.484898877195}
  \meshline{144,144,144}{0.477427122239}{0.550737006641}{0.462019016635}{0.548916275590}
  \meshline{144,144,144}{0.489488826614}{0.484124185274}{0.480508366447}{0.482968359608}
  \meshline{144,144,144}{0.519836818203}{0.484875033280}{0.541099403121}{0.482520389644}
  \meshline{144,144,144}{0.519836818203}{0.484875033280}{0.516947157525}{0.484966316164}
  \meshline{144,144,144}{0.578129710927}{0.545180382591}{0.566597667970}{0.547453841766}
  \meshline{144,144,144}{0.507591636136}{0.552317099776}{0.513072711424}{0.552429275595}
  \meshline{144,144,144}{0.477427122239}{0.550737006641}{0.480361699089}{0.551098815646}
  \meshline{144,144,144}{0.541378074336}{0.482480085515}{0.541656913769}{0.482421166241}
  \meshline{144,144,144}{0.588662079085}{0.619417025838}{0.602674131470}{0.617507940277}
  \meshline{144,144,144}{0.623059516422}{0.671545613204}{0.636204645621}{0.670698543310}
  \meshline{144,144,144}{0.491073688190}{0.623044799832}{0.497866352990}{0.623297865268}
  \meshline{144,144,144}{0.549649425673}{0.622664335949}{0.561522506303}{0.621997501238}
  \meshline{144,144,144}{0.617194219105}{0.615296395975}{0.603221254947}{0.617415552257}
  \meshline{144,144,144}{0.561522506303}{0.621997501238}{0.571922423815}{0.621021185195}
  \meshline{144,144,144}{0.588662079085}{0.619417025838}{0.582095767480}{0.620124661370}
  \meshline{144,144,144}{0.599234727628}{0.672498034892}{0.614303314687}{0.671717509362}
  \meshline{144,144,144}{0.586247982921}{0.672788889006}{0.599234727628}{0.672498034892}
  \meshline{144,144,144}{0.535167023474}{0.551347964096}{0.532022154181}{0.551656337796}
  \meshline{144,144,144}{0.535167023474}{0.551347964096}{0.549598708074}{0.549985656123}
  \meshline{144,144,144}{0.566597667970}{0.547453841766}{0.554945457951}{0.549301562750}
  \meshline{144,144,144}{0.494978232547}{0.552080657297}{0.507591636136}{0.552317099776}
  \meshline{144,144,144}{0.551422826648}{0.549835751348}{0.549598708074}{0.549985656123}
  \meshline{144,144,144}{0.532022154181}{0.551656337796}{0.530578484918}{0.551706684440}
  \meshline{144,144,144}{0.494978232547}{0.552080657297}{0.484838051450}{0.551383189885}
  \meshline{144,144,144}{0.543323370059}{0.622866070804}{0.546432669887}{0.622811007719}
  \meshline{144,144,144}{0.497866352990}{0.623297865268}{0.512021039334}{0.623521931015}
  \meshline{144,144,144}{0.549649425673}{0.622664335949}{0.546432669887}{0.622811007719}
  \meshline{144,144,144}{0.481257611695}{0.622668895455}{0.491073688190}{0.623044799832}
  \meshline{144,144,144}{0.460290858834}{0.621348968032}{0.466610343083}{0.621787960801}
  \meshline{144,144,144}{0.453399278858}{0.620591298313}{0.460290858834}{0.621348968032}
  \meshline{144,144,144}{0.466610343083}{0.621787960801}{0.481257611695}{0.622668895455}
  \meshline{144,144,144}{0.453399278858}{0.620591298313}{0.437162030307}{0.619020267495}
  \meshline{144,144,144}{0.552652351080}{0.673486728925}{0.564701143220}{0.673276440178}
  \meshline{144,144,144}{0.543323370059}{0.622866070804}{0.513842858039}{0.623528109288}
  \meshline{144,144,144}{0.618976991617}{0.671641546993}{0.614303314687}{0.671717509362}
  \meshline{144,144,144}{0.513842858039}{0.623528109288}{0.512021039334}{0.623521931015}
  \meshline{144,144,144}{0.528486108408}{0.673474857351}{0.531524462756}{0.673456323498}
  \meshline{144,144,144}{0.476955506641}{0.672488266903}{0.479260531771}{0.672562615444}
  \meshline{144,144,144}{0.474137698710}{0.672370782831}{0.476955506641}{0.672488266903}
  \meshline{144,144,144}{0.479260531771}{0.672562615444}{0.495838834965}{0.673040668016}
  \meshline{144,144,144}{0.363457289616}{0.605163223140}{0.355765091145}{0.602899617514}
  \meshline{144,144,144}{0.527164646276}{0.673472740175}{0.528486108408}{0.673474857351}
  \meshline{144,144,144}{0.513016434513}{0.673370760877}{0.499058223578}{0.673097454432}
  \meshline{144,144,144}{0.445316108093}{0.671200657250}{0.442559132993}{0.671111170539}
  \meshline{144,144,144}{0.396630072029}{0.612773055362}{0.409610233915}{0.615095610376}
  \meshline{144,144,144}{0.403521503420}{0.534065515132}{0.394759725061}{0.530744350170}
  \meshline{144,144,144}{0.427292451379}{0.617559094083}{0.437162030307}{0.619020267495}
  \meshline{144,144,144}{0.388511586769}{0.527906352302}{0.394759725061}{0.530744350170}
  \meshline{144,144,144}{0.386971230083}{0.610646427724}{0.378930968854}{0.609146279466}
  \meshline{144,144,144}{0.443452468412}{0.545492774382}{0.443892591994}{0.545601348989}
  \meshline{144,144,144}{0.444320578436}{0.545676228643}{0.457145040196}{0.548009485793}
  \meshline{144,144,144}{0.427402497850}{0.541702462654}{0.443452468412}{0.545492774382}
  \meshline{144,144,144}{0.453190484121}{0.476640780140}{0.462927412072}{0.479378724987}
  \meshline{144,144,144}{0.480508366447}{0.482968359608}{0.470489144564}{0.481278286592}
  \meshline{144,144,144}{0.462927412072}{0.479378724987}{0.470489144564}{0.481278286592}
  \meshline{144,144,144}{0.440613933445}{0.472144918232}{0.441002469001}{0.472315584925}
  \meshline{144,144,144}{0.444015745767}{0.545625329545}{0.444320578436}{0.545676228643}
  \meshline{144,144,144}{0.411178639786}{0.536849175447}{0.419106102437}{0.539121117556}
  \meshline{144,144,144}{0.419106102437}{0.539121117556}{0.427402497850}{0.541702462654}
  \meshline{144,144,144}{0.388511586769}{0.527906352302}{0.380575113251}{0.524586637758}
  \meshline{144,144,144}{0.457145040196}{0.548009485793}{0.462019016635}{0.548916275590}
  \meshline{144,144,144}{0.403521503420}{0.534065515132}{0.411178639786}{0.536849175447}
  \meshline{144,144,144}{0.380575113251}{0.524586637758}{0.374518538775}{0.521475466618}
  \meshline{144,144,144}{0.444015745767}{0.545625329545}{0.443892591994}{0.545601348989}
  \meshline{144,144,144}{0.453190484121}{0.476640780140}{0.441002469001}{0.472315584925}
  \meshline{144,144,144}{0.323833992204}{0.593053589134}{0.315464477971}{0.589753535901}
  \meshline{144,144,144}{0.480361699089}{0.551098815646}{0.484838051450}{0.551383189885}
  \meshline{144,144,144}{0.410049144851}{0.455978783941}{0.405504830819}{0.452414832547}
  \meshline{144,144,144}{0.423125345623}{0.463605465380}{0.419805392835}{0.461970105173}
  \meshline{144,144,144}{0.323833992204}{0.593053589134}{0.338209249962}{0.597947913333}
  \meshline{144,144,144}{0.386971230083}{0.610646427724}{0.396630072029}{0.612773055362}
  \meshline{144,144,144}{0.368370867833}{0.606554437366}{0.363457289616}{0.605163223140}
  \meshline{144,144,144}{0.090770035037}{0.539506979235}{0.090382563348}{0.538492263794}
  \meshline{144,144,144}{0.351362600283}{0.508050069325}{0.364059491826}{0.516131096247}
  \meshline{144,144,144}{0.324576939073}{0.486830640999}{0.317849766780}{0.480910784861}
  \meshline{144,144,144}{0.276776720258}{0.418601273588}{0.278534654941}{0.422133640751}
  \meshline{144,144,144}{0.350986167996}{0.507815683360}{0.349771649198}{0.506904481711}
  \meshline{144,144,144}{0.324576939073}{0.486830640999}{0.337145658376}{0.497833339584}
  \meshline{144,144,144}{0.364059491826}{0.516131096247}{0.374518538775}{0.521475466618}
  \meshline{144,144,144}{0.349771649198}{0.506904481711}{0.337145658376}{0.497833339584}
  \meshline{144,144,144}{0.351362600283}{0.508050069325}{0.350986167996}{0.507815683360}
  \meshline{144,144,144}{0.354643707348}{0.379340338216}{0.354640252557}{0.379325671157}
  \meshline{144,144,144}{0.275508129014}{0.414992903998}{0.268754595445}{0.393314018584}
  \meshline{144,144,144}{0.396758464001}{0.444734962004}{0.385994143139}{0.435672119374}
  \meshline{144,144,144}{0.315746941763}{0.478725881072}{0.313500894972}{0.476031998061}
  \meshline{144,144,144}{0.385994143139}{0.435672119374}{0.380425014686}{0.428632802431}
  \meshline{144,144,144}{0.296951314769}{0.455668707126}{0.292623968726}{0.449082896201}
  \meshline{144,144,144}{0.380425014686}{0.428632802431}{0.373875015272}{0.420452814980}
  \meshline{144,144,144}{0.440613933445}{0.472144918232}{0.439497441585}{0.471601980298}
  \meshline{144,144,144}{0.306110387739}{0.467596027073}{0.313500894972}{0.476031998061}
  \meshline{144,144,144}{0.286951929644}{0.439866801496}{0.292623968726}{0.449082896201}
  \meshline{144,144,144}{0.315746941763}{0.478725881072}{0.317849766780}{0.480910784861}
  \meshline{144,144,144}{0.354643707348}{0.379340338216}{0.354648380475}{0.379352028011}
  \meshline{144,144,144}{0.354648380475}{0.379352028011}{0.361900585659}{0.399598507965}
  \meshline{144,144,144}{0.396758464001}{0.444734962004}{0.405504830819}{0.452414832547}
  \meshline{144,144,144}{0.415706291248}{0.459606274547}{0.419805392835}{0.461970105173}
  \meshline{144,144,144}{0.410049144851}{0.455978783941}{0.415706291248}{0.459606274547}
  \meshline{144,144,144}{0.315169778118}{0.801809338443}{0.327192237546}{0.798477544750}
  \meshline{144,144,144}{0.355765091145}{0.602899617514}{0.344800052601}{0.599932035737}
  \meshline{144,144,144}{0.344800052601}{0.599932035737}{0.338209249962}{0.597947913333}
  \meshline{144,144,144}{0.330810524592}{0.661560586085}{0.338202094888}{0.662436116276}
  \meshline{144,144,144}{0.287832509466}{0.577489256291}{0.296670373374}{0.581529531399}
  \meshline{144,144,144}{0.315403417498}{0.589726168379}{0.301280447034}{0.583832414079}
  \meshline{144,144,144}{0.478465919648}{0.395682052928}{0.478032959987}{0.395512172617}
  \meshline{144,144,144}{0.368541598487}{0.412245243160}{0.367058730384}{0.409379397960}
  \meshline{144,144,144}{0.172448257719}{0.455073068150}{0.173711421104}{0.457921974599}
  \meshline{144,144,144}{0.315403417498}{0.589726168379}{0.315464477971}{0.589753535901}
  \meshline{144,144,144}{0.301280447034}{0.583832414079}{0.296670373374}{0.581529531399}
  \meshline{144,144,144}{0.368541598487}{0.412245243160}{0.369202183471}{0.413238649787}
  \meshline{144,144,144}{0.454588690179}{0.369659962357}{0.450281984126}{0.355650025873}
  \meshline{144,144,144}{0.305826060244}{0.467204026389}{0.306110387739}{0.467596027073}
  \meshline{144,144,144}{0.305826060244}{0.467204026389}{0.296951314769}{0.455668707126}
  \meshline{144,144,144}{0.265151931763}{0.564370434290}{0.283052059366}{0.575032238206}
  \meshline{144,144,144}{0.260414020034}{0.561716935508}{0.265151931763}{0.564370434290}
  \meshline{144,144,144}{0.247209638611}{0.552576543129}{0.256667417066}{0.559283832236}
  \meshline{144,144,144}{0.256667417066}{0.559283832236}{0.260414020034}{0.561716935508}
  \meshline{144,144,144}{0.236126576411}{0.543546308911}{0.238230562199}{0.545293447952}
  \meshline{144,144,144}{0.247209638611}{0.552576543129}{0.238230562199}{0.545293447952}
  \meshline{144,144,144}{0.231852448706}{0.539643073191}{0.224510514534}{0.533273039286}
  \meshline{144,144,144}{0.231852448706}{0.539643073191}{0.236126576411}{0.543546308911}
  \meshline{144,144,144}{0.222231467006}{0.531080031383}{0.217643309665}{0.525919550344}
  \meshline{144,144,144}{0.208758529853}{0.516497827859}{0.217643309665}{0.525919550344}
  \meshline{144,144,144}{0.155496296172}{0.308402490680}{0.154309484498}{0.320588653171}
  \meshline{144,144,144}{0.181092972639}{0.474163789919}{0.180124811195}{0.472447581330}
  \meshline{144,144,144}{0.275508129014}{0.414992903998}{0.276158962723}{0.417082240678}
  \meshline{144,144,144}{0.276158962723}{0.417082240678}{0.276776720258}{0.418601273588}
  \meshline{144,144,144}{0.268754595445}{0.393314018584}{0.268217909916}{0.390562166219}
  \meshline{144,144,144}{0.286951929644}{0.439866801496}{0.278534654941}{0.422133640751}
  \meshline{144,144,144}{0.168077375954}{0.254213895048}{0.165738131836}{0.261466046380}
  \meshline{144,144,144}{0.163182720925}{0.269997977431}{0.160382799237}{0.281596150765}
  \meshline{144,144,144}{0.160136814705}{0.415736151124}{0.156691431019}{0.396744539640}
  \meshline{144,144,144}{0.160948514657}{0.418768906275}{0.164410424369}{0.430879513995}
  \meshline{144,144,144}{0.272637789471}{0.291703668015}{0.271445911666}{0.295906659466}
  \meshline{144,144,144}{0.280258049195}{0.272126583911}{0.278540202525}{0.276279134348}
  \meshline{144,144,144}{0.267017233835}{0.312312028615}{0.271445911666}{0.295906659466}
  \meshline{144,144,144}{0.265732191609}{0.320821670812}{0.267017233835}{0.312312028615}
  \meshline{144,144,144}{0.263466184545}{0.351067336374}{0.264002532221}{0.365163239511}
  \meshline{144,144,144}{0.264820258885}{0.327062434982}{0.265732191609}{0.320821670812}
  \meshline{144,144,144}{0.278540202525}{0.276279134348}{0.272637789471}{0.291703668015}
  \meshline{144,144,144}{0.264344617251}{0.335212164101}{0.263418165417}{0.346084488789}
  \meshline{144,144,144}{0.153426054120}{0.367821189544}{0.153089440372}{0.362718970936}
  \meshline{144,144,144}{0.160382799237}{0.281596150765}{0.159898774125}{0.283756383307}
  \meshline{144,144,144}{0.152771059591}{0.349442125399}{0.152722656459}{0.343967187984}
  \meshline{144,144,144}{0.156691431019}{0.396744539640}{0.155297520116}{0.387194200248}
  \meshline{144,144,144}{0.160136814705}{0.415736151124}{0.160948514657}{0.418768906275}
  \meshline{144,144,144}{0.156432693055}{0.302892451531}{0.155496296172}{0.308402490680}
  \meshline{144,144,144}{0.152771059591}{0.349442125399}{0.153089440372}{0.362718970936}
  \meshline{144,144,144}{0.154309484498}{0.320588653171}{0.153638970119}{0.326566989610}
  \meshline{144,144,144}{0.154204053950}{0.378576957647}{0.153426054120}{0.367821189544}
  \meshline{144,144,144}{0.154204053950}{0.378576957647}{0.155297520116}{0.387194200248}
  \meshline{144,144,144}{0.163182720925}{0.269997977431}{0.165738131836}{0.261466046380}
  \meshline{144,144,144}{0.159077070968}{0.288609593833}{0.159898774125}{0.283756383307}
  \meshline{144,144,144}{0.181092972639}{0.474163789919}{0.189119381494}{0.489355790933}
  \meshline{144,144,144}{0.264002532221}{0.365163239511}{0.264845994342}{0.371221923607}
  \meshline{144,144,144}{0.264845994342}{0.371221923607}{0.265637849841}{0.378104050667}
  \meshline{144,144,144}{0.166248921879}{0.437967123457}{0.164410424369}{0.430879513995}
  \meshline{144,144,144}{0.156432693055}{0.302892451531}{0.159077070968}{0.288609593833}
  \meshline{144,144,144}{0.264344617251}{0.335212164101}{0.264820258885}{0.327062434982}
  \meshline{144,144,144}{0.263466184545}{0.351067336374}{0.263418165417}{0.346084488789}
  \meshline{144,144,144}{0.265637849841}{0.378104050667}{0.268217909916}{0.390562166219}
  \meshline{144,144,144}{0.099844423231}{0.140957115899}{0.098431908373}{0.142968839953}
  \meshline{144,144,144}{0.088970887173}{0.161426590938}{0.087555922153}{0.164954258816}
  \meshline{144,144,144}{0.099844423231}{0.140957115899}{0.111016994332}{0.124019644551}
  \meshline{144,144,144}{0.117010514402}{0.117358096063}{0.111016994332}{0.124019644551}
  \meshline{144,144,144}{0.088970887173}{0.161426590938}{0.089712011701}{0.160062706404}
  \meshline{144,144,144}{0.064050798366}{0.253632145859}{0.062931992019}{0.260800025535}
  \meshline{144,144,144}{0.087555922153}{0.164954258816}{0.081896258736}{0.178188369215}
  \meshline{144,144,144}{0.089712011701}{0.160062706404}{0.098431908373}{0.142968839953}
  \meshline{144,144,144}{0.066962749794}{0.236777238027}{0.064050798366}{0.253632145859}
  \meshline{144,144,144}{0.072164807553}{0.210710985646}{0.068267322436}{0.228045891868}
  \meshline{144,144,144}{0.081896258736}{0.178188369215}{0.080140294573}{0.184138428899}
  \meshline{144,144,144}{0.080140294573}{0.184138428899}{0.075747814770}{0.196540851457}
  \meshline{144,144,144}{0.072164807553}{0.210710985646}{0.072603673214}{0.208793036429}
  \meshline{144,144,144}{0.072603673214}{0.208793036429}{0.075747814770}{0.196540851457}
  \meshline{144,144,144}{0.153570343742}{0.327915940990}{0.152722656459}{0.343967187984}
  \meshline{144,144,144}{0.153570343742}{0.327915940990}{0.153638970119}{0.326566989610}
  \meshline{144,144,144}{0.068267322436}{0.228045891868}{0.067773334653}{0.231286363841}
  \meshline{144,144,144}{0.061727282445}{0.272778986692}{0.060783729083}{0.280535803854}
  \meshline{144,144,144}{0.062931992019}{0.260800025535}{0.061727282445}{0.272778986692}
  \meshline{144,144,144}{0.059118548760}{0.301707419347}{0.059754726355}{0.293991762120}
  \meshline{144,144,144}{0.066962749794}{0.236777238027}{0.067773334653}{0.231286363841}
  \meshline{144,144,144}{0.058042715227}{0.326211268256}{0.058050570630}{0.325827473446}
  \meshline{144,144,144}{0.059118548760}{0.301707419347}{0.058105122054}{0.324704682454}
  \meshline{144,144,144}{0.058042715227}{0.326211268256}{0.058021503158}{0.328312139039}
  \meshline{144,144,144}{0.058050570630}{0.325827473446}{0.058105122054}{0.324704682454}
  \meshline{144,144,144}{0.058021503158}{0.328312139039}{0.057720151995}{0.349736140364}
  \meshline{144,144,144}{0.057775393114}{0.356276082164}{0.058042470097}{0.371781052101}
  \meshline{144,144,144}{0.057775393114}{0.356276082164}{0.057720151995}{0.349736140364}
  \meshline{144,144,144}{0.663422505510}{0.368473494814}{0.661457285641}{0.377445233671}
  \meshline{144,144,144}{0.654587565591}{0.398742169881}{0.659519729808}{0.385800076335}
  \meshline{144,144,144}{0.653290659684}{0.402176318233}{0.652429806573}{0.403871173475}
  \meshline{144,144,144}{0.657923395869}{0.738301672467}{0.645058588306}{0.736611148300}
  \meshline{144,144,144}{0.675727684782}{0.667566557042}{0.675574714702}{0.667590480804}
  \meshline{144,144,144}{0.674636367184}{0.667675222812}{0.653974730830}{0.669519716210}
  \meshline{144,144,144}{0.653974730830}{0.669519716210}{0.650622952328}{0.669604806236}
  \meshline{144,144,144}{0.668133685403}{0.739252903311}{0.663835051452}{0.738870687545}
  \meshline{144,144,144}{0.582886998999}{0.672969045210}{0.586247982921}{0.672788889006}
  \meshline{144,144,144}{0.618976991617}{0.671641546993}{0.623059516422}{0.671545613204}
  \meshline{144,144,144}{0.650622952328}{0.669604806236}{0.636204645621}{0.670698543310}
  \meshline{144,144,144}{0.635332670624}{0.735457375429}{0.623605781878}{0.734416334697}
  \meshline{144,144,144}{0.635332670624}{0.735457375429}{0.645058588306}{0.736611148300}
  \meshline{144,144,144}{0.566301903775}{0.730304636399}{0.577914287015}{0.730933906603}
  \meshline{144,144,144}{0.600831321673}{0.732600248682}{0.604662677140}{0.732988468820}
  \meshline{144,144,144}{0.623605781878}{0.734416334697}{0.604662677140}{0.732988468820}
  \meshline{144,144,144}{0.698004101177}{0.743567849388}{0.704217438236}{0.744760193303}
  \meshline{144,144,144}{0.663835051452}{0.738870687545}{0.657923395869}{0.738301672467}
  \meshline{144,144,144}{0.685160061627}{0.741651342268}{0.668133685403}{0.739252903311}
  \meshline{144,144,144}{0.764214626277}{0.757343739122}{0.767589000303}{0.758002113254}
  \meshline{144,144,144}{0.730100454245}{0.749100902088}{0.723309945099}{0.748104835193}
  \meshline{144,144,144}{0.578306958550}{0.673101927764}{0.564701143220}{0.673276440178}
  \meshline{144,144,144}{0.582886998999}{0.672969045210}{0.578306958550}{0.673101927764}
  \meshline{144,144,144}{0.459227319750}{0.727417837856}{0.444653237075}{0.727573209476}
  \meshline{144,144,144}{0.555284406901}{0.729638339966}{0.545815722285}{0.729261491952}
  \meshline{144,144,144}{0.531524462756}{0.673456323498}{0.544877994905}{0.673493584144}
  \meshline{144,144,144}{0.552652351080}{0.673486728925}{0.544877994905}{0.673493584144}
  \meshline{144,144,144}{0.499058223578}{0.673097454432}{0.495838834965}{0.673040668016}
  \meshline{144,144,144}{0.600831321673}{0.732600248682}{0.598802015789}{0.732415951772}
  \meshline{144,144,144}{0.527164646276}{0.673472740175}{0.513016434513}{0.673370760877}
  \meshline{144,144,144}{0.459227319750}{0.727417837856}{0.469921229130}{0.727396186526}
  \meshline{144,144,144}{0.512108635267}{0.728097397497}{0.511983661352}{0.728094821305}
  \meshline{144,144,144}{0.537185497074}{0.728872573579}{0.545815722285}{0.729261491952}
  \meshline{144,144,144}{0.848778129206}{0.621916386619}{0.829613284798}{0.632473744697}
  \meshline{144,144,144}{0.916249566371}{0.543560865844}{0.914333470737}{0.547955796455}
  \meshline{144,144,144}{0.905618565924}{0.564995681901}{0.914333470737}{0.547955796455}
  \meshline{144,144,144}{0.898548486258}{0.575950840240}{0.890365964698}{0.586930600036}
  \meshline{144,144,144}{0.905618565924}{0.564995681901}{0.900280939049}{0.573361010186}
  \meshline{144,144,144}{0.865574261368}{0.610476862058}{0.874584110873}{0.602890116762}
  \meshline{144,144,144}{0.848778129206}{0.621916386619}{0.849598516976}{0.621530126741}
  \meshline{144,144,144}{0.849598516976}{0.621530126741}{0.859719914489}{0.614602574577}
  \meshline{144,144,144}{0.859719914489}{0.614602574577}{0.865574261368}{0.610476862058}
  \meshline{144,144,144}{0.890365964698}{0.586930600036}{0.885955858578}{0.591464303146}
  \meshline{144,144,144}{0.874584110873}{0.602890116762}{0.885955858578}{0.591464303146}
  \meshline{144,144,144}{0.781776135354}{0.762122392717}{0.771610642318}{0.759020138222}
  \meshline{144,144,144}{0.800402504199}{0.768459140396}{0.810249396266}{0.772097677806}
  \meshline{144,144,144}{0.723309945099}{0.748104835193}{0.711247969364}{0.745654002086}
  \meshline{144,144,144}{0.816620723853}{0.774954061124}{0.810249396266}{0.772097677806}
  \meshline{144,144,144}{0.764214626277}{0.757343739122}{0.750212043927}{0.753514894998}
  \meshline{144,144,144}{0.743209003425}{0.752307284484}{0.750212043927}{0.753514894998}
  \meshline{144,144,144}{0.730100454245}{0.749100902088}{0.743209003425}{0.752307284484}
  \meshline{144,144,144}{0.767589000303}{0.758002113254}{0.771610642318}{0.759020138222}
  \meshline{144,144,144}{0.711247969364}{0.745654002086}{0.704217438236}{0.744760193303}
  \meshline{144,144,144}{0.833035689754}{0.783009418281}{0.837228626142}{0.784973767669}
  \meshline{144,144,144}{0.903428374673}{0.849573643493}{0.896961819618}{0.840175251915}
  \meshline{144,144,144}{0.857079925543}{0.798068766360}{0.873246592350}{0.810973619432}
  \meshline{144,144,144}{0.849164506799}{0.792530883473}{0.837228626142}{0.784973767669}
  \meshline{144,144,144}{0.800402504199}{0.768459140396}{0.792685853401}{0.766338867901}
  \meshline{144,144,144}{0.857079925543}{0.798068766360}{0.854319598680}{0.795731019762}
  \meshline{144,144,144}{0.882246400849}{0.821042875790}{0.887957887440}{0.827090021590}
  \meshline{144,144,144}{0.833035689754}{0.783009418281}{0.825437304624}{0.779627089654}
  \meshline{144,144,144}{0.849164506799}{0.792530883473}{0.854319598680}{0.795731019762}
  \meshline{144,144,144}{0.890881707068}{0.830398972633}{0.892903625999}{0.833487377450}
  \meshline{144,144,144}{0.882246400849}{0.821042875790}{0.873246592350}{0.810973619432}
  \meshline{144,144,144}{0.892903625999}{0.833487377450}{0.896961819618}{0.840175251915}
  \meshline{144,144,144}{0.918308205479}{0.881322492925}{0.920395021770}{0.887814646420}
  \meshline{144,144,144}{0.912694596677}{0.868044825096}{0.918308205479}{0.881322492925}
  \meshline{144,144,144}{0.920395021770}{0.887814646420}{0.922861329723}{0.896893127125}
  \meshline{144,144,144}{0.890881707068}{0.830398972633}{0.887957887440}{0.827090021590}
  \meshline{144,144,144}{0.792685853401}{0.766338867901}{0.781776135354}{0.762122392717}
  \meshline{144,144,144}{0.816620723853}{0.774954061124}{0.825437304624}{0.779627089654}
  \meshline{144,144,144}{0.935867254896}{0.954998124778}{0.934566903036}{0.947800119820}
  \meshline{144,144,144}{0.930199525040}{0.924470765452}{0.933407313035}{0.939698895537}
  \meshline{144,144,144}{0.903428374673}{0.849573643493}{0.907869328420}{0.857871415515}
  \meshline{144,144,144}{0.926527558412}{0.907706619533}{0.922861329723}{0.896893127125}
  \meshline{144,144,144}{0.929385434403}{0.920427527837}{0.926527558412}{0.907706619533}
  \meshline{144,144,144}{0.929949947365}{0.922872741179}{0.929385434403}{0.920427527837}
  \meshline{144,144,144}{0.929949947365}{0.922872741179}{0.930199525040}{0.924470765452}
  \meshline{144,144,144}{0.912694596677}{0.868044825096}{0.907869328420}{0.857871415515}
  \meshline{144,144,144}{0.807063473925}{0.905245033478}{0.802962921263}{0.898695170395}
  \meshline{144,144,144}{0.505260854991}{0.401388725049}{0.496790165260}{0.400581562836}
  \meshline{144,144,144}{0.478465919648}{0.395682052928}{0.479248006232}{0.395925317049}
  \meshline{144,144,144}{0.466028031682}{0.385733792671}{0.458258284870}{0.377752284976}
  \meshline{144,144,144}{0.478032959987}{0.395512172617}{0.477080837963}{0.394966305260}
  \meshline{144,144,144}{0.477080837963}{0.394966305260}{0.466028031682}{0.385733792671}
  \meshline{144,144,144}{0.479248006232}{0.395925317049}{0.496790165260}{0.400581562836}
  \meshline{144,144,144}{0.377057314321}{0.666434387485}{0.370122862291}{0.665998602355}
  \meshline{144,144,144}{0.378930968854}{0.609146279466}{0.368370867833}{0.606554437366}
  \meshline{144,144,144}{0.474137698710}{0.672370782831}{0.459704015599}{0.671896816098}
  \meshline{144,144,144}{0.427292451379}{0.617559094083}{0.417206217458}{0.616304999270}
  \meshline{144,144,144}{0.289573331757}{0.655160730972}{0.295751774657}{0.656529285790}
  \meshline{144,144,144}{0.417206217458}{0.616304999270}{0.409610233915}{0.615095610376}
  \meshline{144,144,144}{0.399770118511}{0.668503698947}{0.387324402400}{0.667553715119}
  \meshline{144,144,144}{0.407496612773}{0.668904420520}{0.425832750432}{0.670136387507}
  \meshline{144,144,144}{0.355514935615}{0.664350873530}{0.354712820005}{0.664296369902}
  \meshline{144,144,144}{0.399770118511}{0.668503698947}{0.407496612773}{0.668904420520}
  \meshline{144,144,144}{0.393077889751}{0.728589618311}{0.398309935451}{0.728532482909}
  \meshline{144,144,144}{0.377057314321}{0.666434387485}{0.387324402400}{0.667553715119}
  \meshline{144,144,144}{0.303327609500}{0.657785909440}{0.311901679196}{0.658827866699}
  \meshline{144,144,144}{0.370122862291}{0.665998602355}{0.355514935615}{0.664350873530}
  \meshline{144,144,144}{0.311901679196}{0.658827866699}{0.318572782079}{0.659643520915}
  \meshline{144,144,144}{0.289573331757}{0.655160730972}{0.275914087315}{0.653169579863}
  \meshline{144,144,144}{0.266267710069}{0.650764526088}{0.275914087315}{0.653169579863}
  \meshline{144,144,144}{0.295751774657}{0.656529285790}{0.303327609500}{0.657785909440}
  \meshline{144,144,144}{0.210262669261}{0.636282832175}{0.188005616730}{0.627816275988}
  \meshline{144,144,144}{0.225578651300}{0.641092528227}{0.219510276700}{0.639242222354}
  \meshline{144,144,144}{0.287832509466}{0.577489256291}{0.283052059366}{0.575032238206}
  \meshline{144,144,144}{0.188005616730}{0.627816275988}{0.187511442045}{0.627601215633}
  \meshline{144,144,144}{0.369492819929}{0.729776923550}{0.346389040013}{0.731550704702}
  \meshline{144,144,144}{0.338202094888}{0.662436116276}{0.354712820005}{0.664296369902}
  \meshline{144,144,144}{0.318572782079}{0.659643520915}{0.330810524592}{0.661560586085}
  \meshline{144,144,144}{0.425849240099}{0.670137111228}{0.425832750432}{0.670136387507}
  \meshline{144,144,144}{0.398309935451}{0.728532482909}{0.413170600829}{0.728140220009}
  \meshline{144,144,144}{0.425849240099}{0.670137111228}{0.442559132993}{0.671111170539}
  \meshline{144,144,144}{0.459704015599}{0.671896816098}{0.445316108093}{0.671200657250}
  \meshline{144,144,144}{0.435336785815}{0.727550403324}{0.422199515566}{0.727837911779}
  \meshline{144,144,144}{0.444653237075}{0.727573209476}{0.435336785815}{0.727550403324}
  \meshline{144,144,144}{0.305688101296}{0.735102879542}{0.311532817341}{0.734563700129}
  \meshline{144,144,144}{0.422199515566}{0.727837911779}{0.416641695374}{0.727982399901}
  \meshline{144,144,144}{0.416641695374}{0.727982399901}{0.413170600829}{0.728140220009}
  \meshline{144,144,144}{0.479431418914}{0.727467807131}{0.469921229130}{0.727396186526}
  \meshline{144,144,144}{0.479431418914}{0.727467807131}{0.488114574397}{0.727616519999}
  \meshline{144,144,144}{0.511983661352}{0.728094821305}{0.496652980885}{0.727727017096}
  \meshline{144,144,144}{0.528013488967}{0.728558570109}{0.537185497074}{0.728872573579}
  \meshline{144,144,144}{0.460785826386}{0.777495695435}{0.450953839518}{0.777799913579}
  \meshline{144,144,144}{0.496652980885}{0.727727017096}{0.488114574397}{0.727616519999}
  \meshline{144,144,144}{0.512108635267}{0.728097397497}{0.512255231075}{0.728102866518}
  \meshline{144,144,144}{0.528013488967}{0.728558570109}{0.512255231075}{0.728102866518}
  \meshline{144,144,144}{0.504479878450}{0.777307365104}{0.512466466583}{0.777483785889}
  \meshline{144,144,144}{0.477554983396}{0.777047416291}{0.473542286997}{0.777036304731}
  \meshline{144,144,144}{0.528660604369}{0.778351793455}{0.544312206636}{0.779661760131}
  \meshline{144,144,144}{0.471623687698}{0.777101957879}{0.460785826386}{0.777495695435}
  \meshline{144,144,144}{0.450953839518}{0.777799913579}{0.447838170046}{0.777984900224}
  \meshline{144,144,144}{0.477554983396}{0.777047416291}{0.491971982319}{0.776993562692}
  \meshline{144,144,144}{0.473542286997}{0.777036304731}{0.471623687698}{0.777101957879}
  \meshline{144,144,144}{0.436799270789}{0.778658793296}{0.447838170046}{0.777984900224}
  \meshline{144,144,144}{0.422431917884}{0.779939587362}{0.419163669891}{0.780333514887}
  \meshline{144,144,144}{0.350351586453}{0.791769872300}{0.353907990986}{0.791008362990}
  \meshline{144,144,144}{0.798405200791}{0.893018870602}{0.802962921263}{0.898695170395}
  \meshline{144,144,144}{0.680786007101}{0.808796851622}{0.695376616666}{0.815033137766}
  \meshline{144,144,144}{0.375012626226}{0.729658278591}{0.369492819929}{0.729776923550}
  \meshline{144,144,144}{0.328618255389}{0.732892661287}{0.334103805253}{0.732660233720}
  \meshline{144,144,144}{0.491971982319}{0.776993562692}{0.504479878450}{0.777307365104}
  \meshline{144,144,144}{0.812450539378}{0.913527023798}{0.807063473925}{0.905245033478}
  \meshline{144,144,144}{0.773230064921}{0.865291421061}{0.767281544877}{0.859428840940}
  \meshline{144,144,144}{0.375012626226}{0.729658278591}{0.393077889751}{0.728589618311}
  \meshline{144,144,144}{0.344745272260}{0.731592271482}{0.346389040013}{0.731550704702}
  \meshline{144,144,144}{0.344745272260}{0.731592271482}{0.334103805253}{0.732660233720}
  \meshline{144,144,144}{0.422431917884}{0.779939587362}{0.423469576151}{0.779822770564}
  \meshline{144,144,144}{0.419163669891}{0.780333514887}{0.407090603860}{0.781648949191}
  \meshline{144,144,144}{0.370998612451}{0.787304474311}{0.381241817358}{0.785371176523}
  \meshline{144,144,144}{0.370998612451}{0.787304474311}{0.358360179467}{0.790161713490}
  \meshline{144,144,144}{0.521351869855}{0.778021048880}{0.512466466583}{0.777483785889}
  \meshline{144,144,144}{0.547429120658}{0.779871320391}{0.551174699547}{0.780238337430}
  \meshline{144,144,144}{0.555284406901}{0.729638339966}{0.566301903775}{0.730304636399}
  \meshline{144,144,144}{0.590700532527}{0.785446476128}{0.577678616876}{0.783604784719}
  \meshline{144,144,144}{0.583479605434}{0.731387413400}{0.577914287015}{0.730933906603}
  \meshline{144,144,144}{0.544312206636}{0.779661760131}{0.547429120658}{0.779871320391}
  \meshline{144,144,144}{0.598802015789}{0.732415951772}{0.583479605434}{0.731387413400}
  \meshline{144,144,144}{0.528660604369}{0.778351793455}{0.521351869855}{0.778021048880}
  \meshline{144,144,144}{0.492627809751}{0.847634275292}{0.486491687354}{0.847771070721}
  \meshline{144,144,144}{0.492627809751}{0.847634275292}{0.494958042092}{0.847658304242}
  \meshline{144,144,144}{0.469114413977}{0.916086042487}{0.479602765138}{0.915090748192}
  \meshline{144,144,144}{0.451951245993}{0.849770122722}{0.454881088300}{0.849540489146}
  \meshline{144,144,144}{0.828820855706}{0.948085865997}{0.822633794247}{0.932892254198}
  \meshline{144,144,144}{0.381241817358}{0.785371176523}{0.387330113637}{0.784359349678}
  \meshline{144,144,144}{0.401070556074}{0.782349357636}{0.407090603860}{0.781648949191}
  \meshline{144,144,144}{0.401070556074}{0.782349357636}{0.387330113637}{0.784359349678}
  \meshline{144,144,144}{0.353907990986}{0.791008362990}{0.358360179467}{0.790161713490}
  \meshline{144,144,144}{0.338381830018}{0.794958187721}{0.327192237546}{0.798477544750}
  \meshline{144,144,144}{0.338381830018}{0.794958187721}{0.350351586453}{0.791769872300}
  \meshline{144,144,144}{0.194557031025}{0.497287126291}{0.198759854296}{0.503527221554}
  \meshline{144,144,144}{0.194557031025}{0.497287126291}{0.189119381494}{0.489355790933}
  \meshline{144,144,144}{0.205681955215}{0.512499887452}{0.198759854296}{0.503527221554}
  \meshline{144,144,144}{0.205681955215}{0.512499887452}{0.208758529853}{0.516497827859}
  \meshline{144,144,144}{0.167072464139}{0.440411436237}{0.166248921879}{0.437967123457}
  \meshline{144,144,144}{0.172448257719}{0.455073068150}{0.167072464139}{0.440411436237}
  \meshline{144,144,144}{0.173711421104}{0.457921974599}{0.180124811195}{0.472447581330}
  \meshline{144,144,144}{0.090770035037}{0.539506979235}{0.091476733047}{0.540789712292}
  \meshline{144,144,144}{0.118323974869}{0.580868269030}{0.121617419583}{0.584651441799}
  \meshline{144,144,144}{0.118323974869}{0.580868269030}{0.109302495519}{0.570956492746}
  \meshline{144,144,144}{0.099525527217}{0.555918650433}{0.102683928923}{0.560979924929}
  \meshline{144,144,144}{0.102683928923}{0.560979924929}{0.109302495519}{0.570956492746}
  \meshline{144,144,144}{0.091476733047}{0.540789712292}{0.099525527217}{0.555918650433}
  \meshline{144,144,144}{0.210262669261}{0.636282832175}{0.219510276700}{0.639242222354}
  \meshline{144,144,144}{0.121617419583}{0.584651441799}{0.130179209108}{0.593279132289}
  \meshline{144,144,144}{0.130179209108}{0.593279132289}{0.135820539099}{0.598163202569}
  \meshline{144,144,144}{0.224510514534}{0.533273039286}{0.222231467006}{0.531080031383}
  \meshline{144,144,144}{0.090382563348}{0.538492263794}{0.083463570446}{0.523399213489}
  \meshline{144,144,144}{0.082683081958}{0.521148874542}{0.081764979837}{0.517892603981}
  \meshline{144,144,144}{0.149498010160}{0.607353193504}{0.154311092373}{0.610699939669}
  \meshline{144,144,144}{0.187147274902}{0.627404040291}{0.169505141034}{0.619439569817}
  \meshline{144,144,144}{0.252127475251}{0.647571299984}{0.243402409514}{0.646000741020}
  \meshline{144,144,144}{0.252127475251}{0.647571299984}{0.266267710069}{0.650764526088}
  \meshline{144,144,144}{0.228666091614}{0.641776863465}{0.243402409514}{0.646000741020}
  \meshline{144,144,144}{0.225578651300}{0.641092528227}{0.228666091614}{0.641776863465}
  \meshline{144,144,144}{0.058878318297}{0.391854147694}{0.058281566084}{0.379106367819}
  \meshline{144,144,144}{0.058042470097}{0.371781052101}{0.058281566084}{0.379106367819}
  \meshline{144,144,144}{0.059991201094}{0.408862365749}{0.061078081943}{0.419834686486}
  \meshline{144,144,144}{0.059991201094}{0.408862365749}{0.059072958782}{0.394095542041}
  \meshline{144,144,144}{0.058878318297}{0.391854147694}{0.059072958782}{0.394095542041}
  \meshline{144,144,144}{0.073912106081}{0.492847455998}{0.074919745849}{0.497340946131}
  \meshline{144,144,144}{0.062282923628}{0.430999718619}{0.061078081943}{0.419834686486}
  \meshline{144,144,144}{0.062282923628}{0.430999718619}{0.063260301163}{0.438414583059}
  \meshline{144,144,144}{0.066266816510}{0.457341251610}{0.066742466834}{0.460809929708}
  \meshline{144,144,144}{0.074919745849}{0.497340946131}{0.081764979837}{0.517892603981}
  \meshline{144,144,144}{0.083463570446}{0.523399213489}{0.082683081958}{0.521148874542}
  \meshline{144,144,144}{0.063260301163}{0.438414583059}{0.066266816510}{0.457341251610}
  \meshline{144,144,144}{0.066742466834}{0.460809929708}{0.067190686717}{0.463297984007}
  \meshline{144,144,144}{0.067190686717}{0.463297984007}{0.070493889833}{0.479687582996}
  \meshline{144,144,144}{0.073912106081}{0.492847455998}{0.070493889833}{0.479687582996}
  \meshline{144,144,144}{0.650155342254}{0.798722480977}{0.641021598479}{0.796374683118}
  \meshline{144,144,144}{0.698004101177}{0.743567849388}{0.692163480530}{0.742567564371}
  \meshline{144,144,144}{0.605167664250}{0.788088462778}{0.622390425638}{0.791715797143}
  \meshline{144,144,144}{0.564274589787}{0.781678496104}{0.551174699547}{0.780238337430}
  \meshline{144,144,144}{0.666888836165}{0.804095730639}{0.662035929380}{0.802438931434}
  \meshline{144,144,144}{0.623203242153}{0.791903031608}{0.637718411504}{0.795365616970}
  \meshline{144,144,144}{0.592788619434}{0.785806362797}{0.590700532527}{0.785446476128}
  \meshline{144,144,144}{0.650155342254}{0.798722480977}{0.662035929380}{0.802438931434}
  \meshline{144,144,144}{0.577678616876}{0.783604784719}{0.564274589787}{0.781678496104}
  \meshline{144,144,144}{0.586735644264}{0.862536202642}{0.587364354643}{0.862705623316}
  \meshline{144,144,144}{0.605167664250}{0.788088462778}{0.596654703475}{0.786589485639}
  \meshline{144,144,144}{0.623203242153}{0.791903031608}{0.622390425638}{0.791715797143}
  \meshline{144,144,144}{0.637718411504}{0.795365616970}{0.641021598479}{0.796374683118}
  \meshline{144,144,144}{0.635282384317}{0.883785677224}{0.641099853317}{0.886997047566}
  \meshline{144,144,144}{0.615955161636}{0.874022690585}{0.621833741085}{0.876628281097}
  \meshline{144,144,144}{0.605414688357}{0.869197930046}{0.589074011095}{0.863322363662}
  \meshline{144,144,144}{0.587773246613}{0.862836967929}{0.589074011095}{0.863322363662}
  \meshline{144,144,144}{0.596654703475}{0.786589485639}{0.592788619434}{0.785806362797}
  \meshline{144,144,144}{0.514349679442}{0.848482678092}{0.494958042092}{0.847658304242}
  \meshline{144,144,144}{0.518116501441}{0.848735244121}{0.524077754697}{0.849460035268}
  \meshline{144,144,144}{0.537727902699}{0.851076276875}{0.524077754697}{0.849460035268}
  \meshline{144,144,144}{0.551878993886}{0.853477509393}{0.561514482808}{0.855667644827}
  \meshline{144,144,144}{0.587364354643}{0.862705623316}{0.587773246613}{0.862836967929}
  \meshline{144,144,144}{0.561514482808}{0.855667644827}{0.569443081595}{0.857411900042}
  \meshline{144,144,144}{0.615955161636}{0.874022690585}{0.605414688357}{0.869197930046}
  \meshline{144,144,144}{0.569443081595}{0.857411900042}{0.586735644264}{0.862536202642}
  \meshline{144,144,144}{0.724758008709}{1.116192932779}{0.720331420548}{1.126178623521}
  \meshline{144,144,144}{0.538051608820}{0.920814987696}{0.551007047618}{0.924466583528}
  \meshline{144,144,144}{0.635282384317}{0.883785677224}{0.621833741085}{0.876628281097}
  \meshline{144,144,144}{0.700534201617}{0.817683717633}{0.724275545303}{0.829211887796}
  \meshline{144,144,144}{0.747414725864}{0.844019124474}{0.743331115566}{0.840910333649}
  \meshline{144,144,144}{0.697891231310}{0.816244574999}{0.695376616666}{0.815033137766}
  \meshline{144,144,144}{0.754399904155}{0.848763171596}{0.762582989538}{0.855564166742}
  \meshline{144,144,144}{0.724275545303}{0.829211887796}{0.729594643126}{0.832581197869}
  \meshline{144,144,144}{0.729594643126}{0.832581197869}{0.743331115566}{0.840910333649}
  \meshline{144,144,144}{0.781817016180}{0.873094716152}{0.788699203690}{0.880747763865}
  \meshline{144,144,144}{0.754399904155}{0.848763171596}{0.747414725864}{0.844019124474}
  \meshline{144,144,144}{0.798405200791}{0.893018870602}{0.788699203690}{0.880747763865}
  \meshline{144,144,144}{0.700534201617}{0.817683717633}{0.697891231310}{0.816244574999}
  \meshline{144,144,144}{0.818559535929}{0.924893371835}{0.812450539378}{0.913527023798}
  \meshline{144,144,144}{0.328618255389}{0.732892661287}{0.314667378930}{0.734457544511}
  \meshline{144,144,144}{0.283863777013}{0.738289844442}{0.281763226255}{0.738499971838}
  \meshline{144,144,144}{0.234237198048}{0.747720422196}{0.238601837218}{0.746425683755}
  \meshline{144,144,144}{0.221541964721}{0.750375651241}{0.234237198048}{0.747720422196}
  \meshline{144,144,144}{0.221541964721}{0.750375651241}{0.212578686304}{0.753395928963}
  \meshline{144,144,144}{0.191802184676}{0.760194951107}{0.182819376804}{0.762984711799}
  \meshline{144,144,144}{0.818559535929}{0.924893371835}{0.822633794247}{0.932892254198}
  \meshline{144,144,144}{0.934566903036}{0.947800119820}{0.933407313035}{0.939698895537}
  \meshline{144,144,144}{0.935867254896}{0.954998124778}{0.937391127120}{0.966325839139}
  \meshline{144,144,144}{0.938684377681}{0.977693740558}{0.939293416974}{0.983512064248}
  \meshline{144,144,144}{0.937391127120}{0.966325839139}{0.938684377681}{0.977693740558}
  \meshline{144,144,144}{0.940875027443}{1.002702160915}{0.939606157683}{0.988474756691}
  \meshline{144,144,144}{0.941553286818}{1.016829133157}{0.940875027443}{1.002702160915}
  \meshline{144,144,144}{0.839287058657}{0.981760666966}{0.841183841117}{0.991434413578}
  \meshline{144,144,144}{0.841969600900}{0.995002872655}{0.841183841117}{0.991434413578}
  \meshline{144,144,144}{0.835358866499}{0.967249426263}{0.831010519478}{0.954268446254}
  \meshline{144,144,144}{0.831010519478}{0.954268446254}{0.828820855706}{0.948085865997}
  \meshline{144,144,144}{0.838234831592}{0.977771751379}{0.835358866499}{0.967249426263}
  \meshline{144,144,144}{0.942259777699}{1.059085283298}{0.941962420445}{1.076229971550}
  \meshline{144,144,144}{0.941976759976}{1.027980310270}{0.941828145377}{1.021486819457}
  \meshline{144,144,144}{0.842521546885}{0.998031536909}{0.845108987843}{1.015023424129}
  \meshline{144,144,144}{0.837289755507}{1.128110607290}{0.841521897284}{1.109999803376}
  \meshline{144,144,144}{0.941976759976}{1.027980310270}{0.942321565568}{1.040016989224}
  \meshline{144,144,144}{0.941828145377}{1.021486819457}{0.941553286818}{1.016829133157}
  \meshline{144,144,144}{0.942262754875}{1.053884070695}{0.942259777699}{1.059085283298}
  \meshline{144,144,144}{0.930556011688}{1.177233383321}{0.930643471235}{1.176890057897}
  \meshline{144,144,144}{0.826233833983}{1.160768283532}{0.824237875935}{1.165360592873}
  \meshline{144,144,144}{0.930556011688}{1.177233383321}{0.930394534653}{1.177846675157}
  \meshline{144,144,144}{0.826233833983}{1.160768283532}{0.830833376450}{1.149009540268}
  \meshline{144,144,144}{0.847169679341}{1.059233288400}{0.846685748462}{1.066943672209}
  \meshline{144,144,144}{0.844245456669}{1.093658565814}{0.844359149717}{1.092511013658}
  \meshline{144,144,144}{0.842521546885}{0.998031536909}{0.841969600900}{0.995002872655}
  \meshline{144,144,144}{0.845864638619}{1.022814973668}{0.847065553482}{1.037118398462}
  \meshline{144,144,144}{0.940881005541}{1.099032109495}{0.939603841565}{1.113429190654}
  \meshline{144,144,144}{0.941962420445}{1.076229971550}{0.941663272957}{1.081987496173}
  \meshline{144,144,144}{0.942321565568}{1.040016989224}{0.942262754875}{1.053884070695}
  \meshline{144,144,144}{0.839287058657}{0.981760666966}{0.838234831592}{0.977771751379}
  \meshline{144,144,144}{0.830833376450}{1.149009540268}{0.833945809033}{1.139423662083}
  \meshline{144,144,144}{0.937322238412}{1.137300780226}{0.936126878408}{1.146285436446}
  \meshline{144,144,144}{0.845864638619}{1.022814973668}{0.845108987843}{1.015023424129}
  \meshline{144,144,144}{0.941663272957}{1.081987496173}{0.940881005541}{1.099032109495}
  \meshline{144,144,144}{0.939209088832}{1.119249696460}{0.938864245471}{1.123086392387}
  \meshline{144,144,144}{0.939209088832}{1.119249696460}{0.939603841565}{1.113429190654}
  \meshline{144,144,144}{0.930785351467}{1.176121697902}{0.935123377243}{1.152811762789}
  \meshline{144,144,144}{0.930643471235}{1.176890057897}{0.930785351467}{1.176121697902}
  \meshline{144,144,144}{0.935123377243}{1.152811762789}{0.936126878408}{1.146285436446}
  \meshline{144,144,144}{0.927011001320}{1.193867521904}{0.930394534653}{1.177846675157}
  \meshline{144,144,144}{0.937322238412}{1.137300780226}{0.938864245471}{1.123086392387}
  \meshline{144,144,144}{0.927011001320}{1.193867521904}{0.924009469105}{1.203507977790}
  \meshline{144,144,144}{0.815700317440}{1.182488840086}{0.813972678064}{1.185841663184}
  \meshline{144,144,144}{0.812099272126}{1.188741083632}{0.805038685893}{1.200332961497}
  \meshline{144,144,144}{0.797591052042}{1.210458250070}{0.796534684555}{1.211813441675}
  \meshline{144,144,144}{0.841825291942}{1.108544770746}{0.843505942960}{1.098135199638}
  \meshline{144,144,144}{0.812099272126}{1.188741083632}{0.813972678064}{1.185841663184}
  \meshline{144,144,144}{0.815700317440}{1.182488840086}{0.824237875935}{1.165360592873}
  \meshline{144,144,144}{0.847123940644}{1.050329442783}{0.847169679341}{1.059233288400}
  \meshline{144,144,144}{0.835858680725}{1.133845035710}{0.833945809033}{1.139423662083}
  \meshline{144,144,144}{0.844245456669}{1.093658565814}{0.844181528911}{1.094138907839}
  \meshline{144,144,144}{0.846685748462}{1.066943672209}{0.846204958056}{1.077077112913}
  \meshline{144,144,144}{0.847123940644}{1.050329442783}{0.847065553482}{1.037118398462}
  \meshline{144,144,144}{0.728921207027}{0.997495570906}{0.730609810293}{1.004109772418}
  \meshline{144,144,144}{0.736578010496}{1.045527097682}{0.736573192117}{1.045380191983}
  \meshline{144,144,144}{0.719660361998}{0.973165647948}{0.722588615128}{0.979479799199}
  \meshline{144,144,144}{0.736578010496}{1.045527097682}{0.736565774108}{1.045762904281}
  \meshline{144,144,144}{0.917297441257}{1.224393452288}{0.920626292447}{1.214535635236}
  \meshline{144,144,144}{0.924009469105}{1.203507977790}{0.920626292447}{1.214535635236}
  \meshline{144,144,144}{0.913582449254}{1.232061884046}{0.917297441257}{1.224393452288}
  \meshline{144,144,144}{0.913582449254}{1.232061884046}{0.908111773931}{1.245342866372}
  \meshline{144,144,144}{0.805038685893}{1.200332961497}{0.797591052042}{1.210458250070}
  \meshline{144,144,144}{0.782401334324}{1.228510618039}{0.789999554166}{1.220545640817}
  \meshline{144,144,144}{0.844359149717}{1.092511013658}{0.846204958056}{1.077077112913}
  \meshline{144,144,144}{0.841825291942}{1.108544770746}{0.841521897284}{1.109999803376}
  \meshline{144,144,144}{0.844181528911}{1.094138907839}{0.843505942960}{1.098135199638}
  \meshline{144,144,144}{0.895117121225}{1.267546078683}{0.900996688636}{1.257121130010}
  \meshline{144,144,144}{0.900996688636}{1.257121130010}{0.908111773931}{1.245342866372}
  \meshline{144,144,144}{0.878207283900}{1.287579668294}{0.885709777962}{1.279855339172}
  \meshline{144,144,144}{0.889242396549}{1.274952213578}{0.895117121225}{1.267546078683}
  \meshline{144,144,144}{0.868277321307}{1.296834154075}{0.873807110519}{1.292546764541}
  \meshline{144,144,144}{0.885709777962}{1.279855339172}{0.889242396549}{1.274952213578}
  \meshline{144,144,144}{0.782401334324}{1.228510618039}{0.778111333064}{1.233073717136}
  \meshline{144,144,144}{0.734387782767}{1.080107327804}{0.730364974432}{1.098325814702}
  \meshline{144,144,144}{0.778111333064}{1.233073717136}{0.772679117235}{1.237747941644}
  \meshline{144,144,144}{0.835858680725}{1.133845035710}{0.837289755507}{1.128110607290}
  \meshline{144,144,144}{0.734731378475}{1.353765817664}{0.720374164657}{1.356150313184}
  \meshline{144,144,144}{0.789999554166}{1.220545640817}{0.796534684555}{1.211813441675}
  \meshline{144,144,144}{0.767031582383}{1.243243967228}{0.755587824233}{1.252229995576}
  \meshline{144,144,144}{0.767031582383}{1.243243967228}{0.772679117235}{1.237747941644}
  \meshline{144,144,144}{0.538579859362}{1.321593317823}{0.531576621718}{1.322051420743}
  \meshline{144,144,144}{0.714031124603}{1.139020310467}{0.709631580988}{1.147177541310}
  \meshline{144,144,144}{0.873807110519}{1.292546764541}{0.878207283900}{1.287579668294}
  \meshline{144,144,144}{0.860250946279}{1.304151240226}{0.868277321307}{1.296834154075}
  \meshline{144,144,144}{0.691058457023}{1.172450591432}{0.683868287738}{1.179906864145}
  \meshline{144,144,144}{0.506452418129}{1.184472302003}{0.518224037441}{1.183352914323}
  \meshline{144,144,144}{0.709631580988}{1.147177541310}{0.700231886290}{1.160647453467}
  \meshline{144,144,144}{0.720331420548}{1.126178623521}{0.717297118806}{1.133256389408}
  \meshline{144,144,144}{0.717297118806}{1.133256389408}{0.714031124603}{1.139020310467}
  \meshline{144,144,144}{0.729113440028}{1.102681738059}{0.724758008709}{1.116192932779}
  \meshline{144,144,144}{0.753746417386}{1.253726310973}{0.755587824233}{1.252229995576}
  \meshline{144,144,144}{0.695064598066}{1.287220193208}{0.696197210715}{1.286694694692}
  \meshline{144,144,144}{0.753746417386}{1.253726310973}{0.752789064879}{1.254339853565}
  \meshline{144,144,144}{0.714364821953}{1.278146437567}{0.700748861155}{1.284509965895}
  \meshline{144,144,144}{0.621355661199}{1.310130006734}{0.602756971142}{1.313595833399}
  \meshline{144,144,144}{0.742002428298}{1.262390428094}{0.752789064879}{1.254339853565}
  \meshline{144,144,144}{0.716520499547}{1.277155344855}{0.729167204572}{1.270168522611}
  \meshline{144,144,144}{0.696197210715}{1.286694694692}{0.700748861155}{1.284509965895}
  \meshline{144,144,144}{0.664374592703}{1.298852072015}{0.672772160327}{1.295651210640}
  \meshline{144,144,144}{0.672772160327}{1.295651210640}{0.695064598066}{1.287220193208}
  \meshline{144,144,144}{0.442276151583}{1.020965654224}{0.445852027249}{1.016028940833}
  \meshline{144,144,144}{0.698936069416}{1.162586899496}{0.700231886290}{1.160647453467}
  \meshline{144,144,144}{0.584188215829}{1.238833636731}{0.596011562779}{1.235108286350}
  \meshline{144,144,144}{0.646131631351}{1.210818366799}{0.638479532315}{1.215237266515}
  \meshline{144,144,144}{0.609268165254}{1.229836926445}{0.609009723629}{1.229960978300}
  \meshline{144,144,144}{0.678972289192}{1.185056882286}{0.659804323482}{1.201144280786}
  \meshline{144,144,144}{0.691058457023}{1.172450591432}{0.697409530238}{1.164451147697}
  \meshline{144,144,144}{0.678972289192}{1.185056882286}{0.683868287738}{1.179906864145}
  \meshline{144,144,144}{0.697409530238}{1.164451147697}{0.698936069416}{1.162586899496}
  \meshline{144,144,144}{0.514349679442}{0.848482678092}{0.518116501441}{0.848735244121}
  \meshline{144,144,144}{0.537727902699}{0.851076276875}{0.551878993886}{0.853477509393}
  \meshline{144,144,144}{0.529749630359}{1.008954822784}{0.531569391141}{1.010405609044}
  \meshline{144,144,144}{0.509647175208}{0.915519452087}{0.519998177463}{0.917091360230}
  \meshline{144,144,144}{0.569575439719}{0.932251615291}{0.557849808045}{0.926977656716}
  \meshline{144,144,144}{0.557849808045}{0.926977656716}{0.551007047618}{0.924466583528}
  \meshline{144,144,144}{0.601505890764}{0.953143377737}{0.590892175305}{0.944324082675}
  \meshline{144,144,144}{0.390465555025}{0.863690479841}{0.400231524419}{0.860569856267}
  \meshline{144,144,144}{0.446667681374}{0.850580176005}{0.451479139470}{0.849820308207}
  \meshline{144,144,144}{0.144857654311}{1.011977795718}{0.146099288201}{1.000831849057}
  \meshline{144,144,144}{0.350203690585}{0.881655889977}{0.366126668326}{0.873568299286}
  \meshline{144,144,144}{0.135820539099}{0.598163202569}{0.149498010160}{0.607353193504}
  \meshline{144,144,144}{0.187147274902}{0.627404040291}{0.187511442045}{0.627601215633}
  \meshline{144,144,144}{0.169505141034}{0.619439569817}{0.159163229358}{0.613201544503}
  \meshline{144,144,144}{0.157743572633}{0.775184990361}{0.171535797194}{0.768189288017}
  \meshline{144,144,144}{0.176017715739}{0.766127265381}{0.182819376804}{0.762984711799}
  \meshline{144,144,144}{0.171535797194}{0.768189288017}{0.176017715739}{0.766127265381}
  \meshline{144,144,144}{0.264200962867}{0.824395955636}{0.258106478296}{0.827654437638}
  \meshline{144,144,144}{0.145146011583}{0.782467566244}{0.141607582571}{0.785166517014}
  \meshline{144,144,144}{0.200526183834}{0.756666339273}{0.191802184676}{0.760194951107}
  \meshline{144,144,144}{0.212578686304}{0.753395928963}{0.200526183834}{0.756666339273}
  \meshline{144,144,144}{0.208179805650}{0.866933868932}{0.200679270421}{0.875186121646}
  \meshline{144,144,144}{0.122405908967}{0.800722141972}{0.123401083395}{0.799877601418}
  \meshline{144,144,144}{0.145146011583}{0.782467566244}{0.157480708509}{0.775347453064}
  \meshline{144,144,144}{0.133485251134}{0.790685951253}{0.141607582571}{0.785166517014}
  \meshline{144,144,144}{0.157743572633}{0.775184990361}{0.157480708509}{0.775347453064}
  \meshline{144,144,144}{0.111197659811}{0.812149806897}{0.104803085204}{0.820755373667}
  \meshline{144,144,144}{0.111197659811}{0.812149806897}{0.121111074759}{0.802145362130}
  \meshline{144,144,144}{0.123401083395}{0.799877601418}{0.133485251134}{0.790685951253}
  \meshline{144,144,144}{0.121111074759}{0.802145362130}{0.122405908967}{0.800722141972}
  \meshline{144,144,144}{0.187085180998}{0.893143176070}{0.200679270421}{0.875186121646}
  \meshline{144,144,144}{0.091506606695}{0.841309306027}{0.085325397969}{0.853066073265}
  \meshline{144,144,144}{0.229140119512}{0.847777222388}{0.238974469044}{0.840467329915}
  \meshline{144,144,144}{0.248816061547}{0.833973619338}{0.242114212276}{0.838042982126}
  \meshline{144,144,144}{0.091506606695}{0.841309306027}{0.093455738779}{0.837423385648}
  \meshline{144,144,144}{0.074447897011}{0.882131658269}{0.070172037836}{0.895438027078}
  \meshline{144,144,144}{0.093455738779}{0.837423385648}{0.104803085204}{0.820755373667}
  \meshline{144,144,144}{0.075241848114}{0.879277197628}{0.074447897011}{0.882131658269}
  \meshline{144,144,144}{0.085325397969}{0.853066073265}{0.077332720900}{0.873839528060}
  \meshline{144,144,144}{0.075588260290}{0.878164556234}{0.077332720900}{0.873839528060}
  \meshline{144,144,144}{0.075241848114}{0.879277197628}{0.075588260290}{0.878164556234}
  \meshline{144,144,144}{0.221605284337}{0.854048459945}{0.229140119512}{0.847777222388}
  \meshline{144,144,144}{0.208179805650}{0.866933868932}{0.217559744800}{0.857744412707}
  \meshline{144,144,144}{0.221605284337}{0.854048459945}{0.217559744800}{0.857744412707}
  \meshline{144,144,144}{0.242114212276}{0.838042982126}{0.238974469044}{0.840467329915}
  \meshline{144,144,144}{0.248816061547}{0.833973619338}{0.258106478296}{0.827654437638}
  \meshline{144,144,144}{0.066285285548}{0.911781427028}{0.068729444174}{0.901623707389}
  \meshline{144,144,144}{0.064829824230}{0.919830535953}{0.066285285548}{0.911781427028}
  \meshline{144,144,144}{0.070172037836}{0.895438027078}{0.068729444174}{0.901623707389}
  \meshline{144,144,144}{0.064829824230}{0.919830535953}{0.062797573031}{0.928820194520}
  \meshline{144,144,144}{0.157548251918}{0.953126743966}{0.162558764390}{0.938512232631}
  \meshline{144,144,144}{0.187085180998}{0.893143176070}{0.185338707832}{0.895412002888}
  \meshline{144,144,144}{0.176684881141}{0.909176842988}{0.184622381735}{0.896576574140}
  \meshline{144,144,144}{0.168458357744}{0.925613899052}{0.170498570732}{0.920784729415}
  \meshline{144,144,144}{0.184622381735}{0.896576574140}{0.185338707832}{0.895412002888}
  \meshline{144,144,144}{0.170498570732}{0.920784729415}{0.174629383017}{0.913328315341}
  \meshline{144,144,144}{0.060395505863}{0.944403267030}{0.059227447911}{0.951711663890}
  \meshline{144,144,144}{0.154872925326}{0.961750739503}{0.150943953087}{0.975434478845}
  \meshline{144,144,144}{0.176684881141}{0.909176842988}{0.174629383017}{0.913328315341}
  \meshline{144,144,144}{0.157548251918}{0.953126743966}{0.156283036962}{0.956509287999}
  \meshline{144,144,144}{0.168458357744}{0.925613899052}{0.162558764390}{0.938512232631}
  \meshline{144,144,144}{0.654142915287}{0.895675463759}{0.654312586075}{0.895789405608}
  \meshline{144,144,144}{0.654142915287}{0.895675463759}{0.641099853317}{0.886997047566}
  \meshline{144,144,144}{0.669692947188}{0.907749711436}{0.654774446799}{0.896157747808}
  \meshline{144,144,144}{0.569575439719}{0.932251615291}{0.583572863352}{0.939839673205}
  \meshline{144,144,144}{0.609896445727}{0.959940603600}{0.615545153883}{0.965743320524}
  \meshline{144,144,144}{0.695103049923}{0.933562203200}{0.701521823096}{0.942209463131}
  \meshline{144,144,144}{0.654774446799}{0.896157747808}{0.654312586075}{0.895789405608}
  \meshline{144,144,144}{0.642252739963}{1.010402305563}{0.645169438168}{1.018872428648}
  \meshline{144,144,144}{0.622720450111}{0.974668186679}{0.630555007061}{0.985615082392}
  \meshline{144,144,144}{0.648890124631}{1.046793223529}{0.645169438168}{1.018872428648}
  \meshline{144,144,144}{0.634602030068}{0.992911367734}{0.639728155748}{1.003082421742}
  \meshline{144,144,144}{0.583572863352}{0.939839673205}{0.590892175305}{0.944324082675}
  \meshline{144,144,144}{0.639728155748}{1.003082421742}{0.642252739963}{1.010402305563}
  \meshline{144,144,144}{0.634602030068}{0.992911367734}{0.630555007061}{0.985615082392}
  \meshline{144,144,144}{0.601505890764}{0.953143377737}{0.609896445727}{0.959940603600}
  \meshline{144,144,144}{0.622720450111}{0.974668186679}{0.615545153883}{0.965743320524}
  \meshline{144,144,144}{0.689461368873}{0.927515868112}{0.695103049923}{0.933562203200}
  \meshline{144,144,144}{0.701521823096}{0.942209463131}{0.706026923939}{0.948479388571}
  \meshline{144,144,144}{0.736573192117}{1.045380191983}{0.735384961981}{1.029201217959}
  \meshline{144,144,144}{0.689461368873}{0.927515868112}{0.680477082254}{0.917542127929}
  \meshline{144,144,144}{0.674099959577}{0.911852148120}{0.669692947188}{0.907749711436}
  \meshline{144,144,144}{0.674099959577}{0.911852148120}{0.680477082254}{0.917542127929}
  \meshline{144,144,144}{0.710544083439}{0.956286114205}{0.706026923939}{0.948479388571}
  \meshline{144,144,144}{0.722588615128}{0.979479799199}{0.726269805245}{0.990359062507}
  \meshline{144,144,144}{0.719660361998}{0.973165647948}{0.715761636251}{0.964854524754}
  \meshline{144,144,144}{0.710544083439}{0.956286114205}{0.715761636251}{0.964854524754}
  \meshline{144,144,144}{0.540500650857}{1.021254542553}{0.531569391141}{1.010405609044}
  \meshline{144,144,144}{0.549970560425}{1.044646936282}{0.548742646536}{1.034977322668}
  \meshline{144,144,144}{0.549970560425}{1.044646936282}{0.551097688483}{1.053981514598}
  \meshline{144,144,144}{0.649596733018}{1.052672001469}{0.649323286366}{1.055117104948}
  \meshline{144,144,144}{0.550507797175}{1.058259235492}{0.548996319118}{1.063447792213}
  \meshline{144,144,144}{0.642212605641}{1.090933419998}{0.643567112187}{1.086417235637}
  \meshline{144,144,144}{0.548996319118}{1.063447792213}{0.538672506853}{1.083415880945}
  \meshline{144,144,144}{0.540500650857}{1.021254542553}{0.548742646536}{1.034977322668}
  \meshline{144,144,144}{0.609009723629}{1.229960978300}{0.608849448227}{1.230026374790}
  \meshline{144,144,144}{0.538672506853}{1.083415880945}{0.538615191300}{1.083486238625}
  \meshline{144,144,144}{0.613307212201}{1.136613726036}{0.619554796099}{1.130210788776}
  \meshline{144,144,144}{0.605251013517}{1.144877336262}{0.613307212201}{1.136613726036}
  \meshline{144,144,144}{0.538531826496}{1.083551145582}{0.524383312858}{1.094213868791}
  \meshline{144,144,144}{0.586709684146}{1.158710788839}{0.600252042676}{1.148791219356}
  \meshline{144,144,144}{0.659804323482}{1.201144280786}{0.658048005315}{1.202568386689}
  \meshline{144,144,144}{0.605251013517}{1.144877336262}{0.600252042676}{1.148791219356}
  \meshline{144,144,144}{0.655406397423}{1.204355095219}{0.658048005315}{1.202568386689}
  \meshline{144,144,144}{0.550507797175}{1.058259235492}{0.551097688483}{1.053981514598}
  \meshline{144,144,144}{0.538615191300}{1.083486238625}{0.538531826496}{1.083551145582}
  \meshline{144,144,144}{0.507628477842}{0.999537434108}{0.528646557391}{1.008413399731}
  \meshline{144,144,144}{0.646131631351}{1.210818366799}{0.655406397423}{1.204355095219}
  \meshline{144,144,144}{0.632883947492}{1.218635805062}{0.638479532315}{1.215237266515}
  \meshline{144,144,144}{0.611107249901}{1.228951529280}{0.632883947492}{1.218635805062}
  \meshline{144,144,144}{0.611107249901}{1.228951529280}{0.609268165254}{1.229836926445}
  \meshline{144,144,144}{0.596011562779}{1.235108286350}{0.608474939511}{1.230159464075}
  \meshline{144,144,144}{0.506572751156}{1.099535535036}{0.520225472299}{1.095582701355}
  \meshline{144,144,144}{0.458511426230}{1.092209722717}{0.471727549642}{1.098952016012}
  \meshline{144,144,144}{0.520225472299}{1.095582701355}{0.524383312858}{1.094213868791}
  \meshline{144,144,144}{0.560608085162}{1.172061727746}{0.577240288414}{1.164022364285}
  \meshline{144,144,144}{0.532553442510}{1.180761188307}{0.518224037441}{1.183352914323}
  \meshline{144,144,144}{0.543601775672}{1.177723757084}{0.559251519378}{1.172594037159}
  \meshline{144,144,144}{0.473715621063}{1.184373805035}{0.474108255286}{1.184415414075}
  \meshline{144,144,144}{0.539019115893}{1.179269201206}{0.532553442510}{1.180761188307}
  \meshline{144,144,144}{0.539019115893}{1.179269201206}{0.543601775672}{1.177723757084}
  \meshline{144,144,144}{0.506452418129}{1.184472302003}{0.499014898555}{1.185149174599}
  \meshline{144,144,144}{0.559251519378}{1.172594037159}{0.559790323954}{1.172421739805}
  \meshline{144,144,144}{0.497087840920}{1.101184689800}{0.487412426100}{1.101394653299}
  \meshline{144,144,144}{0.481406963120}{0.998343346657}{0.488717768629}{0.997890316807}
  \meshline{144,144,144}{0.471727549642}{1.098952016012}{0.474859856626}{1.100155028798}
  \meshline{144,144,144}{0.500050953888}{0.914894192385}{0.491560600242}{0.914715045626}
  \meshline{144,144,144}{0.501498305162}{0.998279961639}{0.507628477842}{0.999537434108}
  \meshline{144,144,144}{0.608849448227}{1.230026374790}{0.608474939511}{1.230159464075}
  \meshline{144,144,144}{0.582438825268}{1.239418671485}{0.584188215829}{1.238833636731}
  \meshline{144,144,144}{0.586709684146}{1.158710788839}{0.577240288414}{1.164022364285}
  \meshline{144,144,144}{0.560102507224}{1.172299135307}{0.560608085162}{1.172061727746}
  \meshline{144,144,144}{0.560102507224}{1.172299135307}{0.559790323954}{1.172421739805}
  \meshline{144,144,144}{0.517534900401}{1.251241369669}{0.522784691483}{1.250954675463}
  \meshline{144,144,144}{0.473715621063}{1.184373805035}{0.451310560689}{1.180877880069}
  \meshline{144,144,144}{0.477043830131}{1.184497981242}{0.499014898555}{1.185149174599}
  \meshline{144,144,144}{0.474594148784}{1.184440775256}{0.474108255286}{1.184415414075}
  \meshline{144,144,144}{0.477043830131}{1.184497981242}{0.474594148784}{1.184440775256}
  \meshline{144,144,144}{0.506572751156}{1.099535535036}{0.497087840920}{1.101184689800}
  \meshline{144,144,144}{0.487412426100}{1.101394653299}{0.474859856626}{1.100155028798}
  \meshline{144,144,144}{0.451249752453}{1.180866687117}{0.451310560689}{1.180877880069}
  \meshline{144,144,144}{0.439763651328}{1.073928531595}{0.444646659195}{1.080793056930}
  \meshline{144,144,144}{0.451089745236}{1.180820904794}{0.451249752453}{1.180866687117}
  \meshline{144,144,144}{0.391582308822}{1.154388039760}{0.400673206593}{1.160369044762}
  \meshline{144,144,144}{0.391582308822}{1.154388039760}{0.377551800823}{1.143121383301}
  \meshline{144,144,144}{0.458511426230}{1.092209722717}{0.452025228994}{1.087303648870}
  \meshline{144,144,144}{0.452025228994}{1.087303648870}{0.444646659195}{1.080793056930}
  \meshline{144,144,144}{0.373549861446}{1.139412691781}{0.365695928593}{1.130326698041}
  \meshline{144,144,144}{0.351267719095}{1.110215040494}{0.349851642418}{1.108059035943}
  \meshline{144,144,144}{0.377551800823}{1.143121383301}{0.373549861446}{1.139412691781}
  \meshline{144,144,144}{0.365695928593}{1.130326698041}{0.360691171923}{1.124653628002}
  \meshline{144,144,144}{0.335231435941}{1.054760454762}{0.335778676918}{1.038117610001}
  \meshline{144,144,144}{0.351267719095}{1.110215040494}{0.360691171923}{1.124653628002}
  \meshline{144,144,144}{0.348468532151}{1.105227939238}{0.342158207523}{1.089363733126}
  \meshline{144,144,144}{0.337048218247}{1.069223537736}{0.335231435941}{1.054760454762}
  \meshline{144,144,144}{0.335778676918}{1.038117610001}{0.335916812218}{1.035751882955}
  \meshline{144,144,144}{0.338295640391}{1.024415071811}{0.335916812218}{1.035751882955}
  \meshline{144,144,144}{0.338295640391}{1.024415071811}{0.340450067898}{1.013807813839}
  \meshline{144,144,144}{0.337048218247}{1.069223537736}{0.338035480724}{1.075710948114}
  \meshline{144,144,144}{0.342158207523}{1.089363733126}{0.338035480724}{1.075710948114}
  \meshline{144,144,144}{0.347471699334}{0.996223681846}{0.347155686868}{0.996996697300}
  \meshline{144,144,144}{0.340450067898}{1.013807813839}{0.341012327436}{1.011978362817}
  \meshline{144,144,144}{0.278157143371}{0.949259236450}{0.281756970647}{0.943421685560}
  \meshline{144,144,144}{0.297134886994}{0.924176803414}{0.293606207668}{0.927799179656}
  \meshline{144,144,144}{0.281756970647}{0.943421685560}{0.285528508403}{0.938542382910}
  \meshline{144,144,144}{0.269649115224}{0.963976162853}{0.264733233593}{0.973748706407}
  \meshline{144,144,144}{0.269649115224}{0.963976162853}{0.272014072710}{0.959006041206}
  \meshline{144,144,144}{0.292241649788}{0.929420630079}{0.285528508403}{0.938542382910}
  \meshline{144,144,144}{0.278157143371}{0.949259236450}{0.272014072710}{0.959006041206}
  \meshline{144,144,144}{0.261140973188}{0.983234888747}{0.257530964853}{0.993145023647}
  \meshline{144,144,144}{0.316144498006}{0.905351549621}{0.307928908458}{0.912477711253}
  \meshline{144,144,144}{0.326732418647}{0.896932764147}{0.329545265515}{0.894748735200}
  \meshline{144,144,144}{0.371936818910}{0.870888026049}{0.366126668326}{0.873568299286}
  \meshline{144,144,144}{0.293606207668}{0.927799179656}{0.292241649788}{0.929420630079}
  \meshline{144,144,144}{0.316144498006}{0.905351549621}{0.326732418647}{0.896932764147}
  \meshline{144,144,144}{0.383166646935}{0.866455198089}{0.390465555025}{0.863690479841}
  \meshline{144,144,144}{0.347471699334}{0.996223681846}{0.347703130325}{0.995835259101}
  \meshline{144,144,144}{0.360778851353}{0.974369445796}{0.364280597237}{0.970384542515}
  \meshline{144,144,144}{0.341012327436}{1.011978362817}{0.347155686868}{0.996996697300}
  \meshline{144,144,144}{0.347703130325}{0.995835259101}{0.358027310140}{0.978322926953}
  \meshline{144,144,144}{0.287408920167}{0.812598837800}{0.277367720707}{0.817612015308}
  \meshline{144,144,144}{0.358027310140}{0.978322926953}{0.360778851353}{0.974369445796}
  \meshline{144,144,144}{0.371380374884}{0.962279171914}{0.381124163175}{0.953034609576}
  \meshline{144,144,144}{0.364280597237}{0.970384542515}{0.371380374884}{0.962279171914}
  \meshline{144,144,144}{0.398979408511}{0.939757354603}{0.387652545984}{0.948033855396}
  \meshline{144,144,144}{0.387652545984}{0.948033855396}{0.381124163175}{0.953034609576}
  \meshline{144,144,144}{0.452881369413}{1.011238095750}{0.445852027249}{1.016028940833}
  \meshline{144,144,144}{0.433052407874}{1.040676722283}{0.435586750622}{1.033787269912}
  \meshline{144,144,144}{0.416440796997}{0.930529773865}{0.408804324546}{0.934551980932}
  \meshline{144,144,144}{0.432845434344}{1.046997498465}{0.433052407874}{1.040676722283}
  \meshline{144,144,144}{0.398979408511}{0.939757354603}{0.408804324546}{0.934551980932}
  \meshline{144,144,144}{0.452881369413}{1.011238095750}{0.468576013212}{1.001586858854}
  \meshline{144,144,144}{0.453404469850}{0.918466272488}{0.451198076877}{0.918896060019}
  \meshline{144,144,144}{0.500050953888}{0.914894192385}{0.509647175208}{0.915519452087}
  \meshline{144,144,144}{0.433684628296}{0.923777121134}{0.428396994798}{0.925823648911}
  \meshline{144,144,144}{0.469114413977}{0.916086042487}{0.453404469850}{0.918466272488}
  \meshline{144,144,144}{0.486491687354}{0.847771070721}{0.473763424191}{0.847973868191}
  \meshline{144,144,144}{0.519998177463}{0.917091360230}{0.532012098215}{0.919109872161}
  \meshline{144,144,144}{0.427638607580}{0.853617829895}{0.429168224279}{0.853287219631}
  \meshline{144,144,144}{0.428396994798}{0.925823648911}{0.416440796997}{0.930529773865}
  \meshline{144,144,144}{0.488717768629}{0.997890316807}{0.501498305162}{0.998279961639}
  \meshline{144,144,144}{0.468576013212}{1.001586858854}{0.481406963120}{0.998343346657}
  \meshline{144,144,144}{0.479602765138}{0.915090748192}{0.491560600242}{0.914715045626}
  \meshline{144,144,144}{0.454881088300}{0.849540489146}{0.473763424191}{0.847973868191}
  \meshline{144,144,144}{0.446667681374}{0.850580176005}{0.429168224279}{0.853287219631}
  \meshline{144,144,144}{0.538051608820}{0.920814987696}{0.532012098215}{0.919109872161}
  \meshline{144,144,144}{0.350092297613}{0.881709292823}{0.350047858601}{0.881733017131}
  \meshline{144,144,144}{0.350203690585}{0.881655889977}{0.350092297613}{0.881709292823}
  \meshline{144,144,144}{0.350047858601}{0.881733017131}{0.330441776607}{0.894173848227}
  \meshline{144,144,144}{0.436269548464}{0.923007415608}{0.451198076877}{0.918896060019}
  \meshline{144,144,144}{0.433684628296}{0.923777121134}{0.436269548464}{0.923007415608}
  \meshline{144,144,144}{0.451951245993}{0.849770122722}{0.451479139470}{0.849820308207}
  \meshline{144,144,144}{0.528646557391}{1.008413399731}{0.529749630359}{1.008954822784}
  \meshline{144,144,144}{0.410283752165}{0.857649375497}{0.427638607580}{0.853617829895}
  \meshline{144,144,144}{0.371936818910}{0.870888026049}{0.383166646935}{0.866455198089}
  \meshline{144,144,144}{0.307928908458}{0.912477711253}{0.297134886994}{0.924176803414}
  \meshline{144,144,144}{0.330441776607}{0.894173848227}{0.329545265515}{0.894748735200}
  \meshline{144,144,144}{0.410283752165}{0.857649375497}{0.400231524419}{0.860569856267}
  \meshline{144,144,144}{0.561749794778}{1.244759862078}{0.582438825268}{1.239418671485}
  \meshline{144,144,144}{0.560354113439}{1.245063976483}{0.542321774385}{1.248513200059}
  \meshline{144,144,144}{0.560354113439}{1.245063976483}{0.561749794778}{1.244759862078}
  \meshline{144,144,144}{0.549846788112}{1.371848082245}{0.532864062013}{1.372206998900}
  \meshline{144,144,144}{0.542321774385}{1.248513200059}{0.527599506919}{1.250366995364}
  \meshline{144,144,144}{0.527599506919}{1.250366995364}{0.522784691483}{1.250954675463}
  \meshline{144,144,144}{0.063286923723}{1.170588934765}{0.061561468845}{1.161841530176}
  \meshline{144,144,144}{0.499259761513}{1.252193401802}{0.517534900401}{1.251241369669}
  \meshline{144,144,144}{0.499259761513}{1.252193401802}{0.487678810248}{1.252280290433}
  \meshline{144,144,144}{0.487678810248}{1.252280290433}{0.478490424992}{1.251988304593}
  \meshline{144,144,144}{0.499198425560}{1.323049543269}{0.497339873920}{1.323053357806}
  \meshline{144,144,144}{0.439763651328}{1.073928531595}{0.434698129347}{1.060867743615}
  \meshline{144,144,144}{0.432845434344}{1.046997498465}{0.434698129347}{1.060867743615}
  \meshline{144,144,144}{0.249391327970}{1.040437977040}{0.249390141280}{1.040463927728}
  \meshline{144,144,144}{0.249941968687}{1.066658126637}{0.249392052266}{1.040517919211}
  \meshline{144,144,144}{0.249391327970}{1.040437977040}{0.249402799375}{1.040321814265}
  \meshline{144,144,144}{0.271825577190}{0.820076244333}{0.264200962867}{0.824395955636}
  \meshline{144,144,144}{0.298578611299}{0.808436433610}{0.308678417172}{0.804174079995}
  \meshline{144,144,144}{0.298578611299}{0.808436433610}{0.287408920167}{0.812598837800}
  \meshline{144,144,144}{0.511948565673}{1.322933385140}{0.526347840821}{1.322225213926}
  \meshline{144,144,144}{0.249941968687}{1.066658126637}{0.251256048624}{1.075876691389}
  \meshline{144,144,144}{0.308678417172}{0.804174079995}{0.315169778118}{0.801809338443}
  \meshline{144,144,144}{0.435586750622}{1.033787269912}{0.442276151583}{1.020965654224}
  \meshline{144,144,144}{0.531576621718}{1.322051420743}{0.526347840821}{1.322225213926}
  \meshline{144,144,144}{0.594126436399}{1.315252495105}{0.598258866472}{1.314527417359}
  \meshline{144,144,144}{0.566443537181}{1.319192597889}{0.554125732270}{1.320289104213}
  \meshline{144,144,144}{0.292816810948}{0.736904643258}{0.283863777013}{0.738289844442}
  \meshline{144,144,144}{0.248442203956}{0.744370352385}{0.238601837218}{0.746425683755}
  \meshline{144,144,144}{0.305688101296}{0.735102879542}{0.292816810948}{0.736904643258}
  \meshline{144,144,144}{0.281763226255}{0.738499971838}{0.266998534883}{0.740793219301}
  \meshline{144,144,144}{0.311532817341}{0.734563700129}{0.314667378930}{0.734457544511}
  \meshline{144,144,144}{0.271825577190}{0.820076244333}{0.277367720707}{0.817612015308}
  \meshline{144,144,144}{0.598258866472}{1.314527417359}{0.602756971142}{1.313595833399}
  \meshline{144,144,144}{0.554860296319}{1.371608329862}{0.576537139623}{1.370799955743}
  \meshline{144,144,144}{0.566443537181}{1.319192597889}{0.577714040761}{1.317654331901}
  \meshline{144,144,144}{0.576537139623}{1.370799955743}{0.577120247272}{1.370760306711}
  \meshline{144,144,144}{0.577714040761}{1.317654331901}{0.594126436399}{1.315252495105}
  \meshline{144,144,144}{0.625630223930}{1.309147880257}{0.629485088448}{1.308088181082}
  \meshline{144,144,144}{0.664374592703}{1.298852072015}{0.655138337320}{1.301496174526}
  \meshline{144,144,144}{0.654301363373}{1.301745091908}{0.652852224117}{1.302114313559}
  \meshline{144,144,144}{0.640341962062}{1.305551290066}{0.629485088448}{1.308088181082}
  \meshline{144,144,144}{0.654301363373}{1.301745091908}{0.655138337320}{1.301496174526}
  \meshline{144,144,144}{0.640341962062}{1.305551290066}{0.652852224117}{1.302114313559}
  \meshline{144,144,144}{0.554125732270}{1.320289104213}{0.538579859362}{1.321593317823}
  \meshline{144,144,144}{0.554860296319}{1.371608329862}{0.549846788112}{1.371848082245}
  \meshline{144,144,144}{0.493176287455}{1.372672678283}{0.506175923085}{1.372614046515}
  \meshline{144,144,144}{0.511948565673}{1.322933385140}{0.499198425560}{1.323049543269}
  \meshline{144,144,144}{0.460627327011}{1.372429270367}{0.454946271520}{1.372214833275}
  \meshline{144,144,144}{0.497339873920}{1.323053357806}{0.476927077777}{1.322962753133}
  \meshline{144,144,144}{0.471546121885}{1.322807218014}{0.460306583389}{1.322374316574}
  \meshline{144,144,144}{0.506175923085}{1.372614046515}{0.511205107401}{1.372546997729}
  \meshline{144,144,144}{0.528266792686}{1.372346439302}{0.532864062013}{1.372206998900}
  \meshline{144,144,144}{0.460627327011}{1.372429270367}{0.469095562213}{1.372520363432}
  \meshline{144,144,144}{0.433064880918}{1.246861957841}{0.446663133326}{1.249080523203}
  \meshline{144,144,144}{0.528266792686}{1.372346439302}{0.511205107401}{1.372546997729}
  \meshline{144,144,144}{0.484378044139}{1.372629603331}{0.493176287455}{1.372672678283}
  \meshline{144,144,144}{0.457386755876}{1.250504936649}{0.467425128198}{1.251285149569}
  \meshline{144,144,144}{0.579916931068}{1.370590364869}{0.577120247272}{1.370760306711}
  \meshline{144,144,144}{0.598564571722}{1.369594890488}{0.579916931068}{1.370590364869}
  \meshline{144,144,144}{0.484378044139}{1.372629603331}{0.469095562213}{1.372520363432}
  \meshline{144,144,144}{0.598564571722}{1.369594890488}{0.603813092212}{1.369403724717}
  \meshline{144,144,144}{0.603813092212}{1.369403724717}{0.620105759308}{1.368111006258}
  \meshline{144,144,144}{0.632972843383}{1.367334024282}{0.625242185397}{1.367879986426}
  \meshline{144,144,144}{0.632972843383}{1.367334024282}{0.644882947696}{1.366228280517}
  \meshline{144,144,144}{0.399728110196}{1.316533121595}{0.398406246633}{1.316334018385}
  \meshline{144,144,144}{0.471546121885}{1.322807218014}{0.476927077777}{1.322962753133}
  \meshline{144,144,144}{0.432180630694}{1.320298421648}{0.428154682911}{1.320000427611}
  \meshline{144,144,144}{0.460306583389}{1.322374316574}{0.452548732161}{1.321918396295}
  \meshline{144,144,144}{0.666078678287}{1.364074499806}{0.656151412794}{1.364777837682}
  \meshline{144,144,144}{0.625242185397}{1.367879986426}{0.620105759308}{1.368111006258}
  \meshline{144,144,144}{0.621355661199}{1.310130006734}{0.625630223930}{1.309147880257}
  \meshline{144,144,144}{0.684072612321}{1.361743628881}{0.682430164621}{1.362056370737}
  \meshline{144,144,144}{0.426589157917}{1.319865318708}{0.428154682911}{1.320000427611}
  \meshline{144,144,144}{0.478490424992}{1.251988304593}{0.467425128198}{1.251285149569}
  \meshline{144,144,144}{0.379731999950}{1.369072155842}{0.398744936056}{1.370316436537}
  \meshline{144,144,144}{0.445462114814}{1.321442862785}{0.452548732161}{1.321918396295}
  \meshline{144,144,144}{0.656151412794}{1.364777837682}{0.644882947696}{1.366228280517}
  \meshline{144,144,144}{0.682430164621}{1.362056370737}{0.680715459590}{1.362288452618}
  \meshline{144,144,144}{0.680715459590}{1.362288452618}{0.666078678287}{1.364074499806}
  \meshline{144,144,144}{0.702632262469}{1.358969366312}{0.684072612321}{1.361743628881}
  \meshline{144,144,144}{0.432180630694}{1.320298421648}{0.445462114814}{1.321442862785}
  \meshline{144,144,144}{0.401615475977}{1.316730046914}{0.426589157917}{1.319865318708}
  \meshline{144,144,144}{0.742002428298}{1.262390428094}{0.732462067314}{1.268271961102}
  \meshline{144,144,144}{0.753892768218}{1.349418659842}{0.743332611492}{1.351576051124}
  \meshline{144,144,144}{0.729167204572}{1.270168522611}{0.732462067314}{1.268271961102}
  \meshline{144,144,144}{0.785880746917}{1.340546230944}{0.774036189104}{1.344200540974}
  \meshline{144,144,144}{0.716671727671}{1.356998905926}{0.720374164657}{1.356150313184}
  \meshline{144,144,144}{0.716671727671}{1.356998905926}{0.702632262469}{1.358969366312}
  \meshline{144,144,144}{0.716520499547}{1.277155344855}{0.714364821953}{1.278146437567}
  \meshline{144,144,144}{0.454946271520}{1.372214833275}{0.440422246594}{1.371936452714}
  \meshline{144,144,144}{0.403855921916}{1.370475356113}{0.421086129900}{1.371274868118}
  \meshline{144,144,144}{0.427763725856}{1.371639834600}{0.421086129900}{1.371274868118}
  \meshline{144,144,144}{0.403855921916}{1.370475356113}{0.400755689165}{1.370369125737}
  \meshline{144,144,144}{0.332617769894}{1.365386050230}{0.316039617776}{1.363334981150}
  \meshline{144,144,144}{0.400755689165}{1.370369125737}{0.398744936056}{1.370316436537}
  \meshline{144,144,144}{0.440422246594}{1.371936452714}{0.427763725856}{1.371639834600}
  \meshline{144,144,144}{0.344074473649}{1.366148289627}{0.332617769894}{1.365386050230}
  \meshline{144,144,144}{0.400673206593}{1.160369044762}{0.407132415717}{1.164235440463}
  \meshline{144,144,144}{0.401615475977}{1.316730046914}{0.399728110196}{1.316533121595}
  \meshline{144,144,144}{0.378066984106}{1.312803734135}{0.398406246633}{1.316334018385}
  \meshline{144,144,144}{0.379731999950}{1.369072155842}{0.374411723143}{1.368864711947}
  \meshline{144,144,144}{0.365531755793}{1.368297276238}{0.353844552886}{1.367327012016}
  \meshline{144,144,144}{0.374411723143}{1.368864711947}{0.365531755793}{1.368297276238}
  \meshline{144,144,144}{0.860250946279}{1.304151240226}{0.851933109461}{1.309694979355}
  \meshline{144,144,144}{0.812088647328}{1.331386834995}{0.824628326494}{1.325877478697}
  \meshline{144,144,144}{0.774036189104}{1.344200540974}{0.763750880622}{1.347225689429}
  \meshline{144,144,144}{0.734731378475}{1.353765817664}{0.743332611492}{1.351576051124}
  \meshline{144,144,144}{0.824628326494}{1.325877478697}{0.838634635724}{1.317772438236}
  \meshline{144,144,144}{0.789708680861}{1.339631298594}{0.802323012983}{1.334877096985}
  \meshline{144,144,144}{0.753892768218}{1.349418659842}{0.763750880622}{1.347225689429}
  \meshline{144,144,144}{0.812088647328}{1.331386834995}{0.806214738207}{1.333769506416}
  \meshline{144,144,144}{0.785880746917}{1.340546230944}{0.789708680861}{1.339631298594}
  \meshline{144,144,144}{0.806214738207}{1.333769506416}{0.802323012983}{1.334877096985}
  \meshline{144,144,144}{0.344074473649}{1.366148289627}{0.353844552886}{1.367327012016}
  \meshline{144,144,144}{0.316039617776}{1.363334981150}{0.312310781458}{1.363098136371}
  \meshline{144,144,144}{0.312310781458}{1.363098136371}{0.306217420917}{1.362417315601}
  \meshline{144,144,144}{0.295124500515}{1.360833947747}{0.306217420917}{1.362417315601}
  \meshline{144,144,144}{0.378066984106}{1.312803734135}{0.374764289691}{1.312233981140}
  \meshline{144,144,144}{0.340498394296}{1.304161779535}{0.331942377157}{1.302009643996}
  \meshline{144,144,144}{0.374764289691}{1.312233981140}{0.358681060247}{1.308821726085}
  \meshline{144,144,144}{0.340498394296}{1.304161779535}{0.351103519428}{1.307097085379}
  \meshline{144,144,144}{0.358681060247}{1.308821726085}{0.351103519428}{1.307097085379}
  \meshline{144,144,144}{0.851933109461}{1.309694979355}{0.845735322317}{1.314176664697}
  \meshline{144,144,144}{0.845735322317}{1.314176664697}{0.838634635724}{1.317772438236}
  \meshline{144,144,144}{0.666888836165}{0.804095730639}{0.680786007101}{0.808796851622}
  \meshline{144,144,144}{0.773230064921}{0.865291421061}{0.781817016180}{0.873094716152}
  \meshline{144,144,144}{0.762582989538}{0.855564166742}{0.767281544877}{0.859428840940}
  \meshline{144,144,144}{0.939293416974}{0.983512064248}{0.939606157683}{0.988474756691}
  \meshline{144,144,144}{0.159163229358}{0.613201544503}{0.154311092373}{0.610699939669}
  \meshline{144,144,144}{0.149655920670}{0.981693661619}{0.146933443099}{0.996071691497}
  \meshline{144,144,144}{0.649519656565}{1.051329715831}{0.649596733018}{1.052672001469}
  \meshline{144,144,144}{0.730609810293}{1.004109772418}{0.733997227716}{1.018155259649}
  \meshline{144,144,144}{0.734387782767}{1.080107327804}{0.736126650926}{1.064029997318}
  \meshline{144,144,144}{0.735287493400}{1.028580847549}{0.733997227716}{1.018155259649}
  \meshline{144,144,144}{0.736233934214}{1.063296614040}{0.736565774108}{1.045762904281}
  \meshline{144,144,144}{0.730026762550}{1.100030773384}{0.729113440028}{1.102681738059}
  \meshline{144,144,144}{0.648890124631}{1.046793223529}{0.649519656565}{1.051329715831}
  \meshline{144,144,144}{0.730026762550}{1.100030773384}{0.730170749232}{1.099456102643}
  \meshline{144,144,144}{0.647427413861}{1.071463102406}{0.643567112187}{1.086417235637}
  \meshline{144,144,144}{0.631487824339}{1.113620956257}{0.634288467375}{1.108669479190}
  \meshline{144,144,144}{0.640350867634}{1.095097071010}{0.642212605641}{1.090933419998}
  \meshline{144,144,144}{0.619554796099}{1.130210788776}{0.623733237006}{1.124347662844}
  \meshline{144,144,144}{0.728921207027}{0.997495570906}{0.726269805245}{0.990359062507}
  \meshline{144,144,144}{0.735384961981}{1.029201217959}{0.735287493400}{1.028580847549}
  \meshline{144,144,144}{0.631487824339}{1.113620956257}{0.623733237006}{1.124347662844}
  \meshline{144,144,144}{0.730170749232}{1.099456102643}{0.730364974432}{1.098325814702}
  \meshline{144,144,144}{0.640350867634}{1.095097071010}{0.634288467375}{1.108669479190}
  \meshline{144,144,144}{0.736126650926}{1.064029997318}{0.736233934214}{1.063296614040}
  \meshline{144,144,144}{0.647427413861}{1.071463102406}{0.649323286366}{1.055117104948}
  \meshline{144,144,144}{0.416104208936}{1.168331253612}{0.407132415717}{1.164235440463}
  \meshline{144,144,144}{0.416104208936}{1.168331253612}{0.429145442005}{1.174175883844}
  \meshline{144,144,144}{0.449429784028}{1.249424707124}{0.457386755876}{1.250504936649}
  \meshline{144,144,144}{0.428439664006}{1.245926940886}{0.413011556911}{1.242309438597}
  \meshline{144,144,144}{0.433064880918}{1.246861957841}{0.428439664006}{1.245926940886}
  \meshline{144,144,144}{0.446663133326}{1.249080523203}{0.449429784028}{1.249424707124}
  \meshline{144,144,144}{0.429145442005}{1.174175883844}{0.451089745236}{1.180820904794}
  \meshline{144,144,144}{0.388918565796}{1.234835707274}{0.408195764088}{1.241108453772}
  \meshline{144,144,144}{0.408195764088}{1.241108453772}{0.413011556911}{1.242309438597}
  \meshline{144,144,144}{0.249392052266}{1.040517919211}{0.249390141280}{1.040463927728}
  \meshline{144,144,144}{0.249402799375}{1.040321814265}{0.250871424477}{1.023401597528}
  \meshline{144,144,144}{0.261140973188}{0.983234888747}{0.264733233593}{0.973748706407}
  \meshline{144,144,144}{0.251433204772}{1.020394230904}{0.254233404378}{1.006190143813}
  \meshline{144,144,144}{0.156283036962}{0.956509287999}{0.154872925326}{0.961750739503}
  \meshline{144,144,144}{0.250871424477}{1.023401597528}{0.251433204772}{1.020394230904}
  \meshline{144,144,144}{0.254233404378}{1.006190143813}{0.257530964853}{0.993145023647}
  \meshline{144,144,144}{0.058622730389}{0.957884930573}{0.059007289683}{0.953708635209}
  \meshline{144,144,144}{0.142680396314}{1.040845904801}{0.142655779438}{1.056537496446}
  \meshline{144,144,144}{0.053900949351}{1.018048144664}{0.054166198859}{1.010486587809}
  \meshline{144,144,144}{0.144040114023}{1.018317432756}{0.143814774904}{1.021935331259}
  \meshline{144,144,144}{0.142733547432}{1.063049540593}{0.142655779438}{1.056537496446}
  \meshline{144,144,144}{0.143814774904}{1.021935331259}{0.142782162343}{1.033876599829}
  \meshline{144,144,144}{0.144040114023}{1.018317432756}{0.144857654311}{1.011977795718}
  \meshline{144,144,144}{0.062797573031}{0.928820194520}{0.062039544659}{0.932638250967}
  \meshline{144,144,144}{0.150943953087}{0.975434478845}{0.149655920670}{0.981693661619}
  \meshline{144,144,144}{0.058622730389}{0.957884930573}{0.057278249030}{0.967515424203}
  \meshline{144,144,144}{0.059007289683}{0.953708635209}{0.059227447911}{0.951711663890}
  \meshline{144,144,144}{0.062039544659}{0.932638250967}{0.060395505863}{0.944403267030}
  \meshline{144,144,144}{0.142680396314}{1.040845904801}{0.142782162343}{1.033876599829}
  \meshline{144,144,144}{0.146099288201}{1.000831849057}{0.146933443099}{0.996071691497}
  \meshline{144,144,144}{0.057278249030}{0.967515424203}{0.056217437518}{0.980395568208}
  \meshline{144,144,144}{0.056217437518}{0.980395568208}{0.056101655388}{0.981960237933}
  \meshline{144,144,144}{0.290299985949}{1.286744863142}{0.277390549879}{1.280494849366}
  \meshline{144,144,144}{0.059232773719}{1.145284659584}{0.059964658556}{1.149571213538}
  \meshline{144,144,144}{0.143381059472}{1.071282340888}{0.143991446626}{1.080465670109}
  \meshline{144,144,144}{0.147381020623}{1.104946666677}{0.146749454215}{1.101792870065}
  \meshline{144,144,144}{0.152281751736}{1.127852210112}{0.152922985722}{1.129859234647}
  \meshline{144,144,144}{0.146749454215}{1.101792870065}{0.146383001019}{1.099021362287}
  \meshline{144,144,144}{0.053325191792}{1.051050469017}{0.053378459895}{1.061015988161}
  \meshline{144,144,144}{0.252457018232}{1.085043707435}{0.251256048624}{1.075876691389}
  \meshline{144,144,144}{0.054166198859}{1.010486587809}{0.054546197478}{1.001362156446}
  \meshline{144,144,144}{0.058445368368}{1.138465757772}{0.059232773719}{1.145284659584}
  \meshline{144,144,144}{0.055128835388}{1.103471848254}{0.054319344489}{1.091417845861}
  \meshline{144,144,144}{0.054101133491}{1.084569469081}{0.053480176869}{1.070339398636}
  \meshline{144,144,144}{0.053480176869}{1.070339398636}{0.053378459895}{1.061015988161}
  \meshline{144,144,144}{0.054101133491}{1.084569469081}{0.054319344489}{1.091417845861}
  \meshline{144,144,144}{0.057030163351}{1.126166220089}{0.056190770061}{1.116159229767}
  \meshline{144,144,144}{0.055128835388}{1.103471848254}{0.055492592873}{1.108784059215}
  \meshline{144,144,144}{0.056190770061}{1.116159229767}{0.055492592873}{1.108784059215}
  \meshline{144,144,144}{0.058445368368}{1.138465757772}{0.057246783908}{1.129233196829}
  \meshline{144,144,144}{0.053271434747}{1.039700085437}{0.053361331574}{1.032584619303}
  \meshline{144,144,144}{0.053325191792}{1.051050469017}{0.053271434747}{1.039700085437}
  \meshline{144,144,144}{0.145535367140}{1.091583444096}{0.146383001019}{1.099021362287}
  \meshline{144,144,144}{0.143381059472}{1.071282340888}{0.142733547432}{1.063049540593}
  \meshline{144,144,144}{0.145535367140}{1.091583444096}{0.143991446626}{1.080465670109}
  \meshline{144,144,144}{0.054546197478}{1.001362156446}{0.056101655388}{0.981960237933}
  \meshline{144,144,144}{0.152281751736}{1.127852210112}{0.152062598053}{1.126902683302}
  \meshline{144,144,144}{0.053361331574}{1.032584619303}{0.053900949351}{1.018048144664}
  \meshline{144,144,144}{0.349851642418}{1.108059035943}{0.348468532151}{1.105227939238}
  \meshline{144,144,144}{0.255181755302}{1.096286914088}{0.257543474768}{1.105509904554}
  \meshline{144,144,144}{0.248442203956}{0.744370352385}{0.266998534883}{0.740793219301}
  \meshline{144,144,144}{0.152922985722}{1.129859234647}{0.158405602609}{1.147844842671}
  \meshline{144,144,144}{0.314880407107}{1.296305510386}{0.297197402637}{1.289315071529}
  \meshline{144,144,144}{0.331942377157}{1.302009643996}{0.316668117244}{1.296832244877}
  \meshline{144,144,144}{0.257543474768}{1.105509904554}{0.264128106482}{1.123124802638}
  \meshline{144,144,144}{0.252457018232}{1.085043707435}{0.255181755302}{1.096286914088}
  \meshline{144,144,144}{0.275060203110}{1.144817016264}{0.284964429140}{1.159850771179}
  \meshline{144,144,144}{0.264128106482}{1.123124802638}{0.266619183318}{1.128977409753}
  \meshline{144,144,144}{0.266619183318}{1.128977409753}{0.274128470455}{1.143091970710}
  \meshline{144,144,144}{0.284964429140}{1.159850771179}{0.285687065256}{1.160872393679}
  \meshline{144,144,144}{0.307119184810}{1.185379694665}{0.297170613752}{1.175002515405}
  \meshline{144,144,144}{0.307119184810}{1.185379694665}{0.318199494023}{1.195275606947}
  \meshline{144,144,144}{0.165041077006}{1.164715263502}{0.171937426126}{1.180290439872}
  \meshline{144,144,144}{0.158405602609}{1.147844842671}{0.163919294672}{1.162247390187}
  \meshline{144,144,144}{0.164376442905}{1.163396267144}{0.163919294672}{1.162247390187}
  \meshline{144,144,144}{0.164376442905}{1.163396267144}{0.165041077006}{1.164715263502}
  \meshline{144,144,144}{0.275060203110}{1.144817016264}{0.274128470455}{1.143091970710}
  \meshline{144,144,144}{0.287349580125}{1.162898982256}{0.297170613752}{1.175002515405}
  \meshline{144,144,144}{0.171937426126}{1.180290439872}{0.177417579187}{1.189468149362}
  \meshline{144,144,144}{0.207445867265}{1.230492814020}{0.201020354805}{1.222893619023}
  \meshline{144,144,144}{0.197467782539}{1.219098147876}{0.193791209667}{1.214100097803}
  \meshline{144,144,144}{0.185487546378}{1.202656229620}{0.181315515527}{1.196721198170}
  \meshline{144,144,144}{0.381009260463}{1.231849338953}{0.371212396730}{1.227900207533}
  \meshline{144,144,144}{0.314880407107}{1.296305510386}{0.316668117244}{1.296832244877}
  \meshline{144,144,144}{0.275631443041}{1.357678512734}{0.281864422809}{1.358886783817}
  \meshline{144,144,144}{0.297197402637}{1.289315071529}{0.290299985949}{1.286744863142}
  \meshline{144,144,144}{0.271413587333}{1.277630290861}{0.277390549879}{1.280494849366}
  \meshline{144,144,144}{0.321749429415}{1.198334609468}{0.318199494023}{1.195275606947}
  \meshline{144,144,144}{0.351841365326}{1.218050147784}{0.335693026211}{1.208365954514}
  \meshline{144,144,144}{0.321749429415}{1.198334609468}{0.331849231717}{1.205791610244}
  \meshline{144,144,144}{0.257725607553}{1.270055676237}{0.268897065948}{1.276089634371}
  \meshline{144,144,144}{0.245765727847}{1.262159537959}{0.234053416233}{1.254198289150}
  \meshline{144,144,144}{0.197467782539}{1.219098147876}{0.201020354805}{1.222893619023}
  \meshline{144,144,144}{0.207445867265}{1.230492814020}{0.216220767864}{1.238684434691}
  \meshline{144,144,144}{0.066236974633}{1.185601065418}{0.070079674016}{1.200818841620}
  \meshline{144,144,144}{0.285687065256}{1.160872393679}{0.287349580125}{1.162898982256}
  \meshline{144,144,144}{0.351841365326}{1.218050147784}{0.355368005771}{1.220129721748}
  \meshline{144,144,144}{0.388918565796}{1.234835707274}{0.386506756453}{1.234076964613}
  \meshline{144,144,144}{0.368023101221}{1.226263225119}{0.355368005771}{1.220129721748}
  \meshline{144,144,144}{0.381009260463}{1.231849338953}{0.386506756453}{1.234076964613}
  \meshline{144,144,144}{0.368023101221}{1.226263225119}{0.371212396730}{1.227900207533}
  \meshline{144,144,144}{0.216220767864}{1.238684434691}{0.222525230438}{1.244805877849}
  \meshline{144,144,144}{0.257725607553}{1.270055676237}{0.247093985603}{1.263106509265}
  \meshline{144,144,144}{0.249657598618}{1.352697690042}{0.254989196731}{1.353979116729}
  \meshline{144,144,144}{0.331849231717}{1.205791610244}{0.335693026211}{1.208365954514}
  \meshline{144,144,144}{0.185487546378}{1.202656229620}{0.193791209667}{1.214100097803}
  \meshline{144,144,144}{0.064251844615}{1.176679807118}{0.063286923723}{1.170588934765}
  \meshline{144,144,144}{0.227940143310}{1.249034215176}{0.222525230438}{1.244805877849}
  \meshline{144,144,144}{0.234053416233}{1.254198289150}{0.227940143310}{1.249034215176}
  \meshline{144,144,144}{0.268897065948}{1.276089634371}{0.271413587333}{1.277630290861}
  \meshline{144,144,144}{0.245765727847}{1.262159537959}{0.247093985603}{1.263106509265}
  \meshline{144,144,144}{0.257739999521}{1.354651581183}{0.275631443041}{1.357678512734}
  \meshline{144,144,144}{0.212256048806}{1.343297572648}{0.203219658162}{1.340943472389}
  \meshline{144,144,144}{0.057246783908}{1.129233196829}{0.057030163351}{1.126166220089}
  \meshline{144,144,144}{0.061561468845}{1.161841530176}{0.059964658556}{1.149571213538}
  \meshline{144,144,144}{0.091956732516}{1.257023343987}{0.088005675977}{1.248679397717}
  \meshline{144,144,144}{0.066236974633}{1.185601065418}{0.064251844615}{1.176679807118}
  \meshline{144,144,144}{0.073330911647}{1.213353894458}{0.079034299950}{1.228787580407}
  \meshline{144,144,144}{0.159675613406}{1.322201156280}{0.155282101779}{1.320286385539}
  \meshline{144,144,144}{0.152062598053}{1.126902683302}{0.147381020623}{1.104946666677}
  \meshline{144,144,144}{0.257739999521}{1.354651581183}{0.254989196731}{1.353979116729}
  \meshline{144,144,144}{0.238069108939}{1.350407052337}{0.227192399002}{1.347974159610}
  \meshline{144,144,144}{0.249657598618}{1.352697690042}{0.238069108939}{1.350407052337}
  \meshline{144,144,144}{0.227192399002}{1.347974159610}{0.212256048806}{1.343297572648}
  \meshline{144,144,144}{0.203219658162}{1.340943472389}{0.186259836420}{1.334750536772}
  \meshline{144,144,144}{0.159675613406}{1.322201156280}{0.173909453081}{1.329914199405}
  \meshline{144,144,144}{0.173909453081}{1.329914199405}{0.182411429575}{1.333088779390}
  \meshline{144,144,144}{0.182411429575}{1.333088779390}{0.186259836420}{1.334750536772}
  \meshline{144,144,144}{0.131159682497}{1.303824216131}{0.135901374029}{1.307336055348}
  \meshline{144,144,144}{0.150825193036}{1.317553912561}{0.155282101779}{1.320286385539}
  \meshline{144,144,144}{0.150825193036}{1.317553912561}{0.135901374029}{1.307336055348}
  \meshline{144,144,144}{0.131159682497}{1.303824216131}{0.117525351855}{1.290772324944}
  \meshline{144,144,144}{0.113135275125}{1.286424783142}{0.101749525480}{1.272331239160}
  \meshline{144,144,144}{0.113135275125}{1.286424783142}{0.114101342713}{1.287623977348}
  \meshline{144,144,144}{0.101749525480}{1.272331239160}{0.097683509144}{1.266143211510}
  \meshline{144,144,144}{0.114101342713}{1.287623977348}{0.117525351855}{1.290772324944}
  \meshline{144,144,144}{0.091956732516}{1.257023343987}{0.097683509144}{1.266143211510}
  \meshline{144,144,144}{0.073330911647}{1.213353894458}{0.070079674016}{1.200818841620}
  \meshline{144,144,144}{0.079960363908}{1.231423669710}{0.079034299950}{1.228787580407}
  \meshline{144,144,144}{0.079960363908}{1.231423669710}{0.088005675977}{1.248679397717}
  \meshline{144,144,144}{0.181315515527}{1.196721198170}{0.177417579187}{1.189468149362}
  \meshline{144,144,144}{0.281864422809}{1.358886783817}{0.295124500515}{1.360833947747}
\end{pgfscope}


==> nodal_rect_D0.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.4, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshtriangle{168,0,57}{1.000000000000}{0.015625000000}{0.984375000000}{0.000000000000}{1.000000000000}{0.000000000000}
  \meshline{168,0,57}{0.984375000000}{0.000000000000}{1.000000000000}{0.015625000000}
  \meshline{168,0,57}{0.788552805548}{0.706013892961}{0.806954449178}{0.706229317430}
  \meshline{168,0,57}{0.752281643889}{0.705543793928}{0.756730951235}{0.705576895997}
  \meshline{168,0,57}{0.731764739147}{0.705089196699}{0.733237620797}{0.705014513498}
  \meshline{168,0,57}{0.694557689386}{0.704433315312}{0.675558667626}{0.703889685901}
  \meshline{168,0,57}{0.769790978146}{0.705535322971}{0.775461586552}{0.705464766405}
  \meshline{168,0,57}{0.698545299311}{0.704273137125}{0.703048278742}{0.704213193991}
  \meshline{168,0,57}{0.703048278742}{0.704213193991}{0.731764739147}{0.705089196699}
  \meshline{168,0,57}{0.751118122443}{0.705429017531}{0.752281643889}{0.705543793928}
  \meshline{168,0,57}{0.733237620797}{0.705014513498}{0.744247571013}{0.705301794285}
  \meshline{168,0,57}{0.769790978146}{0.705535322971}{0.756730951235}{0.705576895997}
  \meshline{168,0,57}{0.784940508964}{0.705567146328}{0.788552805548}{0.706013892961}
  \meshline{168,0,57}{0.356694775179}{0.697795652690}{0.371365047992}{0.698140580807}
  \meshline{168,0,57}{0.694557689386}{0.704433315312}{0.698545299311}{0.704273137125}
  \meshline{168,0,57}{0.632641671653}{0.703293183635}{0.627565340374}{0.703116217321}
  \meshline{168,0,57}{0.584774847243}{0.702370443278}{0.575594428959}{0.702102623299}
  \meshline{168,0,57}{0.594462858675}{0.702376554353}{0.584774847243}{0.702370443278}
  \meshline{168,0,57}{0.632641671653}{0.703293183635}{0.646867663627}{0.703636473544}
  \meshline{168,0,57}{0.607547685511}{0.702802558310}{0.613437432772}{0.702720271168}
  \meshline{168,0,57}{0.624824701782}{0.703003023586}{0.613437432772}{0.702720271168}
  \meshline{168,0,57}{0.646867663627}{0.703636473544}{0.653622049588}{0.703467538166}
  \meshline{168,0,57}{0.624824701782}{0.703003023586}{0.627565340374}{0.703116217321}
  \meshline{168,0,57}{0.671177176935}{0.704038514055}{0.675558667626}{0.703889685901}
  \meshline{168,0,57}{0.607547685511}{0.702802558310}{0.594462858675}{0.702376554353}
  \meshline{168,0,57}{0.671177176935}{0.704038514055}{0.653622049588}{0.703467538166}
  \meshline{168,0,57}{0.528820391113}{0.701114889104}{0.554628880128}{0.701670311344}
  \meshline{168,0,57}{0.557308753553}{0.701747140091}{0.555899856477}{0.701710439544}
  \meshline{168,0,57}{0.557308753553}{0.701747140091}{0.575594428959}{0.702102623299}
  \meshline{168,0,57}{0.555899856477}{0.701710439544}{0.555430230274}{0.701690874458}
  \meshline{168,0,57}{0.528820391113}{0.701114889104}{0.520802375171}{0.700932225082}
  \meshline{168,0,57}{0.555430230274}{0.701690874458}{0.554628880128}{0.701670311344}
  \meshline{168,0,57}{0.847586898640}{0.706993589645}{0.853087090979}{0.706490816007}
  \meshline{168,0,57}{0.832240085351}{0.705914428551}{0.847586898640}{0.706993589645}
  \meshline{168,0,57}{0.907279051191}{0.707358896116}{0.919787003427}{0.707588825141}
  \meshline{168,0,57}{0.822796134424}{0.706599179713}{0.832240085351}{0.705914428551}
  \meshline{168,0,57}{0.941451912158}{0.708212290753}{0.951254823602}{0.706032400491}
  \meshline{168,0,57}{0.874318501563}{0.707131852730}{0.894829495568}{0.706650552916}
  \meshline{168,0,57}{0.899175772508}{0.707233613394}{0.897346359055}{0.706871412780}
  \meshline{168,0,57}{0.784940508964}{0.705567146328}{0.775461586552}{0.705464766405}
  \meshline{168,0,57}{0.822796134424}{0.706599179713}{0.808484006153}{0.706356076290}
  \meshline{168,0,57}{0.808484006153}{0.706356076290}{0.807454631993}{0.706300204583}
  \meshline{168,0,57}{0.807454631993}{0.706300204583}{0.806954449178}{0.706229317430}
  \meshline{168,0,57}{0.961647553134}{0.707889137565}{0.951254823602}{0.706032400491}
  \meshline{168,0,57}{0.751118122443}{0.705429017531}{0.744247571013}{0.705301794285}
  \meshline{168,0,57}{0.961647553134}{0.707889137565}{0.972514329535}{0.706113765394}
  \meshline{168,0,57}{0.894829495568}{0.706650552916}{0.897346359055}{0.706871412780}
  \meshline{168,0,57}{0.853087090979}{0.706490816007}{0.860475213778}{0.706224317283}
  \meshline{168,0,57}{0.860475213778}{0.706224317283}{0.874318501563}{0.707131852730}
  \meshline{168,0,57}{0.972514329535}{0.706113765394}{0.981822143479}{0.705826073687}
  \meshline{168,0,57}{0.919787003427}{0.707588825141}{0.923254251412}{0.706976557028}
  \meshline{168,0,57}{0.923254251412}{0.706976557028}{0.941451912158}{0.708212290753}
  \meshline{168,0,57}{0.907279051191}{0.707358896116}{0.899175772508}{0.707233613394}
  \meshline{168,0,57}{1.000000000000}{0.721875000000}{0.981822143479}{0.705826073687}
  \meshline{168,0,57}{0.396071319671}{0.698568547955}{0.374326753447}{0.698085476457}
  \meshline{168,0,57}{0.430641498973}{0.699152599173}{0.419643778340}{0.699025323100}
  \meshline{168,0,57}{0.320518214302}{0.697357726360}{0.310667124252}{0.697303076446}
  \meshline{168,0,57}{0.371365047992}{0.698140580807}{0.374326753447}{0.698085476457}
  \meshline{168,0,57}{0.414800392875}{0.698861152422}{0.419643778340}{0.699025323100}
  \meshline{168,0,57}{0.396071319671}{0.698568547955}{0.397464827544}{0.698552327197}
  \meshline{168,0,57}{0.401550897985}{0.698613974958}{0.397464827544}{0.698552327197}
  \meshline{168,0,57}{0.414800392875}{0.698861152422}{0.401550897985}{0.698613974958}
  \meshline{168,0,57}{0.452284316805}{0.699647280803}{0.468480162953}{0.699937444762}
  \meshline{168,0,57}{0.430641498973}{0.699152599173}{0.447473588207}{0.699533058408}
  \meshline{168,0,57}{0.452284316805}{0.699647280803}{0.449061777434}{0.699581515108}
  \meshline{168,0,57}{0.449061777434}{0.699581515108}{0.447473588207}{0.699533058408}
  \meshline{168,0,57}{0.471241992999}{0.699974070836}{0.468480162953}{0.699937444762}
  \meshline{168,0,57}{0.511955169698}{0.700766569534}{0.520802375171}{0.700932225082}
  \meshline{168,0,57}{0.497094766206}{0.700499448830}{0.493817123386}{0.700446495061}
  \meshline{168,0,57}{0.497094766206}{0.700499448830}{0.500960493331}{0.700583558529}
  \meshline{168,0,57}{0.500960493331}{0.700583558529}{0.511955169698}{0.700766569534}
  \meshline{168,0,57}{0.471241992999}{0.699974070836}{0.481289408984}{0.700167881300}
  \meshline{168,0,57}{0.481289408984}{0.700167881300}{0.493817123386}{0.700446495061}
  \meshline{168,0,57}{0.339714487825}{0.697487966523}{0.343856473391}{0.697639822298}
  \meshline{168,0,57}{0.324601172447}{0.697203780022}{0.320518214302}{0.697357726360}
  \meshline{168,0,57}{0.324601172447}{0.697203780022}{0.336549898383}{0.697384908249}
  \meshline{168,0,57}{0.339714487825}{0.697487966523}{0.336549898383}{0.697384908249}
  \meshline{168,0,57}{0.356694775179}{0.697795652690}{0.343856473391}{0.697639822298}
  \meshline{168,0,57}{0.061895397679}{0.693626320702}{0.056635578554}{0.693859517453}
  \meshline{168,0,57}{0.032739989702}{0.694515996353}{0.034102406968}{0.694538391124}
  \meshline{168,0,57}{0.083699819059}{0.695230126295}{0.078959071667}{0.694832676112}
  \meshline{168,0,57}{0.074814007141}{0.693756905018}{0.078959071667}{0.694832676112}
  \meshline{168,0,57}{0.099745831883}{0.694343697818}{0.083699819059}{0.695230126295}
  \meshline{168,0,57}{0.127876967908}{0.695013683171}{0.117456571031}{0.694275005506}
  \meshline{168,0,57}{0.074814007141}{0.693756905018}{0.061895397679}{0.693626320702}
  \meshline{168,0,57}{0.054052032351}{0.694814792161}{0.034102406968}{0.694538391124}
  \meshline{168,0,57}{0.054052032351}{0.694814792161}{0.056635578554}{0.693859517453}
  \meshline{168,0,57}{0.030221242090}{0.694356928078}{0.016419033480}{0.694916988514}
  \meshline{168,0,57}{0.032358371843}{0.694302119677}{0.030221242090}{0.694356928078}
  \meshline{168,0,57}{0.000000000000}{0.696875000000}{0.016419033480}{0.694916988514}
  \meshline{168,0,57}{0.032739989702}{0.694515996353}{0.032358371843}{0.694302119677}
  \meshline{168,0,57}{0.108312948057}{0.693653009652}{0.117456571031}{0.694275005506}
  \meshline{168,0,57}{0.154291087150}{0.695035571111}{0.151906489989}{0.695259680757}
  \meshline{168,0,57}{0.161583850075}{0.694873998485}{0.176870055541}{0.695061674813}
  \meshline{168,0,57}{0.151906489989}{0.695259680757}{0.134284337862}{0.694433152060}
  \meshline{168,0,57}{0.127876967908}{0.695013683171}{0.134284337862}{0.694433152060}
  \meshline{168,0,57}{0.108312948057}{0.693653009652}{0.099745831883}{0.694343697818}
  \meshtriangle{168,0,57}{0.000000000000}{0.000000000000}{0.015625000000}{0.000000000000}{0.000000000000}{0.031250000000}
  \meshline{168,0,57}{0.015625000000}{0.000000000000}{0.000000000000}{0.031250000000}
  \meshline{168,0,57}{0.256108565443}{0.696098595307}{0.242412968858}{0.695788914926}
  \meshline{168,0,57}{0.259256990086}{0.696217552399}{0.260458539209}{0.696295675523}
  \meshline{168,0,57}{0.298590100150}{0.697097061872}{0.310667124252}{0.697303076446}
  \meshline{168,0,57}{0.285868278356}{0.696298219065}{0.293374693413}{0.696732858417}
  \meshline{168,0,57}{0.185904940693}{0.695573630564}{0.197311860586}{0.695535960481}
  \meshline{168,0,57}{0.260458539209}{0.696295675523}{0.274902961466}{0.696517825534}
  \meshline{168,0,57}{0.256108565443}{0.696098595307}{0.259256990086}{0.696217552399}
  \meshline{168,0,57}{0.242412968858}{0.695788914926}{0.236144893776}{0.696177476125}
  \meshline{168,0,57}{0.176870055541}{0.695061674813}{0.185904940693}{0.695573630564}
  \meshline{168,0,57}{0.207688382534}{0.695524061338}{0.213271775628}{0.695813585365}
  \meshline{168,0,57}{0.221817787846}{0.695960029922}{0.236144893776}{0.696177476125}
  \meshline{168,0,57}{0.207688382534}{0.695524061338}{0.197311860586}{0.695535960481}
  \meshline{168,0,57}{0.221817787846}{0.695960029922}{0.213271775628}{0.695813585365}
  \meshline{168,0,57}{0.161583850075}{0.694873998485}{0.154291087150}{0.695035571111}
  \meshline{168,0,57}{0.285868278356}{0.696298219065}{0.274902961466}{0.696517825534}
  \meshline{168,0,57}{0.293374693413}{0.696732858417}{0.298590100150}{0.697097061872}
  \meshtriangle{168,0,57}{0.984375000000}{1.400000000000}{1.000000000000}{1.378125000000}{1.000000000000}{1.400000000000}
  \meshline{168,0,57}{1.000000000000}{1.378125000000}{0.984375000000}{1.400000000000}
  \meshline{168,0,57}{0.015625000000}{1.400000000000}{0.000000000000}{1.371875000000}
  \meshtriangle{168,0,57}{0.000000000000}{1.371875000000}{0.015625000000}{1.400000000000}{0.000000000000}{1.400000000000}
\end{pgfscope}


==> nodal_rect_N.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.9, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{144,144,144}{0.082182505951}{1.118839040191}{0.105900868634}{1.118838996359}
  \meshline{144,144,144}{0.018523224300}{1.118827019874}{0.039852700500}{1.118831048871}
  \meshline{144,144,144}{0.151206280880}{0.780622333812}{0.133431204883}{0.780618048812}
  \meshline{144,144,144}{0.198421835315}{0.780650098748}{0.184186349948}{0.780632693608}
  \meshline{144,144,144}{0.279586396361}{1.118929567817}{0.272938755121}{1.118919753319}
  \meshline{144,144,144}{0.165155242381}{1.118867518313}{0.152228040343}{1.118850053407}
  \meshline{144,144,144}{0.119080935093}{1.118832966584}{0.135693941009}{1.118833309216}
  \meshline{144,144,144}{0.135693941009}{1.118833309216}{0.152228040343}{1.118850053407}
  \meshline{144,144,144}{0.119080935093}{1.118832966584}{0.105900868634}{1.118838996359}
  \meshline{144,144,144}{0.232091658403}{1.118900579687}{0.204316812333}{1.118887592659}
  \meshline{144,144,144}{0.186672643756}{1.118883874799}{0.165155242381}{1.118867518313}
  \meshline{144,144,144}{0.155744954220}{1.284962940763}{0.146382982143}{1.284958328621}
  \meshline{144,144,144}{0.143416432501}{1.284955801468}{0.116458656001}{1.284942349206}
  \meshline{144,144,144}{0.182613883458}{1.284977750986}{0.155744954220}{1.284962940763}
  \meshline{144,144,144}{0.200016243353}{1.284989258323}{0.191404626537}{1.284983878111}
  \meshline{144,144,144}{0.227628237673}{1.285009948516}{0.200016243353}{1.284989258323}
  \meshline{144,144,144}{0.254477541227}{1.285031390927}{0.263650845963}{1.285038473168}
  \meshline{144,144,144}{0.143416432501}{1.284955801468}{0.146382982143}{1.284958328621}
  \meshline{144,144,144}{0.080495183467}{1.284929927450}{0.103643894693}{1.284937690315}
  \meshline{144,144,144}{0.103643894693}{1.284937690315}{0.116458656001}{1.284942349206}
  \meshline{144,144,144}{0.182613883458}{1.284977750986}{0.191404626537}{1.284983878111}
  \meshline{144,144,144}{0.331531550450}{1.118973730767}{0.304590545191}{1.118939517454}
  \meshline{144,144,144}{0.186672643756}{1.118883874799}{0.197491324014}{1.118880483901}
  \meshline{144,144,144}{0.263650845963}{1.285038473168}{0.300319567404}{1.285077899741}
  \meshline{144,144,144}{0.064767055130}{1.284925946224}{0.045582732785}{1.284921316595}
  \meshline{144,144,144}{0.018523224300}{1.118827019874}{0.000000000000}{1.118805241786}
  \meshline{144,144,144}{0.056994750961}{1.118826997172}{0.039852700500}{1.118831048871}
  \meshline{144,144,144}{0.082182505951}{1.118839040191}{0.056994750961}{1.118826997172}
  \meshline{144,144,144}{0.254477541227}{1.285031390927}{0.227628237673}{1.285009948516}
  \meshline{144,144,144}{0.064767055130}{1.284925946224}{0.080495183467}{1.284929927450}
  \meshline{144,144,144}{0.019642193762}{1.284914498292}{0.030294120876}{1.284916185307}
  \meshline{144,144,144}{0.019642193762}{1.284914498292}{0.000000000000}{1.284910071644}
  \meshline{144,144,144}{0.045582732785}{1.284921316595}{0.030294120876}{1.284916185307}
  \meshline{144,144,144}{0.347498537893}{1.118984677684}{0.374949504376}{1.119018428183}
  \meshline{144,144,144}{0.272938755121}{1.118919753319}{0.254683736394}{1.118921236452}
  \meshline{144,144,144}{0.232091658403}{1.118900579687}{0.238390573358}{1.118899090786}
  \meshline{144,144,144}{0.374949504376}{1.119018428183}{0.387305071165}{1.119036250050}
  \meshline{144,144,144}{0.410301812037}{1.119049530921}{0.435890751758}{1.119055687256}
  \meshline{144,144,144}{0.404376127793}{1.119042528880}{0.387305071165}{1.119036250050}
  \meshline{144,144,144}{0.238390573358}{1.118899090786}{0.254683736394}{1.118921236452}
  \meshline{144,144,144}{0.304590545191}{1.118939517454}{0.279586396361}{1.118929567817}
  \meshline{144,144,144}{0.197491324014}{1.118880483901}{0.204316812333}{1.118887592659}
  \meshline{144,144,144}{0.114233504902}{0.780610825648}{0.077776006856}{0.780589850675}
  \meshline{144,144,144}{0.151206280880}{0.780622333812}{0.184186349948}{0.780632693608}
  \meshline{144,144,144}{0.313426568892}{0.780713341726}{0.345511726162}{0.780753760074}
  \meshline{144,144,144}{0.308352581660}{0.780710875760}{0.306015514150}{0.780709681671}
  \meshline{144,144,144}{0.306015514150}{0.780709681671}{0.295826923563}{0.780697972188}
  \meshline{144,144,144}{0.276641706357}{0.780690504362}{0.295826923563}{0.780697972188}
  \meshline{144,144,144}{0.375852181181}{0.780764968371}{0.375173026190}{0.780764034344}
  \meshline{144,144,144}{0.331531550450}{1.118973730767}{0.347498537893}{1.118984677684}
  \meshline{144,144,144}{0.342265133472}{1.285126067406}{0.333389050398}{1.285114921641}
  \meshline{144,144,144}{0.300319567404}{1.285077899741}{0.302828884251}{1.285080061881}
  \meshline{144,144,144}{0.000000000000}{0.780578308606}{0.001401320412}{0.780577468946}
  \meshline{144,144,144}{0.001401320412}{0.780577468946}{0.035851505833}{0.780601599846}
  \meshline{144,144,144}{0.146822969952}{0.614291359497}{0.160721201377}{0.614300190677}
  \meshline{144,144,144}{0.057400789924}{0.780584444923}{0.064662512408}{0.780590619563}
  \meshline{144,144,144}{0.057400789924}{0.780584444923}{0.035851505833}{0.780601599846}
  \meshline{144,144,144}{0.064662512408}{0.780590619563}{0.077776006856}{0.780589850675}
  \meshline{144,144,144}{0.127177526412}{0.614285795655}{0.146822969952}{0.614291359497}
  \meshline{144,144,144}{0.114233504902}{0.780610825648}{0.133431204883}{0.780618048812}
  \meshline{144,144,144}{0.198421835315}{0.780650098748}{0.209289912903}{0.780649922092}
  \meshline{144,144,144}{0.268668734802}{0.780680339076}{0.276641706357}{0.780690504362}
  \meshline{144,144,144}{0.055635614730}{0.614250573763}{0.035092710741}{0.614245888015}
  \meshline{144,144,144}{0.268668734802}{0.780680339076}{0.236053118423}{0.780674822650}
  \meshline{144,144,144}{0.209289912903}{0.780649922092}{0.236053118423}{0.780674822650}
  \meshline{144,144,144}{0.376789397733}{0.780765582430}{0.375852181181}{0.780764968371}
  \meshline{144,144,144}{0.313426568892}{0.780713341726}{0.308352581660}{0.780710875760}
  \meshline{144,144,144}{0.375173026190}{0.780764034344}{0.345511726162}{0.780753760074}
  \meshline{144,144,144}{0.661162154593}{1.285538138057}{0.630954621951}{1.285504781724}
  \meshline{144,144,144}{0.522812632744}{1.285364102681}{0.501866424263}{1.285335745015}
  \meshline{144,144,144}{0.081929635131}{0.614264616078}{0.107234918924}{0.614280224214}
  \meshline{144,144,144}{0.333389050398}{1.285114921641}{0.302828884251}{1.285080061881}
  \meshline{144,144,144}{0.127177526412}{0.614285795655}{0.107234918924}{0.614280224214}
  \meshline{144,144,144}{0.181160088763}{0.614313195393}{0.205779548102}{0.614329878089}
  \meshline{144,144,144}{0.227813786286}{0.614350449799}{0.235753822470}{0.614356128710}
  \meshline{144,144,144}{0.181160088763}{0.614313195393}{0.160721201377}{0.614300190677}
  \meshline{144,144,144}{0.227813786286}{0.614350449799}{0.205779548102}{0.614329878089}
  \meshline{144,144,144}{0.139347475044}{1.644777453679}{0.140469891869}{1.644811349054}
  \meshline{144,144,144}{0.029703549557}{1.644618939354}{0.048559728112}{1.644840580726}
  \meshline{144,144,144}{0.029703549557}{1.644618939354}{0.000000000000}{1.644776616579}
  \meshline{144,144,144}{0.061253428863}{1.644758372008}{0.088806232620}{1.645311171441}
  \meshline{144,144,144}{0.061253428863}{1.644758372008}{0.051992371258}{1.644857445706}
  \meshline{144,144,144}{0.051992371258}{1.644857445706}{0.048559728112}{1.644840580726}
  \meshline{144,144,144}{0.088806232620}{1.645311171441}{0.097001426688}{1.645242806071}
  \meshline{144,144,144}{0.358867609518}{1.645692655586}{0.320955581627}{1.645317243388}
  \meshline{144,144,144}{0.358867609518}{1.645692655586}{0.364970027338}{1.645751846184}
  \meshline{144,144,144}{0.260429408672}{1.645177697598}{0.232294296677}{1.645686571984}
  \meshline{144,144,144}{0.318764282105}{1.645300603371}{0.320955581627}{1.645317243388}
  \meshline{144,144,144}{0.342265133472}{1.285126067406}{0.372169652906}{1.285163805231}
  \meshline{144,144,144}{0.035092710741}{0.614245888015}{0.013472590926}{0.614244541545}
  \meshline{144,144,144}{0.081929635131}{0.614264616078}{0.070234936306}{0.614255567943}
  \meshline{144,144,144}{0.055635614730}{0.614250573763}{0.070234936306}{0.614255567943}
  \meshline{144,144,144}{0.013472590926}{0.614244541545}{0.000000000000}{0.614243398484}
  \meshline{144,144,144}{0.298279247964}{0.614421444175}{0.296255767473}{0.614418491152}
  \meshline{144,144,144}{0.358945896535}{0.614494549374}{0.355550552426}{0.614490883112}
  \meshline{144,144,144}{0.269985878410}{0.614388163710}{0.242439633818}{0.614364464296}
  \meshline{144,144,144}{0.355550552426}{0.614490883112}{0.354624169814}{0.614489669702}
  \meshline{144,144,144}{0.269985878410}{0.614388163710}{0.296255767473}{0.614418491152}
  \meshline{144,144,144}{0.301765570297}{0.614424478766}{0.328825117355}{0.614457211773}
  \meshline{144,144,144}{0.423055675886}{0.614566941379}{0.399825713781}{0.614539583945}
  \meshline{144,144,144}{0.457715241140}{0.614613788016}{0.472984227782}{0.614633071015}
  \meshline{144,144,144}{0.556328003854}{0.780949275614}{0.522212525535}{0.780912985522}
  \meshline{144,144,144}{0.299508200310}{0.614422706983}{0.298279247964}{0.614421444175}
  \meshline{144,144,144}{0.328825117355}{0.614457211773}{0.354624169814}{0.614489669702}
  \meshline{144,144,144}{0.474315033557}{0.780881175404}{0.454354565487}{0.780848719600}
  \meshline{144,144,144}{0.454354565487}{0.780848719600}{0.437986206013}{0.780837366898}
  \meshline{144,144,144}{0.376789397733}{0.780765582430}{0.415762701264}{0.780822561088}
  \meshline{144,144,144}{0.415762701264}{0.780822561088}{0.437986206013}{0.780837366898}
  \meshline{144,144,144}{0.512126301380}{0.780917650486}{0.503241133994}{0.780897173233}
  \meshline{144,144,144}{0.474315033557}{0.780881175404}{0.503241133994}{0.780897173233}
  \meshline{144,144,144}{0.522212525535}{0.780912985522}{0.512126301380}{0.780917650486}
  \meshline{144,144,144}{0.587255332449}{0.780992357356}{0.606281130141}{0.781010433639}
  \meshline{144,144,144}{0.556328003854}{0.780949275614}{0.569992539774}{0.780963001654}
  \meshline{144,144,144}{0.507737203551}{0.614681413187}{0.536150244215}{0.614717676521}
  \meshline{144,144,144}{0.650669225566}{0.614866781368}{0.667602696632}{0.614886587931}
  \meshline{144,144,144}{0.536150244215}{0.614717676521}{0.554202785503}{0.614743593448}
  \meshline{144,144,144}{0.457715241140}{0.614613788016}{0.428516573663}{0.614577231805}
  \meshline{144,144,144}{0.358945896535}{0.614494549374}{0.392897796761}{0.614533317344}
  \meshline{144,144,144}{0.399825713781}{0.614539583945}{0.392897796761}{0.614533317344}
  \meshline{144,144,144}{0.472984227782}{0.614633071015}{0.496731325830}{0.614666788665}
  \meshline{144,144,144}{0.502791776482}{0.614675558917}{0.507737203551}{0.614681413187}
  \meshline{144,144,144}{0.502791776482}{0.614675558917}{0.496731325830}{0.614666788665}
  \meshline{144,144,144}{0.423055675886}{0.614566941379}{0.428516573663}{0.614577231805}
  \meshline{144,144,144}{0.268114392493}{1.645214900139}{0.265031698952}{1.645266432012}
  \meshline{144,144,144}{0.188370435399}{1.645510545623}{0.213275923435}{1.645460483740}
  \meshline{144,144,144}{0.188370435399}{1.645510545623}{0.171924578362}{1.645006478299}
  \meshline{144,144,144}{0.141561898423}{1.644802927141}{0.169372016084}{1.645080571836}
  \meshline{144,144,144}{0.141561898423}{1.644802927141}{0.140469891869}{1.644811349054}
  \meshline{144,144,144}{0.169372016084}{1.645080571836}{0.171924578362}{1.645006478299}
  \meshline{144,144,144}{0.097001426688}{1.645242806071}{0.139347475044}{1.644777453679}
  \meshline{144,144,144}{0.398073956282}{1.646092158857}{0.391767124399}{1.645992282768}
  \meshline{144,144,144}{0.299508200310}{0.614422706983}{0.301765570297}{0.614424478766}
  \meshline{144,144,144}{0.587255332449}{0.780992357356}{0.569992539774}{0.780963001654}
  \meshline{144,144,144}{0.627568179080}{0.781014136795}{0.606281130141}{0.781010433639}
  \meshline{144,144,144}{0.527382661242}{1.119131212340}{0.546592839848}{1.119153342966}
  \meshline{144,144,144}{0.410301812037}{1.119049530921}{0.404376127793}{1.119042528880}
  \meshline{144,144,144}{0.527382661242}{1.119131212340}{0.505459180235}{1.119130736628}
  \meshline{144,144,144}{0.435890751758}{1.119055687256}{0.449708028373}{1.119083915621}
  \meshline{144,144,144}{0.631972389775}{1.119249491073}{0.641580527599}{1.119264483357}
  \meshline{144,144,144}{0.465671665947}{1.119094901753}{0.496581479473}{1.119123387066}
  \meshline{144,144,144}{0.496581479473}{1.119123387066}{0.505459180235}{1.119130736628}
  \meshline{144,144,144}{0.449708028373}{1.119083915621}{0.465671665947}{1.119094901753}
  \meshline{144,144,144}{0.561377042978}{1.119182352935}{0.574496224740}{1.119196844144}
  \meshline{144,144,144}{0.596641866076}{0.614798090577}{0.602396418119}{0.614805335755}
  \meshline{144,144,144}{0.591196183384}{0.614791514268}{0.596641866076}{0.614798090577}
  \meshline{144,144,144}{0.569846786410}{0.614766848706}{0.554202785503}{0.614743593448}
  \meshline{144,144,144}{0.569846786410}{0.614766848706}{0.591196183384}{0.614791514268}
  \meshline{144,144,144}{0.747725260225}{0.614973288575}{0.750708613139}{0.614977647709}
  \meshline{144,144,144}{0.683566674848}{0.781077280616}{0.671511172765}{0.781071925936}
  \meshline{144,144,144}{0.671511172765}{0.781071925936}{0.649188235496}{0.781032153856}
  \meshline{144,144,144}{0.632004254759}{0.614838513489}{0.650669225566}{0.614866781368}
  \meshline{144,144,144}{0.213275923435}{1.645460483740}{0.232294296677}{1.645686571984}
  \meshline{144,144,144}{0.260429408672}{1.645177697598}{0.265031698952}{1.645266432012}
  \meshline{144,144,144}{0.294071715816}{1.646051961097}{0.318764282105}{1.645300603371}
  \meshline{144,144,144}{0.425651196147}{1.646130952840}{0.398073956282}{1.646092158857}
  \meshline{144,144,144}{0.471100184734}{1.285292205480}{0.481487766384}{1.285307070341}
  \meshline{144,144,144}{0.419640976646}{1.285227661424}{0.406091934045}{1.285213030444}
  \meshline{144,144,144}{0.460092848229}{1.285278909270}{0.471100184734}{1.285292205480}
  \meshline{144,144,144}{0.391767124399}{1.645992282768}{0.364970027338}{1.645751846184}
  \meshline{144,144,144}{0.610207112216}{1.285476034336}{0.605561636470}{1.285469946911}
  \meshline{144,144,144}{0.712567822598}{1.285591526622}{0.709886658628}{1.285588961033}
  \meshline{144,144,144}{0.572041802147}{1.285423962390}{0.535729214744}{1.285378516490}
  \meshline{144,144,144}{0.572041802147}{1.285423962390}{0.576646876776}{1.285429512879}
  \meshline{144,144,144}{0.605561636470}{1.285469946911}{0.576646876776}{1.285429512879}
  \meshline{144,144,144}{0.630954621951}{1.285504781724}{0.610207112216}{1.285476034336}
  \meshline{144,144,144}{0.522812632744}{1.285364102681}{0.535729214744}{1.285378516490}
  \meshline{144,144,144}{0.481487766384}{1.285307070341}{0.501866424263}{1.285335745015}
  \meshline{144,144,144}{0.460092848229}{1.285278909270}{0.437560847289}{1.285247347674}
  \meshline{144,144,144}{0.406091934045}{1.285213030444}{0.392344869285}{1.285191101165}
  \meshline{144,144,144}{0.235753822470}{0.614356128710}{0.242439633818}{0.614364464296}
  \meshline{144,144,144}{0.570198937971}{0.253773455026}{0.559690278740}{0.253934026120}
  \meshline{144,144,144}{0.440194848966}{0.253627640483}{0.443515024423}{0.253600344863}
  \meshline{144,144,144}{0.886640631631}{0.254780394395}{0.898688479732}{0.255008164080}
  \meshline{144,144,144}{0.799433148725}{1.119380489058}{0.801913627117}{1.119379720718}
  \meshline{144,144,144}{0.627568179080}{0.781014136795}{0.636993247597}{0.781028865757}
  \meshline{144,144,144}{0.636993247597}{0.781028865757}{0.649188235496}{0.781032153856}
  \meshline{144,144,144}{0.683566674848}{0.781077280616}{0.704604381241}{0.781060144121}
  \meshline{144,144,144}{0.720138595377}{0.614945875881}{0.715767523412}{0.614940277812}
  \meshline{144,144,144}{0.731122292247}{0.781100724879}{0.749903758290}{0.781105279198}
  \meshline{144,144,144}{0.882902602152}{0.781179264627}{0.872566554642}{0.781166386808}
  \meshline{144,144,144}{0.756844266841}{0.781114348354}{0.782923172625}{0.781118010646}
  \meshline{144,144,144}{0.701477485926}{1.119316929965}{0.703621173945}{1.119317122580}
  \meshline{144,144,144}{0.706314423109}{0.781060721250}{0.704604381241}{0.781060144121}
  \meshline{144,144,144}{0.681414557167}{0.614901739908}{0.697524493819}{0.614918709602}
  \meshline{144,144,144}{0.632004254759}{0.614838513489}{0.602396418119}{0.614805335755}
  \meshline{144,144,144}{0.294071715816}{1.646051961097}{0.268114392493}{1.645214900139}
  \meshline{144,144,144}{0.419640976646}{1.285227661424}{0.437560847289}{1.285247347674}
  \meshline{144,144,144}{0.372169652906}{1.285163805231}{0.392344869285}{1.285191101165}
  \meshline{144,144,144}{0.558046937256}{1.646652674469}{0.544030568972}{1.646321112704}
  \meshline{144,144,144}{0.509423477508}{1.646143273101}{0.544030568972}{1.646321112704}
  \meshline{144,144,144}{0.667622007238}{1.646828939069}{0.671731415373}{1.646919640667}
  \meshline{144,144,144}{0.455448439202}{1.645907419511}{0.468816828168}{1.646213058694}
  \meshline{144,144,144}{0.642559282129}{1.647005640689}{0.628717429603}{1.646768004451}
  \meshline{144,144,144}{0.588626080025}{1.646646586485}{0.567401331987}{1.646418806882}
  \meshline{144,144,144}{0.609119994669}{1.646718846089}{0.628717429603}{1.646768004451}
  \meshline{144,144,144}{0.468816828168}{1.646213058694}{0.472569886015}{1.646331716130}
  \meshline{144,144,144}{0.642559282129}{1.647005640689}{0.667622007238}{1.646828939069}
  \meshline{144,144,144}{0.558046937256}{1.646652674469}{0.567401331987}{1.646418806882}
  \meshline{144,144,144}{0.434680681713}{1.645977971790}{0.455448439202}{1.645907419511}
  \meshline{144,144,144}{0.472569886015}{1.646331716130}{0.498098018865}{1.646461102772}
  \meshline{144,144,144}{0.609119994669}{1.646718846089}{0.588626080025}{1.646646586485}
  \meshline{144,144,144}{0.425651196147}{1.646130952840}{0.434680681713}{1.645977971790}
  \meshline{144,144,144}{0.498098018865}{1.646461102772}{0.509423477508}{1.646143273101}
  \meshline{144,144,144}{0.561377042978}{1.119182352935}{0.546592839848}{1.119153342966}
  \meshline{144,144,144}{0.599061133481}{1.119220797824}{0.574496224740}{1.119196844144}
  \meshline{144,144,144}{0.673146394294}{1.285550135551}{0.668381106655}{1.285545830775}
  \meshline{144,144,144}{0.599061133481}{1.119220797824}{0.621069371473}{1.119249289657}
  \meshline{144,144,144}{0.631972389775}{1.119249491073}{0.621069371473}{1.119249289657}
  \meshline{144,144,144}{0.661162154593}{1.285538138057}{0.668381106655}{1.285545830775}
  \meshline{144,144,144}{0.754625253943}{1.119343939380}{0.740413543296}{1.119331859311}
  \meshline{144,144,144}{0.641580527599}{1.119264483357}{0.666656116115}{1.119263006740}
  \meshline{144,144,144}{0.666656116115}{1.119263006740}{0.701477485926}{1.119316929965}
  \meshline{144,144,144}{0.443515024423}{0.253600344863}{0.447027182973}{0.253666365052}
  \meshline{144,144,144}{0.404163627276}{0.253157467084}{0.389060245664}{0.253300615681}
  \meshline{144,144,144}{0.679176013586}{0.254195607250}{0.690598544149}{0.254283235579}
  \meshline{144,144,144}{0.814493561390}{0.254836331920}{0.842352160457}{0.254759631626}
  \meshline{144,144,144}{0.833350523013}{0.781151771058}{0.824280501891}{0.781152491754}
  \meshline{144,144,144}{0.824280501891}{0.781152491754}{0.800816083732}{0.781126174473}
  \meshline{144,144,144}{0.833350523013}{0.781151771058}{0.854737956642}{0.781174460159}
  \meshline{144,144,144}{0.786182077123}{0.781120483180}{0.800816083732}{0.781126174473}
  \meshline{144,144,144}{0.749903758290}{0.781105279198}{0.756844266841}{0.781114348354}
  \meshline{144,144,144}{0.890007420980}{0.781173718269}{0.882902602152}{0.781179264627}
  \meshline{144,144,144}{0.731122292247}{0.781100724879}{0.706314423109}{0.781060721250}
  \meshline{144,144,144}{0.930495690113}{0.781191057133}{0.956992756164}{0.781199775728}
  \meshline{144,144,144}{0.930495690113}{0.781191057133}{0.922910123019}{0.781186183380}
  \meshline{144,144,144}{0.965455436152}{0.781208336474}{0.956992756164}{0.781199775728}
  \meshline{144,144,144}{1.000000000000}{0.781211327545}{0.994026272417}{0.781205892511}
  \meshline{144,144,144}{0.768395893062}{0.614993339513}{0.784663559745}{0.615006292683}
  \meshline{144,144,144}{0.697524493819}{0.614918709602}{0.715767523412}{0.614940277812}
  \meshline{144,144,144}{0.681414557167}{0.614901739908}{0.667602696632}{0.614886587931}
  \meshline{144,144,144}{0.738221049489}{0.614964395068}{0.720138595377}{0.614945875881}
  \meshline{144,144,144}{0.776531104411}{0.254602150961}{0.794687615212}{0.254867554687}
  \meshline{144,144,144}{0.959981825022}{0.254540629843}{0.995301061313}{0.255012564174}
  \meshline{144,144,144}{0.807350047546}{0.254694927101}{0.814493561390}{0.254836331920}
  \meshline{144,144,144}{0.807350047546}{0.254694927101}{0.794687615212}{0.254867554687}
  \meshline{144,144,144}{0.842352160457}{0.254759631626}{0.858733436449}{0.254871311230}
  \meshline{144,144,144}{0.858733436449}{0.254871311230}{0.880096502986}{0.254960353305}
  \meshline{144,144,144}{0.761848051372}{0.254564758462}{0.733268040816}{0.254593014202}
  \meshline{144,144,144}{0.776531104411}{0.254602150961}{0.761848051372}{0.254564758462}
  \meshline{144,144,144}{0.898688479732}{0.255008164080}{0.921050057026}{0.254689846273}
  \meshline{144,144,144}{0.944034297105}{0.254796934700}{0.921050057026}{0.254689846273}
  \meshline{144,144,144}{0.886640631631}{0.254780394395}{0.880096502986}{0.254960353305}
  \meshline{144,144,144}{0.959981825022}{0.254540629843}{0.944034297105}{0.254796934700}
  \meshline{144,144,144}{1.000000000000}{0.254902869880}{0.995301061313}{0.255012564174}
  \meshline{144,144,144}{0.930258350034}{1.119430882990}{0.941495937669}{1.119423250792}
  \meshline{144,144,144}{0.774889455314}{1.119340398938}{0.754625253943}{1.119343939380}
  \meshline{144,144,144}{0.890007420980}{0.781173718269}{0.922910123019}{0.781186183380}
  \meshline{144,144,144}{0.965455436152}{0.781208336474}{0.994026272417}{0.781205892511}
  \meshline{144,144,144}{0.782923172625}{0.781118010646}{0.786182077123}{0.781120483180}
  \meshline{144,144,144}{0.810125846433}{0.615025218440}{0.784663559745}{0.615006292683}
  \meshline{144,144,144}{0.888322881734}{0.615072068998}{0.913984992522}{0.615085526609}
  \meshline{144,144,144}{0.820287822442}{0.615031684023}{0.848647491396}{0.615049203624}
  \meshline{144,144,144}{0.872566554642}{0.781166386808}{0.854737956642}{0.781174460159}
  \meshline{144,144,144}{0.942719842555}{0.615092713420}{0.965879127823}{0.615097816986}
  \meshline{144,144,144}{0.965879127823}{0.615097816986}{0.978392306812}{0.615102491666}
  \meshline{144,144,144}{0.888322881734}{0.615072068998}{0.888176221529}{0.615071983316}
  \meshline{144,144,144}{0.849246649480}{0.615049536699}{0.888176221529}{0.615071983316}
  \meshline{144,144,144}{0.820287822442}{0.615031684023}{0.810125846433}{0.615025218440}
  \meshline{144,144,144}{0.849246649480}{0.615049536699}{0.848647491396}{0.615049203624}
  \meshline{144,144,144}{0.913984992522}{0.615085526609}{0.920339030328}{0.615086134562}
  \meshline{144,144,144}{0.747725260225}{0.614973288575}{0.738221049489}{0.614964395068}
  \meshline{144,144,144}{0.768395893062}{0.614993339513}{0.750708613139}{0.614977647709}
  \meshline{144,144,144}{0.029216703034}{0.252511512935}{0.027290264862}{0.252495959931}
  \meshline{144,144,144}{0.163550484208}{0.252544187380}{0.154268775535}{0.252675953262}
  \meshline{144,144,144}{0.708845030338}{0.254155527943}{0.690598544149}{0.254283235579}
  \meshline{144,144,144}{0.708845030338}{0.254155527943}{0.722588952991}{0.254578953977}
  \meshline{144,144,144}{0.679176013586}{0.254195607250}{0.652603097081}{0.254308457096}
  \meshline{144,144,144}{0.733268040816}{0.254593014202}{0.722588952991}{0.254578953977}
  \meshline{144,144,144}{0.645581892268}{0.254335766541}{0.649547167377}{0.254231428082}
  \meshline{144,144,144}{0.645581892268}{0.254335766541}{0.616123625890}{0.253711935488}
  \meshline{144,144,144}{0.570198937971}{0.253773455026}{0.597481822366}{0.254202963713}
  \meshline{144,144,144}{0.649547167377}{0.254231428082}{0.652603097081}{0.254308457096}
  \meshline{144,144,144}{0.495209257684}{0.253731623343}{0.477088646130}{0.253319891980}
  \meshline{144,144,144}{0.507646157973}{0.253881222986}{0.495209257684}{0.253731623343}
  \meshline{144,144,144}{0.559690278740}{0.253934026120}{0.528906331317}{0.253784817014}
  \meshline{144,144,144}{0.597481822366}{0.254202963713}{0.597666079921}{0.254201624346}
  \meshline{144,144,144}{0.447027182973}{0.253666365052}{0.477088646130}{0.253319891980}
  \meshline{144,144,144}{0.528906331317}{0.253784817014}{0.507646157973}{0.253881222986}
  \meshline{144,144,144}{0.616123625890}{0.253711935488}{0.597666079921}{0.254201624346}
  \meshline{144,144,144}{0.740413543296}{1.119331859311}{0.705558929493}{1.119319795681}
  \meshline{144,144,144}{0.703621173945}{1.119317122580}{0.705558929493}{1.119319795681}
  \meshline{144,144,144}{0.799433148725}{1.119380489058}{0.774889455314}{1.119340398938}
  \meshline{144,144,144}{0.835612097935}{1.119389919223}{0.804391759568}{1.119382103563}
  \meshline{144,144,144}{0.804391759568}{1.119382103563}{0.801913627117}{1.119379720718}
  \meshline{144,144,144}{0.817421074839}{1.285682492993}{0.818186626652}{1.285683116283}
  \meshline{144,144,144}{0.784110064067}{1.285655805694}{0.781372223738}{1.285653463496}
  \meshline{144,144,144}{0.751223711897}{1.285627887155}{0.752809725860}{1.285629212236}
  \meshline{144,144,144}{0.781372223738}{1.285653463496}{0.752809725860}{1.285629212236}
  \meshline{144,144,144}{0.784110064067}{1.285655805694}{0.784237062729}{1.285655917674}
  \meshline{144,144,144}{0.709886658628}{1.285588961033}{0.673146394294}{1.285550135551}
  \meshline{144,144,144}{0.751223711897}{1.285627887155}{0.712567822598}{1.285591526622}
  \meshline{144,144,144}{0.695184121399}{1.647429824586}{0.706451059721}{1.647574818079}
  \meshline{144,144,144}{0.927894166255}{1.285738477541}{0.914187992689}{1.285732741478}
  \meshline{144,144,144}{0.875060878378}{1.119406971325}{0.851562752516}{1.119405223061}
  \meshline{144,144,144}{0.911366093969}{1.119406281381}{0.887368805679}{1.119405964749}
  \meshline{144,144,144}{0.941495937669}{1.119423250792}{0.952797054006}{1.119434739387}
  \meshline{144,144,144}{0.887368805679}{1.119405964749}{0.875060878378}{1.119406971325}
  \meshline{144,144,144}{0.911366093969}{1.119406281381}{0.930258350034}{1.119430882990}
  \meshline{144,144,144}{0.984204595121}{1.119440148647}{0.969044823995}{1.119425246108}
  \meshline{144,144,144}{0.851562752516}{1.119405223061}{0.835612097935}{1.119389919223}
  \meshline{144,144,144}{0.969044823995}{1.119425246108}{0.952797054006}{1.119434739387}
  \meshline{144,144,144}{0.984204595121}{1.119440148647}{1.000000000000}{1.119438353106}
  \meshline{144,144,144}{1.000000000000}{1.285756846552}{0.989801036396}{1.285753940330}
  \meshline{144,144,144}{0.930644200620}{1.285738344370}{0.939732799380}{1.285743336196}
  \meshline{144,144,144}{0.818186626652}{1.285683116283}{0.860698428993}{1.285711856717}
  \meshline{144,144,144}{0.860698428993}{1.285711856717}{0.865899030262}{1.285715192869}
  \meshline{144,144,144}{0.784237062729}{1.285655917674}{0.817421074839}{1.285682492993}
  \meshline{144,144,144}{0.865899030262}{1.285715192869}{0.899385410954}{1.285726815978}
  \meshline{144,144,144}{0.989801036396}{1.285753940330}{0.963181867311}{1.285749782857}
  \meshline{144,144,144}{0.927894166255}{1.285738477541}{0.930644200620}{1.285738344370}
  \meshline{144,144,144}{0.899385410954}{1.285726815978}{0.903020734703}{1.285728183317}
  \meshline{144,144,144}{0.939732799380}{1.285743336196}{0.963181867311}{1.285749782857}
  \meshline{144,144,144}{0.903020734703}{1.285728183317}{0.914187992689}{1.285732741478}
  \meshline{144,144,144}{0.921639997753}{1.647114223059}{0.960357956095}{1.647741852090}
  \meshline{144,144,144}{1.000000000000}{0.615109566063}{0.978392306812}{0.615102491666}
  \meshline{144,144,144}{0.942719842555}{0.615092713420}{0.920339030328}{0.615086134562}
  \meshline{144,144,144}{0.674825702022}{1.646876660256}{0.671731415373}{1.646919640667}
  \meshline{144,144,144}{0.706451059721}{1.647574818079}{0.726610566749}{1.647752931566}
  \meshline{144,144,144}{0.746655431644}{1.647266904604}{0.726610566749}{1.647752931566}
  \meshline{144,144,144}{0.695184121399}{1.647429824586}{0.674825702022}{1.646876660256}
  \meshline{144,144,144}{0.138909697321}{0.252246595796}{0.154268775535}{0.252675953262}
  \meshline{144,144,144}{0.185148114804}{0.252961667105}{0.163550484208}{0.252544187380}
  \meshline{144,144,144}{0.113041414778}{0.252491261474}{0.109847278960}{0.252522352893}
  \meshline{144,144,144}{0.223603592591}{0.253122336540}{0.239136370934}{0.252917615069}
  \meshline{144,144,144}{0.868214775909}{1.647390162619}{0.838614760996}{1.647467020817}
  \meshline{144,144,144}{0.757430097522}{1.647387956211}{0.785802308315}{1.646989657725}
  \meshline{144,144,144}{0.757430097522}{1.647387956211}{0.746655431644}{1.647266904604}
  \meshline{144,144,144}{0.790636167771}{1.647070420686}{0.792223269802}{1.647082126931}
  \meshline{144,144,144}{0.838614760996}{1.647467020817}{0.828691236428}{1.647527127499}
  \meshline{144,144,144}{0.792223269802}{1.647082126931}{0.797176596593}{1.646987386591}
  \meshline{144,144,144}{0.790636167771}{1.647070420686}{0.785802308315}{1.646989657725}
  \meshline{144,144,144}{0.868214775909}{1.647390162619}{0.872636573640}{1.647427573591}
  \meshline{144,144,144}{0.828691236428}{1.647527127499}{0.797176596593}{1.646987386591}
  \meshline{144,144,144}{0.977977144381}{1.647527294204}{1.000000000000}{1.647669854433}
  \meshline{144,144,144}{0.872636573640}{1.647427573591}{0.915023992505}{1.647108262358}
  \meshline{144,144,144}{0.921639997753}{1.647114223059}{0.921165590900}{1.647127262522}
  \meshline{144,144,144}{0.915023992505}{1.647108262358}{0.920746708780}{1.647115048578}
  \meshline{144,144,144}{0.921165590900}{1.647127262522}{0.920746708780}{1.647115048578}
  \meshline{144,144,144}{0.977977144381}{1.647527294204}{0.960357956095}{1.647741852090}
  \meshline{144,144,144}{0.113041414778}{0.252491261474}{0.121969316797}{0.252663253991}
  \meshline{144,144,144}{0.138909697321}{0.252246595796}{0.121969316797}{0.252663253991}
  \meshline{144,144,144}{0.074468194895}{0.252331169431}{0.070453330131}{0.252285001960}
  \meshline{144,144,144}{0.036253286691}{0.252580806012}{0.029216703034}{0.252511512935}
  \meshline{144,144,144}{0.074468194895}{0.252331169431}{0.096101307044}{0.252720500657}
  \meshline{144,144,144}{0.000000000000}{0.252235551791}{0.027290264862}{0.252495959931}
  \meshline{144,144,144}{0.036253286691}{0.252580806012}{0.065563445661}{0.252460326110}
  \meshline{144,144,144}{0.070453330131}{0.252285001960}{0.065563445661}{0.252460326110}
  \meshline{144,144,144}{0.109847278960}{0.252522352893}{0.096101307044}{0.252720500657}
  \meshline{144,144,144}{0.223603592591}{0.253122336540}{0.205368890416}{0.252944297670}
  \meshline{144,144,144}{0.345243470319}{0.253214589545}{0.325386036067}{0.253025762934}
  \meshline{144,144,144}{0.258690064775}{0.253152396169}{0.239136370934}{0.252917615069}
  \meshline{144,144,144}{0.185148114804}{0.252961667105}{0.205368890416}{0.252944297670}
  \meshline{144,144,144}{0.258690064775}{0.253152396169}{0.277016480807}{0.253015709823}
  \meshline{144,144,144}{0.282128340288}{0.253060331375}{0.277016480807}{0.253015709823}
  \meshline{144,144,144}{0.282128340288}{0.253060331375}{0.295789375041}{0.253204195950}
  \meshline{144,144,144}{0.295789375041}{0.253204195950}{0.325386036067}{0.253025762934}
  \meshline{144,144,144}{0.404163627276}{0.253157467084}{0.440194848966}{0.253627640483}
  \meshline{144,144,144}{0.372548575142}{0.253010522916}{0.389060245664}{0.253300615681}
  \meshline{144,144,144}{0.345243470319}{0.253214589545}{0.372548575142}{0.253010522916}
\end{pgfscope}


==> nodal_rect_N0.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.9, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{168,0,57}{0.551782213807}{0.950064380588}{0.584946161434}{0.950089624449}
  \meshline{168,0,57}{0.051814955474}{0.949759926061}{0.054044942187}{0.949760224482}
  \meshline{168,0,57}{0.031432220952}{0.949754285831}{0.016289984683}{0.949755804235}
  \meshline{168,0,57}{0.108602132514}{0.949767658173}{0.126370090047}{0.949773973184}
  \meshline{168,0,57}{0.054044942187}{0.949760224482}{0.058386935898}{0.949759445703}
  \meshline{168,0,57}{0.000000000000}{0.949755362808}{0.016289984683}{0.949755804235}
  \meshline{168,0,57}{0.089116057293}{0.949759094924}{0.108602132514}{0.949767658173}
  \meshline{168,0,57}{0.051814955474}{0.949759926061}{0.031432220952}{0.949754285831}
  \meshline{168,0,57}{0.180069159175}{0.949793348949}{0.191217662390}{0.949798188078}
  \meshline{168,0,57}{0.126370090047}{0.949773973184}{0.138368064155}{0.949779079269}
  \meshline{168,0,57}{0.161310229578}{0.949787598443}{0.144841646600}{0.949781404419}
  \meshline{168,0,57}{0.180069159175}{0.949793348949}{0.161310229578}{0.949787598443}
  \meshline{168,0,57}{0.089116057293}{0.949759094924}{0.081126622289}{0.949756734457}
  \meshline{168,0,57}{0.138368064155}{0.949779079269}{0.144841646600}{0.949781404419}
  \meshline{168,0,57}{0.058386935898}{0.949759445703}{0.081126622289}{0.949756734457}
  \meshline{168,0,57}{0.191217662390}{0.949798188078}{0.214473291228}{0.949812193305}
  \meshline{168,0,57}{0.243724782745}{0.949831332342}{0.244371047749}{0.949831624003}
  \meshline{168,0,57}{0.273419634851}{0.949848600620}{0.273584439683}{0.949848712706}
  \meshline{168,0,57}{0.243724782745}{0.949831332342}{0.214473291228}{0.949812193305}
  \meshline{168,0,57}{0.266324521494}{0.949844522889}{0.273419634851}{0.949848600620}
  \meshline{168,0,57}{0.266324521494}{0.949844522889}{0.244683966346}{0.949831815628}
  \meshline{168,0,57}{0.316129239897}{0.949876018914}{0.325887201413}{0.949883016433}
  \meshline{168,0,57}{0.244683966346}{0.949831815628}{0.244371047749}{0.949831624003}
  \meshline{168,0,57}{0.325887201413}{0.949883016433}{0.342946413176}{0.949894942223}
  \meshline{168,0,57}{0.360485664277}{0.949905863656}{0.342946413176}{0.949894942223}
  \meshline{168,0,57}{0.375411469986}{0.949919433054}{0.402817613060}{0.949941488584}
  \meshline{168,0,57}{0.316129239897}{0.949876018914}{0.273584439683}{0.949848712706}
  \meshline{168,0,57}{0.375411469986}{0.949919433054}{0.360485664277}{0.949905863656}
  \meshline{168,0,57}{0.402817613060}{0.949941488584}{0.424212924084}{0.949957200797}
  \meshline{168,0,57}{0.610518683109}{0.950110869101}{0.597218376767}{0.950100662105}
  \meshline{168,0,57}{0.549412317522}{0.950062333656}{0.547239113243}{0.950060728284}
  \meshline{168,0,57}{0.584946161434}{0.950089624449}{0.597218376767}{0.950100662105}
  \meshline{168,0,57}{0.522303057280}{0.950038784961}{0.547239113243}{0.950060728284}
  \meshline{168,0,57}{0.492689087381}{0.950015277949}{0.497808012971}{0.950019526303}
  \meshline{168,0,57}{0.480125289247}{0.950004203543}{0.492689087381}{0.950015277949}
  \meshline{168,0,57}{0.444084084000}{0.949972620133}{0.424212924084}{0.949957200797}
  \meshline{168,0,57}{0.480125289247}{0.950004203543}{0.444084084000}{0.949972620133}
  \meshline{168,0,57}{0.706013857054}{0.950181235603}{0.721074526523}{0.950191401207}
  \meshline{168,0,57}{0.787132678646}{0.950227937511}{0.766734194288}{0.950216430799}
  \meshline{168,0,57}{0.631219404965}{0.950128006729}{0.638757067542}{0.950132164467}
  \meshline{168,0,57}{0.638757067542}{0.950132164467}{0.656870704386}{0.950141513181}
  \meshline{168,0,57}{0.551782213807}{0.950064380588}{0.549412317522}{0.950062333656}
  \meshline{168,0,57}{0.758691127771}{0.950211375018}{0.766734194288}{0.950216430799}
  \meshline{168,0,57}{0.668133986483}{0.950151545675}{0.692167163139}{0.950170783572}
  \meshline{168,0,57}{0.631219404965}{0.950128006729}{0.610518683109}{0.950110869101}
  \meshline{168,0,57}{0.758691127771}{0.950211375018}{0.744482234690}{0.950204295804}
  \meshline{168,0,57}{0.802952604956}{0.950235451811}{0.822879302225}{0.950244444710}
  \meshline{168,0,57}{0.522303057280}{0.950038784961}{0.497808012971}{0.950019526303}
  \meshline{168,0,57}{0.822879302225}{0.950244444710}{0.842948507525}{0.950255026993}
  \meshline{168,0,57}{0.706013857054}{0.950181235603}{0.692167163139}{0.950170783572}
  \meshline{168,0,57}{0.744482234690}{0.950204295804}{0.721074526523}{0.950191401207}
  \meshline{168,0,57}{0.668133986483}{0.950151545675}{0.656870704386}{0.950141513181}
  \meshline{168,0,57}{0.842948507525}{0.950255026993}{0.863278891221}{0.950262829372}
  \meshline{168,0,57}{0.965873567550}{0.950282635665}{0.953009446971}{0.950284235051}
  \meshline{168,0,57}{0.943774478162}{0.950284444384}{0.953009446971}{0.950284235051}
  \meshline{168,0,57}{0.965873567550}{0.950282635665}{0.999688471041}{0.950278401984}
  \meshline{168,0,57}{1.000000000000}{0.950278310617}{0.999688471041}{0.950278401984}
  \meshline{168,0,57}{0.913478672294}{0.950273484042}{0.902936683912}{0.950269761145}
  \meshline{168,0,57}{0.881497468671}{0.950266865046}{0.902936683912}{0.950269761145}
  \meshline{168,0,57}{0.802952604956}{0.950235451811}{0.787132678646}{0.950227937511}
  \meshline{168,0,57}{0.881497468671}{0.950266865046}{0.863278891221}{0.950262829372}
  \meshline{168,0,57}{0.932306507770}{0.950279378444}{0.943774478162}{0.950284444384}
  \meshline{168,0,57}{0.932306507770}{0.950279378444}{0.913478672294}{0.950273484042}
\end{pgfscope}


==> nodal_rectsquare_D.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.2, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{144,144,144}{0.428985506465}{0.296486826482}{0.429278306217}{0.303738963937}
  \meshline{144,144,144}{0.959617084721}{0.217038331483}{0.959752435296}{0.218659458338}
  \meshline{144,144,144}{0.815109106515}{0.256105719388}{0.815447137006}{0.257029514661}
  \meshline{144,144,144}{0.953126999314}{0.176754051476}{0.950756623252}{0.168224254673}
  \meshline{144,144,144}{0.955006436321}{0.186753726264}{0.956701613792}{0.197048611111}
  \meshline{144,144,144}{0.953126999314}{0.176754051476}{0.955006436321}{0.186753726264}
  \meshline{144,144,144}{0.956701613792}{0.197048611111}{0.959617084721}{0.217038331483}
  \meshline{144,144,144}{0.959752435296}{0.218659458338}{0.959806831714}{0.219670823084}
  \meshline{144,144,144}{0.961510037989}{0.235566904973}{0.959806831714}{0.219670823084}
  \meshline{144,144,144}{0.906682352922}{0.081568797535}{0.918420731790}{0.095033516738}
  \meshline{144,144,144}{0.949031302601}{0.159514635656}{0.946194775145}{0.149902684954}
  \meshline{144,144,144}{0.934164284656}{0.119458948622}{0.935843614918}{0.122807561525}
  \meshline{144,144,144}{0.946194775145}{0.149902684954}{0.943907241905}{0.142589448993}
  \meshline{144,144,144}{0.950756623252}{0.168224254673}{0.949031302601}{0.159514635656}
  \meshline{144,144,144}{0.943907241905}{0.142589448993}{0.938448500399}{0.129851159743}
  \meshline{144,144,144}{0.935843614918}{0.122807561525}{0.938448500399}{0.129851159743}
  \meshline{144,144,144}{0.855193746346}{0.151355887769}{0.846971212482}{0.141805464929}
  \meshline{144,144,144}{0.934164284656}{0.119458948622}{0.919540002663}{0.096385075746}
  \meshline{144,144,144}{0.789135583047}{0.035044321254}{0.781444572208}{0.033354191910}
  \meshline{144,144,144}{0.919147766676}{0.095755163524}{0.919540002663}{0.096385075746}
  \meshline{144,144,144}{0.906682352922}{0.081568797535}{0.895762906163}{0.073186642326}
  \meshline{144,144,144}{0.919147766676}{0.095755163524}{0.918420731790}{0.095033516738}
  \meshline{144,144,144}{0.860433813788}{0.159064605580}{0.868424681079}{0.170422095662}
  \meshline{144,144,144}{0.885209584551}{0.205200210224}{0.882436095917}{0.199115141126}
  \meshline{144,144,144}{0.882436095917}{0.199115141126}{0.876476768869}{0.185226426498}
  \meshline{144,144,144}{0.893744109646}{0.233052573323}{0.896739541746}{0.244656529792}
  \meshline{144,144,144}{0.893744109646}{0.233052573323}{0.892949188912}{0.230136844543}
  \meshline{144,144,144}{0.896739541746}{0.244656529792}{0.898407274047}{0.254577347901}
  \meshline{144,144,144}{0.961510037989}{0.235566904973}{0.961760240041}{0.239687244261}
  \meshline{144,144,144}{0.828030960443}{0.123937269466}{0.834906897304}{0.129372822030}
  \meshline{144,144,144}{0.886801202625}{0.209684046322}{0.892949188912}{0.230136844543}
  \meshline{144,144,144}{0.962768179995}{0.249905605839}{0.961760240041}{0.239687244261}
  \meshline{144,144,144}{0.878066074399}{0.062564306287}{0.886232852480}{0.066664921554}
  \meshline{144,144,144}{0.899254580515}{0.258864490233}{0.898407274047}{0.254577347901}
  \meshline{144,144,144}{0.965134617771}{0.307801844920}{0.964775452644}{0.295047882760}
  \meshline{144,144,144}{0.823804280964}{0.306295770390}{0.821414305706}{0.282530565555}
  \meshline{144,144,144}{0.823804280964}{0.306295770390}{0.823949386271}{0.308041645257}
  \meshline{144,144,144}{0.886232852480}{0.066664921554}{0.889621643032}{0.068339569061}
  \meshline{144,144,144}{0.895762906163}{0.073186642326}{0.889621643032}{0.068339569061}
  \meshline{144,144,144}{0.847519396488}{0.048743831723}{0.851320203736}{0.050591586368}
  \meshline{144,144,144}{0.878066074399}{0.062564306287}{0.869175644110}{0.057261964666}
  \meshline{144,144,144}{0.815109106515}{0.256105719388}{0.809651812679}{0.240356137881}
  \meshline{144,144,144}{0.869175644110}{0.057261964666}{0.851320203736}{0.050591586368}
  \meshline{144,144,144}{0.842197452108}{0.046868013002}{0.847519396488}{0.048743831723}
  \meshline{144,144,144}{0.829037069218}{0.042767115476}{0.816031243665}{0.039820086125}
  \meshline{144,144,144}{0.800902981491}{0.105103811073}{0.812380577644}{0.111785144346}
  \meshline{144,144,144}{0.798930761424}{0.103787569422}{0.796019399077}{0.102175878375}
  \meshline{144,144,144}{0.860433813788}{0.159064605580}{0.855193746346}{0.151355887769}
  \meshline{144,144,144}{0.809785894838}{0.038844939569}{0.813604979166}{0.039442998709}
  \meshline{144,144,144}{0.834906897304}{0.129372822030}{0.840649586177}{0.135102409405}
  \meshline{144,144,144}{0.809785894838}{0.038844939569}{0.799190419134}{0.036445429855}
  \meshline{144,144,144}{0.816031243665}{0.039820086125}{0.813604979166}{0.039442998709}
  \meshline{144,144,144}{0.829037069218}{0.042767115476}{0.842197452108}{0.046868013002}
  \meshline{144,144,144}{0.963100034764}{0.256099525943}{0.962768179995}{0.249905605839}
  \meshline{144,144,144}{0.902708872492}{0.287692624683}{0.902463437429}{0.283341137992}
  \meshline{144,144,144}{0.963100034764}{0.256099525943}{0.964000605138}{0.267901243992}
  \meshline{144,144,144}{0.820787620549}{0.279491739261}{0.816316119445}{0.260793437857}
  \meshline{144,144,144}{0.828030960443}{0.123937269466}{0.822450111832}{0.119127912957}
  \meshline{144,144,144}{0.812380577644}{0.111785144346}{0.822450111832}{0.119127912957}
  \meshline{144,144,144}{0.964000605138}{0.267901243992}{0.964239621575}{0.277126222404}
  \meshline{144,144,144}{0.964239621575}{0.277126222404}{0.964663353108}{0.286635422831}
  \meshline{144,144,144}{0.964663353108}{0.286635422831}{0.964723647632}{0.290082335993}
  \meshline{144,144,144}{0.964723647632}{0.290082335993}{0.964775452644}{0.295047882760}
  \meshline{144,144,144}{0.899254580515}{0.258864490233}{0.900868901997}{0.268623378616}
  \meshline{144,144,144}{0.894501305886}{0.402055248399}{0.894336212415}{0.402908864340}
  \meshline{144,144,144}{0.902463437429}{0.283341137992}{0.902016318365}{0.280090121726}
  \meshline{144,144,144}{0.903994058558}{0.319051310788}{0.903791226907}{0.334379097397}
  \meshline{144,144,144}{0.902016318365}{0.280090121726}{0.900868901997}{0.268623378616}
  \meshline{144,144,144}{0.903966973794}{0.308999728611}{0.902708872492}{0.287692624683}
  \meshline{144,144,144}{0.757043543010}{0.463054203230}{0.734547012288}{0.478376427030}
  \meshline{144,144,144}{0.815563592278}{0.257498742887}{0.816316119445}{0.260793437857}
  \meshline{144,144,144}{0.846971212482}{0.141805464929}{0.840649586177}{0.135102409405}
  \meshline{144,144,144}{0.823746694932}{0.329099882413}{0.822802158010}{0.337599102647}
  \meshline{144,144,144}{0.823870462550}{0.311343445816}{0.823746694932}{0.329099882413}
  \meshline{144,144,144}{0.823870462550}{0.311343445816}{0.823949386271}{0.308041645257}
  \meshline{144,144,144}{0.755726664668}{0.333243605125}{0.757013607142}{0.315597839115}
  \meshline{144,144,144}{0.820787620549}{0.279491739261}{0.821414305706}{0.282530565555}
  \meshline{144,144,144}{0.769813439178}{0.180615632788}{0.764869265521}{0.176293722331}
  \meshline{144,144,144}{0.755899593002}{0.168181410096}{0.764869265521}{0.176293722331}
  \meshline{144,144,144}{0.796019399077}{0.102175878375}{0.783591532502}{0.095785077723}
  \meshline{144,144,144}{0.800902981491}{0.105103811073}{0.798930761424}{0.103787569422}
  \meshline{144,144,144}{0.751781869365}{0.165044854474}{0.755899593002}{0.168181410096}
  \meshline{144,144,144}{0.770860604831}{0.090564948906}{0.783591532502}{0.095785077723}
  \meshline{144,144,144}{0.770860604831}{0.090564948906}{0.764270771240}{0.087450799893}
  \meshline{144,144,144}{0.764270771240}{0.087450799893}{0.756417363094}{0.084605847099}
  \meshline{144,144,144}{0.803655003227}{0.227934275116}{0.801915173141}{0.224048292124}
  \meshline{144,144,144}{0.724196399646}{0.224917385359}{0.716118071452}{0.216312830091}
  \meshline{144,144,144}{0.783476311787}{0.196104463254}{0.776831487801}{0.188201065319}
  \meshline{144,144,144}{0.714087173380}{0.214437478934}{0.715398303314}{0.215560665016}
  \meshline{144,144,144}{0.783476311787}{0.196104463254}{0.789976413870}{0.204462640549}
  \meshline{144,144,144}{0.776831487801}{0.188201065319}{0.769813439178}{0.180615632788}
  \meshline{144,144,144}{0.747896271393}{0.265579301513}{0.750048849396}{0.270333730665}
  \meshline{144,144,144}{0.799513341524}{0.220187036085}{0.789976413870}{0.204462640549}
  \meshline{144,144,144}{0.735955058112}{0.241998338438}{0.742701187700}{0.252665955342}
  \meshline{144,144,144}{0.715398303314}{0.215560665016}{0.716118071452}{0.216312830091}
  \meshline{144,144,144}{0.735955058112}{0.241998338438}{0.728054841658}{0.229751607563}
  \meshline{144,144,144}{0.671970338327}{0.065185621554}{0.682286148914}{0.066691551677}
  \meshline{144,144,144}{0.724196399646}{0.224917385359}{0.728054841658}{0.229751607563}
  \meshline{144,144,144}{0.702432505173}{0.204181369979}{0.697153710414}{0.200559404281}
  \meshline{144,144,144}{0.664849447414}{0.251919895348}{0.672432876472}{0.259903651209}
  \meshline{144,144,144}{0.702432505173}{0.204181369979}{0.714087173380}{0.214437478934}
  \meshline{144,144,144}{0.677182066892}{0.189107128392}{0.688795973030}{0.194840959181}
  \meshline{144,144,144}{0.697153710414}{0.200559404281}{0.688795973030}{0.194840959181}
  \meshline{144,144,144}{0.729728439718}{0.076337519157}{0.735963762613}{0.078035476219}
  \meshline{144,144,144}{0.722617867917}{0.146144501224}{0.718499386223}{0.144117026610}
  \meshline{144,144,144}{0.718499386223}{0.144117026610}{0.703348972610}{0.137186156213}
  \meshline{144,144,144}{0.734915887258}{0.153145858986}{0.722617867917}{0.146144501224}
  \meshline{144,144,144}{0.697828631040}{0.069193168285}{0.706908425449}{0.071074248411}
  \meshline{144,144,144}{0.675063446408}{0.023248393539}{0.680231983171}{0.023465143460}
  \meshline{144,144,144}{0.740830544599}{0.156870345506}{0.751781869365}{0.165044854474}
  \meshline{144,144,144}{0.734915887258}{0.153145858986}{0.740830544599}{0.156870345506}
  \meshline{144,144,144}{0.706908425449}{0.071074248411}{0.717415137837}{0.073258953284}
  \meshline{144,144,144}{0.724551554593}{0.075216676920}{0.729728439718}{0.076337519157}
  \meshline{144,144,144}{0.717415137837}{0.073258953284}{0.724551554593}{0.075216676920}
  \meshline{144,144,144}{0.809651812679}{0.240356137881}{0.803655003227}{0.227934275116}
  \meshline{144,144,144}{0.799513341524}{0.220187036085}{0.801915173141}{0.224048292124}
  \meshline{144,144,144}{0.815447137006}{0.257029514661}{0.815563592278}{0.257498742887}
  \meshline{144,144,144}{0.754823717901}{0.290670732324}{0.756239522081}{0.297707635687}
  \meshline{144,144,144}{0.750048849396}{0.270333730665}{0.751355141006}{0.274197722995}
  \meshline{144,144,144}{0.679346635294}{0.270065198031}{0.672432876472}{0.259903651209}
  \meshline{144,144,144}{0.584247191381}{0.059803677113}{0.570948010633}{0.060118353126}
  \meshline{144,144,144}{0.694261491503}{0.133965304416}{0.701128087514}{0.136344808301}
  \meshline{144,144,144}{0.682286148914}{0.066691551677}{0.697828631040}{0.069193168285}
  \meshline{144,144,144}{0.740657750354}{0.028273415991}{0.746973857736}{0.028864376588}
  \meshline{144,144,144}{0.886801202625}{0.209684046322}{0.885209584551}{0.205200210224}
  \meshline{144,144,144}{0.871257439376}{0.175682643051}{0.868424681079}{0.170422095662}
  \meshline{144,144,144}{0.871257439376}{0.175682643051}{0.876476768869}{0.185226426498}
  \meshline{144,144,144}{0.679346635294}{0.270065198031}{0.683311652446}{0.276653621223}
  \meshline{144,144,144}{0.643632179227}{0.384628428121}{0.627947919792}{0.390158442266}
  \meshline{144,144,144}{0.436980077740}{0.258925619264}{0.433553681392}{0.268234409598}
  \meshline{144,144,144}{0.677182066892}{0.189107128392}{0.662701741466}{0.181788357020}
  \meshline{144,144,144}{0.689404391582}{0.328966191820}{0.687241809674}{0.337104869999}
  \meshline{144,144,144}{0.691221280153}{0.316912144351}{0.689404391582}{0.328966191820}
  \meshline{144,144,144}{0.689230062331}{0.294985100109}{0.691168447847}{0.303488988079}
  \meshline{144,144,144}{0.703348972610}{0.137186156213}{0.701128087514}{0.136344808301}
  \meshline{144,144,144}{0.694261491503}{0.133965304416}{0.683904901850}{0.130081295483}
  \meshline{144,144,144}{0.665315000396}{0.124810034695}{0.679851123078}{0.128742961924}
  \meshline{144,144,144}{0.653520649352}{0.022356893653}{0.653289757520}{0.022344853749}
  \meshline{144,144,144}{0.636818345491}{0.119296088353}{0.619932621652}{0.117221368009}
  \meshline{144,144,144}{0.653520649352}{0.022356893653}{0.653701129032}{0.022370642129}
  \meshline{144,144,144}{0.668480557783}{0.064835648918}{0.654141933455}{0.063104593177}
  \meshline{144,144,144}{0.715728160962}{0.025789271089}{0.706311587767}{0.025019787809}
  \meshline{144,144,144}{0.715728160962}{0.025789271089}{0.725079720817}{0.026558573761}
  \meshline{144,144,144}{0.698818260027}{0.024792153191}{0.706311587767}{0.025019787809}
  \meshline{144,144,144}{0.746973857736}{0.028864376588}{0.748226558261}{0.028864376588}
  \meshline{144,144,144}{0.728619805723}{0.027063721822}{0.740657750354}{0.028273415991}
  \meshline{144,144,144}{0.728619805723}{0.027063721822}{0.725079720817}{0.026558573761}
  \meshline{144,144,144}{0.662022960013}{0.372967371447}{0.671649834269}{0.363671599208}
  \meshline{144,144,144}{0.683311652446}{0.276653621223}{0.686153848135}{0.283318613575}
  \meshline{144,144,144}{0.686153848135}{0.283318613575}{0.689230062331}{0.294985100109}
  \meshline{144,144,144}{0.631777644829}{0.231059682773}{0.643396685358}{0.236019440024}
  \meshline{144,144,144}{0.647611784847}{0.238534751214}{0.643396685358}{0.236019440024}
  \meshline{144,144,144}{0.565562017613}{0.116693064499}{0.558965143268}{0.117250258858}
  \meshline{144,144,144}{0.613250239727}{0.225915189554}{0.620051062561}{0.227831714304}
  \meshline{144,144,144}{0.629365584549}{0.172131856323}{0.617340513509}{0.170116946709}
  \meshline{144,144,144}{0.652306134847}{0.178117503416}{0.662701741466}{0.181788357020}
  \meshline{144,144,144}{0.664849447414}{0.251919895348}{0.653232077317}{0.242930904143}
  \meshline{144,144,144}{0.647611784847}{0.238534751214}{0.653232077317}{0.242930904143}
  \meshline{144,144,144}{0.593408354268}{0.223928329068}{0.604490380740}{0.224840053113}
  \meshline{144,144,144}{0.691168447847}{0.303488988079}{0.691221280153}{0.316912144351}
  \meshline{144,144,144}{0.687241809674}{0.337104869999}{0.684384542225}{0.343582092730}
  \meshline{144,144,144}{0.753298876549}{0.345829724751}{0.752573836005}{0.349173473266}
  \meshline{144,144,144}{0.757013607142}{0.315597839115}{0.757069223598}{0.314864114587}
  \meshline{144,144,144}{0.742516084652}{0.374803388233}{0.748717118463}{0.358789914265}
  \meshline{144,144,144}{0.753298876549}{0.345829724751}{0.755726664668}{0.333243605125}
  \meshline{144,144,144}{0.716696877669}{0.487259414415}{0.704075604852}{0.492000194068}
  \meshline{144,144,144}{0.762942205583}{0.030677558783}{0.751146128042}{0.029108088047}
  \meshline{144,144,144}{0.749934243839}{0.082578691122}{0.756417363094}{0.084605847099}
  \meshline{144,144,144}{0.735963762613}{0.078035476219}{0.749934243839}{0.082578691122}
  \meshline{144,144,144}{0.683904901850}{0.130081295483}{0.679851123078}{0.128742961924}
  \meshline{144,144,144}{0.756239522081}{0.297707635687}{0.757025981701}{0.313749554156}
  \meshline{144,144,144}{0.757069223598}{0.314864114587}{0.757025981701}{0.313749554156}
  \meshline{144,144,144}{0.668480557783}{0.064835648918}{0.670240717767}{0.064975270086}
  \meshline{144,144,144}{0.698818260027}{0.024792153191}{0.680231983171}{0.023465143460}
  \meshline{144,144,144}{0.649818579825}{0.062770590077}{0.654141933455}{0.063104593177}
  \meshline{144,144,144}{0.670240717767}{0.064975270086}{0.671970338327}{0.065185621554}
  \meshline{144,144,144}{0.641731823773}{0.061939731102}{0.633462397329}{0.061375581340}
  \meshline{144,144,144}{0.545820319316}{0.061239030486}{0.564798989923}{0.060253829025}
  \meshline{144,144,144}{0.654994244881}{0.022425302427}{0.653701129032}{0.022370642129}
  \meshline{144,144,144}{0.628942816270}{0.021631812772}{0.636018752668}{0.021841510050}
  \meshline{144,144,144}{0.641731823773}{0.061939731102}{0.649818579825}{0.062770590077}
  \meshline{144,144,144}{0.653289757520}{0.022344853749}{0.636018752668}{0.021841510050}
  \meshline{144,144,144}{0.570958163782}{0.021339977270}{0.577546182694}{0.021236891706}
  \meshline{144,144,144}{0.628942816270}{0.021631812772}{0.610043889479}{0.021375275885}
  \meshline{144,144,144}{0.592222983935}{0.021210493110}{0.583496443966}{0.021246989180}
  \meshline{144,144,144}{0.599974677817}{0.021268310625}{0.610043889479}{0.021375275885}
  \meshline{144,144,144}{0.592222983935}{0.021210493110}{0.599974677817}{0.021268310625}
  \meshline{144,144,144}{0.611201824581}{0.060268135873}{0.621794732819}{0.060668145382}
  \meshline{144,144,144}{0.595051839836}{0.059901643616}{0.611201824581}{0.060268135873}
  \meshline{144,144,144}{0.521744977300}{0.022346443662}{0.538159690932}{0.021858439116}
  \meshline{144,144,144}{0.642195124978}{0.119952941527}{0.649663404778}{0.121497040329}
  \meshline{144,144,144}{0.654994244881}{0.022425302427}{0.675063446408}{0.023248393539}
  \meshline{144,144,144}{0.577546182694}{0.021236891706}{0.583496443966}{0.021246989180}
  \meshline{144,144,144}{0.562329717373}{0.021387141115}{0.570958163782}{0.021339977270}
  \meshline{144,144,144}{0.558927667776}{0.021387141115}{0.562329717373}{0.021387141115}
  \meshline{144,144,144}{0.633462397329}{0.061375581340}{0.621794732819}{0.060668145382}
  \meshline{144,144,144}{0.636818345491}{0.119296088353}{0.642195124978}{0.119952941527}
  \meshline{144,144,144}{0.544906218108}{0.061307135956}{0.545472107597}{0.061254826470}
  \meshline{144,144,144}{0.595051839836}{0.059901643616}{0.584247191381}{0.059803677113}
  \meshline{144,144,144}{0.539645363821}{0.021786418241}{0.538950272603}{0.021816402713}
  \meshline{144,144,144}{0.570948010633}{0.060118353126}{0.564798989923}{0.060253829025}
  \meshline{144,144,144}{0.528854204445}{0.062445366821}{0.544906218108}{0.061307135956}
  \meshline{144,144,144}{0.665315000396}{0.124810034695}{0.649663404778}{0.121497040329}
  \meshline{144,144,144}{0.610615989470}{0.116574267696}{0.619932621652}{0.117221368009}
  \meshline{144,144,144}{0.620051062561}{0.227831714304}{0.631777644829}{0.231059682773}
  \meshline{144,144,144}{0.596016379256}{0.116089402395}{0.591206391542}{0.115835566935}
  \meshline{144,144,144}{0.647497276250}{0.176671264019}{0.652306134847}{0.178117503416}
  \meshline{144,144,144}{0.629365584549}{0.172131856323}{0.642733500306}{0.175573950823}
  \meshline{144,144,144}{0.647497276250}{0.176671264019}{0.642733500306}{0.175573950823}
  \meshline{144,144,144}{0.545820319316}{0.061239030486}{0.545472107597}{0.061254826470}
  \meshline{144,144,144}{0.520713148511}{0.063369095450}{0.513414464742}{0.064029352994}
  \meshline{144,144,144}{0.542024135027}{0.021747123685}{0.539645363821}{0.021786418241}
  \meshline{144,144,144}{0.542024135027}{0.021747123685}{0.558927667776}{0.021387141115}
  \meshline{144,144,144}{0.538159690932}{0.021858439116}{0.538950272603}{0.021816402713}
  \meshline{144,144,144}{0.515275378645}{0.022662632954}{0.505244802384}{0.022915999003}
  \meshline{144,144,144}{0.573015650637}{0.116268069545}{0.584589724123}{0.116001149051}
  \meshline{144,144,144}{0.559615515094}{0.170798876118}{0.562983944125}{0.170351506249}
  \meshline{144,144,144}{0.481646817523}{0.024308696411}{0.485245580215}{0.023960580481}
  \meshline{144,144,144}{0.521744977300}{0.022346443662}{0.515275378645}{0.022662632954}
  \meshline{144,144,144}{0.520713148511}{0.063369095450}{0.528854204445}{0.062445366821}
  \meshline{144,144,144}{0.485245580215}{0.023960580481}{0.492245358329}{0.023569153822}
  \meshline{144,144,144}{0.466826894817}{0.025084867884}{0.481646817523}{0.024308696411}
  \meshline{144,144,144}{0.452760347880}{0.025965994962}{0.466826894817}{0.025084867884}
  \meshline{144,144,144}{0.502221894518}{0.065358731881}{0.495120663215}{0.066256882289}
  \meshline{144,144,144}{0.541606310832}{0.119265557117}{0.545736462754}{0.118842853048}
  \meshline{144,144,144}{0.573015650637}{0.116268069545}{0.565562017613}{0.116693064499}
  \meshline{144,144,144}{0.608151831465}{0.169082080839}{0.617340513509}{0.170116946709}
  \meshline{144,144,144}{0.596016379256}{0.116089402395}{0.610615989470}{0.116574267696}
  \meshline{144,144,144}{0.584589724123}{0.116001149051}{0.589026824406}{0.115828994759}
  \meshline{144,144,144}{0.600472307539}{0.168646481092}{0.595283632950}{0.168473143890}
  \meshline{144,144,144}{0.595283632950}{0.168473143890}{0.579958849493}{0.168775527998}
  \meshline{144,144,144}{0.608151831465}{0.169082080839}{0.600472307539}{0.168646481092}
  \meshline{144,144,144}{0.508707462266}{0.125885501732}{0.505642209375}{0.126695083322}
  \meshline{144,144,144}{0.545736462754}{0.118842853048}{0.558965143268}{0.117250258858}
  \meshline{144,144,144}{0.591206391542}{0.115835566935}{0.589026824406}{0.115828994759}
  \meshline{144,144,144}{0.604490380740}{0.224840053113}{0.613250239727}{0.225915189554}
  \meshline{144,144,144}{0.500840716576}{0.190104620083}{0.514639899311}{0.183485281025}
  \meshline{144,144,144}{0.502221894518}{0.065358731881}{0.513414464742}{0.064029352994}
  \meshline{144,144,144}{0.446052748494}{0.075436788496}{0.458099012323}{0.072903679348}
  \meshline{144,144,144}{0.452760347880}{0.025965994962}{0.448166252572}{0.026509818428}
  \meshline{144,144,144}{0.422622367945}{0.081502034115}{0.412581674633}{0.084816171331}
  \meshline{144,144,144}{0.474410599065}{0.069786173823}{0.458719309769}{0.072750266570}
  \meshline{144,144,144}{0.437571128689}{0.077941973101}{0.446052748494}{0.075436788496}
  \meshline{144,144,144}{0.479339909137}{0.068821367517}{0.474410599065}{0.069786173823}
  \meshline{144,144,144}{0.458099012323}{0.072903679348}{0.458719309769}{0.072750266570}
  \meshline{144,144,144}{0.526706736143}{0.121595217391}{0.508707462266}{0.125885501732}
  \meshline{144,144,144}{0.483973181121}{0.133239954721}{0.480640906290}{0.134575366103}
  \meshline{144,144,144}{0.541606310832}{0.119265557117}{0.539103145325}{0.119636497070}
  \meshline{144,144,144}{0.483973181121}{0.133239954721}{0.505642209375}{0.126695083322}
  \meshline{144,144,144}{0.459186212546}{0.143698602398}{0.470143273909}{0.138436197353}
  \meshline{144,144,144}{0.539103145325}{0.119636497070}{0.526706736143}{0.121595217391}
  \meshline{144,144,144}{0.445731261386}{0.150261461690}{0.438328077506}{0.154807867033}
  \meshline{144,144,144}{0.470143273909}{0.138436197353}{0.480640906290}{0.134575366103}
  \meshline{144,144,144}{0.457278605373}{0.144530873975}{0.459186212546}{0.143698602398}
  \meshline{144,144,144}{0.532814358028}{0.177079128383}{0.527509812294}{0.178572755529}
  \meshline{144,144,144}{0.454906094468}{0.228770053713}{0.466094993025}{0.215294174938}
  \meshline{144,144,144}{0.500840716576}{0.190104620083}{0.496004105860}{0.192953951504}
  \meshline{144,144,144}{0.511514280167}{0.263283563240}{0.505038120843}{0.274316085694}
  \meshline{144,144,144}{0.524033879808}{0.179819262681}{0.514639899311}{0.183485281025}
  \meshline{144,144,144}{0.450737464013}{0.233538685342}{0.454906094468}{0.228770053713}
  \meshline{144,144,144}{0.433140817253}{0.157786034084}{0.438328077506}{0.154807867033}
  \meshline{144,144,144}{0.480364562878}{0.202895621233}{0.496004105860}{0.192953951504}
  \meshline{144,144,144}{0.527509812294}{0.178572755529}{0.524033879808}{0.179819262681}
  \meshline{144,144,144}{0.532814358028}{0.177079128383}{0.543327454529}{0.174067380366}
  \meshline{144,144,144}{0.543327454529}{0.174067380366}{0.554292756700}{0.171885281829}
  \meshline{144,144,144}{0.547804901931}{0.233492731095}{0.540228820012}{0.237049810676}
  \meshline{144,144,144}{0.475002744043}{0.207728443187}{0.480364562878}{0.202895621233}
  \meshline{144,144,144}{0.576716742100}{0.224931391367}{0.593408354268}{0.223928329068}
  \meshline{144,144,144}{0.492245358329}{0.023569153822}{0.505244802384}{0.022915999003}
  \meshline{144,144,144}{0.479339909137}{0.068821367517}{0.495120663215}{0.066256882289}
  \meshline{144,144,144}{0.449003820856}{0.235848425975}{0.440611607821}{0.250028460578}
  \meshline{144,144,144}{0.574728003894}{0.225227885658}{0.575603329137}{0.225036845056}
  \meshline{144,144,144}{0.526205849115}{0.246544760487}{0.522602710640}{0.250280293890}
  \meshline{144,144,144}{0.559615515094}{0.170798876118}{0.554292756700}{0.171885281829}
  \meshline{144,144,144}{0.579958849493}{0.168775527998}{0.562983944125}{0.170351506249}
  \meshline{144,144,144}{0.511514280167}{0.263283563240}{0.522602710640}{0.250280293890}
  \meshline{144,144,144}{0.449003820856}{0.235848425975}{0.450737464013}{0.233538685342}
  \meshline{144,144,144}{0.428985506465}{0.296486826482}{0.429896420786}{0.286901430484}
  \meshline{144,144,144}{0.475002744043}{0.207728443187}{0.466094993025}{0.215294174938}
  \meshline{144,144,144}{0.457278605373}{0.144530873975}{0.455935234074}{0.145224714701}
  \meshline{144,144,144}{0.445731261386}{0.150261461690}{0.455935234074}{0.145224714701}
  \meshline{144,144,144}{0.547804901931}{0.233492731095}{0.558575684927}{0.229209368585}
  \meshline{144,144,144}{0.558575684927}{0.229209368585}{0.574728003894}{0.225227885658}
  \meshline{144,144,144}{0.436980077740}{0.258925619264}{0.440611607821}{0.250028460578}
  \meshline{144,144,144}{0.747896271393}{0.265579301513}{0.742701187700}{0.252665955342}
  \meshline{144,144,144}{0.754823717901}{0.290670732324}{0.751355141006}{0.274197722995}
  \meshline{144,144,144}{0.752573836005}{0.349173473266}{0.751842486453}{0.351214727974}
  \meshline{144,144,144}{0.675681144941}{0.359052283119}{0.684384542225}{0.343582092730}
  \meshline{144,144,144}{0.711055290377}{0.414804761374}{0.700047824222}{0.422960406710}
  \meshline{144,144,144}{0.654707664248}{0.378171717088}{0.643632179227}{0.384628428121}
  \meshline{144,144,144}{0.627947919792}{0.390158442266}{0.625861032680}{0.390888177377}
  \meshline{144,144,144}{0.648304155096}{0.445495403267}{0.632358227438}{0.448260828625}
  \meshline{144,144,144}{0.674218367339}{0.361020778197}{0.675681144941}{0.359052283119}
  \meshline{144,144,144}{0.576716742100}{0.224931391367}{0.575603329137}{0.225036845056}
  \meshline{144,144,144}{0.433553681392}{0.268234409598}{0.432062318031}{0.274390107345}
  \meshline{144,144,144}{0.498258224671}{0.300828420236}{0.499622345153}{0.318003209937}
  \meshline{144,144,144}{0.498168199343}{0.299151997883}{0.498201580494}{0.298372752694}
  \meshline{144,144,144}{0.505038120843}{0.274316085694}{0.504010221808}{0.276105056699}
  \meshline{144,144,144}{0.503534476384}{0.277088941063}{0.504010221808}{0.276105056699}
  \meshline{144,144,144}{0.498455043643}{0.297326316760}{0.503534476384}{0.277088941063}
  \meshline{144,144,144}{0.538052612831}{0.373947789472}{0.547251167740}{0.379538756056}
  \meshline{144,144,144}{0.535768937785}{0.435755875980}{0.549208556256}{0.440520633011}
  \meshline{144,144,144}{0.654707664248}{0.378171717088}{0.662022960013}{0.372967371447}
  \meshline{144,144,144}{0.588322175858}{0.392880899439}{0.582922563825}{0.391794871288}
  \meshline{144,144,144}{0.540228820012}{0.237049810676}{0.530480099070}{0.243561873833}
  \meshline{144,144,144}{0.526205849115}{0.246544760487}{0.530480099070}{0.243561873833}
  \meshline{144,144,144}{0.502165493664}{0.327661720815}{0.499622345153}{0.318003209937}
  \meshline{144,144,144}{0.502165493664}{0.327661720815}{0.508453927265}{0.342680303824}
  \meshline{144,144,144}{0.498258224671}{0.300828420236}{0.498168199343}{0.299151997883}
  \meshline{144,144,144}{0.509664855655}{0.344820188665}{0.518183483833}{0.356332532376}
  \meshline{144,144,144}{0.518183483833}{0.356332532376}{0.521874798609}{0.360112494534}
  \meshline{144,144,144}{0.673627093952}{0.437338746821}{0.679802353750}{0.434802913824}
  \meshline{144,144,144}{0.695940233870}{0.425927103184}{0.682448756437}{0.433274927729}
  \meshline{144,144,144}{0.715643726849}{0.410354317816}{0.711055290377}{0.414804761374}
  \meshline{144,144,144}{0.742516084652}{0.374803388233}{0.739814927925}{0.379532490385}
  \meshline{144,144,144}{0.751842486453}{0.351214727974}{0.748717118463}{0.358789914265}
  \meshline{144,144,144}{0.739814927925}{0.379532490385}{0.734410765351}{0.388730628174}
  \meshline{144,144,144}{0.724636047955}{0.401272388807}{0.728312939081}{0.396528475938}
  \meshline{144,144,144}{0.715643726849}{0.410354317816}{0.724636047955}{0.401272388807}
  \meshline{144,144,144}{0.674218367339}{0.361020778197}{0.671649834269}{0.363671599208}
  \meshline{144,144,144}{0.430289095894}{0.316365952518}{0.432155109143}{0.328029965737}
  \meshline{144,144,144}{0.498201580494}{0.298372752694}{0.498455043643}{0.297326316760}
  \meshline{144,144,144}{0.444416613416}{0.359095209020}{0.448767405620}{0.367077122675}
  \meshline{144,144,144}{0.509664855655}{0.344820188665}{0.508453927265}{0.342680303824}
  \meshline{144,144,144}{0.439293683966}{0.349356732553}{0.444416613416}{0.359095209020}
  \meshline{144,144,144}{0.624502686863}{0.391149595358}{0.607868039872}{0.393148600772}
  \meshline{144,144,144}{0.612270186746}{0.449785894800}{0.627837487143}{0.448921163509}
  \meshline{144,144,144}{0.662082939670}{0.441706100494}{0.665505503980}{0.440687932331}
  \meshline{144,144,144}{0.628059371163}{0.504687696978}{0.615270512248}{0.504237724623}
  \meshline{144,144,144}{0.553413642508}{0.441774622853}{0.571989833340}{0.446196262533}
  \meshline{144,144,144}{0.627837487143}{0.448921163509}{0.632358227438}{0.448260828625}
  \meshline{144,144,144}{0.624502686863}{0.391149595358}{0.625861032680}{0.390888177377}
  \meshline{144,144,144}{0.590878081360}{0.393037709966}{0.589270088230}{0.392993731829}
  \meshline{144,144,144}{0.590878081360}{0.393037709966}{0.607868039872}{0.393148600772}
  \meshline{144,144,144}{0.521874798609}{0.360112494534}{0.530689549418}{0.368408949437}
  \meshline{144,144,144}{0.552318706598}{0.382413645442}{0.566808194184}{0.388074050446}
  \meshline{144,144,144}{0.430582792468}{0.280057700728}{0.429896420786}{0.286901430484}
  \meshline{144,144,144}{0.430582792468}{0.280057700728}{0.432062318031}{0.274390107345}
  \meshline{144,144,144}{0.445993814808}{0.448801543595}{0.450242728504}{0.451941518036}
  \meshline{144,144,144}{0.665505503980}{0.440687932331}{0.673627093952}{0.437338746821}
  \meshline{144,144,144}{0.648304155096}{0.445495403267}{0.662082939670}{0.441706100494}
  \meshline{144,144,144}{0.682063950230}{0.498457242917}{0.680874400117}{0.498816795702}
  \meshline{144,144,144}{0.682063950230}{0.498457242917}{0.688666018230}{0.496620307480}
  \meshline{144,144,144}{0.680874400117}{0.498816795702}{0.676839184026}{0.499517071339}
  \meshline{144,144,144}{0.538052612831}{0.373947789472}{0.530689549418}{0.368408949437}
  \meshline{144,144,144}{0.566808194184}{0.388074050446}{0.569576362526}{0.388960749232}
  \meshline{144,144,144}{0.547251167740}{0.379538756056}{0.552318706598}{0.382413645442}
  \meshline{144,144,144}{0.679802353750}{0.434802913824}{0.682448756437}{0.433274927729}
  \meshline{144,144,144}{0.700047824222}{0.422960406710}{0.695940233870}{0.425927103184}
  \meshline{144,144,144}{0.777611082606}{0.443994279989}{0.771255654235}{0.450487753841}
  \meshline{144,144,144}{0.716696877669}{0.487259414415}{0.733303856358}{0.479006218118}
  \meshline{144,144,144}{0.728312939081}{0.396528475938}{0.734410765351}{0.388730628174}
  \meshline{144,144,144}{0.699456599715}{0.493729873871}{0.688666018230}{0.496620307480}
  \meshline{144,144,144}{0.789359294978}{0.429226044955}{0.795626872485}{0.419204960877}
  \meshline{144,144,144}{0.355666102428}{0.325674074830}{0.355680007262}{0.325804522380}
  \meshline{144,144,144}{0.699456599715}{0.493729873871}{0.704075604852}{0.492000194068}
  \meshline{144,144,144}{0.366410903428}{0.231477395907}{0.363114390109}{0.240177479678}
  \meshline{144,144,144}{0.436118993020}{0.340410412141}{0.439293683966}{0.349356732553}
  \meshline{144,144,144}{0.430289095894}{0.316365952518}{0.429464354917}{0.312017682103}
  \meshline{144,144,144}{0.455072286579}{0.375980484069}{0.461485674773}{0.384190286661}
  \meshline{144,144,144}{0.789359294978}{0.429226044955}{0.783864186340}{0.436240548753}
  \meshline{144,144,144}{0.455072286579}{0.375980484069}{0.448767405620}{0.367077122675}
  \meshline{144,144,144}{0.425627574110}{0.433419201241}{0.434593725988}{0.441112874161}
  \meshline{144,144,144}{0.436118993020}{0.340410412141}{0.432155109143}{0.328029965737}
  \meshline{144,144,144}{0.795626872485}{0.419204960877}{0.798274218031}{0.415167388311}
  \meshline{144,144,144}{0.761020678769}{0.460054498043}{0.757043543010}{0.463054203230}
  \meshline{144,144,144}{0.353186958633}{0.282100279247}{0.352753474530}{0.285127057260}
  \meshline{144,144,144}{0.358711788372}{0.253666630062}{0.355268372181}{0.266136935825}
  \meshline{144,144,144}{0.372114649792}{0.221102813436}{0.366410903428}{0.231477395907}
  \meshline{144,144,144}{0.385184473405}{0.201447003597}{0.392712114951}{0.192059025997}
  \meshline{144,144,144}{0.372550797011}{0.220253539188}{0.372114649792}{0.221102813436}
  \meshline{144,144,144}{0.380085637570}{0.207913173704}{0.372965531073}{0.219640173903}
  \meshline{144,144,144}{0.409728970643}{0.175505324427}{0.399424589140}{0.185126395268}
  \meshline{144,144,144}{0.399424589140}{0.185126395268}{0.392712114951}{0.192059025997}
  \meshline{144,144,144}{0.411841295314}{0.173612112461}{0.413691035246}{0.172320472822}
  \meshline{144,144,144}{0.411841295314}{0.173612112461}{0.409728970643}{0.175505324427}
  \meshline{144,144,144}{0.360085798908}{0.247646966227}{0.361224818561}{0.244294548614}
  \meshline{144,144,144}{0.380085637570}{0.207913173704}{0.385184473405}{0.201447003597}
  \meshline{144,144,144}{0.372550797011}{0.220253539188}{0.372965531073}{0.219640173903}
  \meshline{144,144,144}{0.358711788372}{0.253666630062}{0.360085798908}{0.247646966227}
  \meshline{144,144,144}{0.520597271164}{0.486174199707}{0.529488007183}{0.489212832409}
  \meshline{144,144,144}{0.269619310298}{0.185395197424}{0.281297517957}{0.168490656326}
  \meshline{144,144,144}{0.391918970364}{0.399452701510}{0.397153927843}{0.406488805689}
  \meshline{144,144,144}{0.504328383875}{0.480032964686}{0.498390927966}{0.477682857866}
  \meshline{144,144,144}{0.466277131467}{0.389520277358}{0.461485674773}{0.384190286661}
  \meshline{144,144,144}{0.425627574110}{0.433419201241}{0.417393720733}{0.426989777541}
  \meshline{144,144,144}{0.408355194128}{0.418360018219}{0.409342242877}{0.419338970532}
  \meshline{144,144,144}{0.473134060375}{0.396560778207}{0.466277131467}{0.389520277358}
  \meshline{144,144,144}{0.501572404577}{0.418610475211}{0.487998263999}{0.409241998195}
  \meshline{144,144,144}{0.487998263999}{0.409241998195}{0.485556067706}{0.407204761317}
  \meshline{144,144,144}{0.502969988932}{0.419534326539}{0.505311042442}{0.420851429396}
  \meshline{144,144,144}{0.361224818561}{0.244294548614}{0.363114390109}{0.240177479678}
  \meshline{144,144,144}{0.334330670898}{0.120963050894}{0.341487980625}{0.116940454745}
  \meshline{144,144,144}{0.428541831419}{0.079964426522}{0.437571128689}{0.077941973101}
  \meshline{144,144,144}{0.392781326635}{0.031962273973}{0.406690933852}{0.030332010559}
  \meshline{144,144,144}{0.400176262452}{0.089213787958}{0.382524957989}{0.095777719432}
  \meshline{144,144,144}{0.325497328953}{0.127334343574}{0.334330670898}{0.120963050894}
  \meshline{144,144,144}{0.378656284400}{0.097534924032}{0.382524957989}{0.095777719432}
  \meshline{144,144,144}{0.378656284400}{0.097534924032}{0.369731264767}{0.102038184713}
  \meshline{144,144,144}{0.309277372472}{0.140128241302}{0.294811340849}{0.153489835502}
  \meshline{144,144,144}{0.422622367945}{0.081502034115}{0.428541831419}{0.079964426522}
  \meshline{144,144,144}{0.412581674633}{0.084816171331}{0.404511912811}{0.087529157116}
  \meshline{144,144,144}{0.404511912811}{0.087529157116}{0.400176262452}{0.089213787958}
  \meshline{144,144,144}{0.360423775004}{0.106202770189}{0.369731264767}{0.102038184713}
  \meshline{144,144,144}{0.310842717276}{0.138640949024}{0.309277372472}{0.140128241302}
  \meshline{144,144,144}{0.321008690041}{0.130301714348}{0.311154105388}{0.138407206754}
  \meshline{144,144,144}{0.281297517957}{0.168490656326}{0.290808114397}{0.158143038797}
  \meshline{144,144,144}{0.290808114397}{0.158143038797}{0.294811340849}{0.153489835502}
  \meshline{144,144,144}{0.448166252572}{0.026509818428}{0.442891390575}{0.027010704427}
  \meshline{144,144,144}{0.353837713178}{0.109482375266}{0.360423775004}{0.106202770189}
  \meshline{144,144,144}{0.341487980625}{0.116940454745}{0.353837713178}{0.109482375266}
  \meshline{144,144,144}{0.385904220345}{0.032917142994}{0.380965964475}{0.033922399128}
  \meshline{144,144,144}{0.435320470921}{0.027540229134}{0.442891390575}{0.027010704427}
  \meshline{144,144,144}{0.435320470921}{0.027540229134}{0.429299373201}{0.028004847334}
  \meshline{144,144,144}{0.385904220345}{0.032917142994}{0.392781326635}{0.031962273973}
  \meshline{144,144,144}{0.429299373201}{0.028004847334}{0.417022016826}{0.029558105338}
  \meshline{144,144,144}{0.368835255759}{0.035380383194}{0.380965964475}{0.033922399128}
  \meshline{144,144,144}{0.321008690041}{0.130301714348}{0.325497328953}{0.127334343574}
  \meshline{144,144,144}{0.311154105388}{0.138407206754}{0.310842717276}{0.138640949024}
  \meshline{144,144,144}{0.267717500611}{0.187940055483}{0.269619310298}{0.185395197424}
  \meshline{144,144,144}{0.815133170194}{0.375662971706}{0.813431749494}{0.381838190833}
  \meshline{144,144,144}{0.806518965736}{0.399246199120}{0.806897123746}{0.398436818334}
  \meshline{144,144,144}{0.798274218031}{0.415167388311}{0.806518965736}{0.399246199120}
  \meshline{144,144,144}{0.813431749494}{0.381838190833}{0.807884817873}{0.395790805552}
  \meshline{144,144,144}{0.815133170194}{0.375662971706}{0.819952193911}{0.357612216687}
  \meshline{144,144,144}{0.821549262025}{0.348860905455}{0.819952193911}{0.357612216687}
  \meshline{144,144,144}{0.822802158010}{0.337599102647}{0.821549262025}{0.348860905455}
  \meshline{144,144,144}{0.761020678769}{0.460054498043}{0.764204708183}{0.457022090934}
  \meshline{144,144,144}{0.734547012288}{0.478376427030}{0.734266476421}{0.478556191076}
  \meshline{144,144,144}{0.647158369491}{0.568148359266}{0.655549267718}{0.568699317414}
  \meshline{144,144,144}{0.734266476421}{0.478556191076}{0.733303856358}{0.479006218118}
  \meshline{144,144,144}{0.738587013819}{0.562552536772}{0.735499105406}{0.563327643881}
  \meshline{144,144,144}{0.413691035246}{0.172320472822}{0.433140817253}{0.157786034084}
  \meshline{144,144,144}{0.355666102428}{0.325674074830}{0.352799518806}{0.306372619535}
  \meshline{144,144,144}{0.243929690195}{0.246683146457}{0.246861540709}{0.236623603232}
  \meshline{144,144,144}{0.256368403164}{0.209018822331}{0.263677764381}{0.195548475429}
  \meshline{144,144,144}{0.256368403164}{0.209018822331}{0.255209603506}{0.212163762579}
  \meshline{144,144,144}{0.255209603506}{0.212163762579}{0.251659502176}{0.220602888329}
  \meshline{144,144,144}{0.251659502176}{0.220602888329}{0.249001565599}{0.228983380610}
  \meshline{144,144,144}{0.263677764381}{0.195548475429}{0.267717500611}{0.187940055483}
  \meshline{144,144,144}{0.246861540709}{0.236623603232}{0.249001565599}{0.228983380610}
  \meshline{144,144,144}{0.225705414491}{0.075769773029}{0.226355014254}{0.075380210040}
  \meshline{144,144,144}{0.407647285458}{0.417509758239}{0.408355194128}{0.418360018219}
  \meshline{144,144,144}{0.466355631460}{0.461757061136}{0.480298855765}{0.468945210512}
  \meshline{144,144,144}{0.450242728504}{0.451941518036}{0.453692487563}{0.454225100865}
  \meshline{144,144,144}{0.473134060375}{0.396560778207}{0.485556067706}{0.407204761317}
  \meshline{144,144,144}{0.502969988932}{0.419534326539}{0.501572404577}{0.418610475211}
  \meshline{144,144,144}{0.484730309320}{0.471271016568}{0.480298855765}{0.468945210512}
  \meshline{144,144,144}{0.406690933852}{0.030332010559}{0.417022016826}{0.029558105338}
  \meshline{144,144,144}{0.806897123746}{0.398436818334}{0.807884817873}{0.395790805552}
  \meshline{144,144,144}{0.931480620769}{0.538642761555}{0.925292245748}{0.552297476458}
  \meshline{144,144,144}{0.777611082606}{0.443994279989}{0.783864186340}{0.436240548753}
  \meshline{144,144,144}{0.764204708183}{0.457022090934}{0.771255654235}{0.450487753841}
  \meshline{144,144,144}{0.353186958633}{0.282100279247}{0.355268372181}{0.266136935825}
  \meshline{144,144,144}{0.243929690195}{0.246683146457}{0.242644570659}{0.257218688017}
  \meshline{144,144,144}{0.242644570659}{0.257218688017}{0.241530630088}{0.263809294116}
  \meshline{144,144,144}{0.240474332407}{0.278849442992}{0.240780231354}{0.289195889850}
  \meshline{144,144,144}{0.241155697342}{0.271937847427}{0.241530630088}{0.263809294116}
  \meshline{144,144,144}{0.240474332407}{0.278849442992}{0.241155697342}{0.271937847427}
  \meshline{144,144,144}{0.226630131229}{0.075238488111}{0.226355014254}{0.075380210040}
  \meshline{144,144,144}{0.207984236974}{0.085418547394}{0.225705414491}{0.075769773029}
  \meshline{144,144,144}{0.407647285458}{0.417509758239}{0.397153927843}{0.406488805689}
  \meshline{144,144,144}{0.417393720733}{0.426989777541}{0.409342242877}{0.419338970532}
  \meshline{144,144,144}{0.391918970364}{0.399452701510}{0.385829739619}{0.392134222406}
  \meshline{144,144,144}{0.498390927966}{0.477682857866}{0.485699466984}{0.471727039038}
  \meshline{144,144,144}{0.526730909913}{0.431935518153}{0.519593335962}{0.428671392366}
  \meshline{144,144,144}{0.535768937785}{0.435755875980}{0.526730909913}{0.431935518153}
  \meshline{144,144,144}{0.636961397876}{0.504685904600}{0.652954462362}{0.503241762606}
  \meshline{144,144,144}{0.601403875678}{0.562941474449}{0.579530384004}{0.559155355086}
  \meshline{144,144,144}{0.036833704993}{0.817687266012}{0.037131874526}{0.811604506860}
  \meshline{144,144,144}{0.660436114116}{0.502583691459}{0.676839184026}{0.499517071339}
  \meshline{144,144,144}{0.660436114116}{0.502583691459}{0.652954462362}{0.503241762606}
  \meshline{144,144,144}{0.352848339948}{0.288848973528}{0.352799518806}{0.306372619535}
  \meshline{144,144,144}{0.249176034826}{0.340093025347}{0.249463887306}{0.340986892512}
  \meshline{144,144,144}{0.187716441322}{0.098798087908}{0.202392662421}{0.088345665904}
  \meshline{144,144,144}{0.295603244800}{0.050201528164}{0.298751202483}{0.049626627620}
  \meshline{144,144,144}{0.226630131229}{0.075238488111}{0.245483334961}{0.066710026452}
  \meshline{144,144,144}{0.202392662421}{0.088345665904}{0.207984236974}{0.085418547394}
  \meshline{144,144,144}{0.170463085284}{0.113030603683}{0.186096432615}{0.100106101207}
  \meshline{144,144,144}{0.147515907782}{0.140320532607}{0.141921171357}{0.148086908181}
  \meshline{144,144,144}{0.187403476195}{0.098990729159}{0.187716441322}{0.098798087908}
  \meshline{144,144,144}{0.152908389584}{0.132736839430}{0.167165514986}{0.116682115991}
  \meshline{144,144,144}{0.152908389584}{0.132736839430}{0.150704574081}{0.135378359428}
  \meshline{144,144,144}{0.170463085284}{0.113030603683}{0.167165514986}{0.116682115991}
  \meshline{144,144,144}{0.186096432615}{0.100106101207}{0.187403476195}{0.098990729159}
  \meshline{144,144,144}{0.257003789104}{0.062208152827}{0.245483334961}{0.066710026452}
  \meshline{144,144,144}{0.257003789104}{0.062208152827}{0.263598885672}{0.060077991151}
  \meshline{144,144,144}{0.295603244800}{0.050201528164}{0.286617786638}{0.052779727929}
  \meshline{144,144,144}{0.355555659645}{0.469720915653}{0.341816133547}{0.460768202912}
  \meshline{144,144,144}{0.316525517255}{0.439621232429}{0.320504115332}{0.443377841298}
  \meshline{144,144,144}{0.690149910211}{0.568632129663}{0.675010267715}{0.569217884343}
  \meshline{144,144,144}{0.790185263530}{0.544840667245}{0.778499640737}{0.550778831452}
  \meshline{144,144,144}{0.763548436687}{0.555871101139}{0.756531084446}{0.558566534543}
  \meshline{144,144,144}{0.738587013819}{0.562552536772}{0.756531084446}{0.558566534543}
  \meshline{144,144,144}{0.735499105406}{0.563327643881}{0.717354255688}{0.566195823362}
  \meshline{144,144,144}{0.712013946585}{0.567148935537}{0.717354255688}{0.566195823362}
  \meshline{144,144,144}{0.888788532469}{0.423198849826}{0.892488135860}{0.409579951079}
  \meshline{144,144,144}{0.240811360010}{0.296284046158}{0.241046766189}{0.298699529447}
  \meshline{144,144,144}{0.123267175068}{0.356497635631}{0.118971069715}{0.344130897089}
  \meshline{144,144,144}{0.112594924230}{0.314402493080}{0.111402535511}{0.307112928721}
  \meshline{144,144,144}{0.110424936513}{0.247836728215}{0.112212184264}{0.232850331240}
  \meshline{144,144,144}{0.109383506151}{0.275254656519}{0.109440633452}{0.276461440904}
  \meshline{144,144,144}{0.109440633452}{0.276461440904}{0.109739022373}{0.280410466634}
  \meshline{144,144,144}{0.118271061424}{0.203980018648}{0.113540607550}{0.224641116168}
  \meshline{144,144,144}{0.112594924230}{0.314402493080}{0.113773710839}{0.322586263621}
  \meshline{144,144,144}{0.109739022373}{0.280410466634}{0.111402535511}{0.307112928721}
  \meshline{144,144,144}{0.136906514143}{0.157417106347}{0.134041257772}{0.162225873533}
  \meshline{144,144,144}{0.119215292919}{0.200669902750}{0.125355480390}{0.181619575888}
  \meshline{144,144,144}{0.134041257772}{0.162225873533}{0.132652383534}{0.165232258671}
  \meshline{144,144,144}{0.286617786638}{0.052779727929}{0.280377061034}{0.054581568361}
  \meshline{144,144,144}{0.263598885672}{0.060077991151}{0.273094425543}{0.057178479443}
  \meshline{144,144,144}{0.280377061034}{0.054581568361}{0.273094425543}{0.057178479443}
  \meshline{144,144,144}{0.367241966200}{0.035737034146}{0.368835255759}{0.035380383194}
  \meshline{144,144,144}{0.367241966200}{0.035737034146}{0.352559174732}{0.038078743443}
  \meshline{144,144,144}{0.647506754993}{0.904109811458}{0.647382603455}{0.894335324408}
  \meshline{144,144,144}{0.868505992744}{0.470566632595}{0.863720101689}{0.479186721845}
  \meshline{144,144,144}{0.763548436687}{0.555871101139}{0.778499640737}{0.550778831452}
  \meshline{144,144,144}{0.834951446237}{0.513704377048}{0.838528050390}{0.510550815277}
  \meshline{144,144,144}{0.802938873115}{0.538620487086}{0.796799600843}{0.541908721188}
  \meshline{144,144,144}{0.840111309018}{0.508669645018}{0.838528050390}{0.510550815277}
  \meshline{144,144,144}{0.352559174732}{0.038078743443}{0.340087736420}{0.040112288592}
  \meshline{144,144,144}{0.338197211413}{0.040547592179}{0.340087736420}{0.040112288592}
  \meshline{144,144,144}{0.317560114388}{0.044855821099}{0.307241250170}{0.047717848990}
  \meshline{144,144,144}{0.317560114388}{0.044855821099}{0.336396893238}{0.041089118911}
  \meshline{144,144,144}{0.338197211413}{0.040547592179}{0.336396893238}{0.041089118911}
  \meshline{144,144,144}{0.298751202483}{0.049626627620}{0.307241250170}{0.047717848990}
  \meshline{144,144,144}{0.352848339948}{0.288848973528}{0.352690756143}{0.286662364361}
  \meshline{144,144,144}{0.355705366366}{0.325907658116}{0.355680007262}{0.325804522380}
  \meshline{144,144,144}{0.352690756143}{0.286662364361}{0.352753474530}{0.285127057260}
  \meshline{144,144,144}{0.258760390080}{0.364770347478}{0.258928958934}{0.365148458091}
  \meshline{144,144,144}{0.248967402391}{0.339042308352}{0.249176034826}{0.340093025347}
  \meshline{144,144,144}{0.242428241975}{0.309235617122}{0.243056666399}{0.314869037861}
  \meshline{144,144,144}{0.241046766189}{0.298699529447}{0.242428241975}{0.309235617122}
  \meshline{144,144,144}{0.240780231354}{0.289195889850}{0.240811360010}{0.296284046158}
  \meshline{144,144,144}{0.316525517255}{0.439621232429}{0.311634901518}{0.434955583782}
  \meshline{144,144,144}{0.289469880217}{0.501411583990}{0.294973990516}{0.504212777728}
  \meshline{144,144,144}{0.287097338917}{0.409378208001}{0.282940761697}{0.403664607231}
  \meshline{144,144,144}{0.306723621819}{0.430602250539}{0.311634901518}{0.434955583782}
  \meshline{144,144,144}{0.302711390505}{0.426441203051}{0.294571544151}{0.417565311914}
  \meshline{144,144,144}{0.542230998857}{0.492787955352}{0.529488007183}{0.489212832409}
  \meshline{144,144,144}{0.447149585025}{0.607028421526}{0.458275960011}{0.610185625834}
  \meshline{144,144,144}{0.659772513086}{0.568633551658}{0.675010267715}{0.569217884343}
  \meshline{144,144,144}{0.712013946585}{0.567148935537}{0.695475375109}{0.568326527308}
  \meshline{144,144,144}{0.647158369491}{0.568148359266}{0.635201191954}{0.567306877763}
  \meshline{144,144,144}{0.628889298040}{0.566394351190}{0.635201191954}{0.567306877763}
  \meshline{144,144,144}{0.617939953855}{0.565350351086}{0.604340268102}{0.563429404183}
  \meshline{144,144,144}{0.659772513086}{0.568633551658}{0.655549267718}{0.568699317414}
  \meshline{144,144,144}{0.466164565686}{0.652166438408}{0.458601178052}{0.650042056221}
  \meshline{144,144,144}{0.370303048290}{0.633590099066}{0.360690372438}{0.632860200890}
  \meshline{144,144,144}{0.554914739612}{0.553666804941}{0.565727036960}{0.556038455343}
  \meshline{144,144,144}{0.583841473345}{0.649377398889}{0.572481103213}{0.645520635919}
  \meshline{144,144,144}{0.604340268102}{0.563429404183}{0.601403875678}{0.562941474449}
  \meshline{144,144,144}{0.617939953855}{0.565350351086}{0.628889298040}{0.566394351190}
  \meshline{144,144,144}{0.636961397876}{0.504685904600}{0.628059371163}{0.504687696978}
  \meshline{144,144,144}{0.549228085806}{0.494824359109}{0.557517420735}{0.496739663492}
  \meshline{144,144,144}{0.562998711486}{0.498056824825}{0.570282044846}{0.499379528883}
  \meshline{144,144,144}{0.554914739612}{0.553666804941}{0.545644194611}{0.551381132351}
  \meshline{144,144,144}{0.615270512248}{0.504237724623}{0.607660639164}{0.504138804582}
  \meshline{144,144,144}{0.570282044846}{0.499379528883}{0.576917521982}{0.500593007779}
  \meshline{144,144,144}{0.607660639164}{0.504138804582}{0.592413645826}{0.502728045890}
  \meshline{144,144,144}{0.857903790572}{0.486987962147}{0.855407200837}{0.490704341545}
  \meshline{144,144,144}{0.857903790572}{0.486987962147}{0.863720101689}{0.479186721845}
  \meshline{144,144,144}{0.849053483513}{0.498928198911}{0.855407200837}{0.490704341545}
  \meshline{144,144,144}{0.332423460037}{0.452991884642}{0.341816133547}{0.460768202912}
  \meshline{144,144,144}{0.116083200579}{0.331896762442}{0.113773710839}{0.322586263621}
  \meshline{144,144,144}{0.165154968766}{0.422192871006}{0.174619768002}{0.432497391110}
  \meshline{144,144,144}{0.118971069715}{0.344130897089}{0.116083200579}{0.331896762442}
  \meshline{144,144,144}{0.124792764905}{0.360941436320}{0.123267175068}{0.356497635631}
  \meshline{144,144,144}{0.131920303197}{0.376585140748}{0.124792764905}{0.360941436320}
  \meshline{144,144,144}{0.373505486637}{0.372483480900}{0.380565144590}{0.384762901660}
  \meshline{144,144,144}{0.371532920686}{0.369411241148}{0.365275878689}{0.355462348905}
  \meshline{144,144,144}{0.258928958934}{0.365148458091}{0.267808021679}{0.381710357887}
  \meshline{144,144,144}{0.520597271164}{0.486174199707}{0.512689019863}{0.483374196792}
  \meshline{144,144,144}{0.562998711486}{0.498056824825}{0.557517420735}{0.496739663492}
  \meshline{144,144,144}{0.591831276225}{0.502667268117}{0.592413645826}{0.502728045890}
  \meshline{144,144,144}{0.576917521982}{0.500593007779}{0.591831276225}{0.502667268117}
  \meshline{144,144,144}{0.612270186746}{0.449785894800}{0.609808221985}{0.449922896361}
  \meshline{144,144,144}{0.495247376399}{0.536572780897}{0.501942608010}{0.538675341533}
  \meshline{144,144,144}{0.549228085806}{0.494824359109}{0.542230998857}{0.492787955352}
  \meshline{144,144,144}{0.504328383875}{0.480032964686}{0.512689019863}{0.483374196792}
  \meshline{144,144,144}{0.485699466984}{0.471727039038}{0.484730309320}{0.471271016568}
  \meshline{144,144,144}{0.482775552962}{0.617063510763}{0.476371136937}{0.615204131026}
  \meshline{144,144,144}{0.403322610998}{0.497999423165}{0.427371289158}{0.509842426732}
  \meshline{144,144,144}{0.435604889220}{0.513474320592}{0.447927314845}{0.518900567532}
  \meshline{144,144,144}{0.369673542595}{0.534415793980}{0.367827952813}{0.533820364126}
  \meshline{144,144,144}{0.447927314845}{0.518900567532}{0.457533732649}{0.522620061357}
  \meshline{144,144,144}{0.435604889220}{0.513474320592}{0.431970713449}{0.511989221637}
  \meshline{144,144,144}{0.431970713449}{0.511989221637}{0.427371289158}{0.509842426732}
  \meshline{144,144,144}{0.387184566389}{0.540864111997}{0.402126985003}{0.546335179957}
  \meshline{144,144,144}{0.355555659645}{0.469720915653}{0.359479020763}{0.472635267777}
  \meshline{144,144,144}{0.435336083191}{0.557794601974}{0.418690342336}{0.552148238633}
  \meshline{144,144,144}{0.417425128283}{0.551663181074}{0.418690342336}{0.552148238633}
  \meshline{144,144,144}{0.406566032357}{0.596642915144}{0.388266755957}{0.592467869068}
  \meshline{144,144,144}{0.372778489837}{0.480827523611}{0.359479020763}{0.472635267777}
  \meshline{144,144,144}{0.332423460037}{0.452991884642}{0.320504115332}{0.443377841298}
  \meshline{144,144,144}{0.321024594451}{0.515110431390}{0.332788506028}{0.520263070136}
  \meshline{144,144,144}{0.160313616711}{0.582356377330}{0.169729781492}{0.579042384054}
  \meshline{144,144,144}{0.372778489837}{0.480827523611}{0.382384277009}{0.486873078756}
  \meshline{144,144,144}{0.389238851955}{0.490491931149}{0.397410789611}{0.495081413548}
  \meshline{144,144,144}{0.435169375294}{0.603988997353}{0.447149585025}{0.607028421526}
  \meshline{144,144,144}{0.349269860146}{0.526756439109}{0.342641308613}{0.523875071658}
  \meshline{144,144,144}{0.356599308489}{0.529382759026}{0.367827952813}{0.533820364126}
  \meshline{144,144,144}{0.294973990516}{0.504212777728}{0.302145851213}{0.507302917914}
  \meshline{144,144,144}{0.422340499885}{0.641556224533}{0.431287726169}{0.643574279225}
  \meshline{144,144,144}{0.413029309849}{0.598407417951}{0.406566032357}{0.596642915144}
  \meshline{144,144,144}{0.413810751946}{0.550369198506}{0.417425128283}{0.551663181074}
  \meshline{144,144,144}{0.386764033611}{0.592054634016}{0.388266755957}{0.592467869068}
  \meshline{144,144,144}{0.358021300916}{0.586100595556}{0.386764033611}{0.592054634016}
  \meshline{144,144,144}{0.425591085129}{0.601313524491}{0.413029309849}{0.598407417951}
  \meshline{144,144,144}{0.253879081943}{0.639229419485}{0.270525523732}{0.636098147969}
  \meshline{144,144,144}{0.370303048290}{0.633590099066}{0.378485289355}{0.634667447292}
  \meshline{144,144,144}{0.384462061538}{0.539998395345}{0.387184566389}{0.540864111997}
  \meshline{144,144,144}{0.412702071986}{0.639742017753}{0.408155633356}{0.638971586479}
  \meshline{144,144,144}{0.389238851955}{0.490491931149}{0.382384277009}{0.486873078756}
  \meshline{144,144,144}{0.403322610998}{0.497999423165}{0.397410789611}{0.495081413548}
  \meshline{144,144,144}{0.413810751946}{0.550369198506}{0.402126985003}{0.546335179957}
  \meshline{144,144,144}{0.089922772365}{0.627285610519}{0.077737699341}{0.643451463935}
  \meshline{144,144,144}{0.302145851213}{0.507302917914}{0.315694980501}{0.513174105019}
  \meshline{144,144,144}{0.318172577759}{0.514031416459}{0.321024594451}{0.515110431390}
  \meshline{144,144,144}{0.351496821498}{0.584730316659}{0.337148266878}{0.582100544059}
  \meshline{144,144,144}{0.337148266878}{0.582100544059}{0.333772536583}{0.581750591873}
  \meshline{144,144,144}{0.342641308613}{0.523875071658}{0.332788506028}{0.520263070136}
  \meshline{144,144,144}{0.369673542595}{0.534415793980}{0.384462061538}{0.539998395345}
  \meshline{144,144,144}{0.356599308489}{0.529382759026}{0.349269860146}{0.526756439109}
  \meshline{144,144,144}{0.593347529571}{0.448979646721}{0.609808221985}{0.449922896361}
  \meshline{144,144,144}{0.802938873115}{0.538620487086}{0.810430778366}{0.533287683931}
  \meshline{144,144,144}{0.790185263530}{0.544840667245}{0.796799600843}{0.541908721188}
  \meshline{144,144,144}{0.821904151171}{0.525575154565}{0.810430778366}{0.533287683931}
  \meshline{144,144,144}{0.834951446237}{0.513704377048}{0.821904151171}{0.525575154565}
  \meshline{144,144,144}{0.507194516454}{0.787227102453}{0.508474963066}{0.788120931381}
  \meshline{144,144,144}{0.880670653383}{0.445942449807}{0.871207062103}{0.465536874993}
  \meshline{144,144,144}{0.849053483513}{0.498928198911}{0.840111309018}{0.508669645018}
  \meshline{144,144,144}{0.871207062103}{0.465536874993}{0.868505992744}{0.470566632595}
  \meshline{144,144,144}{0.248967402391}{0.339042308352}{0.243056666399}{0.314869037861}
  \meshline{144,144,144}{0.429278306217}{0.303738963937}{0.429464354917}{0.312017682103}
  \meshline{144,144,144}{0.365275878689}{0.355462348905}{0.362479784105}{0.349379446427}
  \meshline{144,144,144}{0.380565144590}{0.384762901660}{0.385829739619}{0.392134222406}
  \meshline{144,144,144}{0.362009194189}{0.347813458380}{0.362479784105}{0.349379446427}
  \meshline{144,144,144}{0.355705366366}{0.325907658116}{0.362009194189}{0.347813458380}
  \meshline{144,144,144}{0.371532920686}{0.369411241148}{0.373505486637}{0.372483480900}
  \meshline{144,144,144}{0.282940761697}{0.403664607231}{0.274385596295}{0.392246686908}
  \meshline{144,144,144}{0.258760390080}{0.364770347478}{0.249463887306}{0.340986892512}
  \meshline{144,144,144}{0.267808021679}{0.381710357887}{0.274385596295}{0.392246686908}
  \meshline{144,144,144}{0.550691675222}{0.441049975707}{0.553413642508}{0.441774622853}
  \meshline{144,144,144}{0.549208556256}{0.440520633011}{0.550691675222}{0.441049975707}
  \meshline{144,144,144}{0.581823075115}{0.447910704618}{0.593347529571}{0.448979646721}
  \meshline{144,144,144}{0.589270088230}{0.392993731829}{0.588322175858}{0.392880899439}
  \meshline{144,144,144}{0.571989833340}{0.446196262533}{0.581823075115}{0.447910704618}
  \meshline{144,144,144}{0.422340499885}{0.641556224533}{0.412702071986}{0.639742017753}
  \meshline{144,144,144}{0.385589703623}{0.635424462760}{0.402900676482}{0.638276642823}
  \meshline{144,144,144}{0.416192891545}{0.698479210737}{0.420780355433}{0.699297561066}
  \meshline{144,144,144}{0.385589703623}{0.635424462760}{0.378485289355}{0.634667447292}
  \meshline{144,144,144}{0.322172404092}{0.579872068369}{0.315948884805}{0.578759773041}
  \meshline{144,144,144}{0.351496821498}{0.584730316659}{0.356125667833}{0.585614719957}
  \meshline{144,144,144}{0.358021300916}{0.586100595556}{0.356125667833}{0.585614719957}
  \meshline{144,144,144}{0.282589448792}{0.574508489119}{0.271958527256}{0.573856554549}
  \meshline{144,144,144}{0.949233944853}{0.485573196704}{0.948307079063}{0.490861487948}
  \meshline{144,144,144}{0.230574702306}{0.471552750123}{0.216364740991}{0.463169167115}
  \meshline{144,144,144}{0.151062129695}{0.406331567919}{0.147282124907}{0.402082666154}
  \meshline{144,144,144}{0.230574702306}{0.471552750123}{0.231213791892}{0.472009924345}
  \meshline{144,144,144}{0.183313535685}{0.439317790482}{0.186774447971}{0.442634220767}
  \meshline{144,144,144}{0.231637190526}{0.472294722339}{0.252101059319}{0.483744476821}
  \meshline{144,144,144}{0.186774447971}{0.442634220767}{0.191395108728}{0.446138648018}
  \meshline{144,144,144}{0.165154968766}{0.422192871006}{0.157319168468}{0.414826877538}
  \meshline{144,144,144}{0.174619768002}{0.432497391110}{0.183313535685}{0.439317790482}
  \meshline{144,144,144}{0.141003268553}{0.393055505727}{0.132723924745}{0.378252774216}
  \meshline{144,144,144}{0.131920303197}{0.376585140748}{0.132723924745}{0.378252774216}
  \meshline{144,144,144}{0.212257356325}{0.460224094556}{0.216364740991}{0.463169167115}
  \meshline{144,144,144}{0.191395108728}{0.446138648018}{0.200623005772}{0.453005838859}
  \meshline{144,144,144}{0.151062129695}{0.406331567919}{0.157319168468}{0.414826877538}
  \meshline{144,144,144}{0.141003268553}{0.393055505727}{0.143889749535}{0.397159442981}
  \meshline{144,144,144}{0.287097338917}{0.409378208001}{0.294571544151}{0.417565311914}
  \meshline{144,144,144}{0.302711390505}{0.426441203051}{0.306723621819}{0.430602250539}
  \meshline{144,144,144}{0.212257356325}{0.460224094556}{0.200623005772}{0.453005838859}
  \meshline{144,144,144}{0.425591085129}{0.601313524491}{0.435169375294}{0.603988997353}
  \meshline{144,144,144}{0.443177606542}{0.560561617192}{0.435336083191}{0.557794601974}
  \meshline{144,144,144}{0.484441093151}{0.573657019619}{0.467038622162}{0.568134467782}
  \meshline{144,144,144}{0.408155633356}{0.638971586479}{0.402900676482}{0.638276642823}
  \meshline{144,144,144}{0.298073021377}{0.576414343694}{0.315948884805}{0.578759773041}
  \meshline{144,144,144}{0.315694980501}{0.513174105019}{0.318172577759}{0.514031416459}
  \meshline{144,144,144}{0.231637190526}{0.472294722339}{0.231213791892}{0.472009924345}
  \meshline{144,144,144}{0.252101059319}{0.483744476821}{0.255926331502}{0.485752756741}
  \meshline{144,144,144}{0.263380692450}{0.489374596225}{0.270222390949}{0.492427158804}
  \meshline{144,144,144}{0.147282124907}{0.402082666154}{0.143889749535}{0.397159442981}
  \meshline{144,144,144}{0.289469880217}{0.501411583990}{0.277070582650}{0.496032484234}
  \meshline{144,144,144}{0.270222390949}{0.492427158804}{0.277070582650}{0.496032484234}
  \meshline{144,144,144}{0.263380692450}{0.489374596225}{0.255926331502}{0.485752756741}
  \meshline{144,144,144}{0.200150489122}{0.574556887987}{0.189668975659}{0.575217425487}
  \meshline{144,144,144}{0.246808296317}{0.641348767876}{0.223815201689}{0.649009182635}
  \meshline{144,144,144}{0.145397358479}{0.586391988689}{0.150272131338}{0.585131818280}
  \meshline{144,144,144}{0.468071084123}{0.526965446083}{0.477759995935}{0.530445840455}
  \meshline{144,144,144}{0.457533732649}{0.522620061357}{0.468071084123}{0.526965446083}
  \meshline{144,144,144}{0.493887075907}{0.536126381926}{0.483412425274}{0.532423225605}
  \meshline{144,144,144}{0.451920795836}{0.563267964981}{0.460378636344}{0.566092552823}
  \meshline{144,144,144}{0.501942608010}{0.538675341533}{0.517266115693}{0.543573155766}
  \meshline{144,144,144}{0.478580668363}{0.530739868828}{0.477759995935}{0.530445840455}
  \meshline{144,144,144}{0.509284535433}{0.581155251325}{0.490768843946}{0.575562223512}
  \meshline{144,144,144}{0.478580668363}{0.530739868828}{0.483412425274}{0.532423225605}
  \meshline{144,144,144}{0.535838500295}{0.548899626282}{0.520298440938}{0.544454863959}
  \meshline{144,144,144}{0.533197818742}{0.588093930587}{0.535469439942}{0.588700499675}
  \meshline{144,144,144}{0.520908741398}{0.584531589937}{0.533197818742}{0.588093930587}
  \meshline{144,144,144}{0.490768843946}{0.575562223512}{0.484441093151}{0.573657019619}
  \meshline{144,144,144}{0.493887075907}{0.536126381926}{0.495247376399}{0.536572780897}
  \meshline{144,144,144}{0.535838500295}{0.548899626282}{0.545644194611}{0.551381132351}
  \meshline{144,144,144}{0.576362394762}{0.558492778706}{0.579530384004}{0.559155355086}
  \meshline{144,144,144}{0.520298440938}{0.544454863959}{0.517266115693}{0.543573155766}
  \meshline{144,144,144}{0.511830504127}{0.581917555379}{0.509284535433}{0.581155251325}
  \meshline{144,144,144}{0.478018341629}{0.713525858423}{0.471831653959}{0.711605617681}
  \meshline{144,144,144}{0.557411240128}{0.594740141156}{0.557056842251}{0.594634178361}
  \meshline{144,144,144}{0.520908741398}{0.584531589937}{0.511830504127}{0.581917555379}
  \meshline{144,144,144}{0.576362394762}{0.558492778706}{0.565727036960}{0.556038455343}
  \meshline{144,144,144}{0.535469439942}{0.588700499675}{0.554195066760}{0.593843539828}
  \meshline{144,144,144}{0.570443018024}{0.689543560250}{0.554189390777}{0.682521427964}
  \meshline{144,144,144}{0.499707764513}{0.622110920653}{0.482775552962}{0.617063510763}
  \meshline{144,144,144}{0.229221590890}{0.572646748861}{0.220731207354}{0.573133323832}
  \meshline{144,144,144}{0.200150489122}{0.574556887987}{0.210928741094}{0.573262280223}
  \meshline{144,144,144}{0.250177739403}{0.572552653733}{0.251220494413}{0.572678352635}
  \meshline{144,144,144}{0.251220494413}{0.572678352635}{0.267246085492}{0.573229250816}
  \meshline{144,144,144}{0.247048830795}{0.572498641947}{0.250177739403}{0.572552653733}
  \meshline{144,144,144}{0.247048830795}{0.572498641947}{0.233075508624}{0.572213006192}
  \meshline{144,144,144}{0.322172404092}{0.579872068369}{0.333772536583}{0.581750591873}
  \meshline{144,144,144}{0.271958527256}{0.573856554549}{0.267246085492}{0.573229250816}
  \meshline{144,144,144}{0.298073021377}{0.576414343694}{0.297011479297}{0.576201047464}
  \meshline{144,144,144}{0.282589448792}{0.574508489119}{0.295434741151}{0.575963801392}
  \meshline{144,144,144}{0.297011479297}{0.576201047464}{0.295434741151}{0.575963801392}
  \meshline{144,144,144}{0.150272131338}{0.585131818280}{0.160313616711}{0.582356377330}
  \meshline{144,144,144}{0.451920795836}{0.563267964981}{0.443177606542}{0.560561617192}
  \meshline{144,144,144}{0.467038622162}{0.568134467782}{0.460378636344}{0.566092552823}
  \meshline{144,144,144}{0.138936305663}{0.589299626419}{0.118121631789}{0.601122135113}
  \meshline{144,144,144}{0.189668975659}{0.575217425487}{0.178782314924}{0.577290613914}
  \meshline{144,144,144}{0.275931044650}{0.634855798257}{0.270525523732}{0.636098147969}
  \meshline{144,144,144}{0.466164565686}{0.652166438408}{0.480618463399}{0.656128890679}
  \meshline{144,144,144}{0.220731207354}{0.573133323832}{0.210928741094}{0.573262280223}
  \meshline{144,144,144}{0.178782314924}{0.577290613914}{0.169729781492}{0.579042384054}
  \meshline{144,144,144}{0.438203806928}{0.645002039409}{0.454473180404}{0.649072263840}
  \meshline{144,144,144}{0.106009792763}{0.610408667576}{0.104167267205}{0.611776270015}
  \meshline{144,144,144}{0.438203806928}{0.645002039409}{0.431287726169}{0.643574279225}
  \meshline{144,144,144}{0.381801252723}{0.695570621050}{0.366341160833}{0.695665936201}
  \meshline{144,144,144}{0.345557158195}{0.631857997958}{0.332154617789}{0.631103320866}
  \meshline{144,144,144}{0.246808296317}{0.641348767876}{0.253879081943}{0.639229419485}
  \meshline{144,144,144}{0.294312158498}{0.632835675714}{0.303548396868}{0.632285393742}
  \meshline{144,144,144}{0.301740876190}{0.775854377796}{0.303800440098}{0.774670884009}
  \meshline{144,144,144}{0.402455123040}{0.750565045136}{0.414507844697}{0.751718726661}
  \meshline{144,144,144}{0.335377188627}{0.698298046939}{0.322406481788}{0.701020906147}
  \meshline{144,144,144}{0.288140445310}{0.633470449101}{0.275931044650}{0.634855798257}
  \meshline{144,144,144}{0.223815201689}{0.649009182635}{0.222563533251}{0.649527815252}
  \meshline{144,144,144}{0.201066480910}{0.659846566215}{0.222563533251}{0.649527815252}
  \meshline{144,144,144}{0.047592748174}{0.729561926490}{0.049545102314}{0.718458531550}
  \meshline{144,144,144}{0.179674405893}{0.673991155163}{0.184742855462}{0.669991028916}
  \meshline{144,144,144}{0.091814929255}{0.624338685188}{0.097949560535}{0.618318882292}
  \meshline{144,144,144}{0.184742855462}{0.669991028916}{0.200647014947}{0.660117651970}
  \meshline{144,144,144}{0.157164798028}{0.694917127562}{0.171614803297}{0.680315944015}
  \meshline{144,144,144}{0.200973037972}{0.659899665408}{0.201066480910}{0.659846566215}
  \meshline{144,144,144}{0.171614803297}{0.680315944015}{0.179674405893}{0.673991155163}
  \meshline{144,144,144}{0.102785458171}{0.613209015353}{0.104167267205}{0.611776270015}
  \meshline{144,144,144}{0.102785458171}{0.613209015353}{0.097949560535}{0.618318882292}
  \meshline{144,144,144}{0.138936305663}{0.589299626419}{0.145397358479}{0.586391988689}
  \meshline{144,144,144}{0.118027513321}{0.601175111477}{0.118121631789}{0.601122135113}
  \meshline{144,144,144}{0.117729239820}{0.601417624114}{0.118027513321}{0.601175111477}
  \meshline{144,144,144}{0.089922772365}{0.627285610519}{0.091814929255}{0.624338685188}
  \meshline{144,144,144}{0.073012643335}{0.653291724631}{0.067543298350}{0.663144474912}
  \meshline{144,144,144}{0.416192891545}{0.698479210737}{0.406229399421}{0.697348572941}
  \meshline{144,144,144}{0.458601178052}{0.650042056221}{0.454473180404}{0.649072263840}
  \meshline{144,144,144}{0.106009792763}{0.610408667576}{0.117729239820}{0.601417624114}
  \meshline{144,144,144}{0.073012643335}{0.653291724631}{0.077737699341}{0.643451463935}
  \meshline{144,144,144}{0.062397035812}{0.675937930347}{0.067543298350}{0.663144474912}
  \meshline{144,144,144}{0.143297082090}{0.711277561482}{0.138016228483}{0.718837684352}
  \meshline{144,144,144}{0.053489871911}{0.704858334792}{0.055003625670}{0.697384767119}
  \meshline{144,144,144}{0.062397035812}{0.675937930347}{0.057587488669}{0.688813653291}
  \meshline{144,144,144}{0.055003625670}{0.697384767119}{0.057587488669}{0.688813653291}
  \meshline{144,144,144}{0.044168750183}{0.747271576455}{0.046986143200}{0.731885001631}
  \meshline{144,144,144}{0.053489871911}{0.704858334792}{0.049545102314}{0.718458531550}
  \meshline{144,144,144}{0.152391973145}{0.699631231619}{0.157164798028}{0.694917127562}
  \meshline{144,144,144}{0.043293161919}{0.752954879854}{0.042322141908}{0.761105159639}
  \meshline{144,144,144}{0.046986143200}{0.731885001631}{0.047592748174}{0.729561926490}
  \meshline{144,144,144}{0.044168750183}{0.747271576455}{0.043293161919}{0.752954879854}
  \meshline{144,144,144}{0.040082888127}{0.779325188294}{0.041358196154}{0.770055887417}
  \meshline{144,144,144}{0.041358196154}{0.770055887417}{0.042322141908}{0.761105159639}
  \meshline{144,144,144}{0.501404402356}{0.622611790018}{0.499707764513}{0.622110920653}
  \meshline{144,144,144}{0.542426015982}{0.635487517449}{0.544242391632}{0.636029822716}
  \meshline{144,144,144}{0.443598145776}{0.703647407697}{0.457524396662}{0.707189833074}
  \meshline{144,144,144}{0.501270857873}{0.662687170440}{0.495490073383}{0.660737166759}
  \meshline{144,144,144}{0.476371136937}{0.615204131026}{0.465746518146}{0.612154083820}
  \meshline{144,144,144}{0.152391973145}{0.699631231619}{0.149840044585}{0.702918226782}
  \meshline{144,144,144}{0.226414000803}{0.752275023533}{0.220458453079}{0.759254712057}
  \meshline{144,144,144}{0.121106088829}{0.750726955695}{0.128061106688}{0.735794668793}
  \meshline{144,144,144}{0.130877498364}{0.731161478857}{0.138016228483}{0.718837684352}
  \meshline{144,144,144}{0.149840044585}{0.702918226782}{0.143297082090}{0.711277561482}
  \meshline{144,144,144}{0.226414000803}{0.752275023533}{0.227719606825}{0.750981948389}
  \meshline{144,144,144}{0.479011562778}{0.713885407821}{0.478018341629}{0.713525858423}
  \meshline{144,144,144}{0.457524396662}{0.707189833074}{0.460331661485}{0.707967847470}
  \meshline{144,144,144}{0.443598145776}{0.703647407697}{0.434299048483}{0.701684880078}
  \meshline{144,144,144}{0.417207472003}{0.751982406210}{0.418084642479}{0.752111833109}
  \meshline{144,144,144}{0.362901697242}{0.695646425890}{0.366341160833}{0.695665936201}
  \meshline{144,144,144}{0.401109506241}{0.696787766823}{0.402761907983}{0.696911429412}
  \meshline{144,144,144}{0.384059256718}{0.695625192075}{0.401109506241}{0.696787766823}
  \meshline{144,144,144}{0.434299048483}{0.701684880078}{0.420780355433}{0.699297561066}
  \meshline{144,144,144}{0.402761907983}{0.696911429412}{0.406229399421}{0.697348572941}
  \meshline{144,144,144}{0.384059256718}{0.695625192075}{0.381801252723}{0.695570621050}
  \meshline{144,144,144}{0.554189390777}{0.682521427964}{0.551087697125}{0.681184266832}
  \meshline{144,144,144}{0.501404402356}{0.622611790018}{0.501824009857}{0.622738129504}
  \meshline{144,144,144}{0.120565544649}{0.751913698876}{0.114131286571}{0.767961299420}
  \meshline{144,144,144}{0.039156972210}{0.786002552333}{0.040082888127}{0.779325188294}
  \meshline{144,144,144}{0.038056160655}{0.798452980692}{0.039156972210}{0.786002552333}
  \meshline{144,144,144}{0.107838829460}{0.788038975615}{0.110087215564}{0.781364488836}
  \meshline{144,144,144}{0.491948300233}{0.659649081251}{0.495490073383}{0.660737166759}
  \meshline{144,144,144}{0.458352020795}{0.762038239485}{0.452163453780}{0.760022329189}
  \meshline{144,144,144}{0.316563865905}{0.702057539698}{0.322406481788}{0.701020906147}
  \meshline{144,144,144}{0.351357748424}{0.632043244341}{0.345557158195}{0.631857997958}
  \meshline{144,144,144}{0.361770081962}{0.695699811286}{0.362901697242}{0.695646425890}
  \meshline{144,144,144}{0.292782130344}{0.632864904981}{0.294312158498}{0.632835675714}
  \meshline{144,144,144}{0.313200934521}{0.631583664207}{0.314461701435}{0.631557412041}
  \meshline{144,144,144}{0.314461701435}{0.631557412041}{0.332154617789}{0.631103320866}
  \meshline{144,144,144}{0.303548396868}{0.632285393742}{0.312331876163}{0.631672697111}
  \meshline{144,144,144}{0.292782130344}{0.632864904981}{0.288140445310}{0.633470449101}
  \meshline{144,144,144}{0.358817480484}{0.696001046095}{0.335377188627}{0.698298046939}
  \meshline{144,144,144}{0.360690372438}{0.632860200890}{0.351357748424}{0.632043244341}
  \meshline{144,144,144}{0.313200934521}{0.631583664207}{0.312331876163}{0.631672697111}
  \meshline{144,144,144}{0.293871392274}{0.708939692251}{0.293981853166}{0.708909443073}
  \meshline{144,144,144}{0.313943441369}{0.702666400270}{0.293981853166}{0.708909443073}
  \meshline{144,144,144}{0.293871392274}{0.708939692251}{0.293690035830}{0.709010858568}
  \meshline{144,144,144}{0.240144459925}{0.739459360778}{0.236051317337}{0.743344637703}
  \meshline{144,144,144}{0.276394514606}{0.716146967548}{0.269506273394}{0.719817785816}
  \meshline{144,144,144}{0.257621029925}{0.726548541473}{0.269506273394}{0.719817785816}
  \meshline{144,144,144}{0.293690035830}{0.709010858568}{0.276394514606}{0.716146967548}
  \meshline{144,144,144}{0.240757380771}{0.739000449919}{0.240144459925}{0.739459360778}
  \meshline{144,144,144}{0.242230536320}{0.737998212201}{0.257621029925}{0.726548541473}
  \meshline{144,144,144}{0.036833704993}{0.817687266012}{0.035823838190}{0.834017399447}
  \meshline{144,144,144}{0.283163559785}{0.790597895334}{0.286855325540}{0.787422857618}
  \meshline{144,144,144}{0.286855325540}{0.787422857618}{0.300427852627}{0.776896673099}
  \meshline{144,144,144}{0.253415962191}{0.833952170010}{0.257367842070}{0.825917694257}
  \meshline{144,144,144}{0.317007567094}{0.766942164320}{0.319651411796}{0.765609230423}
  \meshline{144,144,144}{0.373421067518}{0.751115637605}{0.356439766559}{0.753647460644}
  \meshline{144,144,144}{0.317007567094}{0.766942164320}{0.303800440098}{0.774670884009}
  \meshline{144,144,144}{0.323305694698}{0.764150841518}{0.319651411796}{0.765609230423}
  \meshline{144,144,144}{0.362452278112}{0.813302390196}{0.370197176247}{0.810457798762}
  \meshline{144,144,144}{0.301740876190}{0.775854377796}{0.300427852627}{0.776896673099}
  \meshline{144,144,144}{0.278104933749}{0.796245176968}{0.271256366065}{0.803904980764}
  \meshline{144,144,144}{0.323305694698}{0.764150841518}{0.335469540156}{0.759144864950}
  \meshline{144,144,144}{0.278104933749}{0.796245176968}{0.283163559785}{0.790597895334}
  \meshline{144,144,144}{0.260994825727}{0.818918746502}{0.265727185760}{0.812090949548}
  \meshline{144,144,144}{0.337454097704}{0.828058754924}{0.347962223820}{0.820068651917}
  \meshline{144,144,144}{0.265727185760}{0.812090949548}{0.271256366065}{0.803904980764}
  \meshline{144,144,144}{0.315887023817}{0.855430090177}{0.310279106993}{0.872377117778}
  \meshline{144,144,144}{0.257367842070}{0.825917694257}{0.260994825727}{0.818918746502}
  \meshline{144,144,144}{0.121106088829}{0.750726955695}{0.120565544649}{0.751913698876}
  \meshline{144,144,144}{0.110087215564}{0.781364488836}{0.114131286571}{0.767961299420}
  \meshline{144,144,144}{0.178104959624}{0.853113716227}{0.178888956389}{0.849060971123}
  \meshline{144,144,144}{0.038056160655}{0.798452980692}{0.037131874526}{0.811604506860}
  \meshline{144,144,144}{0.035653273802}{0.841570207630}{0.035823838190}{0.834017399447}
  \meshline{144,144,144}{0.035653273802}{0.841570207630}{0.035173287065}{0.852384912317}
  \meshline{144,144,144}{0.103134949161}{0.809608937006}{0.104275223968}{0.803077674321}
  \meshline{144,144,144}{0.176049642655}{0.875901618022}{0.175850237850}{0.884846817323}
  \meshline{144,144,144}{0.097024116990}{0.854022305711}{0.095987178317}{0.874478530492}
  \meshline{144,144,144}{0.034920705836}{0.883627177696}{0.035074535106}{0.899583636058}
  \meshline{144,144,144}{0.034888797301}{0.869587868260}{0.035023317889}{0.864095920318}
  \meshline{144,144,144}{0.035086798226}{0.901149352503}{0.035074535106}{0.899583636058}
  \meshline{144,144,144}{0.034888797301}{0.869587868260}{0.034926917111}{0.882434306686}
  \meshline{144,144,144}{0.035023317889}{0.864095920318}{0.035173287065}{0.852384912317}
  \meshline{144,144,144}{0.034920705836}{0.883627177696}{0.034926917111}{0.882434306686}
  \meshline{144,144,144}{0.503258395673}{0.623185642057}{0.501824009857}{0.622738129504}
  \meshline{144,144,144}{0.521760450594}{0.731981187601}{0.524210342282}{0.733278541202}
  \meshline{144,144,144}{0.491091638639}{0.718216750412}{0.504041988239}{0.723638977971}
  \meshline{144,144,144}{0.471831653959}{0.711605617681}{0.460331661485}{0.707967847470}
  \meshline{144,144,144}{0.511830720173}{0.666177335656}{0.508819892741}{0.665142955982}
  \meshline{144,144,144}{0.630435082416}{0.612316668847}{0.638961731281}{0.613951689484}
  \meshline{144,144,144}{0.524369294473}{0.629636108648}{0.518945127485}{0.628009296454}
  \meshline{144,144,144}{0.518945127485}{0.628009296454}{0.503258395673}{0.623185642057}
  \meshline{144,144,144}{0.524210342282}{0.733278541202}{0.540217378245}{0.742188962842}
  \meshline{144,144,144}{0.479011562778}{0.713885407821}{0.491091638639}{0.718216750412}
  \meshline{144,144,144}{0.514577802882}{0.728609819145}{0.506749959121}{0.724834567871}
  \meshline{144,144,144}{0.587122087130}{0.650377531172}{0.583841473345}{0.649377398889}
  \meshline{144,144,144}{0.605798812830}{0.606934159479}{0.618111390108}{0.609388331890}
  \meshline{144,144,144}{0.557056842251}{0.594634178361}{0.554195066760}{0.593843539828}
  \meshline{144,144,144}{0.524369294473}{0.629636108648}{0.542426015982}{0.635487517449}
  \meshline{144,144,144}{0.511830720173}{0.666177335656}{0.522417142870}{0.670087846302}
  \meshline{144,144,144}{0.514577802882}{0.728609819145}{0.521760450594}{0.731981187601}
  \meshline{144,144,144}{0.587122087130}{0.650377531172}{0.605444449574}{0.657065250495}
  \meshline{144,144,144}{0.549807679973}{0.747986873908}{0.559197531764}{0.754556462113}
  \meshline{144,144,144}{0.578047625610}{0.693369329626}{0.590185144293}{0.698950183208}
  \meshline{144,144,144}{0.535327407037}{0.674811078136}{0.547751495695}{0.679874138902}
  \meshline{144,144,144}{0.581282918419}{0.600951760301}{0.583632471605}{0.601531257880}
  \meshline{144,144,144}{0.501270857873}{0.662687170440}{0.508819892741}{0.665142955982}
  \meshline{144,144,144}{0.559197531764}{0.754556462113}{0.568373504929}{0.761256976026}
  \meshline{144,144,144}{0.522417142870}{0.670087846302}{0.535327407037}{0.674811078136}
  \meshline{144,144,144}{0.550385625465}{0.680921675317}{0.547751495695}{0.679874138902}
  \meshline{144,144,144}{0.565267530136}{0.643014002778}{0.563409416563}{0.642327031181}
  \meshline{144,144,144}{0.596876660100}{0.604649890204}{0.605798812830}{0.606934159479}
  \meshline{144,144,144}{0.557411240128}{0.594740141156}{0.579320093712}{0.600378878021}
  \meshline{144,144,144}{0.565267530136}{0.643014002778}{0.572481103213}{0.645520635919}
  \meshline{144,144,144}{0.544242391632}{0.636029822716}{0.552503960819}{0.638750620556}
  \meshline{144,144,144}{0.568373504929}{0.761256976026}{0.574341154032}{0.766133992380}
  \meshline{144,144,144}{0.520276360346}{0.797428495775}{0.522905397720}{0.799643232737}
  \meshline{144,144,144}{0.563409416563}{0.642327031181}{0.552503960819}{0.638750620556}
  \meshline{144,144,144}{0.550385625465}{0.680921675317}{0.551087697125}{0.681184266832}
  \meshline{144,144,144}{0.581282918419}{0.600951760301}{0.579320093712}{0.600378878021}
  \meshline{144,144,144}{0.549807679973}{0.747986873908}{0.540217378245}{0.742188962842}
  \meshline{144,144,144}{0.532957703773}{0.809614597209}{0.537139606005}{0.813842692576}
  \meshline{144,144,144}{0.574341154032}{0.766133992380}{0.581847428661}{0.772339386307}
  \meshline{144,144,144}{0.478147152404}{0.770117022927}{0.482067052491}{0.772243996526}
  \meshline{144,144,144}{0.470571968465}{0.766990418516}{0.475952804636}{0.769128135122}
  \meshline{144,144,144}{0.657675991314}{0.617599118776}{0.648903318603}{0.615681923985}
  \meshline{144,144,144}{0.596876660100}{0.604649890204}{0.583632471605}{0.601531257880}
  \meshline{144,144,144}{0.630435082416}{0.612316668847}{0.623884400445}{0.610827908894}
  \meshline{144,144,144}{0.618430622845}{0.661580515157}{0.630026259422}{0.666020581225}
  \meshline{144,144,144}{0.506749959121}{0.724834567871}{0.504041988239}{0.723638977971}
  \meshline{144,144,144}{0.495141378482}{0.779408954693}{0.482067052491}{0.772243996526}
  \meshline{144,144,144}{0.458352020795}{0.762038239485}{0.470571968465}{0.766990418516}
  \meshline{144,144,144}{0.475952804636}{0.769128135122}{0.478147152404}{0.770117022927}
  \meshline{144,144,144}{0.424474741446}{0.809706713133}{0.441596356015}{0.815253014113}
  \meshline{144,144,144}{0.370197176247}{0.810457798762}{0.383761894009}{0.807815493652}
  \meshline{144,144,144}{0.443533917388}{0.757358691079}{0.437686874574}{0.756050621269}
  \meshline{144,144,144}{0.507194516454}{0.787227102453}{0.495141378482}{0.779408954693}
  \meshline{144,144,144}{0.478823831759}{0.840680530430}{0.485114630502}{0.847298551249}
  \meshline{144,144,144}{0.417207472003}{0.751982406210}{0.414507844697}{0.751718726661}
  \meshline{144,144,144}{0.358817480484}{0.696001046095}{0.361770081962}{0.695699811286}
  \meshline{144,144,144}{0.313943441369}{0.702666400270}{0.316563865905}{0.702057539698}
  \meshline{144,144,144}{0.191540139246}{0.805356455190}{0.190350859002}{0.807909145390}
  \meshline{144,144,144}{0.214046745612}{0.766577628315}{0.211897360419}{0.769738665864}
  \meshline{144,144,144}{0.356439766559}{0.753647460644}{0.354799205050}{0.753911912776}
  \meshline{144,144,144}{0.335469540156}{0.759144864950}{0.351750064627}{0.754739036789}
  \meshline{144,144,144}{0.098870873231}{0.834930313658}{0.100018417226}{0.826853510612}
  \meshline{144,144,144}{0.100018417226}{0.826853510612}{0.101184178580}{0.818834032467}
  \meshline{144,144,144}{0.107838829460}{0.788038975615}{0.105868384277}{0.796441135707}
  \meshline{144,144,144}{0.098870873231}{0.834930313658}{0.097810481056}{0.846102595215}
  \meshline{144,144,144}{0.103134949161}{0.809608937006}{0.101184178580}{0.818834032467}
  \meshline{144,144,144}{0.105868384277}{0.796441135707}{0.104275223968}{0.803077674321}
  \meshline{144,144,144}{0.480618463399}{0.656128890679}{0.491948300233}{0.659649081251}
  \meshline{144,144,144}{0.443533917388}{0.757358691079}{0.452163453780}{0.760022329189}
  \meshline{144,144,144}{0.403999341284}{0.806587716167}{0.404009239518}{0.806587651400}
  \meshline{144,144,144}{0.437686874574}{0.756050621269}{0.418084642479}{0.752111833109}
  \meshline{144,144,144}{0.211897360419}{0.769738665864}{0.204643220155}{0.779898089832}
  \meshline{144,144,144}{0.215051159135}{0.765330902221}{0.220458453079}{0.759254712057}
  \meshline{144,144,144}{0.194238276882}{0.800359319205}{0.191540139246}{0.805356455190}
  \meshline{144,144,144}{0.236051317337}{0.743344637703}{0.227719606825}{0.750981948389}
  \meshline{144,144,144}{0.194238276882}{0.800359319205}{0.204643220155}{0.779898089832}
  \meshline{144,144,144}{0.458782746912}{0.823400469316}{0.458341445543}{0.823145973827}
  \meshline{144,144,144}{0.508474963066}{0.788120931381}{0.511305847183}{0.790372871275}
  \meshline{144,144,144}{0.415868448297}{0.807973217300}{0.424474741446}{0.809706713133}
  \meshline{144,144,144}{0.404009239518}{0.806587651400}{0.404012882756}{0.806587783524}
  \meshline{144,144,144}{0.441596356015}{0.815253014113}{0.446022662404}{0.816987851323}
  \meshline{144,144,144}{0.354799205050}{0.753911912776}{0.351750064627}{0.754739036789}
  \meshline{144,144,144}{0.399668591784}{0.750497677483}{0.395784370012}{0.750617656788}
  \meshline{144,144,144}{0.415868448297}{0.807973217300}{0.404012882756}{0.806587783524}
  \meshline{144,144,144}{0.402455123040}{0.750565045136}{0.399668591784}{0.750497677483}
  \meshline{144,144,144}{0.395784370012}{0.750617656788}{0.373421067518}{0.751115637605}
  \meshline{144,144,144}{0.383761894009}{0.807815493652}{0.389942311564}{0.806967538202}
  \meshline{144,144,144}{0.249042679581}{0.846467357068}{0.248686321483}{0.847854967221}
  \meshline{144,144,144}{0.347962223820}{0.820068651917}{0.362452278112}{0.813302390196}
  \meshline{144,144,144}{0.315887023817}{0.855430090177}{0.316702398432}{0.852973378506}
  \meshline{144,144,144}{0.244582190198}{0.866206431202}{0.243164705527}{0.878740382899}
  \meshline{144,144,144}{0.244582190198}{0.866206431202}{0.245916139605}{0.858320701181}
  \meshline{144,144,144}{0.389942311564}{0.806967538202}{0.403999341284}{0.806587716167}
  \meshline{144,144,144}{0.250817763834}{0.931694347390}{0.247143690306}{0.918740152059}
  \meshline{144,144,144}{0.243112528696}{0.885414645038}{0.243164705527}{0.878740382899}
  \meshline{144,144,144}{0.329178114360}{0.835510576784}{0.318828800177}{0.849253790453}
  \meshline{144,144,144}{0.243472634504}{0.897732523729}{0.245532886815}{0.911987215061}
  \meshline{144,144,144}{0.246019047395}{0.915043824104}{0.245532886815}{0.911987215061}
  \meshline{144,144,144}{0.249042679581}{0.846467357068}{0.253415962191}{0.833952170010}
  \meshline{144,144,144}{0.245916139605}{0.858320701181}{0.248686321483}{0.847854967221}
  \meshline{144,144,144}{0.181411885649}{0.837284318193}{0.181376381962}{0.837452746191}
  \meshline{144,144,144}{0.182858935050}{0.936590175173}{0.183209301371}{0.938335266885}
  \meshline{144,144,144}{0.176572917836}{0.867675828044}{0.177352191434}{0.860792477781}
  \meshline{144,144,144}{0.184791579590}{0.823564364235}{0.181411885649}{0.837284318193}
  \meshline{144,144,144}{0.190350859002}{0.807909145390}{0.189040842629}{0.811732071710}
  \meshline{144,144,144}{0.329178114360}{0.835510576784}{0.337454097704}{0.828058754924}
  \meshline{144,144,144}{0.243112528696}{0.885414645038}{0.243472634504}{0.897732523729}
  \meshline{144,144,144}{0.311321574302}{0.907399617788}{0.308980113896}{0.897398860954}
  \meshline{144,144,144}{0.319884202112}{0.928980465792}{0.322788456152}{0.933906434472}
  \meshline{144,144,144}{0.182858935050}{0.936590175173}{0.178905578616}{0.918452002592}
  \meshline{144,144,144}{0.097181133730}{0.911229060171}{0.098738958565}{0.927251936773}
  \meshline{144,144,144}{0.317166227902}{0.851847029309}{0.318828800177}{0.849253790453}
  \meshline{144,144,144}{0.313566406740}{0.915300744036}{0.319884202112}{0.928980465792}
  \meshline{144,144,144}{0.308563776335}{0.891577134205}{0.309010804286}{0.883185754379}
  \meshline{144,144,144}{0.308980113896}{0.897398860954}{0.308563776335}{0.891577134205}
  \meshline{144,144,144}{0.316702398432}{0.852973378506}{0.317166227902}{0.851847029309}
  \meshline{144,144,144}{0.309010804286}{0.883185754379}{0.310279106993}{0.872377117778}
  \meshline{144,144,144}{0.184791579590}{0.823564364235}{0.189040842629}{0.811732071710}
  \meshline{144,144,144}{0.353167367727}{1.023477917256}{0.359895361021}{1.025501336192}
  \meshline{144,144,144}{0.520276360346}{0.797428495775}{0.511305847183}{0.790372871275}
  \meshline{144,144,144}{0.491113655796}{0.857508665720}{0.499587594939}{0.875088523283}
  \meshline{144,144,144}{0.446022662404}{0.816987851323}{0.458341445543}{0.823145973827}
  \meshline{144,144,144}{0.459185594331}{0.823679856321}{0.470557404515}{0.832183167551}
  \meshline{144,144,144}{0.458782746912}{0.823400469316}{0.459185594331}{0.823679856321}
  \meshline{144,144,144}{0.176366316279}{0.897055123254}{0.176650314094}{0.900390364724}
  \meshline{144,144,144}{0.246019047395}{0.915043824104}{0.247143690306}{0.918740152059}
  \meshline{144,144,144}{0.598484463550}{0.788713360282}{0.608771546268}{0.800681304571}
  \meshline{144,144,144}{0.637715424445}{0.852146582433}{0.634736422743}{0.843492082139}
  \meshline{144,144,144}{0.499641221436}{0.912754230119}{0.502028140462}{0.903068107371}
  \meshline{144,144,144}{0.178104959624}{0.853113716227}{0.177352191434}{0.860792477781}
  \meshline{144,144,144}{0.175850237850}{0.884846817323}{0.176366316279}{0.897055123254}
  \meshline{144,144,144}{0.178905578616}{0.918452002592}{0.176650314094}{0.900390364724}
  \meshline{144,144,144}{0.178888956389}{0.849060971123}{0.181376381962}{0.837452746191}
  \meshline{144,144,144}{0.176049642655}{0.875901618022}{0.176572917836}{0.867675828044}
  \meshline{144,144,144}{0.096323667599}{0.894361927855}{0.096060145953}{0.879860646430}
  \meshline{144,144,144}{0.097810481056}{0.846102595215}{0.097196674084}{0.851313057345}
  \meshline{144,144,144}{0.096060145953}{0.879860646430}{0.095987178317}{0.874478530492}
  \meshline{144,144,144}{0.097181133730}{0.911229060171}{0.096475894132}{0.903360606681}
  \meshline{144,144,144}{0.183818281554}{0.940039052881}{0.183209301371}{0.938335266885}
  \meshline{144,144,144}{0.258754447300}{0.949947415462}{0.253309335751}{0.938267891074}
  \meshline{144,144,144}{0.105584021157}{0.965373403501}{0.103535514133}{0.955376155412}
  \meshline{144,144,144}{0.097196674084}{0.851313057345}{0.097024116990}{0.854022305711}
  \meshline{144,144,144}{0.149716160964}{1.054544035054}{0.158990348364}{1.064728818617}
  \meshline{144,144,144}{0.267605618384}{0.964409850623}{0.264697558246}{0.959977284247}
  \meshline{144,144,144}{0.258754447300}{0.949947415462}{0.264697558246}{0.959977284247}
  \meshline{144,144,144}{0.189313559776}{0.956560187298}{0.183818281554}{0.940039052881}
  \meshline{144,144,144}{0.311321574302}{0.907399617788}{0.313566406740}{0.915300744036}
  \meshline{144,144,144}{0.250817763834}{0.931694347390}{0.253309335751}{0.938267891074}
  \meshline{144,144,144}{0.337794132221}{0.950838755160}{0.334450937012}{0.947806123006}
  \meshline{144,144,144}{0.282189797352}{0.982099525860}{0.274933949078}{0.973790258229}
  \meshline{144,144,144}{0.274933949078}{0.973790258229}{0.267605618384}{0.964409850623}
  \meshline{144,144,144}{0.298892133258}{0.996962517777}{0.292582032535}{0.991588885856}
  \meshline{144,144,144}{0.326810048428}{0.939147098653}{0.322788456152}{0.933906434472}
  \meshline{144,144,144}{0.326810048428}{0.939147098653}{0.334450937012}{0.947806123006}
  \meshline{144,144,144}{0.355754027895}{0.963387791221}{0.370678948080}{0.969968957664}
  \meshline{144,144,144}{0.337794132221}{0.950838755160}{0.350777185521}{0.960467162630}
  \meshline{144,144,144}{0.522905397720}{0.799643232737}{0.532957703773}{0.809614597209}
  \meshline{144,144,144}{0.541555030543}{0.819377018114}{0.537139606005}{0.813842692576}
  \meshline{144,144,144}{0.550807707465}{0.832557782938}{0.554469931153}{0.838386044079}
  \meshline{144,144,144}{0.098738958565}{0.927251936773}{0.099605451386}{0.932492513427}
  \meshline{144,144,144}{0.101384308421}{0.945338045699}{0.103535514133}{0.955376155412}
  \meshline{144,144,144}{0.096475894132}{0.903360606681}{0.096323667599}{0.894361927855}
  \meshline{144,144,144}{0.201498303577}{0.982418257793}{0.197771072601}{0.974815513911}
  \meshline{144,144,144}{0.209132833301}{0.993916506652}{0.212517424591}{0.998967011977}
  \meshline{144,144,144}{0.201498303577}{0.982418257793}{0.209132833301}{0.993916506652}
  \meshline{144,144,144}{0.253957679209}{1.039327955261}{0.244127249052}{1.031610543391}
  \meshline{144,144,144}{0.212517424591}{0.998967011977}{0.224045513960}{1.012772448023}
  \meshline{144,144,144}{0.564218558066}{0.858825824368}{0.564409475292}{0.859244062563}
  \meshline{144,144,144}{0.554469931153}{0.838386044079}{0.564218558066}{0.858825824368}
  \meshline{144,144,144}{0.541555030543}{0.819377018114}{0.550807707465}{0.832557782938}
  \meshline{144,144,144}{0.192005186403}{0.963253959682}{0.189313559776}{0.956560187298}
  \meshline{144,144,144}{0.197771072601}{0.974815513911}{0.192005186403}{0.963253959682}
  \meshline{144,144,144}{0.099605451386}{0.932492513427}{0.101384308421}{0.945338045699}
  \meshline{144,144,144}{0.107576277417}{0.972177574096}{0.105584021157}{0.965373403501}
  \meshline{144,144,144}{0.112944908692}{0.988876630698}{0.113722664737}{0.991292236081}
  \meshline{144,144,144}{0.037473612966}{0.951492523931}{0.037354932836}{0.950498588954}
  \meshline{144,144,144}{0.113722664737}{0.991292236081}{0.114094823311}{0.992225579210}
  \meshline{144,144,144}{0.108968559001}{0.977659163836}{0.112944908692}{0.988876630698}
  \meshline{144,144,144}{0.046410770269}{1.020745393252}{0.048531942290}{1.030826122455}
  \meshline{144,144,144}{0.037273446643}{0.949254872202}{0.037354932836}{0.950498588954}
  \meshline{144,144,144}{0.039166003554}{0.971189638774}{0.040433300683}{0.980782329007}
  \meshline{144,144,144}{0.037273446643}{0.949254872202}{0.036263214635}{0.933944031575}
  \meshline{144,144,144}{0.035634047991}{0.921668034394}{0.035455314182}{0.914147922893}
  \meshline{144,144,144}{0.035634047991}{0.921668034394}{0.036263214635}{0.933944031575}
  \meshline{144,144,144}{0.035455314182}{0.914147922893}{0.035086798226}{0.901149352503}
  \meshline{144,144,144}{0.205975568609}{1.099058804123}{0.192347085707}{1.091090488505}
  \meshline{144,144,144}{0.058635370845}{1.064039568095}{0.060451845178}{1.068146790517}
  \meshline{144,144,144}{0.041616649675}{0.991880873312}{0.041360222052}{0.989159323840}
  \meshline{144,144,144}{0.119970924966}{1.007157001392}{0.123894105103}{1.014770548546}
  \meshline{144,144,144}{0.130723930553}{1.027436492356}{0.138672768588}{1.040214754060}
  \meshline{144,144,144}{0.046410770269}{1.020745393252}{0.044713090151}{1.011830824513}
  \meshline{144,144,144}{0.041616649675}{0.991880873312}{0.044713090151}{1.011830824513}
  \meshline{144,144,144}{0.050990895364}{1.038348513578}{0.054164500647}{1.051599100258}
  \meshline{144,144,144}{0.048531942290}{1.030826122455}{0.050990895364}{1.038348513578}
  \meshline{144,144,144}{0.119970924966}{1.007157001392}{0.114094823311}{0.992225579210}
  \meshline{144,144,144}{0.126877078245}{1.021174885996}{0.123894105103}{1.014770548546}
  \meshline{144,144,144}{0.037473612966}{0.951492523931}{0.039166003554}{0.971189638774}
  \meshline{144,144,144}{0.108968559001}{0.977659163836}{0.107576277417}{0.972177574096}
  \meshline{144,144,144}{0.146000393748}{1.050135399007}{0.138672768588}{1.040214754060}
  \meshline{144,144,144}{0.174911576113}{1.078780785767}{0.172489656443}{1.076570787678}
  \meshline{144,144,144}{0.174911576113}{1.078780785767}{0.190851997016}{1.090011081944}
  \meshline{144,144,144}{0.190851997016}{1.090011081944}{0.192347085707}{1.091090488505}
  \meshline{144,144,144}{0.172489656443}{1.076570787678}{0.158990348364}{1.064728818617}
  \meshline{144,144,144}{0.205975568609}{1.099058804123}{0.215096367726}{1.103807959966}
  \meshline{144,144,144}{0.223330269505}{1.107301716657}{0.215096367726}{1.103807959966}
  \meshline{144,144,144}{0.237360673263}{1.026191366162}{0.237697719320}{1.026566065736}
  \meshline{144,144,144}{0.254466988082}{1.039702971889}{0.260830977487}{1.043748738416}
  \meshline{144,144,144}{0.237360673263}{1.026191366162}{0.224045513960}{1.012772448023}
  \meshline{144,144,144}{0.237909583429}{1.026760251635}{0.244127249052}{1.031610543391}
  \meshline{144,144,144}{0.273034945051}{1.124220803879}{0.262504047014}{1.121651272979}
  \meshline{144,144,144}{0.323387022740}{1.071919827803}{0.338765775566}{1.076159796162}
  \meshline{144,144,144}{0.237917438672}{1.113554139694}{0.223330269505}{1.107301716657}
  \meshline{144,144,144}{0.254466988082}{1.039702971889}{0.253957679209}{1.039327955261}
  \meshline{144,144,144}{0.260830977487}{1.043748738416}{0.270086191428}{1.049707619090}
  \meshline{144,144,144}{0.282342349578}{1.056388964436}{0.270716195645}{1.050084559153}
  \meshline{144,144,144}{0.300337687300}{1.130409936611}{0.297048238900}{1.129623240656}
  \meshline{144,144,144}{0.221447680720}{1.167111925015}{0.239724177486}{1.169791973016}
  \meshline{144,144,144}{0.253082033995}{1.170913535995}{0.239724177486}{1.169791973016}
  \meshline{144,144,144}{0.317243554561}{1.133237657572}{0.320329100168}{1.133782185635}
  \meshline{144,144,144}{0.316837173084}{1.070265282634}{0.308952606318}{1.067443895248}
  \meshline{144,144,144}{0.041360222052}{0.989159323840}{0.040433300683}{0.980782329007}
  \meshline{144,144,144}{0.126877078245}{1.021174885996}{0.130723930553}{1.027436492356}
  \meshline{144,144,144}{0.155779973238}{1.152009496978}{0.164138007502}{1.155161359701}
  \meshline{144,144,144}{0.164138007502}{1.155161359701}{0.176642469148}{1.158234042113}
  \meshline{144,144,144}{0.149223653975}{1.150263540147}{0.139939474798}{1.146668833818}
  \meshline{144,144,144}{0.359895361021}{1.025501336192}{0.369277226639}{1.027524629286}
  \meshline{144,144,144}{0.146000393748}{1.050135399007}{0.149716160964}{1.054544035054}
  \meshline{144,144,144}{0.081689814782}{1.105013352283}{0.081897850581}{1.105290659545}
  \meshline{144,144,144}{0.058635370845}{1.064039568095}{0.054164500647}{1.051599100258}
  \meshline{144,144,144}{0.060451845178}{1.068146790517}{0.068668506235}{1.086192985476}
  \meshline{144,144,144}{0.108244011214}{1.129833583373}{0.102067319983}{1.124887888398}
  \meshline{144,144,144}{0.082723287992}{1.106117567415}{0.094679091535}{1.119242582426}
  \meshline{144,144,144}{0.094679091535}{1.119242582426}{0.102067319983}{1.124887888398}
  \meshline{144,144,144}{0.081897850581}{1.105290659545}{0.082723287992}{1.106117567415}
  \meshline{144,144,144}{0.081258491570}{1.104328996838}{0.071575568037}{1.090953244051}
  \meshline{144,144,144}{0.068668506235}{1.086192985476}{0.071575568037}{1.090953244051}
  \meshline{144,144,144}{0.112424375709}{1.132056153118}{0.121390349346}{1.138023133505}
  \meshline{144,144,144}{0.112424375709}{1.132056153118}{0.108244011214}{1.129833583373}
  \meshline{144,144,144}{0.131368506609}{1.142589723374}{0.121390349346}{1.138023133505}
  \meshline{144,144,144}{0.139939474798}{1.146668833818}{0.131368506609}{1.142589723374}
  \meshline{144,144,144}{0.155779973238}{1.152009496978}{0.149223653975}{1.150263540147}
  \meshline{144,144,144}{0.196578443336}{1.162686833437}{0.178313208467}{1.158759205999}
  \meshline{144,144,144}{0.176642469148}{1.158234042113}{0.178313208467}{1.158759205999}
  \meshline{144,144,144}{0.219051628244}{1.166816002862}{0.220567031592}{1.167042907305}
  \meshline{144,144,144}{0.219051628244}{1.166816002862}{0.196578443336}{1.162686833437}
  \meshline{144,144,144}{0.221447680720}{1.167111925015}{0.220567031592}{1.167042907305}
  \meshline{144,144,144}{0.273034945051}{1.124220803879}{0.282230011428}{1.126791953916}
  \meshline{144,144,144}{0.263634427209}{1.172214666177}{0.267349818896}{1.172809673770}
  \meshline{144,144,144}{0.297048238900}{1.129623240656}{0.282230011428}{1.126791953916}
  \meshline{144,144,144}{0.248267474683}{1.116810717522}{0.237917438672}{1.113554139694}
  \meshline{144,144,144}{0.253082033995}{1.170913535995}{0.263634427209}{1.172214666177}
  \meshline{144,144,144}{0.262504047014}{1.121651272979}{0.248267474683}{1.116810717522}
  \meshline{144,144,144}{0.282271381503}{1.173863760069}{0.286952805585}{1.174450880708}
  \meshline{144,144,144}{0.270086191428}{1.049707619090}{0.270716195645}{1.050084559153}
  \meshline{144,144,144}{0.081689814782}{1.105013352283}{0.081258491570}{1.104328996838}
  \meshline{144,144,144}{0.368159979161}{1.178391356330}{0.372479705441}{1.178391356330}
  \meshline{144,144,144}{0.282271381503}{1.173863760069}{0.267349818896}{1.172809673770}
  \meshline{144,144,144}{0.286952805585}{1.174450880708}{0.303255799912}{1.175380604343}
  \meshline{144,144,144}{0.303255799912}{1.175380604343}{0.306827390770}{1.175761457742}
  \meshline{144,144,144}{0.298892603825}{1.063755082592}{0.308952606318}{1.067443895248}
  \meshline{144,144,144}{0.338765775566}{1.076159796162}{0.343305289910}{1.077353499484}
  \meshline{144,144,144}{0.582922563825}{0.391794871288}{0.569576362526}{0.388960749232}
  \meshline{144,144,144}{0.445993814808}{0.448801543595}{0.434593725988}{0.441112874161}
  \meshline{144,144,144}{0.463966628061}{0.460357767089}{0.453692487563}{0.454225100865}
  \meshline{144,144,144}{0.466355631460}{0.461757061136}{0.463966628061}{0.460357767089}
  \meshline{144,144,144}{0.505311042442}{0.420851429396}{0.519593335962}{0.428671392366}
  \meshline{144,144,144}{0.925292245748}{0.552297476458}{0.916935365926}{0.564158970956}
  \meshline{144,144,144}{0.913470546516}{0.569935229843}{0.911099793424}{0.572773673992}
  \meshline{144,144,144}{0.931480620769}{0.538642761555}{0.934205184182}{0.533488853766}
  \meshline{144,144,144}{0.939374425830}{0.518452384721}{0.941514903858}{0.513510268031}
  \meshline{144,144,144}{0.458275960011}{0.610185625834}{0.465746518146}{0.612154083820}
  \meshline{144,144,144}{0.233075508624}{0.572213006192}{0.229221590890}{0.572646748861}
  \meshline{144,144,144}{0.240757380771}{0.739000449919}{0.242230536320}{0.737998212201}
  \meshline{144,144,144}{0.200973037972}{0.659899665408}{0.200647014947}{0.660117651970}
  \meshline{144,144,144}{0.130877498364}{0.731161478857}{0.128061106688}{0.735794668793}
  \meshline{144,144,144}{0.214046745612}{0.766577628315}{0.215051159135}{0.765330902221}
  \meshline{144,144,144}{0.605444449574}{0.657065250495}{0.609354900051}{0.658294455764}
  \meshline{144,144,144}{0.618111390108}{0.609388331890}{0.623884400445}{0.610827908894}
  \meshline{144,144,144}{0.609354900051}{0.658294455764}{0.618430622845}{0.661580515157}
  \meshline{144,144,144}{0.648903318603}{0.615681923985}{0.638961731281}{0.613951689484}
  \meshline{144,144,144}{0.578047625610}{0.693369329626}{0.570443018024}{0.689543560250}
  \meshline{144,144,144}{0.668646427245}{0.619585755188}{0.675627887024}{0.620582676473}
  \meshline{144,144,144}{0.630026259422}{0.666020581225}{0.636220086714}{0.668551140329}
  \meshline{144,144,144}{0.691570254932}{0.568668193539}{0.690149910211}{0.568632129663}
  \meshline{144,144,144}{0.606738791745}{0.707700789053}{0.590185144293}{0.698950183208}
  \meshline{144,144,144}{0.680456466667}{0.685786685646}{0.693299434185}{0.691311339979}
  \meshline{144,144,144}{0.627115782878}{0.719380596828}{0.625525367358}{0.718348108369}
  \meshline{144,144,144}{0.610777161772}{0.709936286574}{0.606738791745}{0.707700789053}
  \meshline{144,144,144}{0.609315567292}{0.801433300135}{0.608771546268}{0.800681304571}
  \meshline{144,144,144}{0.598484463550}{0.788713360282}{0.596062292114}{0.785972209889}
  \meshline{144,144,144}{0.586451721763}{0.776514154018}{0.581847428661}{0.772339386307}
  \meshline{144,144,144}{0.680627003630}{0.757989134919}{0.675528829907}{0.754109778091}
  \meshline{144,144,144}{0.739520808160}{0.831695849142}{0.729350116548}{0.814259525814}
  \meshline{144,144,144}{0.586451721763}{0.776514154018}{0.596062292114}{0.785972209889}
  \meshline{144,144,144}{0.630975722982}{0.722038870029}{0.645571229948}{0.731237472149}
  \meshline{144,144,144}{0.611103397329}{0.804208785183}{0.609315567292}{0.801433300135}
  \meshline{144,144,144}{0.611103397329}{0.804208785183}{0.623732129705}{0.822313733998}
  \meshline{144,144,144}{0.625525367358}{0.718348108369}{0.610777161772}{0.709936286574}
  \meshline{144,144,144}{0.627115782878}{0.719380596828}{0.630975722982}{0.722038870029}
  \meshline{144,144,144}{0.723267181298}{0.704866053494}{0.726445763945}{0.706595513709}
  \meshline{144,144,144}{0.753744689655}{0.720472560105}{0.755998424613}{0.721429823274}
  \meshline{144,144,144}{0.699720692894}{0.694296525677}{0.696860328962}{0.692843958467}
  \meshline{144,144,144}{0.798403986473}{0.626599611899}{0.813061056894}{0.624515297196}
  \meshline{144,144,144}{0.722992633738}{0.626503443167}{0.721976890531}{0.626490477312}
  \meshline{144,144,144}{0.822150767219}{0.623338360313}{0.843313382580}{0.617670159037}
  \meshline{144,144,144}{0.872544875543}{0.605016907705}{0.881983047567}{0.599601514839}
  \meshline{144,144,144}{0.646039496221}{0.671917312461}{0.656755988402}{0.676451331129}
  \meshline{144,144,144}{0.758039147460}{0.628320830847}{0.764502102071}{0.628717858877}
  \meshline{144,144,144}{0.661831166562}{0.742654875776}{0.654838021615}{0.738014305885}
  \meshline{144,144,144}{0.798403986473}{0.626599611899}{0.787690301854}{0.627931195846}
  \meshline{144,144,144}{0.764502102071}{0.628717858877}{0.774850297543}{0.628096417864}
  \meshline{144,144,144}{0.787690301854}{0.627931195846}{0.774850297543}{0.628096417864}
  \meshline{144,144,144}{0.717504518155}{0.702064944517}{0.723267181298}{0.704866053494}
  \meshline{144,144,144}{0.699720692894}{0.694296525677}{0.717504518155}{0.702064944517}
  \meshline{144,144,144}{0.749748530879}{0.628333306372}{0.758039147460}{0.628320830847}
  \meshline{144,144,144}{0.743032788039}{0.627882590065}{0.726530981359}{0.626662503486}
  \meshline{144,144,144}{0.706136900980}{0.624747109835}{0.721976890531}{0.626490477312}
  \meshline{144,144,144}{0.749748530879}{0.628333306372}{0.743032788039}{0.627882590065}
  \meshline{144,144,144}{0.706136900980}{0.624747109835}{0.700614372613}{0.624149227605}
  \meshline{144,144,144}{0.695475375109}{0.568326527308}{0.691570254932}{0.568668193539}
  \meshline{144,144,144}{0.722992633738}{0.626503443167}{0.726530981359}{0.626662503486}
  \meshline{144,144,144}{0.700254313600}{0.624073489886}{0.698273958602}{0.623767990532}
  \meshline{144,144,144}{0.693299434185}{0.691311339979}{0.696860328962}{0.692843958467}
  \meshline{144,144,144}{0.656755988402}{0.676451331129}{0.662655468874}{0.678422452514}
  \meshline{144,144,144}{0.689164603303}{0.765925027637}{0.700298122152}{0.776911749281}
  \meshline{144,144,144}{0.813061056894}{0.624515297196}{0.818827812683}{0.623992053307}
  \meshline{144,144,144}{0.822150767219}{0.623338360313}{0.818827812683}{0.623992053307}
  \meshline{144,144,144}{0.857494130482}{0.805542589539}{0.861445553139}{0.811344760409}
  \meshline{144,144,144}{0.853519360448}{0.614092429469}{0.864407660483}{0.609658737397}
  \meshline{144,144,144}{0.746013104526}{0.716357245255}{0.753744689655}{0.720472560105}
  \meshline{144,144,144}{0.755998424613}{0.721429823274}{0.773220152481}{0.731154312485}
  \meshline{144,144,144}{0.778547846650}{0.734520416812}{0.797033560882}{0.746493905170}
  \meshline{144,144,144}{0.775207052507}{0.732274048487}{0.775600359246}{0.732566736250}
  \meshline{144,144,144}{0.775207052507}{0.732274048487}{0.773220152481}{0.731154312485}
  \meshline{144,144,144}{0.778547846650}{0.734520416812}{0.775600359246}{0.732566736250}
  \meshline{144,144,144}{0.797033560882}{0.746493905170}{0.799359698767}{0.747739513672}
  \meshline{144,144,144}{0.654838021615}{0.738014305885}{0.645571229948}{0.731237472149}
  \meshline{144,144,144}{0.675528829907}{0.754109778091}{0.661831166562}{0.742654875776}
  \meshline{144,144,144}{0.701409629608}{0.778074452659}{0.702435361203}{0.779363887764}
  \meshline{144,144,144}{0.689164603303}{0.765925027637}{0.680627003630}{0.757989134919}
  \meshline{144,144,144}{0.715514890417}{0.794003701180}{0.702435361203}{0.779363887764}
  \meshline{144,144,144}{0.848769059504}{0.616305517223}{0.843313382580}{0.617670159037}
  \meshline{144,144,144}{0.726445763945}{0.706595513709}{0.738344493436}{0.712098241299}
  \meshline{144,144,144}{0.818168937526}{0.762766474798}{0.813586611706}{0.758395383665}
  \meshline{144,144,144}{0.805599482917}{0.752338638287}{0.799359698767}{0.747739513672}
  \meshline{144,144,144}{0.845384069061}{0.789316384675}{0.849444214981}{0.793749313318}
  \meshline{144,144,144}{0.848769059504}{0.616305517223}{0.853519360448}{0.614092429469}
  \meshline{144,144,144}{0.890946750024}{0.592867588415}{0.897357839731}{0.587606157701}
  \meshline{144,144,144}{0.746013104526}{0.716357245255}{0.738344493436}{0.712098241299}
  \meshline{144,144,144}{0.813586611706}{0.758395383665}{0.805599482917}{0.752338638287}
  \meshline{144,144,144}{0.728966865161}{0.813637393392}{0.729350116548}{0.814259525814}
  \meshline{144,144,144}{0.906003083040}{0.577707478406}{0.897357839731}{0.587606157701}
  \meshline{144,144,144}{0.916935365926}{0.564158970956}{0.913470546516}{0.569935229843}
  \meshline{144,144,144}{0.911099793424}{0.572773673992}{0.906003083040}{0.577707478406}
  \meshline{144,144,144}{0.872544875543}{0.605016907705}{0.864407660483}{0.609658737397}
  \meshline{144,144,144}{0.890946750024}{0.592867588415}{0.881983047567}{0.599601514839}
  \meshline{144,144,144}{0.728411788321}{0.812888567430}{0.728966865161}{0.813637393392}
  \meshline{144,144,144}{0.563080546913}{0.942286131064}{0.565309907660}{0.935980029596}
  \meshline{144,144,144}{0.939374425830}{0.518452384721}{0.934205184182}{0.533488853766}
  \meshline{144,144,144}{0.941514903858}{0.513510268031}{0.942613014185}{0.510037252052}
  \meshline{144,144,144}{0.953655294006}{0.466638029204}{0.951582348225}{0.476663451821}
  \meshline{144,144,144}{0.945099016444}{0.501033181865}{0.948307079063}{0.490861487948}
  \meshline{144,144,144}{0.887194123062}{0.427544770401}{0.881992708664}{0.442536488661}
  \meshline{144,144,144}{0.881992708664}{0.442536488661}{0.880670653383}{0.445942449807}
  \meshline{144,144,144}{0.888570478899}{0.423850591625}{0.888788532469}{0.423198849826}
  \meshline{144,144,144}{0.888570478899}{0.423850591625}{0.887194123062}{0.427544770401}
  \meshline{144,144,144}{0.892488135860}{0.409579951079}{0.894336212415}{0.402908864340}
  \meshline{144,144,144}{0.899711187249}{0.375783263322}{0.899676064767}{0.375974091086}
  \meshline{144,144,144}{0.955251508174}{0.454813586817}{0.953655294006}{0.466638029204}
  \meshline{144,144,144}{0.965152720835}{0.322617040799}{0.965156799925}{0.322955055608}
  \meshline{144,144,144}{0.960747009792}{0.412077527548}{0.962328231922}{0.396263461529}
  \meshline{144,144,144}{0.903994058558}{0.319051310788}{0.903966973794}{0.308999728611}
  \meshline{144,144,144}{0.955251508174}{0.454813586817}{0.957090605410}{0.445385004548}
  \meshline{144,144,144}{0.945099016444}{0.501033181865}{0.942613014185}{0.510037252052}
  \meshline{144,144,144}{0.951582348225}{0.476663451821}{0.949233944853}{0.485573196704}
  \meshline{144,144,144}{0.899676064767}{0.375974091086}{0.897591286700}{0.388989572704}
  \meshline{144,144,144}{0.965156799925}{0.322955055608}{0.965149859209}{0.323389758582}
  \meshline{144,144,144}{0.899711187249}{0.375783263322}{0.899767093900}{0.375295081627}
  \meshline{144,144,144}{0.902400418919}{0.355108401282}{0.899767093900}{0.375295081627}
  \meshline{144,144,144}{0.903109979201}{0.343593740373}{0.902400418919}{0.355108401282}
  \meshline{144,144,144}{0.897591286700}{0.388989572704}{0.894501305886}{0.402055248399}
  \meshline{144,144,144}{0.903791226907}{0.334379097397}{0.903109979201}{0.343593740373}
  \meshline{144,144,144}{0.965152720835}{0.322617040799}{0.965134617771}{0.307801844920}
  \meshline{144,144,144}{0.958717981337}{0.431172560084}{0.957090605410}{0.445385004548}
  \meshline{144,144,144}{0.960372355731}{0.417140677785}{0.960193864636}{0.419961968637}
  \meshline{144,144,144}{0.958717981337}{0.431172560084}{0.960193864636}{0.419961968637}
  \meshline{144,144,144}{0.964041365236}{0.367303080983}{0.964453607521}{0.360098355775}
  \meshline{144,144,144}{0.960747009792}{0.412077527548}{0.960372355731}{0.417140677785}
  \meshline{144,144,144}{0.962328231922}{0.396263461529}{0.963229201602}{0.384730989918}
  \meshline{144,144,144}{0.964712237568}{0.349044575313}{0.964453607521}{0.360098355775}
  \meshline{144,144,144}{0.964041365236}{0.367303080983}{0.963229201602}{0.384730989918}
  \meshline{144,144,144}{0.965063494085}{0.335101200366}{0.964840433617}{0.344813241016}
  \meshline{144,144,144}{0.316837173084}{1.070265282634}{0.323387022740}{1.071919827803}
  \meshline{144,144,144}{0.500041797742}{0.877948799145}{0.499587594939}{0.875088523283}
  \meshline{144,144,144}{0.479152407439}{0.948407077126}{0.487034083521}{0.939600879915}
  \meshline{144,144,144}{0.500041797742}{0.877948799145}{0.502353490557}{0.895841727705}
  \meshline{144,144,144}{0.502353490557}{0.895841727705}{0.502028140462}{0.903068107371}
  \meshline{144,144,144}{0.646291213776}{0.924135205173}{0.645954315210}{0.927982460070}
  \meshline{144,144,144}{0.564409475292}{0.859244062563}{0.564565070804}{0.859778833087}
  \meshline{144,144,144}{0.571492752302}{0.901435370943}{0.570975222660}{0.890002207062}
  \meshline{144,144,144}{0.564565070804}{0.859778833087}{0.569870840578}{0.880694936256}
  \meshline{144,144,144}{0.570894225660}{0.908381580315}{0.569766029563}{0.916754578570}
  \meshline{144,144,144}{0.237697719320}{1.026566065736}{0.237909583429}{1.026760251635}
  \meshline{144,144,144}{0.282342349578}{1.056388964436}{0.296135810229}{1.062363573587}
  \meshline{144,144,144}{0.306541445658}{1.001801538089}{0.316442921251}{1.008254517722}
  \meshline{144,144,144}{0.306541445658}{1.001801538089}{0.298892133258}{0.996962517777}
  \meshline{144,144,144}{0.296135810229}{1.062363573587}{0.298892603825}{1.063755082592}
  \meshline{144,144,144}{0.355754027895}{0.963387791221}{0.353240326663}{0.962068482999}
  \meshline{144,144,144}{0.316442921251}{1.008254517722}{0.326506315388}{1.013281830568}
  \meshline{144,144,144}{0.331671860918}{1.015553751143}{0.343797956841}{1.020586250562}
  \meshline{144,144,144}{0.353240326663}{0.962068482999}{0.350777185521}{0.960467162630}
  \meshline{144,144,144}{0.377390981151}{1.029160555488}{0.369277226639}{1.027524629286}
  \meshline{144,144,144}{0.402207558168}{1.140056532866}{0.392323301164}{1.139926240876}
  \meshline{144,144,144}{0.343797956841}{1.020586250562}{0.353167367727}{1.023477917256}
  \meshline{144,144,144}{0.328902544107}{1.014448605504}{0.326506315388}{1.013281830568}
  \meshline{144,144,144}{0.370678948080}{0.969968957664}{0.373445242840}{0.970967368136}
  \meshline{144,144,144}{0.373445242840}{0.970967368136}{0.384836864131}{0.973578282629}
  \meshline{144,144,144}{0.328902544107}{1.014448605504}{0.331671860918}{1.015553751143}
  \meshline{144,144,144}{0.359137849842}{1.080181146010}{0.349468023895}{1.078495155466}
  \meshline{144,144,144}{0.343305289910}{1.077353499484}{0.349468023895}{1.078495155466}
  \meshline{144,144,144}{0.376794386087}{1.082435075648}{0.374969489732}{1.082209844517}
  \meshline{144,144,144}{0.420505795204}{1.031342749351}{0.421770037124}{1.031229011805}
  \meshline{144,144,144}{0.390611808084}{1.083579336683}{0.401008457420}{1.083928711170}
  \meshline{144,144,144}{0.382219810962}{1.029702334458}{0.377390981151}{1.029160555488}
  \meshline{144,144,144}{0.390611808084}{1.083579336683}{0.376794386087}{1.082435075648}
  \meshline{144,144,144}{0.360500602314}{1.138277216355}{0.353428267343}{1.137548911594}
  \meshline{144,144,144}{0.402207558168}{1.140056532866}{0.410354182674}{1.140203841545}
  \meshline{144,144,144}{0.340645267024}{1.136528948410}{0.325092941729}{1.134374621503}
  \meshline{144,144,144}{0.340645267024}{1.136528948410}{0.353428267343}{1.137548911594}
  \meshline{144,144,144}{0.374969489732}{1.082209844517}{0.359137849842}{1.080181146010}
  \meshline{144,144,144}{0.382219810962}{1.029702334458}{0.403237147252}{1.031629921386}
  \meshline{144,144,144}{0.404151957370}{1.031669981570}{0.403829505110}{1.031674882868}
  \meshline{144,144,144}{0.427459794905}{1.083739833977}{0.429548871709}{1.083668623826}
  \meshline{144,144,144}{0.381878643538}{1.139375656262}{0.370229308017}{1.138910111230}
  \meshline{144,144,144}{0.403829505110}{1.031674882868}{0.403237147252}{1.031629921386}
  \meshline{144,144,144}{0.429548871709}{1.083668623826}{0.431831697209}{1.083454517728}
  \meshline{144,144,144}{0.380278765341}{1.178498565556}{0.385228739107}{1.178634231151}
  \meshline{144,144,144}{0.381878643538}{1.139375656262}{0.392323301164}{1.139926240876}
  \meshline{144,144,144}{0.412025142573}{1.084218462364}{0.401008457420}{1.083928711170}
  \meshline{144,144,144}{0.317243554561}{1.133237657572}{0.300337687300}{1.130409936611}
  \meshline{144,144,144}{0.325092941729}{1.134374621503}{0.320329100168}{1.133782185635}
  \meshline{144,144,144}{0.126944785853}{0.177618002850}{0.132652383534}{0.165232258671}
  \meshline{144,144,144}{0.125355480390}{0.181619575888}{0.126944785853}{0.177618002850}
  \meshline{144,144,144}{0.141921171357}{0.148086908181}{0.136906514143}{0.157417106347}
  \meshline{144,144,144}{0.150704574081}{0.135378359428}{0.147515907782}{0.140320532607}
  \meshline{144,144,144}{0.118479306126}{0.202904473150}{0.118630082717}{0.202356444122}
  \meshline{144,144,144}{0.109451201025}{0.273781769221}{0.109383506151}{0.275254656519}
  \meshline{144,144,144}{0.110424936513}{0.247836728215}{0.109862583675}{0.255662498718}
  \meshline{144,144,144}{0.118630082717}{0.202356444122}{0.119215292919}{0.200669902750}
  \meshline{144,144,144}{0.118271061424}{0.203980018648}{0.118479306126}{0.202904473150}
  \meshline{144,144,144}{0.113540607550}{0.224641116168}{0.112212184264}{0.232850331240}
  \meshline{144,144,144}{0.109451201025}{0.273781769221}{0.109862583675}{0.255662498718}
  \meshline{144,144,144}{0.700614372613}{0.624149227605}{0.700254313600}{0.624073489886}
  \meshline{144,144,144}{0.662655468874}{0.678422452514}{0.677041847331}{0.684724548333}
  \meshline{144,144,144}{0.636220086714}{0.668551140329}{0.646039496221}{0.671917312461}
  \meshline{144,144,144}{0.698273958602}{0.623767990532}{0.675627887024}{0.620582676473}
  \meshline{144,144,144}{0.668646427245}{0.619585755188}{0.657675991314}{0.617599118776}
  \meshline{144,144,144}{0.677041847331}{0.684724548333}{0.680456466667}{0.685786685646}
  \meshline{144,144,144}{0.701409629608}{0.778074452659}{0.700298122152}{0.776911749281}
  \meshline{144,144,144}{0.728411788321}{0.812888567430}{0.715514890417}{0.794003701180}
  \meshline{144,144,144}{0.634736422743}{0.843492082139}{0.633214097538}{0.840388092847}
  \meshline{144,144,144}{0.630625685890}{0.835842074059}{0.623732129705}{0.822313733998}
  \meshline{144,144,144}{0.739520808160}{0.831695849142}{0.744009409540}{0.841909129789}
  \meshline{144,144,144}{0.644895311081}{0.876544751744}{0.646188654964}{0.883916428808}
  \meshline{144,144,144}{0.647382603455}{0.894335324408}{0.646188654964}{0.883916428808}
  \meshline{144,144,144}{0.641135424691}{0.863084438202}{0.644895311081}{0.876544751744}
  \meshline{144,144,144}{0.640221545030}{0.859157936741}{0.637715424445}{0.852146582433}
  \meshline{144,144,144}{0.744009409540}{0.841909129789}{0.745187919412}{0.844749752519}
  \meshline{144,144,144}{0.474568541974}{1.020717316715}{0.471886185383}{1.021735865156}
  \meshline{144,144,144}{0.568110528498}{0.927071765241}{0.565309907660}{0.935980029596}
  \meshline{144,144,144}{0.568110528498}{0.927071765241}{0.569766029563}{0.916754578570}
  \meshline{144,144,144}{0.646291213776}{0.924135205173}{0.647696864300}{0.912312590782}
  \meshline{144,144,144}{0.642824288270}{0.942450758582}{0.642202763176}{0.945178406549}
  \meshline{144,144,144}{0.754315455391}{0.871421040800}{0.751247978996}{0.861497993179}
  \meshline{144,144,144}{0.750060052790}{0.857473580203}{0.751247978996}{0.861497993179}
  \meshline{144,144,144}{0.757565992402}{0.889935851967}{0.754315455391}{0.871421040800}
  \meshline{144,144,144}{0.759405673243}{0.923716438300}{0.759420864201}{0.924431515924}
  \meshline{144,144,144}{0.757737284640}{0.890686778786}{0.757798167086}{0.891326447147}
  \meshline{144,144,144}{0.759576099410}{0.908917308013}{0.757798167086}{0.891326447147}
  \meshline{144,144,144}{0.750060052790}{0.857473580203}{0.745187919412}{0.844749752519}
  \meshline{144,144,144}{0.757737284640}{0.890686778786}{0.757565992402}{0.889935851967}
  \meshline{144,144,144}{0.570975222660}{0.890002207062}{0.569870840578}{0.880694936256}
  \meshline{144,144,144}{0.571492752302}{0.901435370943}{0.570894225660}{0.908381580315}
  \meshline{144,144,144}{0.630625685890}{0.835842074059}{0.633214097538}{0.840388092847}
  \meshline{144,144,144}{0.641135424691}{0.863084438202}{0.640221545030}{0.859157936741}
  \meshline{144,144,144}{0.755929111924}{0.953447074664}{0.756678969973}{0.947863891778}
  \meshline{144,144,144}{0.735059489454}{1.007505175589}{0.743837002754}{0.989968655767}
  \meshline{144,144,144}{0.877374685332}{0.845133106940}{0.875997377704}{0.841642123141}
  \meshline{144,144,144}{0.647696864300}{0.912312590782}{0.647506754993}{0.904109811458}
  \meshline{144,144,144}{0.747544601494}{0.981331143725}{0.751772703110}{0.969210869465}
  \meshline{144,144,144}{0.721195034184}{1.028490496861}{0.733003560346}{1.010936260707}
  \meshline{144,144,144}{0.733964263181}{1.009587763213}{0.733003560346}{1.010936260707}
  \meshline{144,144,144}{0.818168937526}{0.762766474798}{0.826478946919}{0.769371090957}
  \meshline{144,144,144}{0.857494130482}{0.805542589539}{0.849444214981}{0.793749313318}
  \meshline{144,144,144}{0.826478946919}{0.769371090957}{0.834978228381}{0.777505129480}
  \meshline{144,144,144}{0.887588605256}{0.886973962022}{0.885968001935}{0.876014985247}
  \meshline{144,144,144}{0.885968001935}{0.876014985247}{0.882742314864}{0.863478014908}
  \meshline{144,144,144}{0.875997377704}{0.841642123141}{0.870634564376}{0.828667112931}
  \meshline{144,144,144}{0.881492956715}{0.857975885899}{0.878908794065}{0.850413078441}
  \meshline{144,144,144}{0.867946815781}{0.823588789561}{0.870634564376}{0.828667112931}
  \meshline{144,144,144}{0.882742314864}{0.863478014908}{0.881492956715}{0.857975885899}
  \meshline{144,144,144}{0.887588605256}{0.886973962022}{0.888044428375}{0.890094630758}
  \meshline{144,144,144}{0.735059489454}{1.007505175589}{0.733964263181}{1.009587763213}
  \meshline{144,144,144}{0.845384069061}{0.789316384675}{0.834978228381}{0.777505129480}
  \meshline{144,144,144}{0.877374685332}{0.845133106940}{0.878908794065}{0.850413078441}
  \meshline{144,144,144}{0.861445553139}{0.811344760409}{0.867946815781}{0.823588789561}
  \meshline{144,144,144}{0.747544601494}{0.981331143725}{0.743837002754}{0.989968655767}
  \meshline{144,144,144}{0.759367754911}{0.924895433092}{0.759420864201}{0.924431515924}
  \meshline{144,144,144}{0.755929111924}{0.953447074664}{0.754020478621}{0.960405380156}
  \meshline{144,144,144}{0.751772703110}{0.969210869465}{0.754020478621}{0.960405380156}
  \meshline{144,144,144}{0.759367754911}{0.924895433092}{0.756678969973}{0.947863891778}
  \meshline{144,144,144}{0.759576099410}{0.908917308013}{0.759405673243}{0.923716438300}
  \meshline{144,144,144}{0.889749371800}{0.906372943031}{0.889928240356}{0.908614941465}
  \meshline{144,144,144}{0.887829242374}{0.964796354306}{0.886218634533}{0.977121218614}
  \meshline{144,144,144}{0.890626225069}{0.925739486824}{0.890533326532}{0.922335243239}
  \meshline{144,144,144}{0.888044428375}{0.890094630758}{0.889749371800}{0.906372943031}
  \meshline{144,144,144}{0.890340780439}{0.931600278764}{0.889875560993}{0.948427472236}
  \meshline{144,144,144}{0.890340780439}{0.931600278764}{0.890626225069}{0.925739486824}
  \meshline{144,144,144}{0.887829242374}{0.964796354306}{0.889875560993}{0.948427472236}
  \meshline{144,144,144}{0.889928240356}{0.908614941465}{0.890533326532}{0.922335243239}
  \meshline{144,144,144}{0.964840433617}{0.344813241016}{0.964712237568}{0.349044575313}
  \meshline{144,144,144}{0.965149859209}{0.323389758582}{0.965063494085}{0.335101200366}
  \meshline{144,144,144}{0.478823831759}{0.840680530430}{0.470557404515}{0.832183167551}
  \meshline{144,144,144}{0.491113655796}{0.857508665720}{0.485114630502}{0.847298551249}
  \meshline{144,144,144}{0.407798307602}{1.031596653455}{0.404151957370}{1.031669981570}
  \meshline{144,144,144}{0.466549910133}{0.958574629638}{0.453718406333}{0.966276142243}
  \meshline{144,144,144}{0.440446319726}{1.029130284676}{0.452563624773}{1.026896431543}
  \meshline{144,144,144}{0.420505795204}{1.031342749351}{0.407798307602}{1.031596653455}
  \meshline{144,144,144}{0.440446319726}{1.029130284676}{0.421770037124}{1.031229011805}
  \meshline{144,144,144}{0.403090581393}{0.975830873836}{0.412505370837}{0.976213163552}
  \meshline{144,144,144}{0.415716254307}{0.975989826699}{0.412505370837}{0.976213163552}
  \meshline{144,144,144}{0.403090581393}{0.975830873836}{0.393205473113}{0.975254898003}
  \meshline{144,144,144}{0.393205473113}{0.975254898003}{0.384836864131}{0.973578282629}
  \meshline{144,144,144}{0.452970884748}{0.966607391518}{0.436306066433}{0.972466386106}
  \meshline{144,144,144}{0.430896063159}{0.973765060940}{0.415716254307}{0.975989826699}
  \meshline{144,144,144}{0.453424291655}{0.966424473270}{0.453718406333}{0.966276142243}
  \meshline{144,144,144}{0.430896063159}{0.973765060940}{0.436306066433}{0.972466386106}
  \meshline{144,144,144}{0.469756788850}{1.022257985391}{0.471886185383}{1.021735865156}
  \meshline{144,144,144}{0.473118044795}{0.953849564977}{0.479152407439}{0.948407077126}
  \meshline{144,144,144}{0.452563624773}{1.026896431543}{0.469756788850}{1.022257985391}
  \meshline{144,144,144}{0.466549910133}{0.958574629638}{0.473118044795}{0.953849564977}
  \meshline{144,144,144}{0.487034083521}{0.939600879915}{0.491283829719}{0.933405466759}
  \meshline{144,144,144}{0.496258569628}{0.924499118153}{0.491283829719}{0.933405466759}
  \meshline{144,144,144}{0.499641221436}{0.912754230119}{0.496258569628}{0.924499118153}
  \meshline{144,144,144}{0.563080546913}{0.942286131064}{0.556204167535}{0.955690489512}
  \meshline{144,144,144}{0.497892441808}{1.010425798152}{0.507737160774}{1.005295396674}
  \meshline{144,144,144}{0.526192516913}{0.991570851486}{0.522176541796}{0.995223293574}
  \meshline{144,144,144}{0.453424291655}{0.966424473270}{0.452970884748}{0.966607391518}
  \meshline{144,144,144}{0.488625667595}{1.015362964388}{0.497892441808}{1.010425798152}
  \meshline{144,144,144}{0.474568541974}{1.020717316715}{0.488625667595}{1.015362964388}
  \meshline{144,144,144}{0.498352668871}{1.176775104297}{0.495088815410}{1.176952340681}
  \meshline{144,144,144}{0.520702434381}{0.996295472949}{0.522176541796}{0.995223293574}
  \meshline{144,144,144}{0.526192516913}{0.991570851486}{0.535828542265}{0.983022355743}
  \meshline{144,144,144}{0.520702434381}{0.996295472949}{0.507737160774}{1.005295396674}
  \meshline{144,144,144}{0.463487662427}{1.080043734611}{0.478693636674}{1.076981737293}
  \meshline{144,144,144}{0.494920416181}{1.073349228885}{0.507983691611}{1.069157514175}
  \meshline{144,144,144}{0.490601952586}{1.074457232834}{0.494920416181}{1.073349228885}
  \meshline{144,144,144}{0.520760654844}{1.065141622240}{0.516033231306}{1.066851133788}
  \meshline{144,144,144}{0.478693636674}{1.076981737293}{0.490601952586}{1.074457232834}
  \meshline{144,144,144}{0.458298799515}{1.080725749118}{0.463487662427}{1.080043734611}
  \meshline{144,144,144}{0.516033231306}{1.066851133788}{0.507983691611}{1.069157514175}
  \meshline{144,144,144}{0.544127126273}{1.055158258505}{0.537922368467}{1.057938747691}
  \meshline{144,144,144}{0.548185004821}{1.125725248214}{0.549269654813}{1.125540364898}
  \meshline{144,144,144}{0.520760654844}{1.065141622240}{0.537922368467}{1.057938747691}
  \meshline{144,144,144}{0.557222291890}{1.048359652134}{0.547715264087}{1.053164239545}
  \meshline{144,144,144}{0.546158719636}{1.126094431396}{0.525687040959}{1.130322819486}
  \meshline{144,144,144}{0.509290516920}{1.132978494372}{0.496897501645}{1.134822847217}
  \meshline{144,144,144}{0.574009712794}{1.037717729021}{0.582304673497}{1.031188659122}
  \meshline{144,144,144}{0.544127126273}{1.055158258505}{0.547715264087}{1.053164239545}
  \meshline{144,144,144}{0.574009712794}{1.037717729021}{0.564700939858}{1.043296094459}
  \meshline{144,144,144}{0.468958279075}{1.137733951279}{0.469054854165}{1.137725684337}
  \meshline{144,144,144}{0.425995632981}{1.139968926482}{0.426491013210}{1.139966913722}
  \meshline{144,144,144}{0.445297306682}{1.082466260844}{0.458298799515}{1.080725749118}
  \meshline{144,144,144}{0.487600950609}{1.135935545770}{0.496897501645}{1.134822847217}
  \meshline{144,144,144}{0.469054854165}{1.137725684337}{0.469346890024}{1.137693157199}
  \meshline{144,144,144}{0.557222291890}{1.048359652134}{0.564700939858}{1.043296094459}
  \meshline{144,144,144}{0.638388327921}{1.094759764694}{0.656026107032}{1.084836272147}
  \meshline{144,144,144}{0.445297306682}{1.082466260844}{0.431831697209}{1.083454517728}
  \meshline{144,144,144}{0.427459794905}{1.083739833977}{0.412025142573}{1.084218462364}
  \meshline{144,144,144}{0.604482305477}{1.011658822142}{0.594991294453}{1.020775052183}
  \meshline{144,144,144}{0.615410535373}{0.998396943586}{0.613825931442}{1.000159566025}
  \meshline{144,144,144}{0.626879259086}{0.981469983380}{0.627858703431}{0.979747727701}
  \meshline{144,144,144}{0.620189115278}{0.991229124706}{0.615410535373}{0.998396943586}
  \meshline{144,144,144}{0.703619947806}{1.048512872198}{0.708019044323}{1.044111029781}
  \meshline{144,144,144}{0.721195034184}{1.028490496861}{0.717216656685}{1.033368877823}
  \meshline{144,144,144}{0.690923624993}{1.060085730223}{0.694366985628}{1.056685542976}
  \meshline{144,144,144}{0.674355634368}{1.072931310689}{0.672447254441}{1.074179946713}
  \meshline{144,144,144}{0.674355634368}{1.072931310689}{0.674455452959}{1.072845724257}
  \meshline{144,144,144}{0.656746727996}{1.084479653007}{0.656026107032}{1.084836272147}
  \meshline{144,144,144}{0.672447254441}{1.074179946713}{0.657320845931}{1.084142030269}
  \meshline{144,144,144}{0.657320845931}{1.084142030269}{0.656746727996}{1.084479653007}
  \meshline{144,144,144}{0.618130302548}{1.103872318973}{0.632268111380}{1.097561272998}
  \meshline{144,144,144}{0.618130302548}{1.103872318973}{0.614826955487}{1.105075519152}
  \meshline{144,144,144}{0.638388327921}{1.094759764694}{0.632268111380}{1.097561272998}
  \meshline{144,144,144}{0.717216656685}{1.033368877823}{0.708019044323}{1.044111029781}
  \meshline{144,144,144}{0.690923624993}{1.060085730223}{0.674455452959}{1.072845724257}
  \meshline{144,144,144}{0.642824288270}{0.942450758582}{0.645954315210}{0.927982460070}
  \meshline{144,144,144}{0.637532370030}{0.959632986716}{0.641065200562}{0.948443359592}
  \meshline{144,144,144}{0.642202763176}{0.945178406549}{0.641065200562}{0.948443359592}
  \meshline{144,144,144}{0.694366985628}{1.056685542976}{0.703619947806}{1.048512872198}
  \meshline{144,144,144}{0.292582032535}{0.991588885856}{0.282189797352}{0.982099525860}
  \meshline{144,144,144}{0.370229308017}{1.138910111230}{0.360500602314}{1.138277216355}
  \meshline{144,144,144}{0.427179358506}{1.139945026563}{0.440593028477}{1.139632175901}
  \meshline{144,144,144}{0.437737868764}{1.178608973042}{0.444907949358}{1.178449918214}
  \meshline{144,144,144}{0.440593028477}{1.139632175901}{0.447014627188}{1.139213980557}
  \meshline{144,144,144}{0.468958279075}{1.137733951279}{0.447014627188}{1.139213980557}
  \meshline{144,144,144}{0.410067849142}{1.178752074481}{0.420611877681}{1.178770689755}
  \meshline{144,144,144}{0.380278765341}{1.178498565556}{0.372479705441}{1.178391356330}
  \meshline{144,144,144}{0.410067849142}{1.178752074481}{0.401683359124}{1.178760442077}
  \meshline{144,144,144}{0.391893466395}{1.178685773228}{0.385228739107}{1.178634231151}
  \meshline{144,144,144}{0.426491013210}{1.139966913722}{0.427179358506}{1.139945026563}
  \meshline{144,144,144}{0.410354182674}{1.140203841545}{0.425995632981}{1.139968926482}
  \meshline{144,144,144}{0.452931754118}{1.178346362531}{0.444907949358}{1.178449918214}
  \meshline{144,144,144}{0.321431725354}{1.176389276778}{0.306827390770}{1.175761457742}
  \meshline{144,144,144}{0.349677147220}{1.177781583186}{0.331375104312}{1.177103567674}
  \meshline{144,144,144}{0.321431725354}{1.176389276778}{0.331375104312}{1.177103567674}
  \meshline{144,144,144}{0.368159979161}{1.178391356330}{0.350887844507}{1.177835601575}
  \meshline{144,144,144}{0.350887844507}{1.177835601575}{0.350254999978}{1.177816701111}
  \meshline{144,144,144}{0.349677147220}{1.177781583186}{0.350254999978}{1.177816701111}
  \meshline{144,144,144}{0.434637955528}{1.178669576119}{0.437737868764}{1.178608973042}
  \meshline{144,144,144}{0.434637955528}{1.178669576119}{0.420611877681}{1.178770689755}
  \meshline{144,144,144}{0.401683359124}{1.178760442077}{0.398709707904}{1.178760442077}
  \meshline{144,144,144}{0.469346890024}{1.137693157199}{0.487600950609}{1.135935545770}
  \meshline{144,144,144}{0.455186652915}{1.178346362531}{0.473124954778}{1.177799298806}
  \meshline{144,144,144}{0.509290516920}{1.132978494372}{0.519397404989}{1.131577703757}
  \meshline{144,144,144}{0.548185004821}{1.125725248214}{0.546158719636}{1.126094431396}
  \meshline{144,144,144}{0.513925880309}{1.175961990500}{0.521864352548}{1.175761972842}
  \meshline{144,144,144}{0.580929837847}{1.117173217016}{0.570250917384}{1.120034656960}
  \meshline{144,144,144}{0.565849382814}{1.172411419644}{0.564153884358}{1.172504208271}
  \meshline{144,144,144}{0.525687040959}{1.130322819486}{0.519397404989}{1.131577703757}
  \meshline{144,144,144}{0.498352668871}{1.176775104297}{0.513925880309}{1.175961990500}
  \meshline{144,144,144}{0.475647317369}{1.177799298806}{0.473124954778}{1.177799298806}
  \meshline{144,144,144}{0.494261851007}{1.177020917585}{0.495088815410}{1.176952340681}
  \meshline{144,144,144}{0.494261851007}{1.177020917585}{0.490965461108}{1.177154584861}
  \meshline{144,144,144}{0.490965461108}{1.177154584861}{0.475647317369}{1.177799298806}
  \meshline{144,144,144}{0.398709707904}{1.178760442077}{0.391893466395}{1.178685773228}
  \meshline{144,144,144}{0.455186652915}{1.178346362531}{0.452931754118}{1.178346362531}
  \meshline{144,144,144}{0.556204167535}{0.955690489512}{0.550892368081}{0.965032935979}
  \meshline{144,144,144}{0.550892368081}{0.965032935979}{0.548498587833}{0.967995936074}
  \meshline{144,144,144}{0.627858703431}{0.979747727701}{0.629427187320}{0.976296366955}
  \meshline{144,144,144}{0.613825931442}{1.000159566025}{0.604482305477}{1.011658822142}
  \meshline{144,144,144}{0.591219652032}{1.024199102261}{0.594991294453}{1.020775052183}
  \meshline{144,144,144}{0.537529926917}{0.981376069016}{0.548498587833}{0.967995936074}
  \meshline{144,144,144}{0.537529926917}{0.981376069016}{0.535828542265}{0.983022355743}
  \meshline{144,144,144}{0.582304673497}{1.031188659122}{0.591219652032}{1.024199102261}
  \meshline{144,144,144}{0.626879259086}{0.981469983380}{0.620189115278}{0.991229124706}
  \meshline{144,144,144}{0.637532370030}{0.959632986716}{0.629427187320}{0.976296366955}
  \meshline{144,144,144}{0.549060299594}{1.173712738777}{0.541188841952}{1.174537519368}
  \meshline{144,144,144}{0.587534243605}{1.115318243292}{0.580929837847}{1.117173217016}
  \meshline{144,144,144}{0.614826955487}{1.105075519152}{0.612366479166}{1.105926566417}
  \meshline{144,144,144}{0.585903814860}{1.170646913958}{0.570406569793}{1.172040846118}
  \meshline{144,144,144}{0.565849382814}{1.172411419644}{0.566862356301}{1.172362121361}
  \meshline{144,144,144}{0.552545614080}{1.124721657392}{0.565227092707}{1.121588223112}
  \meshline{144,144,144}{0.549269654813}{1.125540364898}{0.552545614080}{1.124721657392}
  \meshline{144,144,144}{0.612366479166}{1.105926566417}{0.596418765993}{1.112127213553}
  \meshline{144,144,144}{0.570250917384}{1.120034656960}{0.565227092707}{1.121588223112}
  \meshline{144,144,144}{0.587534243605}{1.115318243292}{0.596418765993}{1.112127213553}
  \meshline{144,144,144}{0.585903814860}{1.170646913958}{0.589676438308}{1.170076088846}
  \meshline{144,144,144}{0.531710069895}{1.175000936971}{0.541188841952}{1.174537519368}
  \meshline{144,144,144}{0.531710069895}{1.175000936971}{0.521864352548}{1.175761972842}
  \meshline{144,144,144}{0.549060299594}{1.173712738777}{0.564153884358}{1.172504208271}
  \meshline{144,144,144}{0.594295072045}{1.169225579498}{0.615725703828}{1.166703179785}
  \meshline{144,144,144}{0.594295072045}{1.169225579498}{0.589676438308}{1.170076088846}
  \meshline{144,144,144}{0.617009439442}{1.166563303400}{0.615725703828}{1.166703179785}
  \meshline{144,144,144}{0.570406569793}{1.172040846118}{0.566862356301}{1.172362121361}
  \meshline{144,144,144}{0.617009439442}{1.166563303400}{0.617609930729}{1.166521319853}
  \meshline{144,144,144}{0.877455741931}{1.011132373576}{0.873298875015}{1.021468772377}
  \meshline{144,144,144}{0.882336493969}{0.993172158935}{0.886218634533}{0.977121218614}
  \meshline{144,144,144}{0.877455741931}{1.011132373576}{0.879892993097}{1.002984148971}
  \meshline{144,144,144}{0.882336493969}{0.993172158935}{0.879892993097}{1.002984148971}
  \meshline{144,144,144}{0.873298875015}{1.021468772377}{0.871807534574}{1.024877660558}
  \meshline{144,144,144}{0.849115301326}{1.065085472489}{0.855391508529}{1.055556706415}
  \meshline{144,144,144}{0.865833796553}{1.038346049390}{0.871807534574}{1.024877660558}
  \meshline{144,144,144}{0.858191339339}{1.051724606077}{0.855391508529}{1.055556706415}
  \meshline{144,144,144}{0.704634477507}{1.149527420492}{0.690507807201}{1.153335779291}
  \meshline{144,144,144}{0.635383296447}{1.164002047528}{0.617609930729}{1.166521319853}
  \meshline{144,144,144}{0.661788482237}{1.159703359544}{0.653597634237}{1.160852936600}
  \meshline{144,144,144}{0.683815425152}{1.154461144042}{0.690507807201}{1.153335779291}
  \meshline{144,144,144}{0.713652455245}{1.147325535492}{0.708169711351}{1.148823129082}
  \meshline{144,144,144}{0.713652455245}{1.147325535492}{0.723834862198}{1.144235918391}
  \meshline{144,144,144}{0.740004861938}{1.138856825700}{0.752277763577}{1.133889874446}
  \meshline{144,144,144}{0.723834862198}{1.144235918391}{0.729144328610}{1.142096210862}
  \meshline{144,144,144}{0.672131412504}{1.157398297060}{0.683815425152}{1.154461144042}
  \meshline{144,144,144}{0.635383296447}{1.164002047528}{0.636793209231}{1.163828015898}
  \meshline{144,144,144}{0.661788482237}{1.159703359544}{0.672131412504}{1.157398297060}
  \meshline{144,144,144}{0.636793209231}{1.163828015898}{0.653597634237}{1.160852936600}
  \meshline{144,144,144}{0.708169711351}{1.148823129082}{0.704634477507}{1.149527420492}
  \meshline{144,144,144}{0.740004861938}{1.138856825700}{0.729144328610}{1.142096210862}
  \meshline{144,144,144}{0.752277763577}{1.133889874446}{0.755002682957}{1.133044281862}
  \meshline{144,144,144}{0.755002682957}{1.133044281862}{0.773480169341}{1.124545986918}
  \meshline{144,144,144}{0.778563212175}{1.122551490784}{0.786458738885}{1.118107074215}
  \meshline{144,144,144}{0.778563212175}{1.122551490784}{0.773480169341}{1.124545986918}
  \meshline{144,144,144}{0.808191113410}{1.105008733099}{0.822516445274}{1.092854199893}
  \meshline{144,144,144}{0.786458738885}{1.118107074215}{0.794813118927}{1.113577615380}
  \meshline{144,144,144}{0.798568711053}{1.110780191570}{0.794813118927}{1.113577615380}
  \meshline{144,144,144}{0.823219040580}{1.092264522971}{0.833912883172}{1.083057303542}
  \meshline{144,144,144}{0.833912883172}{1.083057303542}{0.838031043891}{1.078358666484}
  \meshline{144,144,144}{0.845475645263}{1.069750020619}{0.838031043891}{1.078358666484}
  \meshline{144,144,144}{0.822898840680}{1.092581202937}{0.823219040580}{1.092264522971}
  \meshline{144,144,144}{0.845475645263}{1.069750020619}{0.849115301326}{1.065085472489}
  \meshline{144,144,144}{0.860543805645}{1.047451133641}{0.858191339339}{1.051724606077}
  \meshline{144,144,144}{0.865833796553}{1.038346049390}{0.860543805645}{1.047451133641}
  \meshline{144,144,144}{0.808191113410}{1.105008733099}{0.798568711053}{1.110780191570}
  \meshline{144,144,144}{0.822516445274}{1.092854199893}{0.822898840680}{1.092581202937}
  \meshline{144,144,144}{0.775892269716}{0.032254764116}{0.781444572208}{0.033354191910}
  \meshline{144,144,144}{0.789135583047}{0.035044321254}{0.799190419134}{0.036445429855}
  \meshline{144,144,144}{0.762942205583}{0.030677558783}{0.775892269716}{0.032254764116}
  \meshline{144,144,144}{0.748226558261}{0.028864376588}{0.751146128042}{0.029108088047}
\end{pgfscope}


==> nodal_rectsquare_D0.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.2, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshtriangle{168,0,57}{1.000000000000}{0.015625000000}{0.984375000000}{0.000000000000}{1.000000000000}{0.000000000000}
  \meshline{168,0,57}{0.984375000000}{0.000000000000}{1.000000000000}{0.015625000000}
  \meshline{168,0,57}{0.313045550828}{0.546312658753}{0.326000243724}{0.549905091959}
  \meshline{168,0,57}{0.583272926396}{0.624948443868}{0.582672348372}{0.624744552001}
  \meshline{168,0,57}{0.034127014023}{0.497020993637}{0.031615180574}{0.497436407333}
  \meshline{168,0,57}{0.450433234996}{0.585594571934}{0.442351546931}{0.583112490031}
  \meshline{168,0,57}{0.512269398424}{0.603979138363}{0.490937411830}{0.597616843792}
  \meshline{168,0,57}{0.408713914668}{0.573373683475}{0.414996545672}{0.575319476181}
  \meshline{168,0,57}{0.414996545672}{0.575319476181}{0.428802486461}{0.579262985781}
  \meshline{168,0,57}{0.378676957971}{0.564542924101}{0.364725355754}{0.560963865176}
  \meshline{168,0,57}{0.326000243724}{0.549905091959}{0.330469408831}{0.551180529827}
  \meshline{168,0,57}{0.404188488037}{0.571930741731}{0.408713914668}{0.573373683475}
  \meshline{168,0,57}{0.428802486461}{0.579262985781}{0.442351546931}{0.583112490031}
  \meshline{168,0,57}{0.330469408831}{0.551180529827}{0.331954587863}{0.551721800699}
  \meshline{168,0,57}{0.378676957971}{0.564542924101}{0.388393194383}{0.567551682121}
  \meshline{168,0,57}{0.364725355754}{0.560963865176}{0.355123074190}{0.557964382558}
  \meshline{168,0,57}{0.404188488037}{0.571930741731}{0.388393194383}{0.567551682121}
  \meshline{168,0,57}{0.334004806786}{0.552386440928}{0.355123074190}{0.557964382558}
  \meshline{168,0,57}{0.313045550828}{0.546312658753}{0.307221566612}{0.545116796371}
  \meshline{168,0,57}{0.331954587863}{0.551721800699}{0.334004806786}{0.552386440928}
  \meshline{168,0,57}{0.017102335893}{0.497246601208}{0.026830577522}{0.499481204125}
  \meshline{168,0,57}{0.291074180050}{0.540765317445}{0.273465681878}{0.536035719849}
  \meshline{168,0,57}{0.034127014023}{0.497020993637}{0.050663738254}{0.497710964487}
  \meshline{168,0,57}{0.084715171724}{0.502083566386}{0.069693865578}{0.499159777399}
  \meshline{168,0,57}{0.096950362567}{0.501915474559}{0.092193054936}{0.501984619355}
  \meshline{168,0,57}{0.291074180050}{0.540765317445}{0.291648135471}{0.540945136525}
  \meshline{168,0,57}{0.307221566612}{0.545116796371}{0.292305745049}{0.541150591989}
  \meshline{168,0,57}{0.291648135471}{0.540945136525}{0.292305745049}{0.541150591989}
  \meshline{168,0,57}{0.257685259881}{0.532655126665}{0.273465681878}{0.536035719849}
  \meshline{168,0,57}{0.252592553528}{0.531000935829}{0.257685259881}{0.532655126665}
  \meshline{168,0,57}{0.228054985390}{0.525130029803}{0.238149995975}{0.528006519090}
  \meshline{168,0,57}{0.252592553528}{0.531000935829}{0.238149995975}{0.528006519090}
  \meshline{168,0,57}{0.196519849564}{0.518703515614}{0.210653418682}{0.521337133430}
  \meshline{168,0,57}{0.220070660620}{0.523993795744}{0.228054985390}{0.525130029803}
  \meshline{168,0,57}{0.220070660620}{0.523993795744}{0.210653418682}{0.521337133430}
  \meshline{168,0,57}{0.193702168253}{0.517807624632}{0.196519849564}{0.518703515614}
  \meshline{168,0,57}{0.178325522111}{0.515189576233}{0.173301709911}{0.514386799787}
  \meshline{168,0,57}{0.156481191644}{0.511117337870}{0.151506262995}{0.509880870788}
  \meshline{168,0,57}{0.151506262995}{0.509880870788}{0.140039264576}{0.508727550858}
  \meshline{168,0,57}{0.178325522111}{0.515189576233}{0.193702168253}{0.517807624632}
  \meshline{168,0,57}{0.170962294885}{0.513997229835}{0.173301709911}{0.514386799787}
  \meshline{168,0,57}{0.170962294885}{0.513997229835}{0.156481191644}{0.511117337870}
  \meshline{168,0,57}{0.127581664226}{0.506354838955}{0.140039264576}{0.508727550858}
  \meshline{168,0,57}{0.450433234996}{0.585594571934}{0.459349230932}{0.588310073973}
  \meshline{168,0,57}{0.469385407855}{0.591188843292}{0.480134481985}{0.594366539641}
  \meshline{168,0,57}{0.512269398424}{0.603979138363}{0.513149478769}{0.604242648601}
  \meshline{168,0,57}{0.480134481985}{0.594366539641}{0.490937411830}{0.597616843792}
  \meshline{168,0,57}{0.559416832837}{0.617988627582}{0.538380971905}{0.611699033933}
  \meshline{168,0,57}{0.513149478769}{0.604242648601}{0.513825884378}{0.604437416327}
  \meshline{168,0,57}{0.069693865578}{0.499159777399}{0.060158331749}{0.500176996283}
  \meshline{168,0,57}{0.114962103182}{0.505067718770}{0.096950362567}{0.501915474559}
  \meshline{168,0,57}{0.050663738254}{0.497710964487}{0.060158331749}{0.500176996283}
  \meshline{168,0,57}{0.092193054936}{0.501984619355}{0.084715171724}{0.502083566386}
  \meshline{168,0,57}{0.127581664226}{0.506354838955}{0.114962103182}{0.505067718770}
  \meshline{168,0,57}{0.017102335893}{0.497246601208}{0.000000000000}{0.500000000000}
  \meshline{168,0,57}{0.031615180574}{0.497436407333}{0.026830577522}{0.499481204125}
  \meshline{168,0,57}{0.534926493977}{0.610744646221}{0.513825884378}{0.604437416327}
  \meshline{168,0,57}{0.584646681012}{0.625367248528}{0.583272926396}{0.624948443868}
  \meshline{168,0,57}{0.538380971905}{0.611699033933}{0.534926493977}{0.610744646221}
  \meshline{168,0,57}{0.582672348372}{0.624744552001}{0.573094252403}{0.621951208627}
  \meshline{168,0,57}{0.559416832837}{0.617988627582}{0.560269047679}{0.618207964264}
  \meshline{168,0,57}{0.560269047679}{0.618207964264}{0.573094252403}{0.621951208627}
  \meshline{168,0,57}{0.584646681012}{0.625367248528}{0.602570868095}{0.630568728472}
  \meshtriangle{168,0,57}{0.000000000000}{1.178125000000}{0.015625000000}{1.200000000000}{0.000000000000}{1.200000000000}
  \meshline{168,0,57}{0.015625000000}{1.200000000000}{0.000000000000}{1.178125000000}
  \meshline{168,0,57}{0.469385407855}{0.591188843292}{0.459349230932}{0.588310073973}
  \meshline{168,0,57}{0.745685793823}{0.669385122484}{0.731165184067}{0.665728440381}
  \meshline{168,0,57}{0.635756026330}{0.640090082878}{0.619421366977}{0.635449397608}
  \meshline{168,0,57}{0.611278983933}{0.632903889173}{0.602570868095}{0.630568728472}
  \meshline{168,0,57}{0.637551034479}{0.640544147556}{0.656377538822}{0.646064780826}
  \meshline{168,0,57}{0.635756026330}{0.640090082878}{0.636815563678}{0.640374058154}
  \meshline{168,0,57}{0.611278983933}{0.632903889173}{0.619421366977}{0.635449397608}
  \meshline{168,0,57}{0.818374187410}{0.684923494722}{0.835723114304}{0.689194652120}
  \meshline{168,0,57}{0.745821730747}{0.669411299952}{0.746060671522}{0.669458838113}
  \meshline{168,0,57}{0.746060671522}{0.669458838113}{0.762576138896}{0.673081172885}
  \meshline{168,0,57}{0.745685793823}{0.669385122484}{0.745821730747}{0.669411299952}
  \meshline{168,0,57}{0.715693131913}{0.661741775724}{0.702490600822}{0.658281399319}
  \meshline{168,0,57}{0.695176094928}{0.656794724572}{0.683374161149}{0.653132201433}
  \meshline{168,0,57}{0.716429547546}{0.661877969579}{0.715693131913}{0.661741775724}
  \meshline{168,0,57}{0.716429547546}{0.661877969579}{0.717530377521}{0.662111092785}
  \meshline{168,0,57}{0.731165184067}{0.665728440381}{0.717530377521}{0.662111092785}
  \meshline{168,0,57}{0.818374187410}{0.684923494722}{0.811382915067}{0.684181913681}
  \meshline{168,0,57}{0.768239418080}{0.674759301782}{0.762576138896}{0.673081172885}
  \meshline{168,0,57}{0.800156706209}{0.681888026132}{0.788406874493}{0.678982027230}
  \meshline{168,0,57}{0.835723114304}{0.689194652120}{0.844301747436}{0.690304624566}
  \meshline{168,0,57}{0.800156706209}{0.681888026132}{0.811382915067}{0.684181913681}
  \meshline{168,0,57}{0.788406874493}{0.678982027230}{0.783526473771}{0.677605640678}
  \meshline{168,0,57}{0.868246610272}{0.693932032251}{0.853151431238}{0.690984497129}
  \meshline{168,0,57}{0.783526473771}{0.677605640678}{0.768239418080}{0.674759301782}
  \meshline{168,0,57}{0.853151431238}{0.690984497129}{0.844301747436}{0.690304624566}
  \meshline{168,0,57}{0.868246610272}{0.693932032251}{0.871595335440}{0.694143529495}
  \meshline{168,0,57}{0.891289926198}{0.696155687653}{0.877826302682}{0.694687777785}
  \meshline{168,0,57}{0.900413985645}{0.698549518923}{0.911954767351}{0.698867661478}
  \meshline{168,0,57}{0.900413985645}{0.698549518923}{0.891289926198}{0.696155687653}
  \meshline{168,0,57}{0.877826302682}{0.694687777785}{0.871595335440}{0.694143529495}
  \meshline{168,0,57}{0.923284717601}{0.700953202605}{0.931409801389}{0.701255471139}
  \meshline{168,0,57}{0.923284717601}{0.700953202605}{0.911954767351}{0.698867661478}
  \meshline{168,0,57}{0.938496150954}{0.700865939590}{0.931409801389}{0.701255471139}
  \meshline{168,0,57}{0.976289661993}{0.705361869473}{0.979851530142}{0.703915797495}
  \meshline{168,0,57}{0.946118335997}{0.703177343477}{0.959265548969}{0.702317795930}
  \meshline{168,0,57}{1.000000000000}{0.693750000000}{0.979851530142}{0.703915797495}
  \meshline{168,0,57}{0.667944674606}{0.648909987314}{0.674027724527}{0.650938288333}
  \meshline{168,0,57}{0.667944674606}{0.648909987314}{0.656377538822}{0.646064780826}
  \meshline{168,0,57}{0.636815563678}{0.640374058154}{0.637551034479}{0.640544147556}
  \meshline{168,0,57}{0.695176094928}{0.656794724572}{0.702490600822}{0.658281399319}
  \meshline{168,0,57}{0.683374161149}{0.653132201433}{0.674027724527}{0.650938288333}
  \meshline{168,0,57}{0.959265548969}{0.702317795930}{0.976289661993}{0.705361869473}
  \meshline{168,0,57}{0.946118335997}{0.703177343477}{0.938496150954}{0.700865939590}
\end{pgfscope}


==> nodal_rectsquare_N.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.3, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{144,144,144}{0.963081240055}{0.098009433109}{0.986519964162}{0.102370729575}
  \meshline{144,144,144}{0.952052798593}{0.094041048137}{0.940187120615}{0.088140191931}
  \meshline{144,144,144}{0.885887676669}{0.259648170663}{0.896854241720}{0.263595259815}
  \meshline{144,144,144}{0.863606922709}{0.251396558928}{0.885887676669}{0.259648170663}
  \meshline{144,144,144}{0.849948713565}{0.244873666764}{0.827848549207}{0.233673887009}
  \meshline{144,144,144}{0.946620781328}{0.274806202256}{0.928161795392}{0.271535886383}
  \meshline{144,144,144}{0.903305688755}{0.265262552819}{0.928161795392}{0.271535886383}
  \meshline{144,144,144}{0.903305688755}{0.265262552819}{0.896854241720}{0.263595259815}
  \meshline{144,144,144}{0.590835592984}{0.241860509747}{0.598526777808}{0.249737763788}
  \meshline{144,144,144}{0.983631919491}{0.278578167685}{1.000000000000}{0.279181931528}
  \meshline{144,144,144}{0.946620781328}{0.274806202256}{0.953598650325}{0.275983561925}
  \meshline{144,144,144}{0.692723133342}{0.076965445127}{0.697564887241}{0.088299227540}
  \meshline{144,144,144}{0.969914340144}{0.277736236140}{0.983631919491}{0.278578167685}
  \meshline{144,144,144}{0.969914340144}{0.277736236140}{0.953598650325}{0.275983561925}
  \meshline{144,144,144}{1.000000000000}{0.425729734277}{0.963276877342}{0.424211938225}
  \meshline{144,144,144}{0.961907067594}{0.424152818197}{0.963276877342}{0.424211938225}
  \meshline{144,144,144}{0.961253824305}{0.424067488017}{0.961907067594}{0.424152818197}
  \meshline{144,144,144}{0.958192097316}{0.423638241264}{0.914658968607}{0.418135306585}
  \meshline{144,144,144}{0.961253824305}{0.424067488017}{0.958192097316}{0.423638241264}
  \meshline{144,144,144}{0.853443364910}{0.404865817769}{0.863893365296}{0.407761102318}
  \meshline{144,144,144}{0.878652392854}{0.411086470311}{0.897831319975}{0.415555770923}
  \meshline{144,144,144}{0.914658968607}{0.418135306585}{0.897831319975}{0.415555770923}
  \meshline{144,144,144}{0.836665038578}{0.399457115302}{0.827639782680}{0.396676376218}
  \meshline{144,144,144}{0.794825177158}{0.384405159665}{0.790956409617}{0.382804669497}
  \meshline{144,144,144}{0.878652392854}{0.411086470311}{0.863893365296}{0.407761102318}
  \meshline{144,144,144}{0.786132155751}{0.380527277199}{0.790956409617}{0.382804669497}
  \meshline{144,144,144}{0.807926462010}{0.389180501585}{0.794825177158}{0.384405159665}
  \meshline{144,144,144}{0.725735734893}{0.350241020742}{0.756037481100}{0.366865005660}
  \meshline{144,144,144}{0.725735734893}{0.350241020742}{0.720472450897}{0.347443621807}
  \meshline{144,144,144}{0.756037481100}{0.366865005660}{0.786132155751}{0.380527277199}
  \meshline{144,144,144}{0.827639782680}{0.396676376218}{0.807926462010}{0.389180501585}
  \meshline{144,144,144}{0.853443364910}{0.404865817769}{0.836665038578}{0.399457115302}
  \meshline{144,144,144}{0.766347501581}{0.188679098732}{0.755915409819}{0.177606574643}
  \meshline{144,144,144}{0.827848549207}{0.233673887009}{0.815688047798}{0.226135788829}
  \meshline{144,144,144}{0.795740985772}{0.213012051467}{0.773778250729}{0.194947422583}
  \meshline{144,144,144}{0.849948713565}{0.244873666764}{0.863606922709}{0.251396558928}
  \meshline{144,144,144}{0.815688047798}{0.226135788829}{0.795740985772}{0.213012051467}
  \meshline{144,144,144}{0.890702851953}{0.035210176574}{0.888420187810}{0.030916676896}
  \meshline{144,144,144}{0.883306736034}{0.000000000000}{0.885865735582}{0.017817054856}
  \meshline{144,144,144}{0.924910728973}{0.077236074783}{0.905160968204}{0.060682468766}
  \meshline{144,144,144}{0.986519964162}{0.102370729575}{1.000000000000}{0.103742351001}
  \meshline{144,144,144}{0.738947470933}{0.159210151441}{0.755915409819}{0.177606574643}
  \meshline{144,144,144}{0.732124831629}{0.150140804981}{0.738947470933}{0.159210151441}
  \meshline{144,144,144}{0.773778250729}{0.194947422583}{0.766347501581}{0.188679098732}
  \meshline{144,144,144}{0.693589708867}{0.329809795653}{0.715526393867}{0.344508802953}
  \meshline{144,144,144}{0.715526393867}{0.344508802953}{0.720472450897}{0.347443621807}
  \meshline{144,144,144}{0.676377026973}{0.318479693943}{0.693589708867}{0.329809795653}
  \meshline{144,144,144}{0.952052798593}{0.094041048137}{0.963081240055}{0.098009433109}
  \meshline{144,144,144}{0.590835592984}{0.241860509747}{0.582078885043}{0.231516136083}
  \meshline{144,144,144}{0.676377026973}{0.318479693943}{0.672525274670}{0.315540131827}
  \meshline{144,144,144}{0.712498395543}{0.120225655441}{0.723602357453}{0.138342834102}
  \meshline{144,144,144}{0.712498395543}{0.120225655441}{0.706681595234}{0.109621093627}
  \meshline{144,144,144}{0.697564887241}{0.088299227540}{0.706681595234}{0.109621093627}
  \meshline{144,144,144}{0.673612630408}{0.620674803525}{0.701528916721}{0.632313824950}
  \meshline{144,144,144}{0.648174779693}{0.296784397167}{0.650943516203}{0.298834313062}
  \meshline{144,144,144}{0.557940791538}{0.451851134444}{0.533344774227}{0.436523690939}
  \meshline{144,144,144}{0.288279353366}{0.238589455388}{0.268068236113}{0.218032225176}
  \meshline{144,144,144}{0.645231677015}{0.294315503935}{0.623658952296}{0.275449673859}
  \meshline{144,144,144}{0.664141211229}{0.308952685552}{0.672525274670}{0.315540131827}
  \meshline{144,144,144}{0.664141211229}{0.308952685552}{0.650943516203}{0.298834313062}
  \meshline{144,144,144}{0.598526777808}{0.249737763788}{0.616081179640}{0.268103508008}
  \meshline{144,144,144}{0.623658952296}{0.275449673859}{0.616081179640}{0.268103508008}
  \meshline{144,144,144}{0.500742488353}{0.414850543976}{0.523711011696}{0.430487751729}
  \meshline{144,144,144}{0.723602357453}{0.138342834102}{0.732124831629}{0.150140804981}
  \meshline{144,144,144}{0.692723133342}{0.076965445127}{0.687067410981}{0.056601422883}
  \meshline{144,144,144}{0.924910728973}{0.077236074783}{0.940187120615}{0.088140191931}
  \meshline{144,144,144}{0.904020403763}{0.058883218918}{0.904925654173}{0.060372036861}
  \meshline{144,144,144}{0.648174779693}{0.296784397167}{0.645231677015}{0.294315503935}
  \meshline{144,144,144}{0.701528916721}{0.632313824950}{0.713677479238}{0.637277912301}
  \meshline{144,144,144}{0.484592477601}{0.525149868074}{0.505476580757}{0.536661436476}
  \meshline{144,144,144}{0.523711011696}{0.430487751729}{0.533344774227}{0.436523690939}
  \meshline{144,144,144}{0.557940791538}{0.451851134444}{0.563529374045}{0.455464613580}
  \meshline{144,144,144}{0.742592393277}{0.544287290186}{0.735256181891}{0.541256892880}
  \meshline{144,144,144}{0.563529374045}{0.455464613580}{0.565596842891}{0.456758772888}
  \meshline{144,144,144}{0.565596842891}{0.456758772888}{0.577133151807}{0.463489580382}
  \meshline{144,144,144}{0.600984817845}{0.477323815945}{0.595918986516}{0.474587332848}
  \meshline{144,144,144}{0.577133151807}{0.463489580382}{0.595918986516}{0.474587332848}
  \meshline{144,144,144}{0.650672589689}{0.503845505518}{0.643998940327}{0.500358155845}
  \meshline{144,144,144}{0.650672589689}{0.503845505518}{0.677627419881}{0.516776587419}
  \meshline{144,144,144}{0.643998940327}{0.500358155845}{0.623518459648}{0.489896695548}
  \meshline{144,144,144}{0.564326442158}{0.568075187482}{0.552418994506}{0.561984058632}
  \meshline{144,144,144}{0.600984817845}{0.477323815945}{0.623518459648}{0.489896695548}
  \meshline{144,144,144}{0.564326442158}{0.568075187482}{0.583751035964}{0.578188634761}
  \meshline{144,144,144}{0.589792650047}{0.581319945704}{0.601520991989}{0.586973162499}
  \meshline{144,144,144}{0.520068412436}{0.544660475443}{0.545932365163}{0.558617249123}
  \meshline{144,144,144}{0.583751035964}{0.578188634761}{0.589792650047}{0.581319945704}
  \meshline{144,144,144}{0.635106906413}{0.603304120894}{0.621702135566}{0.596999473990}
  \meshline{144,144,144}{0.601520991989}{0.586973162499}{0.621702135566}{0.596999473990}
  \meshline{144,144,144}{0.708319016850}{0.530623640253}{0.687405545635}{0.521199185208}
  \meshline{144,144,144}{0.708319016850}{0.530623640253}{0.735256181891}{0.541256892880}
  \meshline{144,144,144}{0.677627419881}{0.516776587419}{0.681561324275}{0.518678509651}
  \meshline{144,144,144}{0.747307279575}{0.649588929027}{0.751765190978}{0.651318888455}
  \meshline{144,144,144}{0.476422666244}{0.397534320881}{0.480766290429}{0.400903131903}
  \meshline{144,144,144}{0.681561324275}{0.518678509651}{0.687405545635}{0.521199185208}
  \meshline{144,144,144}{0.635106906413}{0.603304120894}{0.660879755955}{0.615014758677}
  \meshline{144,144,144}{0.673612630408}{0.620674803525}{0.660879755955}{0.615014758677}
  \meshline{144,144,144}{0.477755879985}{0.521132113753}{0.449335924223}{0.504962846366}
  \meshline{144,144,144}{0.476422666244}{0.397534320881}{0.457004842604}{0.383608925327}
  \meshline{144,144,144}{0.500742488353}{0.414850543976}{0.484641620101}{0.403706609552}
  \meshline{144,144,144}{0.480766290429}{0.400903131903}{0.484641620101}{0.403706609552}
  \meshline{144,144,144}{0.457004842604}{0.383608925327}{0.433884867009}{0.365829045587}
  \meshline{144,144,144}{0.401425460938}{0.340084193781}{0.373593081486}{0.317265324459}
  \meshline{144,144,144}{0.433181778399}{0.365330566805}{0.433884867009}{0.365829045587}
  \meshline{144,144,144}{0.404697539758}{0.343035767643}{0.401425460938}{0.340084193781}
  \meshline{144,144,144}{0.404697539758}{0.343035767643}{0.428448925002}{0.361623931194}
  \meshline{144,144,144}{0.260393785179}{0.398035001830}{0.254612638799}{0.395101723331}
  \meshline{144,144,144}{0.428448925002}{0.361623931194}{0.433181778399}{0.365330566805}
  \meshline{144,144,144}{0.352196763247}{0.297676570821}{0.345271601361}{0.292166730018}
  \meshline{144,144,144}{0.749794217278}{0.546889083676}{0.742592393277}{0.544287290186}
  \meshline{144,144,144}{0.754600062469}{0.652279276116}{0.751765190978}{0.651318888455}
  \meshline{144,144,144}{0.787534756475}{0.663399045183}{0.802354655357}{0.667662283703}
  \meshline{144,144,144}{0.297699272885}{0.247328985510}{0.306200989976}{0.254880070585}
  \meshline{144,144,144}{0.352196763247}{0.297676570821}{0.373593081486}{0.317265324459}
  \meshline{144,144,144}{0.788112754826}{0.559955377868}{0.804504376626}{0.565104111084}
  \meshline{144,144,144}{0.713677479238}{0.637277912301}{0.747307279575}{0.649588929027}
  \meshline{144,144,144}{0.787534756475}{0.663399045183}{0.771955029493}{0.658267494804}
  \meshline{144,144,144}{0.847620161225}{0.575980199769}{0.839426364051}{0.574165763515}
  \meshline{144,144,144}{0.771955029493}{0.658267494804}{0.754600062469}{0.652279276116}
  \meshline{144,144,144}{0.345271601361}{0.292166730018}{0.334477860226}{0.282589055357}
  \meshline{144,144,144}{0.306200989976}{0.254880070585}{0.321274888585}{0.270277641650}
  \meshline{144,144,144}{0.569226455766}{0.216044864070}{0.582078885043}{0.231516136083}
  \meshline{144,144,144}{0.983758273414}{0.593429750354}{1.000000000000}{0.594022957613}
  \meshline{144,144,144}{0.896041079887}{0.585709775385}{0.914462079716}{0.588287275289}
  \meshline{144,144,144}{0.775050466423}{0.555813322642}{0.788112754826}{0.559955377868}
  \meshline{144,144,144}{0.804504376626}{0.565104111084}{0.833818320430}{0.572675867811}
  \meshline{144,144,144}{0.837556349943}{0.573732349051}{0.833818320430}{0.572675867811}
  \meshline{144,144,144}{0.749794217278}{0.546889083676}{0.775050466423}{0.555813322642}
  \meshline{144,144,144}{0.931680186766}{0.590444953185}{0.914462079716}{0.588287275289}
  \meshline{144,144,144}{0.839426364051}{0.574165763515}{0.837556349943}{0.573732349051}
  \meshline{144,144,144}{0.951979495493}{0.591912185728}{0.931680186766}{0.590444953185}
  \meshline{144,144,144}{0.951979495493}{0.591912185728}{0.963171092985}{0.592939833973}
  \meshline{144,144,144}{0.963171092985}{0.592939833973}{0.983758273414}{0.593429750354}
  \meshline{144,144,144}{0.865956387266}{0.580219294105}{0.869539340858}{0.580906444290}
  \meshline{144,144,144}{0.915049828002}{0.691506344201}{0.896985677098}{0.688854734002}
  \meshline{144,144,144}{0.861508911242}{0.681978721770}{0.837813069794}{0.677104991470}
  \meshline{144,144,144}{0.821928303670}{0.673244393018}{0.837813069794}{0.677104991470}
  \meshline{144,144,144}{0.865956387266}{0.580219294105}{0.847620161225}{0.575980199769}
  \meshline{144,144,144}{0.896041079887}{0.585709775385}{0.869539340858}{0.580906444290}
  \meshline{144,144,144}{0.679641394510}{0.000000000000}{0.681375739133}{0.019115336415}
  \meshline{144,144,144}{0.681375739133}{0.019115336415}{0.683006905630}{0.039101749244}
  \meshline{144,144,144}{0.687067410981}{0.056601422883}{0.683006905630}{0.039101749244}
  \meshline{144,144,144}{0.545932365163}{0.558617249123}{0.552418994506}{0.561984058632}
  \meshline{144,144,144}{0.505279969429}{0.099053381012}{0.518613644862}{0.132469338664}
  \meshline{144,144,144}{0.412610659008}{0.484051516191}{0.430711412582}{0.494543156405}
  \meshline{144,144,144}{0.530664024583}{0.157372226106}{0.535035199527}{0.165020023445}
  \meshline{144,144,144}{0.518907024018}{0.133135513027}{0.518613644862}{0.132469338664}
  \meshline{144,144,144}{0.535035199527}{0.165020023445}{0.551959228580}{0.192021229818}
  \meshline{144,144,144}{0.552785390900}{0.193202505936}{0.551959228580}{0.192021229818}
  \meshline{144,144,144}{0.505279969429}{0.099053381012}{0.502401100831}{0.089636707715}
  \meshline{144,144,144}{0.530664024583}{0.157372226106}{0.518907024018}{0.133135513027}
  \meshline{144,144,144}{0.489171853758}{0.010978523777}{0.490027489033}{0.030451789558}
  \meshline{144,144,144}{0.489171853758}{0.010978523777}{0.488621709428}{0.000000000000}
  \meshline{144,144,144}{0.554291255929}{0.195176496287}{0.552785390900}{0.193202505936}
  \meshline{144,144,144}{0.569226455766}{0.216044864070}{0.554291255929}{0.195176496287}
  \meshline{144,144,144}{0.496103056943}{0.065262903948}{0.502401100831}{0.089636707715}
  \meshline{144,144,144}{0.490027489033}{0.030451789558}{0.493323685875}{0.050634693698}
  \meshline{144,144,144}{0.321274888585}{0.270277641650}{0.334477860226}{0.282589055357}
  \meshline{144,144,144}{0.288279353366}{0.238589455388}{0.297699272885}{0.247328985510}
  \meshline{144,144,144}{0.255579195850}{0.203418603370}{0.251864091361}{0.200014859771}
  \meshline{144,144,144}{0.496103056943}{0.065262903948}{0.493323685875}{0.050634693698}
  \meshline{144,144,144}{0.255579195850}{0.203418603370}{0.268068236113}{0.218032225176}
  \meshline{144,144,144}{0.196048705884}{0.132195502469}{0.205821429399}{0.145331526554}
  \meshline{144,144,144}{0.214445444521}{0.155894637453}{0.226813986044}{0.172247306269}
  \meshline{144,144,144}{0.171504664713}{0.093658575132}{0.181020780706}{0.111554569604}
  \meshline{144,144,144}{0.196048705884}{0.132195502469}{0.191925184484}{0.125109820530}
  \meshline{144,144,144}{0.329082895633}{0.435669258455}{0.318918099895}{0.430343627645}
  \meshline{144,144,144}{0.220907397060}{0.377556098333}{0.234057831119}{0.384334855932}
  \meshline{144,144,144}{0.173294272904}{0.355360379183}{0.196759894777}{0.366555418453}
  \meshline{144,144,144}{0.254612638799}{0.395101723331}{0.234057831119}{0.384334855932}
  \meshline{144,144,144}{0.251864091361}{0.200014859771}{0.236173502522}{0.181677047412}
  \meshline{144,144,144}{0.236173502522}{0.181677047412}{0.226813986044}{0.172247306269}
  \meshline{144,144,144}{0.214445444521}{0.155894637453}{0.205821429399}{0.145331526554}
  \meshline{144,144,144}{0.143988790983}{0.021232441024}{0.145916399703}{0.036562356945}
  \meshline{144,144,144}{0.171504664713}{0.093658575132}{0.164346405566}{0.083803622507}
  \meshline{144,144,144}{0.181020780706}{0.111554569604}{0.191925184484}{0.125109820530}
  \meshline{144,144,144}{0.156185164554}{0.066689948257}{0.150077148185}{0.044788795054}
  \meshline{144,144,144}{0.145916399703}{0.036562356945}{0.150077148185}{0.044788795054}
  \meshline{144,144,144}{0.143988790983}{0.021232441024}{0.141173422658}{0.000000000000}
  \meshline{144,144,144}{0.156185164554}{0.066689948257}{0.164346405566}{0.083803622507}
  \meshline{144,144,144}{0.000000000000}{0.315384264528}{0.024502005478}{0.316390414324}
  \meshline{144,144,144}{0.125024294128}{0.337190372677}{0.121168931378}{0.336312729452}
  \meshline{144,144,144}{0.136093954189}{0.341177974275}{0.161955136720}{0.350341229287}
  \meshline{144,144,144}{0.108563555133}{0.332776860560}{0.121168931378}{0.336312729452}
  \meshline{144,144,144}{0.161955136720}{0.350341229287}{0.173294272904}{0.355360379183}
  \meshline{144,144,144}{0.053220546444}{0.319172282741}{0.035973872304}{0.317485395609}
  \meshline{144,144,144}{0.053220546444}{0.319172282741}{0.061516078704}{0.321228723093}
  \meshline{144,144,144}{0.108563555133}{0.332776860560}{0.088384175079}{0.326504475166}
  \meshline{144,144,144}{0.061516078704}{0.321228723093}{0.088384175079}{0.326504475166}
  \meshline{144,144,144}{0.024502005478}{0.316390414324}{0.035973872304}{0.317485395609}
  \meshline{144,144,144}{0.802354655357}{0.667662283703}{0.821928303670}{0.673244393018}
  \meshline{144,144,144}{0.931313759542}{0.693420630599}{0.915049828002}{0.691506344201}
  \meshline{144,144,144}{0.262508132027}{0.399052913122}{0.291303742817}{0.414530168266}
  \meshline{144,144,144}{0.896985677098}{0.688854734002}{0.861508911242}{0.681978721770}
  \meshline{144,144,144}{1.000000000000}{0.697001110443}{0.988897630541}{0.696558482964}
  \meshline{144,144,144}{0.951263714173}{0.695119680724}{0.931313759542}{0.693420630599}
  \meshline{144,144,144}{0.988897630541}{0.696558482964}{0.967021249463}{0.696137360690}
  \meshline{144,144,144}{0.951263714173}{0.695119680724}{0.967021249463}{0.696137360690}
  \meshline{144,144,144}{0.734269566337}{0.899296528030}{0.735727055960}{0.899973367468}
  \meshline{144,144,144}{0.836332895820}{0.948137204783}{0.833370546461}{0.946782016678}
  \meshline{144,144,144}{0.771095793870}{0.918329074592}{0.735727055960}{0.899973367468}
  \meshline{144,144,144}{0.771095793870}{0.918329074592}{0.772241350478}{0.918830257929}
  \meshline{144,144,144}{0.772241350478}{0.918830257929}{0.774014407660}{0.919597807420}
  \meshline{144,144,144}{0.663919963577}{0.860426521581}{0.684106003788}{0.871411631401}
  \meshline{144,144,144}{0.803215569999}{0.933948481411}{0.774014407660}{0.919597807420}
  \meshline{144,144,144}{0.689773469979}{1.040064740222}{0.695523816278}{1.046506152580}
  \meshline{144,144,144}{0.876551355122}{0.963024603608}{0.872782731719}{0.961392293012}
  \meshline{144,144,144}{0.833370546461}{0.946782016678}{0.803215569999}{0.933948481411}
  \meshline{144,144,144}{0.695523816278}{1.046506152580}{0.713484579820}{1.063996178987}
  \meshline{144,144,144}{0.837275509940}{0.948577632641}{0.836332895820}{0.948137204783}
  \meshline{144,144,144}{0.911378546772}{0.973165097808}{0.924842466778}{0.976908622615}
  \meshline{144,144,144}{0.872782731719}{0.961392293012}{0.837275509940}{0.948577632641}
  \meshline{144,144,144}{0.709517563093}{0.885783121948}{0.700996983217}{0.881301566099}
  \meshline{144,144,144}{0.709517563093}{0.885783121948}{0.734269566337}{0.899296528030}
  \meshline{144,144,144}{0.663919963577}{0.860426521581}{0.649151400625}{0.851586364681}
  \meshline{144,144,144}{0.579929721218}{0.811750481478}{0.593325706018}{0.819328333871}
  \meshline{144,144,144}{0.882165209501}{0.964919656897}{0.876551355122}{0.963024603608}
  \meshline{144,144,144}{0.911378546772}{0.973165097808}{0.882165209501}{0.964919656897}
  \meshline{144,144,144}{0.960196644964}{0.982287011390}{0.954582699224}{0.981495725853}
  \meshline{144,144,144}{0.924842466778}{0.976908622615}{0.954582699224}{0.981495725853}
  \meshline{144,144,144}{0.630973491096}{0.987043259129}{0.638506152835}{0.994039647843}
  \meshline{144,144,144}{0.700996983217}{0.881301566099}{0.684106003788}{0.871411631401}
  \meshline{144,144,144}{0.960196644964}{0.982287011390}{0.970602145656}{0.982796240677}
  \meshline{144,144,144}{0.970602145656}{0.982796240677}{1.000000000000}{0.984556377322}
  \meshline{144,144,144}{0.845803947708}{1.240665189654}{0.836997438987}{1.222958145824}
  \meshline{144,144,144}{0.610571554755}{0.969661643760}{0.601211360139}{0.961665877977}
  \meshline{144,144,144}{0.638506152835}{0.994039647843}{0.658349181089}{1.011171084245}
  \meshline{144,144,144}{0.721756172294}{1.072844364770}{0.713484579820}{1.063996178987}
  \meshline{144,144,144}{0.689773469979}{1.040064740222}{0.682522849622}{1.032955017503}
  \meshline{144,144,144}{0.774710188225}{1.131079324496}{0.751478684560}{1.103040581815}
  \meshline{144,144,144}{0.742661133736}{1.094803607410}{0.729383884760}{1.079886528441}
  \meshline{144,144,144}{0.742661133736}{1.094803607410}{0.751478684560}{1.103040581815}
  \meshline{144,144,144}{0.774710188225}{1.131079324496}{0.776599026425}{1.132874348855}
  \meshline{144,144,144}{0.729383884760}{1.079886528441}{0.721756172294}{1.072844364770}
  \meshline{144,144,144}{0.801024472807}{1.164328306571}{0.778874121596}{1.135236034439}
  \meshline{144,144,144}{0.776599026425}{1.132874348855}{0.778874121596}{1.135236034439}
  \meshline{144,144,144}{0.801024472807}{1.164328306571}{0.811425764338}{1.177349131849}
  \meshline{144,144,144}{0.831758014452}{1.209738828092}{0.836997438987}{1.222958145824}
  \meshline{144,144,144}{0.020117121812}{1.021584184043}{0.030385459311}{1.022308436028}
  \meshline{144,144,144}{0.329082895633}{0.435669258455}{0.352625980146}{0.449514910825}
  \meshline{144,144,144}{0.627084223949}{0.983364083154}{0.630973491096}{0.987043259129}
  \meshline{144,144,144}{0.566484931761}{0.934015591695}{0.585570154322}{0.949591005146}
  \meshline{144,144,144}{0.610571554755}{0.969661643760}{0.627084223949}{0.983364083154}
  \meshline{144,144,144}{0.585570154322}{0.949591005146}{0.601211360139}{0.961665877977}
  \meshline{144,144,144}{0.276829514288}{0.763353595212}{0.277360716821}{0.763569391420}
  \meshline{144,144,144}{0.279207765830}{0.764371326573}{0.310706098750}{0.777742550549}
  \meshline{144,144,144}{0.593325706018}{0.819328333871}{0.614497320115}{0.831651431277}
  \meshline{144,144,144}{0.566484931761}{0.934015591695}{0.542640764514}{0.916106268023}
  \meshline{144,144,144}{0.617337669058}{0.833366153057}{0.649151400625}{0.851586364681}
  \meshline{144,144,144}{0.617337669058}{0.833366153057}{0.616138336499}{0.832633007769}
  \meshline{144,144,144}{0.570159595807}{0.805941390493}{0.579929721218}{0.811750481478}
  \meshline{144,144,144}{0.616138336499}{0.832633007769}{0.614497320115}{0.831651431277}
  \meshline{144,144,144}{0.682522849622}{1.032955017503}{0.658349181089}{1.011171084245}
  \meshline{144,144,144}{0.858369070482}{1.300000000000}{0.854917806478}{1.275764445727}
  \meshline{144,144,144}{0.885865735582}{0.017817054856}{0.888420187810}{0.030916676896}
  \meshline{144,144,144}{0.904020403763}{0.058883218918}{0.890702851953}{0.035210176574}
  \meshline{144,144,144}{0.904925654173}{0.060372036861}{0.905160968204}{0.060682468766}
  \meshline{144,144,144}{0.570159595807}{0.805941390493}{0.560298139856}{0.800224476159}
  \meshline{144,144,144}{0.455848571820}{1.120011542903}{0.463390675144}{1.131744332992}
  \meshline{144,144,144}{0.854613031011}{1.271267106651}{0.854917806478}{1.275764445727}
  \meshline{144,144,144}{0.511458897238}{1.300000000000}{0.510778342370}{1.283635140342}
  \meshline{144,144,144}{0.492755686639}{1.196763235643}{0.500547448417}{1.219612698774}
  \meshline{144,144,144}{0.506741505267}{1.248081903737}{0.503638697425}{1.235136563406}
  \meshline{144,144,144}{0.510270168600}{1.271054328637}{0.510778342370}{1.283635140342}
  \meshline{144,144,144}{0.820658047236}{1.193615992745}{0.811425764338}{1.177349131849}
  \meshline{144,144,144}{0.831758014452}{1.209738828092}{0.820658047236}{1.193615992745}
  \meshline{144,144,144}{0.847148582466}{1.246863763596}{0.854613031011}{1.271267106651}
  \meshline{144,144,144}{0.291303742817}{0.414530168266}{0.318918099895}{0.430343627645}
  \meshline{144,144,144}{0.368836743451}{0.458462388659}{0.384958248265}{0.467978184940}
  \meshline{144,144,144}{0.520068412436}{0.544660475443}{0.516359555958}{0.542683771662}
  \meshline{144,144,144}{0.393934909160}{0.473461541829}{0.384958248265}{0.467978184940}
  \meshline{144,144,144}{0.368836743451}{0.458462388659}{0.352625980146}{0.449514910825}
  \meshline{144,144,144}{0.262508132027}{0.399052913122}{0.260393785179}{0.398035001830}
  \meshline{144,144,144}{0.264349317138}{0.654357982696}{0.303593357029}{0.669961053558}
  \meshline{144,144,144}{0.162544848690}{0.623111295390}{0.177504629406}{0.626765720760}
  \meshline{144,144,144}{0.205320267579}{0.370074850881}{0.196759894777}{0.366555418453}
  \meshline{144,144,144}{0.136093954189}{0.341177974275}{0.128393697123}{0.338224270872}
  \meshline{144,144,144}{0.220907397060}{0.377556098333}{0.205320267579}{0.370074850881}
  \meshline{144,144,144}{0.081446964339}{0.608193259064}{0.118740011324}{0.613758801952}
  \meshline{144,144,144}{0.128393697123}{0.338224270872}{0.125024294128}{0.337190372677}
  \meshline{144,144,144}{0.162544848690}{0.623111295390}{0.135662210771}{0.616954084691}
  \meshline{144,144,144}{0.226138504280}{0.641354704219}{0.214625132496}{0.637456100822}
  \meshline{144,144,144}{0.214625132496}{0.637456100822}{0.206917763833}{0.635345359170}
  \meshline{144,144,144}{0.072255122120}{0.607274346622}{0.044253129805}{0.604402908417}
  \meshline{144,144,144}{0.206917763833}{0.635345359170}{0.177504629406}{0.626765720760}
  \meshline{144,144,144}{0.035970373277}{0.603933984666}{0.044253129805}{0.604402908417}
  \meshline{144,144,144}{0.135662210771}{0.616954084691}{0.118740011324}{0.613758801952}
  \meshline{144,144,144}{0.145829191804}{0.722216633964}{0.116272700382}{0.716211578573}
  \meshline{144,144,144}{0.009070807246}{0.603489894554}{0.000000000000}{0.603157071214}
  \meshline{144,144,144}{0.072255122120}{0.607274346622}{0.078571805687}{0.607785528663}
  \meshline{144,144,144}{0.078571805687}{0.607785528663}{0.081446964339}{0.608193259064}
  \meshline{144,144,144}{0.009070807246}{0.603489894554}{0.035970373277}{0.603933984666}
  \meshline{144,144,144}{0.041793780195}{0.707405879957}{0.060101317820}{0.708888803884}
  \meshline{144,144,144}{0.145829191804}{0.722216633964}{0.150176858275}{0.723181989875}
  \meshline{144,144,144}{0.339305180891}{0.685098717044}{0.349017590718}{0.689326470336}
  \meshline{144,144,144}{0.226138504280}{0.641354704219}{0.264349317138}{0.654357982696}
  \meshline{144,144,144}{0.449335924223}{0.504962846366}{0.436132256904}{0.497553723330}
  \meshline{144,144,144}{0.516359555958}{0.542683771662}{0.505476580757}{0.536661436476}
  \meshline{144,144,144}{0.477755879985}{0.521132113753}{0.484592477601}{0.525149868074}
  \meshline{144,144,144}{0.412610659008}{0.484051516191}{0.393934909160}{0.473461541829}
  \meshline{144,144,144}{0.436132256904}{0.497553723330}{0.430711412582}{0.494543156405}
  \meshline{144,144,144}{0.386992591270}{0.707344394325}{0.381816658664}{0.704756543716}
  \meshline{144,144,144}{0.349017590718}{0.689326470336}{0.379809445478}{0.703813559106}
  \meshline{144,144,144}{0.379809445478}{0.703813559106}{0.381816658664}{0.704756543716}
  \meshline{144,144,144}{0.339305180891}{0.685098717044}{0.312801807758}{0.673556438702}
  \meshline{144,144,144}{0.386992591270}{0.707344394325}{0.416831092632}{0.722044170780}
  \meshline{144,144,144}{0.378491441532}{0.811380141086}{0.394480903175}{0.819892717680}
  \meshline{144,144,144}{0.060101317820}{0.708888803884}{0.088137330353}{0.711859620123}
  \meshline{144,144,144}{0.030731762318}{0.706514933984}{0.041793780195}{0.707405879957}
  \meshline{144,144,144}{0.107327062211}{0.714808962100}{0.088137330353}{0.711859620123}
  \meshline{144,144,144}{0.116272700382}{0.716211578573}{0.107327062211}{0.714808962100}
  \meshline{144,144,144}{0.030731762318}{0.706514933984}{0.008946241454}{0.706154880620}
  \meshline{144,144,144}{0.027907805603}{0.875426333986}{0.028884002702}{0.875481329065}
  \meshline{144,144,144}{0.008946241454}{0.706154880620}{0.000000000000}{0.705885637599}
  \meshline{144,144,144}{0.000000000000}{0.874285677234}{0.027907805603}{0.875426333986}
  \meshline{144,144,144}{0.118335653828}{0.888001499031}{0.074234825373}{0.879903298213}
  \meshline{144,144,144}{0.164370950949}{0.726924610005}{0.150176858275}{0.723181989875}
  \meshline{144,144,144}{0.184626597593}{0.731888038387}{0.201899423087}{0.736892048213}
  \meshline{144,144,144}{0.154364476414}{0.897313631411}{0.178181796487}{0.905284277515}
  \meshline{144,144,144}{0.244260050098}{0.750756027878}{0.253525262970}{0.754250424059}
  \meshline{144,144,144}{0.178181796487}{0.905284277515}{0.184938137549}{0.907698040251}
  \meshline{144,144,144}{0.201899423087}{0.736892048213}{0.220470934787}{0.742603471737}
  \meshline{144,144,144}{0.478802739312}{1.160834574307}{0.485827152041}{1.177817182128}
  \meshline{144,144,144}{0.164370950949}{0.726924610005}{0.184626597593}{0.731888038387}
  \meshline{144,144,144}{0.118335653828}{0.888001499031}{0.121256661399}{0.888701755896}
  \meshline{144,144,144}{0.071401375781}{0.879536489656}{0.028884002702}{0.875481329065}
  \meshline{144,144,144}{0.500547448417}{1.219612698774}{0.503638697425}{1.235136563406}
  \meshline{144,144,144}{0.420186763241}{1.071380455339}{0.438177577369}{1.093349987148}
  \meshline{144,144,144}{0.389135108199}{1.037011743609}{0.412554600056}{1.061719039054}
  \meshline{144,144,144}{0.074234825373}{0.879903298213}{0.071401375781}{0.879536489656}
  \meshline{144,144,144}{0.121256661399}{0.888701755896}{0.154364476414}{0.897313631411}
  \meshline{144,144,144}{0.508211127014}{1.258891177237}{0.510270168600}{1.271054328637}
  \meshline{144,144,144}{0.301421419815}{1.208314147388}{0.309041827554}{1.228273178568}
  \meshline{144,144,144}{0.463390675144}{1.131744332992}{0.469676162177}{1.144099958584}
  \meshline{144,144,144}{0.455848571820}{1.120011542903}{0.438177577369}{1.093349987148}
  \meshline{144,144,144}{0.508211127014}{1.258891177237}{0.506741505267}{1.248081903737}
  \meshline{144,144,144}{0.492755686639}{1.196763235643}{0.489116976816}{1.185406754954}
  \meshline{144,144,144}{0.485827152041}{1.177817182128}{0.489116976816}{1.185406754954}
  \meshline{144,144,144}{0.478802739312}{1.160834574307}{0.469676162177}{1.144099958584}
  \meshline{144,144,144}{0.420186763241}{1.071380455339}{0.415398401081}{1.065090352357}
  \meshline{144,144,144}{0.415398401081}{1.065090352357}{0.412554600056}{1.061719039054}
  \meshline{144,144,144}{0.318865593933}{0.978314923056}{0.334178272709}{0.989073273043}
  \meshline{144,144,144}{0.054041527020}{1.025102205080}{0.062834881860}{1.026554254208}
  \meshline{144,144,144}{0.125370354116}{1.044285783744}{0.130499819136}{1.045954395526}
  \meshline{144,144,144}{0.125370354116}{1.044285783744}{0.095103219743}{1.034115902284}
  \meshline{144,144,144}{0.528093762319}{0.905722031835}{0.539698920912}{0.914015343453}
  \meshline{144,144,144}{0.229642513243}{0.926301011055}{0.210193757211}{0.917574818660}
  \meshline{144,144,144}{0.133054278067}{1.046898759242}{0.138247277401}{1.049237838893}
  \meshline{144,144,144}{0.130499819136}{1.045954395526}{0.133054278067}{1.046898759242}
  \meshline{144,144,144}{0.159562009512}{1.059078108630}{0.138247277401}{1.049237838893}
  \meshline{144,144,144}{0.095103219743}{1.034115902284}{0.073825754515}{1.029031471481}
  \meshline{144,144,144}{0.510193831472}{0.892710990075}{0.490615575615}{0.879194788478}
  \meshline{144,144,144}{0.542640764514}{0.916106268023}{0.539698920912}{0.914015343453}
  \meshline{144,144,144}{0.054041527020}{1.025102205080}{0.030385459311}{1.022308436028}
  \meshline{144,144,144}{0.020117121812}{1.021584184043}{0.000000000000}{1.020852253687}
  \meshline{144,144,144}{0.062834881860}{1.026554254208}{0.073825754515}{1.029031471481}
  \meshline{144,144,144}{0.490615575615}{0.879194788478}{0.480629050839}{0.872131028385}
  \meshline{144,144,144}{0.528093762319}{0.905722031835}{0.512243275637}{0.894268838908}
  \meshline{144,144,144}{0.510193831472}{0.892710990075}{0.512243275637}{0.894268838908}
  \meshline{144,144,144}{0.341028546089}{0.994609042674}{0.359325429877}{1.009113125874}
  \meshline{144,144,144}{0.371421079888}{1.020151468800}{0.386198386572}{1.033990543429}
  \meshline{144,144,144}{0.389135108199}{1.037011743609}{0.386198386572}{1.033990543429}
  \meshline{144,144,144}{0.334178272709}{0.989073273043}{0.341028546089}{0.994609042674}
  \meshline{144,144,144}{0.371421079888}{1.020151468800}{0.359325429877}{1.009113125874}
  \meshline{144,144,144}{0.318865593933}{0.978314923056}{0.306025683435}{0.968961107995}
  \meshline{144,144,144}{0.252819455092}{1.130515791068}{0.268313815196}{1.149847710248}
  \meshline{144,144,144}{0.252819455092}{1.130515791068}{0.243278761260}{1.120823153613}
  \meshline{144,144,144}{0.339764327034}{0.791483711774}{0.310706098750}{0.777742550549}
  \meshline{144,144,144}{0.346648474099}{0.794725315652}{0.339764327034}{0.791483711774}
  \meshline{144,144,144}{0.422323976712}{0.835919013882}{0.417007208663}{0.832865188801}
  \meshline{144,144,144}{0.417007208663}{0.832865188801}{0.394480903175}{0.819892717680}
  \meshline{144,144,144}{0.422323976712}{0.835919013882}{0.428128361089}{0.839549980448}
  \meshline{144,144,144}{0.363178762122}{0.803321908324}{0.373057540013}{0.808317084466}
  \meshline{144,144,144}{0.480629050839}{0.872131028385}{0.463073267626}{0.860958832993}
  \meshline{144,144,144}{0.286639533288}{0.956912916933}{0.306025683435}{0.968961107995}
  \meshline{144,144,144}{0.229642513243}{0.926301011055}{0.250410214895}{0.936255845689}
  \meshline{144,144,144}{0.184938137549}{0.907698040251}{0.210193757211}{0.917574818660}
  \meshline{144,144,144}{0.269231779552}{0.946807646043}{0.250410214895}{0.936255845689}
  \meshline{144,144,144}{0.276829514288}{0.763353595212}{0.274915971880}{0.762636624102}
  \meshline{144,144,144}{0.373057540013}{0.808317084466}{0.378491441532}{0.811380141086}
  \meshline{144,144,144}{0.346648474099}{0.794725315652}{0.363178762122}{0.803321908324}
  \meshline{144,144,144}{0.286639533288}{0.956912916933}{0.269231779552}{0.946807646043}
  \meshline{144,144,144}{0.483000099425}{0.757116179780}{0.464956703156}{0.747184259362}
  \meshline{144,144,144}{0.416831092632}{0.722044170780}{0.435519444998}{0.731655856515}
  \meshline{144,144,144}{0.435519444998}{0.731655856515}{0.444399227586}{0.736334608728}
  \meshline{144,144,144}{0.464956703156}{0.747184259362}{0.444399227586}{0.736334608728}
  \meshline{144,144,144}{0.463073267626}{0.860958832993}{0.449973045649}{0.852638053285}
  \meshline{144,144,144}{0.428128361089}{0.839549980448}{0.449973045649}{0.852638053285}
  \meshline{144,144,144}{0.498089339905}{0.765212814116}{0.483000099425}{0.757116179780}
  \meshline{144,144,144}{0.533960335602}{0.785417781781}{0.511299933424}{0.772546179271}
  \meshline{144,144,144}{0.560298139856}{0.800224476159}{0.533960335602}{0.785417781781}
  \meshline{144,144,144}{0.498089339905}{0.765212814116}{0.511299933424}{0.772546179271}
  \meshline{144,144,144}{0.279207765830}{0.764371326573}{0.277360716821}{0.763569391420}
  \meshline{144,144,144}{0.253525262970}{0.754250424059}{0.274915971880}{0.762636624102}
  \meshline{144,144,144}{0.220470934787}{0.742603471737}{0.244260050098}{0.750756027878}
  \meshline{144,144,144}{0.303593357029}{0.669961053558}{0.309788707325}{0.672324640916}
  \meshline{144,144,144}{0.312801807758}{0.673556438702}{0.309788707325}{0.672324640916}
  \meshline{144,144,144}{0.212693263924}{1.092904153461}{0.199841492114}{1.084634438805}
  \meshline{144,144,144}{0.199841492114}{1.084634438805}{0.159562009512}{1.059078108630}
  \meshline{144,144,144}{0.000000000000}{1.196031207254}{0.004381212973}{1.196157897817}
  \meshline{144,144,144}{0.112795982135}{1.281342698570}{0.115227200802}{1.300000000000}
  \meshline{144,144,144}{0.031959038904}{1.200645548125}{0.004381212973}{1.196157897817}
  \meshline{144,144,144}{0.087630919377}{1.231551143920}{0.087658897535}{1.231581755929}
  \meshline{144,144,144}{0.063593090101}{1.213748641672}{0.045936062398}{1.205243277630}
  \meshline{144,144,144}{0.112795982135}{1.281342698570}{0.109533211573}{1.264578470057}
  \meshline{144,144,144}{0.087569057805}{1.231501836267}{0.087630919377}{1.231551143920}
  \meshline{144,144,144}{0.045936062398}{1.205243277630}{0.031959038904}{1.200645548125}
  \meshline{144,144,144}{0.087569057805}{1.231501836267}{0.063593090101}{1.213748641672}
  \meshline{144,144,144}{0.103656027309}{1.253625134569}{0.087658897535}{1.231581755929}
  \meshline{144,144,144}{0.103656027309}{1.253625134569}{0.109533211573}{1.264578470057}
  \meshline{144,144,144}{0.295461087508}{1.195050135645}{0.280558206763}{1.167614434926}
  \meshline{144,144,144}{0.280558206763}{1.167614434926}{0.268981025041}{1.150778674647}
  \meshline{144,144,144}{0.268313815196}{1.149847710248}{0.268981025041}{1.150778674647}
  \meshline{144,144,144}{0.299569640322}{1.203195877198}{0.295461087508}{1.195050135645}
  \meshline{144,144,144}{0.314159606729}{1.246694966137}{0.315132097471}{1.250432103388}
  \meshline{144,144,144}{0.315132097471}{1.250432103388}{0.315466810623}{1.253960046905}
  \meshline{144,144,144}{0.309041827554}{1.228273178568}{0.314159606729}{1.246694966137}
  \meshline{144,144,144}{0.315466810623}{1.253960046905}{0.320181201765}{1.300000000000}
  \meshline{144,144,144}{0.301421419815}{1.208314147388}{0.299569640322}{1.203195877198}
  \meshline{144,144,144}{0.212693263924}{1.092904153461}{0.217716039159}{1.097240525590}
  \meshline{144,144,144}{0.243278761260}{1.120823153613}{0.217716039159}{1.097240525590}
  \meshline{144,144,144}{0.847148582466}{1.246863763596}{0.845803947708}{1.240665189654}
\end{pgfscope}


==> nodal_rectsquare_N0.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1.3, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{168,0,57}{0.837218746036}{0.797527784041}{0.867515757949}{0.805509591296}
  \meshline{168,0,57}{0.924601097411}{0.815931278769}{0.946374963558}{0.818199416621}
  \meshline{168,0,57}{0.913786238091}{0.814314909405}{0.924601097411}{0.815931278769}
  \meshline{168,0,57}{0.878740589246}{0.807822075197}{0.895159204609}{0.810999375210}
  \meshline{168,0,57}{1.000000000000}{0.821310608861}{0.991580627760}{0.820989180245}
  \meshline{168,0,57}{0.946374963558}{0.818199416621}{0.952736848449}{0.818939224244}
  \meshline{168,0,57}{0.991580627760}{0.820989180245}{0.952736848449}{0.818939224244}
  \meshline{168,0,57}{0.692627178018}{0.744410196916}{0.697481158999}{0.746398173872}
  \meshline{168,0,57}{0.831451841310}{0.795699023120}{0.800165674330}{0.786441224034}
  \meshline{168,0,57}{0.835326508478}{0.796970560402}{0.831451841310}{0.795699023120}
  \meshline{168,0,57}{0.785269532926}{0.781361422222}{0.771318708759}{0.776201958298}
  \meshline{168,0,57}{0.913786238091}{0.814314909405}{0.895159204609}{0.810999375210}
  \meshline{168,0,57}{0.878740589246}{0.807822075197}{0.867515757949}{0.805509591296}
  \meshline{168,0,57}{0.740778733786}{0.764466638190}{0.728536072221}{0.759885085787}
  \meshline{168,0,57}{0.837218746036}{0.797527784041}{0.835326508478}{0.796970560402}
  \meshline{168,0,57}{0.756041343568}{0.770114386326}{0.740778733786}{0.764466638190}
  \meshline{168,0,57}{0.785269532926}{0.781361422222}{0.800165674330}{0.786441224034}
  \meshline{168,0,57}{0.756041343568}{0.770114386326}{0.771318708759}{0.776201958298}
  \meshline{168,0,57}{0.633363006887}{0.717063178181}{0.631670548460}{0.716256842500}
  \meshline{168,0,57}{0.661766060261}{0.730521771614}{0.633363006887}{0.717063178181}
  \meshline{168,0,57}{0.728536072221}{0.759885085787}{0.697481158999}{0.746398173872}
  \meshline{168,0,57}{0.599291958249}{0.700523332065}{0.630670870599}{0.715753583288}
  \meshline{168,0,57}{0.661766060261}{0.730521771614}{0.671131613997}{0.734537467446}
  \meshline{168,0,57}{0.671131613997}{0.734537467446}{0.692627178018}{0.744410196916}
  \meshline{168,0,57}{0.631670548460}{0.716256842500}{0.630670870599}{0.715753583288}
  \meshline{168,0,57}{0.599291958249}{0.700523332065}{0.585590450143}{0.693559004251}
  \meshline{168,0,57}{0.568961399050}{0.685312005757}{0.585590450143}{0.693559004251}
  \meshline{168,0,57}{0.281727754085}{0.544653701460}{0.281271629509}{0.544447086312}
  \meshline{168,0,57}{0.349357196003}{0.574707254663}{0.338746108970}{0.569728259069}
  \meshline{168,0,57}{0.309099599949}{0.556082049875}{0.335020876477}{0.568122649842}
  \meshline{168,0,57}{0.232902384509}{0.524968589002}{0.199732378866}{0.513796997605}
  \meshline{168,0,57}{0.107036398361}{0.489267212610}{0.091514159821}{0.486743706232}
  \meshline{168,0,57}{0.161644051018}{0.502216811818}{0.194150145204}{0.512076527226}
  \meshline{168,0,57}{0.107036398361}{0.489267212610}{0.124866867092}{0.492946718064}
  \meshline{168,0,57}{0.280741056726}{0.544232805391}{0.281271629509}{0.544447086312}
  \meshline{168,0,57}{0.199732378866}{0.513796997605}{0.198033715753}{0.513196221196}
  \meshline{168,0,57}{0.197529784762}{0.513034568981}{0.196977349789}{0.512885531713}
  \meshline{168,0,57}{0.161644051018}{0.502216811818}{0.147401758031}{0.498228635998}
  \meshline{168,0,57}{0.280741056726}{0.544232805391}{0.249772561153}{0.531706369878}
  \meshline{168,0,57}{0.232902384509}{0.524968589002}{0.249772561153}{0.531706369878}
  \meshline{168,0,57}{0.091514159821}{0.486743706232}{0.075489092094}{0.484009506038}
  \meshline{168,0,57}{0.147401758031}{0.498228635998}{0.124866867092}{0.492946718064}
  \meshline{168,0,57}{0.037341860257}{0.480312720618}{0.041021047285}{0.480696038470}
  \meshline{168,0,57}{0.281727754085}{0.544653701460}{0.309099599949}{0.556082049875}
  \meshline{168,0,57}{0.335020876477}{0.568122649842}{0.338746108970}{0.569728259069}
  \meshline{168,0,57}{0.198033715753}{0.513196221196}{0.197529784762}{0.513034568981}
  \meshline{168,0,57}{0.196977349789}{0.512885531713}{0.194150145204}{0.512076527226}
  \meshline{168,0,57}{0.349357196003}{0.574707254663}{0.377674108284}{0.588172044144}
  \meshline{168,0,57}{0.030785833294}{0.480123202741}{0.000000000000}{0.478821469097}
  \meshline{168,0,57}{0.377674108284}{0.588172044144}{0.393340752673}{0.595996904894}
  \meshline{168,0,57}{0.409672296806}{0.603918007378}{0.393340752673}{0.595996904894}
  \meshline{168,0,57}{0.446823514626}{0.622737069934}{0.430659828288}{0.614619682218}
  \meshline{168,0,57}{0.430659828288}{0.614619682218}{0.409672296806}{0.603918007378}
  \meshline{168,0,57}{0.446823514626}{0.622737069934}{0.466794803046}{0.632999584016}
  \meshline{168,0,57}{0.500066701873}{0.650041199219}{0.528525610630}{0.664670176011}
  \meshline{168,0,57}{0.482092676098}{0.640811194531}{0.466794803046}{0.632999584016}
  \meshline{168,0,57}{0.545310674630}{0.673228936366}{0.538690327416}{0.669891953167}
  \meshline{168,0,57}{0.500066701873}{0.650041199219}{0.482092676098}{0.640811194531}
  \meshline{168,0,57}{0.568961399050}{0.685312005757}{0.545310674630}{0.673228936366}
  \meshline{168,0,57}{0.528525610630}{0.664670176011}{0.538690327416}{0.669891953167}
  \meshline{168,0,57}{0.041021047285}{0.480696038470}{0.075489092094}{0.484009506038}
  \meshline{168,0,57}{0.030785833294}{0.480123202741}{0.037341860257}{0.480312720618}
\end{pgfscope}


==> nodal_square_D.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{144,144,144}{0.925571962335}{0.453091383247}{0.928825885053}{0.440357329164}
  \meshline{144,144,144}{0.616695807393}{0.535101723547}{0.626088324177}{0.541284489983}
  \meshline{144,144,144}{0.471688394588}{0.496003325493}{0.462909307697}{0.487386760633}
  \meshline{144,144,144}{0.643202984668}{0.056914827033}{0.631982790296}{0.058071878072}
  \meshline{144,144,144}{0.719775882819}{0.107767781746}{0.734564423544}{0.110096604370}
  \meshline{144,144,144}{0.484618805112}{0.508731529738}{0.491205215629}{0.515358584414}
  \meshline{144,144,144}{0.873709995050}{0.212074250719}{0.869468943920}{0.202868538120}
  \meshline{144,144,144}{0.059174493475}{0.621250324147}{0.059978930628}{0.616184894506}
  \meshline{144,144,144}{0.678271158655}{0.771591851056}{0.679146350677}{0.776538422873}
  \meshline{144,144,144}{0.735579956736}{0.110240788612}{0.739156536326}{0.111046832349}
  \meshline{144,144,144}{0.979144322661}{0.375560264443}{0.978097617909}{0.397697877662}
  \meshline{144,144,144}{0.891193947593}{0.272886674210}{0.892287034765}{0.283703778189}
  \meshline{144,144,144}{0.972094073313}{0.465405926687}{0.974881525651}{0.443631525651}
  \meshline{144,144,144}{0.971865752876}{0.468750000000}{0.971661283378}{0.471661283378}
  \meshline{144,144,144}{0.972094073313}{0.465405926687}{0.971865752876}{0.468750000000}
  \meshline{144,144,144}{0.769930310578}{0.508219506262}{0.785432940674}{0.503421594962}
  \meshline{144,144,144}{0.968818483762}{0.489607029528}{0.971661283378}{0.471661283378}
  \meshline{144,144,144}{0.953387178480}{0.561246541591}{0.957106998845}{0.548560149897}
  \meshline{144,144,144}{0.898074905662}{0.514553172220}{0.894608682378}{0.519471176553}
  \meshline{144,144,144}{0.925571962335}{0.453091383247}{0.921143904762}{0.466501947540}
  \meshline{144,144,144}{0.965956496756}{0.507321931776}{0.968173368951}{0.496405933910}
  \meshline{144,144,144}{0.916843187971}{0.476256511113}{0.919309171161}{0.470984606625}
  \meshline{144,144,144}{0.906686955307}{0.498832370084}{0.916843187971}{0.476256511113}
  \meshline{144,144,144}{0.958010550327}{0.543904465991}{0.959161218027}{0.537714128746}
  \meshline{144,144,144}{0.968173368951}{0.496405933910}{0.968818483762}{0.489607029528}
  \meshline{144,144,144}{0.959161218027}{0.537714128746}{0.965092256598}{0.514117292823}
  \meshline{144,144,144}{0.965956496756}{0.507321931776}{0.965092256598}{0.514117292823}
  \meshline{144,144,144}{0.958010550327}{0.543904465991}{0.957106998845}{0.548560149897}
  \meshline{144,144,144}{0.873784561254}{0.545995020781}{0.883841583096}{0.534024724506}
  \meshline{144,144,144}{0.854711968157}{0.447918993747}{0.843083194119}{0.462609046499}
  \meshline{144,144,144}{0.933195483975}{0.610457728478}{0.935280910293}{0.606257740991}
  \meshline{144,144,144}{0.948940616928}{0.573433396562}{0.947499174427}{0.579114062097}
  \meshline{144,144,144}{0.942404068025}{0.591194770172}{0.941664743128}{0.592444276231}
  \meshline{144,144,144}{0.948940616928}{0.573433396562}{0.953387178480}{0.561246541591}
  \meshline{144,144,144}{0.935280910293}{0.606257740991}{0.938621375115}{0.598663893836}
  \meshline{144,144,144}{0.752841584875}{0.590535883445}{0.748960024735}{0.590297682192}
  \meshline{144,144,144}{0.943902446747}{0.587406486009}{0.947499174427}{0.579114062097}
  \meshline{144,144,144}{0.942404068025}{0.591194770172}{0.943902446747}{0.587406486009}
  \meshline{144,144,144}{0.886755899623}{0.664683072743}{0.896252045569}{0.656708859407}
  \meshline{144,144,144}{0.914954065304}{0.638548930930}{0.904378579269}{0.649325598408}
  \meshline{144,144,144}{0.941664743128}{0.592444276231}{0.938621375115}{0.598663893836}
  \meshline{144,144,144}{0.883841583096}{0.534024724506}{0.884368677338}{0.533438845800}
  \meshline{144,144,144}{0.859882262086}{0.558171935833}{0.873784561254}{0.545995020781}
  \meshline{144,144,144}{0.894608682378}{0.519471176553}{0.884368677338}{0.533438845800}
  \meshline{144,144,144}{0.808242270319}{0.492417396688}{0.813416490702}{0.488924854183}
  \meshline{144,144,144}{0.906402500607}{0.499388715994}{0.906686955307}{0.498832370084}
  \meshline{144,144,144}{0.857174383641}{0.443653471183}{0.854711968157}{0.447918993747}
  \meshline{144,144,144}{0.926166641566}{0.622603118551}{0.920762603562}{0.629908434616}
  \meshline{144,144,144}{0.840583727343}{0.571828894368}{0.857489918508}{0.560252274153}
  \meshline{144,144,144}{0.823260730260}{0.481024355247}{0.829065841896}{0.476964851470}
  \meshline{144,144,144}{0.906402500607}{0.499388715994}{0.906227932404}{0.499661908732}
  \meshline{144,144,144}{0.919309171161}{0.470984606625}{0.921143904762}{0.466501947540}
  \meshline{144,144,144}{0.898074905662}{0.514553172220}{0.906227932404}{0.499661908732}
  \meshline{144,144,144}{0.813416490702}{0.488924854183}{0.823260730260}{0.481024355247}
  \meshline{144,144,144}{0.842870748026}{0.462897452749}{0.843083194119}{0.462609046499}
  \meshline{144,144,144}{0.857174383641}{0.443653471183}{0.864062791931}{0.432897145121}
  \meshline{144,144,144}{0.938235556369}{0.398258920594}{0.935769888113}{0.411113432843}
  \meshline{144,144,144}{0.873124922464}{0.415049718507}{0.875030600952}{0.410853739161}
  \meshline{144,144,144}{0.883151885570}{0.387712495687}{0.886021503871}{0.376858258048}
  \meshline{144,144,144}{0.938713703300}{0.393952909620}{0.941207956048}{0.376186172307}
  \meshline{144,144,144}{0.928825885053}{0.440357329164}{0.931075659948}{0.433510827554}
  \meshline{144,144,144}{0.889920390783}{0.358054721707}{0.889368645530}{0.360623258678}
  \meshline{144,144,144}{0.890105933739}{0.356685097189}{0.889920390783}{0.358054721707}
  \meshline{144,144,144}{0.831670544970}{0.474834193628}{0.842317699666}{0.463471249057}
  \meshline{144,144,144}{0.842870748026}{0.462897452749}{0.842317699666}{0.463471249057}
  \meshline{144,144,144}{0.941693744322}{0.370098881491}{0.941207956048}{0.376186172307}
  \meshline{144,144,144}{0.934272746312}{0.418324565829}{0.931075659948}{0.433510827554}
  \meshline{144,144,144}{0.934791522259}{0.416422953149}{0.934272746312}{0.418324565829}
  \meshline{144,144,144}{0.934791522259}{0.416422953149}{0.935769888113}{0.411113432843}
  \meshline{144,144,144}{0.977903228520}{0.400181507604}{0.978040863873}{0.398262457722}
  \meshline{144,144,144}{0.975437343373}{0.434349102600}{0.974881525651}{0.443631525651}
  \meshline{144,144,144}{0.831959282436}{0.576507850261}{0.840583727343}{0.571828894368}
  \meshline{144,144,144}{0.858605937682}{0.559411040997}{0.857489918508}{0.560252274153}
  \meshline{144,144,144}{0.810692366629}{0.584707997903}{0.813073885980}{0.583783366855}
  \meshline{144,144,144}{0.859882262086}{0.558171935833}{0.858605937682}{0.559411040997}
  \meshline{144,144,144}{0.813073885980}{0.583783366855}{0.831959282436}{0.576507850261}
  \meshline{144,144,144}{0.766964446735}{0.447107571014}{0.744006756462}{0.454681428518}
  \meshline{144,144,144}{0.768236512617}{0.446689594565}{0.766964446735}{0.447107571014}
  \meshline{144,144,144}{0.933195483975}{0.610457728478}{0.926166641566}{0.622603118551}
  \meshline{144,144,144}{0.904378579269}{0.649325598408}{0.901399209118}{0.652809367280}
  \meshline{144,144,144}{0.920762603562}{0.629908434616}{0.914954065304}{0.638548930930}
  \meshline{144,144,144}{0.869713701069}{0.673838108860}{0.868911473974}{0.674113014595}
  \meshline{144,144,144}{0.784989857120}{0.681646769559}{0.800148705273}{0.683909546073}
  \meshline{144,144,144}{0.771749727290}{0.591100357656}{0.783096673858}{0.590634181986}
  \meshline{144,144,144}{0.870520754475}{0.673331762747}{0.869713701069}{0.673838108860}
  \meshline{144,144,144}{0.870520754475}{0.673331762747}{0.886755899623}{0.664683072743}
  \meshline{144,144,144}{0.896252045569}{0.656708859407}{0.901399209118}{0.652809367280}
  \meshline{144,144,144}{0.809337371495}{0.684943117697}{0.824427405773}{0.684756739700}
  \meshline{144,144,144}{0.868911473974}{0.674113014595}{0.851710954806}{0.680735501699}
  \meshline{144,144,144}{0.851710954806}{0.680735501699}{0.836754905676}{0.682904886905}
  \meshline{144,144,144}{0.827771181218}{0.684771410649}{0.824427405773}{0.684756739700}
  \meshline{144,144,144}{0.827771181218}{0.684771410649}{0.829851809857}{0.684383451915}
  \meshline{144,144,144}{0.829851809857}{0.684383451915}{0.836754905676}{0.682904886905}
  \meshline{144,144,144}{0.864062791931}{0.432897145121}{0.870371977081}{0.419942617560}
  \meshline{144,144,144}{0.944673043606}{0.319659326470}{0.944464559839}{0.295852072234}
  \meshline{144,144,144}{0.796568360159}{0.498249250697}{0.808242270319}{0.492417396688}
  \meshline{144,144,144}{0.796568360159}{0.498249250697}{0.790525633547}{0.501472468158}
  \meshline{144,144,144}{0.785432940674}{0.503421594962}{0.790525633547}{0.501472468158}
  \meshline{144,144,144}{0.769930310578}{0.508219506262}{0.767029631280}{0.508800950388}
  \meshline{144,144,144}{0.777894490596}{0.441403790004}{0.783274541928}{0.438473807809}
  \meshline{144,144,144}{0.783274541928}{0.438473807809}{0.783962751434}{0.438084628678}
  \meshline{144,144,144}{0.829065841896}{0.476964851470}{0.831670544970}{0.474834193628}
  \meshline{144,144,144}{0.752242133020}{0.511802466788}{0.740078643639}{0.512395054110}
  \meshline{144,144,144}{0.769029300703}{0.446327777490}{0.768236512617}{0.446689594565}
  \meshline{144,144,144}{0.718516876415}{0.408074451182}{0.736166193548}{0.404765773128}
  \meshline{144,144,144}{0.797682125833}{0.427876536069}{0.803501906355}{0.422103592315}
  \meshline{144,144,144}{0.817320149075}{0.406119624996}{0.812133067863}{0.413315546192}
  \meshline{144,144,144}{0.880894503736}{0.394714166751}{0.883151885570}{0.387712495687}
  \meshline{144,144,144}{0.870371977081}{0.419942617560}{0.873124922464}{0.415049718507}
  \meshline{144,144,144}{0.785582793145}{0.436819806788}{0.783962751434}{0.438084628678}
  \meshline{144,144,144}{0.797682125833}{0.427876536069}{0.785582793145}{0.436819806788}
  \meshline{144,144,144}{0.777894490596}{0.441403790004}{0.769029300703}{0.446327777490}
  \meshline{144,144,144}{0.875030600952}{0.410853739161}{0.880894503736}{0.394714166751}
  \meshline{144,144,144}{0.802354162697}{0.303282558084}{0.800094800148}{0.283382059769}
  \meshline{144,144,144}{0.831820108592}{0.382311859372}{0.834921221654}{0.374946037358}
  \meshline{144,144,144}{0.803501906355}{0.422103592315}{0.812133067863}{0.413315546192}
  \meshline{144,144,144}{0.826611192213}{0.391616630261}{0.823022747214}{0.397987927350}
  \meshline{144,144,144}{0.766555254972}{0.388285528579}{0.768087495711}{0.386698032558}
  \meshline{144,144,144}{0.826611192213}{0.391616630261}{0.831820108592}{0.382311859372}
  \meshline{144,144,144}{0.840199168950}{0.360284431581}{0.836724261939}{0.370210426996}
  \meshline{144,144,144}{0.843704218501}{0.345582209163}{0.840199168950}{0.360284431581}
  \meshline{144,144,144}{0.781601977062}{0.372047473088}{0.779729278851}{0.374786695697}
  \meshline{144,144,144}{0.817320149075}{0.406119624996}{0.823022747214}{0.397987927350}
  \meshline{144,144,144}{0.836724261939}{0.370210426996}{0.834921221654}{0.374946037358}
  \meshline{144,144,144}{0.724843507023}{0.457212351888}{0.723291174107}{0.457334282968}
  \meshline{144,144,144}{0.794245163506}{0.350284415902}{0.792161955497}{0.354332350850}
  \meshline{144,144,144}{0.892598382488}{0.335942724891}{0.893604482961}{0.322097168809}
  \meshline{144,144,144}{0.886021503871}{0.376858258048}{0.889368645530}{0.360623258678}
  \meshline{144,144,144}{0.890105933739}{0.356685097189}{0.892268615965}{0.340840545134}
  \meshline{144,144,144}{0.886611795237}{0.248959573669}{0.888132953408}{0.256017509977}
  \meshline{144,144,144}{0.938713703300}{0.393952909620}{0.938235556369}{0.398258920594}
  \meshline{144,144,144}{0.943397949870}{0.274124011300}{0.943605022319}{0.276567611649}
  \meshline{144,144,144}{0.892268615965}{0.340840545134}{0.892598382488}{0.335942724891}
  \meshline{144,144,144}{0.941693744322}{0.370098881491}{0.943217426221}{0.355323641318}
  \meshline{144,144,144}{0.556417557873}{0.486577057821}{0.560854541722}{0.490746497505}
  \meshline{144,144,144}{0.730438648926}{0.456427073291}{0.724843507023}{0.457212351888}
  \meshline{144,144,144}{0.847262784492}{0.301518478829}{0.847368855080}{0.305691984720}
  \meshline{144,144,144}{0.943858173933}{0.344447200247}{0.944564986118}{0.327816045745}
  \meshline{144,144,144}{0.734497836728}{0.512885414102}{0.740078643639}{0.512395054110}
  \meshline{144,144,144}{0.767029631280}{0.508800950388}{0.752242133020}{0.511802466788}
  \meshline{144,144,144}{0.730438648926}{0.456427073291}{0.744006756462}{0.454681428518}
  \meshline{144,144,144}{0.687971703326}{0.406558582868}{0.702175721256}{0.408620041720}
  \meshline{144,144,144}{0.718516876415}{0.408074451182}{0.716391015927}{0.408271989963}
  \meshline{144,144,144}{0.844353337112}{0.342955686934}{0.844650520062}{0.341054888812}
  \meshline{144,144,144}{0.943858173933}{0.344447200247}{0.943217426221}{0.355323641318}
  \meshline{144,144,144}{0.980375281515}{0.310764968097}{0.980375281515}{0.310084583630}
  \meshline{144,144,144}{0.979233174946}{0.374023129242}{0.979144322661}{0.375560264443}
  \meshline{144,144,144}{0.944690035878}{0.323093911654}{0.944564986118}{0.327816045745}
  \meshline{144,144,144}{0.944673043606}{0.319659326470}{0.944690035878}{0.323093911654}
  \meshline{144,144,144}{0.944052268848}{0.287089928231}{0.943605022319}{0.276567611649}
  \meshline{144,144,144}{0.978040863873}{0.398262457722}{0.978097617909}{0.397697877662}
  \meshline{144,144,144}{0.976860808248}{0.415766247428}{0.977903228520}{0.400181507604}
  \meshline{144,144,144}{0.975437343373}{0.434349102600}{0.976650090745}{0.421891519056}
  \meshline{144,144,144}{0.976860808248}{0.415766247428}{0.976650090745}{0.421891519056}
  \meshline{144,144,144}{0.893386566342}{0.297125214753}{0.893360426995}{0.307365586254}
  \meshline{144,144,144}{0.893360426995}{0.307365586254}{0.893604482961}{0.322097168809}
  \meshline{144,144,144}{0.707256368561}{0.408736815172}{0.702175721256}{0.408620041720}
  \meshline{144,144,144}{0.766555254972}{0.388285528579}{0.764449456147}{0.389819376233}
  \meshline{144,144,144}{0.980375281515}{0.309404199162}{0.980244091582}{0.292668598297}
  \meshline{144,144,144}{0.892287034765}{0.283703778189}{0.893160144273}{0.291092919546}
  \meshline{144,144,144}{0.736166193548}{0.404765773128}{0.744923263263}{0.401353257565}
  \meshline{144,144,144}{0.753859309530}{0.397007450399}{0.744923263263}{0.401353257565}
  \meshline{144,144,144}{0.764449456147}{0.389819376233}{0.753859309530}{0.397007450399}
  \meshline{144,144,144}{0.768087495711}{0.386698032558}{0.779729278851}{0.374786695697}
  \meshline{144,144,144}{0.884074510329}{0.239631171070}{0.879717079237}{0.227513361710}
  \meshline{144,144,144}{0.893160144273}{0.291092919546}{0.893343224181}{0.294067004354}
  \meshline{144,144,144}{0.893386566342}{0.297125214753}{0.893343224181}{0.294067004354}
  \meshline{144,144,144}{0.844546583392}{0.278488301930}{0.841546831119}{0.263596654459}
  \meshline{144,144,144}{0.846970141336}{0.322654534046}{0.847034568913}{0.316442843201}
  \meshline{144,144,144}{0.847368855080}{0.305691984720}{0.847034568913}{0.316442843201}
  \meshline{144,144,144}{0.844353337112}{0.342955686934}{0.843704218501}{0.345582209163}
  \meshline{144,144,144}{0.891193947593}{0.272886674210}{0.890482643903}{0.269081534122}
  \meshline{144,144,144}{0.829504119124}{0.233031379505}{0.822465769012}{0.221302954813}
  \meshline{144,144,144}{0.845643741219}{0.283672884594}{0.844546583392}{0.278488301930}
  \meshline{144,144,144}{0.846212060493}{0.290703443433}{0.845643741219}{0.283672884594}
  \meshline{144,144,144}{0.829504119124}{0.233031379505}{0.835052140590}{0.245553485225}
  \meshline{144,144,144}{0.846212060493}{0.290703443433}{0.847262784492}{0.301518478829}
  \meshline{144,144,144}{0.844650520062}{0.341054888812}{0.846970141336}{0.322654534046}
  \meshline{144,144,144}{0.774507126978}{0.233641110461}{0.781540612180}{0.241644454406}
  \meshline{144,144,144}{0.838344977740}{0.253749658991}{0.841546831119}{0.263596654459}
  \meshline{144,144,144}{0.877556631679}{0.220633995456}{0.876306362031}{0.217273975608}
  \meshline{144,144,144}{0.791425645430}{0.259623843249}{0.794936640082}{0.266200445420}
  \meshline{144,144,144}{0.795631821374}{0.268173558816}{0.799323532670}{0.280460932859}
  \meshline{144,144,144}{0.795631821374}{0.268173558816}{0.794936640082}{0.266200445420}
  \meshline{144,144,144}{0.800094800148}{0.283382059769}{0.799984028910}{0.282696850949}
  \meshline{144,144,144}{0.800787939048}{0.328237063862}{0.800257770571}{0.331086022029}
  \meshline{144,144,144}{0.799984028910}{0.282696850949}{0.799323532670}{0.280460932859}
  \meshline{144,144,144}{0.791425645430}{0.259623843249}{0.784332308316}{0.246194500146}
  \meshline{144,144,144}{0.801119655168}{0.323792420411}{0.802354162697}{0.303282558084}
  \meshline{144,144,144}{0.979749339644}{0.271827221729}{0.979873354600}{0.275427257569}
  \meshline{144,144,144}{0.980375281515}{0.309404199162}{0.980375281515}{0.310084583630}
  \meshline{144,144,144}{0.888132953408}{0.256017509977}{0.890482643903}{0.269081534122}
  \meshline{144,144,144}{0.939084780447}{0.235071182366}{0.941136650965}{0.250908332045}
  \meshline{144,144,144}{0.879717079237}{0.227513361710}{0.877556631679}{0.220633995456}
  \meshline{144,144,144}{0.873709995050}{0.212074250719}{0.876306362031}{0.217273975608}
  \meshline{144,144,144}{0.884074510329}{0.239631171070}{0.886611795237}{0.248959573669}
  \meshline{144,144,144}{0.838344977740}{0.253749658991}{0.835052140590}{0.245553485225}
  \meshline{144,144,144}{0.818255563843}{0.214306976486}{0.822465769012}{0.221302954813}
  \meshline{144,144,144}{0.944052268848}{0.287089928231}{0.944464559839}{0.295852072234}
  \meshline{144,144,144}{0.979131665852}{0.252922764362}{0.979274473019}{0.254842757038}
  \meshline{144,144,144}{0.980244091582}{0.287934345880}{0.979873354600}{0.275427257569}
  \meshline{144,144,144}{0.980260828997}{0.333611286897}{0.980260828997}{0.335178485210}
  \meshline{144,144,144}{0.980244091582}{0.287934345880}{0.980244091582}{0.292668598297}
  \meshline{144,144,144}{0.980165034291}{0.339970953761}{0.980260828997}{0.335178485210}
  \meshline{144,144,144}{0.979868306461}{0.352749961931}{0.979233174946}{0.374023129242}
  \meshline{144,144,144}{0.980375281515}{0.310764968097}{0.980260828997}{0.333611286897}
  \meshline{144,144,144}{0.979868306461}{0.352749961931}{0.980165034291}{0.339970953761}
  \meshline{144,144,144}{0.859988139683}{0.186712829042}{0.865636427600}{0.196710644701}
  \meshline{144,144,144}{0.826729187662}{0.149913263244}{0.814098610024}{0.140914609370}
  \meshline{144,144,144}{0.923841496716}{0.175575747932}{0.919730020668}{0.166624829257}
  \meshline{144,144,144}{0.834770737116}{0.156988344748}{0.826729187662}{0.149913263244}
  \meshline{144,144,144}{0.851865129871}{0.175656933050}{0.856730441060}{0.181522922134}
  \meshline{144,144,144}{0.865636427600}{0.196710644701}{0.869468943920}{0.202868538120}
  \meshline{144,144,144}{0.781540612180}{0.241644454406}{0.784332308316}{0.246194500146}
  \meshline{144,144,144}{0.859988139683}{0.186712829042}{0.856730441060}{0.181522922134}
  \meshline{144,144,144}{0.917313085764}{0.160354667220}{0.913196327768}{0.152874528235}
  \meshline{144,144,144}{0.917313085764}{0.160354667220}{0.919730020668}{0.166624829257}
  \meshline{144,144,144}{0.928496430085}{0.189863385107}{0.926778536871}{0.185255029357}
  \meshline{144,144,144}{0.903674975765}{0.136834348994}{0.899903087794}{0.132035728608}
  \meshline{144,144,144}{0.934824000977}{0.213385502787}{0.933361962940}{0.207452395295}
  \meshline{144,144,144}{0.937389958132}{0.226713661149}{0.934824000977}{0.213385502787}
  \meshline{144,144,144}{0.943397949870}{0.274124011300}{0.941392118380}{0.252768471239}
  \meshline{144,144,144}{0.941392118380}{0.252768471239}{0.941136650965}{0.250908332045}
  \meshline{144,144,144}{0.814098610024}{0.140914609370}{0.809048035463}{0.137216630680}
  \meshline{144,144,144}{0.794570730137}{0.129248306654}{0.784895272581}{0.124480095122}
  \meshline{144,144,144}{0.767476288323}{0.170555019578}{0.759434046462}{0.166823251056}
  \meshline{144,144,144}{0.809048035463}{0.137216630680}{0.802287747365}{0.133486107695}
  \meshline{144,144,144}{0.852280442163}{0.089613682658}{0.853843442169}{0.090354311538}
  \meshline{144,144,144}{0.834770737116}{0.156988344748}{0.843556326647}{0.165855920596}
  \meshline{144,144,144}{0.851865129871}{0.175656933050}{0.843556326647}{0.165855920596}
  \meshline{144,144,144}{0.767819308120}{0.227517448716}{0.757485246331}{0.218036796423}
  \meshline{144,144,144}{0.782659402740}{0.180054998307}{0.786819197503}{0.182631217598}
  \meshline{144,144,144}{0.810376560739}{0.204638561591}{0.818255563843}{0.214306976486}
  \meshline{144,144,144}{0.803809890892}{0.197416732717}{0.789715305790}{0.185014609880}
  \meshline{144,144,144}{0.789715305790}{0.185014609880}{0.786819197503}{0.182631217598}
  \meshline{144,144,144}{0.854372587350}{0.090700880851}{0.853997653317}{0.090437377797}
  \meshline{144,144,144}{0.767359651075}{0.118192215262}{0.784895272581}{0.124480095122}
  \meshline{144,144,144}{0.772182469216}{0.173162650469}{0.782659402740}{0.180054998307}
  \meshline{144,144,144}{0.802287747365}{0.133486107695}{0.797299470834}{0.130500781467}
  \meshline{144,144,144}{0.831487857694}{0.028023300198}{0.837268756065}{0.029239410153}
  \meshline{144,144,144}{0.797299470834}{0.130500781467}{0.794570730137}{0.129248306654}
  \meshline{144,144,144}{0.804335358664}{0.069843808563}{0.786616107580}{0.065065595274}
  \meshline{144,144,144}{0.822688996999}{0.026876378467}{0.831487857694}{0.028023300198}
  \meshline{144,144,144}{0.852280442163}{0.089613682658}{0.829922393380}{0.078611285610}
  \meshline{144,144,144}{0.973956137334}{0.181938056953}{0.971801090589}{0.168394346408}
  \meshline{144,144,144}{0.968832182223}{0.150576928809}{0.969683648818}{0.153291203576}
  \meshline{144,144,144}{0.933361962940}{0.207452395295}{0.928496430085}{0.189863385107}
  \meshline{144,144,144}{0.939084780447}{0.235071182366}{0.937389958132}{0.226713661149}
  \meshline{144,144,144}{0.973956137334}{0.185679310089}{0.974540538065}{0.192474236709}
  \meshline{144,144,144}{0.977796134870}{0.226721555558}{0.977332061301}{0.219854312015}
  \meshline{144,144,144}{0.974540538065}{0.192474236709}{0.975978643850}{0.202434641085}
  \meshline{144,144,144}{0.978339118734}{0.235988180249}{0.978816133749}{0.247468835530}
  \meshline{144,144,144}{0.923841496716}{0.175575747932}{0.926778536871}{0.185255029357}
  \meshline{144,144,144}{0.962654847524}{0.123749218028}{0.957959543738}{0.112287402273}
  \meshline{144,144,144}{0.967443480518}{0.145819300037}{0.962654847524}{0.123749218028}
  \meshline{144,144,144}{0.968832182223}{0.150576928809}{0.967443480518}{0.145819300037}
  \meshline{144,144,144}{0.973956137334}{0.185679310089}{0.973956137334}{0.181938056953}
  \meshline{144,144,144}{0.979131665852}{0.252922764362}{0.978816133749}{0.247468835530}
  \meshline{144,144,144}{0.977332061301}{0.219854312015}{0.976898330345}{0.216416227103}
  \meshline{144,144,144}{0.969683648818}{0.153291203576}{0.970303649039}{0.157397675197}
  \meshline{144,144,144}{0.810376560739}{0.204638561591}{0.803809890892}{0.197416732717}
  \meshline{144,144,144}{0.727688841454}{0.203262252048}{0.717805495428}{0.200238034702}
  \meshline{144,144,144}{0.751902358172}{0.163438753687}{0.740305257733}{0.159728328091}
  \meshline{144,144,144}{0.767476288323}{0.170555019578}{0.772182469216}{0.173162650469}
  \meshline{144,144,144}{0.727688841454}{0.203262252048}{0.735220064822}{0.205663713756}
  \meshline{144,144,144}{0.763265269836}{0.116715810637}{0.767359651075}{0.118192215262}
  \meshline{144,144,144}{0.767819308120}{0.227517448716}{0.774507126978}{0.233641110461}
  \meshline{144,144,144}{0.753804140366}{0.215742970511}{0.757485246331}{0.218036796423}
  \meshline{144,144,144}{0.722183233440}{0.155315288276}{0.730852113854}{0.157364670509}
  \meshline{144,144,144}{0.751902358172}{0.163438753687}{0.759434046462}{0.166823251056}
  \meshline{144,144,144}{0.734564423544}{0.110096604370}{0.735579956736}{0.110240788612}
  \meshline{144,144,144}{0.740499442784}{0.020689244164}{0.754436832734}{0.021263836054}
  \meshline{144,144,144}{0.712276626864}{0.019823096161}{0.723450033174}{0.020102811633}
  \meshline{144,144,144}{0.667937938802}{0.154169630867}{0.676216563667}{0.152970092098}
  \meshline{144,144,144}{0.763265269836}{0.116715810637}{0.758344730645}{0.115480212982}
  \meshline{144,144,144}{0.685156611382}{0.106142598590}{0.683094485691}{0.106232080240}
  \meshline{144,144,144}{0.709580755196}{0.106984231635}{0.719775882819}{0.107767781746}
  \meshline{144,144,144}{0.739156536326}{0.111046832349}{0.747764529959}{0.112801719228}
  \meshline{144,144,144}{0.804335358664}{0.069843808563}{0.805158230523}{0.070023434440}
  \meshline{144,144,144}{0.758344730645}{0.115480212982}{0.750406088352}{0.113244397411}
  \meshline{144,144,144}{0.826141904577}{0.077178675559}{0.805698729617}{0.070153512653}
  \meshline{144,144,144}{0.975978643850}{0.202434641085}{0.976898330345}{0.216416227103}
  \meshline{144,144,144}{0.977796134870}{0.226721555558}{0.978339118734}{0.235988180249}
  \meshline{144,144,144}{0.979274473019}{0.254842757038}{0.979749339644}{0.271827221729}
  \meshline{144,144,144}{0.704294916515}{0.198019076560}{0.712364562306}{0.199260918543}
  \meshline{144,144,144}{0.738425370232}{0.207002539550}{0.735220064822}{0.205663713756}
  \meshline{144,144,144}{0.694348807677}{0.197816622395}{0.684394249464}{0.197520094607}
  \meshline{144,144,144}{0.738425370232}{0.207002539550}{0.753804140366}{0.215742970511}
  \meshline{144,144,144}{0.704294916515}{0.198019076560}{0.694348807677}{0.197816622395}
  \meshline{144,144,144}{0.717805495428}{0.200238034702}{0.712364562306}{0.199260918543}
  \meshline{144,144,144}{0.682678986056}{0.152809390724}{0.678487070270}{0.152760352160}
  \meshline{144,144,144}{0.718095494544}{0.154758043759}{0.706712783442}{0.153151689243}
  \meshline{144,144,144}{0.722183233440}{0.155315288276}{0.718095494544}{0.154758043759}
  \meshline{144,144,144}{0.740305257733}{0.159728328091}{0.737326720088}{0.158817037629}
  \meshline{144,144,144}{0.737326720088}{0.158817037629}{0.730852113854}{0.157364670509}
  \meshline{144,144,144}{0.716391015927}{0.408271989963}{0.707256368561}{0.408736815172}
  \meshline{144,144,144}{0.612210200876}{0.354730254348}{0.606555061001}{0.345987038966}
  \meshline{144,144,144}{0.594354317062}{0.267503005289}{0.599363335778}{0.253741326407}
  \meshline{144,144,144}{0.591231791863}{0.292950430523}{0.593262008402}{0.311299669019}
  \meshline{144,144,144}{0.591279439139}{0.288059608335}{0.591231791863}{0.292950430523}
  \meshline{144,144,144}{0.601897603269}{0.248309856738}{0.599363335778}{0.253741326407}
  \meshline{144,144,144}{0.660848559553}{0.202197619331}{0.642531318076}{0.209211649992}
  \meshline{144,144,144}{0.617636870384}{0.059576677908}{0.631982790296}{0.058071878072}
  \meshline{144,144,144}{0.631276425705}{0.162717190320}{0.609651124670}{0.172378548213}
  \meshline{144,144,144}{0.684394249464}{0.197520094607}{0.676731759647}{0.198424262291}
  \meshline{144,144,144}{0.667026844428}{0.200167145009}{0.676731759647}{0.198424262291}
  \meshline{144,144,144}{0.903674975765}{0.136834348994}{0.909342004023}{0.144873021932}
  \meshline{144,144,144}{0.909342004023}{0.144873021932}{0.913196327768}{0.152874528235}
  \meshline{144,144,144}{0.794245163506}{0.350284415902}{0.798826236382}{0.335614011612}
  \meshline{144,144,144}{0.792161955497}{0.354332350850}{0.786504184715}{0.365034743463}
  \meshline{144,144,144}{0.786504184715}{0.365034743463}{0.781601977062}{0.372047473088}
  \meshline{144,144,144}{0.609651124670}{0.172378548213}{0.609602664450}{0.172402790174}
  \meshline{144,144,144}{0.624884228034}{0.220493471695}{0.628359223044}{0.218098819434}
  \meshline{144,144,144}{0.612877598102}{0.232102819785}{0.612345983196}{0.232628082625}
  \meshline{144,144,144}{0.612345983196}{0.232628082625}{0.611742669589}{0.233530769282}
  \meshline{144,144,144}{0.612877598102}{0.232102819785}{0.624884228034}{0.220493471695}
  \meshline{144,144,144}{0.638235283623}{0.160651006360}{0.632518149761}{0.162270854925}
  \meshline{144,144,144}{0.707794249649}{0.106814891026}{0.709580755196}{0.106984231635}
  \meshline{144,144,144}{0.714590486437}{0.055949615444}{0.719058983527}{0.056115131358}
  \meshline{144,144,144}{0.747764529959}{0.112801719228}{0.750406088352}{0.113244397411}
  \meshline{144,144,144}{0.801119655168}{0.323792420411}{0.800787939048}{0.328237063862}
  \meshline{144,144,144}{0.798826236382}{0.335614011612}{0.800257770571}{0.331086022029}
  \meshline{144,144,144}{0.723291174107}{0.457334282968}{0.719568685609}{0.457070116945}
  \meshline{144,144,144}{0.659457491955}{0.445254776522}{0.654614950546}{0.443233673698}
  \meshline{144,144,144}{0.623698896429}{0.369685366108}{0.615482996018}{0.359624124813}
  \meshline{144,144,144}{0.612210200876}{0.354730254348}{0.615482996018}{0.359624124813}
  \meshline{144,144,144}{0.560295495273}{0.218912303973}{0.556820481783}{0.224634881998}
  \meshline{144,144,144}{0.628359223044}{0.218098819434}{0.639798947076}{0.210553694562}
  \meshline{144,144,144}{0.609602664450}{0.172402790174}{0.609558369040}{0.172432603012}
  \meshline{144,144,144}{0.540818851156}{0.153865175188}{0.538481490369}{0.156123039379}
  \meshline{144,144,144}{0.678359520450}{0.055294856360}{0.693854052873}{0.055289827321}
  \meshline{144,144,144}{0.686577130951}{0.106178336637}{0.707794249649}{0.106814891026}
  \meshline{144,144,144}{0.682678986056}{0.152809390724}{0.698230622713}{0.152692439155}
  \meshline{144,144,144}{0.686577130951}{0.106178336637}{0.685156611382}{0.106142598590}
  \meshline{144,144,144}{0.660848559553}{0.202197619331}{0.667026844428}{0.200167145009}
  \meshline{144,144,144}{0.639798947076}{0.210553694562}{0.642531318076}{0.209211649992}
  \meshline{144,144,144}{0.719058983527}{0.056115131358}{0.744140811244}{0.058333286248}
  \meshline{144,144,144}{0.659609773593}{0.019761568222}{0.672580048107}{0.019694123941}
  \meshline{144,144,144}{0.654579741627}{0.108183264279}{0.641179657448}{0.110255819545}
  \meshline{144,144,144}{0.678359520450}{0.055294856360}{0.672234839579}{0.055526378311}
  \meshline{144,144,144}{0.645380725662}{0.020108056433}{0.659609773593}{0.019761568222}
  \meshline{144,144,144}{0.695225351859}{0.055281627265}{0.695603739887}{0.055290256424}
  \meshline{144,144,144}{0.659688540524}{0.055860760188}{0.672234839579}{0.055526378311}
  \meshline{144,144,144}{0.736037346265}{0.020408463554}{0.740499442784}{0.020689244164}
  \meshline{144,144,144}{0.759954671119}{0.060419734590}{0.745515262459}{0.058439894995}
  \meshline{144,144,144}{0.711102583393}{0.019823096161}{0.712276626864}{0.019823096161}
  \meshline{144,144,144}{0.702208800561}{0.019731504833}{0.692787909750}{0.019608834586}
  \meshline{144,144,144}{0.702208800561}{0.019731504833}{0.711102583393}{0.019823096161}
  \meshline{144,144,144}{0.672694930904}{0.402017709632}{0.665966897510}{0.399699998843}
  \meshline{144,144,144}{0.623698896429}{0.369685366108}{0.634923331792}{0.380255466348}
  \meshline{144,144,144}{0.581362975240}{0.385536283311}{0.586350692910}{0.391572883667}
  \meshline{144,144,144}{0.597020185869}{0.325103032358}{0.594293386257}{0.317112119328}
  \meshline{144,144,144}{0.601224926918}{0.335847796103}{0.597020185869}{0.325103032358}
  \meshline{144,144,144}{0.606555061001}{0.345987038966}{0.601224926918}{0.335847796103}
  \meshline{144,144,144}{0.611742669589}{0.233530769282}{0.601897603269}{0.248309856738}
  \meshline{144,144,144}{0.564102741018}{0.212495119999}{0.569100602983}{0.206643135793}
  \meshline{144,144,144}{0.564102741018}{0.212495119999}{0.560295495273}{0.218912303973}
  \meshline{144,144,144}{0.590284255803}{0.185388990049}{0.582482571865}{0.191612888674}
  \meshline{144,144,144}{0.590284255803}{0.185388990049}{0.595061540376}{0.181625717786}
  \meshline{144,144,144}{0.609558369040}{0.172432603012}{0.609217037237}{0.172654616019}
  \meshline{144,144,144}{0.632543920781}{0.111905649387}{0.625076116981}{0.113467681401}
  \meshline{144,144,144}{0.787421401540}{0.023374100234}{0.807419933683}{0.024941790733}
  \meshline{144,144,144}{0.812797157678}{0.025776140649}{0.809790690876}{0.025270513301}
  \meshline{144,144,144}{0.786616107580}{0.065065595274}{0.776539065896}{0.063337789917}
  \meshline{144,144,144}{0.765948304424}{0.061169940895}{0.776539065896}{0.063337789917}
  \meshline{144,144,144}{0.759954671119}{0.060419734590}{0.765948304424}{0.061169940895}
  \meshline{144,144,144}{0.809790690876}{0.025270513301}{0.807419933683}{0.024941790733}
  \meshline{144,144,144}{0.805158230523}{0.070023434440}{0.805698729617}{0.070153512653}
  \meshline{144,144,144}{0.787421401540}{0.023374100234}{0.782747768836}{0.022803049714}
  \meshline{144,144,144}{0.852893886425}{0.032317549005}{0.858767847236}{0.033315444287}
  \meshline{144,144,144}{0.744140811244}{0.058333286248}{0.745515262459}{0.058439894995}
  \meshline{144,144,144}{0.771133081166}{0.022194344823}{0.759125008128}{0.021263836054}
  \meshline{144,144,144}{0.771133081166}{0.022194344823}{0.782747768836}{0.022803049714}
  \meshline{144,144,144}{0.695225351859}{0.055281627265}{0.693854052873}{0.055289827321}
  \meshline{144,144,144}{0.754436832734}{0.021263836054}{0.759125008128}{0.021263836054}
  \meshline{144,144,144}{0.714590486437}{0.055949615444}{0.695603739887}{0.055290256424}
  \meshline{144,144,144}{0.676655487709}{0.019635129798}{0.672580048107}{0.019694123941}
  \meshline{144,144,144}{0.634923331792}{0.380255466348}{0.636369830074}{0.381394129894}
  \meshline{144,144,144}{0.624967708463}{0.479454126311}{0.613323382833}{0.471669471601}
  \meshline{144,144,144}{0.615683706100}{0.419615816886}{0.622089059956}{0.424396167858}
  \meshline{144,144,144}{0.597564900838}{0.403533682095}{0.597953617909}{0.403870743741}
  \meshline{144,144,144}{0.615683706100}{0.419615816886}{0.611054605733}{0.415579094445}
  \meshline{144,144,144}{0.597564900838}{0.403533682095}{0.597332118097}{0.403302520346}
  \meshline{144,144,144}{0.566289082407}{0.363157295596}{0.572291186344}{0.372961047599}
  \meshline{144,144,144}{0.597332118097}{0.403302520346}{0.586350692910}{0.391572883667}
  \meshline{144,144,144}{0.594293386257}{0.317112119328}{0.593262008402}{0.311299669019}
  \meshline{144,144,144}{0.544106893580}{0.301332222828}{0.542671162554}{0.289630505285}
  \meshline{144,144,144}{0.593069476736}{0.272922341157}{0.591279439139}{0.288059608335}
  \meshline{144,144,144}{0.543500076374}{0.269461764363}{0.545545985663}{0.255430776888}
  \meshline{144,144,144}{0.593069476736}{0.272922341157}{0.594354317062}{0.267503005289}
  \meshline{144,144,144}{0.544106893580}{0.301332222828}{0.544850213324}{0.307561776490}
  \meshline{144,144,144}{0.543500076374}{0.269461764363}{0.542941207557}{0.272874265699}
  \meshline{144,144,144}{0.548030137981}{0.321314719707}{0.549927665636}{0.328164926359}
  \meshline{144,144,144}{0.542941207557}{0.272874265699}{0.542821331496}{0.276652492292}
  \meshline{144,144,144}{0.545545985663}{0.255430776888}{0.549239608274}{0.243204313884}
  \meshline{144,144,144}{0.550317520644}{0.239313448740}{0.550854707661}{0.237936830146}
  \meshline{144,144,144}{0.491444485092}{0.230799302307}{0.491552100721}{0.230208391506}
  \meshline{144,144,144}{0.569100602983}{0.206643135793}{0.582482571865}{0.191612888674}
  \meshline{144,144,144}{0.519660226662}{0.174744830517}{0.512587245124}{0.184706840725}
  \meshline{144,144,144}{0.556820481783}{0.224634881998}{0.550854707661}{0.237936830146}
  \meshline{144,144,144}{0.548679785987}{0.026030864469}{0.547808725766}{0.026175590328}
  \meshline{144,144,144}{0.528782654047}{0.164649426380}{0.523424601005}{0.170446738019}
  \meshline{144,144,144}{0.549239608274}{0.243204313884}{0.550317520644}{0.239313448740}
  \meshline{144,144,144}{0.434980459110}{0.461135095705}{0.442356085051}{0.467931138018}
  \meshline{144,144,144}{0.510602777897}{0.356588455346}{0.499526456513}{0.331577940129}
  \meshline{144,144,144}{0.409328505196}{0.236562402706}{0.409078379197}{0.239841896300}
  \meshline{144,144,144}{0.487576761110}{0.278474500692}{0.487982043268}{0.284764643744}
  \meshline{144,144,144}{0.487282783926}{0.262024846951}{0.487315873339}{0.261483568650}
  \meshline{144,144,144}{0.632518149761}{0.162270854925}{0.631276425705}{0.162717190320}
  \meshline{144,144,144}{0.656463810049}{0.155664499053}{0.667937938802}{0.154169630867}
  \meshline{144,144,144}{0.678487070270}{0.152760352160}{0.676216563667}{0.152970092098}
  \meshline{144,144,144}{0.652283106151}{0.156482617444}{0.638235283623}{0.160651006360}
  \meshline{144,144,144}{0.698230622713}{0.152692439155}{0.706712783442}{0.153151689243}
  \meshline{144,144,144}{0.652283106151}{0.156482617444}{0.656463810049}{0.155664499053}
  \meshline{144,144,144}{0.647625413372}{0.056680539025}{0.659688540524}{0.055860760188}
  \meshline{144,144,144}{0.625076116981}{0.113467681401}{0.616083673301}{0.116135751791}
  \meshline{144,144,144}{0.654579741627}{0.108183264279}{0.662672899096}{0.107392447673}
  \meshline{144,144,144}{0.595061540376}{0.181625717786}{0.597089786278}{0.180444632347}
  \meshline{144,144,144}{0.528782654047}{0.164649426380}{0.538481490369}{0.156123039379}
  \meshline{144,144,144}{0.683094485691}{0.106232080240}{0.662672899096}{0.107392447673}
  \meshline{144,144,144}{0.632543920781}{0.111905649387}{0.641179657448}{0.110255819545}
  \meshline{144,144,144}{0.597089786278}{0.180444632347}{0.609217037237}{0.172654616019}
  \meshline{144,144,144}{0.572768151238}{0.132834234502}{0.581743767990}{0.128044873782}
  \meshline{144,144,144}{0.617173201575}{0.021175865180}{0.627028718080}{0.020837575563}
  \meshline{144,144,144}{0.529668838305}{0.080745677682}{0.542590550093}{0.075977958563}
  \meshline{144,144,144}{0.647625413372}{0.056680539025}{0.643202984668}{0.056914827033}
  \meshline{144,144,144}{0.559418254371}{0.140348394961}{0.555133998037}{0.143118712296}
  \meshline{144,144,144}{0.615639550795}{0.021175865180}{0.617173201575}{0.021175865180}
  \meshline{144,144,144}{0.607997495114}{0.060801371157}{0.600619397104}{0.062247732881}
  \meshline{144,144,144}{0.577269412603}{0.066648796440}{0.578030918858}{0.066530663527}
  \meshline{144,144,144}{0.616083673301}{0.116135751791}{0.607346579349}{0.118395189015}
  \meshline{144,144,144}{0.581743767990}{0.128044873782}{0.589674075415}{0.124822919716}
  \meshline{144,144,144}{0.638538156121}{0.020354228457}{0.627028718080}{0.020837575563}
  \meshline{144,144,144}{0.617636870384}{0.059576677908}{0.607997495114}{0.060801371157}
  \meshline{144,144,144}{0.559418254371}{0.140348394961}{0.572768151238}{0.132834234502}
  \meshline{144,144,144}{0.645380725662}{0.020108056433}{0.638538156121}{0.020354228457}
  \meshline{144,144,144}{0.597728730101}{0.022230102159}{0.610827198520}{0.021410973609}
  \meshline{144,144,144}{0.568307810117}{0.068877032592}{0.560189671094}{0.070863103799}
  \meshline{144,144,144}{0.607346579349}{0.118395189015}{0.603575681831}{0.119592874331}
  \meshline{144,144,144}{0.589674075415}{0.124822919716}{0.603575681831}{0.119592874331}
  \meshline{144,144,144}{0.597728730101}{0.022230102159}{0.581037320113}{0.023104343061}
  \meshline{144,144,144}{0.610827198520}{0.021410973609}{0.615639550795}{0.021175865180}
  \meshline{144,144,144}{0.581037320113}{0.023104343061}{0.574800744668}{0.023824083579}
  \meshline{144,144,144}{0.548679785987}{0.026030864469}{0.563089285445}{0.024592445123}
  \meshline{144,144,144}{0.542590550093}{0.075977958563}{0.559150189409}{0.071227934443}
  \meshline{144,144,144}{0.600619397104}{0.062247732881}{0.590975915517}{0.063688252637}
  \meshline{144,144,144}{0.578030918858}{0.066530663527}{0.590975915517}{0.063688252637}
  \meshline{144,144,144}{0.577269412603}{0.066648796440}{0.568307810117}{0.068877032592}
  \meshline{144,144,144}{0.723450033174}{0.020102811633}{0.736037346265}{0.020408463554}
  \meshline{144,144,144}{0.676655487709}{0.019635129798}{0.692787909750}{0.019608834586}
  \meshline{144,144,144}{0.592069549195}{0.455825260596}{0.597616145502}{0.460410240538}
  \meshline{144,144,144}{0.541640880864}{0.404965149750}{0.535344076299}{0.396963916659}
  \meshline{144,144,144}{0.581362975240}{0.385536283311}{0.572291186344}{0.372961047599}
  \meshline{144,144,144}{0.511810007868}{0.359368842151}{0.511925639701}{0.359623580511}
  \meshline{144,144,144}{0.549927665636}{0.328164926359}{0.555015630455}{0.341254627270}
  \meshline{144,144,144}{0.548030137981}{0.321314719707}{0.544850213324}{0.307561776490}
  \meshline{144,144,144}{0.542671162554}{0.289630505285}{0.542821331496}{0.276652492292}
  \meshline{144,144,144}{0.519660226662}{0.174744830517}{0.523424601005}{0.170446738019}
  \meshline{144,144,144}{0.427117927561}{0.161302739150}{0.436612532986}{0.147095509264}
  \meshline{144,144,144}{0.512587245124}{0.184706840725}{0.510591673934}{0.187416216033}
  \meshline{144,144,144}{0.540818851156}{0.153865175188}{0.555133998037}{0.143118712296}
  \meshline{144,144,144}{0.485644982694}{0.101934163267}{0.477004739451}{0.108026503911}
  \meshline{144,144,144}{0.560189671094}{0.070863103799}{0.559150189409}{0.071227934443}
  \meshline{144,144,144}{0.526086947767}{0.081930002132}{0.506573077590}{0.090734440126}
  \meshline{144,144,144}{0.526086947767}{0.081930002132}{0.529668838305}{0.080745677682}
  \meshline{144,144,144}{0.611054605733}{0.415579094445}{0.597953617909}{0.403870743741}
  \meshline{144,144,144}{0.630102138357}{0.429608250669}{0.622089059956}{0.424396167858}
  \meshline{144,144,144}{0.597616145502}{0.460410240538}{0.606502732778}{0.467194279430}
  \meshline{144,144,144}{0.606502732778}{0.467194279430}{0.613323382833}{0.471669471601}
  \meshline{144,144,144}{0.735954147177}{0.588304990407}{0.748960024735}{0.590297682192}
  \meshline{144,144,144}{0.661516652639}{0.497868742326}{0.648040838418}{0.491961983813}
  \meshline{144,144,144}{0.726514196562}{0.512491250910}{0.734497836728}{0.512885414102}
  \meshline{144,144,144}{0.544323726508}{0.475165595800}{0.556417557873}{0.486577057821}
  \meshline{144,144,144}{0.697859233386}{0.509061951973}{0.690747971502}{0.507424196388}
  \meshline{144,144,144}{0.682015512291}{0.452675079773}{0.683928540758}{0.453242394002}
  \meshline{144,144,144}{0.641333967102}{0.550755223813}{0.638594728245}{0.549303279577}
  \meshline{144,144,144}{0.592069549195}{0.455825260596}{0.581435546536}{0.447073971822}
  \meshline{144,144,144}{0.642229648967}{0.437172195989}{0.630102138357}{0.429608250669}
  \meshline{144,144,144}{0.645623636706}{0.490726300268}{0.641610048210}{0.488402476276}
  \meshline{144,144,144}{0.654614950546}{0.443233673698}{0.642229648967}{0.437172195989}
  \meshline{144,144,144}{0.669637298734}{0.449336523608}{0.682015512291}{0.452675079773}
  \meshline{144,144,144}{0.641610048210}{0.488402476276}{0.624967708463}{0.479454126311}
  \meshline{144,144,144}{0.685010415403}{0.453579413013}{0.683928540758}{0.453242394002}
  \meshline{144,144,144}{0.661516652639}{0.497868742326}{0.669481914546}{0.501073560095}
  \meshline{144,144,144}{0.669481914546}{0.501073560095}{0.678245812108}{0.503844629494}
  \meshline{144,144,144}{0.657339506830}{0.560003622112}{0.659969931390}{0.561323016622}
  \meshline{144,144,144}{0.645623636706}{0.490726300268}{0.648040838418}{0.491961983813}
  \meshline{144,144,144}{0.535874688670}{0.511045929356}{0.539234694440}{0.514310179373}
  \meshline{144,144,144}{0.638594728245}{0.549303279577}{0.626088324177}{0.541284489983}
  \meshline{144,144,144}{0.714174444647}{0.583595586197}{0.706721393166}{0.581420478474}
  \meshline{144,144,144}{0.659969931390}{0.561323016622}{0.662128576185}{0.562201569086}
  \meshline{144,144,144}{0.566289082407}{0.363157295596}{0.563268739754}{0.358266974125}
  \meshline{144,144,144}{0.555015630455}{0.341254627270}{0.557809441708}{0.347297838398}
  \meshline{144,144,144}{0.510591673934}{0.187416216033}{0.500656587191}{0.205059797556}
  \meshline{144,144,144}{0.497397188749}{0.212030251550}{0.500656587191}{0.205059797556}
  \meshline{144,144,144}{0.525346054559}{0.028734913460}{0.529996692588}{0.028361582227}
  \meshline{144,144,144}{0.563089285445}{0.024592445123}{0.574800744668}{0.023824083579}
  \meshline{144,144,144}{0.485644982694}{0.101934163267}{0.490836773502}{0.099277314276}
  \meshline{144,144,144}{0.581982987743}{0.553975475169}{0.588423998653}{0.559483401617}
  \meshline{144,144,144}{0.560854541722}{0.490746497505}{0.575027375708}{0.502876825427}
  \meshline{144,144,144}{0.578331732897}{0.505722940033}{0.591468925933}{0.516441918389}
  \meshline{144,144,144}{0.535874688670}{0.511045929356}{0.523753383592}{0.499277602256}
  \meshline{144,144,144}{0.539234694440}{0.514310179373}{0.541031776783}{0.515971731928}
  \meshline{144,144,144}{0.568805184317}{0.435347798013}{0.562233190097}{0.428781226884}
  \meshline{144,144,144}{0.581435546536}{0.447073971822}{0.575970931375}{0.442150528711}
  \meshline{144,144,144}{0.719568685609}{0.457070116945}{0.701616033918}{0.456555066214}
  \meshline{144,144,144}{0.686517473181}{0.453872650566}{0.701616033918}{0.456555066214}
  \meshline{144,144,144}{0.686517473181}{0.453872650566}{0.685010415403}{0.453579413013}
  \meshline{144,144,144}{0.525346054559}{0.028734913460}{0.508948331297}{0.031309504435}
  \meshline{144,144,144}{0.543611634824}{0.026788725754}{0.547808725766}{0.026175590328}
  \meshline{144,144,144}{0.506068880826}{0.031547421201}{0.492517476554}{0.034145443545}
  \meshline{144,144,144}{0.529996692588}{0.028361582227}{0.543611634824}{0.026788725754}
  \meshline{144,144,144}{0.489654396923}{0.559439696020}{0.489084495832}{0.558834623892}
  \meshline{144,144,144}{0.511712741495}{0.487272370120}{0.510894496709}{0.486459451378}
  \meshline{144,144,144}{0.498047064665}{0.426331226374}{0.489215717935}{0.415457120579}
  \meshline{144,144,144}{0.465424011979}{0.384029783853}{0.471151407546}{0.391936265931}
  \meshline{144,144,144}{0.522966973073}{0.378707800868}{0.524220888870}{0.380463176060}
  \meshline{144,144,144}{0.499526456513}{0.331577940129}{0.498427138028}{0.329115419439}
  \meshline{144,144,144}{0.557809441708}{0.347297838398}{0.563268739754}{0.358266974125}
  \meshline{144,144,144}{0.568805184317}{0.435347798013}{0.575970931375}{0.442150528711}
  \meshline{144,144,144}{0.541710632385}{0.405056129135}{0.541640880864}{0.404965149750}
  \meshline{144,144,144}{0.501634834068}{0.430260700973}{0.513929481309}{0.444334389301}
  \meshline{144,144,144}{0.495569101034}{0.470935721942}{0.510174062973}{0.485734754231}
  \meshline{144,144,144}{0.539587363914}{0.470742298611}{0.540918981025}{0.472028871139}
  \meshline{144,144,144}{0.510894496709}{0.486459451378}{0.510174062973}{0.485734754231}
  \meshline{144,144,144}{0.540918981025}{0.472028871139}{0.544323726508}{0.475165595800}
  \meshline{144,144,144}{0.526675613844}{0.457721386943}{0.532530617568}{0.463596044033}
  \meshline{144,144,144}{0.562233190097}{0.428781226884}{0.554213669954}{0.419859449617}
  \meshline{144,144,144}{0.498047064665}{0.426331226374}{0.501634834068}{0.430260700973}
  \meshline{144,144,144}{0.525314659278}{0.456290034312}{0.513929481309}{0.444334389301}
  \meshline{144,144,144}{0.524220888870}{0.380463176060}{0.535344076299}{0.396963916659}
  \meshline{144,144,144}{0.511925639701}{0.359623580511}{0.513736916542}{0.362742879286}
  \meshline{144,144,144}{0.541710632385}{0.405056129135}{0.541832407150}{0.405199907683}
  \meshline{144,144,144}{0.554213669954}{0.419859449617}{0.551246699246}{0.416622690829}
  \meshline{144,144,144}{0.541832407150}{0.405199907683}{0.551246699246}{0.416622690829}
  \meshline{144,144,144}{0.484162922480}{0.409342984010}{0.482862277621}{0.407592611544}
  \meshline{144,144,144}{0.511712741495}{0.487272370120}{0.523753383592}{0.499277602256}
  \meshline{144,144,144}{0.473914864676}{0.498160114300}{0.484618805112}{0.508731529738}
  \meshline{144,144,144}{0.532530617568}{0.463596044033}{0.539587363914}{0.470742298611}
  \meshline{144,144,144}{0.525314659278}{0.456290034312}{0.526675613844}{0.457721386943}
  \meshline{144,144,144}{0.479149704729}{0.402387754465}{0.471151407546}{0.391936265931}
  \meshline{144,144,144}{0.522966973073}{0.378707800868}{0.522399933043}{0.377811096922}
  \meshline{144,144,144}{0.669637298734}{0.449336523608}{0.659457491955}{0.445254776522}
  \meshline{144,144,144}{0.478360007995}{0.452935228065}{0.481600008147}{0.456499526096}
  \meshline{144,144,144}{0.442356085051}{0.467931138018}{0.448399319626}{0.473862002155}
  \meshline{144,144,144}{0.481600008147}{0.456499526096}{0.486013276234}{0.461070925548}
  \meshline{144,144,144}{0.466783342266}{0.440643213047}{0.459746346354}{0.432926245221}
  \meshline{144,144,144}{0.486013276234}{0.461070925548}{0.495569101034}{0.470935721942}
  \meshline{144,144,144}{0.484162922480}{0.409342984010}{0.489215717935}{0.415457120579}
  \meshline{144,144,144}{0.810692366629}{0.584707997903}{0.809043479771}{0.585025805854}
  \meshline{144,144,144}{0.783096673858}{0.590634181986}{0.790008971222}{0.589345409595}
  \meshline{144,144,144}{0.757106980160}{0.590308564878}{0.752841584875}{0.590535883445}
  \meshline{144,144,144}{0.799709071509}{0.587842577239}{0.809043479771}{0.585025805854}
  \meshline{144,144,144}{0.799709071509}{0.587842577239}{0.790008971222}{0.589345409595}
  \meshline{144,144,144}{0.771749727290}{0.591100357656}{0.757106980160}{0.590308564878}
  \meshline{144,144,144}{0.733014680777}{0.587651131120}{0.714174444647}{0.583595586197}
  \meshline{144,144,144}{0.735040497885}{0.664096794899}{0.725388668141}{0.658792732123}
  \meshline{144,144,144}{0.700982687882}{0.645538146898}{0.700168052015}{0.644957910449}
  \meshline{144,144,144}{0.800148705273}{0.683909546073}{0.809337371495}{0.684943117697}
  \meshline{144,144,144}{0.784989857120}{0.681646769559}{0.773801010422}{0.677943941105}
  \meshline{144,144,144}{0.766603843981}{0.676507734008}{0.756457554690}{0.672886269336}
  \meshline{144,144,144}{0.657339506830}{0.560003622112}{0.641333967102}{0.550755223813}
  \meshline{144,144,144}{0.735200653763}{0.588213927184}{0.733014680777}{0.587651131120}
  \meshline{144,144,144}{0.690062011427}{0.575131081292}{0.693684080404}{0.576636941671}
  \meshline{144,144,144}{0.678531678389}{0.570207769553}{0.669316447626}{0.565573550970}
  \meshline{144,144,144}{0.678531678389}{0.570207769553}{0.690062011427}{0.575131081292}
  \meshline{144,144,144}{0.613208047226}{0.653909857673}{0.616451011959}{0.657767804525}
  \meshline{144,144,144}{0.452026569998}{0.586812569155}{0.460173698028}{0.596997749158}
  \meshline{144,144,144}{0.528622749050}{0.554214106359}{0.531828694054}{0.557497949770}
  \meshline{144,144,144}{0.491205215629}{0.515358584414}{0.501552410687}{0.525850815105}
  \meshline{144,144,144}{0.465605856053}{0.604498623538}{0.475085406636}{0.617899935851}
  \meshline{144,144,144}{0.533901082976}{0.559591068225}{0.551447800582}{0.578745105476}
  \meshline{144,144,144}{0.642640055637}{0.605123667765}{0.647663747457}{0.608788503658}
  \meshline{144,144,144}{0.619933261700}{0.586753973905}{0.633946595500}{0.597985292803}
  \meshline{144,144,144}{0.735200653763}{0.588213927184}{0.735954147177}{0.588304990407}
  \meshline{144,144,144}{0.706721393166}{0.581420478474}{0.695595030320}{0.577170848027}
  \meshline{144,144,144}{0.541031776783}{0.515971731928}{0.546286258258}{0.520890837279}
  \meshline{144,144,144}{0.554209811340}{0.528574426612}{0.546286258258}{0.520890837279}
  \meshline{144,144,144}{0.576112752131}{0.503861363229}{0.578331732897}{0.505722940033}
  \meshline{144,144,144}{0.567755872819}{0.541129873440}{0.566445851521}{0.539815679865}
  \meshline{144,144,144}{0.576112752131}{0.503861363229}{0.575027375708}{0.502876825427}
  \meshline{144,144,144}{0.554209811340}{0.528574426612}{0.566445851521}{0.539815679865}
  \meshline{144,144,144}{0.581982987743}{0.553975475169}{0.570236864664}{0.543392469529}
  \meshline{144,144,144}{0.528622749050}{0.554214106359}{0.516145758310}{0.540891243241}
  \meshline{144,144,144}{0.608966353264}{0.529401126370}{0.599183964119}{0.522524921252}
  \meshline{144,144,144}{0.565625755303}{0.595068770575}{0.574025268776}{0.604489458772}
  \meshline{144,144,144}{0.531828694054}{0.557497949770}{0.533901082976}{0.559591068225}
  \meshline{144,144,144}{0.599372246296}{0.569489804960}{0.606093722107}{0.575142902356}
  \meshline{144,144,144}{0.552980637658}{0.580404878035}{0.551447800582}{0.578745105476}
  \meshline{144,144,144}{0.570236864664}{0.543392469529}{0.567755872819}{0.541129873440}
  \meshline{144,144,144}{0.599183964119}{0.522524921252}{0.591468925933}{0.516441918389}
  \meshline{144,144,144}{0.608966353264}{0.529401126370}{0.616695807393}{0.535101723547}
  \meshline{144,144,144}{0.588423998653}{0.559483401617}{0.594267428032}{0.564852247648}
  \meshline{144,144,144}{0.552980637658}{0.580404878035}{0.562810117410}{0.591467125837}
  \meshline{144,144,144}{0.606093722107}{0.575142902356}{0.617581236363}{0.584684144564}
  \meshline{144,144,144}{0.533548225417}{0.614456515296}{0.521160436699}{0.597251879576}
  \meshline{144,144,144}{0.505922253279}{0.578194919778}{0.498154243197}{0.569044799349}
  \meshline{144,144,144}{0.562810117410}{0.591467125837}{0.565625755303}{0.595068770575}
  \meshline{144,144,144}{0.516145758310}{0.540891243241}{0.507215732572}{0.531578476952}
  \meshline{144,144,144}{0.501552410687}{0.525850815105}{0.507215732572}{0.531578476952}
  \meshline{144,144,144}{0.513060219583}{0.587276736728}{0.518739923498}{0.594353603971}
  \meshline{144,144,144}{0.513060219583}{0.587276736728}{0.508929666381}{0.581936393203}
  \meshline{144,144,144}{0.486777075253}{0.556401311358}{0.489084495832}{0.558834623892}
  \meshline{144,144,144}{0.471688394588}{0.496003325493}{0.473914864676}{0.498160114300}
  \meshline{144,144,144}{0.450149418911}{0.519047915565}{0.444799773747}{0.514123647129}
  \meshline{144,144,144}{0.462909307697}{0.487386760633}{0.458081965072}{0.482822869793}
  \meshline{144,144,144}{0.469109777308}{0.443307527896}{0.478360007995}{0.452935228065}
  \meshline{144,144,144}{0.466783342266}{0.440643213047}{0.469109777308}{0.443307527896}
  \meshline{144,144,144}{0.448399319626}{0.473862002155}{0.458081965072}{0.482822869793}
  \meshline{144,144,144}{0.453237657554}{0.425848035898}{0.450781975896}{0.423375046679}
  \meshline{144,144,144}{0.459746346354}{0.432926245221}{0.453237657554}{0.425848035898}
  \meshline{144,144,144}{0.704451846677}{0.647484735490}{0.721212381014}{0.656992885933}
  \meshline{144,144,144}{0.618727775592}{0.585730926159}{0.619933261700}{0.586753973905}
  \meshline{144,144,144}{0.693684080404}{0.576636941671}{0.695595030320}{0.577170848027}
  \meshline{144,144,144}{0.662128576185}{0.562201569086}{0.669316447626}{0.565573550970}
  \meshline{144,144,144}{0.690747971502}{0.507424196388}{0.678245812108}{0.503844629494}
  \meshline{144,144,144}{0.518739923498}{0.594353603971}{0.521160436699}{0.597251879576}
  \meshline{144,144,144}{0.535046374471}{0.616565521748}{0.533548225417}{0.614456515296}
  \meshline{144,144,144}{0.480880821094}{0.627314509521}{0.475085406636}{0.617899935851}
  \meshline{144,144,144}{0.462494149193}{0.599938527251}{0.465605856053}{0.604498623538}
  \meshline{144,144,144}{0.498154243197}{0.569044799349}{0.489654396923}{0.559439696020}
  \meshline{144,144,144}{0.450149418911}{0.519047915565}{0.460016903753}{0.528681198216}
  \meshline{144,144,144}{0.461779800865}{0.530354950170}{0.460016903753}{0.528681198216}
  \meshline{144,144,144}{0.420206022612}{0.447674388074}{0.428115278075}{0.454953708668}
  \meshline{144,144,144}{0.420428326903}{0.492976248734}{0.434725665853}{0.505168114862}
  \meshline{144,144,144}{0.434980459110}{0.461135095705}{0.431678892608}{0.458131339279}
  \meshline{144,144,144}{0.434725665853}{0.505168114862}{0.444799773747}{0.514123647129}
  \meshline{144,144,144}{0.403120696804}{0.479312326118}{0.390825184573}{0.470209071917}
  \meshline{144,144,144}{0.414675837230}{0.442599172141}{0.420206022612}{0.447674388074}
  \meshline{144,144,144}{0.418079919274}{0.491035949074}{0.403518961559}{0.479593616854}
  \meshline{144,144,144}{0.428115278075}{0.454953708668}{0.431678892608}{0.458131339279}
  \meshline{144,144,144}{0.633946595500}{0.597985292803}{0.642640055637}{0.605123667765}
  \meshline{144,144,144}{0.661710747134}{0.619491920550}{0.664411413357}{0.621299150473}
  \meshline{144,144,144}{0.704451846677}{0.647484735490}{0.700982687882}{0.645538146898}
  \meshline{144,144,144}{0.683363115089}{0.634452808640}{0.681465429110}{0.632890709382}
  \meshline{144,144,144}{0.725388668141}{0.658792732123}{0.721212381014}{0.656992885933}
  \meshline{144,144,144}{0.644433547266}{0.699282961450}{0.645657240585}{0.700850112370}
  \meshline{144,144,144}{0.735040497885}{0.664096794899}{0.746423607441}{0.668618587980}
  \meshline{144,144,144}{0.629846296520}{0.677096911169}{0.633578803768}{0.682050803483}
  \meshline{144,144,144}{0.629846296520}{0.677096911169}{0.622418383659}{0.665925473023}
  \meshline{144,144,144}{0.683363115089}{0.634452808640}{0.700168052015}{0.644957910449}
  \meshline{144,144,144}{0.633578803768}{0.682050803483}{0.635687668222}{0.684711124081}
  \meshline{144,144,144}{0.622418383659}{0.665925473023}{0.619557855510}{0.661745305671}
  \meshline{144,144,144}{0.675833987734}{0.628860642485}{0.681465429110}{0.632890709382}
  \meshline{144,144,144}{0.661710747134}{0.619491920550}{0.647663747457}{0.608788503658}
  \meshline{144,144,144}{0.666750672237}{0.622632965680}{0.675833987734}{0.628860642485}
  \meshline{144,144,144}{0.664411413357}{0.621299150473}{0.666750672237}{0.622632965680}
  \meshline{144,144,144}{0.655385037632}{0.717187929198}{0.647315089112}{0.703364897684}
  \meshline{144,144,144}{0.644433547266}{0.699282961450}{0.635687668222}{0.684711124081}
  \meshline{144,144,144}{0.749611637397}{0.670203393050}{0.746423607441}{0.668618587980}
  \meshline{144,144,144}{0.655385037632}{0.717187929198}{0.659831275316}{0.724638862554}
  \meshline{144,144,144}{0.599096864668}{0.634918401895}{0.607132921474}{0.645300060199}
  \meshline{144,144,144}{0.613208047226}{0.653909857673}{0.607132921474}{0.645300060199}
  \meshline{144,144,144}{0.588325681980}{0.734622997426}{0.589473327179}{0.741767759639}
  \meshline{144,144,144}{0.616451011959}{0.657767804525}{0.619557855510}{0.661745305671}
  \meshline{144,144,144}{0.664637542156}{0.736560370871}{0.669104336289}{0.745609906990}
  \meshline{144,144,144}{0.579157090449}{0.700575179644}{0.583523631591}{0.713864061665}
  \meshline{144,144,144}{0.664637542156}{0.736560370871}{0.662751835233}{0.730758062008}
  \meshline{144,144,144}{0.670929145156}{0.752468938558}{0.678271158655}{0.771591851056}
  \meshline{144,144,144}{0.662751835233}{0.730758062008}{0.659831275316}{0.724638862554}
  \meshline{144,144,144}{0.599372246296}{0.569489804960}{0.594267428032}{0.564852247648}
  \meshline{144,144,144}{0.618727775592}{0.585730926159}{0.617581236363}{0.584684144564}
  \meshline{144,144,144}{0.711252519055}{0.510882638425}{0.697859233386}{0.509061951973}
  \meshline{144,144,144}{0.726514196562}{0.512491250910}{0.717397954367}{0.511983271100}
  \meshline{144,144,144}{0.717397954367}{0.511983271100}{0.711252519055}{0.510882638425}
  \meshline{144,144,144}{0.548281145154}{0.636646696598}{0.535305607417}{0.617003523807}
  \meshline{144,144,144}{0.480880821094}{0.627314509521}{0.489294296418}{0.642532584609}
  \meshline{144,144,144}{0.551059094122}{0.641855275618}{0.548281145154}{0.636646696598}
  \meshline{144,144,144}{0.584870934285}{0.719540048123}{0.583523631591}{0.713864061665}
  \meshline{144,144,144}{0.456964576833}{0.704382621814}{0.457059632303}{0.708468119039}
  \meshline{144,144,144}{0.434300974320}{0.637280350068}{0.439454166342}{0.646585181720}
  \meshline{144,144,144}{0.575138861997}{0.605980443261}{0.585284706835}{0.617878342527}
  \meshline{144,144,144}{0.551059094122}{0.641855275618}{0.559931896857}{0.656719065241}
  \meshline{144,144,144}{0.594903848688}{0.630061737783}{0.587121312385}{0.620442445325}
  \meshline{144,144,144}{0.579157090449}{0.700575179644}{0.573424876862}{0.685448345179}
  \meshline{144,144,144}{0.493090016397}{0.649724063598}{0.489294296418}{0.642532584609}
  \meshline{144,144,144}{0.575138861997}{0.605980443261}{0.574025268776}{0.604489458772}
  \meshline{144,144,144}{0.559931896857}{0.656719065241}{0.562912397291}{0.662984192356}
  \meshline{144,144,144}{0.502900308930}{0.675414001825}{0.498096632070}{0.660963098401}
  \meshline{144,144,144}{0.495212055958}{0.655061903572}{0.498096632070}{0.660963098401}
  \meshline{144,144,144}{0.535305607417}{0.617003523807}{0.535046374471}{0.616565521748}
  \meshline{144,144,144}{0.502900308930}{0.675414001825}{0.504071408117}{0.678071801623}
  \meshline{144,144,144}{0.403518961559}{0.479593616854}{0.403351593192}{0.479469808460}
  \meshline{144,144,144}{0.474966045870}{0.543703531399}{0.463098011494}{0.531735446510}
  \meshline{144,144,144}{0.486777075253}{0.556401311358}{0.474966045870}{0.543703531399}
  \meshline{144,144,144}{0.463098011494}{0.531735446510}{0.461779800865}{0.530354950170}
  \meshline{144,144,144}{0.444699528500}{0.578719140610}{0.452026569998}{0.586812569155}
  \meshline{144,144,144}{0.462494149193}{0.599938527251}{0.460173698028}{0.596997749158}
  \meshline{144,144,144}{0.444699528500}{0.578719140610}{0.440323466541}{0.573808799828}
  \meshline{144,144,144}{0.447910162085}{0.665840288640}{0.448307926987}{0.666837082628}
  \meshline{144,144,144}{0.508929666381}{0.581936393203}{0.505922253279}{0.578194919778}
  \meshline{144,144,144}{0.420428326903}{0.492976248734}{0.418079919274}{0.491035949074}
  \meshline{144,144,144}{0.430137908516}{0.563528971859}{0.440323466541}{0.573808799828}
  \meshline{144,144,144}{0.398375921486}{0.536217646173}{0.408039799071}{0.544109195410}
  \meshline{144,144,144}{0.394056368880}{0.533018620994}{0.382946891576}{0.525728093195}
  \meshline{144,144,144}{0.367542288333}{0.568520229180}{0.364946001908}{0.566769019002}
  \meshline{144,144,144}{0.414606500988}{0.549348741415}{0.426267934112}{0.559767225537}
  \meshline{144,144,144}{0.382946891576}{0.525728093195}{0.376179913070}{0.521135096690}
  \meshline{144,144,144}{0.439454166342}{0.646585181720}{0.443209960205}{0.653931764373}
  \meshline{144,144,144}{0.376179913070}{0.521135096690}{0.373381988656}{0.519583140498}
  \meshline{144,144,144}{0.414606500988}{0.549348741415}{0.408039799071}{0.544109195410}
  \meshline{144,144,144}{0.383305620971}{0.579692621607}{0.389092982546}{0.584016424576}
  \meshline{144,144,144}{0.430137908516}{0.563528971859}{0.426267934112}{0.559767225537}
  \meshline{144,144,144}{0.394056368880}{0.533018620994}{0.398375921486}{0.536217646173}
  \meshline{144,144,144}{0.645657240585}{0.700850112370}{0.647315089112}{0.703364897684}
  \meshline{144,144,144}{0.594903848688}{0.630061737783}{0.597536824956}{0.633143511714}
  \meshline{144,144,144}{0.587121312385}{0.620442445325}{0.585284706835}{0.617878342527}
  \meshline{144,144,144}{0.599096864668}{0.634918401895}{0.597536824956}{0.633143511714}
  \meshline{144,144,144}{0.447910162085}{0.665840288640}{0.443209960205}{0.653931764373}
  \meshline{144,144,144}{0.493090016397}{0.649724063598}{0.495212055958}{0.655061903572}
  \meshline{144,144,144}{0.507445258061}{0.773556478119}{0.506863418168}{0.775135341536}
  \meshline{144,144,144}{0.505784356109}{0.683930041667}{0.508905634050}{0.696443971839}
  \meshline{144,144,144}{0.448307926987}{0.666837082628}{0.448684404045}{0.668157640953}
  \meshline{144,144,144}{0.453948523558}{0.685794935740}{0.448684404045}{0.668157640953}
  \meshline{144,144,144}{0.425896026051}{0.624011664842}{0.429524804131}{0.629413382202}
  \meshline{144,144,144}{0.456167853183}{0.699452100934}{0.453948523558}{0.685794935740}
  \meshline{144,144,144}{0.347351094329}{0.557302680924}{0.342069116244}{0.555367514890}
  \meshline{144,144,144}{0.361371636357}{0.512626338363}{0.355812294342}{0.510011395454}
  \meshline{144,144,144}{0.364946001908}{0.566769019002}{0.356269667561}{0.562120529554}
  \meshline{144,144,144}{0.344011352339}{0.504170168389}{0.325098904078}{0.497065837924}
  \meshline{144,144,144}{0.371470502038}{0.571466230011}{0.367542288333}{0.568520229180}
  \meshline{144,144,144}{0.347351094329}{0.557302680924}{0.356269667561}{0.562120529554}
  \meshline{144,144,144}{0.354112449473}{0.611317162622}{0.344919326981}{0.605486021051}
  \meshline{144,144,144}{0.303889618449}{0.591965254885}{0.290929834643}{0.591361772680}
  \meshline{144,144,144}{0.670929145156}{0.752468938558}{0.669104336289}{0.745609906990}
  \meshline{144,144,144}{0.679146350677}{0.776538422873}{0.682615078133}{0.788284344958}
  \meshline{144,144,144}{0.624285626289}{0.925166320216}{0.630871786985}{0.920414477432}
  \meshline{144,144,144}{0.683201694488}{0.841691515570}{0.682153885292}{0.845771086305}
  \meshline{144,144,144}{0.684371818020}{0.804333052870}{0.684254667916}{0.801889034461}
  \meshline{144,144,144}{0.684901419130}{0.826294400256}{0.683201694488}{0.841691515570}
  \meshline{144,144,144}{0.684901419130}{0.826294400256}{0.685499519466}{0.821382815754}
  \meshline{144,144,144}{0.677266309187}{0.862647487837}{0.682153885292}{0.845771086305}
  \meshline{144,144,144}{0.685499519466}{0.821382815754}{0.684371818020}{0.804333052870}
  \meshline{144,144,144}{0.381550303886}{0.636594806068}{0.374880837291}{0.628576942721}
  \meshline{144,144,144}{0.403559934734}{0.676523935781}{0.404912075384}{0.680080338032}
  \meshline{144,144,144}{0.407876268856}{0.698016654830}{0.408785888982}{0.706495589550}
  \meshline{144,144,144}{0.404912075384}{0.680080338032}{0.405703603708}{0.683424490929}
  \meshline{144,144,144}{0.425896026051}{0.624011664842}{0.420627624940}{0.616760252761}
  \meshline{144,144,144}{0.363560932801}{0.618224391952}{0.374880837291}{0.628576942721}
  \meshline{144,144,144}{0.326059944922}{0.549209986356}{0.342069116244}{0.555367514890}
  \meshline{144,144,144}{0.361371636357}{0.512626338363}{0.373381988656}{0.519583140498}
  \meshline{144,144,144}{0.344011352339}{0.504170168389}{0.355812294342}{0.510011395454}
  \meshline{144,144,144}{0.307753834965}{0.544856957606}{0.312645311125}{0.545719676238}
  \meshline{144,144,144}{0.368035925252}{0.454761614507}{0.371942389709}{0.457412011506}
  \meshline{144,144,144}{0.403351593192}{0.479469808460}{0.403120696804}{0.479312326118}
  \meshline{144,144,144}{0.682615078133}{0.788284344958}{0.684254667916}{0.801889034461}
  \meshline{144,144,144}{0.591270215100}{0.765393194358}{0.589211400898}{0.789602085396}
  \meshline{144,144,144}{0.434300974320}{0.637280350068}{0.429524804131}{0.629413382202}
  \meshline{144,144,144}{0.395209367006}{0.656651594363}{0.397690905227}{0.660990365057}
  \meshline{144,144,144}{0.381550303886}{0.636594806068}{0.387644905296}{0.644384226138}
  \meshline{144,144,144}{0.401482602340}{0.595230829037}{0.397545075198}{0.591617620137}
  \meshline{144,144,144}{0.420627624940}{0.616760252761}{0.411693876454}{0.606196971717}
  \meshline{144,144,144}{0.363560932801}{0.618224391952}{0.360347253752}{0.615459331961}
  \meshline{144,144,144}{0.397545075198}{0.591617620137}{0.389092982546}{0.584016424576}
  \meshline{144,144,144}{0.383305620971}{0.579692621607}{0.371470502038}{0.571466230011}
  \meshline{144,144,144}{0.313576499501}{0.593703801293}{0.326951441181}{0.597646958375}
  \meshline{144,144,144}{0.290929834643}{0.591361772680}{0.286183870883}{0.591260099298}
  \meshline{144,144,144}{0.381474559130}{0.463538332985}{0.390825184573}{0.470209071917}
  \meshline{144,144,144}{0.589099077906}{0.791818713796}{0.588912394049}{0.793211611230}
  \meshline{144,144,144}{0.589211400898}{0.789602085396}{0.589099077906}{0.791818713796}
  \meshline{144,144,144}{0.591270215100}{0.765393194358}{0.589965418808}{0.752330643533}
  \meshline{144,144,144}{0.313576499501}{0.593703801293}{0.303889618449}{0.591965254885}
  \meshline{144,144,144}{0.263177451422}{0.595695534341}{0.259614758622}{0.596769055423}
  \meshline{144,144,144}{0.411693876454}{0.606196971717}{0.409272004517}{0.603270956915}
  \meshline{144,144,144}{0.406507267280}{0.600385245439}{0.409272004517}{0.603270956915}
  \meshline{144,144,144}{0.401482602340}{0.595230829037}{0.406507267280}{0.600385245439}
  \meshline{144,144,144}{0.395209367006}{0.656651594363}{0.387644905296}{0.644384226138}
  \meshline{144,144,144}{0.403559934734}{0.676523935781}{0.397690905227}{0.660990365057}
  \meshline{144,144,144}{0.443311528353}{0.774852064773}{0.447587993730}{0.766496565406}
  \meshline{144,144,144}{0.336083238241}{0.601278429382}{0.344919326981}{0.605486021051}
  \meshline{144,144,144}{0.326951441181}{0.597646958375}{0.330355349758}{0.598605382704}
  \meshline{144,144,144}{0.360347253752}{0.615459331961}{0.354112449473}{0.611317162622}
  \meshline{144,144,144}{0.336083238241}{0.601278429382}{0.330355349758}{0.598605382704}
  \meshline{144,144,144}{0.374545832058}{0.329409497542}{0.373851568665}{0.328520794538}
  \meshline{144,144,144}{0.345867048467}{0.441618149450}{0.343641178842}{0.440436706545}
  \meshline{144,144,144}{0.366197894956}{0.453523041074}{0.368035925252}{0.454761614507}
  \meshline{144,144,144}{0.366197894956}{0.453523041074}{0.348581124511}{0.443380267216}
  \meshline{144,144,144}{0.383146666446}{0.416216026442}{0.377450149715}{0.411198694125}
  \meshline{144,144,144}{0.378940200162}{0.461950571881}{0.381474559130}{0.463538332985}
  \meshline{144,144,144}{0.343641178842}{0.440436706545}{0.331276449400}{0.433984662442}
  \meshline{144,144,144}{0.378940200162}{0.461950571881}{0.371942389709}{0.457412011506}
  \meshline{144,144,144}{0.669730030351}{0.877908783849}{0.659926158253}{0.892489111383}
  \meshline{144,144,144}{0.677266309187}{0.862647487837}{0.671880535980}{0.874251961301}
  \meshline{144,144,144}{0.671880535980}{0.874251961301}{0.669730030351}{0.877908783849}
  \meshline{144,144,144}{0.655616496124}{0.897995270006}{0.646617086928}{0.907245407948}
  \meshline{144,144,144}{0.646617086928}{0.907245407948}{0.644278795370}{0.909459035673}
  \meshline{144,144,144}{0.659926158253}{0.892489111383}{0.655616496124}{0.897995270006}
  \meshline{144,144,144}{0.599422977184}{0.938081485329}{0.584093951108}{0.945743645157}
  \meshline{144,144,144}{0.640721122968}{0.912031593272}{0.644278795370}{0.909459035673}
  \meshline{144,144,144}{0.414675837230}{0.442599172141}{0.402576803349}{0.432376026878}
  \meshline{144,144,144}{0.396671945966}{0.426942043697}{0.402576803349}{0.432376026878}
  \meshline{144,144,144}{0.383146666446}{0.416216026442}{0.396671945966}{0.426942043697}
  \meshline{144,144,144}{0.507513434196}{0.773194925828}{0.507445258061}{0.773556478119}
  \meshline{144,144,144}{0.513107540366}{0.727267430040}{0.512782626587}{0.740159473800}
  \meshline{144,144,144}{0.512461989384}{0.745964347966}{0.512782626587}{0.740159473800}
  \meshline{144,144,144}{0.511912075687}{0.716715461719}{0.513107540366}{0.727267430040}
  \meshline{144,144,144}{0.507767206428}{0.771535777301}{0.507513434196}{0.773194925828}
  \meshline{144,144,144}{0.507767206428}{0.771535777301}{0.512461989384}{0.745964347966}
  \meshline{144,144,144}{0.570447846159}{0.679264081549}{0.572398651069}{0.683183586151}
  \meshline{144,144,144}{0.586171926607}{0.726175406895}{0.588325681980}{0.734622997426}
  \meshline{144,144,144}{0.508905634050}{0.696443971839}{0.511119234297}{0.707197631364}
  \meshline{144,144,144}{0.504071408117}{0.678071801623}{0.505784356109}{0.683930041667}
  \meshline{144,144,144}{0.511912075687}{0.716715461719}{0.511119234297}{0.707197631364}
  \meshline{144,144,144}{0.570447846159}{0.679264081549}{0.562912397291}{0.662984192356}
  \meshline{144,144,144}{0.572398651069}{0.683183586151}{0.573424876862}{0.685448345179}
  \meshline{144,144,144}{0.589473327179}{0.741767759639}{0.589965418808}{0.752330643533}
  \meshline{144,144,144}{0.584870934285}{0.719540048123}{0.586171926607}{0.726175406895}
  \meshline{144,144,144}{0.610552837415}{0.933755877943}{0.620607939699}{0.927514192056}
  \meshline{144,144,144}{0.630871786985}{0.920414477432}{0.640721122968}{0.912031593272}
  \meshline{144,144,144}{0.606133416536}{0.935727715222}{0.599422977184}{0.938081485329}
  \meshline{144,144,144}{0.624285626289}{0.925166320216}{0.620607939699}{0.927514192056}
  \meshline{144,144,144}{0.610552837415}{0.933755877943}{0.606133416536}{0.935727715222}
  \meshline{144,144,144}{0.588316749566}{0.795307788579}{0.588912394049}{0.793211611230}
  \meshline{144,144,144}{0.579740123398}{0.824902799900}{0.575996600686}{0.833266143726}
  \meshline{144,144,144}{0.443819298384}{0.857529490102}{0.445359503186}{0.856293919330}
  \meshline{144,144,144}{0.403592705836}{0.739064269527}{0.402806435061}{0.741144826706}
  \meshline{144,144,144}{0.500531243486}{0.792953216867}{0.494348260013}{0.805725621338}
  \meshline{144,144,144}{0.506863418168}{0.775135341536}{0.501537053887}{0.790729998776}
  \meshline{144,144,144}{0.494348260013}{0.805725621338}{0.490259145200}{0.811728158975}
  \meshline{144,144,144}{0.510403348089}{0.965626917529}{0.491939088718}{0.968700446151}
  \meshline{144,144,144}{0.500531243486}{0.792953216867}{0.501537053887}{0.790729998776}
  \meshline{144,144,144}{0.498598150072}{0.906799276272}{0.510460561874}{0.900631050914}
  \meshline{144,144,144}{0.568736372425}{0.845508436138}{0.575996600686}{0.833266143726}
  \meshline{144,144,144}{0.582204915080}{0.818286104687}{0.579740123398}{0.824902799900}
  \meshline{144,144,144}{0.588316749566}{0.795307788579}{0.582204915080}{0.818286104687}
  \meshline{144,144,144}{0.552845290356}{0.866064484463}{0.552328984159}{0.866635932970}
  \meshline{144,144,144}{0.561624760881}{0.953447428151}{0.573853621018}{0.949028238019}
  \meshline{144,144,144}{0.573853621018}{0.949028238019}{0.584093951108}{0.945743645157}
  \meshline{144,144,144}{0.554670243268}{0.954950352977}{0.540729175763}{0.959358597309}
  \meshline{144,144,144}{0.513436917927}{0.964856688509}{0.519293968437}{0.963488105389}
  \meshline{144,144,144}{0.540729175763}{0.959358597309}{0.533728655071}{0.960679378507}
  \meshline{144,144,144}{0.413747919344}{0.274307480304}{0.416179805437}{0.285302709534}
  \meshline{144,144,144}{0.510602777897}{0.356588455346}{0.511810007868}{0.359368842151}
  \meshline{144,144,144}{0.492868752982}{0.311697084596}{0.497733241638}{0.326963401534}
  \meshline{144,144,144}{0.487337019502}{0.262946382266}{0.487282783926}{0.262024846951}
  \meshline{144,144,144}{0.487576761110}{0.278474500692}{0.487337019502}{0.262946382266}
  \meshline{144,144,144}{0.513736916542}{0.362742879286}{0.522399933043}{0.377811096922}
  \meshline{144,144,144}{0.487982043268}{0.284764643744}{0.490336682593}{0.299080185347}
  \meshline{144,144,144}{0.497733241638}{0.326963401534}{0.498427138028}{0.329115419439}
  \meshline{144,144,144}{0.490336682593}{0.299080185347}{0.490977856241}{0.302614689257}
  \meshline{144,144,144}{0.441092870434}{0.344507191832}{0.438792982454}{0.340054807006}
  \meshline{144,144,144}{0.479149704729}{0.402387754465}{0.482862277621}{0.407592611544}
  \meshline{144,144,144}{0.451035944666}{0.361992206109}{0.448193906229}{0.356818177358}
  \meshline{144,144,144}{0.420444913265}{0.297467563849}{0.418139583169}{0.291923756262}
  \meshline{144,144,144}{0.443191754678}{0.347932450215}{0.448193906229}{0.356818177358}
  \meshline{144,144,144}{0.422083843559}{0.390246641585}{0.429424046738}{0.399389848341}
  \meshline{144,144,144}{0.424875027332}{0.310301604189}{0.420444913265}{0.297467563849}
  \meshline{144,144,144}{0.441578817907}{0.413095042697}{0.439627752321}{0.410743159869}
  \meshline{144,144,144}{0.459498608759}{0.375017680954}{0.451035944666}{0.361992206109}
  \meshline{144,144,144}{0.433697266776}{0.330046616897}{0.438792982454}{0.340054807006}
  \meshline{144,144,144}{0.465424011979}{0.384029783853}{0.459498608759}{0.375017680954}
  \meshline{144,144,144}{0.444039979546}{0.415870367954}{0.441578817907}{0.413095042697}
  \meshline{144,144,144}{0.434221399075}{0.404559427330}{0.429424046738}{0.399389848341}
  \meshline{144,144,144}{0.450781975896}{0.423375046679}{0.444039979546}{0.415870367954}
  \meshline{144,144,144}{0.434221399075}{0.404559427330}{0.439627752321}{0.410743159869}
  \meshline{144,144,144}{0.415074531942}{0.382346772325}{0.422083843559}{0.390246641585}
  \meshline{144,144,144}{0.443191754678}{0.347932450215}{0.441092870434}{0.344507191832}
  \meshline{144,144,144}{0.408240758463}{0.373473497027}{0.402998503329}{0.367548372187}
  \meshline{144,144,144}{0.385883311911}{0.345356819427}{0.392347003677}{0.353806355681}
  \meshline{144,144,144}{0.368704360410}{0.403414506991}{0.374086180522}{0.407953084749}
  \meshline{144,144,144}{0.408240758463}{0.373473497027}{0.415074531942}{0.382346772325}
  \meshline{144,144,144}{0.457487980288}{0.723313249937}{0.456100090938}{0.733620190102}
  \meshline{144,144,144}{0.456964576833}{0.704382621814}{0.456167853183}{0.699452100934}
  \meshline{144,144,144}{0.456100090938}{0.733620190102}{0.452576575250}{0.752134747351}
  \meshline{144,144,144}{0.561624760881}{0.953447428151}{0.554670243268}{0.954950352977}
  \meshline{144,144,144}{0.531742619193}{0.885866418832}{0.516978471498}{0.896031969332}
  \meshline{144,144,144}{0.566456614088}{0.848937756142}{0.568736372425}{0.845508436138}
  \meshline{144,144,144}{0.516978471498}{0.896031969332}{0.510460561874}{0.900631050914}
  \meshline{144,144,144}{0.535806328884}{0.882618180099}{0.531742619193}{0.885866418832}
  \meshline{144,144,144}{0.552328984159}{0.866635932970}{0.535806328884}{0.882618180099}
  \meshline{144,144,144}{0.552845290356}{0.866064484463}{0.553360636537}{0.865372131817}
  \meshline{144,144,144}{0.566456614088}{0.848937756142}{0.553360636537}{0.865372131817}
  \meshline{144,144,144}{0.491686711313}{0.910583613622}{0.498598150072}{0.906799276272}
  \meshline{144,144,144}{0.396391946640}{0.938400653126}{0.413705733032}{0.935456899274}
  \meshline{144,144,144}{0.395414188031}{0.938593498675}{0.395850632984}{0.938517988049}
  \meshline{144,144,144}{0.482144663336}{0.914643455600}{0.491686711313}{0.910583613622}
  \meshline{144,144,144}{0.459329365080}{0.923035520098}{0.482144663336}{0.914643455600}
  \meshline{144,144,144}{0.510403348089}{0.965626917529}{0.513436917927}{0.964856688509}
  \meshline{144,144,144}{0.454646317301}{0.924736506764}{0.457297806830}{0.923907721985}
  \meshline{144,144,144}{0.436886546921}{0.930113675800}{0.454646317301}{0.924736506764}
  \meshline{144,144,144}{0.459329365080}{0.923035520098}{0.457297806830}{0.923907721985}
  \meshline{144,144,144}{0.452132052338}{0.973714271950}{0.443784371996}{0.974769672913}
  \meshline{144,144,144}{0.483400002904}{0.970022271530}{0.491939088718}{0.968700446151}
  \meshline{144,144,144}{0.423740426564}{0.976496031194}{0.413348703101}{0.976990968407}
  \meshline{144,144,144}{0.413705733032}{0.935456899274}{0.424432759464}{0.932685916176}
  \meshline{144,144,144}{0.452132052338}{0.973714271950}{0.463636298700}{0.972599663106}
  \meshline{144,144,144}{0.424432759464}{0.932685916176}{0.436886546921}{0.930113675800}
  \meshline{144,144,144}{0.325088235205}{0.980324529847}{0.304073858787}{0.980370630888}
  \meshline{144,144,144}{0.443531952952}{0.857714753327}{0.422302287859}{0.869648198672}
  \meshline{144,144,144}{0.443531952952}{0.857714753327}{0.443819298384}{0.857529490102}
  \meshline{144,144,144}{0.397180384073}{0.880002855949}{0.404838545440}{0.877201139263}
  \meshline{144,144,144}{0.418837486681}{0.871429507012}{0.422302287859}{0.869648198672}
  \meshline{144,144,144}{0.395850632984}{0.938517988049}{0.396391946640}{0.938400653126}
  \meshline{144,144,144}{0.370377811977}{0.941708961915}{0.395414188031}{0.938593498675}
  \meshline{144,144,144}{0.423740426564}{0.976496031194}{0.434443620954}{0.975351317326}
  \meshline{144,144,144}{0.380203780515}{0.978927256832}{0.380313940320}{0.978919865784}
  \meshline{144,144,144}{0.443784371996}{0.974769672913}{0.434443620954}{0.975351317326}
  \meshline{144,144,144}{0.380313940320}{0.978919865784}{0.380532022678}{0.978905213941}
  \meshline{144,144,144}{0.338016680096}{0.845058442892}{0.332971601783}{0.845651407408}
  \meshline{144,144,144}{0.405551974440}{0.977719020623}{0.380532022678}{0.978905213941}
  \meshline{144,144,144}{0.414754623195}{0.810695339481}{0.418447650221}{0.806939304814}
  \meshline{144,144,144}{0.413348703101}{0.976990968407}{0.405551974440}{0.977719020623}
  \meshline{144,144,144}{0.375880778291}{0.886218460020}{0.368983171143}{0.887804719966}
  \meshline{144,144,144}{0.418837486681}{0.871429507012}{0.404838545440}{0.877201139263}
  \meshline{144,144,144}{0.445359503186}{0.856293919330}{0.462555634056}{0.843021086710}
  \meshline{144,144,144}{0.462555634056}{0.843021086710}{0.466757846330}{0.839625228362}
  \meshline{144,144,144}{0.409231676795}{0.242434686062}{0.410666576394}{0.256829771168}
  \meshline{144,144,144}{0.433697266776}{0.330046616897}{0.429999935189}{0.321117490457}
  \meshline{144,144,144}{0.424875027332}{0.310301604189}{0.426566019145}{0.313778586109}
  \meshline{144,144,144}{0.429999935189}{0.321117490457}{0.426566019145}{0.313778586109}
  \meshline{144,144,144}{0.492868752982}{0.311697084596}{0.490977856241}{0.302614689257}
  \meshline{144,144,144}{0.392347003677}{0.353806355681}{0.394226124322}{0.355970484951}
  \meshline{144,144,144}{0.368704360410}{0.403414506991}{0.362018895614}{0.398486016427}
  \meshline{144,144,144}{0.362018895614}{0.398486016427}{0.345555363775}{0.386024726315}
  \meshline{144,144,144}{0.348581124511}{0.443380267216}{0.345867048467}{0.441618149450}
  \meshline{144,144,144}{0.374086180522}{0.407953084749}{0.377450149715}{0.411198694125}
  \meshline{144,144,144}{0.331276449400}{0.433984662442}{0.324389418396}{0.431224988764}
  \meshline{144,144,144}{0.324389418396}{0.431224988764}{0.306522216024}{0.423297693523}
  \meshline{144,144,144}{0.394226124322}{0.355970484951}{0.402998503329}{0.367548372187}
  \meshline{144,144,144}{0.345117584243}{0.385653630738}{0.345555363775}{0.386024726315}
  \meshline{144,144,144}{0.385883311911}{0.345356819427}{0.375084606509}{0.330087070167}
  \meshline{144,144,144}{0.375084606509}{0.330087070167}{0.374545832058}{0.329409497542}
  \meshline{144,144,144}{0.344665468820}{0.385280801801}{0.345117584243}{0.385653630738}
  \meshline{144,144,144}{0.328484496943}{0.373188086542}{0.344665468820}{0.385280801801}
  \meshline{144,144,144}{0.363570111131}{0.313144282837}{0.373851568665}{0.328520794538}
  \meshline{144,144,144}{0.418139583169}{0.291923756262}{0.416179805437}{0.285302709534}
  \meshline{144,144,144}{0.457059632303}{0.708468119039}{0.457487980288}{0.723313249937}
  \meshline{144,144,144}{0.464968737960}{0.972408532216}{0.463636298700}{0.972599663106}
  \meshline{144,144,144}{0.479684175811}{0.970375636139}{0.483400002904}{0.970022271530}
  \meshline{144,144,144}{0.471083185890}{0.971473121344}{0.464968737960}{0.972408532216}
  \meshline{144,144,144}{0.479684175811}{0.970375636139}{0.471083185890}{0.971473121344}
  \meshline{144,144,144}{0.447587993730}{0.766496565406}{0.450006849143}{0.759797153015}
  \meshline{144,144,144}{0.418447650221}{0.806939304814}{0.432474994917}{0.791765621865}
  \meshline{144,144,144}{0.437189719891}{0.784867859657}{0.441415703703}{0.778627860993}
  \meshline{144,144,144}{0.476593070444}{0.829344325869}{0.466757846330}{0.839625228362}
  \meshline{144,144,144}{0.490259145200}{0.811728158975}{0.483472175681}{0.821537384310}
  \meshline{144,144,144}{0.341755965344}{0.276124335930}{0.344475250344}{0.281970181264}
  \meshline{144,144,144}{0.412024867067}{0.266274047874}{0.413747919344}{0.274307480304}
  \meshline{144,144,144}{0.412024867067}{0.266274047874}{0.410666576394}{0.256829771168}
  \meshline{144,144,144}{0.412647897548}{0.199300927379}{0.411967907420}{0.202596631771}
  \meshline{144,144,144}{0.418155176221}{0.181233652828}{0.412647897548}{0.199300927379}
  \meshline{144,144,144}{0.491962753703}{0.229060490893}{0.497397188749}{0.212030251550}
  \meshline{144,144,144}{0.491552100721}{0.230208391506}{0.491962753703}{0.229060490893}
  \meshline{144,144,144}{0.488264003915}{0.245238558984}{0.487315873339}{0.261483568650}
  \meshline{144,144,144}{0.488264003915}{0.245238558984}{0.491444485092}{0.230799302307}
  \meshline{144,144,144}{0.301388373407}{0.490382142024}{0.295980474813}{0.489586043550}
  \meshline{144,144,144}{0.310102455383}{0.361253156104}{0.308873396979}{0.360622846542}
  \meshline{144,144,144}{0.311440000336}{0.362039067054}{0.310102455383}{0.361253156104}
  \meshline{144,144,144}{0.289652435954}{0.417713364445}{0.295968030298}{0.419916907235}
  \meshline{144,144,144}{0.355784895727}{0.301206339855}{0.353306176789}{0.296683789662}
  \meshline{144,144,144}{0.353306176789}{0.296683789662}{0.344475250344}{0.281970181264}
  \meshline{144,144,144}{0.363570111131}{0.313144282837}{0.355784895727}{0.301206339855}
  \meshline{144,144,144}{0.341755965344}{0.276124335930}{0.336116283438}{0.264211690299}
  \meshline{144,144,144}{0.411599233797}{0.205611339009}{0.409091992561}{0.221026519019}
  \meshline{144,144,144}{0.409091992561}{0.221026519019}{0.409328505196}{0.236562402706}
  \meshline{144,144,144}{0.411599233797}{0.205611339009}{0.411967907420}{0.202596631771}
  \meshline{144,144,144}{0.327274939790}{0.244558416548}{0.320080127128}{0.220233470330}
  \meshline{144,144,144}{0.443311528353}{0.774852064773}{0.441415703703}{0.778627860993}
  \meshline{144,144,144}{0.452576575250}{0.752134747351}{0.450006849143}{0.759797153015}
  \meshline{144,144,144}{0.432474994917}{0.791765621865}{0.437189719891}{0.784867859657}
  \meshline{144,144,144}{0.328469884543}{0.980316256148}{0.330300266823}{0.980270254226}
  \meshline{144,144,144}{0.228850274674}{0.770463417553}{0.227876542141}{0.769546212789}
  \meshline{144,144,144}{0.281807240696}{0.845232067334}{0.296542669804}{0.846962417137}
  \meshline{144,144,144}{0.370377811977}{0.941708961915}{0.365043937357}{0.942406981367}
  \meshline{144,144,144}{0.342370828987}{0.892160116595}{0.345446661405}{0.891697046405}
  \meshline{144,144,144}{0.375880778291}{0.886218460020}{0.383744839155}{0.884223828717}
  \meshline{144,144,144}{0.353855937149}{0.890205617674}{0.368983171143}{0.887804719966}
  \meshline{144,144,144}{0.483472175681}{0.821537384310}{0.478414470303}{0.827341329489}
  \meshline{144,144,144}{0.476593070444}{0.829344325869}{0.478414470303}{0.827341329489}
  \meshline{144,144,144}{0.409078379197}{0.239841896300}{0.409231676795}{0.242434686062}
  \meshline{144,144,144}{0.397180384073}{0.880002855949}{0.383744839155}{0.884223828717}
  \meshline{144,144,144}{0.348507905108}{0.943601262688}{0.347777173770}{0.943621216932}
  \meshline{144,144,144}{0.353855937149}{0.890205617674}{0.345446661405}{0.891697046405}
  \meshline{144,144,144}{0.279315100516}{0.487430487476}{0.273560766001}{0.487028779599}
  \meshline{144,144,144}{0.269734458296}{0.412389135534}{0.279479419614}{0.414941770285}
  \meshline{144,144,144}{0.269734458296}{0.412389135534}{0.261129727723}{0.411083182189}
  \meshline{144,144,144}{0.295968030298}{0.419916907235}{0.306522216024}{0.423297693523}
  \meshline{144,144,144}{0.279479419614}{0.414941770285}{0.289652435954}{0.417713364445}
  \meshline{144,144,144}{0.214789602511}{0.318432023110}{0.203000359408}{0.316610053384}
  \meshline{144,144,144}{0.328484496943}{0.373188086542}{0.311440000336}{0.362039067054}
  \meshline{144,144,144}{0.290351687892}{0.348771663148}{0.308873396979}{0.360622846542}
  \meshline{144,144,144}{0.290351687892}{0.348771663148}{0.287054054747}{0.347256673194}
  \meshline{144,144,144}{0.258626665916}{0.332859352828}{0.260021155492}{0.333764202123}
  \meshline{144,144,144}{0.268037203904}{0.337894482448}{0.260021155492}{0.333764202123}
  \meshline{144,144,144}{0.256825188426}{0.332019491073}{0.258626665916}{0.332859352828}
  \meshline{144,144,144}{0.268037203904}{0.337894482448}{0.287054054747}{0.347256673194}
  \meshline{144,144,144}{0.319618753142}{0.218966608177}{0.319363714272}{0.217334039641}
  \meshline{144,144,144}{0.333044042110}{0.258144947742}{0.334665200662}{0.261633640880}
  \meshline{144,144,144}{0.319791477810}{0.219470948706}{0.320080127128}{0.220233470330}
  \meshline{144,144,144}{0.350774870892}{0.943441259666}{0.365043937357}{0.942406981367}
  \meshline{144,144,144}{0.336116283438}{0.264211690299}{0.334665200662}{0.261633640880}
  \meshline{144,144,144}{0.243719303614}{0.326830868501}{0.256825188426}{0.332019491073}
  \meshline{144,144,144}{0.243719303614}{0.326830868501}{0.234571927299}{0.323585219314}
  \meshline{144,144,144}{0.333044042110}{0.258144947742}{0.327274939790}{0.244558416548}
  \meshline{144,144,144}{0.315772654038}{0.198209470632}{0.319363714272}{0.217334039641}
  \meshline{144,144,144}{0.319791477810}{0.219470948706}{0.319618753142}{0.218966608177}
  \meshline{144,144,144}{0.320726749618}{0.143886887809}{0.319993914284}{0.146983003977}
  \meshline{144,144,144}{0.419419857000}{0.177566166175}{0.422520588950}{0.171332953100}
  \meshline{144,144,144}{0.398792352514}{0.062019642160}{0.395774560026}{0.063334785271}
  \meshline{144,144,144}{0.316244338037}{0.163569710278}{0.315444638551}{0.171804750364}
  \meshline{144,144,144}{0.408614916491}{0.057238654482}{0.422887604040}{0.052223608805}
  \meshline{144,144,144}{0.315796724731}{0.190439432482}{0.315772654038}{0.198209470632}
  \meshline{144,144,144}{0.198938485232}{0.316004547399}{0.178784055596}{0.314914824658}
  \meshline{144,144,144}{0.418155176221}{0.181233652828}{0.419419857000}{0.177566166175}
  \meshline{144,144,144}{0.422520588950}{0.171332953100}{0.427117927561}{0.161302739150}
  \meshline{144,144,144}{0.178784055596}{0.314914824658}{0.176257499419}{0.314880006729}
  \meshline{144,144,144}{0.203000359408}{0.316610053384}{0.198938485232}{0.316004547399}
  \meshline{144,144,144}{0.143977462737}{0.320931399334}{0.157529532440}{0.316950450248}
  \meshline{144,144,144}{0.326333183140}{0.131572847903}{0.330104268947}{0.122241494147}
  \meshline{144,144,144}{0.214789602511}{0.318432023110}{0.222018526070}{0.320649021741}
  \meshline{144,144,144}{0.234571927299}{0.323585219314}{0.222018526070}{0.320649021741}
  \meshline{144,144,144}{0.315796724731}{0.190439432482}{0.314868906864}{0.181509135498}
  \meshline{144,144,144}{0.970303649039}{0.157397675197}{0.971801090589}{0.168394346408}
  \meshline{144,144,144}{0.837268756065}{0.029239410153}{0.852893886425}{0.032317549005}
  \meshline{144,144,144}{0.853843442169}{0.090354311538}{0.853997653317}{0.090437377797}
  \meshline{144,144,144}{0.826141904577}{0.077178675559}{0.829922393380}{0.078611285610}
  \meshline{144,144,144}{0.878635740257}{0.107906296837}{0.872925465886}{0.103109411929}
  \meshline{144,144,144}{0.878635740257}{0.107906296837}{0.888680726961}{0.117678397457}
  \meshline{144,144,144}{0.822688996999}{0.026876378467}{0.812797157678}{0.025776140649}
  \meshline{144,144,144}{0.854372587350}{0.090700880851}{0.872925465886}{0.103109411929}
  \meshline{144,144,144}{0.887244105500}{0.041563277247}{0.898867150263}{0.045315547530}
  \meshline{144,144,144}{0.906314342076}{0.049343024179}{0.898867150263}{0.045315547530}
  \meshline{144,144,144}{0.921386754805}{0.058982391892}{0.919312418664}{0.057300943464}
  \meshline{144,144,144}{0.933041629798}{0.070140621588}{0.938305805638}{0.074831132486}
  \meshline{144,144,144}{0.933041629798}{0.070140621588}{0.921386754805}{0.058982391892}
  \meshline{144,144,144}{0.939153162424}{0.075852009757}{0.940036917370}{0.077451401477}
  \meshline{144,144,144}{0.888680726961}{0.117678397457}{0.899903087794}{0.132035728608}
  \meshline{144,144,144}{0.952467260648}{0.096977547073}{0.954932488711}{0.102066854104}
  \meshline{144,144,144}{0.957959543738}{0.112287402273}{0.954932488711}{0.102066854104}
  \meshline{144,144,144}{0.940036917370}{0.077451401477}{0.952467260648}{0.096977547073}
  \meshline{144,144,144}{0.906314342076}{0.049343024179}{0.919312418664}{0.057300943464}
  \meshline{144,144,144}{0.938305805638}{0.074831132486}{0.939153162424}{0.075852009757}
  \meshline{144,144,144}{0.860429849374}{0.033485563816}{0.858767847236}{0.033315444287}
  \meshline{144,144,144}{0.863086843939}{0.034062842335}{0.877780347792}{0.037893427921}
  \meshline{144,144,144}{0.887244105500}{0.041563277247}{0.877780347792}{0.037893427921}
  \meshline{144,144,144}{0.860429849374}{0.033485563816}{0.863086843939}{0.034062842335}
  \meshline{144,144,144}{0.650245875549}{0.391481434506}{0.662282953501}{0.397996518050}
  \meshline{144,144,144}{0.636369830074}{0.381394129894}{0.650245875549}{0.391481434506}
  \meshline{144,144,144}{0.662282953501}{0.397996518050}{0.665966897510}{0.399699998843}
  \meshline{144,144,144}{0.682840458946}{0.405487412930}{0.672694930904}{0.402017709632}
  \meshline{144,144,144}{0.687971703326}{0.406558582868}{0.682840458946}{0.405487412930}
  \meshline{144,144,144}{0.506168563132}{0.090893219926}{0.506573077590}{0.090734440126}
  \meshline{144,144,144}{0.766603843981}{0.676507734008}{0.773801010422}{0.677943941105}
  \meshline{144,144,144}{0.749611637397}{0.670203393050}{0.756457554690}{0.672886269336}
  \meshline{144,144,144}{0.319188589820}{0.495279144011}{0.301388373407}{0.490382142024}
  \meshline{144,144,144}{0.323482481920}{0.496396261202}{0.325098904078}{0.497065837924}
  \meshline{144,144,144}{0.397443468336}{0.823311874359}{0.384082310886}{0.830815482855}
  \meshline{144,144,144}{0.339660776676}{0.798239195422}{0.339880661738}{0.798173795602}
  \meshline{144,144,144}{0.380381049655}{0.832480820408}{0.369026602504}{0.837153110333}
  \meshline{144,144,144}{0.405762332642}{0.730303026755}{0.407904320467}{0.722041083958}
  \meshline{144,144,144}{0.405703603708}{0.683424490929}{0.407876268856}{0.698016654830}
  \meshline{144,144,144}{0.368696664498}{0.783786749367}{0.376168758663}{0.778666387318}
  \meshline{144,144,144}{0.390464228949}{0.763697649996}{0.399801632368}{0.746494183896}
  \meshline{144,144,144}{0.414754623195}{0.810695339481}{0.399205130542}{0.822066619364}
  \meshline{144,144,144}{0.397443468336}{0.823311874359}{0.399205130542}{0.822066619364}
  \meshline{144,144,144}{0.408785888982}{0.706495589550}{0.408118758119}{0.719618930566}
  \meshline{144,144,144}{0.407904320467}{0.722041083958}{0.408118758119}{0.719618930566}
  \meshline{144,144,144}{0.403592705836}{0.739064269527}{0.405762332642}{0.730303026755}
  \meshline{144,144,144}{0.399801632368}{0.746494183896}{0.402806435061}{0.741144826706}
  \meshline{144,144,144}{0.368696664498}{0.783786749367}{0.359928090471}{0.789583047136}
  \meshline{144,144,144}{0.382758669870}{0.771698568127}{0.390464228949}{0.763697649996}
  \meshline{144,144,144}{0.210304758057}{0.640933047719}{0.217452153405}{0.629246031031}
  \meshline{144,144,144}{0.241649968540}{0.549245070000}{0.235878422595}{0.551570650526}
  \meshline{144,144,144}{0.323482481920}{0.496396261202}{0.319188589820}{0.495279144011}
  \meshline{144,144,144}{0.279315100516}{0.487430487476}{0.295980474813}{0.489586043550}
  \meshline{144,144,144}{0.533728655071}{0.960679378507}{0.519293968437}{0.963488105389}
  \meshline{144,144,144}{0.191567378644}{0.797536554152}{0.195279103993}{0.801608641822}
  \meshline{144,144,144}{0.332971601783}{0.845651407408}{0.322907653333}{0.846926042728}
  \meshline{144,144,144}{0.335971985273}{0.892635608821}{0.342370828987}{0.892160116595}
  \meshline{144,144,144}{0.291097190549}{0.893014584378}{0.290646391677}{0.892988645126}
  \meshline{144,144,144}{0.335971985273}{0.892635608821}{0.321188196817}{0.893698983880}
  \meshline{144,144,144}{0.340685962137}{0.844687881239}{0.338016680096}{0.845058442892}
  \meshline{144,144,144}{0.321188196817}{0.893698983880}{0.315036213816}{0.893678611089}
  \meshline{144,144,144}{0.359187094988}{0.979757921017}{0.365286146930}{0.979528154607}
  \meshline{144,144,144}{0.359187094988}{0.979757921017}{0.349647430871}{0.979939010300}
  \meshline{144,144,144}{0.349647430871}{0.979939010300}{0.330300266823}{0.980270254226}
  \meshline{144,144,144}{0.365286146930}{0.979528154607}{0.380203780515}{0.978927256832}
  \meshline{144,144,144}{0.273406925643}{0.943292680165}{0.282205144886}{0.943959100483}
  \meshline{144,144,144}{0.327724187693}{0.980326381314}{0.328469884543}{0.980316256148}
  \meshline{144,144,144}{0.348507905108}{0.943601262688}{0.350774870892}{0.943441259666}
  \meshline{144,144,144}{0.345138706233}{0.943733909515}{0.328903825598}{0.944588324797}
  \meshline{144,144,144}{0.309696444622}{0.944622957543}{0.304272592056}{0.944680925213}
  \meshline{144,144,144}{0.327724187693}{0.980326381314}{0.325088235205}{0.980324529847}
  \meshline{144,144,144}{0.347777173770}{0.943621216932}{0.345138706233}{0.943733909515}
  \meshline{144,144,144}{0.328903825598}{0.944588324797}{0.309696444622}{0.944622957543}
  \meshline{144,144,144}{0.304034565489}{0.893845996656}{0.291097190549}{0.893014584378}
  \meshline{144,144,144}{0.282148601778}{0.980088781028}{0.281484959451}{0.980088781028}
  \meshline{144,144,144}{0.302746901195}{0.944667168268}{0.287626181651}{0.944132164488}
  \meshline{144,144,144}{0.233396532956}{0.978064570560}{0.224044430662}{0.977728850716}
  \meshline{144,144,144}{0.220659129956}{0.936419632522}{0.228009228692}{0.937767576344}
  \meshline{144,144,144}{0.268415272160}{0.979794046346}{0.278763238907}{0.980020305235}
  \meshline{144,144,144}{0.248135442335}{0.940693614191}{0.253895876163}{0.941557982369}
  \meshline{144,144,144}{0.282148601778}{0.980088781028}{0.300916547317}{0.980370630888}
  \meshline{144,144,144}{0.287626181651}{0.944132164488}{0.282205144886}{0.943959100483}
  \meshline{144,144,144}{0.304073858787}{0.980370630888}{0.300916547317}{0.980370630888}
  \meshline{144,144,144}{0.304272592056}{0.944680925213}{0.302746901195}{0.944667168268}
  \meshline{144,144,144}{0.250587319452}{0.487954641677}{0.250454808820}{0.487963056226}
  \meshline{144,144,144}{0.273560766001}{0.487028779599}{0.250587319452}{0.487954641677}
  \meshline{144,144,144}{0.333316925711}{0.117649484834}{0.331279314266}{0.120177023185}
  \meshline{144,144,144}{0.316244338037}{0.163569710278}{0.319993914284}{0.146983003977}
  \meshline{144,144,144}{0.330104268947}{0.122241494147}{0.331279314266}{0.120177023185}
  \meshline{144,144,144}{0.333316925711}{0.117649484834}{0.343781702424}{0.102321181763}
  \meshline{144,144,144}{0.320726749618}{0.143886887809}{0.326333183140}{0.131572847903}
  \meshline{144,144,144}{0.381574695522}{0.071512604546}{0.380089196347}{0.072320318174}
  \meshline{144,144,144}{0.445997290412}{0.135420982580}{0.440492414436}{0.141153024837}
  \meshline{144,144,144}{0.457357157445}{0.123567380576}{0.445997290412}{0.135420982580}
  \meshline{144,144,144}{0.477004739451}{0.108026503911}{0.470103503573}{0.112372028873}
  \meshline{144,144,144}{0.440492414436}{0.141153024837}{0.436612532986}{0.147095509264}
  \meshline{144,144,144}{0.462981639502}{0.118290159057}{0.457357157445}{0.123567380576}
  \meshline{144,144,144}{0.490836773502}{0.099277314276}{0.506168563132}{0.090893219926}
  \meshline{144,144,144}{0.462981639502}{0.118290159057}{0.470103503573}{0.112372028873}
  \meshline{144,144,144}{0.343781702424}{0.102321181763}{0.352220401978}{0.094247949672}
  \meshline{144,144,144}{0.352220401978}{0.094247949672}{0.354372391377}{0.091942531567}
  \meshline{144,144,144}{0.365749628207}{0.081950011610}{0.379464813773}{0.072798566140}
  \meshline{144,144,144}{0.381574695522}{0.071512604546}{0.395774560026}{0.063334785271}
  \meshline{144,144,144}{0.408614916491}{0.057238654482}{0.401498582187}{0.061097382378}
  \meshline{144,144,144}{0.425312091563}{0.051108455256}{0.422887604040}{0.052223608805}
  \meshline{144,144,144}{0.354372391377}{0.091942531567}{0.365749628207}{0.081950011610}
  \meshline{144,144,144}{0.425312091563}{0.051108455256}{0.441052075080}{0.046055875382}
  \meshline{144,144,144}{0.453363803486}{0.042236837947}{0.445248203076}{0.044384845990}
  \meshline{144,144,144}{0.489079620793}{0.034520356246}{0.474161334096}{0.038075300535}
  \meshline{144,144,144}{0.445248203076}{0.044384845990}{0.441052075080}{0.046055875382}
  \meshline{144,144,144}{0.379464813773}{0.072798566140}{0.380089196347}{0.072320318174}
  \meshline{144,144,144}{0.398792352514}{0.062019642160}{0.401498582187}{0.061097382378}
  \meshline{144,144,144}{0.314868906864}{0.181509135498}{0.315444638551}{0.171804750364}
  \meshline{144,144,144}{0.285080516536}{0.542688646493}{0.277177330621}{0.542573787326}
  \meshline{144,144,144}{0.297328310573}{0.543313846106}{0.285080516536}{0.542688646493}
  \meshline{144,144,144}{0.277177330621}{0.542573787326}{0.267524004108}{0.543727746387}
  \meshline{144,144,144}{0.312645311125}{0.545719676238}{0.317184880424}{0.547012079022}
  \meshline{144,144,144}{0.326059944922}{0.549209986356}{0.317184880424}{0.547012079022}
  \meshline{144,144,144}{0.250347526713}{0.487986742418}{0.250070435893}{0.488054058173}
  \meshline{144,144,144}{0.244072553671}{0.409396120889}{0.244059495773}{0.409395396293}
  \meshline{144,144,144}{0.250347526713}{0.487986742418}{0.250454808820}{0.487963056226}
  \meshline{144,144,144}{0.261129727723}{0.411083182189}{0.244072553671}{0.409396120889}
  \meshline{144,144,144}{0.275541619538}{0.593337028835}{0.263177451422}{0.595695534341}
  \meshline{144,144,144}{0.275541619538}{0.593337028835}{0.286183870883}{0.591260099298}
  \meshline{144,144,144}{0.307753834965}{0.544856957606}{0.297328310573}{0.543313846106}
  \meshline{144,144,144}{0.267524004108}{0.543727746387}{0.261104409159}{0.544342506469}
  \meshline{144,144,144}{0.244785346253}{0.604002558868}{0.241296129226}{0.606230023182}
  \meshline{144,144,144}{0.251853897081}{0.546734450585}{0.261104409159}{0.544342506469}
  \meshline{144,144,144}{0.251853897081}{0.546734450585}{0.241649968540}{0.549245070000}
  \meshline{144,144,144}{0.198517839000}{0.503653324752}{0.184905995120}{0.512141032191}
  \meshline{144,144,144}{0.205382097629}{0.499954095221}{0.198517839000}{0.503653324752}
  \meshline{144,144,144}{0.137411644951}{0.564736084277}{0.140144818868}{0.559533184522}
  \meshline{144,144,144}{0.235878422595}{0.551570650526}{0.227930694922}{0.555378022200}
  \meshline{144,144,144}{0.210695213787}{0.565908093123}{0.199888212200}{0.574630378523}
  \meshline{144,144,144}{0.219468015511}{0.494551306239}{0.214615909477}{0.496589411679}
  \meshline{144,144,144}{0.227930694922}{0.555378022200}{0.218053247946}{0.560401848678}
  \meshline{144,144,144}{0.183971538597}{0.512764338866}{0.181185040320}{0.515143910006}
  \meshline{144,144,144}{0.219468015511}{0.494551306239}{0.229410843309}{0.491816039896}
  \meshline{144,144,144}{0.229410843309}{0.491816039896}{0.250070435893}{0.488054058173}
  \meshline{144,144,144}{0.217452153405}{0.629246031031}{0.224992113977}{0.620083488733}
  \meshline{144,144,144}{0.244785346253}{0.604002558868}{0.259614758622}{0.596769055423}
  \meshline{144,144,144}{0.205382097629}{0.499954095221}{0.214615909477}{0.496589411679}
  \meshline{144,144,144}{0.183971538597}{0.512764338866}{0.184905995120}{0.512141032191}
  \meshline{144,144,144}{0.382758669870}{0.771698568127}{0.376168758663}{0.778666387318}
  \meshline{144,144,144}{0.288440200229}{0.801081726968}{0.303352272578}{0.802134094287}
  \meshline{144,144,144}{0.207355885404}{0.739567905936}{0.209173193296}{0.743334205438}
  \meshline{144,144,144}{0.198821574441}{0.676231334657}{0.197379162348}{0.692121904921}
  \meshline{144,144,144}{0.241296129226}{0.606230023182}{0.228802445080}{0.616101788645}
  \meshline{144,144,144}{0.198421510630}{0.706727759601}{0.199119502362}{0.711675869044}
  \meshline{144,144,144}{0.205819539261}{0.649658387247}{0.201460638815}{0.663226180916}
  \meshline{144,144,144}{0.205819539261}{0.649658387247}{0.210304758057}{0.640933047719}
  \meshline{144,144,144}{0.160378556659}{0.741300549129}{0.163072514411}{0.749808847391}
  \meshline{144,144,144}{0.228802445080}{0.616101788645}{0.224992113977}{0.620083488733}
  \meshline{144,144,144}{0.168099638033}{0.618893216734}{0.164986103030}{0.625556671026}
  \meshline{144,144,144}{0.185142733441}{0.590163400078}{0.180430902695}{0.597026574434}
  \meshline{144,144,144}{0.180430902695}{0.597026574434}{0.172616461805}{0.609672585683}
  \meshline{144,144,144}{0.199119502362}{0.711675869044}{0.201254465612}{0.718737835175}
  \meshline{144,144,144}{0.201254465612}{0.718737835175}{0.207355885404}{0.739567905936}
  \meshline{144,144,144}{0.211092879882}{0.746125792060}{0.224340577007}{0.764563614264}
  \meshline{144,144,144}{0.195279103993}{0.801608641822}{0.209154010044}{0.814235393402}
  \meshline{144,144,144}{0.151800331460}{0.828850735963}{0.161475800538}{0.839230816940}
  \meshline{144,144,144}{0.224340577007}{0.764563614264}{0.227876542141}{0.769546212789}
  \meshline{144,144,144}{0.211092879882}{0.746125792060}{0.209173193296}{0.743334205438}
  \meshline{144,144,144}{0.243845341721}{0.782803455766}{0.228850274674}{0.770463417553}
  \meshline{144,144,144}{0.171032504563}{0.767461585949}{0.167105213077}{0.759643002396}
  \meshline{144,144,144}{0.163072514411}{0.749808847391}{0.167105213077}{0.759643002396}
  \meshline{144,144,144}{0.198421510630}{0.706727759601}{0.197320871928}{0.695772760110}
  \meshline{144,144,144}{0.156382055469}{0.726433115343}{0.157693753402}{0.732735561604}
  \meshline{144,144,144}{0.177124477171}{0.778260471240}{0.171032504563}{0.767461585949}
  \meshline{144,144,144}{0.045249869362}{0.898139338816}{0.048893213698}{0.904569902455}
  \meshline{144,144,144}{0.177124477171}{0.778260471240}{0.183466886096}{0.787910487856}
  \meshline{144,144,144}{0.191567378644}{0.797536554152}{0.183466886096}{0.787910487856}
  \meshline{144,144,144}{0.185142733441}{0.590163400078}{0.192574324946}{0.581653083795}
  \meshline{144,144,144}{0.119087089855}{0.604830843647}{0.116809010351}{0.612317146729}
  \meshline{144,144,144}{0.210695213787}{0.565908093123}{0.218053247946}{0.560401848678}
  \meshline{144,144,144}{0.199888212200}{0.574630378523}{0.192574324946}{0.581653083795}
  \meshline{144,144,144}{0.181185040320}{0.515143910006}{0.168808632644}{0.524994674875}
  \meshline{144,144,144}{0.168808632644}{0.524994674875}{0.165526878956}{0.527837314664}
  \meshline{144,144,144}{0.280074378832}{0.845021786981}{0.271807671298}{0.843095585617}
  \meshline{144,144,144}{0.243845341721}{0.782803455766}{0.253212494566}{0.788512863287}
  \meshline{144,144,144}{0.152624273316}{0.687511825396}{0.152768674170}{0.690724118067}
  \meshline{144,144,144}{0.157693753402}{0.732735561604}{0.160378556659}{0.741300549129}
  \meshline{144,144,144}{0.152742715016}{0.685358162300}{0.152624273316}{0.687511825396}
  \meshline{144,144,144}{0.197320871928}{0.695772760110}{0.197379162348}{0.692121904921}
  \meshline{144,144,144}{0.153776500548}{0.668732050431}{0.152742715016}{0.685358162300}
  \meshline{144,144,144}{0.156691141413}{0.653014653383}{0.153776500548}{0.668732050431}
  \meshline{144,144,144}{0.200028903547}{0.668096510747}{0.198821574441}{0.676231334657}
  \meshline{144,144,144}{0.152768674170}{0.690724118067}{0.153194984029}{0.705449540042}
  \meshline{144,144,144}{0.164986103030}{0.625556671026}{0.164022596795}{0.627826713398}
  \meshline{144,144,144}{0.109178082920}{0.728685916077}{0.112200257445}{0.745444985119}
  \meshline{144,144,144}{0.164022596795}{0.627826713398}{0.161200709810}{0.636872465783}
  \meshline{144,144,144}{0.200028903547}{0.668096510747}{0.201460638815}{0.663226180916}
  \meshline{144,144,144}{0.153918190875}{0.712033952487}{0.156382055469}{0.726433115343}
  \meshline{144,144,144}{0.153918190875}{0.712033952487}{0.153194984029}{0.705449540042}
  \meshline{144,144,144}{0.107698866685}{0.714201541256}{0.106325252232}{0.698396840550}
  \meshline{144,144,144}{0.019653256469}{0.681406520123}{0.019690309345}{0.702810806195}
  \meshline{144,144,144}{0.106349891298}{0.678284117574}{0.106559938349}{0.675217002149}
  \meshline{144,144,144}{0.157972589057}{0.646690410409}{0.161200709810}{0.636872465783}
  \meshline{144,144,144}{0.113804078803}{0.752428810808}{0.112200257445}{0.745444985119}
  \meshline{144,144,144}{0.106349891298}{0.678284117574}{0.106402765402}{0.683251669842}
  \meshline{144,144,144}{0.108712520944}{0.651148278025}{0.109135449236}{0.648483579325}
  \meshline{144,144,144}{0.108712520944}{0.651148278025}{0.106559938349}{0.675217002149}
  \meshline{144,144,144}{0.111477047608}{0.634162243611}{0.109135449236}{0.648483579325}
  \meshline{144,144,144}{0.107698866685}{0.714201541256}{0.108339544035}{0.723210138914}
  \meshline{144,144,144}{0.106402765402}{0.683251669842}{0.106325252232}{0.698396840550}
  \meshline{144,144,144}{0.055312407775}{0.682539507860}{0.055301513200}{0.679703373532}
  \meshline{144,144,144}{0.156691141413}{0.653014653383}{0.157972589057}{0.646690410409}
  \meshline{144,144,144}{0.056144850208}{0.719442039562}{0.057349264404}{0.732638241683}
  \meshline{144,144,144}{0.057185850391}{0.640219553837}{0.058811827169}{0.624325246139}
  \meshline{144,144,144}{0.055859922174}{0.660545296142}{0.056256285447}{0.652691255077}
  \meshline{144,144,144}{0.113030930579}{0.628323431188}{0.114979629561}{0.619294400455}
  \meshline{144,144,144}{0.058811827169}{0.624325246139}{0.059174493475}{0.621250324147}
  \meshline{144,144,144}{0.065749187800}{0.582176655260}{0.066342501897}{0.578367325047}
  \meshline{144,144,144}{0.057185850391}{0.640219553837}{0.056256285447}{0.652691255077}
  \meshline{144,144,144}{0.065749187800}{0.582176655260}{0.062327415279}{0.598509639596}
  \meshline{144,144,144}{0.019798906204}{0.662360118593}{0.019661613524}{0.676116868538}
  \meshline{144,144,144}{0.078124117563}{0.828406207591}{0.072754426337}{0.812255688333}
  \meshline{144,144,144}{0.108339544035}{0.723210138914}{0.109178082920}{0.728685916077}
  \meshline{144,144,144}{0.113804078803}{0.752428810808}{0.116727183804}{0.761869696125}
  \meshline{144,144,144}{0.146941701136}{0.822121749251}{0.151800331460}{0.828850735963}
  \meshline{144,144,144}{0.019690309345}{0.702810806195}{0.019890478864}{0.712730777362}
  \meshline{144,144,144}{0.055312407775}{0.682539507860}{0.055310873930}{0.696737461414}
  \meshline{144,144,144}{0.055859922174}{0.660545296142}{0.055335520451}{0.677900020746}
  \meshline{144,144,144}{0.019642381443}{0.678182777870}{0.019653256469}{0.681406520123}
  \meshline{144,144,144}{0.055634045463}{0.707815866419}{0.055310873930}{0.696737461414}
  \meshline{144,144,144}{0.056144850208}{0.719442039562}{0.055634045463}{0.707815866419}
  \meshline{144,144,144}{0.019971552781}{0.721070656128}{0.019971552781}{0.719093847402}
  \meshline{144,144,144}{0.020176323021}{0.647098748042}{0.020123014629}{0.649880491368}
  \meshline{144,144,144}{0.061311244755}{0.766350660219}{0.060686882517}{0.762350805188}
  \meshline{144,144,144}{0.057349264404}{0.732638241683}{0.057704581455}{0.738704815776}
  \meshline{144,144,144}{0.020176323021}{0.646215612000}{0.020176323021}{0.645332475957}
  \meshline{144,144,144}{0.059035599215}{0.749962984831}{0.057704581455}{0.738704815776}
  \meshline{144,144,144}{0.023514347204}{0.788674630105}{0.023624282062}{0.790403018709}
  \meshline{144,144,144}{0.059035599215}{0.749962984831}{0.060686882517}{0.762350805188}
  \meshline{144,144,144}{0.020176323021}{0.645332475957}{0.020694510447}{0.627042466719}
  \meshline{144,144,144}{0.020176323021}{0.647098748042}{0.020176323021}{0.646215612000}
  \meshline{144,144,144}{0.118450828670}{0.768073609170}{0.116727183804}{0.761869696125}
  \meshline{144,144,144}{0.061311244755}{0.766350660219}{0.062358353822}{0.770677989258}
  \meshline{144,144,144}{0.122921486780}{0.779867206785}{0.124821526838}{0.784409158017}
  \meshline{144,144,144}{0.139345000670}{0.811895062996}{0.146941701136}{0.822121749251}
  \meshline{144,144,144}{0.020471747167}{0.735868416708}{0.020683841836}{0.742238767861}
  \meshline{144,144,144}{0.020471747167}{0.735868416708}{0.019971552781}{0.721070656128}
  \meshline{144,144,144}{0.020788938031}{0.743670328266}{0.020683841836}{0.742238767861}
  \meshline{144,144,144}{0.023624282062}{0.790887491027}{0.024809748558}{0.806583688231}
  \meshline{144,144,144}{0.021962545028}{0.767411712882}{0.023514347204}{0.788674630105}
  \meshline{144,144,144}{0.062358353822}{0.770677989258}{0.064876453885}{0.784312117308}
  \meshline{144,144,144}{0.122921486780}{0.779867206785}{0.118450828670}{0.768073609170}
  \meshline{144,144,144}{0.133335721487}{0.802069626248}{0.139345000670}{0.811895062996}
  \meshline{144,144,144}{0.019971552781}{0.719093847402}{0.019890478864}{0.712730777362}
  \meshline{144,144,144}{0.233375397843}{0.829680013069}{0.237138537669}{0.831690979072}
  \meshline{144,144,144}{0.221768478944}{0.823409885318}{0.233375397843}{0.829680013069}
  \meshline{144,144,144}{0.209154010044}{0.814235393402}{0.209640619189}{0.814594054523}
  \meshline{144,144,144}{0.259332768611}{0.791954944195}{0.253212494566}{0.788512863287}
  \meshline{144,144,144}{0.215248501552}{0.875167285849}{0.208477891066}{0.872167805352}
  \meshline{144,144,144}{0.221768478944}{0.823409885318}{0.209640619189}{0.814594054523}
  \meshline{144,144,144}{0.188199407288}{0.860968899368}{0.182498750569}{0.856853911558}
  \meshline{144,144,144}{0.312843973635}{0.802744642204}{0.303352272578}{0.802134094287}
  \meshline{144,144,144}{0.305285775014}{0.847436370720}{0.319808820646}{0.847099808667}
  \meshline{144,144,144}{0.237138537669}{0.831690979072}{0.251670022282}{0.837270061787}
  \meshline{144,144,144}{0.259332768611}{0.791954944195}{0.268750132994}{0.795420573587}
  \meshline{144,144,144}{0.261016548367}{0.840691800435}{0.271807671298}{0.843095585617}
  \meshline{144,144,144}{0.261016548367}{0.840691800435}{0.259008497205}{0.840146042375}
  \meshline{144,144,144}{0.259008497205}{0.840146042375}{0.251670022282}{0.837270061787}
  \meshline{144,144,144}{0.171165902525}{0.848312131706}{0.182498750569}{0.856853911558}
  \meshline{144,144,144}{0.161475800538}{0.839230816940}{0.166493175556}{0.844568337490}
  \meshline{144,144,144}{0.171165902525}{0.848312131706}{0.166493175556}{0.844568337490}
  \meshline{144,144,144}{0.070149426618}{0.804956153043}{0.072754426337}{0.812255688333}
  \meshline{144,144,144}{0.202446028874}{0.868709710180}{0.208477891066}{0.872167805352}
  \meshline{144,144,144}{0.202446028874}{0.868709710180}{0.188199407288}{0.860968899368}
  \meshline{144,144,144}{0.066342501897}{0.578367325047}{0.067746674571}{0.572369538505}
  \meshline{144,144,144}{0.061598709591}{0.604139856107}{0.062327415279}{0.598509639596}
  \meshline{144,144,144}{0.061598709591}{0.604139856107}{0.059978930628}{0.616184894506}
  \meshline{144,144,144}{0.021441300336}{0.610979840479}{0.021234894745}{0.614452417881}
  \meshline{144,144,144}{0.071809898319}{0.555707623210}{0.067746674571}{0.572369538505}
  \meshline{144,144,144}{0.022682417683}{0.589962558837}{0.022182906461}{0.599279190687}
  \meshline{144,144,144}{0.024305569403}{0.569581313803}{0.022682417683}{0.588779069289}
  \meshline{144,144,144}{0.025699965924}{0.554548548966}{0.026510528995}{0.544007766587}
  \meshline{144,144,144}{0.076281519468}{0.542674731351}{0.071809898319}{0.555707623210}
  \meshline{144,144,144}{0.020694510447}{0.627042466719}{0.021234894745}{0.614452417881}
  \meshline{144,144,144}{0.022182906461}{0.599279190687}{0.021441300336}{0.610979840479}
  \meshline{144,144,144}{0.022682417683}{0.589962558837}{0.022682417683}{0.588779069289}
  \meshline{144,144,144}{0.152904805781}{0.542327912635}{0.165526878956}{0.527837314664}
  \meshline{144,144,144}{0.150933334967}{0.544409265326}{0.152904805781}{0.542327912635}
  \meshline{144,144,144}{0.140144818868}{0.559533184522}{0.147277551933}{0.549646293120}
  \meshline{144,144,144}{0.172616461805}{0.609672585683}{0.170849967743}{0.612734306198}
  \meshline{144,144,144}{0.137411644951}{0.564736084277}{0.131765133632}{0.574485617641}
  \meshline{144,144,144}{0.150933334967}{0.544409265326}{0.147277551933}{0.549646293120}
  \meshline{144,144,144}{0.131765133632}{0.574485617641}{0.126694786915}{0.586218385978}
  \meshline{144,144,144}{0.122725934861}{0.594908888834}{0.126694786915}{0.586218385978}
  \meshline{144,144,144}{0.168099638033}{0.618893216734}{0.170849967743}{0.612734306198}
  \meshline{144,144,144}{0.119087089855}{0.604830843647}{0.122725934861}{0.594908888834}
  \meshline{144,144,144}{0.076281519468}{0.542674731351}{0.077848953723}{0.536879776315}
  \meshline{144,144,144}{0.035303373872}{0.487378205368}{0.032560607348}{0.500388084232}
  \meshline{144,144,144}{0.100613050386}{0.488373786027}{0.100785150339}{0.488006628114}
  \meshline{144,144,144}{0.121359626365}{0.459604285946}{0.120447278805}{0.460745208414}
  \meshline{144,144,144}{0.023624282062}{0.790645254868}{0.023624282062}{0.790403018709}
  \meshline{144,144,144}{0.021604095876}{0.763503210236}{0.021962545028}{0.767411712882}
  \meshline{144,144,144}{0.020788938031}{0.743670328266}{0.021604095876}{0.763503210236}
  \meshline{144,144,144}{0.026652202904}{0.820069812583}{0.026818326396}{0.822819180692}
  \meshline{144,144,144}{0.023624282062}{0.790887491027}{0.023624282062}{0.790645254868}
  \meshline{144,144,144}{0.024809748558}{0.806583688231}{0.026652202904}{0.820069812583}
  \meshline{144,144,144}{0.223356524863}{0.878531619875}{0.236737096567}{0.883050694015}
  \meshline{144,144,144}{0.255333769597}{0.887906004151}{0.259692351826}{0.888933180830}
  \meshline{144,144,144}{0.215248501552}{0.875167285849}{0.223356524863}{0.878531619875}
  \meshline{144,144,144}{0.236737096567}{0.883050694015}{0.237026366237}{0.883133011221}
  \meshline{144,144,144}{0.238058977243}{0.883380696464}{0.237026366237}{0.883133011221}
  \meshline{144,144,144}{0.267636680031}{0.942840615715}{0.273406925643}{0.943292680165}
  \meshline{144,144,144}{0.253895876163}{0.941557982369}{0.267636680031}{0.942840615715}
  \meshline{144,144,144}{0.210983938426}{0.933977929603}{0.220659129956}{0.936419632522}
  \meshline{144,144,144}{0.238058977243}{0.883380696464}{0.255333769597}{0.887906004151}
  \meshline{144,144,144}{0.259692351826}{0.888933180830}{0.269728530583}{0.890496477384}
  \meshline{144,144,144}{0.274507757192}{0.891276167386}{0.269728530583}{0.890496477384}
  \meshline{144,144,144}{0.274507757192}{0.891276167386}{0.287840857715}{0.892669647687}
  \meshline{144,144,144}{0.248135442335}{0.940693614191}{0.238716398779}{0.939648469724}
  \meshline{144,144,144}{0.113030930579}{0.628323431188}{0.111477047608}{0.634162243611}
  \meshline{144,144,144}{0.116809010351}{0.612317146729}{0.114979629561}{0.619294400455}
  \meshline{144,144,144}{0.032560607348}{0.500388084232}{0.030339562897}{0.513162697130}
  \meshline{144,144,144}{0.098646319606}{0.492084587478}{0.091837335944}{0.504172422374}
  \meshline{144,144,144}{0.084126542132}{0.521189645974}{0.080887712720}{0.529076965724}
  \meshline{144,144,144}{0.077848953723}{0.536879776315}{0.080887712720}{0.529076965724}
  \meshline{144,144,144}{0.084126542132}{0.521189645974}{0.091837335944}{0.504172422374}
  \meshline{144,144,144}{0.069353409671}{0.802553712466}{0.064876453885}{0.784312117308}
  \meshline{144,144,144}{0.078124117563}{0.828406207591}{0.078961050576}{0.830996762816}
  \meshline{144,144,144}{0.069713873135}{0.803839740446}{0.070149426618}{0.804956153043}
  \meshline{144,144,144}{0.129153135888}{0.794583026578}{0.124821526838}{0.784409158017}
  \meshline{144,144,144}{0.133335721487}{0.802069626248}{0.129153135888}{0.794583026578}
  \meshline{144,144,144}{0.078961050576}{0.830996762816}{0.080106841321}{0.833657967439}
  \meshline{144,144,144}{0.191023408364}{0.928813386588}{0.201083841902}{0.931740111616}
  \meshline{144,144,144}{0.158612675489}{0.969667561482}{0.145350638897}{0.967921449369}
  \meshline{144,144,144}{0.027318208751}{0.539563409110}{0.026510528995}{0.544007766587}
  \meshline{144,144,144}{0.028433758834}{0.530844061543}{0.027318208751}{0.539563409110}
  \meshline{144,144,144}{0.037308371129}{0.474164451483}{0.036422353846}{0.479235610019}
  \meshline{144,144,144}{0.029258235405}{0.521331247733}{0.028433758834}{0.530844061543}
  \meshline{144,144,144}{0.029258235405}{0.521331247733}{0.030339562897}{0.513162697130}
  \meshline{144,144,144}{0.110254744185}{0.473107116293}{0.101068842408}{0.487547060291}
  \meshline{144,144,144}{0.110254744185}{0.473107116293}{0.120447278805}{0.460745208414}
  \meshline{144,144,144}{0.098646319606}{0.492084587478}{0.100613050386}{0.488373786027}
  \meshline{144,144,144}{0.037308371129}{0.474164451483}{0.039318547588}{0.465816283651}
  \meshline{144,144,144}{0.035303373872}{0.487378205368}{0.036422353846}{0.479235610019}
  \meshline{144,144,144}{0.041772968455}{0.456970931654}{0.039318547588}{0.465816283651}
  \meshline{144,144,144}{0.100785150339}{0.488006628114}{0.101068842408}{0.487547060291}
  \meshline{144,144,144}{0.045782785879}{0.441535138280}{0.042901740002}{0.451605365092}
  \meshline{144,144,144}{0.055076258766}{0.415533696912}{0.056671803060}{0.410385720919}
  \meshline{144,144,144}{0.096603833203}{0.863826592775}{0.100508861875}{0.868398990825}
  \meshline{144,144,144}{0.095445398578}{0.862188004489}{0.093923566212}{0.859377642912}
  \meshline{144,144,144}{0.108953573633}{0.879991095657}{0.100508861875}{0.868398990825}
  \meshline{144,144,144}{0.095445398578}{0.862188004489}{0.096603833203}{0.863826592775}
  \meshline{144,144,144}{0.115562303386}{0.886406708090}{0.126029681483}{0.895879108843}
  \meshline{144,144,144}{0.093923566212}{0.859377642912}{0.085438896135}{0.845231765452}
  \meshline{144,144,144}{0.157297108227}{0.915597687057}{0.141619444055}{0.906770955414}
  \meshline{144,144,144}{0.116787781908}{0.960230470968}{0.099997354073}{0.954066363639}
  \meshline{144,144,144}{0.137007617660}{0.903637325204}{0.141619444055}{0.906770955414}
  \meshline{144,144,144}{0.126029681483}{0.895879108843}{0.137007617660}{0.903637325204}
  \meshline{144,144,144}{0.037127650473}{0.875853628053}{0.040809910237}{0.886062088481}
  \meshline{144,144,144}{0.027547343100}{0.828231881321}{0.030356824794}{0.844307327437}
  \meshline{144,144,144}{0.045249869362}{0.898139338816}{0.040809910237}{0.886062088481}
  \meshline{144,144,144}{0.033197939931}{0.860538851661}{0.035847620565}{0.868748265070}
  \meshline{144,144,144}{0.108953573633}{0.879991095657}{0.115562303386}{0.886406708090}
  \meshline{144,144,144}{0.055128262573}{0.915958079312}{0.065102594013}{0.928921493651}
  \meshline{144,144,144}{0.037127650473}{0.875853628053}{0.035847620565}{0.868748265070}
  \meshline{144,144,144}{0.067985789005}{0.932643134108}{0.079357267520}{0.940995271224}
  \meshline{144,144,144}{0.087172029392}{0.947086900514}{0.099997354073}{0.954066363639}
  \meshline{144,144,144}{0.055128262573}{0.915958079312}{0.052693021488}{0.912405827444}
  \meshline{144,144,144}{0.079357267520}{0.940995271224}{0.084376416739}{0.945384858784}
  \meshline{144,144,144}{0.052693021488}{0.912405827444}{0.048893213698}{0.904569902455}
  \meshline{144,144,144}{0.158758596016}{0.916314798207}{0.157297108227}{0.915597687057}
  \meshline{144,144,144}{0.025699965924}{0.554548548966}{0.024500542199}{0.564444250233}
  \meshline{144,144,144}{0.062988394723}{0.397622511351}{0.056671803060}{0.410385720919}
  \meshline{144,144,144}{0.173078425541}{0.315425255793}{0.176257499419}{0.314880006729}
  \meshline{144,144,144}{0.116109814536}{0.333834409206}{0.118430080733}{0.332576780550}
  \meshline{144,144,144}{0.173078425541}{0.315425255793}{0.157529532440}{0.316950450248}
  \meshline{144,144,144}{0.045782785879}{0.441535138280}{0.049622078417}{0.430283035943}
  \meshline{144,144,144}{0.042901740002}{0.451605365092}{0.041772968455}{0.456970931654}
  \meshline{144,144,144}{0.049622078417}{0.430283035943}{0.050262496233}{0.427836239679}
  \meshline{144,144,144}{0.080106841321}{0.833657967439}{0.085438896135}{0.845231765452}
  \meshline{144,144,144}{0.175535073636}{0.923674953465}{0.184089223084}{0.926866190017}
  \meshline{144,144,144}{0.030356824794}{0.844307327437}{0.033197939931}{0.860538851661}
  \meshline{144,144,144}{0.067985789005}{0.932643134108}{0.065102594013}{0.928921493651}
  \meshline{144,144,144}{0.119722736138}{0.960948283278}{0.140673142019}{0.966501285352}
  \meshline{144,144,144}{0.119722736138}{0.960948283278}{0.118372616405}{0.960653119230}
  \meshline{144,144,144}{0.206285602182}{0.933117279108}{0.201083841902}{0.931740111616}
  \meshline{144,144,144}{0.184101177950}{0.973946818914}{0.170727433501}{0.972445737008}
  \meshline{144,144,144}{0.116787781908}{0.960230470968}{0.117878154389}{0.960576479024}
  \meshline{144,144,144}{0.145350638897}{0.967921449369}{0.140673142019}{0.966501285352}
  \meshline{144,144,144}{0.118372616405}{0.960653119230}{0.117878154389}{0.960576479024}
  \meshline{144,144,144}{0.184089223084}{0.926866190017}{0.191023408364}{0.928813386588}
  \meshline{144,144,144}{0.206285602182}{0.933117279108}{0.210983938426}{0.933977929603}
  \meshline{144,144,144}{0.024305569403}{0.569581313803}{0.024500542199}{0.564444250233}
  \meshline{144,144,144}{0.196927100958}{0.412817911882}{0.183709793257}{0.417314903480}
  \meshline{144,144,144}{0.161579681099}{0.426635907361}{0.168338544490}{0.423093972617}
  \meshline{144,144,144}{0.168338544490}{0.423093972617}{0.178136100506}{0.419109262145}
  \meshline{144,144,144}{0.152315696022}{0.432841053438}{0.150683740708}{0.434056720502}
  \meshline{144,144,144}{0.122183475507}{0.458845400443}{0.121359626365}{0.459604285946}
  \meshline{144,144,144}{0.150683740708}{0.434056720502}{0.138331666172}{0.442867996592}
  \meshline{144,144,144}{0.122183475507}{0.458845400443}{0.138331666172}{0.442867996592}
  \meshline{144,144,144}{0.161579681099}{0.426635907361}{0.152315696022}{0.432841053438}
  \meshline{144,144,144}{0.178136100506}{0.419109262145}{0.183709793257}{0.417314903480}
  \meshline{144,144,144}{0.196927100958}{0.412817911882}{0.211689063205}{0.410492573638}
  \meshline{144,144,144}{0.211689063205}{0.410492573638}{0.217554623940}{0.409480843722}
  \meshline{144,144,144}{0.217554623940}{0.409480843722}{0.243978422763}{0.409397523437}
  \meshline{144,144,144}{0.244059495773}{0.409395396293}{0.243978422763}{0.409397523437}
  \meshline{144,144,144}{0.027547343100}{0.828231881321}{0.026818326396}{0.822819180692}
  \meshline{144,144,144}{0.184101177950}{0.973946818914}{0.190614352631}{0.974826537360}
  \meshline{144,144,144}{0.158612675489}{0.969667561482}{0.166091087979}{0.971395249205}
  \meshline{144,144,144}{0.159865048443}{0.916703445600}{0.175535073636}{0.923674953465}
  \meshline{144,144,144}{0.159865048443}{0.916703445600}{0.158758596016}{0.916314798207}
  \meshline{144,144,144}{0.166091087979}{0.971395249205}{0.170727433501}{0.972445737008}
  \meshline{144,144,144}{0.339880661738}{0.798173795602}{0.340277061372}{0.798000803802}
  \meshline{144,144,144}{0.315525470595}{0.802512562826}{0.312843973635}{0.802744642204}
  \meshline{144,144,144}{0.340685962137}{0.844687881239}{0.353165337114}{0.842094507587}
  \meshline{144,144,144}{0.322907653333}{0.846926042728}{0.319808820646}{0.847099808667}
  \meshline{144,144,144}{0.287840857715}{0.892669647687}{0.290646391677}{0.892988645126}
  \meshline{144,144,144}{0.304034565489}{0.893845996656}{0.315036213816}{0.893678611089}
  \meshline{144,144,144}{0.338153616236}{0.798502591107}{0.339660776676}{0.798239195422}
  \meshline{144,144,144}{0.359928090471}{0.789583047136}{0.340277061372}{0.798000803802}
  \meshline{144,144,144}{0.338153616236}{0.798502591107}{0.315525470595}{0.802512562826}
  \meshline{144,144,144}{0.380381049655}{0.832480820408}{0.384082310886}{0.830815482855}
  \meshline{144,144,144}{0.363046302474}{0.839156115198}{0.369026602504}{0.837153110333}
  \meshline{144,144,144}{0.353165337114}{0.842094507587}{0.363046302474}{0.839156115198}
  \meshline{144,144,144}{0.296542669804}{0.846962417137}{0.305285775014}{0.847436370720}
  \meshline{144,144,144}{0.280074378832}{0.845021786981}{0.281807240696}{0.845232067334}
  \meshline{144,144,144}{0.283553046537}{0.800013938994}{0.288440200229}{0.801081726968}
  \meshline{144,144,144}{0.268750132994}{0.795420573587}{0.283553046537}{0.800013938994}
  \meshline{144,144,144}{0.203543047171}{0.975729743647}{0.190614352631}{0.974826537360}
  \meshline{144,144,144}{0.453363803486}{0.042236837947}{0.465881884240}{0.039229189321}
  \meshline{144,144,144}{0.465881884240}{0.039229189321}{0.474161334096}{0.038075300535}
  \meshline{144,144,144}{0.492517476554}{0.034145443545}{0.489079620793}{0.034520356246}
  \meshline{144,144,144}{0.506068880826}{0.031547421201}{0.508948331297}{0.031309504435}
  \meshline{144,144,144}{0.019798906204}{0.662360118593}{0.020123014629}{0.649880491368}
  \meshline{144,144,144}{0.019642381443}{0.678182777870}{0.019642381443}{0.677756788784}
  \meshline{144,144,144}{0.019642381443}{0.677756788784}{0.019661613524}{0.676116868538}
  \meshline{144,144,144}{0.055301513200}{0.679703373532}{0.055335520451}{0.677900020746}
  \meshline{144,144,144}{0.069353409671}{0.802553712466}{0.069713873135}{0.803839740446}
  \meshline{144,144,144}{0.140320909301}{0.321903921419}{0.143977462737}{0.320931399334}
  \meshline{144,144,144}{0.087172029392}{0.947086900514}{0.084376416739}{0.945384858784}
  \meshline{144,144,144}{0.245246003941}{0.978870406299}{0.238473320621}{0.978432796135}
  \meshline{144,144,144}{0.203543047171}{0.975729743647}{0.217093700479}{0.977202113016}
  \meshline{144,144,144}{0.224044430662}{0.977728850716}{0.217093700479}{0.977202113016}
  \meshline{144,144,144}{0.238716398779}{0.939648469724}{0.228009228692}{0.937767576344}
  \meshline{144,144,144}{0.278763238907}{0.980020305235}{0.281484959451}{0.980088781028}
  \meshline{144,144,144}{0.268415272160}{0.979794046346}{0.261185102421}{0.979407654773}
  \meshline{144,144,144}{0.245246003941}{0.978870406299}{0.261185102421}{0.979407654773}
  \meshline{144,144,144}{0.233396532956}{0.978064570560}{0.238473320621}{0.978432796135}
  \meshline{144,144,144}{0.074262558815}{0.376476666007}{0.079227993819}{0.370567941575}
  \meshline{144,144,144}{0.114317532149}{0.335351927204}{0.100423290824}{0.345219069233}
  \meshline{144,144,144}{0.086747786645}{0.359261453189}{0.079227993819}{0.370567941575}
  \meshline{144,144,144}{0.094046528238}{0.352539553050}{0.086747786645}{0.359261453189}
  \meshline{144,144,144}{0.094046528238}{0.352539553050}{0.100423290824}{0.345219069233}
  \meshline{144,144,144}{0.064184271465}{0.394428039145}{0.066867308937}{0.389857354691}
  \meshline{144,144,144}{0.074262558815}{0.376476666007}{0.066867308937}{0.389857354691}
  \meshline{144,144,144}{0.064184271465}{0.394428039145}{0.062988394723}{0.397622511351}
  \meshline{144,144,144}{0.055076258766}{0.415533696912}{0.050262496233}{0.427836239679}
  \meshline{144,144,144}{0.118430080733}{0.332576780550}{0.140320909301}{0.321903921419}
  \meshline{144,144,144}{0.114317532149}{0.335351927204}{0.116109814536}{0.333834409206}
\end{pgfscope}


==> nodal_square_D0.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{168,0,57}{0.766609825226}{0.766719269677}{0.765487174969}{0.765083203449}
  \meshline{168,0,57}{0.811561312743}{0.811847460615}{0.817377223827}{0.817113592207}
  \meshline{168,0,57}{0.715728308765}{0.715698518681}{0.716141134529}{0.716011104163}
  \meshline{168,0,57}{0.500059391378}{0.499926183663}{0.500215797441}{0.500081571663}
  \meshline{168,0,57}{0.499830569470}{0.499696007625}{0.500059391378}{0.499926183663}
  \meshline{168,0,57}{0.500215797441}{0.500081571663}{0.512008328330}{0.511859558422}
  \meshline{168,0,57}{0.469489977260}{0.469334102079}{0.477577410141}{0.477540327599}
  \meshline{168,0,57}{0.614988738888}{0.614858219794}{0.625580168160}{0.625364963034}
  \meshline{168,0,57}{0.750011539563}{0.749869344678}{0.734190039262}{0.733672428821}
  \meshline{168,0,57}{0.625580168160}{0.625364963034}{0.627534649431}{0.627507799545}
  \meshline{168,0,57}{0.483983491996}{0.483821648628}{0.477577410141}{0.477540327599}
  \meshline{168,0,57}{0.542358587900}{0.542116469198}{0.545256458021}{0.545084752088}
  \meshline{168,0,57}{0.520729228102}{0.520676956588}{0.512008328330}{0.511859558422}
  \meshline{168,0,57}{0.520729228102}{0.520676956588}{0.527638275756}{0.527463574922}
  \meshline{168,0,57}{0.645131883304}{0.645014867648}{0.643736077182}{0.643498990912}
  \meshline{168,0,57}{0.670877244835}{0.670939275438}{0.672507937613}{0.672303126130}
  \meshline{168,0,57}{0.578532096436}{0.578369982653}{0.565346856883}{0.565108343188}
  \meshline{168,0,57}{0.609170827383}{0.609261224092}{0.614988738888}{0.614858219794}
  \meshline{168,0,57}{0.562396206545}{0.562343277455}{0.554671269625}{0.554593737447}
  \meshline{168,0,57}{0.545256458021}{0.545084752088}{0.554671269625}{0.554593737447}
  \meshline{168,0,57}{0.565346856883}{0.565108343188}{0.563511800729}{0.563360668561}
  \meshline{168,0,57}{0.562396206545}{0.562343277455}{0.563511800729}{0.563360668561}
  \meshline{168,0,57}{0.583761139096}{0.583722690058}{0.578532096436}{0.578369982653}
  \meshline{168,0,57}{0.586076847826}{0.585842589533}{0.583761139096}{0.583722690058}
  \meshline{168,0,57}{0.601448655556}{0.601179449863}{0.606577560777}{0.606376456299}
  \meshline{168,0,57}{0.542358587900}{0.542116469198}{0.527638275756}{0.527463574922}
  \meshline{168,0,57}{0.499830569470}{0.499696007625}{0.483983491996}{0.483821648628}
  \meshline{168,0,57}{0.450022759438}{0.449965808711}{0.465183500299}{0.464862491039}
  \meshline{168,0,57}{0.422190506602}{0.422029492598}{0.418406111329}{0.418462699013}
  \meshline{168,0,57}{0.449497505555}{0.449394594287}{0.435811738236}{0.435612370145}
  \meshline{168,0,57}{0.465183500299}{0.464862491039}{0.469489977260}{0.469334102079}
  \meshline{168,0,57}{0.450022759438}{0.449965808711}{0.449497505555}{0.449394594287}
  \meshline{168,0,57}{0.657125013635}{0.657140863030}{0.670877244835}{0.670939275438}
  \meshline{168,0,57}{0.594903846659}{0.594893911620}{0.586076847826}{0.585842589533}
  \meshline{168,0,57}{0.606577560777}{0.606376456299}{0.609170827383}{0.609261224092}
  \meshline{168,0,57}{0.601448655556}{0.601179449863}{0.594903846659}{0.594893911620}
  \meshline{168,0,57}{0.431463379672}{0.431144327357}{0.434873806285}{0.434568335471}
  \meshline{168,0,57}{0.643736077182}{0.643498990912}{0.643374614428}{0.643087626534}
  \meshline{168,0,57}{0.685941002613}{0.686025497395}{0.674096551918}{0.673650793213}
  \meshline{168,0,57}{0.699596051009}{0.699504289321}{0.701870228021}{0.701382662435}
  \meshline{168,0,57}{0.701870228021}{0.701382662435}{0.715728308765}{0.715698518681}
  \meshline{168,0,57}{0.672507937613}{0.672303126130}{0.674096551918}{0.673650793213}
  \meshline{168,0,57}{0.645131883304}{0.645014867648}{0.657125013635}{0.657140863030}
  \meshline{168,0,57}{0.699596051009}{0.699504289321}{0.685941002613}{0.686025497395}
  \meshline{168,0,57}{0.730883454954}{0.731220400867}{0.734190039262}{0.733672428821}
  \meshline{168,0,57}{0.716141134529}{0.716011104163}{0.730883454954}{0.731220400867}
  \meshline{168,0,57}{0.629184251290}{0.629374965603}{0.643374614428}{0.643087626534}
  \meshline{168,0,57}{0.750011539563}{0.749869344678}{0.750096654453}{0.749928539738}
  \meshline{168,0,57}{0.793433417746}{0.794441094393}{0.799542464467}{0.799046507543}
  \meshline{168,0,57}{0.828351943797}{0.828848662385}{0.820381179772}{0.819728021023}
  \meshline{168,0,57}{0.793433417746}{0.794441094393}{0.783615233408}{0.783128859135}
  \meshline{168,0,57}{0.629184251290}{0.629374965603}{0.627534649431}{0.627507799545}
  \meshline{168,0,57}{0.751017583064}{0.750820719094}{0.765487174969}{0.765083203449}
  \meshline{168,0,57}{0.750096654453}{0.749928539738}{0.751017583064}{0.750820719094}
  \meshline{168,0,57}{0.769921888233}{0.770342774154}{0.783615233408}{0.783128859135}
  \meshline{168,0,57}{0.769921888233}{0.770342774154}{0.766609825226}{0.766719269677}
  \meshline{168,0,57}{0.799542464467}{0.799046507543}{0.804976133525}{0.804518908186}
  \meshline{168,0,57}{0.857063280601}{0.857601759821}{0.862370656647}{0.860625804034}
  \meshline{168,0,57}{0.841020715546}{0.841318864354}{0.842555608812}{0.842585233948}
  \meshline{168,0,57}{0.811561312743}{0.811847460615}{0.804976133525}{0.804518908186}
  \meshline{168,0,57}{0.828351943797}{0.828848662385}{0.841020715546}{0.841318864354}
  \meshline{168,0,57}{0.817377223827}{0.817113592207}{0.820381179772}{0.819728021023}
  \meshline{168,0,57}{0.857063280601}{0.857601759821}{0.844224974563}{0.843682472698}
  \meshline{168,0,57}{0.917495565553}{0.916651754615}{0.931123089864}{0.928938747733}
  \meshline{168,0,57}{0.874270378581}{0.873944158374}{0.873351085512}{0.872864304310}
  \meshline{168,0,57}{0.842555608812}{0.842585233948}{0.844224974563}{0.843682472698}
  \meshline{168,0,57}{0.874558395490}{0.874448209281}{0.885094498732}{0.884503573969}
  \meshline{168,0,57}{0.903261055492}{0.901115208004}{0.890306662389}{0.889239210760}
  \meshline{168,0,57}{0.431463379672}{0.431144327357}{0.422190506602}{0.422029492598}
  \meshline{168,0,57}{0.905426690457}{0.906036744672}{0.911559266220}{0.913210181082}
  \meshline{168,0,57}{0.885094498732}{0.884503573969}{0.889260232930}{0.888448366111}
  \meshline{168,0,57}{0.889260232930}{0.888448366111}{0.889545385044}{0.888573268461}
  \meshline{168,0,57}{0.874558395490}{0.874448209281}{0.874270378581}{0.873944158374}
  \meshline{168,0,57}{0.862370656647}{0.860625804034}{0.873351085512}{0.872864304310}
  \meshline{168,0,57}{0.931123089864}{0.928938747733}{0.932826545972}{0.932436835201}
  \meshline{168,0,57}{0.932826545972}{0.932436835201}{0.935918079419}{0.937375137527}
  \meshline{168,0,57}{0.889545385044}{0.888573268461}{0.890306662389}{0.889239210760}
  \meshline{168,0,57}{0.917495565553}{0.916651754615}{0.911559266220}{0.913210181082}
  \meshline{168,0,57}{0.905426690457}{0.906036744672}{0.903261055492}{0.901115208004}
  \meshline{168,0,57}{0.959097732307}{0.953490055957}{0.949091316124}{0.944261307322}
  \meshline{168,0,57}{0.935918079419}{0.937375137527}{0.949091316124}{0.944261307322}
  \meshline{168,0,57}{0.409797321615}{0.409533693369}{0.400519791511}{0.400434866628}
  \meshline{168,0,57}{0.959533032445}{0.958068003519}{0.976625873627}{0.976254430141}
  \meshline{168,0,57}{0.400519791511}{0.400434866628}{0.399304523145}{0.399079222174}
  \meshline{168,0,57}{0.434873806285}{0.434568335471}{0.435811738236}{0.435612370145}
  \meshline{168,0,57}{0.409797321615}{0.409533693369}{0.418406111329}{0.418462699013}
  \meshline{168,0,57}{0.384766718635}{0.384422023650}{0.379818287901}{0.379620774345}
  \meshline{168,0,57}{0.977232699558}{0.976314124248}{1.000000000000}{0.968750000000}
  \meshline{168,0,57}{0.959097732307}{0.953490055957}{0.959533032445}{0.958068003519}
  \meshtriangle{168,0,57}{0.984375000000}{1.000000000000}{1.000000000000}{0.984375000000}{1.000000000000}{1.000000000000}
  \meshline{168,0,57}{0.976625873627}{0.976254430141}{0.977232699558}{0.976314124248}
  \meshline{168,0,57}{1.000000000000}{0.984375000000}{0.984375000000}{1.000000000000}
  \meshline{168,0,57}{0.389570475442}{0.389732006058}{0.399304523145}{0.399079222174}
  \meshline{168,0,57}{0.370683619952}{0.370889564112}{0.364740414623}{0.364524301278}
  \meshline{168,0,57}{0.370683619952}{0.370889564112}{0.379818287901}{0.379620774345}
  \meshline{168,0,57}{0.360004464447}{0.359454755023}{0.364740414623}{0.364524301278}
  \meshline{168,0,57}{0.389570475442}{0.389732006058}{0.384766718635}{0.384422023650}
  \meshline{168,0,57}{0.342979958931}{0.342465443733}{0.352421322429}{0.352624414490}
  \meshline{168,0,57}{0.317335155940}{0.316789608402}{0.329547036638}{0.328936138413}
  \meshline{168,0,57}{0.352421322429}{0.352624414490}{0.360004464447}{0.359454755023}
  \meshline{168,0,57}{0.329547036638}{0.328936138413}{0.337648423456}{0.337924929396}
  \meshline{168,0,57}{0.277553543353}{0.277310357551}{0.272409632420}{0.271518667716}
  \meshline{168,0,57}{0.313999129322}{0.313919283173}{0.311816515898}{0.312093393489}
  \meshline{168,0,57}{0.342979958931}{0.342465443733}{0.337648423456}{0.337924929396}
  \meshline{168,0,57}{0.317335155940}{0.316789608402}{0.313999129322}{0.313919283173}
  \meshline{168,0,57}{0.303795868766}{0.302963150139}{0.311816515898}{0.312093393489}
  \meshline{168,0,57}{0.272409632420}{0.271518667716}{0.262960920562}{0.263326661908}
  \meshline{168,0,57}{0.277553543353}{0.277310357551}{0.284693722820}{0.284943633210}
  \meshline{168,0,57}{0.303795868766}{0.302963150139}{0.297279202012}{0.297201326937}
  \meshline{168,0,57}{0.072933855978}{0.072636872371}{0.065074175388}{0.062006735839}
  \meshline{168,0,57}{0.297279202012}{0.297201326937}{0.290744431929}{0.290196935213}
  \meshline{168,0,57}{0.245308335227}{0.245366411545}{0.244383440560}{0.244015649387}
  \meshline{168,0,57}{0.284693722820}{0.284943633210}{0.290744431929}{0.290196935213}
  \meshline{168,0,57}{0.241521070379}{0.241080373135}{0.244383440560}{0.244015649387}
  \meshline{168,0,57}{0.256213119315}{0.256141135092}{0.256408923426}{0.256388024322}
  \meshline{168,0,57}{0.256408923426}{0.256388024322}{0.262960920562}{0.263326661908}
  \meshline{168,0,57}{0.222221997035}{0.222212810383}{0.226597543256}{0.226924700876}
  \meshline{168,0,57}{0.256213119315}{0.256141135092}{0.245308335227}{0.245366411545}
  \meshline{168,0,57}{0.241521070379}{0.241080373135}{0.234904311951}{0.234167837132}
  \meshline{168,0,57}{0.208658844505}{0.208202416016}{0.222221997035}{0.222212810383}
  \meshline{168,0,57}{0.169962247434}{0.169407806146}{0.170471566530}{0.169892344526}
  \meshline{168,0,57}{0.234904311951}{0.234167837132}{0.226597543256}{0.226924700876}
  \meshline{168,0,57}{0.208658844505}{0.208202416016}{0.203729745006}{0.203505056606}
  \meshtriangle{168,0,57}{1.000000000000}{0.000000000000}{1.000000000000}{0.015625000000}{0.984375000000}{0.000000000000}
  \meshline{168,0,57}{0.984375000000}{0.000000000000}{1.000000000000}{0.015625000000}
  \meshline{168,0,57}{0.150920388483}{0.149546870690}{0.133451497070}{0.133820562682}
  \meshline{168,0,57}{0.132630672136}{0.132659814665}{0.131947112448}{0.131390818725}
  \meshline{168,0,57}{0.168070646960}{0.167794841035}{0.169550029692}{0.169159867307}
  \meshline{168,0,57}{0.168070646960}{0.167794841035}{0.154047376467}{0.154330596593}
  \meshline{168,0,57}{0.203729745006}{0.203505056606}{0.201955162367}{0.202070254971}
  \meshline{168,0,57}{0.192212857592}{0.191542260171}{0.201955162367}{0.202070254971}
  \meshline{168,0,57}{0.192212857592}{0.191542260171}{0.184835027792}{0.185471140167}
  \meshline{168,0,57}{0.169962247434}{0.169407806146}{0.169550029692}{0.169159867307}
  \meshline{168,0,57}{0.184835027792}{0.185471140167}{0.170471566530}{0.169892344526}
  \meshline{168,0,57}{0.122480328628}{0.122193410513}{0.118034152580}{0.118655550705}
  \meshline{168,0,57}{0.154047376467}{0.154330596593}{0.150920388483}{0.149546870690}
  \meshtriangle{168,0,57}{0.000000000000}{0.984375000000}{0.015625000000}{1.000000000000}{0.000000000000}{1.000000000000}
  \meshline{168,0,57}{0.015625000000}{1.000000000000}{0.000000000000}{0.984375000000}
  \meshline{168,0,57}{0.129152954581}{0.128616794947}{0.131947112448}{0.131390818725}
  \meshline{168,0,57}{0.132630672136}{0.132659814665}{0.133451497070}{0.133820562682}
  \meshline{168,0,57}{0.122480328628}{0.122193410513}{0.129152954581}{0.128616794947}
  \meshline{168,0,57}{0.088902147550}{0.087886173606}{0.098335167509}{0.097018265111}
  \meshline{168,0,57}{0.043432331451}{0.045080525912}{0.045067835127}{0.045292848198}
  \meshline{168,0,57}{0.015625000000}{0.000000000000}{0.022026220262}{0.028784720304}
  \meshline{168,0,57}{0.045067835127}{0.045292848198}{0.058755657999}{0.060204609572}
  \meshline{168,0,57}{0.065074175388}{0.062006735839}{0.058755657999}{0.060204609572}
  \meshline{168,0,57}{0.072933855978}{0.072636872371}{0.083508110909}{0.083715955801}
  \meshline{168,0,57}{0.118034152580}{0.118655550705}{0.111994932872}{0.110156517828}
  \meshline{168,0,57}{0.111994932872}{0.110156517828}{0.099281094043}{0.098957147047}
  \meshline{168,0,57}{0.029631657236}{0.029413473686}{0.043432331451}{0.045080525912}
  \meshline{168,0,57}{0.022026220262}{0.028784720304}{0.029631657236}{0.029413473686}
  \meshtriangle{168,0,57}{0.015625000000}{0.000000000000}{0.000000000000}{0.031250000000}{0.000000000000}{0.000000000000}
  \meshline{168,0,57}{0.088902147550}{0.087886173606}{0.085858977959}{0.085273563113}
  \meshline{168,0,57}{0.083508110909}{0.083715955801}{0.085858977959}{0.085273563113}
  \meshline{168,0,57}{0.099281094043}{0.098957147047}{0.098335167509}{0.097018265111}
  \meshline{168,0,57}{0.000000000000}{0.031250000000}{0.015625000000}{0.000000000000}
\end{pgfscope}


==> nodal_square_N.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{144,144,144}{0.879993636883}{0.413065250577}{0.910893362559}{0.422127786233}
  \meshline{144,144,144}{0.651777769638}{0.536099838225}{0.676779244494}{0.556962929083}
  \meshline{144,144,144}{0.299274159034}{0.700823502724}{0.307695519069}{0.709149275803}
  \meshline{144,144,144}{0.933953880556}{0.303157413992}{0.912910267084}{0.297594149116}
  \meshline{144,144,144}{0.572606008620}{0.356703190566}{0.572171121263}{0.356216472293}
  \meshline{144,144,144}{0.889426877916}{0.289197125204}{0.912910267084}{0.297594149116}
  \meshline{144,144,144}{0.946013200061}{0.428986799939}{0.937500000000}{0.428048367986}
  \meshline{144,144,144}{0.735235346218}{0.158537939892}{0.746374025021}{0.175189335622}
  \meshline{144,144,144}{0.792999219583}{0.372372320963}{0.795669390953}{0.373824220104}
  \meshline{144,144,144}{0.858919541756}{0.566525260589}{0.883753556477}{0.574797811042}
  \meshline{144,144,144}{0.946013200061}{0.428986799939}{0.995473582070}{0.432973582070}
  \meshline{144,144,144}{0.831252548334}{0.554717998370}{0.851812608291}{0.563144063854}
  \meshline{144,144,144}{0.735208721136}{0.500385636614}{0.760396901419}{0.516324539510}
  \meshline{144,144,144}{0.877161114951}{0.412176568365}{0.879993636883}{0.413065250577}
  \meshline{144,144,144}{0.740666600967}{0.606428035214}{0.743261711070}{0.608066747635}
  \meshline{144,144,144}{0.911467725011}{0.422277187820}{0.937500000000}{0.428048367986}
  \meshline{144,144,144}{0.911467725011}{0.422277187820}{0.910893362559}{0.422127786233}
  \meshline{144,144,144}{0.877161114951}{0.412176568365}{0.835798681569}{0.395258065009}
  \meshline{144,144,144}{0.824818736747}{0.551286546832}{0.789890186610}{0.533947313166}
  \meshline{144,144,144}{0.702675960782}{0.578354225279}{0.715144039504}{0.587520912314}
  \meshline{144,144,144}{0.700187855922}{0.475184939904}{0.683317681528}{0.461592664536}
  \meshline{144,144,144}{0.832313870882}{0.393766571834}{0.835798681569}{0.395258065009}
  \meshline{144,144,144}{0.769001372283}{0.521897877229}{0.789890186610}{0.533947313166}
  \meshline{144,144,144}{0.831252548334}{0.554717998370}{0.829069503102}{0.553572639749}
  \meshline{144,144,144}{0.671561995616}{0.452273673152}{0.639743034568}{0.424199445066}
  \meshline{144,144,144}{0.958110437767}{0.590605543661}{0.944680299659}{0.589283094610}
  \meshline{144,144,144}{0.886355361717}{0.575547236436}{0.910649437374}{0.582588836539}
  \meshline{144,144,144}{0.884139436048}{0.574935073892}{0.886355361717}{0.575547236436}
  \meshline{144,144,144}{0.910649437374}{0.582588836539}{0.916805198122}{0.583893780783}
  \meshline{144,144,144}{0.884139436048}{0.574935073892}{0.883753556477}{0.574797811042}
  \meshline{144,144,144}{0.790017043396}{0.370346424253}{0.792999219583}{0.372372320963}
  \meshline{144,144,144}{0.990245692230}{0.710492884585}{0.955294129582}{0.707253969326}
  \meshline{144,144,144}{0.864634231964}{0.679448861997}{0.863949123093}{0.679105906817}
  \meshline{144,144,144}{0.743261711070}{0.608066747635}{0.764147305203}{0.623313536202}
  \meshline{144,144,144}{0.876835441343}{0.283638580312}{0.883487779530}{0.286893208379}
  \meshline{144,144,144}{0.944680299659}{0.589283094610}{0.916805198122}{0.583893780783}
  \meshline{144,144,144}{0.851812608291}{0.563144063854}{0.858919541756}{0.566525260589}
  \meshline{144,144,144}{0.795669390953}{0.373824220104}{0.832313870882}{0.393766571834}
  \meshline{144,144,144}{0.764147305203}{0.623313536202}{0.780649349574}{0.633090800014}
  \meshline{144,144,144}{0.676779244494}{0.556962929083}{0.685050774643}{0.563539410763}
  \meshline{144,144,144}{0.760396901419}{0.516324539510}{0.763574143676}{0.518544003235}
  \meshline{144,144,144}{0.769001372283}{0.521897877229}{0.763574143676}{0.518544003235}
  \meshline{144,144,144}{0.780649349574}{0.633090800014}{0.802251541558}{0.647385639919}
  \meshline{144,144,144}{0.802251541558}{0.647385639919}{0.814615434531}{0.653908730803}
  \meshline{144,144,144}{0.740666600967}{0.606428035214}{0.738065842511}{0.604598478746}
  \meshline{144,144,144}{0.829069503102}{0.553572639749}{0.824818736747}{0.551286546832}
  \meshline{144,144,144}{0.738065842511}{0.604598478746}{0.715144039504}{0.587520912314}
  \meshline{144,144,144}{0.702675960782}{0.578354225279}{0.685050774643}{0.563539410763}
  \meshline{144,144,144}{0.509137126852}{0.621943514992}{0.511754502823}{0.624948527543}
  \meshline{144,144,144}{0.651777769638}{0.536099838225}{0.629296584929}{0.515949032268}
  \meshline{144,144,144}{0.671561995616}{0.452273673152}{0.683317681528}{0.461592664536}
  \meshline{144,144,144}{0.718694305621}{0.488596710948}{0.714388490310}{0.485285854971}
  \meshline{144,144,144}{0.623241790261}{0.510786504532}{0.618897375708}{0.506922363268}
  \meshline{144,144,144}{0.618897375708}{0.506922363268}{0.592677694050}{0.482419527112}
  \meshline{144,144,144}{0.550858314301}{0.441768526682}{0.558197596695}{0.449002423655}
  \meshline{144,144,144}{0.587493627204}{0.477622159483}{0.592677694050}{0.482419527112}
  \meshline{144,144,144}{0.623241790261}{0.510786504532}{0.629296584929}{0.515949032268}
  \meshline{144,144,144}{0.719904113660}{0.316991069580}{0.706764101615}{0.305562673990}
  \meshline{144,144,144}{0.587493627204}{0.477622159483}{0.574736813365}{0.465390499769}
  \meshline{144,144,144}{0.616348137823}{0.402252461197}{0.597572115018}{0.383543338309}
  \meshline{144,144,144}{0.457087617181}{0.678431828427}{0.436735731734}{0.653607206890}
  \meshline{144,144,144}{0.574736813365}{0.465390499769}{0.558197596695}{0.449002423655}
  \meshline{144,144,144}{0.573707421945}{0.357869159669}{0.572606008620}{0.356703190566}
  \meshline{144,144,144}{0.467861880005}{0.352462198681}{0.469294657824}{0.354223175797}
  \meshline{144,144,144}{0.513416202243}{0.402931222876}{0.522955795208}{0.413281092808}
  \meshline{144,144,144}{0.591127024484}{0.376909830180}{0.597572115018}{0.383543338309}
  \meshline{144,144,144}{0.639596885571}{0.424071202578}{0.639743034568}{0.424199445066}
  \meshline{144,144,144}{0.790017043396}{0.370346424253}{0.764666302003}{0.353956458710}
  \meshline{144,144,144}{0.354218341650}{0.469617142695}{0.368830096291}{0.482868418134}
  \meshline{144,144,144}{0.522955795208}{0.413281092808}{0.533111743984}{0.423789232540}
  \meshline{144,144,144}{0.619593838663}{0.405440701849}{0.616348137823}{0.402252461197}
  \meshline{144,144,144}{0.591127024484}{0.376909830180}{0.573707421945}{0.357869159669}
  \meshline{144,144,144}{0.639596885571}{0.424071202578}{0.619593838663}{0.405440701849}
  \meshline{144,144,144}{0.718694305621}{0.488596710948}{0.735208721136}{0.500385636614}
  \meshline{144,144,144}{0.700187855922}{0.475184939904}{0.714388490310}{0.485285854971}
  \meshline{144,144,144}{0.452066848077}{0.561452175349}{0.479940748237}{0.590370425316}
  \meshline{144,144,144}{0.430557140818}{0.540208539199}{0.427762834359}{0.537556070251}
  \meshline{144,144,144}{0.403702627860}{0.514312363650}{0.394119286811}{0.505455569582}
  \meshline{144,144,144}{0.533111743984}{0.423789232540}{0.550858314301}{0.441768526682}
  \meshline{144,144,144}{0.549841536208}{0.330582521609}{0.547168642259}{0.327324578529}
  \meshline{144,144,144}{0.492258508517}{0.380007595309}{0.485194876656}{0.372069603676}
  \meshline{144,144,144}{0.549841536208}{0.330582521609}{0.572171121263}{0.356216472293}
  \meshline{144,144,144}{0.479940748237}{0.590370425316}{0.482209685279}{0.592695025602}
  \meshline{144,144,144}{0.492469480427}{0.380228524723}{0.492258508517}{0.380007595309}
  \meshline{144,144,144}{0.492933202010}{0.380716559849}{0.492469480427}{0.380228524723}
  \meshline{144,144,144}{0.487766288625}{0.246402536383}{0.471417464422}{0.218705783739}
  \meshline{144,144,144}{0.453953732962}{0.186529132810}{0.466575637628}{0.210877708704}
  \meshline{144,144,144}{0.658093777065}{0.251488534590}{0.672765209788}{0.268952716493}
  \meshline{144,144,144}{0.764666302003}{0.353956458710}{0.756045317427}{0.347638532751}
  \meshline{144,144,144}{0.697563881707}{0.296109755177}{0.706764101615}{0.305562673990}
  \meshline{144,144,144}{0.658093777065}{0.251488534590}{0.644007265050}{0.232033904069}
  \meshline{144,144,144}{0.431891069842}{0.541548094117}{0.430557140818}{0.540208539199}
  \meshline{144,144,144}{0.469294657824}{0.354223175797}{0.485194876656}{0.372069603676}
  \meshline{144,144,144}{0.492933202010}{0.380716559849}{0.513416202243}{0.402931222876}
  \meshline{144,144,144}{0.412343650955}{0.284965162671}{0.417335327657}{0.291088752410}
  \meshline{144,144,144}{0.439813787404}{0.319572154168}{0.448804053535}{0.329850008526}
  \meshline{144,144,144}{0.448804053535}{0.329850008526}{0.467861880005}{0.352462198681}
  \meshline{144,144,144}{0.423230543710}{0.298075489327}{0.439813787404}{0.319572154168}
  \meshline{144,144,144}{0.471417464422}{0.218705783739}{0.466575637628}{0.210877708704}
  \meshline{144,144,144}{0.493098070402}{0.254825134855}{0.501445367151}{0.266395022276}
  \meshline{144,144,144}{0.412343650955}{0.284965162671}{0.393481866281}{0.258782101159}
  \meshline{144,144,144}{0.487766288625}{0.246402536383}{0.493098070402}{0.254825134855}
  \meshline{144,144,144}{0.531630301402}{0.308348560531}{0.547168642259}{0.327324578529}
  \meshline{144,144,144}{0.524195589181}{0.298121305340}{0.531630301402}{0.308348560531}
  \meshline{144,144,144}{0.501445367151}{0.266395022276}{0.513244315990}{0.283778610374}
  \meshline{144,144,144}{0.524195589181}{0.298121305340}{0.513244315990}{0.283778610374}
  \meshline{144,144,144}{0.577511738916}{0.086502002291}{0.574286282210}{0.072982926152}
  \meshline{144,144,144}{0.837085963478}{0.261910174770}{0.860824282729}{0.276086708779}
  \meshline{144,144,144}{0.625717191450}{0.203801945780}{0.608525501739}{0.171326580614}
  \meshline{144,144,144}{0.672765209788}{0.268952716493}{0.680123664132}{0.277710885552}
  \meshline{144,144,144}{0.509137126852}{0.621943514992}{0.492068782136}{0.603410399844}
  \meshline{144,144,144}{0.463742618720}{0.686153797365}{0.466722277643}{0.689871415029}
  \meshline{144,144,144}{0.427762834359}{0.537556070251}{0.403702627860}{0.514312363650}
  \meshline{144,144,144}{0.452066848077}{0.561452175349}{0.431891069842}{0.541548094117}
  \meshline{144,144,144}{0.269409162175}{0.401495517741}{0.269678943097}{0.401709162201}
  \meshline{144,144,144}{0.307329168474}{0.430501080501}{0.273918079807}{0.404964024128}
  \meshline{144,144,144}{0.381893007900}{0.494202143764}{0.394119286811}{0.505455569582}
  \meshline{144,144,144}{0.354218341650}{0.469617142695}{0.347280549288}{0.463457558035}
  \meshline{144,144,144}{0.156030815051}{0.440171342480}{0.159256336685}{0.441559591501}
  \meshline{144,144,144}{0.336296668199}{0.454437907877}{0.347280549288}{0.463457558035}
  \meshline{144,144,144}{0.309119034484}{0.431866262564}{0.307329168474}{0.430501080501}
  \meshline{144,144,144}{0.269678943097}{0.401709162201}{0.273918079807}{0.404964024128}
  \meshline{144,144,144}{0.417335327657}{0.291088752410}{0.423230543710}{0.298075489327}
  \meshline{144,144,144}{0.635765085462}{0.219113013988}{0.625717191450}{0.203801945780}
  \meshline{144,144,144}{0.591247419253}{0.131908315923}{0.603639423378}{0.161304605153}
  \meshline{144,144,144}{0.635765085462}{0.219113013988}{0.640618221387}{0.227060815723}
  \meshline{144,144,144}{0.247826377765}{0.488810442475}{0.269322963015}{0.503023110731}
  \meshline{144,144,144}{0.166486619203}{0.335598429594}{0.171759374195}{0.338710466272}
  \meshline{144,144,144}{0.269409162175}{0.401495517741}{0.240115815905}{0.380399095922}
  \meshline{144,144,144}{0.336296668199}{0.454437907877}{0.309119034484}{0.431866262564}
  \meshline{144,144,144}{0.449272252722}{0.177138784597}{0.451876076901}{0.182728579825}
  \meshline{144,144,144}{0.711080228156}{0.111457004235}{0.708456352984}{0.103618805819}
  \meshline{144,144,144}{0.708456352984}{0.103618805819}{0.699924564998}{0.079146390619}
  \meshline{144,144,144}{0.644007265050}{0.232033904069}{0.640618221387}{0.227060815723}
  \meshline{144,144,144}{0.605360685555}{0.165509867293}{0.608525501739}{0.171326580614}
  \meshline{144,144,144}{0.309348195729}{0.532270806906}{0.322752265039}{0.543456407466}
  \meshline{144,144,144}{0.381893007900}{0.494202143764}{0.368830096291}{0.482868418134}
  \meshline{144,144,144}{0.351438440709}{0.567550924051}{0.364855038619}{0.580064625153}
  \meshline{144,144,144}{0.296589969645}{0.522730542434}{0.275169121270}{0.507347903952}
  \meshline{144,144,144}{0.193419351229}{0.457401290210}{0.199320096759}{0.460923896159}
  \meshline{144,144,144}{0.367542800735}{0.221641169824}{0.373562232100}{0.230481680123}
  \meshline{144,144,144}{0.373562232100}{0.230481680123}{0.388603422767}{0.252595864711}
  \meshline{144,144,144}{0.393481866281}{0.258782101159}{0.388603422767}{0.252595864711}
  \meshline{144,144,144}{0.367542800735}{0.221641169824}{0.365646831765}{0.218135852550}
  \meshline{144,144,144}{0.453953732962}{0.186529132810}{0.451876076901}{0.182728579825}
  \meshline{144,144,144}{0.577511738916}{0.086502002291}{0.582564072930}{0.105893990946}
  \meshline{144,144,144}{0.603639423378}{0.161304605153}{0.604663134559}{0.163993233958}
  \meshline{144,144,144}{0.711080228156}{0.111457004235}{0.713183095185}{0.115919131115}
  \meshline{144,144,144}{0.269322963015}{0.503023110731}{0.272290091736}{0.505126972502}
  \meshline{144,144,144}{0.240712247162}{0.484262741449}{0.247826377765}{0.488810442475}
  \meshline{144,144,144}{0.574286282210}{0.072982926152}{0.570145345752}{0.045731414630}
  \meshline{144,144,144}{0.586296962857}{0.116575347207}{0.582564072930}{0.105893990946}
  \meshline{144,144,144}{0.586296962857}{0.116575347207}{0.591247419253}{0.131908315923}
  \meshline{144,144,144}{0.604663134559}{0.163993233958}{0.605360685555}{0.165509867293}
  \meshline{144,144,144}{0.275169121270}{0.507347903952}{0.272290091736}{0.505126972502}
  \meshline{144,144,144}{0.240712247162}{0.484262741449}{0.220817087565}{0.471976509826}
  \meshline{144,144,144}{0.220817087565}{0.471976509826}{0.199320096759}{0.460923896159}
  \meshline{144,144,144}{0.213586557907}{0.362885197321}{0.229798920299}{0.373404364913}
  \meshline{144,144,144}{0.568680891846}{0.035374631694}{0.567937457806}{0.013600518284}
  \meshline{144,144,144}{0.570145345752}{0.045731414630}{0.568680891846}{0.035374631694}
  \meshline{144,144,144}{0.567937457806}{0.013600518284}{0.567147628941}{0.000000000000}
  \meshline{144,144,144}{0.696529743484}{0.063632684046}{0.699924564998}{0.079146390619}
  \meshline{144,144,144}{0.689027533149}{0.000000000000}{0.689170721256}{0.002192955936}
  \meshline{144,144,144}{0.696529743484}{0.063632684046}{0.691505934841}{0.038035545021}
  \meshline{144,144,144}{0.240115815905}{0.380399095922}{0.229798920299}{0.373404364913}
  \meshline{144,144,144}{0.182253743746}{0.345188665291}{0.213586557907}{0.362885197321}
  \meshline{144,144,144}{0.105366374849}{0.308780143178}{0.114669753228}{0.312223608487}
  \meshline{144,144,144}{0.193419351229}{0.457401290210}{0.188187516134}{0.454587903295}
  \meshline{144,144,144}{0.307743300075}{0.104606755139}{0.319975857259}{0.134946972317}
  \meshline{144,144,144}{0.958110437767}{0.590605543661}{1.000000000000}{0.593479497782}
  \meshline{144,144,144}{0.837085963478}{0.261910174770}{0.829698713726}{0.257596812626}
  \meshline{144,144,144}{0.680123664132}{0.277710885552}{0.697563881707}{0.296109755177}
  \meshline{144,144,144}{0.756045317427}{0.347638532751}{0.745860760741}{0.339140828071}
  \meshline{144,144,144}{0.482209685279}{0.592695025602}{0.492068782136}{0.603410399844}
  \meshline{144,144,144}{0.573484447850}{0.697573635934}{0.563082790108}{0.685148455947}
  \meshline{144,144,144}{0.544726787559}{0.662746032296}{0.563082790108}{0.685148455947}
  \meshline{144,144,144}{0.525799466717}{0.640469736316}{0.537156808883}{0.653589711450}
  \meshline{144,144,144}{0.525799466717}{0.640469736316}{0.511754502823}{0.624948527543}
  \meshline{144,144,144}{0.537156808883}{0.653589711450}{0.544726787559}{0.662746032296}
  \meshline{144,144,144}{0.271923378229}{0.675357618189}{0.260969791789}{0.665656194955}
  \meshline{144,144,144}{0.188187516134}{0.454587903295}{0.159256336685}{0.441559591501}
  \meshline{144,144,144}{0.000854847916}{0.406809087711}{0.033582416208}{0.408151003541}
  \meshline{144,144,144}{0.082060423243}{0.416453812426}{0.095600720974}{0.419307127347}
  \meshline{144,144,144}{0.115901271769}{0.425189698014}{0.095600720974}{0.419307127347}
  \meshline{144,144,144}{0.156030815051}{0.440171342480}{0.125097815122}{0.428066986292}
  \meshline{144,144,144}{0.072457420870}{0.573990140710}{0.076985347596}{0.575196100984}
  \meshline{144,144,144}{0.868175806166}{0.145397204644}{0.846330054604}{0.121935126901}
  \meshline{144,144,144}{0.713183095185}{0.115919131115}{0.725400626887}{0.141950038861}
  \meshline{144,144,144}{0.725400626887}{0.141950038861}{0.735235346218}{0.158537939892}
  \meshline{144,144,144}{0.689170721256}{0.002192955936}{0.691505934841}{0.038035545021}
  \meshline{144,144,144}{0.138958311650}{0.322048694523}{0.114669753228}{0.312223608487}
  \meshline{144,144,144}{0.330236425800}{0.549648053797}{0.351438440709}{0.567550924051}
  \meshline{144,144,144}{0.309348195729}{0.532270806906}{0.296589969645}{0.522730542434}
  \meshline{144,144,144}{0.330236425800}{0.549648053797}{0.322752265039}{0.543456407466}
  \meshline{144,144,144}{0.390523638480}{0.605033194008}{0.414372713932}{0.628904683170}
  \meshline{144,144,144}{0.299274159034}{0.700823502724}{0.285140492020}{0.686890172894}
  \meshline{144,144,144}{0.373638265107}{0.587940611148}{0.379151803331}{0.593299038916}
  \meshline{144,144,144}{0.373638265107}{0.587940611148}{0.364855038619}{0.580064625153}
  \meshline{144,144,144}{0.285140492020}{0.686890172894}{0.271923378229}{0.675357618189}
  \meshline{144,144,144}{0.936789880937}{0.703703501795}{0.921428811248}{0.700044891802}
  \meshline{144,144,144}{0.835160134314}{0.665639642518}{0.814615434531}{0.653908730803}
  \meshline{144,144,144}{0.893107107009}{0.690850164828}{0.898426496952}{0.692292015402}
  \meshline{144,144,144}{0.835160134314}{0.665639642518}{0.862476084238}{0.678361908900}
  \meshline{144,144,144}{0.863949123093}{0.679105906817}{0.862476084238}{0.678361908900}
  \meshline{144,144,144}{0.864634231964}{0.679448861997}{0.870288132151}{0.681657424338}
  \meshline{144,144,144}{0.893107107009}{0.690850164828}{0.870288132151}{0.681657424338}
  \meshline{144,144,144}{0.921428811248}{0.700044891802}{0.898426496952}{0.692292015402}
  \meshline{144,144,144}{0.656757767359}{0.820129751037}{0.657910452648}{0.821806346978}
  \meshline{144,144,144}{0.936789880937}{0.703703501795}{0.955294129582}{0.707253969326}
  \meshline{144,144,144}{0.990245692230}{0.710492884585}{1.000000000000}{0.711187838001}
  \meshline{144,144,144}{0.776605552352}{0.212507619850}{0.779492088150}{0.215351356830}
  \meshline{144,144,144}{0.773493154097}{0.208902563284}{0.776605552352}{0.212507619850}
  \meshline{144,144,144}{0.779492088150}{0.215351356830}{0.797084174110}{0.232288984504}
  \meshline{144,144,144}{0.826289882966}{0.255309128741}{0.820648056940}{0.250818348317}
  \meshline{144,144,144}{0.797084174110}{0.232288984504}{0.820648056940}{0.250818348317}
  \meshline{144,144,144}{0.817119600900}{0.073643251286}{0.818644722907}{0.076615414446}
  \meshline{144,144,144}{0.846330054604}{0.121935126901}{0.840434084606}{0.114775629361}
  \meshline{144,144,144}{0.802964755656}{0.000000000000}{0.804002931626}{0.011790963149}
  \meshline{144,144,144}{0.818644722907}{0.076615414446}{0.840434084606}{0.114775629361}
  \meshline{144,144,144}{0.815905900809}{0.070180383977}{0.807171838112}{0.038247282862}
  \meshline{144,144,144}{0.868175806166}{0.145397204644}{0.893607674747}{0.165332105588}
  \meshline{144,144,144}{0.746374025021}{0.175189335622}{0.755941922245}{0.188401823630}
  \meshline{144,144,144}{0.773493154097}{0.208902563284}{0.755941922245}{0.188401823630}
  \meshline{144,144,144}{0.876835441343}{0.283638580312}{0.860824282729}{0.276086708779}
  \meshline{144,144,144}{0.817119600900}{0.073643251286}{0.815905900809}{0.070180383977}
  \meshline{144,144,144}{0.804002931626}{0.011790963149}{0.807171838112}{0.038247282862}
  \meshline{144,144,144}{0.883487779530}{0.286893208379}{0.889426877916}{0.289197125204}
  \meshline{144,144,144}{0.986171417816}{0.310032540010}{1.000000000000}{0.310765106521}
  \meshline{144,144,144}{0.829698713726}{0.257596812626}{0.826289882966}{0.255309128741}
  \meshline{144,144,144}{0.899733951240}{0.169420417684}{0.897306605751}{0.168031845604}
  \meshline{144,144,144}{0.968190239677}{0.309153172981}{0.965862987715}{0.308789678710}
  \meshline{144,144,144}{0.968190239677}{0.309153172981}{0.986171417816}{0.310032540010}
  \meshline{144,144,144}{0.933953880556}{0.303157413992}{0.965862987715}{0.308789678710}
  \meshline{144,144,144}{0.936331536770}{0.186400496927}{0.938402944987}{0.187060447011}
  \meshline{144,144,144}{0.897306605751}{0.168031845604}{0.893607674747}{0.165332105588}
  \meshline{144,144,144}{0.965428514369}{0.193536583702}{0.987451586073}{0.195992186048}
  \meshline{144,144,144}{0.965428514369}{0.193536583702}{0.938402944987}{0.187060447011}
  \meshline{144,144,144}{0.987451586073}{0.195992186048}{1.000000000000}{0.197013725887}
  \meshline{144,144,144}{0.899733951240}{0.169420417684}{0.920512464377}{0.179085990968}
  \meshline{144,144,144}{0.936331536770}{0.186400496927}{0.920512464377}{0.179085990968}
  \meshline{144,144,144}{0.745860760741}{0.339140828071}{0.733746451094}{0.329640758358}
  \meshline{144,144,144}{0.719904113660}{0.316991069580}{0.733746451094}{0.329640758358}
  \meshline{144,144,144}{0.484974851851}{0.714560653767}{0.491175053025}{0.722565037888}
  \meshline{144,144,144}{0.436735731734}{0.653607206890}{0.423474052323}{0.639060659688}
  \meshline{144,144,144}{0.346485492196}{0.754822290593}{0.342859983283}{0.750336246162}
  \meshline{144,144,144}{0.326648021446}{0.730195358220}{0.342859983283}{0.750336246162}
  \meshline{144,144,144}{0.390523638480}{0.605033194008}{0.379151803331}{0.593299038916}
  \meshline{144,144,144}{0.423474052323}{0.639060659688}{0.414372713932}{0.628904683170}
  \meshline{144,144,144}{0.457087617181}{0.678431828427}{0.463742618720}{0.686153797365}
  \meshline{144,144,144}{0.419920234017}{0.902042472208}{0.417397353605}{0.894050196321}
  \meshline{144,144,144}{0.484974851851}{0.714560653767}{0.466722277643}{0.689871415029}
  \meshline{144,144,144}{0.509550402998}{0.750068174674}{0.512387837520}{0.754028640881}
  \meshline{144,144,144}{0.509550402998}{0.750068174674}{0.491175053025}{0.722565037888}
  \meshline{144,144,144}{0.514833956384}{0.757876047070}{0.522983422071}{0.771943096572}
  \meshline{144,144,144}{0.512387837520}{0.754028640881}{0.514833956384}{0.757876047070}
  \meshline{144,144,144}{0.537545399404}{0.796813003951}{0.522983422071}{0.771943096572}
  \meshline{144,144,144}{0.688204735437}{0.886414916419}{0.682122775822}{0.872397025063}
  \meshline{144,144,144}{0.600596387307}{0.734138157428}{0.590545353698}{0.719543126615}
  \meshline{144,144,144}{0.573484447850}{0.697573635934}{0.576244887809}{0.700934112946}
  \meshline{144,144,144}{0.600596387307}{0.734138157428}{0.609554905157}{0.745567341127}
  \meshline{144,144,144}{0.626087945416}{0.769980605984}{0.627490743181}{0.771767599350}
  \meshline{144,144,144}{0.590545353698}{0.719543126615}{0.576244887809}{0.700934112946}
  \meshline{144,144,144}{0.537545399404}{0.796813003951}{0.541070112465}{0.804440017895}
  \meshline{144,144,144}{0.541070112465}{0.804440017895}{0.551976496881}{0.825930860107}
  \meshline{144,144,144}{0.657910452648}{0.821806346978}{0.659169992942}{0.823877971091}
  \meshline{144,144,144}{0.627490743181}{0.771767599350}{0.628754740418}{0.773518739886}
  \meshline{144,144,144}{0.626087945416}{0.769980605984}{0.609554905157}{0.745567341127}
  \meshline{144,144,144}{0.656757767359}{0.820129751037}{0.628754740418}{0.773518739886}
  \meshline{144,144,144}{0.674029562932}{0.853933912787}{0.659169992942}{0.823877971091}
  \meshline{144,144,144}{0.551976496881}{0.825930860107}{0.560987567715}{0.846212278946}
  \meshline{144,144,144}{0.571904603545}{0.876318175786}{0.572526683382}{0.878238478434}
  \meshline{144,144,144}{0.571214917459}{0.874545015689}{0.560987567715}{0.846212278946}
  \meshline{144,144,144}{0.581762271241}{0.908998675833}{0.578954078198}{0.896854343083}
  \meshline{144,144,144}{0.332206301617}{0.158462514784}{0.336244582032}{0.168540534652}
  \meshline{144,144,144}{0.432047449422}{0.135873466009}{0.427069958291}{0.123167427982}
  \meshline{144,144,144}{0.449272252722}{0.177138784597}{0.438862628182}{0.154860850640}
  \meshline{144,144,144}{0.332206301617}{0.158462514784}{0.319975857259}{0.134946972317}
  \meshline{144,144,144}{0.080574903640}{0.300474322168}{0.067728609780}{0.297112168036}
  \meshline{144,144,144}{0.365646831765}{0.218135852550}{0.351068616043}{0.194908595169}
  \meshline{144,144,144}{0.303347996372}{0.088735198062}{0.305413348012}{0.097747137063}
  \meshline{144,144,144}{0.336244582032}{0.168540534652}{0.339621060299}{0.175837693406}
  \meshline{144,144,144}{0.115901271769}{0.425189698014}{0.125097815122}{0.428066986292}
  \meshline{144,144,144}{0.082060423243}{0.416453812426}{0.066183556309}{0.412619426518}
  \meshline{144,144,144}{0.066183556309}{0.412619426518}{0.055140674421}{0.411103516703}
  \meshline{144,144,144}{0.000854847916}{0.406809087711}{0.000000000000}{0.406756951706}
  \meshline{144,144,144}{0.195551115072}{0.620860799246}{0.219313578776}{0.636332464788}
  \meshline{144,144,144}{0.138747457150}{0.593727585783}{0.141015446659}{0.594626782647}
  \meshline{144,144,144}{0.079221369476}{0.699675398316}{0.092739055764}{0.704292307480}
  \meshline{144,144,144}{0.231333238586}{0.797082431055}{0.254168761991}{0.824497075491}
  \meshline{144,144,144}{0.674029562932}{0.853933912787}{0.676107152596}{0.857812491960}
  \meshline{144,144,144}{0.676107152596}{0.857812491960}{0.682122775822}{0.872397025063}
  \meshline{144,144,144}{0.688204735437}{0.886414916419}{0.689669653242}{0.891344173615}
  \meshline{144,144,144}{0.708099674040}{0.964507262737}{0.709104084328}{0.979342732891}
  \meshline{144,144,144}{0.710861031248}{1.000000000000}{0.709104084328}{0.979342732891}
  \meshline{144,144,144}{0.708099674040}{0.964507262737}{0.703084115913}{0.938396155330}
  \meshline{144,144,144}{0.703084115913}{0.938396155330}{0.701631834033}{0.929594004190}
  \meshline{144,144,144}{0.689669653242}{0.891344173615}{0.701631834033}{0.929594004190}
  \meshline{144,144,144}{0.572526683382}{0.878238478434}{0.578954078198}{0.896854343083}
  \meshline{144,144,144}{0.593480382853}{1.000000000000}{0.593460236655}{0.999652838519}
  \meshline{144,144,144}{0.586097543842}{0.924955369922}{0.581762271241}{0.908998675833}
  \meshline{144,144,144}{0.588854717790}{0.941697203969}{0.590950041929}{0.955348926870}
  \meshline{144,144,144}{0.593460236655}{0.999652838519}{0.590950041929}{0.955348926870}
  \meshline{144,144,144}{0.571904603545}{0.876318175786}{0.571214917459}{0.874545015689}
  \meshline{144,144,144}{0.586097543842}{0.924955369922}{0.588854717790}{0.941697203969}
  \meshline{144,144,144}{0.432047449422}{0.135873466009}{0.438862628182}{0.154860850640}
  \meshline{144,144,144}{0.420884412392}{0.100999461200}{0.416738694795}{0.087668764384}
  \meshline{144,144,144}{0.411246357281}{0.058362307515}{0.411045925464}{0.055963268229}
  \meshline{144,144,144}{0.411247449909}{0.058369314476}{0.411246357281}{0.058362307515}
  \meshline{144,144,144}{0.420884412392}{0.100999461200}{0.427069958291}{0.123167427982}
  \meshline{144,144,144}{0.033582416208}{0.408151003541}{0.055140674421}{0.411103516703}
  \meshline{144,144,144}{0.031482402794}{0.291480321637}{0.031486255170}{0.291480813701}
  \meshline{144,144,144}{0.105366374849}{0.308780143178}{0.098446122217}{0.306950101417}
  \meshline{144,144,144}{0.000000000000}{0.289088185507}{0.031475044171}{0.291479982278}
  \meshline{144,144,144}{0.031486255170}{0.291480813701}{0.067728609780}{0.297112168036}
  \meshline{144,144,144}{0.129075499485}{0.590543744417}{0.138747457150}{0.593727585783}
  \meshline{144,144,144}{0.105410385525}{0.582161623032}{0.129075499485}{0.590543744417}
  \meshline{144,144,144}{0.044447711981}{0.570079508259}{0.068866716299}{0.573375755954}
  \meshline{144,144,144}{0.166010303705}{0.605552934796}{0.149638298559}{0.598570213398}
  \meshline{144,144,144}{0.027486765433}{0.568518990904}{0.000000000000}{0.566840319159}
  \meshline{144,144,144}{0.038339241700}{0.569098023586}{0.027486765433}{0.568518990904}
  \meshline{144,144,144}{0.141015446659}{0.594626782647}{0.149638298559}{0.598570213398}
  \meshline{144,144,144}{0.072457420870}{0.573990140710}{0.068866716299}{0.573375755954}
  \meshline{144,144,144}{0.177412807634}{0.611337481938}{0.195551115072}{0.620860799246}
  \meshline{144,144,144}{0.234365110608}{0.645682445057}{0.219313578776}{0.636332464788}
  \meshline{144,144,144}{0.092739055764}{0.704292307480}{0.111152975484}{0.710983793912}
  \meshline{144,144,144}{0.002341767859}{0.688914856826}{0.034309751201}{0.690863899700}
  \meshline{144,144,144}{0.038420242004}{0.806627507731}{0.062971167629}{0.813727340168}
  \meshline{144,144,144}{0.111152975484}{0.710983793912}{0.132469401761}{0.720366162657}
  \meshline{144,144,144}{0.132469401761}{0.720366162657}{0.141426027838}{0.725069228812}
  \meshline{144,144,144}{0.051448762877}{0.693701746757}{0.079221369476}{0.699675398316}
  \meshline{144,144,144}{0.193470992661}{0.759432304946}{0.220130059360}{0.783760733929}
  \meshline{144,144,144}{0.141426027838}{0.725069228812}{0.164606346014}{0.738778769382}
  \meshline{144,144,144}{0.002341767859}{0.688914856826}{0.000000000000}{0.688789724879}
  \meshline{144,144,144}{0.051448762877}{0.693701746757}{0.034309751201}{0.690863899700}
  \meshline{144,144,144}{0.038420242004}{0.806627507731}{0.010195330827}{0.803391360771}
  \meshline{144,144,144}{0.167123016411}{0.740324488218}{0.193470992661}{0.759432304946}
  \meshline{144,144,144}{0.164606346014}{0.738778769382}{0.166435454066}{0.739830825654}
  \meshline{144,144,144}{0.167123016411}{0.740324488218}{0.166435454066}{0.739830825654}
  \meshline{144,144,144}{0.010195330827}{0.803391360771}{0.000000000000}{0.802725921378}
  \meshline{144,144,144}{0.078921944462}{0.819708214222}{0.062971167629}{0.813727340168}
  \meshline{144,144,144}{0.078921944462}{0.819708214222}{0.109504189595}{0.836080069600}
  \meshline{144,144,144}{0.220995511601}{0.784580150111}{0.231333238586}{0.797082431055}
  \meshline{144,144,144}{0.220130059360}{0.783760733929}{0.220995511601}{0.784580150111}
  \meshline{144,144,144}{0.112688480011}{0.838322550611}{0.109504189595}{0.836080069600}
  \meshline{144,144,144}{0.254168761991}{0.824497075491}{0.256097024534}{0.827037101985}
  \meshline{144,144,144}{0.322747773872}{0.725967685306}{0.326648021446}{0.730195358220}
  \meshline{144,144,144}{0.290145399396}{0.891104126013}{0.293673725864}{0.901625543041}
  \meshline{144,144,144}{0.112688480011}{0.838322550611}{0.136125200228}{0.858597446491}
  \meshline{144,144,144}{0.156500000821}{0.882486664204}{0.170512165546}{0.902069827499}
  \meshline{144,144,144}{0.346485492196}{0.754822290593}{0.349695137776}{0.759537688990}
  \meshline{144,144,144}{0.382261971282}{0.810656723427}{0.367230649542}{0.784682000793}
  \meshline{144,144,144}{0.367230649542}{0.784682000793}{0.349695137776}{0.759537688990}
  \meshline{144,144,144}{0.322747773872}{0.725967685306}{0.307695519069}{0.709149275803}
  \meshline{144,144,144}{0.410799543752}{0.873102745038}{0.417397353605}{0.894050196321}
  \meshline{144,144,144}{0.404252923899}{0.856190261699}{0.396316095927}{0.837473085190}
  \meshline{144,144,144}{0.431729497928}{0.974298356033}{0.431259607503}{0.963688844539}
  \meshline{144,144,144}{0.382261971282}{0.810656723427}{0.382361407341}{0.810820429892}
  \meshline{144,144,144}{0.421464410152}{0.909440084296}{0.425584940678}{0.925328801617}
  \meshline{144,144,144}{0.382361407341}{0.810820429892}{0.382445655073}{0.810982591138}
  \meshline{144,144,144}{0.431066013688}{0.962254887080}{0.431259607503}{0.963688844539}
  \meshline{144,144,144}{0.279221101009}{0.866252752853}{0.276153033937}{0.860494116862}
  \meshline{144,144,144}{0.410799543752}{0.873102745038}{0.404252923899}{0.856190261699}
  \meshline{144,144,144}{0.425584940678}{0.925328801617}{0.427851556145}{0.936924768074}
  \meshline{144,144,144}{0.419920234017}{0.902042472208}{0.421464410152}{0.909440084296}
  \meshline{144,144,144}{0.396316095927}{0.837473085190}{0.382445655073}{0.810982591138}
  \meshline{144,144,144}{0.290145399396}{0.891104126013}{0.284907046980}{0.879413492760}
  \meshline{144,144,144}{0.276153033937}{0.860494116862}{0.261759407312}{0.836617416245}
  \meshline{144,144,144}{0.256097024534}{0.827037101985}{0.261759407312}{0.836617416245}
  \meshline{144,144,144}{0.299864689662}{0.920284147516}{0.293673725864}{0.901625543041}
  \meshline{144,144,144}{0.279221101009}{0.866252752853}{0.284907046980}{0.879413492760}
  \meshline{144,144,144}{0.243149338573}{0.652163100648}{0.260969791789}{0.665656194955}
  \meshline{144,144,144}{0.171759374195}{0.338710466272}{0.182253743746}{0.345188665291}
  \meshline{144,144,144}{0.351068616043}{0.194908595169}{0.339621060299}{0.175837693406}
  \meshline{144,144,144}{0.166486619203}{0.335598429594}{0.138958311650}{0.322048694523}
  \meshline{144,144,144}{0.291359227658}{0.031479941834}{0.288910486819}{0.000000000000}
  \meshline{144,144,144}{0.291950972260}{0.040828332015}{0.291359227658}{0.031479941834}
  \meshline{144,144,144}{0.291950972260}{0.040828332015}{0.293953469017}{0.051083300097}
  \meshline{144,144,144}{0.080574903640}{0.300474322168}{0.098446122217}{0.306950101417}
  \meshline{144,144,144}{0.293953469017}{0.051083300097}{0.303347996372}{0.088735198062}
  \meshline{144,144,144}{0.305413348012}{0.097747137063}{0.307743300075}{0.104606755139}
  \meshline{144,144,144}{0.416738694795}{0.087668764384}{0.411247449909}{0.058369314476}
  \meshline{144,144,144}{0.031482402794}{0.291480321637}{0.031475044171}{0.291479982278}
  \meshline{144,144,144}{0.105410385525}{0.582161623032}{0.076985347596}{0.575196100984}
  \meshline{144,144,144}{0.038339241700}{0.569098023586}{0.044447711981}{0.570079508259}
  \meshline{144,144,144}{0.166010303705}{0.605552934796}{0.177412807634}{0.611337481938}
  \meshline{144,144,144}{0.243149338573}{0.652163100648}{0.234365110608}{0.645682445057}
  \meshline{144,144,144}{0.195157452422}{0.971479213987}{0.195414327274}{0.974894023935}
  \meshline{144,144,144}{0.176734035284}{0.913773701331}{0.170512165546}{0.902069827499}
  \meshline{144,144,144}{0.136125200228}{0.858597446491}{0.146086122509}{0.868452042851}
  \meshline{144,144,144}{0.146086122509}{0.868452042851}{0.150602421913}{0.873882278038}
  \meshline{144,144,144}{0.181625258409}{0.926062476627}{0.176734035284}{0.913773701331}
  \meshline{144,144,144}{0.427851556145}{0.936924768074}{0.431066013688}{0.962254887080}
  \meshline{144,144,144}{0.308703775778}{0.962915583355}{0.310313852035}{0.991505677325}
  \meshline{144,144,144}{0.431729497928}{0.974298356033}{0.433170983692}{1.000000000000}
  \meshline{144,144,144}{0.304310040978}{0.940568763528}{0.299864689662}{0.920284147516}
  \meshline{144,144,144}{0.150602421913}{0.873882278038}{0.156500000821}{0.882486664204}
  \meshline{144,144,144}{0.195414327274}{0.974894023935}{0.196722019048}{1.000000000000}
  \meshline{144,144,144}{0.194347177573}{0.967948531674}{0.195157452422}{0.971479213987}
  \meshline{144,144,144}{0.194347177573}{0.967948531674}{0.188693275646}{0.945360884177}
  \meshline{144,144,144}{0.181625258409}{0.926062476627}{0.188693275646}{0.945360884177}
  \meshline{144,144,144}{0.307578615971}{0.954290366888}{0.304310040978}{0.940568763528}
  \meshline{144,144,144}{0.310877831452}{1.000000000000}{0.310313852035}{0.991505677325}
  \meshline{144,144,144}{0.307578615971}{0.954290366888}{0.308703775778}{0.962915583355}
  \meshline{144,144,144}{1.000000000000}{0.433282313220}{0.995473582070}{0.432973582070}
  \meshline{144,144,144}{0.411045925464}{0.055963268229}{0.406358827335}{0.000000000000}
\end{pgfscope}


==> nodal_square_N0.tex <==
\begin{pgfscope}
  % Written by OCaml Mesh.  width: 1, height: 1, xmin: 0, ymin: 0
  % \meshline{R,G,B}{x1}{y1}{x2}{y2}
  \providecommand{\meshline}[5]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfusepath{stroke}
    \end{pgfscope}}
  % \meshpoint{point number}{x}{y}
  \providecommand{\meshpoint}[3]{}
  % \meshtriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshtriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfilltriangle{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}
  \providecommand{\meshfilltriangle}[7]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfusepath{fill}
    \end{pgfscope}}
  % \meshfillquadrilateral{R,G,B}{x1}{y1}{x2}{y2}{x3}{y3}{x4}{y4}
  \providecommand{\meshfillquadrilateral}[9]{%
    \begin{pgfscope}
      \definecolor{ocamlmesh}{RGB}{#1}
      \pgfsetcolor{ocamlmesh}
      \pgfpathmoveto{\pgfpointxy{#2}{#3}}
      \pgfpathlineto{\pgfpointxy{#4}{#5}}
      \pgfpathlineto{\pgfpointxy{#6}{#7}}
      \pgfpathlineto{\pgfpointxy{#8}{#9}}
      \pgfusepath{fill}
    \end{pgfscope}}
  \meshline{168,0,57}{0.642397373507}{0.642801347347}{0.660717375378}{0.661385502756}
  \meshline{168,0,57}{0.727369748939}{0.727352852814}{0.749202226935}{0.749683533460}
  \meshline{168,0,57}{0.668848462814}{0.669398643348}{0.660717375378}{0.661385502756}
  \meshline{168,0,57}{0.589473260606}{0.589833518932}{0.568365464214}{0.568688615964}
  \meshline{168,0,57}{0.668848462814}{0.669398643348}{0.675875104206}{0.675878678176}
  \meshline{168,0,57}{0.749202226935}{0.749683533460}{0.749653284914}{0.750172254423}
  \meshline{168,0,57}{0.619720710947}{0.620204915261}{0.615394575602}{0.615587259959}
  \meshline{168,0,57}{0.675875104206}{0.675878678176}{0.688364918059}{0.689104400639}
  \meshline{168,0,57}{0.688364918059}{0.689104400639}{0.701991914486}{0.701979592636}
  \meshline{168,0,57}{0.619720710947}{0.620204915261}{0.642397373507}{0.642801347347}
  \meshline{168,0,57}{0.610084821172}{0.610077115831}{0.615394575602}{0.615587259959}
  \meshline{168,0,57}{0.610084821172}{0.610077115831}{0.589473260606}{0.589833518932}
  \meshline{168,0,57}{0.534462436467}{0.534710481103}{0.567988332079}{0.568303535385}
  \meshline{168,0,57}{0.568365464214}{0.568688615964}{0.568196958264}{0.568515764247}
  \meshline{168,0,57}{0.567988332079}{0.568303535385}{0.568196958264}{0.568515764247}
  \meshline{168,0,57}{0.534462436467}{0.534710481103}{0.527983280869}{0.528140260729}
  \meshline{168,0,57}{0.433728282728}{0.433988883059}{0.449267450866}{0.449451816983}
  \meshline{168,0,57}{0.499969628606}{0.500250772774}{0.527983280869}{0.528140260729}
  \meshline{168,0,57}{0.449267450866}{0.449451816983}{0.458000000412}{0.458276224454}
  \meshline{168,0,57}{0.469580170693}{0.469758913003}{0.499681310632}{0.499963091757}
  \meshline{168,0,57}{0.430174447655}{0.430501286690}{0.420818165049}{0.421152316003}
  \meshline{168,0,57}{0.397295640783}{0.397549048670}{0.399173165007}{0.399521668571}
  \meshline{168,0,57}{0.397295640783}{0.397549048670}{0.394583648480}{0.394663340824}
  \meshline{168,0,57}{0.399173165007}{0.399521668571}{0.420818165049}{0.421152316003}
  \meshline{168,0,57}{0.394583648480}{0.394663340824}{0.367645270762}{0.368143575389}
  \meshline{168,0,57}{0.469580170693}{0.469758913003}{0.458000000412}{0.458276224454}
  \meshline{168,0,57}{0.499969628606}{0.500250772774}{0.499681310632}{0.499963091757}
  \meshline{168,0,57}{0.353982488683}{0.353753544544}{0.367645270762}{0.368143575389}
  \meshline{168,0,57}{0.433728282728}{0.433988883059}{0.430174447655}{0.430501286690}
  \meshline{168,0,57}{0.353982488683}{0.353753544544}{0.340255313198}{0.340646284499}
  \meshline{168,0,57}{0.319524159304}{0.319840851893}{0.319194006019}{0.319548078010}
  \meshline{168,0,57}{0.319524159304}{0.319840851893}{0.340255313198}{0.340646284499}
  \meshline{168,0,57}{0.289014273193}{0.289226639734}{0.318822625671}{0.319206421702}
  \meshline{168,0,57}{0.271942141313}{0.272557856513}{0.289014273193}{0.289226639734}
  \meshline{168,0,57}{0.779777751207}{0.779760841149}{0.773053949801}{0.774066400577}
  \meshline{168,0,57}{0.773053949801}{0.774066400577}{0.750687832826}{0.751272288261}
  \meshline{168,0,57}{0.797689364561}{0.798780193267}{0.779777751207}{0.779760841149}
  \meshline{168,0,57}{0.701991914486}{0.701979592636}{0.712411896836}{0.713317675899}
  \meshline{168,0,57}{0.712411896836}{0.713317675899}{0.727369748939}{0.727352852814}
  \meshline{168,0,57}{0.750687832826}{0.751272288261}{0.749653284914}{0.750172254423}
  \meshline{168,0,57}{0.811423712053}{0.811049232620}{0.827431203246}{0.829341516024}
  \meshline{168,0,57}{0.871374856937}{0.870662708158}{0.853433893277}{0.855379346513}
  \meshline{168,0,57}{0.967017557293}{0.970077455748}{0.964604777683}{0.966375797754}
  \meshline{168,0,57}{0.803505815698}{0.803625974534}{0.811423712053}{0.811049232620}
  \meshline{168,0,57}{0.895280781835}{0.895014909511}{0.883364309674}{0.885475157153}
  \meshline{168,0,57}{0.941212302088}{0.944975871277}{0.915744382088}{0.916158534782}
  \meshline{168,0,57}{0.853433893277}{0.855379346513}{0.844618255728}{0.845003060258}
  \meshline{168,0,57}{0.206908203679}{0.208153879420}{0.200505794471}{0.201032678556}
  \meshline{168,0,57}{0.191293774220}{0.191119704906}{0.200505794471}{0.201032678556}
  \meshline{168,0,57}{0.318822625671}{0.319206421702}{0.319194006019}{0.319548078010}
  \meshline{168,0,57}{0.259341758507}{0.259923397415}{0.271942141313}{0.272557856513}
  \meshline{168,0,57}{0.253862847751}{0.253812467815}{0.259341758507}{0.259923397415}
  \meshline{168,0,57}{0.229409849998}{0.230321367848}{0.253862847751}{0.253812467815}
  \meshline{168,0,57}{0.179531156009}{0.180231746685}{0.191293774220}{0.191119704906}
  \meshline{168,0,57}{0.159832031434}{0.160227846052}{0.165497039135}{0.166521257689}
  \meshline{168,0,57}{0.152144317529}{0.151883529650}{0.137583529620}{0.137157181786}
  \meshline{168,0,57}{0.159832031434}{0.160227846052}{0.152144317529}{0.151883529650}
  \meshline{168,0,57}{0.107719641716}{0.108071470528}{0.131155404907}{0.132266110557}
  \meshline{168,0,57}{0.105740579039}{0.106746937429}{0.101124811035}{0.103001618325}
  \meshline{168,0,57}{0.105740579039}{0.106746937429}{0.107719641716}{0.108071470528}
  \meshline{168,0,57}{0.032187381404}{0.033771565314}{0.029960090867}{0.033109125093}
  \meshline{168,0,57}{0.032187381404}{0.033771565314}{0.058166502332}{0.057904441751}
  \meshline{168,0,57}{0.058166502332}{0.057904441751}{0.067905326380}{0.072530423076}
  \meshline{168,0,57}{0.000000000000}{0.003142001434}{0.029960090867}{0.033109125093}
  \meshline{168,0,57}{0.080713475440}{0.081154135303}{0.067905326380}{0.072530423076}
  \meshline{168,0,57}{0.179531156009}{0.180231746685}{0.165497039135}{0.166521257689}
  \meshline{168,0,57}{0.137583529620}{0.137157181786}{0.131155404907}{0.132266110557}
  \meshline{168,0,57}{0.229409849998}{0.230321367848}{0.206908203679}{0.208153879420}
  \meshline{168,0,57}{0.080713475440}{0.081154135303}{0.101124811035}{0.103001618325}
  \meshline{168,0,57}{0.871374856937}{0.870662708158}{0.883364309674}{0.885475157153}
  \meshline{168,0,57}{0.910094572043}{0.912438510120}{0.915744382088}{0.916158534782}
  \meshline{168,0,57}{0.895280781835}{0.895014909511}{0.910094572043}{0.912438510120}
  \meshline{168,0,57}{0.827431203246}{0.829341516024}{0.844618255728}{0.845003060258}
  \meshline{168,0,57}{0.803505815698}{0.803625974534}{0.797689364561}{0.798780193267}
  \meshline{168,0,57}{0.941212302088}{0.944975871277}{0.947127909017}{0.947926744767}
  \meshline{168,0,57}{0.981628000730}{0.987121999270}{0.994488214682}{1.000000000000}
  \meshline{168,0,57}{0.967017557293}{0.970077455748}{0.968578557834}{0.974665920968}
  \meshline{168,0,57}{0.981628000730}{0.987121999270}{0.968578557834}{0.974665920968}
  \meshline{168,0,57}{0.947127909017}{0.947926744767}{0.964604777683}{0.966375797754}
\end{pgfscope}

